On P vs. NP, Geometric Complexity Theory, and the Riemann Hypothesis

Geometric complexity theory (GCT) is an approach to the $P$ vs. $NP$ and related problems. A high level overview of this research plan and the results obtained so far was presented in a series of three lectures in the Institute of Advanced study, Princeton, Feb 9-11, 2009. This article contains the material covered in those lectures after some revision, and gives a mathematical overview of GCT. No background in algebraic geometry, representation theory or quantum groups is assumed.

==> abs_abstract.tex <==
\subsection*{Abstract}
Geometric complexity
theory (GCT) is an approach to the P vs. NP and related problems
suggested in the articles \cite{GCTpram}, henceforth referred to as 
GCTweak, \cite{GCT1}-\cite{GCT8}, henceforth
referred to as GCT1-8, and 
\cite{GCTflip}, henceforth referred to as GCTflip.
A high level overview of the basic plan of GCT was given in 
a series of three lectures in the Institute of Advanced study, Princeton,
Feb 9-11, 2009.  This article contains the material covered in the first of
those lectures after some revision, and gives a short  overview of GCT.
A full overview based on all  three lectures is available
separately  on the author's home page.
No background in algebraic geometry, representation theory
or quantum groups is assumed. 
The video lectures for this series are available at:

http://video.ias.edu/csdm/pvsnp

It may  help to go through these video lectures along with this article.




==> feasibility.tex <==
\section{Are nonelementary techniques necessary?: The feasibility barrier} 
Given the difficulty of  proving the positivity hypotheses (PH),
one can ask if  there is    a much easier elementary approach towards
the $P$ vs. $NP$ and related problems. 
In this section, we discuss the feasibilty barrier that
any approach towards these problems would have to cross,
and then point out why elementary techniques may not suffice to cross  
this barrier. 



It would be helpful to first review the development
of GCT  in this context. It  began with a  concrete
lower bound, namely, the special case of the $P \not = NC$ conjecture
 \cite{GCTpram}, which says that 
the $P$-complete max-flow problem
cannot be solved in $\polylog(N)$ parallel time using $\poly(N)$ 
processors in the PRAM model without bit operations, which
includes virtually all known parallel algorithms for algebraic 
and weighted optimization problems.  Here $N$ denotes
the total bit length of the input (not just the number of input parameters).
We shall refer to this result as 
{\em the characteristic zero (nonuniform) version of the $P$ vs. $NC$ problem},
though, unlike the characteristic zero versions of the $P$ vs. $NP$ and
$\#P$ vs. $NC$ problems, this one does address the issue of bitlengths.
Its  proof is
based on classical algebraic geometry, and as such, this may be regarded  
as  the first unconditional lower bound  to come out of GCT. 
Since it is a formal implication of the usual $P \not = NC$ conjecture 
(because the bitlengths are taken into account),
it can be stated in purely elementary, combinatorial terms. And yet, 
we do not have any  elementary combinatorial proof of  this result  so far. 

At present, this is the only analogue  of any of
the three fundamental lower bound 
problems in Figure~\ref{fig:complexityclasses}--namely, 
$P$ vs. $NP$, $\#P$ vs. $NC$ or $P$ vs. $NC$--that
we can prove unconditionally in a natural and realistic model of computation. 
Ultimately, any approach towards these  problems 
has to prove  some such 
natural and realistic analogue, though 
not necessarily this specific one, to demonstrate its effectiveness. 
That we cannot do so at present without algebraic 
geometry  seems to suggest that it may  be indipensible in their study. 

But classical algebraic geometry may not suffice 
in view of the  barrier towards these  problems 
pointed out  in \cite{GCTpram} (cf. its  last chapter). We shall
refer to it as the {\em algebraic degree barrier}, though it was not
given any name there. This  says that 
any low-degree proof technique, such as the one there,
which associates with a computation algebraic 
objects (polynomials, varieties, etc.) 
and then reasons solely on the basis of the degrees of those 
objects would not work.
The recent  algebrization barrier \cite{aaronson}
also says  something similar.

The article \cite{GCTpram} also suggested a plan  for bypassing the
algebraic degree barrier: namely, associate with the complexity classes 
algebraic varieties with group action, which   intuitively 
captures the symmetries of computation, and then reason on the basis of
the deeper representation theoretic structure of these
varieties, instead of just  their degrees.
This led to the construction of such varieties in \cite{GCT1}. 
The approach based on their analysis  (cf. GCT1, GCT2)
automatically bypasses the algebraic degree  barrier along with
the natural proof \cite{rudich} and relativization \cite{solovay} barriers
in characteristic zero (cf. \cite{GCTflip}). But that is
not enough. Because soon after GCT2, 
this approach ran into a really formidable barrier, namely the
feasibility ($P$) barrier (cf.  GCTflip1 and \cite{GCTbarriers}), which seems 
to be the main barrier towards  the $P$ vs. $NP$ and related problems.

Before we describe it, 
let us first explain why its presence should not be surprising.
For this, let us  observe that 
the earlier three barriers--algebraic-degree, natural proof 
and relativization--are all
{\em local} in the sense that
they apply to  specific subclasses (areas)  of mathematical techniques. 
They are more like {\em guiding posts},
rather than barriers in a strict sense,
which tell us which classes of techniques must be avoided.


But  the $P \not = NP$ conjecture  itself  is a {\em universal} statement
regarding all of mathematics. Namely, 
if this conjecture fails to hold,
every theorem in mathematics that has a proof of reasonable 
length  can be proved  effiiciently by a computer in 
time polynomial in the length of its shortest proof.
Given the universal nature of this problem, it then stands to reason that
the main  barrier towards this problem--the root cause of its 
difficulty--should also be
{\em universal}. By this, we mean that, unlike 
local barriers, such a barrier 
must be encountered by every
proof technique for the $P\not = NP$ conjecture 
regardless of which subarea of mathematical techniques it belongs to.

The {\em feasibility barrier} 
is  that universal complexity-theoretic barrier, which
every technique, not just GCT, has to deal with. Given its unversal
nature, it cannot be fully formalized. Not surprisingly,
because a barrier that can be fully formalized would tend to be 
local. 

To describe it, we need to 
first  reexamine the trivial, brute-force approach to 
the $\#P$ vs. $NC$ 
problem based on trivial obstructions (Figure~\ref{fig:trivial})
that we considered 
in Section~\ref{smeaning}, the argument for the $P$ vs. $NP$ problem
being similar. Certainly, this trivial approach is not really an approach
because it is just a restatement 
of the original    $\#P$ vs. $NC$ problem in the nonuniform setting. 
But let us analyze  what is wrong with it  from the
complexity theoretic perspective. An obvious shortcoming is that the 
the obstruction $O_n$ is very large, i.e. has exponential $2^{\poly(n)}$
size, and is  hard to verify, i.e., takes exponential $2^{\poly(n)}$
time to verify.
It is in this sense that this trivial approach can be called {\em infeasible}.

Any approach to the $\#P$ vs. $NC$ or the $P$ vs. $NP$ problem has to 
answer the following question: 

\begin{question} \label{qfeasible}
Why should the approach even be  feasible?
That is, in what sense is it fundamentally 
different from the  trivial, infeasible approach, and not just a restatement? 
\end{question}



Specifically, 
any approach to this  problem has to prove for every $n$
existence of some
cause $O_n$, which we shall call an {\em obstruction} as per that approach.
To answer the above question, the approach has to justify why 
the problem of proving existence of an obstruction (OH)  as per that 
approach should even be  feasible. For this, it has to do the following:

\begin{description} 
\item[I] Clearly formulate the notion of an obstruction (``proof-certificate''
of hardness) and the Obstruction Hypothesis (OH),
whose validity implies existence of such an obstruction, as in  GCT. 
\item[II] Clearly formulate the notion of feasibility, and justify 
why it is a reasonable  
notion; i.e., in what sense it is fundamentally
different from  a   brute-force search, just as the literature in 
complexity theory justifies polynomial-time as a reasonable theoretical notion
of feasibility. 
\item[III] Using this notion, show in what sense  the obstruction and 
the associated OH as per that approach 
are  fundamentally different (i.e. easier) 
from the trivial obstruction and the associated 
IOH (cf. (\ref{eqioh})) for the brute-force, infeasible   approach;
IOH for the $P$ vs. $NP$ is similar to (\ref{eqioh}).
\item[IV] 
Provide also some    mathematical evidence for the practical feasibility 
of OH in addition to just theoretical feasibility.
This is desirable since
theoretical feasibility (e.g. polynomial time) 
does not necessarily mean practical feasibility.
\end{description}

By the {\em feasibility barrier}, we mean the problem of answering 
Question~\ref{qfeasible} clearly in this fashion. It is universal in 
the sense that, for any approach to be considered nontrivial,
this question has to be answered. 
Until then,  however sophisticated the  approach 
may be, it cannot be considered to be more than 
a  restatement of the original lower bound statement.

We need to clarify what we mean by a restatement here. After all, OH 
as per any approach has to be a {\em logical (mathematical) restatement} 
in the sense 
that is should also be a tautology like the original IOH. What is meant
is that it should not be a {\em complexity-theoretic restatement}; i.e.,
it should be easier to verify than the original IOH in some definite 
sense--as per some complexity measure--as specified by  that approach. 

The most obvious  complexity measures are space and time. 
Hence a  natural way to cross the feasiblity barrier is by assigning 
the most obvious and natural complexity-theoretic meaning to the phrase 
feasible: namely,  ``short and easy to verify'', as suggested by the
$P$ vs. $NP$ problem itself. 

This leads to:
\begin{defn} 
A proof technique for the $\#P$ vs. $NC$ or the
$P$ vs. $NP$ problem in the nonuniform setting
is called  a {\em natural explicit proof technique} or simply 
a {\em natural proof technique}  if 
it shows existence of an
explicit family $\{O_n\}$ of {\em obstructions} to efficient computation 
of some function $f(x)=f(x_1,\ldots, x_n)$ in $\#P$ or $NP$ by circuits
of size $m=\poly(n)$ 
(also polylog depth in the case of $\#P$ vs. $NC$ problem), where
explicit means feasible; i.e.,  short and easy to verify. 
Specifically:
\begin{enumerate} 
\item Shortness:  $O_n$ has a specification of $\poly(n)$ size.
The $\poly(n)$ bound here should 
be independent of $m$ as long as $m$ is small enough, 
say $\le 2^{\polylog(n)}$. 

\item Ease of verification: 
Given $n$ and $m \le 2^{\polylog(n)}$, whether $O_n$ is an obstruction 
(as per that approach) 
for computation of $f(x_1,\ldots, x_n)$ by circuits of size $m$ can 
be verified in $O(\poly(n))$ time--this bound is independent of $m$ 
as long as $m$ is small enough as above.
\end{enumerate}

In other words, the problem of verification of OH as per the approach
belongs to $NP$
(it is assumed  here that the proof technique explicitly specifies OH). 
\end{defn}



We shall call any natural approach (proof strategy) to cross the feasibility 
barrier the {\em flip} (from the feasible to the infeasible). 
Here  we only assume that 
the approach strives to  prove existence of obstructions. In other words,
explicitness here
does not mean  that an explicit  $O_n$, for every $n$, can 
actually be constructed efficiently  (say, in $\poly(n)$ time);
if the approach also does that (optional), i.e. if $OH \in P$,
then  we call it strongly explicit.

\noindent {\em Remark 1:} The notion of a natural proof here is
different from the one 
in \cite{rudich},
which we shall refer to as  a {\em natural probabilistic   proof}
to avoid any confusion. Henceforth in this paper,
whenever we say a natural proof, we  always mean a natural explicit
proof, unless mentioned otherwise.

\noindent {\em Remark 2:} 
Explicit construction is not needed to 
bypass any of the local barriers; cf. \cite{GCT2append}.
For example, the local natural-probabilistic-proof barrier does not preclude 
nonconstructive proof techniques, such as  the ones in algebraic geometry 
surrounding the proof of the Riemann Hypothesis over finite fields 
\cite{weil2}, which are fundamentally different from the nonconstructive 
probabilistic techniques used in the proofs of lower bounds for 
constant-depth circuits, nor does it preclude nonexplicit (inefficient)
constructive techniques. Essentially all of algebraic geometry and 
respresentation theory consists of such nonconstructive or 
nonexplicit-constructive techniques outside the scope of that barrier
in a precise sense explained in  \cite{GCTappend}.


\noindent {\em Remark 3:}  However, going for explicit construction
does not mean that such nonconstructive techniques are of no use.
On the contrary (cf. Section~\ref{sphprove}) the proof of  correctness
of the explicit construction in GCT  would depend on PH, 
and the plan for proving 
Plethysm PH described in Figure~\ref{fig:lift} would need significant extension
of the nonconstructive proof techniques surronding the Riemann Hypothesis
over finite fields. In other words, nonconstructive techniques 
can  be   used to prove correctness of  
explicit (polynomial-time) verification/construction algorithms. 


The main result of GCT (cf. Theorems~\ref{tquasi} and \ref{tgct6}) 
in the  context of the  feasibility barrier  can be restated 
as follows:

\begin{theorem} 
The feasibility barrier can be crossed naturally in characteristic zero for
the $P$ vs. $NP$ and $\#P$ vs. $NC$ problems assuming the
mathematical positivity hypothesis PH1. That is, the complexity-theoretic
IOH (infeasible) can be reduced to the complexity-theoretic OH/POH  (feasible)
assuming the mathematical PH1/PH4.
\end{theorem}



As we saw above, the  mathematical 
positivity  may turn out to be  a  formidable issue.
This leads to an obvious question: 

\begin{question}
Are  such  mathematical positivity properties  really necessary to
prove the  $P \not =NP$ and related conjectures? 
\end{question} 

The existing mathematical evidence \cite{} suggests that any natural approach
to cross this barrier may  have to say  something deep regarding 
Plethysm PH  either explicitly or {\em implicitly}, even if
the approach does not utter a word about algebraic geometry or
representation theory.
That is,  Plethysm PH and PH0   may indeed be 
the heart of the  fundamental lower bound problems in complexity theory;
cf \cite{GCTbarriers} for a detailed story and a precise meaning of the key 
phrase {\em implicit}.

So if we wish to get around the  positivity issues in mathematics, 
we ought to look for unnatural approaches. This leads to the final
inevitable question: 

\begin{question} 
Are there unnatural  approaches to cross the feasibility 
barrier towards the $P$ vs. $NP$ and related problems? 
\end{question}

Quite possibly, yes, and presumably, several. But unfortunately
the mathematical and complexity theoretic evidence and arguments 
in \cite{} also suggest that unnatural proofs of the $P \not = NP$ 
and $\#P \not = NC$ conjectures may be  harder than natural proofs,
as one may intuitively expect. Specifically, \cite{} introduce a
theoretical measure of proof complexity called 
{\em explicit proof complexity}. It a measure of the mathematical diffculty
of proofs of  problems that  are naturally 
endowed with the notion of a ``proof-certificate'',
such as   the fundamental lower bound problems under consideration.
It also gives mathematical evidence towards its  practical value. Unnatural 
proofs would be harder than natural proofs as per this measure of
proof complexity, just as exponential-time algorithms are harder than
polynomial-time algorithms as per the worst-case  measure of time-complexity.



So unless there is a definite  unnatural approach towards
these  problems  supported 
by concrete mathematical support for the four steps (I)-(IV) above,
it may be best  to stick to the natural.




==> feasibility_barrier.tex <==
\section{Epilogue: the feasibility barrier}
Such a barrier should be expected because 
the $P \not = NP$ conjecture   is a {\em universal} statement
regarding all of mathematics: namely, 
if this conjecture fails to hold,
every theorem in mathematics that has a proof of reasonable 
length  can be proved  effiiciently by a computer in 
time polynomial in the length of its shortest proof.
Hence, 
given the universal nature of this problem, it then stands to reason that
the main  barrier towards this problem--the root cause of its 
difficulty--should also be {\em universal}.

And indeed,  there is such a universal barrier, which we shall
call the {\em feasibility barrier}. It is simply the 
the task of answering Question~\ref{}.
That is, answering why the given 
approach should even  be considered theoretically feasible, and not to be 
just a restatement of the original problem.
Until then,
however sophisticated the  approach 
may be, it cannot be considered to be more than 
a  restatement of the original lower bound statement.
We need to clarify  what we mean by a restatement here. After all, OH 
as per any approach has to be a {\em logical (mathematical) restatement} 
in the sense 
that is should also be a tautology like the original IOH. What is meant
is that it should not be a {\em complexity-theoretic restatement}; i.e.,
it should be theoretically easier to prove OH than
the original IOH as per some definite complexity measure 
 as specified by  the approach. 

Specifically, 
any approach to the $P$ vs. $NP$  problem has to prove for every $n$
existence of some
cause of hardness  $O_n$, 
which we shall call an {\em obstruction} as per that approach.
To answer Question~\ref{}, the approach has to justify why 
the problem of proving existence of an obstruction (OH)  as per that 
approach should  be  theoretically feasible.
For this, it has to do the following:

\begin{description} 
\item[I] Clearly formulate the notion of an obstruction (``proof-certificate''
of hardness) and the Obstruction Hypothesis (OH),
whose validity implies existence of such an obstruction.
\item[II] Clearly formulate the notion of {\em theoretical feasibility},
and justify 
why it is a reasonable  
notion; i.e., in what sense it means  something fundamentally
different from  a   brute-force search, just as the literature in 
complexity theory justifies polynomial-time as a reasonable  notion
of theoretical feasibility. 
\item[III] Using this notion, show in what sense the task of 
recognizing (verifying) an obstruction as per that approach should be
considered theoretically feasible. Because, if the approach 
cannot even recognize an obstruction effectively, how is it going to
prove its existence? 

\item [IV] Furthermore, using this notion, show in what sense
the task of proving existence of an  obstruction (OH) as per that 
approach--i.e. the discovery of an obstruction in that approach--is
theoretically feasible; 
i.e., fundamentally different from the brute-force
infeasible verification of IOH (\ref{}).
\end{description}

In addition, the approach should also 
provide  some    mathematical justification as to why proving  OH 
may plausibly become practically feasible once  
its theoretical feasibility is proven.
%This is desirable since
%theoretical feasibility (e.g. polynomial time) 
%does not automatically  mean practical feasibility.


By the {\em feasibility barrier}, we mean the problem of answering 
Question~\ref{qfeasible} clearly in this fashion. 


The most obvious and  natural way to cross the 
feasiblity barrier is by assigning 
the most obvious and natural complexity-theoretic meaning to the phrases
``theoretically feasible to verify'' and ``theoretically feasible to
discover'': namely, 
``short and easy to verify'' and ``easy to discover''  as suggested by the
$P$ vs. $NP$ problem itself.  This is the flip, the defining  strategy of GCT. 
The main result of GCT6,  mentioned above, says that 
the feasibility barrier can be crossed in characteristic zero via the flip
assuming  the posivitiy hypotheses PH1/4, 
as supported by  the mathematical evidence in GCT6,7,8.
But the difficulty  of proving these positivity hypotheses makes the 
task of implementing the flip difficult.
So the next question is: 

\begin{question} 
Are there  alternatives to  GCT, i.e., to its defining strategy--the flip?  
\end{question}

Quite possibly yes, and perhaps, several.
But the mathematical evidence and arguments 
in GCTflip suggest that the flip based on explicit constructions
may be among the easiest approaches 
to the $P$ vs. $NP$ and related problems, though certainly there is 
no reason to believe that this should be  the only approach.


==> flip.tex <==
\section{Preface}
Geometric complexity
theory (GCT) is an approach to the fundamental problems 
of complexity theory, such as $P$ vs. $NP$ \cite{cook,karp,levin}, 
$\#P$ vs. $NC$ \cite{valiant} and $P$ vs. $NC$ 
(Figure~\ref{fig:complexityclassesp}), 
suggested in the articles \cite{GCTpram}, henceforth referred to as 
GCTweak,  \cite{GCT1}-\cite{GCT8}, henceforth
referred to as GCT1-8, and 
\cite{GCTflip}, henceforth referred to as GCTflip.
A  high level overview of the basic plan of GCT was given in 
a series of three lectures in the Institute of Advanced study, Princeton,
Feb 9-11, 2009.  This article contains the material covered in
those lectures after some revision, and gives a mathematical  overview of GCT.
No background in algebraic geometry, representation theory
or quantum groups is assumed. 
A short overview based on the first lecture is available
separately on the author's home  page. 
The video lectures for this series are available at:

http://video.ias.edu/csdm/pvsnp

It may  help to go through these video lectures along with this article.

\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes}
      \label{fig:complexityclassesp}
\end{figure} 

In this preface, we give a nonmathematical overview of GCT.
Specifically, we wish to describe at a high level 
the main barrier  
towards the $P$ vs. $NP$ and related problems, called the {\em feasibility
barrier}, and the basic strategy of GCT for crossing it, called 
the {\em flip} [GCT6,GCTflip], and  the rationale behind this
strategy by giving a brief historical account of GCT's development
and its main results.
This barrier is {\em universal} in 
the sense that it has to be crossed by every approach towards the $P$ vs. 
$NP$ problem, not just GCT, regardless of which areas of mathematics it goes
through. In contrast, the other known barriers 
such as relativization \cite{solovay}, natural-proof \cite{rudich},
algebraic-degree [GCTweak],  algebrization  \cite{aaronson} barriers
are {\em local} in the
sense that they are only applicable to specific areas of mathematical
techniques and hence can simply be bypassed, as in GCT. 
In other words, a local barrier is like a guiding post which tells 
us what must not be done, and hence must  be bypassed,  whereas 
a universal barrier cannot be bypassed no matter what, because it tells us
what must be done, i.e., it has to be crossed.
Due its universality, the feasibility barrier
captures the root cause of all the 
difficulties in the $P$ vs. $NP$ and related  problems, and it turns 
out to quiet formidable, as expected. 
This barrier was not explicitly described  in 
the original lectures. But 
all the mathematical effort in   GCT as described in these lectures 
in a sense goes towards crossing this barrier.
Hence, we wish
to describe  it explicitly here and explain why its so  formidable, 
so that the fundamental difficulty that
GCT is trying to overcome,
and the need for the nonelementary techniques that enter into GCT to 
deal with it  would be clear at a high level before we 
get into any mathematics. 

Before we do so, let us  remark  that the 
presence of such a universal barrier should not be surprising,
because 
the $P \not = NP$ conjecture    is itself a {\em universal} statement
regarding all of mathematics. Namely, 
if this conjecture fails to hold,
every theorem in mathematics that has a proof of reasonable 
length  can be proved  efficiently by a computer in 
time polynomial in the length of its shortest proof. No other known
conjecture in mathematics has such stunning mathematical sweep. 
Given the universal nature of this problem, it then stands to reason that
the main  barrier towards this problem--the root cause of its 
difficulty--should also be
{\em universal}. The feasibility barrier is this universal barrier.
Due to its universal nature, it 
cannot be  fully formalized like the local barriers, because any barrier
that can be fully formalized would tend to be local. But since it is the 
root cause of the difficulty of the $P$ vs. $NP$ problem, 
we wish to  state it as clearly as possible. 

\ignore{Rather it is 
a philosophical barrier, and as such, the discussion in this preface 
is necessarily  somewhat philosophical. Readers not interested in 
such  discussion may wish to skip this preface, and proceed 
directly to the lectures. Some others may wish to read 
the first lecture, which gives a short mathematical overview of GCT,
first before reading
this preface. While some others may wish to read this first to get
an idea of the root difficulty that GCT is battling with and the
need for  nonelementary techniques that enter into it before 
getting into any mathematics. We will leave the exact choice to the
reader.}



\subsection{The feasibility barrier}
%Let us now describe the feasibility barrier.
Towards that end,  let us 
fix an appropriate $NP$-complete function $f(X)=f(x_1,\ldots,x_n)$. 
The goal of the nonuniform $P$ vs. $NP$ problem  is to show that 
there does not exist a circuit $C=C(X)$ of size 
$m=\poly(n)$ size that computes $f(X)$, $n\rightarrow \infty$. 
In symbols: 
\begin{equation} \label{eqiohp}
\forall n, m=\poly(n) \ \forall C \exists x : f(X)\not = f_C(X). 
\end{equation}

Equivalently, the goal is to prove:

\noindent {\bf (IOH)}: For every large enough $n$, and $m=\poly(n)$,
there  exists a {\em trivial obstruction
(i.e. a ``proof-certificate'' of hardness)} to efficient computation of
$f(X)$, namely, 
a table (cf. Figure~\ref{fig:trivialtonew}that lists for each $C$ as above a counterexample  $X$ so that
$f(X)\not = f_C(X)$, where $f_C(X)$ is the function computed by $C$.


The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$.
Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. 
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time to decide if such a table exists for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. So
we call  this trivial, brute force 
strategy of proving the nonuniform $P$ vs. $NP$ conjecture,
based on existence of trivial obstructions,  a {\em theoretically
infeasible strategy}. Also because
it is really just a restatement of the original problem.
Hence, the terminology  IOH (Infeasible Obstruction Hypothesis)--we also
call it {\em theoretically infeasible}. 


Any approach to the  $P$ vs. $NP$ problem has to 
answer the following question: 

\begin{question} \label{qfeasible} {\bf (Feasibility Barrier)} [GCTflip,GCT6]
Why should the approach be    feasible (i.e., lead to a proof) 
even theoretically?
That is, in what sense is it fundamentally 
different from the  trivial, infeasible approach above, 
and not just a restatement of the original problem? 
\end{question}

This question is fundamental  because,  in view of the universality 
of the $P \not =  $NP$ conjecture, it has always been questioned right from
the begining  why it
should even be provable. For example,  why can it not be 
independent of the formal axioms of mathematics? This was studied 
in some early works; cf. \cite{aaronsonformal} their  survey. It 
was also the 
motivation behind identifying  the fundamental 
barriers towards this problem,
such as the relativization \icte{}, natural-proof \cite{},
algebraic-degree [GCTweak] and algebrization  barriers \cite{}.
These barriers  roughly say that the proof techniques akin to
the ones used for proving the classical hierachy theorems,
the lower bounds for constant depth circuits,  the weaker form
of the $P\not = NC$ conjecture [GCTweak], and the $IP=PSPACE$ result  
would not work for the $P$ vs. $NP$ (and related) problems,
in a sense because the $P$ vs. $NP$ problem itself
stands in their way, rendering them theoretically infeasible, so to say.
Admittedly, such proof techniques constitute  only  very specific 
subareas of mathematics, which is why these  barriers can be considered 
local,  and we cannot conclude anything about the proof techniques
which go through other areas of mathematics on the basis of such local
barriers. But one can still wonder if the $P$ vs. $NP$ problem could not
stand in the way of every proof technique like this, rendering it
theoretically infeasible, and thereby precluding its own proof. This
does not seem inconceivable since the problem itself says that the discovery
is hard, and so, why could it not make the discovery of its own proof hard?
Hence arises the question:
why should a given proof technique 
be even theoretically feasible, as per some 
reasonable notion of theoretical feasibility. 
The feasibility barrier is simply the task of answering this 
fundamental question, which has been lurking in the background of the $P$ vs.
$NP$ problem right from the begining.
It is universal in the sense that every approach has to answer
Question~\ref{qfeasible}, and
until it is answered clearly,
however sophisticated an approach may be, it cannot be
considered to be more than a  restatement of the original problem.

Now we have specify what is meant by answering
Question~\ref{} clearly. For this,
the approach has to:
\begin{description}
\item[A] Come up with a new notion of obstruction (i.e. the cause
or proof-certificate of hardness as per that approach), which
is fundamentally different from the trivial obstruction, and thus 
precisely formulate the new Obstruction Hypothesis (OH), which says 
that such obstructions should exist when $m=\poly(n)$, and which provably 
implies the old IOH.

\item [B] Precisely formulate the notion of theoretical feasibility, 
and  justify why it is reasonable notion, i.e., why does a theoretically
feasible problem as per this notion means a problem that can be solved 
by a technique that is fundamentally better than the brute-force search, 
\item [C] 
Justify on the basis of  concrete mathematical results 
why the problem (OH) of proving existence of  such obstructions
should  be considered theoretically feasible as per this notion
in contrast to the theoretically infeasible IOH.
One possible way to do this is by justifying why that problem of 
recognizing (verifying) an obstruction is 
theoretically feasible as per this notion. After all,  every 
approach is in a sense a search for obstructions. It is possible 
that the approach may seek 
to prove existence of obstructions by a nonconstructive 
method, without exhibiting any obstruction explicitly. But if it is not
theoretically feasible for the approach to even recognize (verify) 
what is searching for,
then there is a serious problem.
\item [D] Justify why it is plausible
that the task of proving OH should
become practically feasible once its theoretical feasibility is established.
One possible way is to prove concrete nontrivial lower bounds 
in weaker settings using the approach to demonstrate that theoretical
feasibility can lead to practical feasiblity in nontrivial cases.
\end{description}
By the feasibility barrier, we will mean the task of answering Question~\ref{}
in this manner. \ignore{This question may seem very naive,
but  answering it satisfactorily 
turns out to be a formidable challenge. In fact, this   seems to be 
the main barrier towards the $P$ vs. $NP$ and related problems.}


\subsection{The flip}
The most obvious and natural strategy for crossing the feasibility barrier
is suggested by the $P$ vs. $NP$ problem itself. For that, 
let us see what is wrong with the trivial obstruction from the 
complexity-theoretic point view. That is quite clear. First, it is long,
i.e.,  its description takes exponential space. Second, it is hard to
verify (and also construct); i.e., this  takes exponential time.
Since $NP$ is the class of problems with ``proof-certificates'' that 
are short (of polynomial-size) and easy to verify (in polynomial-time), 
this then leads to the following stategy for proving the nonuniform
$P\not = NP$ conjecture, with the obvious complexity-theoretic
interpretation of the phrase theoretically feasible.


\noindent {\bf The flip  [GCT6,GCTflip]: Going for explicit construction}

\noindent {\bf I. (Theoretical feasibility of verification):}
Formulate a new notion of obstruction
(``proof-certificate of hardness'') that is {\em explicit}, by which 
we mean {\em short and easy-to-verify}: i.e., 
for any $n$ and $m< 2^n$, if there exists such an 
obstruction to efficient computation of $f(X)$ by circuits of size $m$,
then there also exists a short  obstruction with description of
$\poly(n)$ size bitlength, 
whose validity as an obstruction can be verified 
in $\poly(n)$ time.
This means that problem of verifying (recognizing)
an obstruction belongs to $P$, 
and hence, is theoretically feasible (``easy'').

Intuitively, we can think of the new obstruction as an 
encryption of a some trivial obstruction of exponential
size which is highly compressable
in the information theoretic sense--i.e., such that 
its description can be encrypted in polynomial size--and furthermore,
such that the encrypted information can also be verified fast in polynomial
time; cf. Figure~\ref{fig:trivialtonew}.
At the surface, it is hard to believe that 
such an obstruction can even exist. To see why, let us note that 
the problem of  verifying 
if a given $X$ is a counterexample is already intractable since 
it requires evaluating the NP-complete function $f(X)$, which cannot 
be evaluated  efficiently assuming $P \not = NP$, and furthermore
$f_C(X)$, which too cannot be evaluated  in polynomial time if the size $m$ of
$C$ is superpolynomial (say $n^{\log n}$). To verify the new obstruction,
in effect, we  are 
{\em implicitly} verifying   all exponentially many  rows of some 
trivial obstruction  in polynomial time (but without 
even knowing what that trivial obstruction is, since the verification 
procedure cannot affort to decrypt the new obstruction to get an exponential
size trivial obstruction).
It may seem that 
such a scheme could not possibly exist. 
The challenge in implementing this step of the flip
lies in  showing that such an unbelievable
obstruction actually exists.  Of course, the actual implementation 
does not have to  encrypt any trivial obstructions. The 
new obstruction could be such that its existence implies existence of
a trivial obstruction in a highly indirect way,
without actually telling how to get any
trivial obstruction from a new obstruction.




\begin{figure} 
\begin{center}
\epsfig{file=trivialtonew.eps, scale=.6}
\end{center}
      \caption{From trivial to new obstruction}
      \label{fig:trivialtonew}
\end{figure} 


\noindent {\bf II. (Theoretical feasibility of discovery) [optional]:} 
Give a $\poly(n)$  time algorithm for deciding,
for any given $n$ and $m< 2^n$,
if there exists such a new  obstruction, and constructing
one if one exists. This means the problem of discovering an obstruction
belongs to $P$, and hence, is theoretically feasible (``easy'').

\noindent {\bf III. (Practical feasibility):} 
Using the ``easy'' criterion for recognizing an obstruction 
in step I, prove:

\noindent {\bf OH (Obstruction Hypothesis):} If 
$m=\poly(n)$, then for sufficiently large $n$, there exists 
such an obstruction $O_n$. 

We call such an obstruction family $\{O_n\}$  {\em explicit};
as explained later (Section~\ref{}),  this is explicit 
in the same spirit  that the family of Ramanujan graphs (or rather their
labels) in \cite{} is explicit.

If we also have an ``easy'' procedure for discovering an obstruction 
in step II, then this amounts to  proving that this 
procedure always discovers and constructs
an obstruction $O_n$  successfully when $m=\poly(n)$--i.e., the discovery
procedure works correctly (successfully). So this step amount to 
proving correctness of the discovery program.
If it is, we 
call such an obstruction family $\{O_n\}$ {\em strongly explicit}.

We will call a proof of the $P\not = NP$ conjecture {\em explicit} if 
it is based on the flip and carries out the step I, and {\em strongly explicit}
if it carries out both steps I and II.


We shall say that OH is {\em theoretically feasible}, as against
theoretically infeasible IOH, 
once the steps I and II have been carried out, 
since the associated problems of verifying and constructing an obstruction 
then belong to $P$; i.e., 
the theoretically infeasible task of proving IOH is transformed 
into a theoretically feasible task of proving OH.
Hence, the name of this stategy {\em the flip}:
from the infeasible to the feasible. 
Another reason for this terminology is the following. 
The  problem of verifying IOH 
belongs to the complexity class $\Pi_3$, as is clear from its form
(\ref{eqiohp}), since the problem of verifying the condition
$f(X)\not = f_C(X)$ therein belongs to co-NP.
(Of course,  we expect IOH to be 
a tautology, and hence, $O(1)$-time verifiable eventually, 
but we do not know that as yet). 
In contrast,  the problem of verifying OH belongs to $NP$, once
the step I has been carried out, and to  $P$, once the step II has been
carried out. Thus the flip brings down the 
obstruction hypothesis from the infeasible region in the complexity 
hierarachy to the feasible region. 
And hence,  we will say that
the feasibility barrier is  crossed once steps I and II are  carried out.

The main question now is how to implement this flip, i.e., how to 
carry out the necessary explicit constructions. 
Though the strategy itself
is extremely simple, 
this  turns out to be a massive challenge
because of the counterintuitive nature of the flip
as explained in the step I. 
All the mathematical results of GCT together suggest that the flip
should  be possible, however counterintuitive it   may seem.
GCT suggests a strategy for implementing the flip for the $P$ 
vs. $NP$ and related problems, and 
proves two concrete lower bound results by implementing it in the
weaker settings.
Before we elaborate on these results, let us make  a few remarks.

\subsection*{Remarks}

\noindent (0) Theoretical feasibility is a meaningful issue  in the
context of the $P$ vs. $NP$ problem only because of its universality.
For  mathematical problems which are not universal, it  can be
meaningless. For example, consider 
the assertion: 

\[ \forall n \forall x_1,\ldots, x_n \exists k 
\forall y_1,\ldots, y_n > 0  ((\sum_i y_i)^{n-k}-1) (\prod_i x_i)= 0.
\] 
where $x_i$'s and $y_i$'s  are integer  variables. 
The problem of verifying this, as per the brute-force verification strategy, 
belongs to $\Pi_3$, and hence, we may call it theoretical infeasible,
and yet,  that makes no sense since this is clearly a trivial tautology (let 
$n=k$).
Thus theoretical infeasiblity/feasibility 
means nothing here. Indeed, it is well known
in proof theory that the logical complexity of an assertion, i.e., the
number of alternating quantifiers in it, is in general no index of its
mathematical difficulty. In the context of the $P$ vs. $NP$ problem it is. 
Because eliminating the quantifying variables in IOH,
which is what the nonuniform $P$ vs. $NP$ 
problem is all about, is extremely difficult because of its universality,
and hence, theoretical feasibility is a fundamental issue.

Theoretical feasibility is also a meaningful  issue in other 
fundamental problems of complexity theory,
such as the $P$ vs. $NC$ and $\#P$ vs. $NC$ problems. 
Because, though they are not universal, we simply think of them as brothers
and sisters of the $P$ vs. $NP$ problem.




\noindent (1)  Step II  has been labelled optional, because
there may exist a  proof of the $P\not = NP$ conjecture
along the  lines of the flip  that  takes substantial
short cuts in this step, though we do not know at present the nature of
such short cuts. 
For example,  a proof technique may simply get lucky and come 
up with a right guess for the obstruction family (since it is meant to be
carried out by humans and not machines). 
But substantial short cuts in step I seem difficult. After all, if the proof
technique cannot even recognize easily what it is searching for, then
there is  a serious problem.

\noindent {(2)} Theoretical 
feasibility of OH does not automatically  imply that the task of 
actually proving it would be practically feasible.
For that, it is also necessary
that the algorithms for verifying and discovering an obstruction in
steps I and II have a simple enough structure that can be used for
proving OH in step III; i.e.,  for proving correctness of the discovery 
procedure.
In other words, theoretically feasibility only
says that there is a good chance of practical
feasibility, just 
as the membership of a problem in $P$ does not automatically imply 
that it is practically feasible, but only says that there is a good
chance of it being practically feasible. The implementation scheme 
also has to prove some concrete 
lower bounds in weaker settings to justify that 
theoretical feasiblity can lead to practical feasibility;
cf. Sections~\ref{} and \ref{} for such lower bounds in GCT.




\noindent {(3)} 
The feasibility barriers and the 
flips for the other fundamental problems of complexity theory,
such as the $\#P$ vs. $NC$ and $P$ vs. $NC$ problems, 
are  similar. The flip is the defining strategy of GCT. That is,
we define GCT abstractly  as any (geometric\footnote{
We are putting geometric 
in  paranthesis here, because the results
of GCT, such as the weak form of the $P \not =NC$ conjecture 
proved in GCTweak and  discussed below, suggest  that 
geometry should  enter automatically
in any natural implementation of the flip,
if not explicitly, at least implicitly as a driving intuition.
So we do not look at  geometry as a defining feature, but rather 
as something  inevitable.})  approach to the $P$ vs. $NP$ and 
related problems based on the flip. 

\noindent (4) The flip is only the most obvious and natural way to cross
the feasibility barrier. But we are not saying that it is the only one.
There may exist  nonobvious and 
unnatural (e.g. nonconstructive) ways
to cross this barrier, perhaps several; cf. Section~\ref{} for more on this.
\ignore{At present,  we only know 
that one class of nonconstructive techniques 
would not work, namely the ones with probabilistic flavour, which
are ruled out by the natural-proof-barrier \cite{rudich}. 
But the probabilistic  proofs constitute  only a 
small subarea of nonconstructive proofs. Vast areas of
nonconstructive proofs in  mathematics, such as the ones  in algebraic 
geometry and representation theory, are of fundamentally different nature
than probabilistic proofs. The natural-proof-barrier does not apply to
such  nonconstructive techniques. Indeed, it is easy to show [GCTflip] 
that any proof technique that uses any representation-theoretic (symmetry)
property of the function $f(X)$ in any way
would automatically bypass the natural
proof barrier even if it is nonconstructive; cf. Remark~\ref{} for 
a precise statement. Further, GCT6 also proves 
a concrete lower bound (discussed below) using a nonconstructive 
technique,  which simultaneously crosses (in characteristic zero)
all the known local barriers (namely,
natural-proof, relativization, and algebraic-degree/algebrization,
or rather their appropriate analogues in characteristic zero)
ana also a weak  analogue of the feasibility barrier in that setting.
This says that nonexplicit or 
nonconstructive proof techniques can bypass  the 
the known local barriers, and  there is no reason to believe why
they cannot  cross the universal feasibility barrier as well.}

But the mathematical evidence given in [GCT6,GCTflip], some of which is
discussed below,  suggests that 
such unnatural ways may turn out to be much harder than the natural way,
as one may intuitively expect, and that the natural way may well
be among the easiest ways to cross the barrier. So unless there 
is a concrete unnatural approach
towards the $P$ vs. $NP$ and related problems--where by concrete, we mean: (1)
a concrete alternative definition of theoretical feadibility,
(2) a precise  definition of OH, and (3) concrete results 
that provide a good justification 
for its theoretical feasibility as per this notion--it may be best to stick
to the natural: the flip (GCT).

(5) The notion of a natural proof here is different from the one 
in \cite{}, to which will shall refer to as a {\em natural proabilistic proof}
to avoid any confusion. Henceforth, whenever we say natural we mean 
explicit.





\subsection{A weak form of the $P\not = NC$ conjecture}
A  weak form of the flip  for the $P$ vs. $NC$ problem was implemented 
in GCTweak, much before 
the flip was formalized in GCT6 and GCTflip. Specifically, 
GCTweak proves 
a special case of the $P \not = NC$ conjecture, which we shall call
its {\em weak form}, and which can be considered to be the
first concrete lower bound result of GCT. It  says that 
the $P$-complete max-flow problem
cannot be solved in $\polylog(N)$ parallel time using $\poly(N)$
processors in the PRAM model without bit operations,
which is quite realistic and natural
since it includes virtually all known parallel algorithms for algebraic 
and weighted optimization problems, and  
where $N$ denotes
the total bit length of the input, not just the number of input parameters.
The proof technique of this result can be considered to be a weak form
of the flip in the sense that  for each branching program $C$  (i.e. 
a circuit with arithmetic, branching and comparison operations) 
of depth $\log^a N$ and size $\poly(N)$, or even 
$2^{\log^a N}$, $a$ a positive constant, 
it produces an  explicit   counter example (i.e., a proof-certificate of
hardness) $X$ such that the output of $C$
on $X$ is different from what is expected in the maxflow (decision) problem.
Explicit in this context
means computable in $\log ^b N$ time using $2^{\log ^b N}$ 
processors, $b=O(a)$. 
This is weak in the sense that the obstruction here is   a proof 
certificate of hardness against a specific circuit  rather than the
whole class of circuits of small depth and size (which is far harder to
achieve), hence we shall call such proof certificates {\em weakly explicit}. 

\noindent Remark:
Weak explicitness was not  specifically mentioned 
in GCTweak. But it is easy to see, 
and as would be elaborated in the revised version of GCTflip,  that 
the proof technique there actually
produces a weakly 
explicit proof certificate of hardness, though the goal was only
to prove its existence (which is why explicitness was not mentioned).
In other words, the proof technique produces a weakly 
explicit proof-certificate of hardness  whether one cares for it or not.


Another notable feature of the proof technique in GCTweak is that it is 
intrinsically  geometric, being 
based on classical algebraic geometry, though 
the lower bound result itself can be stated in purely 
elementary and combinatorial terms, being a formal special case of the 
$P \not = NC$ conjecture. No elementary or combinatorial 
proof of this result 
is known so far, and also no proof, even nonelmentary, which
does not carry out any explicit construction. 
At present, this weak form of the $P\not = NC$ conjecture seems to be the
only known  special case of any
of the three fundamental lower bound problems in 
Figure~\ref{fig:complexityclassesp}--namely, the $P$ vs. $NP$,
$P$ vs. $NC$ or $\#P$ vs. $NC$ problems--that  holds unconditionally (and 
superpolynomially) in a realistic and 
natural model of computation. That its only known proof needs 
geometry and explicit construction   provides  a nontrivial support for the
geometric approach based  the flip (GCT), albeit only in the weak setting, and
hence, in retrospect, we shall refer to its proof technique as {\em weak GCT}.


\subsection{On the flip in general for characteristic zero}
But the  weak GCT turns out to be too weak to yield any result
in the context of 
the $\#P$ vs. $NC$ and $P$ vs. $NP$ problems. The later work in GCT--the 
subject of this overview--focusses on the characteristic zero versions of
these problems.  By the 
(nonuniform) characteristic zero version of the $\#P$ vs. $NC$ problem, we 
mean the  permanent vs. determinant problem \cite{valiant} in 
characteristic zero. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented 
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$.
 %; cf. Figure~\ref{fig:matrices}. 
By linear representation, we mean
the  entries   of $Y$ are  (possibly nonhomogeneous) 
linear functions 
of the entries of $X$. 
There is an analogous (nonuniform) characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.










The main result of GCT in this context [GCT6,7,8]
is a conjectural scheme for implementing the flip 
for the $\#P$ vs. $NC$ and $P$ vs. $NP$  problems 
in characteristic zero.
Specifically, GCT1 and 2 reduce these problems to showing 
nonexistence of embeddings among certain algebraic varieties associated 
with the complexity classes under consideration (e.g. 
$\#P$ and $NC$ in the first problem), and then 
define  a new (nontrivial) notion of obstruction,
which is a   representation-theoretic 
object  whose existence obstructs such embedding.
It is shown in GCT6 that the problem of verifying (the specification label of)
this obstruction (or rather its restricted form) belongs to $P$--i.e.,
the step I of the flip can be implemented--assuming 
certain positivity hypothesis called PH1.
This says that 
certain  representation-theoretic counting  functions
associated with the above algebraic varieties  have positive  convex formulae. 
By a positive  formula, we mean a $\#P$-formula, like the usual one
for the permanent, which does not have any alternating signs. (In contrast,
the usual formula for the determinant is not positive since it has
alternating signs). By a convex positive formula, we mean a positive convex
representation as the number of integer points in an explicitly 
specified polytope, like the one for the permanent of a $0-1$-matrix 
as the number of integer points in the perfect matching polytope--this
representation is both positive (since each integer point is counted 
with a positive sign) and convex. 
GCT6 also shows that the problem of discovering  (the specification label of)
such a (restricted)  obstruction  belongs to $P$--i.e. the step
II can also be implemented--assuming a positivity hypothesis PH4, which
is a stronger form of PH1.
Furthermore, GCT6,7,and 8   provide an evidence in support of validity
of PH1, PH4, and OH.
As far as the step III (practical feasibility of proving OH)
is concerned, nothing can be said at this
point, since its implementation would depend on explicit forms of
the polytopes in PH1 and PH4, which we do not know at present.

\subsection{The weak form of the generalized $\#P$ vs. $NC$ problem}
But GCT6 also proves a concrete lower bound--namely
a certain  weak form of the generalized 
$\#P \not = NC$ conjecture--using this flip strategy. The relevant positivity 
hypotheses and OH can be proven unconditionally in this weak setting. 

\noindent {\em Remark:} This lower bound 
is a generalization of the weak form of the
$\#P$ vs. $NC$ problem that was mentioned in the original IAS lectures,
and which, as it turns out \cite{boris}, has an elementary proof. 
But this generlization is much more nontrivial, and has 
no elementary proof, though its statement is again elementary; cf. 
Section~\ref{sweak} for its precise statement and a sketch of its proof. 

The proof of the weak form of the generalized $\#P \not = NC$ conjecture 
is helpful  in the context of the flip 
for two reasons. First, it suggests  that 
PH1 (and PH4) should be provable, if true (as suggested by the evidence 
in GCT6,7,8),  since its  weak form which arises  in this proof can be proved
unconditionally (it
turns out to be a classical result of representation theory). Second,
it suggests that once PH1 and PH4 are proved, proving OH can be
practically feasible if  the convex polytopes in PH1 and PH4 are
reasonably well bahaved, like the polytopes that arise in this proof;
i.e., there is a good chance that 
theoretical feasibility of OH after steps I and II 
can lead to its practical feasibility in step III.
Thus this lower bound provides a second concrete support for 
GCT/flip, in addition to the weak form of the
$P\not = NC$ conjecture mentioned before.

\subsection{How to prove positivity?}
Coming to back to general problem,  the next  main task now is to prove PH1.
GCT6,7,8  suggest  an approach for proving it via the theory of
nonstandard quantum groups, which are generalizations of
standard quantum groups \cite{drinfeld}. At the heart of this approach lie
certain conjectural positivity hypotheses [GCT8] in the theory
these nonstandard quantum groups, which are  generalizations of the
known positivity results \cite{kazhdan,lusztig} for the standard quantum group.
The only known proofs of these positivity results relie on the 
Riemann hypothesis over finite fields \cite{weil2}, which is
itself a profound  positivity result in mathematics. 
Thus the
implementation of the flip proposed in GCT6,7,8 
seems to need  as yet unknown nonstandard
extension of the work surrounding this central positivity theorem,
which encompasses several areas of 
of mathematics, such as algebraic geometry, representation theory,
quantum groups and so forth, and  a parallel nonstandard 
extension of complexity theory
to show that the relavant counting  functions in algebraic geometry
and representation theory belong to $\#P$  assuming such nonstandard 
mathematical extension.
When the underlying field of computation is finite (as in 
the usual case of the $P$ vs. $NP$ problem), it 
may need such nonstandard  extensions in several other fields as well--such as,
number theory, arithmetic algebraic geometry, automorphic  forms,
and so forth; cf. GCT11.

\subsection{Is there a simpler alternative to GCT?}
Given that GCT has turned out to be so challenging, one may then ask if 
there is a substantially simpler alternative to GCT. But as we mentioned
earlier,
the mathematical evidence in GCTflip suggests that the feasibility 
barrier is truly formidable, and however hard it may be to believe,
GCT/flip may be ``among the easiest'' ways to cross the this barrier;
for the precise meaning of the phrase ``among the easiest''
see GCTflip, and also Section~\ref{sposnece} 
for its brief discussion.
Thus reallistically, the feasibility barrier  may not be crossed 
without major extensions in 
several branches of mathematics and 
complexity theory as needed in GCT. 
This too should not be surprising 
in view of the   universality of the barrier and the $P$ vs. $NP$ problem.
Indeed, convergence of 
so many mathematical fields  in GCT should be 
taken as a testimony to the universality and 
grandeur of  the $P$ vs. $NP$ problem.

In summary, what has been done in GCT so far is only the easy initial
part--easy in comparison to what remains to be done--and the real
hard part (positivity) is yet to begin. And the hard part
seems so hard that any further progress on that may not be feasible 
without substantial interaction between mathematics, complexity theory,
and also theoretical physics 
(because of nonstandard quantum groups). 
It is our hope that this work is a small step in that direction.






The rest of this article is organized 
in the form of three chapters, one per lecture.
The first lecture gives an overview of the basic plan of implementing the
flip in GCT,  which
is elaborated in the subsequent two lectures.




\noindent {\em Acknowledgement:} The author is deeply grateful to 
Madhav Nori, his teacher and mentor in  mathematics, 
to Milind Sohoni and Hari Narayanan, who  collaborated in the crucial initial
papers GCT1-4 and 5,
which paved the way for the flip papers  GCTflip, GCT6,7, and  8, and to 
Avi Wigderson for arranging the lectures and the hospitality in IAS.



==> lecture.tex <==
\section{{\bf \LARGE Lecture 1 (Overview)}}

The goal of this lecture is to give a high level overview of 
geometric complexity theory (GCT), an 
approach towards the fundamental lower bounds in complexity theory; 
specifically
\ignore{The complexity classes that we are concerned with 
are the well known ones: $P$, the class of problems that can be solved 
in polynomial time,  $NP$, the class of problems whose solutions can be
verified in polynomial time,  $\#P$, the counting class
associated with $NP$,  and 
$NC$, the class of problems that can be solved 
in polylogarithmic time using polynomial number of processors.
The  fundamental lower bound problems that we are concerned with are:}

\noindent (1) 
The $P$ vs. $NP$ problem:  show that $P \not = NP$, and 

\noindent (2) 
The  $\#P$ vs. $NC$ problem: show that 
$\#P \not = NC$.

We shall be dealing with the  nonuniform versions of these problems 
in characteristic zero; i.e. , when
the underlying field of computation is of characteristic zero, 
say $\Q$ or $\C$. The problems that
need to be addressed to extend this approach to the usual forms of 
these problems, when the underlying field of computation is finite,
would be discussed in  GCT11. 

The nonuniform (characteristic zero) version of the $\#P$ vs. $NC$ problem
is also referred to as the permanent vs. determinant problem \cite{valiant}. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented 
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$; cf. Figure~\ref{fig:matrices}. 
By linear representation, we mean
the  entries  $y_{ij}$'s of $Y$ are affine (i.e., possibly nonhomogeneous) 
linear combinations 
of the entries $x_{lk}$'s of $X$. %; i.e., 
%\[ y_{i j} = \sum_{l,k\le n} a_{i,j}^{l,k} x_{l,k} + a_{i,j}^{n+1,n+1}, \]
%for some complex 
%$a_{i,j}^{l,k}$, $l,k \le n+1$, $i,j \le m$.
There is an analogous characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.


The main results of GCT hold for the characteristic zero versions 
of both of the problems above. But to keep the treatment simple, we shall 
only concentrate on the characteristic zero,  nonuniform
version of the $\#P$ vs. $NC$ problem, since this illustrates all the basic
ideas. 
In this lecture we shall give an outline of the GCT approach to this 
problem via algebraic geometry and representation theory, and
in the next two lectures elaborate it  further. 

\ignore{
\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes}
      \label{fig:complexityclasses}
\end{figure} 
}

\begin{figure}
\begin{center}
\psfragscanon
\psfrag{X}{$X$}
\psfrag{Y}{$Y$}
\psfrag{n}{$n$}
\psfrag{m}{$m$}
\psfrag{xlk}{$x_{l k}$}
\psfrag{yij}{$y_{i j}$}
\psfrag{barX}{$\bar X$}
\epsfig{file=matrices.eps, scale=.6}
\end{center}
      \caption{Linear representation $Y$ of a matrix $X$}
      \label{fig:matrices}
\end{figure} 


\section*{Why is algebraic geometry needed?}
Before we proceed any further, we have to  explain  why algebraic 
geometry is even needed, when the statements of these problems are 
purely elementary.

It would be helpful to first review the development
of GCT in this context. It  began with a  concrete
lower bound result, namely, the special case of the $P \not = NC$ conjecture
 \cite{GCTpram}, which says that 
the $P$-complete max-flow problem
cannot be solved in $\polylog(n)$ parallel time using $\poly(n)$ 
processors in the PRAM model without bit operations,  where $n$ denotes
the total bit length of the input (not just the number of input parameters).
We shall refer to this result
 as the {\em weak  form} of the $P$ vs. $NC$ problem. Its  proof is
based on classical algebraic geometry, and as such, this may be considered 
to be the first unconditional lower bound result to come out of GCT. 
Since it is a formal implication of the usual $P \not = NC$ conjecture,
it can be stated in purely elementary, combinatorial terms. And yet 
no elementary combinatorial proof of  this result is known so far. 
This suggested that geometry may be indipensible in
in the deeper study of the fundamental lower bound problems.



Another evidence is provided by the following 
weak form of $\#P$ vs. $NC$ problem. 
To define it, we have to first give an equivalent 
homogeneous restatement of the permanent vs. determinant problem. 
Let $\bar X$ be an $(n+1)\times (n+1)$ variable matrix. 
We identify $X$ with the $n \times n$ principal top-left minor of $\bar X$.
Let $z=\bar x_{n+1,n+1}$ be the bottom-right entry of $\bar X$, which is
not in $X$; we will use it as a homogenizing variable.
The problem now is to show that
for any large enough $n$, 
there do not exist complex numbers $a_{i,j}^{l,k}$, $l,k \le n+1$, 
$i,j \le m$,  such that, with 
\[ y_{i j} = \sum_{l,k\le n+1} a_{i,j}^{l,k} \bar x_{l,k}, \] 
$\perm(X)z^{m-n}=\det (Y)$, when $m$ is as above; here $\bar x_{l,k}$'s 
denote the
entries of $\bar X$. It is easy to check that this homogeneous form 
of the permanent vs. determinant problem is equivalent to the nonhomogeneous 
form given before.  

By the classical theorem of symmetric functions, 
$\det(Y)$ can be written explicitly as a polynomial 
$e(w_0, \ldots, w_{m})$, where $w_i =\trace(Y^i)$. 
Hence, the following can be thought of as 
a weaker  homogeneous  form of the $\#P$ vs. $NC$ problem:

\begin{theorem} (The weak form of the $\#P$ vs. $NC$ problem)  \label{tweak}

There do not exist complex numbers $b_i^l, c_j^k$, $l,k \le n+1$, $i,j \le m$,
and a polynomial $e(w_0,\ldots, w_m)$, 
such that, with 
\[ y_{i j} = \sum_{l,k\le n} b_i^l c_j^k  \bar x_{l,k}, \]
$\perm(X)z^{m-n}=g(Y)$, where  $g(Y)=e(\trace(Y^0),\ldots, \trace(Y^m))$, 
and  $m$ is as above. In fact, this holds
for any $m\ge n$. 
\end{theorem} 


That this holds for any $m \ge n$ indicates that this weak form is
too weak from the complexity theoretic perspective (unlike the 
weak form of the $P$ vs. $NC$ result above); it is  a mathematical 
result rather than complexity-theoretic.
It  too  can be easily proven  using  classical algebraic geometry 
\cite{GCT2append}. But no 
elementary proof, which  does not need  any nontrivial
algebraic geometry, is known so far   \footnote{There seems to be 
a serious gap in an  elementary 
proof proposed earlier by two  attendees of  the IAS lectures}. 

But at the same time  the 
classical algebraic geometry does not seem sufficient
for proving the general forms of the fundamental lower bound problems for
the following reasons. 
First, the classical techniques 
 used in \cite{GCTpram} are all degree-based  techniques, related in one way or other
other to Bezout's theorem in algebraic geometry. 
As was pointed out in the last of chapter 
of \cite{GCTpram}, such low-degree techniques would not work in the context
of the fundamental lower bound problems;
the recent  algebraization barrier \cite{aaronson} 
also says  something similar. 
The classical technique used for proving the weak form of the
$\#P$ vs. $NC$ result is   a low-degree technique. But it too has
a serious limitation: namely, it is naturalizable; i.e., cannot cross the
natural proof barrier in \cite{rudich}, because  it works for most
functions in place of the permanent. 

This suggests that something much more than classical geometry may be  needed 
for going further.
During the course of these lectures, we shall instantiate the 
basic strategy of GCT for the general form to provide a ``correct'' 
proof of the weak form of the $\#P$ vs. $NC$ result,
which does not have the   limitations of the ``wrong'' proof above.


\section*{Basic plan} 
We now proceed to outline the basic mathematical plan of GCT focussing on
the general permanent vs. determinant problem in characteristic zero. 
The weak form, which is not mentioned in any of the main GCT papers,
will only be  used  as a simple  example to test and illustrate 
the basic ideas as they are developed.

The first  step (GCT1,2) is to reduce this nonexistence problem 
to an existence problem--specifically, to the problem of proving 
existence of a family $\{O_n\}$ of obstructions; cf. Figure~\ref{fig:firststep}.
Here an {\em obstruction} $O_n$ is meant to be a proof-certificate of
hardness of $\perm(X)$, $X$ an $n\times n$ variable matrix,
just as Kurotowski minor is a proof-certificate of nonplanarity of a given
graph.  Specifically,  it would be some 
algebro-geometric-representation-theoretic gadget, 
whose existence for every $n$, would serve as a 
guarantee that $\perm(X)$ cannot be represented linearly as $\det(Y)$,
when $m=2^{\log^a n}$, $a>0$ fixed, $n\rightarrow \infty$. 

\begin{figure} 
\begin{center}\psfragscanon
\psfrag{on}{$\{O_n\}$}
\epsfig{file=firststep.eps, scale=.8}
\end{center}
      \caption{Reduction from nonexistence to existence}
      \label{fig:firststep}
\end{figure}


This reduction to existence is carried out as follows.
GCT1 associates with 
the complexity class $\#P$ a family $\{X_{\#P}(n,m)\}$ of (group-theoretic)
class varieties, and with the complexity class $NC$ a family of 
$\{X_{NC}(n,m)$ of (group-theoretic) class varieties such that: 
if $\perm(X)$, $\dim(X)=n$, can be represented as $\det(Y)$, $\dim(Y)=m
>n$, then 

\begin{equation} \label{eqembed} 
X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation} 

Each  class variety is a  (projective) algebraic variety, by which
we mean the zero set of  a system of mutivariate 
homogeneous polynomials with coefficients in $\C$  (akin to the 
usual curves  and surfaces). It is  group-theoretic in the 
sense that it is  constructed using group-theoretic operations 
and the general linear group $G=GL_l(\C)$, $l=m^2$, of $l\times l$ invertible
complex matrices acts on it. Here action means moving the points 
of the class variety around, just as $G$ moves the points of $\C^l$ around 
by the standard action via invertible linear transformations.
The goal is to show that the inclusion (\ref{eqembed}) is impossible;
cf. Figure~\ref{fig:class}. 

\begin{figure} 
\begin{center} \psfragscanon
\psfrag{xsharp}{$X_{\#P}(n,m)$}
      \psfrag{xnc}{$X_{NC}(n,m)$}
      \psfrag{g}{$G=GL_l(\C)$, $l=m^2$}
      \psfrag{Obstruction}{\mbox{Obstruction}}
\epsfig{file=class.eps, scale=.5}
\end{center}
      \caption{Class varieties}
      \label{fig:class}
\end{figure} 



Since each class variety has a $G$-action, the space of polynomial functions 
on each class variety has a  representation-theoretic structure, which 
puts constraints on which  representations of $G$ can live on that variety
(i.e. in the space of polynomial ) functions on that variety).
Informally, an obstruction is an irreducible (minimal)  representation of $G$
that can live on $X_{\#P}(n,m)$ but not on $X_{NC}(n,m)$; 
cf. Figure~\ref{fig:class}.
An existence of such an obstruction $O_n$, for every $n$, assuming
$m=2^{\log^a n}$, $a>1$ fixed, would show that the inclusion (\ref{eqembed}) 
is not possible--because otherwise $O_n$ could be found on $X_{NC}(n,m)$,
which is not possible. Thus existence of an obstuction blocks the
inclusion (\ref{eqembed}).


To define an obstruction formally, we need to recall some basic representation
theory.  By a classical result of Weyl, the irreducible 
(polynomial) representations of $G=GL_l(\C)$ are in one-to-one correspondence 
with the partitions of length at most $l$. By a partition $\lambda$ 
of length at most $l$, we mean an integral sequence $\lambda_1 \ge 
\lambda_2 \cdots \ge \lambda_k > 0$, $k\le l$; $k$ is called its length.
The irreducible 
representation of $G$ in correpsondence with $\lambda$ is denoted 
by $V_\lambda(G)$, and is called the {\em Weyl module} of $G$ indexed by 
$\lambda$. Symbolically:

\[\mbox{Irreducible representations of } G \stackrel{\mbox{Weyl}}{\Longleftrightarrow} \quad \mbox{partitions} \ \lambda. \]  

\[\mbox{Weyl module  } V_\lambda(G)  \longleftrightarrow \lambda. \] 


Now suppose $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$. 
Suppose to the contrary that 

\begin{equation} \label{eqembed2}   X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation}

Let $R_{\#P}(n,m)$ denote the homogeneous coordinate ring of 
$X_{\#P}(n,m)$; i.e. the ring of polynomial functions on $X_{\#P}(n.m)$
(though the  functions here are not functions in usual sense--i.e. 
their range is not $\C$--but we shall not worry about this). 
Let $X_{\#P}(n,m)_d$ be the degree-$d$-component of $X_{\#P}(n, m)$ consisting
of functions of degree $d$. We define $R_{NC}(n,m)$ and $R_{NC}(n,m)_d$
similarly. Since $X_{\#P}(n,m)$ has the action of $G$, $R_{\#P}(n,m)$ 
also has an action of $G$; i.e., it is a representation of $G$. Hence,
$R_{\#P}(n,m)_d$ is a finite dimensional representation of $G$. 
Similarly, $R_{NC}(n,m)$ is a represenation of $G$, and $R_{NC}(n,m)_d$
a finite dimensional representation of $G$. 



If (\ref{eqembed2} holds, then we get a natural map from $R_{NC}(n,m)$ to
$R_{\#P}(n,m)$ obtained by restriction of a function on $X_{NC}(n,m)$ to
$X_{\#P}(n,m)$; cf. Figure~\ref{fig:restriction}.
By basic algebraic geometry, this map
is surjective and is a $G$-homomorphism.
Furthermore, it is degree-preserving. This means there
is a surjective $G$-homomorphism from $R_{NC}(n,m)_d$ to 
$R_{\#P}(n,m)_d$. Symbolically: 

\begin{equation} \label{eqsurjection}
R_{\#}(n,m)_d <<-- R_{NC}(n,m)_d.
\end{equation}

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{Xp}{\small $X_{\#P}(n,m)$}
\psfrag{Xnc}{\small $X_{NC}(n,m)$}
\epsfig{file=restriction.eps, scale=.6}
\end{center}
      \caption{Restriction}
      \label{fig:restriction}
\end{figure}


Let $R_{\#P}(n,m)_d^*$ denote the dual of $R_{\#P}(n,m)_d$; i.e., the 
set of linear maps from $R_{\#P}(n,m)_d$ to $\C$. Then (\ref{eqsurjection})
implies that there is an injective $G$-homomorphism from 
$R_{\#P}(n,m)^*$ to $R_{NC}(n,m)^*$. Symbolically: 

\begin{equation} \label{eqinclusion}
R_{\#}(n,m)_d^*  \hookrightarrow {NC}(n,m)_d^*.
\end{equation}

\begin{defn} (GCT2)
An obstruction $O_n$ is a Weyl module $V_\lambda(G)$ that 
occurs in $R_{\#P}(n,m)_d^*$  but not in $R_{NC}(n,m)_d^*$, for some $d$. 

We call $\lambda$ an {\em obstruction label}, and sometimes,
by abuse of notation, an obstruction as well.
\end{defn}

\begin{prop} (GCT2)
Existence of an obstruction $O_n$, for all $n\rightarrow \infty$, 
with $m=2^{\log^a n}$, $a>1$ fixed, implies $\perm(X)$, $\dim(X)=n$, 
cannnot be represented linearly as 
$\det(Y)$, $\dim(Y)=m$. 
\end{prop}

This follows just from the definition of an obstruction.

This leads to:

\begin{goal} 
Prove existence of an obstruction family $\{O_n\}$ using 
the {\em exceptional} nature of $\perm(X)$ and $\det(Y)$. 
\end{goal} 

Exceptional here means completely characterized by symmetries 
in the following sense. 
Clearly, for any $A,B \in GL_m(\C)$, with $\det(A)\det(B)=1$, 
\[ \det(Y)=\det(A Y^* B), \] 
when $Y^*=Y$ or $Y^t$. Let us think of $Y$ as a variable $m\times m$ matrix.
Let $\sym^m(Y)$ be the space of homogeneous forms of degree $m$ 
in the $m^2$ variable entries of $Y$. Then it follows from classical
representation theory that $\det(Y)$ is the only form in $\sym^m(Y)$ 
with this property. Thus $\det(Y)$ is completely characterized 
by its symmetries and hence is an exceptional form in $\sym^m(Y)$ 
in this sense. 

Simlarly, for any diagonal or permutation matrices $A,B$, 
\[ \perm(X)=\perm(AX^*B), \]
when $X^*=X$ or $X^t$. And this completely characterizes $\perm(X)$ 
in the space of forms of degree $n$ in the entries of $X$.
So $\perm(X)$ is also exceptional in this sense.


\subsection*{The weak case}
\begin{theorem} \cite{GCT2append} \label{tgct2append}
There exists a family  $\{O_n\}$ of obstructions in the weak form of 
the $\#P$ vs. $NC$ problem in characteristic zero.
\end{theorem}

(Class varieties and obstructions are defined in a similar fashion 
in the weak form--we omit their formal definitions). This result 
implies Theorem~\ref{tweak} and provides its 
 ``correct'' proof. We shall outline it briefly in the next lecture.
It is based on a detailed study of the $G$-action on class varieties
based on:
\begin{enumerate} 
\item The work on stability in geometric invariant theory by 
Hilbert, Mumford, Kempf and others. 
\item Peter-Weyl theorem for $G=GL_l(\C)$, which the algebraic form 
of the (noncommutative) harmonic analysis on the unitary group 
$U_l(\C)$. 
\item An extension of an induction technique 
in the Borel-Weil theorem of geometric representation theory.
\end{enumerate}

\subsection*{The general case} 
Now we proceed to the general case, our  main interest. 

Towards that end, we shall associate with the class varieties 
certain representation-theoretic functions. 
Let $F_{\lambda,n,m}(k)$ denote the number of occurences (multiplicity)  of
the Weyl module $V_{k\lambda}(G)$ in $R_{\#P}(n,m)$, and 
$G_{\lambda,n,m}(k)$ the number of occurences of 
$V_{k\lambda}(G)$ in $R_{NC}(n,m)$. Thus these are statistical functions
associated with the class varieties, where the statistics associates 
with every number $k$ the multiplicity of the corresponding
Weyl module $V_{k\lambda}(G)$; cf. Figure~\ref{fig:statistics}.

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{l}{$\lambda$}
\psfrag{2l}{$2 \lambda$}
\psfrag{3l}{$3 \lambda$}
\psfrag{v1}{$V_\lambda(G)$}
\psfrag{v2}{$V_{2 \lambda}(G)$}
\psfrag{v3}{$V_{3\lambda}(G)$}
\epsfig{file=statistics.eps, scale=1}
\end{center}
      \caption{statistics}
      \label{fig:statistics}
\end{figure}

We will also need a definition.
Let us  call a function $f(k)$ quasipolynomial if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k_)$ for all nonnegative integral $k=i$ modulo $l$; $l$ is
called the period of the quasi-polynomial. Thus  quasi-polynomials
are hybrids of  polynomial and periodic functions. 

A fundamental example of a quasi-polynomial is the Ehrhart quasi-polynomial
$f_P(k)$ of the polytope $P$ with rational vertices. It is defined
to the number of integer points in the dilated polytope $kP$. By the 
classical result of Ehrhart, it is known to be a quasi-polynomial.




\begin{theorem} (GCT6) \label{tquasi}
The functions $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ 
are quasi-polynomials assumming the singularities of the class varieties
$X_{\#P}(n,m)$ and $X_{NC}(n,m)$ are rational. 

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem} 

Here rational singulary means a singularity that is nice in
a certain algebro-geometric sense that we shall not elaborate.

The proof of this result follows from a detailed study of the behaviour
of the singularities of class varieties under the action of the 
group $G$. This is based on
\begin{enumerate} 
\item The 
resolutions of singularities in characteristic zero, as per 
Hironaka \cite{hironaka}: 
this  roughly says 
that the singularities of any algebraic variety in characteristic zero
can be untangled (resolved) nicely in a systematic fashion; cf.
 Figure~\ref{fig:resolution}.
\item Cohomological works of Boutot, Brion, Kempf, Flenner and others
bases on this resolution.
\end{enumerate} 


\begin{figure} 
\begin{center} 
\epsfig{file=resolution.eps, scale=.5}
      \caption{Resolution}
      \label{fig:resolution}
\end{center}
\end{figure}


As such, this proof is highly nonconstructive. It gives no effective
bound on the period $l$--it just says that $l$  is finite.

\begin{hypo} {\bf (PH) [Positivity Hypothesis]} \label{hph}

For every $\lambda,n,m\ge n$, 
there exist polytopes $P=P_{\lambda,n,m}$ and $Q=Q_{\lambda,n,m}$ 
such that 
\begin{equation} 
\begin{array}{l}
F_{\lambda,n,m}(k)=f_P(k), \\
G_{\lambda,n,m}(k)=f_Q(k).
\end{array}
\end{equation}
If such $P$ and $Q$ exist, their dimensions are guaranteed to be
polynomial in $n$ and the length of $l$ by the proof of Theorem~\ref{tquasi}.
It is also assumed here that there exists for $P_{\lambda,n,m}$ a specification
of the form $A x \le b$, where $A$ is independent of $\lambda$, and $b$ is 
a piecewise homogeneous linear function of $\lambda$, so that
$P_{k\lambda,n,m}=k P_{\lambda,n,m}$. Similarly for $Q_{\lambda,n,m}$.

Analogous positivity hypothesis for the $P$ vs. $NP$ problem in characteristic
zero.
\end{hypo} 

When this holds, we say that $F_{\lambda,n,m}(k)$ and 
$G_{\lambda,n,m}(k)$ have {\em positive convex representations}. 
Here positivity refers to the fact that the Ehhart quasipolynomial 
$f_P(k)$ is a positive expression:
\[ f_P(k)=\sum_{v} 1,\] 
where $v$ ranges over all integer points in $kP$--there are no 
alternating signs in this expression.
Convexity refers to convexity of the polytopes $P$ and $Q$. 

\begin{theorem} (GCT6)
There exists a family $\{O_n\}$ of obstructions 
for the general $\#P$ vs. $NC$ problem in characteristic zero, 
for $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$, 
assuming, 

\begin{enumerate} 
\item PH, and
\item OH (Obstruction Hypothesis): 

For all $n\rightarrow \infty$,  there exists $\lambda$ such that 
$P_{\lambda,n,m}\not = \empty$ and $Q_{\lambda,n,m}=\empty$.
\end{enumerate}

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem}

We call  $\lambda$ a {\em relaxed obstruction}
(or rather, relaxed obstruction-label)
if  satisfies OH. In this case, $k\lambda$, for some integer $k\ge 1$ is
an obstruction--we just have to choose $k$ so that the scaled polytope 
$P_{k\lambda,n,m}=k P_{\lambda,n,m}$ contains an integer point 
(and $Q_{k \lambda,n,m}=k Q_{\lambda,n,m}$ will continue to be empty). 
Henceforth, whenever we say obstruction, we actually mean relaxed 
obstruction.




\subsection*{The flip: Explicit construction of obstructions} 
In principle PH may have a nonconstructive proof, like that
of Theorem~\ref{tquasi}, which only tells  that such polytopes 
exist without explicitly constructing them. But proving OH may not be feasible
unless the polytopes $P$ and $Q$ in PH are given explicitly.

This  suggests the following strategy for proving 
existence of obstructions.


\noindent (1) Prove the following stronger explicit form 
of PH:

\begin{hypo} {\bf ($PH^+$)} 
There exist {\em explicit} 
polytopes $P_{\lambda,n,m}$ and $Q_{\lambda,n,m}$ satisfying PH.
Explicit means: 

\begin{enumerate}
\item  The polytopes are specified by explicit systems of linear constraints,
each constraint of bitlength $\poly(n,\bitlength{\lambda}, \bitlength{m})$
(here $\bitlength{m}$ occurs instead of $m$). 


\item  The membership problems for the polytopes
$P_{\lambda,n,m}$ and $Q_{\lambda,n,m}$ belong to the complexity class $P$.
That is,  given a point $x$, whether it belongs to $P_{\lambda,n,m}$ 
or $Q_{\lambda,n,m}$ can be decided in time that is polynomial in
$n$, the bitlength $\bitlength{\lambda}$ of $\lambda$, the 
bitlength $\bitlength{x}$ of $x$ and $\bitlength{m}$. 
Furthermore, we assume that if $x$ does not belong to the polytope,
then the membership algorithm also gives a hyperplane separating 
$x$ from the polytope in the spirit of \cite{lovasz}. 
\end{enumerate} 
\end{hypo}

In particular, $PH^+$ implies that the functions $F_{\lambda,n,m}(k)$ and
$G_{\lambda,n,m}(k)$ belong to the complexity class $\#P$. 


\noindent (2a) {\bf [The flip]}

Let $m=2^{\log ^a n}$, for a fixed $a>1$. 
Using explicit forms of the polytopes $P$ and $Q$ in $PH^+$,
show existence of  an {\em explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of obstructions  satisfying OH. 
We say that an obstruction (proof-certificate) 
$\lambda_n$ is {\em explicit} if is ``short'' and ``easy to verify'':

\begin{enumerate} 
\item  Short: This means its bitlength $\bitlength{\lambda_n}$ 
is $\poly(n)$,
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  

\item Easy to verify: given $n, m \le 2^{\log^a n}$ and 
$\lambda_n$, whether 
$\lambda_n$ is a valid obstruction 
can be verified 
in $\poly(n,\bitlength{\lambda})$ time. In particular, this is
$\poly(n)$ when $\bitlength{\lambda}=\poly(n)$. 
\end{enumerate}. 

Existence of an explicit family of obstructions is equivalent to saying
that the problem of deciding existence of obstructions belongs to $NP$.
This definition of explicitness is quite natural since the class $NP$ 
is a class of problems whose proof-certificates (witnesses) are 
short and easy to verify. As such, the flip--going for 
explicit  obstructions--is
a proof-strategy that is literally given to us on a platter 
by the $P$ vs. $NP$ 
problem itself. The terminology flip would be explained later.


It should be stressed that we are primarily interested in only proving 
existence of obstructions. Whether they are explicit or not 
does not really matter in the original statement of the problem.
But we need to know the polytopes $P$ and
$Q$ explicitly ($PH^+$) here so that proving OH is feasible. 
In other words,   if we do not
even know what the polytopes $P$ and $Q$ look like, 
it seems unlikely that anything  could be said regarding OH. 
But once  $PH^+$ is proved, existence of an explicit family follows
automatically,   as a bonus, whether we care for it or not. 

To see why, let us observe that 
the second condition above  (ease of verification) follows directly
from $PH^+$ and the polynomial time algorithm for 
linear programming with polytopes given by separation oracles \cite{lovasz}. 
And shortness is also a direct consequence of $PH^+$. 

Thus it is as if the $P$ vs. $NP$ problem is forcing us to go
for explicit obstructions.


\noindent (2b) {\bf [The strong flip (optional)]} 

Using explicit forms of the polytopes $P$ and $Q$ in $PH^+$,
construct (rather than just show existence of) 
a {\em strongly explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of obstructions  satisfying OH. We say that an explict family 
of obstructions is strongly explicit if,
for each $n$, a valid obstruction-label
$\lambda_n$ can be constructed in $\poly(n)$ time.
In particular, the height and the bitlength of
of $\lambda$ is meant to be $\poly(n)$ (short) 
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  


For the purposes of the lower bound problems that we are interested in--namely,
the $P$ vs. $NP$ and the $\#P$ vs. $NC$ problems in characteristic zero--the
flip (just explicit  
existence) would suffice and the stronger flip (explicit construction)
is optional. But the stronger flip can give us deeper insight into these
lower bound problems; cf. GCTflip for more on this.

Now we turn to a few obvious questions.

\subsection*{Why should PH, $PH^+$,  and OH hold?} 

Mathematical evidence for this is given in GCT2,4,6,7,8.
We shall discuss this a bit in the third lecture.


\subsection*{What has been achieved by all this?: The meaning of the flip} 
Let us now take a stock of what has been achieved so far
in the context of the 
$\#P\not = NC$ conjecture in the nonuniform setting (characteristic zero),
the argument for the $P$ vs. $NP$ problem in characteristic zero
being  similar. The goal of this conjecture is to prove that 
$\perm(X)$ cannot be computed by an arithmetic circuit $C$ over $X$ with
coefficients in $\C$ of size $m=\poly(n)$, or more generally,
$m \le 2^{\log^a n}$, for some fixed $a>1$, and depth $O(\log^a n)$.
Or in symbols:

\[ {\bf (IOH):}  \forall n  \forall C \exists X:
\perm(X)\not = f_C(X),\] 

where $f_C(X)$ denotes the function computed by $C$, and $n$ is supposed
to be sufficiently large.
For given $X$ and $C$ of $\poly(n)$ size, the problem 
of deciding if  $\perm(X) = f_C(X)$ belongs to $\#P$ (or rather, $P^{\#P}$). 
Since there are two alternating layers of quantifiers in the above
condition, the problem of verifying it belongs to $\Pi^2 \#P$,
as of now, which is very high in the complexity hierarchy
 (cf. Figure~\ref{fig:IOHcomplexity}).
Hence, we  refer to the original hypothesis to be proven above as IOH 
(Infeasible Obstruction Hypothesis). Of course, IOH is expected to 
be a tautology, and hence is expected to  be verifiable in $O(1)$ time--but
we do not know that as yet. 



\begin{sidewaysfigure} 
\begin{center}
\psfragscanon
\psfrag{sigma2p}{{\small $\Pi^2 \#P$}}
\psfrag{sigma1p}{$\Sigma^1 \#P$}
\psfrag{P}{{\small $P$}}
\psfrag{NP}{{\small $NP$}}
\psfrag{T}{$T$}
\psfrag{#P}{$\# P$}
\psfrag{inNP}{$\in NP$}
\psfrag{inP}{$\in P$}
\psfrag{insigma2p}{$\in \Pi^2 \#P$}
\psfrag{PHplus}{$PH^+$}
\psfrag{PHtil}{$PH^\dagger$}
\epsfig{file=IOHcomplexity.eps, scale=.8}
\end{center}
      \caption{Positivity as a means to eliminate the variables in and 
reduce the complexity of the  obstruction hypothesis}
      \label{fig:IOHcomplexity}
\end{sidewaysfigure}



Equivalently, the goal is to prove existence of a {\em trivial obstruction},
which is a table that lists for each $C$ as above a counterexample  $X$ so that
$\perm(X)\not = f_C(X)$; cf. Figure~\ref{fig:trivial}.
The number of rows of this table is equal
to the number of circuits $C$'s of size $m\le  2^{\log^a n}$ and depth
$O(\log^a n)$. Thus the size of this table is more than
exponential; i.e. $2^{O(m)}$. 
The time to verify whether a given table is also more than exponential,
and so also the time to decide if such at table exists and construct 
one, for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. So
we refer to  this trivial, brute force 
strategy of proving IOH, based on existence of trivial obstructions,
as an {\em infeasible strategy}. 

\begin{figure} 
\begin{center} 
\epsfig{file=trivial.eps, scale=.5}
\end{center}
      \caption{A trivial obstruction}
      \label{fig:trivial}
\end{figure}


In contrast, assuming $PH^+$, the problem  of verifying OH belongs 
to $NP$ as we have already observed. Thus, assuming $PH^+$, we have 
transformed the original infeasible obstruction 
hypothesis $IOH \in \Pi^2 \#P$ to a new  obstuction hypothesis 
$OH \in NP$, in the process bringing down the time to verify an obstruction
from the exponential (for the original trivial obstruction) to polynomial
(for the new obstruction); cf. Figure~\ref{fig:IOHcomplexity}.  
Intuitively, the new obstruction captures  the essence of the old obstruction
in short space.
In effect,  the task of verification of an obstruction has been 
transformed from the infeasible (exponential-time) to the feasible 
(polynomial-time), hence the name of this strategy: the flip,
from the infeasible to the feasible.
Positivity ($PH^+$) is used in this flip as a means  to
eliminate the quantifying variables in IOH and bring down the 
the complexity of the obstruction hypothesis; cf. Figure~\ref{fig:IOHcomplexity}. 




This process can be extended further. Assuming an additional
positivity hypothesis $PH^\dagger$ to be specified below,
$OH \in NP$ can be transformed 
to POH (Positivity Obstruction Hypothesis) that belongs to $P$; i.e.,
which can be verified in polynomial time, and an obstruction,
if it exists, can also be constructed in polynomial time; 
cf. Figure~\ref{fig:IOHcomplexity}. 
Once this final positivity hypothesis POH is proven, the obstruction
hypothesis is reduced to a tautology, which can be verified in
$O(1)$ time. This  would then give us 
the final $O(1)$-size  proof. 

Thus the basic idea of the flip is to use positivity systematically
as a means to elminate the quantifiers  and bring down the complexity 
of the  obstruction hypothesis until it is finally
transformed into an $O(1)$-time verifiable  tautology;
 cf. Figure~\ref{fig:IOHcomplexity}. 

Now let us specify $PH^\dagger$ and POH.
Towards that end, let  $k$ be the length of $\lambda$; 
it could be anything $\le l=m^2$. 
Define 

\begin{equation} 
\begin{array}{l}
\bar P_{n,m}= \{ \lambda: P_{\lambda,n,m} \not = \empty \} \subseteq \C^k, \\
\bar Q_{n,m}= \{ \lambda: Q_{\lambda,n,m} \not = \empty \} \subseteq \C^k.
\end{array}
\end{equation}

Then: 

\begin{hypo}  {\bf $PH^\dagger$} 

The sets $\bar P_{n,m}$ and $\bar Q_{n,m}$ are convex polytopes in $\C^k$.
Furthermore, the membership problems for these problems belong to 
$P$ and so also the problem of deciding if $\mbox{vol}(\bar P_{n,m}
\setminus \bar Q_{n,m})$, the volume of the relative complement 
$\bar P_{n,m} \setminus \bar Q_{n,m}$, is nonzero (positive);
i.e. if $\bar P_{n,m} \subseteq \bar Q_{n,m}$. By polynomial time,
we mean $\poly(n,l,\bitlength{m})$ time. This is $\poly(n)$ time,
if $m\le 2^{o(n)}$ and $l =\poly(n)$. 
\end{hypo}

\begin{hypo} {\bf (POH)}

For all $n\rightarrow \infty$, assuming $m=2^{\log^a n}$, $a>1$ fixed, 

\[ \mbox{vol}(\bar P_{n,m} \setminus \bar Q_{n,m}) > 0, \] 

for $k=(n+1)^2$. 
\end{hypo} 

Thus POH says that  the line-shaded area in Figure~\ref{fig:POH} has positive
volume for all large enough $n$. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{P}{$\bar P_{n,m}$}
\psfrag{Q}{$\bar Q_{n,m}$}
\epsfig{file=POH.eps, scale=1}
\end{center}
      \caption{POH}
      \label{fig:POH}
\end{figure}


\subsection*{How to prove $PH$?} 
The goal is to extend the proof of the
PH needed to prove Theorem~\ref{tgct2append} for
the weak form to that of the PH for the general form 
(cf. Hypothesis~\ref{hph}).
One crucial ingradient of the PH needed for the weak form is the classical
positive convex interpretation for the Littlewood-Richardson (LR) coefficient
$c_{\alpha,\beta}^\lambda$, which is defined to be 
the number of occurences of the Weyl module $V_{\lambda(G)}$ in the 
tensor product of $V_{\alpha}(G)$ and $V_\beta(G)$. We shall refer to
it as PH[LR].   What is needed to prove PH in the
general case is a similar positive convex interpretation for the
so-called plethysm constants in representation theory, of which the 
Littlewood-Richardson coefficient is a very special case--we shall refer this
as PH[Plethysm].  This  happens to be a fundamental open problem of
representation theory, older than the $P$ vs. $NP$ problem itself, and 
has been studied intensively in the last century. It turns out 
be at the heart of this approach towards $P$ vs $NP$, $\#P$ vs. $NC$ and
related problems. 


A basic plan to prove PH[Plethysm] is given in (GCT6).
It is partially 
implemented in GCT4,6,7,8; cf. Figure~\ref{fig:lift} for a pictorial
depiction of the plan. It seeks to extend the  proof of PH[LR] based 
on the theory of the  standard quantum group to the plethysm setting. 
In the  theory of the standard quantum group, PH[LR] comes out as 
a consequence of a  (proof of a) deep positivity results, which
we shall refer to as Ph0[LR]. It says that  that the 
tensor product of two representations of the standard quantum group 
has a canonical basis whose structure coefficients are all positive 
polynomials (i.e., polynomials with nonnegative coefficients).
The only known proof of this
result is based on the Riemann Hypothesis over finite fields (RHf), proved by
Deligne \cite{weil2} 
based on the work of Grothendick, and the related works \cite{beilinson}. 
The Riemann Hypothesis is  itself a deep positivity statement in mathematics,
from which   PH[LR] can  thus be 
deduced, as shown on the bottom row of Figure~\ref{fig:lift}.

If one were only interested in PH[LR], one  does not 
need this  powerful machinery, becuase it has a  much simpler 
algebraic-combinatorical  proof. 
But the plan to extend the
proof of PH[LR] to PH[Plethysm] in GCT6,7,8 is like a huge
inductive spiral. To  make it work,  one  needs a 
stronger inductive hypothesis than PH, which is precisely  PH0.
Thus what is needed now 
is a systematic lifting up of the bottom arrow in Figure~\ref{fig:lift}.

Initial  steps in this direction have been taken in GCT7,8. 
First, GCT7 constructs a {\em nonstandard quantumg group}, which
generalizes the notion of a standard quantum group, and plays that 
same role in the plethysm setting that the standard quantum group plays
in the LR setting. Second, GCT8 gives an algorithm to construct 
a canonical basis for the representation of the nonstandard quantum group
that is conjecturally correct and has the property PH0[Plethysm],
which is a natuaral generalization of PH0[LR] in the plethysm setting.
Now what is needed to prove PH0[Plethysm], and thus fill in the 
commutative digram in Figure~\ref{fig:lift}, is an appropriate nonstandard 
extension of the Riemann hypothesis over finite fields and the related work,
from which then PH0[Plethysm] can be deduced. This is the big open 
problem here, far beyound our personal expertize. But it is 
our hope that the field of mathematics would have something to say about it.


\subsection*{How to prove OH or POH?} 
We have nothing to say on this at this point,
since the  proof of OH and POH 
would really depend on the explicit forms of the
polytopes $P$ and $Q$ that arise in   $PH^+$. 


\ignore{
\subsection*{Is all this necessary?} 
Finally, one may  ask: if the positivity problems are so formidable, can
they not be avoided somehow? Unfortunately, there is a formidable 
barrier towards the $P$ vs. $NP$ and related problems, called the
{\em feasibility barrier}, which seems universal in the sense that
any approach towards these problems would have to tackle it, not just GCT. 
The existing mathematical evidence suggests that any natural approach
to cross this barrier may have to battle with  some deep positivity hypotheses 
in the spirit of PH  (though  not exactly PH) one way or the other.
That is,  positivity  may indeed be 
the heart of the  fundamental lower bound problems in complexity theory;
cf \cite{} for a detailed story.
}









































 

































\begin{sidewaysfigure} 
\begin{center} 
\epsfig{file=lift.eps, scale=.8}
\end{center}
      \caption{Lift}
      \label{fig:lift}
\end{sidewaysfigure} 



\ignore{\begin{figure} 
\psfragscanon
\psfrag{P}{$P\not = NP$ and $\#P\not = NC$ conjectures (characteristic zero)}
\epsfig{file=barriers.eps, scale=1}
      \caption{The feasibility barrier towards $P$ vs. $NP$}
      \label{fig:barriers}
\end{figure}}



==> lecture1_10.tex <==
\section*{Introduction}

This article   gives a mathematical  overview of
geometric complexity theory (GCT), an
approach  towards the fundamental lower bound problems  in complexity theory, 
such as (Figure~\ref{fig:complexityclasses}):

\noindent (1) 
The $P$ vs. $NP$ problem \cite{cook,karp,levin}: 
 show that $P \not = NP$;


\noindent (2) 
The  $\#P$ vs. $NC$ problem \cite{valiant}: show that 
$\#P \not = NC$.

\noindent (3) The $P$ vs. $NC$ problem: show that $P \not = NC$.



We  focus here on only the nonuniform versions of the above problems 
in characteristic zero; i.e., when
the underlying field of computation is of characteristic zero, 
say $\Q$ or $\C$--what this means will be explained below.
The additional problems that
need to be addressed when the underlying field of computation is finite
would be discussed in  GCT11. 


The nonuniform
characteristic zero version of the $P\not = NC$ conjecture (in fact,
something stronger) was already proved  in GCTlocal. We shall refer
to it as the $P\not = NC$ result without bit operations.
It says that the max flow problem cannot be solved in the 
PRAM model without bit operations in $\polylog(N)$ time using 
$\poly(N)$ processors where $N$ is the bitlength of the input.
This  may be considered to be the first unconditional lower bound result of
GCT, because, though it can be stated in purely elementary combinatorial
terms, being a formal implication of the $P\not = NC$ conjecture, its
proof is intrinsically geometric, and no elementary proof is known so far. 
Furthermore, its proof  technique may be considered to be a weaker (local)
form of the {\em flip}, the basic guiding strategy of GCT, which  was 
refined and formalized much later in GCTflip. 
This  was the begining of  this  geometric approach in complexity theory.
The later work in GCT-- the subject of this overview--focusses on the other 
two problems above, namely
the $P$ vs. $NP$ and $\#P$ vs. $NC$ problems. 


The nonuniform (characteristic zero) version of the $\#P$ vs. $NC$ problem
is also known as the permanent vs. determinant problem \cite{valiant}. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented %(cf. Figure~\ref{fig:matrices})
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$. %; the best known lower bound on $m$ at present is 
% quadratic \cite{ressayre}.
By linear representation, we mean
the  entries   of $Y$ are  (possibly nonhomogeneous) 
linear functions of the entries of $X$. 
There is an analogous characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.
The main results of GCT for the $\#P$ vs. $NC$ problem in 
characteristic zero also extend to the $P$ vs. $NP$ problem in characteristic
zero. But here we 
concentrate  on only the former problem,
since this illustrates all the basic ideas. 



The complementary article \cite{GCTexplicit} gives a complexity-theoretic
overview of GCT. It describes   the main complexity theoretic
barrier towards these problems 
called the {\em complexity barrier} and the defining
strategy of GCT for crossing it called the {\em flip} [GCT6,GCTflip]: 
which is to go 
for {\em explicit proofs}. By an explicit proof 
we mean a proof that provides proof certificates of hardness  for the 
hard function under consideration that are short (of polynomial size) 
and easy to verify (in polynomial time). This barrier turns out to be
extremely formidable and is the root cause of all difficulties 
in these problems. Nonelementary techniques are brought into GCT precisely
to cross this barrier. It is not discussed in these lectures. 
The goal here is to describe the basic ideas of GCT at a concrete mathematical
level without getting into such meta issues. But the readers who wish
to know the need for the nonelementary techniques in GCT before getting
into any mathematics   may wish to read that
article before this one. On the other hand, the readers who would rather avoid 
meta issues before getting a concrete mathematical
picture  may wish to read this article first. We  leave the
 choice to the readers.

The original IAS lectures stated a lower bound called a 
{\em weak form  of the $\#P$ vs. $NC$
problem}. This is a special case of a far more general result 
GCT, which may be considered its second unconditional lower bound result, and 
which we shall call {\em a mathematical form of the $\#P \not = NC$ 
conjecture}.  It is essentially a direct consequence of the general 
results in GCT1 and 2 in conjunction with a fundamental result \cite{kempf} 
of geometric invariant theory \cite{mumford} that was used there, though
the lower bound was not stated there. It would appear in revised GCT6
with an explicit proof which needs an additional result \cite{ariki} 
in representation theory.
The article \cite{boris} showed that the weak form  stated in the IAS 
lectures is  too weak because it has a direct elementary proof 
which is naturalizable, i.e., which  does not cross the natural proof barrier
\cite{rudich}. Hence in this article it has been replaced with the 
mathematical form of the $\#P\not = NC$ conjecture mentioned above; cf. 
Section~\ref{sweaklec1}. 
We cannot prove this  mathematical form by such elementary 
proof techniques for the reasons given in Sections~\ref{sweaklec1} and 
\ref{sweak}. 





The rest of this article is organized in the form of three chapters,
one per  lecture. The first gives a short mathematical 
overview of the basic plan of GCT,  
which is elaborated in the next two lectures. 


\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes}
      \label{fig:complexityclasses}
\end{figure} 




\noindent {\em Acknowledgement:} The author is grateful to 
Avi Wigderson for arranging the lectures and the hospitality,
to the authors of \cite{boris} for pointing out weakness of the 
lower bound stated during the lectures, and to Shrawan Kumar for
bringing the reference \cite{ariki} to his attention and 
helpful discussions.




\chapter{Basic plan} 
We now outline the basic  plan of GCT focussing on
the  permanent vs. determinant problem in characteristic zero. 

\section{Characterization by symmetries} \label{scharsym}
We begin by observing that 
the permanent and the determinant are 
{\em exceptional} polynomial functions. By exceptional we mean
that they are  completely characterized by the symmetries in the 
following sense.


Let  $Y$ be a variable $m\times m$ matrix.
Let $\sym^m(Y)$ be the space of homogeneous forms of degree $m$ 
in the $m^2$ variable entries of $Y$. Then, by the  classical
representation theory,  $\det(Y)$ is the only form in $\sym^m(Y)$ 
such that, for any $A,B \in GL_m(\C)$ with $\det(A)\det(B)=1$, 

\noindent  {\bf (D):} $\det(Y)=\det(A Y^* B)$,

where $Y^*=Y$ or $Y^t$. 
Thus $\det(Y)$ is completely characterized 
by its symmetries, and hence, is  exceptional. We shall refer 
to this characteristic property of the determinant as property (D)
henceforth.

Similarly, $\perm(X)$ is the only form 
in the space of forms of degree $n$ in the entries of $X$ such that, 
for any diagonal or permutation matrices $A,B$,

\noindent  {\bf (P):} $\perm(X)=\perm(AX^*B)$, 

where $X^*=X$ or $X^t$  with obvious constraints 
on the product of the diagonal entries of $A$ and $B$ when they are diagonal.
Thus $\perm(X)$ is also
completely characterized   by its symmetries, and hence, is
exceptional.
We shall refer 
to this characteristic property of the permanent as property (P)
henceforth.


A basic idea [GCT1]  is to a get a handle on 
the permanent vs. determinant problem 
by exploiting exceptional nature of these polynomials--i.e.,
their characteristic properties (P) and  (D).
Representation theory and 
algebraic geometry enter inevitably into  the study of these properties,
because
to understand symmetries representation theory (of groups of symmetries)
becomes indispensible, and to understand  deeper properties 
of representations  algebraic geometry becomes indispensible. 


\section{A mathematical form of the  $\#P \not = NC$ conjecture} 
\label{sweaklec1}
To show how these characteristic properties can be exploited, 
we now state one application of 
GCT in the form of a concrete lower bound result--namely a 
mathematical form of the 
$\#P \not = NC$ conjecture (Theorem~\ref{tgenweaklec1} below)--before
going any further.

We begin by observing that 
the permanent vs. determinant conjecture clearly implies  that 
$\perm(X)$ of any $n \times n$ variable matrix $X$ can not be represented 
as an $NC$-computable polynomial in the traces of $\bar X^j$, $j \ge 0$,
$\bar X=B X C$
for any (possibly singular) $n\times n$ matrices $B$ and $C$, since
$X^j$ can be computed fast in parallel. This can be proved unconditionally.
In fact, something stronger.

\begin{prop}  \label{pweaklec1}
There do not exist (possibly singular) $n\times n$ complex
matrices $B$ and $C$  and a polynomial 
$e(w_0,\ldots, w_n)$ such that $\perm(X) = g(BXC)$, 
where $g(X)=e(\trace(X^0), \trace(X), \ldots, \trace(X^n))$. 
\end{prop}
This was referred to as 
the weak form of the $\#P$ vs. $NC$ problem in the original IAS lecture. 
The article \cite{boris} showed that this is too  weak 
by giving an  elementary
proof \cite{boris} for it that is naturalizable, i.e.,
which cannot cross the
natural proof barrier \cite{rudich} because it works for most functions in
place of the permanent. The proof technique of
the quadratic lower bound \cite{ressayre}
for the permanent is also naturalizable.

We now state a much more general lower bound, which
was not stated in the IAS lecture, and which does not have such 
a naturalizable proof. For that we need a definition.

\begin{defn} \label{dgenperm}
A polynomial function $p(X_1,\ldots,X_k)$ (of any degree)
in the entries of $k$ $n\times n$ variable matrices $X_1,\ldots,X_k$  
is called a  {\em generalized permanent} if it has exactly 
the same symmetries as that of the permanent; i.e.,
for all nonsingular $n\times n$ matrices $U_i$ and $V_i$, $i \le k$, 
\[ p(U_1 X_1 V_1,\ldots, U_k X_k V_k)=p(X_1,\ldots,X_k) 
\mbox{\ iff\ } \perm(U_i X V_i)=\perm (X) \quad \forall i.\] 
\end{defn}

A precise description of the symmetries of the permanent  is given
by the property (P). Hence, $U_i$ and $V_i$ above have to be permutation
or diagonal matrices (with obvious constraints on the product of their 
diagonal entries), or 
product of such matrices.
When $k=1$ and $n$ is arbitrary,
there is just one generalized permanent of degree $n$, namely
the usual permanent itself. 
At the other extreme, 
when $n=1$ and $k$ is arbitrary, every function in $k$ variables 
is a generalized permanent. 
For general  $n$ and $k$, almost any polynomial 
in $\perm(X_i)$'s, $i \le k$, is  a generalized permanent, but 
there are many others besides these.
For general degrees, 
the dimension of the 
space spanned by  generalized permanents can be  exponential
in $n$; cf. Section~\ref{sweak}. 
In general,  the space of generalized permanents has a highly nontrivial
structure that  is intimately linked  to some
fundamental problems of representation theory;
cf. Section~\ref{sweak} and  [GCT6].


Now we have the following:

\begin{obs}[Implication of the nonuniform $\#P \not = NC$ conjecture]

Assuming the nonuniform $\#P \not = NC$ conjecture in characteristic zero,
no $\#P$-complete generalized permanent  $p(X_1,\ldots,X_k)$ of $\poly(n,k)$ 
degree can be expressed as an $NC$-computable polynomial function of the 
traces of  $\bar X_i^j$, $1 \le i \le k$, $j=\poly(n,k)$, where 
$\bar X_i=B_i X_i C_i$,  $i \le k$,  for any $n\times n$ complex (possibly
singular) matrices $B_i$ and $C_i$.
\end{obs}
(Here $X_i^j$ are  clearly $NC$-computable).

When $n=1$ and $k$ is arbitrary, this implication is  equivalent 
to the original nonuniform $\#P \not = NC$ conjecture (in characteristic 
zero),
since then any polynomial in $x_1,\ldots, x_k$ is a generalized permanent,
and a polynomial function of  the traces of  $x_i$'s means any
polynomial in $x_1,\ldots,x_k$. This, i.e., the 
general $\#P \not = NC$ conjecture in characteristic zero, 
cannot be proved unconditionally at present.
But the next case of this implication,  $n>1$ and $k$ arbitrary, can be:

\vfil \eject 
\begin{theorem}[GCT1,2,6]

\noindent {\bf (A mathematical form of the  $\#P \not = NC$ conjecture)}
 \label{tgenweaklec1}

The implication above holds unconditionally for any $n>1$ and arbitrary $k$.

In fact, something stronger then holds. Namely, 
when  $n>1$ and $k$ is arbitrary, no generalized permanent $p(X_1,\ldots,X_k)$
can be expressed as a polynomial function of the traces of 
$\bar X_i^j$, $1 \le i \le k$, $j \ge 0$,  where 
$\bar X_i=B_i X_i C_i$,  $i \le k$,  for any $n\times n$ complex (possibly
singular) matrices $B_i$ and $C_i$.
\end{theorem}

When  $k=1$ and $p(X_1)$ is the usual permanent, this specializes to
Proposition~\ref{pweaklec1}.


We are calling this a mathematical form for two reasons. 
First, it needs  no restriction on the computational complexity of
$p(X_1,\ldots,X_k)$ or the polynomial in the traces,
(though for trivial reasons
we can assume without loss of generality that 
the polynomial in the traces is computable in $2^{\poly(n,k,d)}$ time, 
where $d$ is  the degree of $p$). 
Thus it is rather in the spirit of the classical result of Galois theory 
which says that a  polynomial  whose Galois group is not
solvable cannot be solved by any number of
radical operations, without any restriction on the number of such
operations (though again there is a trivial  upper bound on the number of
such operations needed if the polynomial is solvable by radicals). 
Second, observe that 
the permanent has two characteristic properties: 1) the property 
P (mathematical), and 2) $\#P$-completeness (complexity-theoretic). 
The usual complexity theoretic form of the $\#P\not = NC$ conjecture
is a lower bound for  all polynomial functions with 
the  $\#P$-completeness property, whereas the mathematical form 
is  a lower bound for all polynomial functions with the 
property (P).  In other words,  the complexity theoretic form
is associated with the $\#P$-completeness property of the
permanent and the mathematical form with 
the mathematical property (P). 




The result indicates that there is thus a chasm
between the two adjacent cases: $n=1$, $k$ arbitrary (the usual nonuniform
complexity theoretic $\#P \not = NC$ conjecture), and 
$n=2$, $k$ arbitrary (its mathematical form above). 
The complexity theoretic form is   much harder than the mathematical
form, and  a proof technique for the easier mathematical form
can be expected to give us a crucial insight into what is needed to prove 
the harder  complexity theoretic form.


For some specific
generalized permanents (cf. Section~\ref{sweak}), this result again has
an elementary naturalizable proof as in \cite{boris}.
It also has an elementary naturalizable proof for a generic 
generalized permanent, just as the fact that a generic polynomial is
hard to compute has an elementary naturalizable proof.
The nontrivial part of this 
result (which needs nonelementary proof) 
is that it holds for any generalized permanent.
Indeed the basic difference between the complexity theoretic 
and the mathematical  settings is
the following. The complexity theoretic  (i.e. the usual) $\#P \not = NC$
conjecture 
is complete in the sense 
that if it is proved for one $\#P$-complete function (say
the permanent), it automatically 
holds for all $\#P$-completeness functions (because
of the theory of $\#P$-completeness). But there is no such completeness
theory at the mathematical level. Hence, a mathematical
lower bound  for a specific 
generalized permanent, e.g., the permanent,
does not say anything about all (even $\#P$-complete)
generalized permanents. To get 
similar completeness,   the  mathematical
form of the $\#P\not = NC$ conjecture above  covers up this lack of 
completeness theory
at the mathematical level by proving a result for all polynomial functions
with property (P), not just a specific one. 
The articles \cite{boris,ressayre} suggest that without such completeness
a restricted weaker form of the $\#P\not =NC$ conjecture
may be  provable by  a naturalizable proof technique. 



In contrast, it may be conjectured that Theorem~\ref{tgenweaklec1} cannot 
be proved by a naturalizable technique. This is because 
the only thing that is common among  all generalized permanents is the
property (P).  Hence any proof of this result would be 
essentially  forced
to rely only on  this property like  its GCT proof (cf. Section~\ref{sweak}).
Any such proof automatically passes the natural proof 
barrier since it is easy to show [GCT6] that most functions do not
have property (P) when $n>1$ and $k$ is arbitrary.
\ignore{It may be remarked that the algebraic degree barrier is not 
applicable in the permanent vs. determinant problem because both
permanent and determinant have the same degree. It is not applicable
in the context of Theorem~\ref{tgenweaklec1} as well for the same reasons.
Similarly, the relativization barrier is not applicable in the context
of the permanent vs. determinant problem because the $NC$-computation 
has been algebrized in it in the form of the determinant, and the
relativization barrier does not apply to such algebraic techniques 
(just as it does not apply to the proof of the 
$IP=PSPACE$ result).
The relativization barrier does not apply in the context of 
Theorem~\ref{tgenweaklec1} 
for the same reason. Thus it can be said that the proof technique of
Theorem~\ref{tgenweaklec1} crosses the
natural proof, algebraic degree (algebrization)
and relativization barriers simultaneously.

Ultimately, any approach to the $\#P \not = NC$ conjecture
is expected to prove some restricted
form of this conjecture, not necessarily Theorem~\ref{tgenweaklec1},
whose proof crosses these barriers simultaneously.
At present, we do not have any other lower bound  result of this kind.}



Though the statement of Theorem~\ref{tgenweaklec1} is elementary, its proof 
is nonelementary and is based on  some fundamental results 
in geometric invariant theory \cite{kempf,mumford} and
the results in GCT1 and 2 
based on these results. These nonelementary techniques
are needed to cope up with the  nontrivial underlying difficulties in
the problem explained in Section~\ref{sweak}. 




\section{From nonexistence to existence}
The rest of this lecture  outlines  the GCT approach to 
the general  permanent vs. determinant problem,
and then  points out 
the crucial steps in this plan which can be completely executed
for the   mathematical form  of the $\#P\not = NC$ conjecture above,
but which are conjectural at present for 
the general (i.e. complexity theoretic) permanent vs. determinant problem. 

The first  step 
(GCT1,2) is to reduce this nonexistence problem--i.e., that there is no
small linear representation  of the permanent as a determinant--to
an existence problem--specifically, to the problem of proving 
existence of a family $\{O_n\}$ of obstructions; 
cf. Figure~\ref{fig:firststep}.
Here an {\em obstruction} $O_n$ is a proof-certificate of
hardness of $\perm(X)$, $X$ an $n\times n$ variable matrix,
just as the Kurotowski minor is a proof-certificate of the nonplanarity of a 
graph.  Specifically,  it is some 
algebro-geometric-representation-theoretic gadget
whose existence for every $n$  serves as a 
guarantee that $\perm(X)$ cannot be represented linearly as $\det(Y)$,
when $m=2^{\log^a n}$, $a>0$ fixed, $n\rightarrow \infty$ (i.e., for
$n$ greater than a large enough constant depending on $a$). 



\begin{figure} 
\begin{center}\psfragscanon
\psfrag{on}{$\{O_n\}$}
\epsfig{file=firststep.eps, scale=.8}
\end{center}
      \caption{Reduction from nonexistence to existence}
      \label{fig:firststep}
\end{figure}



This reduction to existence is carried out as follows (cf. lecture 2 for 
details).


First, we associate (GCT1) with 
the complexity class $\#P$ a family $\{X_{\#P}(n,m)\}$ of (group-theoretic)
class varieties (what this means is explained below),
and with the complexity class $NC$ a family of 
$\{X_{NC}(n,m)\}$ of (group-theoretic) class varieties such that: 
if $\perm(X)$, $\dim(X)=n$, can be represented linearly 
as $\det(Y)$, $\dim(Y)=m>n$, then 

\begin{equation} \label{eqembed} 
X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation} 

Each  class variety is a  (projective) algebraic variety, by which
we mean that it is the zero set of  a system of multivariate 
homogeneous polynomials with coefficients in $\C$  (akin to the 
usual curves  and surfaces). It is  group-theoretic in the 
sense that it is  constructed using group-theoretic operations 
and the general linear group $G=GL_l(\C)$, $l=m^2$, of $l\times l$ invertible
complex matrices acts on it, and furthermore the groups of
symmetries of the permanent and the determinant, which we shall
refer to as $G_{perm}$ and $G_{det}$,  are embedded in this group $G$
as its subgroups in some way. Here action means moving the points 
of the class variety around, just as $G$ moves the points of $\C^l$ around 
by the standard action via invertible linear transformations.
The goal is to show that the inclusion (\ref{eqembed}) is impossible
(obstructions are meant to ensure this);
cf. Figure~\ref{fig:class}. 

\begin{figure} 
\begin{center} \psfragscanon
\psfrag{xsharp}{$X_{\#P}(n,m)$}
      \psfrag{xnc}{$X_{NC}(n,m)$}
      \psfrag{g}{$G=GL_l(\C)$, $l=m^2$}
      \psfrag{Obstruction}{\mbox{Obstruction}}
\epsfig{file=class.eps, scale=.5}
\end{center}
      \caption{Class varieties}
      \label{fig:class}
\end{figure} 



Since each class variety has a $G$-action, the space of polynomial functions 
on each class variety has a  representation-theoretic structure, which 
puts constraints on which  representations of $G$ can live on that variety
(i.e., in the space of polynomial  functions on that variety).
Informally, an obstruction is an irreducible (minimal)  representation of $G$
that can live on $X_{\#P}(n,m)$ but not on $X_{NC}(n,m)$; 
cf. Figure~\ref{fig:class}.
Existence of  an obstruction $O_n$, for every $n$, assuming
$m=2^{\log^a n}$, $a>1$ fixed, implies  that the inclusion (\ref{eqembed}) 
is not possible, since  $O_n$ cannot live  on $X_{NC}(n,m)$.
Thus  an obstruction blocks the inclusion (\ref{eqembed}).


To define an obstruction formally, we need to recall some basic representation
theory.  By a classical result of Weyl, the irreducible 
(polynomial) representations of $G=GL_l(\C)$ are in one-to-one correspondence 
with the partitions  $\lambda$ of length  at most $l$, by which we mean 
integral sequences $\lambda_1 \ge 
\lambda_2 \cdots \ge \lambda_k > 0$, $k \le l$,
where  $k$ is called the  length
of $\lambda$. The irreducible 
representation of $G$ in correspondence with $\lambda$ is denoted 
by $V_\lambda(G)$, and is called the {\em Weyl module} of $G$ indexed by 
$\lambda$. Symbolically:

\[\mbox{Irreducible representations of } G \stackrel{\mbox{Weyl}}{\Longleftrightarrow} \quad \mbox{partitions} \ \lambda. \]  

\[\mbox{Weyl module  } V_\lambda(G)  \longleftrightarrow \lambda. \] 
Weyl also proved that every finite dimensional representation of $G$ 
can be decomposed into irreducible representations--i.e.,
can be written as a direct sum of Weyl modules. Thus Weyl modules 
are the basic building blocks of the representation theory of 
$G$, and every finite dimensional representation of $G$ can be thought
of as a complex building made out of these blocks. 


Now suppose $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$. 
Suppose to the contrary that 

\begin{equation} \label{eqembed2}   X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation}

Let $R_{\#P}(n,m)$ denote the homogeneous coordinate ring of 
$X_{\#P}(n,m)$; i.e., the ring of polynomial functions 
\footnote{Though the  functions here are not functions in usual sense;
but let us  not worry about this} on $X_{\#P}(n.m)$. 
Let $R_{\#P}(n,m)_d$ be the degree-$d$-component of $R_{\#P}(n, m)$ consisting
of functions of degree $d$. We define $R_{NC}(n,m)$ and $R_{NC}(n,m)_d$
similarly. Since $X_{\#P}(n,m)$ has the action of $G$, $R_{\#P}(n,m)$ 
also has an action of $G$; i.e., it is a representation of $G$. Hence,
$R_{\#P}(n,m)_d$ is a finite dimensional representation of $G$. 
Similarly, $R_{NC}(n,m)$ is a representation of $G$, and $R_{NC}(n,m)_d$
a finite dimensional representation of $G$. 



If (\ref{eqembed2}) holds, then we get a natural map from $R_{NC}(n,m)$ to
$R_{\#P}(n,m)$ obtained by restricting a function on $X_{NC}(n,m)$ to
$X_{\#P}(n,m)$. %; cf. Figure~\ref{fig:restriction}.
By basic algebraic geometry, this map
is surjective and is a $G$-homomorphism.
Furthermore, it is degree-preserving. This means there
is a surjective $G$-homomorphism from $R_{NC}(n,m)_d$ to 
$R_{\#P}(n,m)_d$. Symbolically: 

\begin{equation} \label{eqsurjection}
R_{\#}(n,m)_d \leftarrow  R_{NC}(n,m)_d.
\end{equation}

\ignore{
\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{Xp}{\small $X_{\#P}(n,m)$}
\psfrag{Xnc}{\small $X_{NC}(n,m)$}
\epsfig{file=restriction.eps, scale=.6}
\end{center}
      \caption{Restriction}
      \label{fig:restriction}
\end{figure}
}

Let $R_{\#P}(n,m)_d^*$ denote the dual of $R_{\#P}(n,m)_d$; i.e., the 
set of linear maps from $R_{\#P}(n,m)_d$ to $\C$. Then (\ref{eqsurjection})
implies that there is an injective $G$-homomorphism from 
$R_{\#P}(n,m)^*_d$ to $R_{NC}(n,m)^*_d$. Symbolically: 

\begin{equation} \label{eqinclusion}
R_{\#}(n,m)_d^*  \hookrightarrow {NC}(n,m)_d^*.
\end{equation}

\begin{defn} (GCT2)
An obstruction $O_n$ is a Weyl module $V_\lambda(G)$ that 
occurs as a subrepresentation 
in $R_{\#P}(n,m)_d^*$  but not in $R_{NC}(n,m)_d^*$, for some $d$. 
We call $\lambda$ an {\em obstruction label}, and sometimes,
by abuse of notation, an obstruction as well.

A strong obstruction $O_n$ is a Weyl module $V_\lambda(G)$ 
that occurs as a subrepresentation in $R_{\#P}(n,m)_d^*$ but 
does not contain a nonzero 
invariant (fix point) of the subgroup $G_{det} \subset G$ of the symmetries 
of the determinant.
It can be shown \cite{GCT2} that a strong obstruction
is an obstruction in the above sense.
\end{defn}

Here by  an invariant we mean a point in $V_{\lambda}(G)$ 
which is fixed (does not move) with respect to the action of the subgroup
$G_{det} \subset G$.

\begin{prop} (GCT2)
Existence of an obstruction $O_n$, for all $n\rightarrow \infty$, 
with $m=2^{\log^a n}$, $a>1$ fixed, implies $\perm(X)$, $\dim(X)=n$, 
cannot be represented linearly as 
$\det(Y)$, $\dim(Y)=m$. 
\end{prop}

This   follows just from the definition of an obstruction, and 
leads to:

\begin{goal} \label{gobs} (GCT2)
Prove existence of a (strong) 
obstruction family $\{O_n=V_{\lambda_n}(G)\}$ using 
the  exceptional 
nature of $\perm(X)$ and $\det(Y)$, i.e., using the 
properties (P) and (D) in  Section~\ref{scharsym}.
\end{goal} 

\section{Obstructions for the mathematical form} \label{sobsweak}

The following result achieves this goal for the mathematical form
(Theorem~\ref{tgenweaklec1}).
\begin{theorem} 
There exists a (strong)  obstruction family $\{O_n\}$ for the mathematical
form  of the $\#P \not = NC$ conjecture.
\end{theorem}

This implies Theorem~\ref{tgenweaklec1}.
The notion of obstructions here is similar 
to the one in the general case. 

The proof of this result  based on the results of GCT1 and 2 in
geometric invariant theory \cite{mumford} is outlined in the third lecture.
It produces  a 
family $\{O_n=V_\lambda(G)\}$ of (strong) obstructions, with a different $G$
than in the general complexity theoretic case.
Furthermore this family  is {\em strongly explicit} in the sense  that 
the specification $\lambda_n$ of each $O_n$
has polynomial, in fact,  $O(n)$ bitlength, and  
can be constructed in polynomial, in fact, $O(n)$ time (regardless of the 
complexity  of the polynomial in the traces in the statement of 
Theorem~\ref{tgenweaklec1}).

\ignore{\noindent {\em Remark:}
There is also a second nonconstructive proof of this result 
(cf. Section~\ref{sweak}).
This gives a concrete evidence 
that explicit construction is not needed to cross the 
natural proof   barrier. Because 
any proof that relies only on the property (P) automatically
bypasses this barrier, as remarked before.
But   this nonconstructive
proof is not any easier than the explicit proof.
Indeed, the whole proof
structure  here is such that its easiest implementation  yields 
obstructions explicitly 
whether one cares for them or not. We shall see the same phenomenon
in the general case in what follows.
}

\section{Towards existence of obstructions in general via positivity}
We now proceed to describe the main results of GCT for the general
(complexity-theoretic)
permanent vs. determinant problem in the context of
Goal~\ref{gobs}. 



Towards that end, we  define 
certain representation-theoretic {\em stretching} functions. 
Let $F_{\lambda,n,m}(k)$ denote the number of occurences (multiplicity)  of
the Weyl module $V_{k\lambda}(G)$ in $R_{\#P}(n,m)^*$ (i.e. 
$R_{\#P}(n,m)^*_d$, for some $d$)  as a subrepresentation.
Let $G_{\lambda,m}(k)$ denote the multiplicity of the trivial one dimensional
representation (invariant) of $G_{det} \subset G$ in 
$V_{k\lambda}(G)$. In other words, $G_{\lambda,m}(k)$ is the dimension
of the subspace of invariants of $G_{det}$ in $V_{k \lambda}(G)$.
These are statistical functions
associated with the class variety $X_{\#P}(n,m)$ 
and the subgroup embedding  $G_{det} \hookrightarrow  G$.
In the first case,  the statistics associates 
with every number (stretching parameter) $k$  
the multiplicity of the corresponding
Weyl module $V_{k\lambda}(G)$ in $R_{\#P}(n,m)^*$ and in the second 
case the dimension of the subspace of invariants of the symmetries of the
determinant in $V_{k \lambda}(G)$; cf. Figure~\ref{fig:statistics}.

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{l}{$\lambda$}
\psfrag{2l}{$2 \lambda$}
\psfrag{3l}{$3 \lambda$}
\psfrag{v1}{$V_\lambda(G)$}
\psfrag{v2}{$V_{2 \lambda}(G)$}
\psfrag{v3}{$V_{3\lambda}(G)$}
\epsfig{file=statistics.eps, scale=1}
\end{center}
      \caption{statistics}
      \label{fig:statistics}
\end{figure}


Let us  call a function $f(k)$ {\em quasipolynomial}, if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k)$ for all nonnegative integral $k=i$ modulo $l$;
here  $l$ is
called the period of the  quasi-polynomial. 
Thus  quasi-polynomials
are hybrids of  polynomial and periodic functions. 
We say that $f(k)$ is an 
{\em asymptotic quasipolynomial} if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k)$ for all nonnegative integral $k=i$ modulo $l$ for 
$k\ge a(f)$, for 
some nonnegative integer depending on $f$. The minimum 
$a(f)$ for which this holds is called the {\em deviation from 
quasipolynomiality}. Thus $f(k)$ is a (strict) quasipolynomial when this
deviation is zero.

A fundamental example of a quasi-polynomial is the Ehrhart quasi-polynomial
$f_P(k)$ of a polytope $P$ with rational vertices. It is defined
to be the number of integer points in the dilated polytope $kP$. By the 
classical result of Ehrhart, it is known to be a quasi-polynomial.
More generally, let $P(k)$ be a polytope parametrized by nonnegative
integral $k$: i.e., 
defined by a linear system of the form: 
\begin{equation} \label{eqpara}
A x \le k b + c,
\end{equation}
where $A$ is an $m \times n$ matrix, $x$ a variable $n$-vector, and 
$b$ and $c$ some constant $m$-vectors. Let $f_P(k)$ be the number 
of integer points in $P(k)$.  It is known to be  an asymptotic
 quasi-polynomial. We shall call it the asymptotic 
Ehrhart quasi-polynomial  of the parametrized polytope $P(k)$. 
In what follows, we  denote a parametrized polytope $P(k)$ by 
just $P$. 
From the context it should be clear whether $P$ is a usual nonparametrized 
polytope or a parametrized polytope.









\begin{theorem} (GCT6) \label{tquasi}

\noindent (a) The  function $G_{\lambda,m}(k)$ is a quasi-polynomial.


\noindent (b) The function $F_{\lambda,n,m}(k)$ is 
an asymptotic quasi polynomial.

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem} 


The proof of Theorem~\ref{tquasi} is based on:
\begin{enumerate} 
\item The classical work of Hilbert in invariant theory, 
\item The 
resolutions of singularities in characteristic zero
\cite{hironaka}: 
this  roughly says 
that the singularities of any algebraic variety in characteristic zero
can be untangled (resolved) nicely in a systematic fashion; cf.
 Figure~\ref{fig:resolution}.
\item Cohomological works of Boutot, Brion,  Flenner, Kempf  and others
based on this resolution; cf.  \cite{boutot,dehy} and
GCT6 for the history and other references.
\end{enumerate} 


\begin{figure} 
\begin{center} 
\epsfig{file=resolution.eps, scale=.5}
      \caption{Resolution}
      \label{fig:resolution}
\end{center}
\end{figure}


As such, this proof is highly nonconstructive. It gives no effective
bound on the period $l$--it just says that $l$  is finite.

\noindent {\em Remark:} 
The original IAS lecture   stated a conditional form of (b),
which said that $F_{\lambda,n,m}(k)$ is a quasi-polynomial if the
singularities of the class variety $X_{\#P}(n,m)$ are rational and normal 
(in some algebro-geometric sense). 
Recently, Shrawan Kumar  \cite{shrawan}  has shown that 
the singularities of $X_{\#P}(n,m)$ are not normal if $m>n$. This means 
$F_{\lambda,n,m}(k)$ need not be  a quasi-polynomial and 
asymptotic quasi-polynomiality as in  (b) is all that we can expect.
This is fine 
as long as the singularities of $X_{\#P}(n,m)$ are not too bad 
in the sense described in Remark 3  after Hypothesis~\ref{hph1} below.

The following hypothesis 
says that $G_{\lambda,m}(k)$  can be realized as the Ehrhart quasi-polynomial
of a polytope, and 
$F_{\lambda,n,m}(k)$ 
can be realized as the asymptotic Ehrhart quasi-polynomial 
of a parametrized  polytope.

\begin{hypo} {\bf (PH) [Positivity Hypothesis]} \label{hph} (GCT6)

\noindent (a) For every $\lambda,n,m\ge n$, 
there exists   a parametrized  polytope $P=P_{\lambda,n,m}(k)$ 
such that 
\begin{equation} \label{eqP}
F_{\lambda,n,m}(k)=f_P(k).
\end{equation} 
It is also assumed here that there exists for $P_{\lambda,n,m}$ a specification
of the form (\ref{eqpara}),
 where $A$ is independent of $\lambda$, and $b$ and $c$ 
are  piecewise homogeneous linear functions of $\lambda$.


\noindent (b) For every $m$, there exists a (usual nonparametrized) 
polytope  $Q=Q_{\lambda,m}$  such that
\begin{equation} \label{eqQ}
G_{\lambda,m}(k)=f_Q(k).
\end{equation}
It is assumed here that there exists for $Q_{\lambda,m}$ a 
specification of the form (\ref{eqpara}) with $k=1$ and $c=0$  
where $A$ is independent of $\lambda$, and $b$ is 
is a  piecewise homogeneous linear function of $\lambda$.




Analogous positivity hypothesis also holds 
for the $P$ vs. $NP$ problem in characteristic zero.
\end{hypo} 



If such $P$ and $Q$ exist, their dimensions are guaranteed to be
small by the proof of Theorem~\ref{tquasi}: specifically,
the dimension $P$ is guaranteed to be bounded by a 
polynomial in $n$, and the dimension of $Q$ 
by a polynomial in $n$ (but independent 
of $m$), if the length of $\lambda$ is $\poly(n)$ (as it would be in 
our applications).






When PH holds, we say that $F_{\lambda,n,m}(k)$ and 
$G_{\lambda,m}(k)$ have  {\em positive convex representations}. 
Here positivity refers to the fact that the Ehhart function 
$f_P(k)$ is a positive expression:
\[ f_P(k)=\sum_{v} 1,\] 
where $v$ ranges over all integer points in $P(k)$--there are no 
alternating signs in this expression.
Convexity refers to the  convexity of the polytopes $P(k)$ and $Q$. 


But, a  priori, it is not at all clear why PH should  even hold. 
Many numerical functions in mathematics are quasi-polynomials 
or asymptotic quasi-polynomials (e.g., the Hilbert function 
\footnote {Hilbert function $h_Z(k)$ of a projective algebraic variety $Z$
is defined to be $\dim(R(Z)_k)$, where $R(Z)$ is the homogeneous coordinate 
ring of $Z$ and $R(Z)_k$ its degree $k$-component.} of any projective
variety), but they rarely have positive convex representations.
PH is expected to hold 
because of the exceptional nature of the determinant and the permanent. 
For concrete  mathematical evidence and justification, see  GCT6,7, and 8. 


The hypothesis 
PH alone is not sufficient to prove the existence of obstructions.
The precise statement of a sufficient condition is given in 
the theorem below.




\begin{theorem} (GCT6) \label{tgct6}
There exists a family $\{O_n\}$ of (strong) obstructions 
for the  $\#P$ vs. $NC$ problem in characteristic zero, 
for $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$, 
assuming, 

\begin{enumerate} 
\item PH, and
\item OH (Obstruction Hypothesis): 

For all $n\rightarrow \infty$,  there exists $\lambda$ such that 
$P_{\lambda,n,m}(k) \not = \emptyset$ for all large enough $k$ and
$Q_{\lambda,m}=\emptyset$.
\end{enumerate}

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem}

Mathematical evidence and arguments in support of OH are given in GCT6.
The analogous OH that arises in the context of the mathematical form
of the $\#P\not = NC$ conjecture can be  proven unconditionally.

We call  $\lambda$ a {\em polyhedral  obstruction}
(or rather, polyhedral  obstruction-label)
if it satisfies OH. In this case, $k\lambda$, for some integer $k\ge 1$ is
a (strong)  obstruction--we just have to choose $k$ large enough 
so that 
$P_{\lambda,n,m}(k)$ contains an integer point.
Henceforth, whenever we say obstruction, we actually mean polyhedral
obstruction.

There is a fundamental difference between the nature of PH and OH.
PH is a {\em mathematical hypothesis}, because there is no 
constraint on what $m$ should be in comparison to $n$ in its statement.
In contrast, OH is a {\em complexity theoretic hypothesis}, because 
$m$ needs to be small in comparison to $n$ for it to hold.


%\subsection{Why should PH  and OH hold?} 

%Mathematical evidence for this is given in GCT2,4,6,7,8.
%We shall discuss some of this  in the third lecture.


\section{The flip: Explicit construction of obstructions} 
\label{sflip}
In principle PH may have a nonconstructive proof (like that
of Theorem~\ref{tquasi})  which only tells  that such polytopes 
exist without explicitly constructing them. But proving OH may not be feasible
unless the polytopes $P$ and $Q$ in PH are given explicitly.
This  suggests the following strategy for proving 
existence of obstructions proposed in  GCT6 and  GCTflip.


\noindent (1) Prove the following stronger explicit form 
of PH, which is reasonable since the polytopes $P$ and $Q$, if they exist,
are already guaranteed to be of small (polynomial) dimension:

\begin{hypo} {\bf (PH1)}  \label{hph1} (GCT6)

\noindent (a) There exists an {\em explicit} 
parametrized polytope $P_{\lambda,n,m}=P_{\lambda,n,m}(k)$ 
as in  PH (a).
Explicit means: 

\begin{enumerate}
\item  The polytope is specified by an explicit system of linear constraints,
where the bitlength of (the description of) 
each constraint is  $\poly(n,\bitlength{\lambda}, \bitlength{m})$.
Here and in what follows, $\bitlength{z}$ denotes the bitlength of the 
description of $z$.

\item  The membership problem for the polytope
$P_{\lambda,n,m}(k)$  also 
belongs to the complexity class $P$.
That is,  given a point $x$, whether it belongs to $P_{\lambda,n,m}(k)$ 
can also be decided in $\poly(\bitlength{x},\bitlength{\lambda},
n,\bitlength{m})$
time.
Furthermore, we assume that if $x$ does not belong to the polytope,
then the membership algorithm also gives a hyperplane separating 
$x$ from the polytope in the spirit of \cite{lovasz}. 
\end{enumerate} 

\noindent (b) There exists a similar  explicit 
(nonparametrized) polytope $Q_{\lambda,m}$  satisfying   PH (b)
with the polynomial bounds that 
depend on $n$ and the bitlength of $\lambda$, but not on $m$.
\end{hypo}

\noindent {\em Remark 1:} 
Note the occurrence of  $\bitlength{m}$  instead of $m$ in the polynomial
bounds in (a) (which implies that the bounds here become $\poly(n)$
when $m<2^n$ and $\bitlength{\lambda}=\poly(n)$), and the absence 
of $m$ in the polynomial bounds in (b), which means they again are 
$\poly(n)$ when  $\bitlength{\lambda}=\poly(n)$).
The reasons for this will be explained in Lecture 3 
(cf. remarks before Hypothesis~\ref{hph1tilde} and 
after Hypothesis~\ref{hph1restatement}). 



\noindent {\em Remark 2:} 
In particular, PH1 implies that the functions $F_{\lambda,n,m}(k)$ and
$G_{\lambda,m}(k)$ belong to the complexity class $\#P$. 

\noindent {\em Remark 3:} PH1 
also implies that the deviation from quasipolynomiality 
of $F_{\lambda,n,m}(k)$ is small, specifically, 
$2^{O(\poly(\bitlength{\lambda},n,\bitlength{m}))}$, i.e.,  the bitlength
of the deviation is polynomial.  As remarked after Theorem~\ref{tquasi},
this deviation would have been zero, i.e., $F_{\lambda,n,m}(k)$ would
have been a (strict) quasi-polynomial, if the singularities of the class
variety $X_{\#P}(n,m)$ were all normal and rational, which, as we know now,
is not the case \cite{shrawan}. So small deviation from quasi-polynomiality
implied by PH1 
basically means that the deviation from rationality and normality of
the singularities
of the class variety $X_{\#P}(n,m)$ is small (cf. Theorem~\ref{tquasi}).
This is the basic minimum that is required by PH1.


Like PH, PH1 is also a mathematical hypothesis in the sense that
it puts  no constraint on what $m$ should be in comparison to $n$. 
Of course, unlike PH, there is some complexity theoretic aspect to it, 
but it is secondary in comparison to the complexity-theoretic aspect of 
OH, since smallness  of $m$ with respect to  $n$ is the 
crux of the lower bound  problems under consideration. 





\noindent (2a) {\bf [The flip]}

Let $m=2^{\log ^a n}$, for a fixed $a>1$. 
Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
show existence of  an {\em explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of (polyhedral) obstructions  satisfying OH. 
We say that an obstruction (proof-certificate) 
$\lambda_n$ is {\em explicit} if is ``short'' and ``easy to verify'':


\begin{enumerate} 
\item  Short: This means its bitlength $\bitlength{\lambda_n}$ 
is $\poly(n)$,
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  

\item Easy to verify: given $n, m \le 2^{n}$ and 
$\lambda_n$, whether 
$\lambda_n$ is a valid polyhedral obstruction 
can be verified 
in $\poly(n,\bitlength{\lambda})$ time. In particular, this is
$\poly(n)$ when $\bitlength{\lambda}=\poly(n)$. 
\end{enumerate}

Existence of an explicit family of polyhedral 
obstructions is equivalent to saying
that the problem of deciding existence of polyhedral obstructions
for given $n$ in unary and $m$ in binary 
belongs to $NP$--we shall refer to this decision problem as $DP(OH)$.
This definition of explicitness is quite natural since the class $NP$ 
is a class of problems whose proof-certificates (witnesses) are 
short and easy to verify. As such, the flip--going for 
explicit  obstructions--is
a proof-strategy that is literally given to us on a platter 
by the $P$ vs. $NP$ 
problem itself. Why it is called flip will be explained later.


It should be stressed that we are primarily interested in only proving 
existence of obstructions. Whether they are explicit or not 
does not really matter in the original statement of the problem.
But we need to know the polytopes $P$ and
$Q$ explicitly (as in PH1)  so that proving OH is feasible. 
%In other words,   if we do not
%even know what the polytopes $P$ and $Q$ look like, 
%it seems unlikely that anything  could be said regarding OH. 
But once  PH1 is proved, existence of an explicit family follows
automatically,   as a bonus, whether we care for it or not. 

To see why, let us observe that 
the second condition above  (ease of verification) follows directly
from PH1 and the polynomial time algorithm for 
linear programming on  polytopes given by separation oracles \cite{lovasz}. 
Shortness  also follows from PH1. 

Thus it is as if the $P$ vs. $NP$ problem is forcing us to go
for explicit obstructions.


\noindent (2b) {\bf [The strong flip (optional)]} 

Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
construct (rather than just show existence of) 
a {\em strongly explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of obstructions  satisfying OH. We say that an explicit family 
of obstructions is strongly explicit if,
for each $n$, a valid obstruction-label
$\lambda_n$ can be constructed in $\poly(n)$ time.
In particular, the height and the bitlength of
 $\lambda$ is $\poly(n)$ (short) 
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  


For the purposes of the lower bound problems that we are interested in, the
flip (just explicit  
existence) would suffice and the stronger flip (explicit construction)
is optional. But the stronger flip can give us deeper insight into these
lower bound problems; cf. \cite{GCTexplicit} and GCTflip for more on this.

Now we turn to a few obvious questions.



\section{What has been achieved by all this?: The meaning of the flip} 
\label{smeaning}
Let us now see what has been achieved so far
in the context of the 
$\#P\not = NC$ conjecture in the nonuniform setting (characteristic zero),
the argument for the $P$ vs. $NP$ problem in characteristic zero
being  similar. 
At  first glance,
it may seem that all that GCT has achieved 
is to exchange a known difficult problem of 
complexity theory with a new very difficult problem of algebraic geometry.
In order to see that something is gained in exchange let us reexamine the 
original question.

The goal of the original  conjecture is to prove that 
$\perm(X)$, $\dim(X)=n$,  cannot be computed by an arithmetic circuit $C$
of size $m=\poly(n)$, or more generally,
$m \le 2^{\log^a n}$, for some fixed $a>1$, and depth $O(\log^a n)$.
Symbolically, 
let  $f_C(X)$ denote the function computed by $C$. Then we want to prove that
\begin{equation} \label{eqioh} 
 {\bf (IOH):}  \forall n \ge n_0 \forall C \exists X:
\perm(X)\not = f_C(X),
\end{equation} 
where $n_0$ is a sufficiently large constant and $C$ ranges over 
circuits of size $m=\poly(n)$.
For given $X$ and $C$, the problem 
of deciding if  $\perm(X) \not = f_C(X)$
belongs to  $P^{\#P}$.  Let $DP(IOH)$ denote the decision problem 
of deciding for given $n$ and $m$ (in unary) whether 
(\ref{eqioh}) holds with $C$ ranging over circuits of size $m$.
Since there are two alternating layers of quantifiers in (\ref{eqioh}), it
belongs to $\Pi_2^{\#P}$, which is very high in the complexity hierarchy
(cf. Figure~\ref{fig:IOHcomplexity}).
Hence, we  refer to the original hypothesis (\ref{eqioh}) 
to be proven  as IOH 
(Infeasible Obstruction Hypothesis). Of course, IOH is expected to 
be a tautology, and hence (\ref{eqioh})
is expected to  be verifiable for small  $m=\poly(n)$ 
in $O(1)$ time--but
we do not know that as yet. 



\begin{sidewaysfigure} 
\begin{center}
\psfragscanon
\psfrag{sigma2p}{{\small $\Pi_2^{\#P}$}}
\psfrag{sigma1p}{$\Sigma_1^{\#P}$}
\psfrag{P}{{\small $P$}}
\psfrag{NP}{{\small $NP$}}
\psfrag{T}{$T$}
\psfrag{#P}{$\# P$}
\psfrag{inNP}{$DP(OH) \in NP$}
\psfrag{inP}{$DP(POH) \in P$}
\psfrag{insigma2p}{$DP(IOH) \in \Pi_2^{\#P}$}
\psfrag{PHplus}{PH1}
\psfrag{PHtil}{$PH^\dagger$}
\epsfig{file=IOHcomplexity.eps, scale=.8}
\end{center}
      \caption{Positivity as a means to eliminate the quantifiers and 
reduce the complexity of the  decision problem associated 
with the obstruction hypothesis}
      \label{fig:IOHcomplexity}
\end{sidewaysfigure}



Equivalently, the goal of IOH 
is to prove existence of a {\em trivial obstruction},
which is a table that lists for each small $C$
as above a counterexample  $X$ so that
$\perm(X)\not = f_C(X)$; cf. Figure~\ref{fig:trivial}.
The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$ and depth
$O(\log^a n)$. Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. (Well, only
if the underlying field of computation is finite. For infinite fields, 
such as $\Q$ or $\C$ in this paper, 
there is another notion of a trivial obstruction (cf. 
GCT6). But let us imagine that the underlying
field is finite for this argument.)
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time to decide if such a table exists and construct 
one (optional) for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. That is why we 
call  this trivial, brute force 
strategy of proving IOH, based on existence of trivial obstructions,
an {\em infeasible strategy}. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{eq}{$\perm(X)\not = f_C(X)$}
\epsfig{file=trivial.eps, scale=.5}
\end{center}
      \caption{A trivial obstruction}
      \label{fig:trivial}
\end{figure}


In contrast, assuming PH1, $DP(OH)$, the decision 
problem  of deciding if a new polyhedral obstruction exists, belongs 
to $NP$ (in a stronger sense assuming that $n$ is given in unary but
$m$ is given in binary
instead of unary) as we have already observed. Thus, assuming PH1, we have 
transformed the original decision problem for trivial obstructions
$DP(IOH) \in \Pi_2^{\#P}$ to the  decision problem for the  new polyhedral 
obstructions $DP(OH) \in NP$,
in the process bringing down the time to verify an obstruction
from  exponential (for the original trivial obstruction) to polynomial
(for the new polyhedral obstruction); cf. Figure~\ref{fig:IOHcomplexity}.  
It is crucial here that PH1, the main tool for this reduction, is a 
mathematical hypothesis,  not complexity-theoretic (cf. the remarks
after Theorem~\ref{tgct6} and Hypothesis~\ref{hph1}).
The task of verifying  an obstruction has also been 
transformed from the infeasible (exponential-time) to the feasible 
(polynomial-time). Hence the name of this strategy: the flip,
from the infeasible to the feasible.
Positivity (PH1) is used in the flip as a means  to
eliminate the quantifying variables in IOH and bring down the 
complexity of the decision problem associated with the obstruction hypothesis;
cf. Figure~\ref{fig:IOHcomplexity}. 




This process can be extended further. Assuming an additional
positivity hypothesis PH4 specified below,
$OH$, whose associated decision problem  $DP(OH)$ belongs to $NP$,
can be transformed 
to POH (Positivity Obstruction Hypothesis),  whose associated
decision problem $DP(POH) \in P$; i.e.,  whether a new obstruction 
exists for given $n$ in unary and $m$ in binary 
can then be decided in polynomial time,
and if so, it can also be constructed in polynomial time; 
cf. Figure~\ref{fig:IOHcomplexity}. (The hypothesis is called PH4 instead
of PH2, because PH2 and PH3 are some other positivity hypotheses in GCT6
that complement PH1). 
Once this final positivity hypothesis POH is proven, the obstruction
hypothesis is reduced to a tautology (FOH: Final Obstruction Hypothesis),
which can be verified and constructed in
$O(1)$ time--i.e., the associated decision problem $DP(FOH)$ 
is $O(1)$-time solvable. This  would then give us 
the final $O(1)$-size  proof. 

Thus the basic idea of the flip is to use positivity systematically
as a means to eliminate the quantifiers  and reduce the complexity 
of the decision problem associated with 
the  obstruction hypothesis until 
the obstruction hypothesis  is finally 
reduced to  an $O(1)$-time verifiable  tautology;
cf. Figure~\ref{fig:IOHcomplexity}. 

Now let us specify PH4 and POH.
Towards that end, let  $k \le l=m^2$ be the length of $\lambda$.
Define 

\begin{equation} 
\begin{array}{l}
\bar P_{n,m}= \{ \lambda: P_{\lambda,n,m} \not = \emptyset \} \subseteq \C^k, \\
\bar Q_{m}= \{ \lambda: Q_{\lambda,m} \not = \emptyset \} \subseteq \C^k.
\end{array}
\end{equation}

The following is a consequence of a fundamental result \cite{brion} in 
geometric invariant theory \cite{mumford}.
\begin{theorem} 
The sets $\bar P_{n,m}$ and $\bar Q_{m}$ are convex polytopes in $\C^k$.
\end{theorem} 


Then: 

\begin{hypo}  {\bf PH4} (GCT6)
The membership problems for these polytopes belong to 
$P$ and so also the problem of deciding if $\mbox{vol}(\bar P_{n,m}
\setminus \bar Q_{m})$, the volume of the relative complement 
$\bar P_{n,m} \setminus \bar Q_{m}$, is nonzero (positive);
i.e. if $\bar P_{n,m} \not \subseteq \bar Q_{m}$. By polynomial time,
we mean $\poly(n,l,\bitlength{m})$ time. This is $\poly(n)$,
if $m\le 2^{o(n)}$ and $l =\poly(n)$. 
\end{hypo}

\begin{hypo} {\bf (POH)}

For all $n\rightarrow \infty$, assuming $m=2^{\log^a n}$, $a>1$ fixed, 

\[ \mbox{vol}(\bar P_{n,m} \setminus \bar Q_{m}) > 0, \] 

for $k=(n+1)^2$. 
\end{hypo} 

\ignore{
Thus POH says that  the line-shaded area in Figure~\ref{fig:POH} has positive
volume for all large enough $n$. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{P}{$\bar P_{n,m}$}
\psfrag{Q}{$\bar Q_{n,m}$}
\epsfig{file=POH.eps, scale=1}
\end{center}
      \caption{POH}
      \label{fig:POH}
\end{figure}
}

\section{How to prove PH?}  \label{sphprove}
There is  a basic prototype of PH in representation theory,
which will be described in detail towards the end of Lecture 3. We shall
refer to it  as Plethysm PH. It says that the stretching functions 
akin to $F_{\lambda,n,m}(k)$ and $G_{\lambda,m}(k)$
associated with  fundamental  multiplicities 
in representation theory called plethysm constants also have analogous 
positive convex representations. 

This  is   known for a very special case of the plethysm constant 
called the  Littlewood-Richardson (LR) coefficient
$c_{\alpha,\beta}^\lambda$. It is  defined to be 
the number of occurences of the Weyl module $V_{\lambda}(G)$ in the 
tensor product of $V_{\alpha}(G)$ and $V_\beta(G)$, considered as a 
$G$-module by letting 
$G$ act on each factor of the tensor product independently. 
The classical Littlewood-Richardson rule, which we shall refer to as LR PH,
implies that the stretching function 
$\tilde c_{\alpha,\beta}^\lambda (k) = c_{k \alpha, k \beta}^{k \lambda}$
associated with the Littlewood-Richardson coefficient has a
positive convex representation.

Plethysm PH   happens to be a fundamental open problem of
representation theory, older than the $P$ vs. $NP$ problem itself. It 
has been studied intensively in the last century, and is known to be
formidable. And  now,  as explained the third lecture, it also turns out to 
be  the heart of this approach towards the $P$ vs $NP$, the
$\#P$ vs. $NC$ problems.



A basic plan to prove Plethysm PH is given in GCT6.
It is partially 
implemented in GCT7 and 8. See Figure~\ref{fig:lift} for a pictorial
depiction of the plan. It strives  to extend the  proof of LR PH based 
on the theory of the  standard quantum group \cite{drinfeld,kashiwara,lusztig}.
There it
comes out as a consequence of a  (proof of a) deep positivity result
\cite{kazhdan,lusztig}, which
we shall refer to as LR PH0. It says that   the 
tensor product of two representations of the standard quantum group 
has a canonical basis \cite{kashiwara,lusztig} 
whose structure coefficients are all positive \cite{lusztig}
polynomials (i.e., polynomials with nonnegative coefficients).
The only known proof of this
result is based on the Riemann Hypothesis over finite fields 
proved in \cite{weil2},  and the related works \cite{beilinson}. 
This Riemann Hypothesis over finite fields 
is  itself a deep positivity statement in mathematics,
from which   LR PH can  thus be 
deduced, as shown on the bottom row of Figure~\ref{fig:lift}.

If one were only interested in LR PH, one  does not 
need this  powerful machinery, because it has a  much simpler 
algebraic-combinatorial  proof. 
But the plan to extend the
proof of LR PH to Plethysm PH in GCT6,7,8 is like a huge
inductive spiral. To  make it work,  one  needs a 
stronger inductive hypothesis than Plethysm PH--this is precisely  Plethysm 
PH0 (which  will be
described in the third lecture; cf. Hypothesis~\ref{hplph0}).
Thus what is needed now 
is a systematic lifting  of the bottom arrow in Figure~\ref{fig:lift}
to the top, so as to complete the  commutative diagram, so to speak. 

Initial  steps in this direction have been taken in GCT7,8. 
First, GCT7 constructs a {\em nonstandard quantum group}, which
generalizes the notion of a standard quantum group \cite{drinfeld},
 and plays the
same role in the plethysm setting that the standard quantum group plays
in the LR setting. Second, GCT8 gives an algorithm to construct 
a canonical basis for a representation of the nonstandard quantum group
that is conjecturally correct and has the property Plethysm PH0,
which is a   generalization of LR PH0  supported by experimental
evidence.
Now what is needed to complete  the 
commutative diagram in Figure~\ref{fig:lift} is an appropriate nonstandard 
extension of the Riemann hypothesis over finite fields and the related works
\cite{beilinson,weil2,kazhdan,lusztig}
from which  Plethysm PH0 can be deduced. This--the top-right corner 
of the diagram--is the   main  open problem at the heart of this approach. 

\section{How to prove OH or POH?} 
We do not  know, 
since the  proof of OH and POH 
would really depend on the explicit forms of the
polytopes that arise in   PH1/PH4, and we have no idea about them
at this point.
GCT does suggest  that proving OH/POH  should be feasible 
``in theory'', i.e., {\em theoretically feasible},  assuming PH1/4,
since then DP(OH)/DP(POH)  belong to NP/P and polynomial-time
is complexity theory stands for feasible ``in theory''. 
In other words,
GCT gives a reason to believe now that proving 
the  $P\not = NP$ conjecture should be theoretically feasible. Even this
was  always questioned  in the field of complexity theory so far, because 
the $P$ vs. $NP$ problem is a universal statement regarding all of mathematics
(that says theorems cannot be proven automatically).
But, as we also know by now, 
there is a huge gap between  theory and  practice--e.g., 
just because  some problem is in $P$ does not 
necessarily mean that it is feasible in practice. Similarly,
the actual implementation of the GCT flip via positivity is expected to be 
immensely difficult ``in practice'', as Figure~\ref{fig:lift} suggests. 







\section{Is positivity  necessary?} \label{sposnece}
\ignore{
Though the statement of this result is elementary, its proof is nonelementary,
as expected,  since the generalized permanents are highly nontrivial
and mathematically formidable objects. Specifically, the problem
of finding a $\#P$-basis for the space of generalized permanents 
is intimately related to some formidable problems of representation
theory and algebraic geometry,
and the  simplest analogue of this problem 
which can be solved at present  \cite{}
requires the deep Riemann Hypothesis over finite fields \cite{} for its
proof; cf. Section~\ref{}.
The proof of Theorem~\ref{} proceeds at an abstract level 
through algebraic geometry and representation theory without
having to know anything about such a basis.
At present, it is open if there is any alternative 
weaker form of the $\#P \not = NC$  conjecture,
which cannot be proved by relativizable, low-degree or 
naturalizable  techniques, but which can still be proved by elementary 
or not so  nonelementary techniques; that is, whether the earlier known
barriers mentioned above can 
be simultaneously bypassed in an elementary way in the context of 
the $\#P$ vs. $NC$ (or $P$ vs. $NC$  or $P$ vs. $NP$) problem.


\section{Why are we going for explicit obstructions?}
In a sense, the proof of the weak form turns out to be nonelementary
because of the difficulty of explicit construction. Specifically, algorithm 
to construct an obstruction $O_n$ for each $n$ is very simple, but to
show that it is correct requires nontrivial algebraic geometry,
just as the construction 
of an explicit family of Ramanujan graphs in \cite{} is very simple,
but to show that it is correct requires nontrivial algebraic geometry.
We already know, e.g. from this example of Ramanujan graphs, that 
explicit constructions can require highly nonelementary techniques.
So the question now arises: why are we going for such difficult explicit
constructions? Can they not be avoided somehow? 
After all, to solve the original problem we only need to show existence
of obstructions. We do not have to construct them explicitly.

Furthermore,  explicit construction is not needed to 
cross any of the barriers mentioned above (e.g. the natural-proof-barrier).
This is because {\em any} proof technique which uses symmetries of the
permanent would automatically bypass the natural-proof barrier
in the context of the permanent vs. determinant problem,
even if it does not utter a word about explicit construction, since
most functions have no symmetries. Indeed, the weak form of 
the generalized $\#P$ vs. $NC$ problem itself has two proofs, one
purely nonconstructive and one through explicit construction--the major 
chunk of both proofs being  the same, except for the last step,
which is carried out via a counting argument in the former proof and via
explicit construction in the latter. Since the nonconstructive proof too
is based on symmetries, it also crosses the natural-proof barrier.
This provides a concrete evidence that explicit construction is not 
necessary for crossing the earlier known  barriers.

Then why are we still going for explicit construction? 
Before we go any further, we wish to briefly state  the motivation
behind  going for the flip (explicit construction),
since this is an important issue. 
}

Finally,  if the positivity problems are so hard,  one may ask if 
they can not be avoided somehow. Unfortunately, there is a formidable 
barrier towards the $P$ vs. $NP$ and related problems, called the
{\em complexity  barrier} \cite{GCTexplicit,GCTflip}
which is universal in the sense that
any approach towards these problems would have to tackle it, not just GCT. 
The flip, i.e., explicit construction of obstructions, is the most natural
and obvious way to cross this barrier, and  the natural way may well be 
among the most effective. The 
existing mathematical evidence suggests that any such natural approach
to cross this barrier would have to say  something deep regarding positivity
(Plethysm PH/PH0)  either explicitly or {\em implicitly}, even if
the approach does not utter a word about algebraic geometry or
representation theory.
That is,  Plethysm PH and PH0   may indeed be 
the heart of the  fundamental lower bound problems in complexity theory;
a detailed story and a precise meaning of the key 
phrase {\em implicit} would appear in the revised version of GCTflip.

%\input{feasibility}









































 

































\begin{sidewaysfigure} 
\begin{center} 
\epsfig{file=lift.eps, scale=.8}
\end{center}
      \caption{A commutative diagram}
      \label{fig:lift}
\end{sidewaysfigure} 



\ignore{\begin{figure} 
\psfragscanon
\psfrag{P}{$P\not = NP$ and $\#P\not = NC$ conjectures (characteristic zero)}
\epsfig{file=barriers.eps, scale=1}
      \caption{The feasibility barrier towards $P$ vs. $NP$}
      \label{fig:barriers}
\end{figure}}


%\input{lecture1_maintext}


==> lecture1_2.tex <==
\section{{\bf \LARGE Lecture 1 (Overview)}}

The goal of this lecture is to give a high level overview of 
geometric complexity theory (GCT), an 
approach towards the fundamental lower bounds in complexity theory; 
specifically
\ignore{The complexity classes that we are concerned with 
are the well known ones: $P$, the class of problems that can be solved 
in polynomial time,  $NP$, the class of problems whose solutions can be
verified in polynomial time,  $\#P$, the counting class
associated with $NP$,  and 
$NC$, the class of problems that can be solved 
in polylogarithmic time using polynomial number of processors.
The  fundamental lower bound problems that we are concerned with are:}

\noindent (1) 
The $P$ vs. $NP$ problem \cite{cook,karp,levin}: 
 show that $P \not = NP$;


\noindent (2) 
The  $\#P$ vs. $NC$ problem \cite{valiant}: show that 
$\#P \not = NC$.

We shall be dealing with the  
nonuniform versions of these problems 
in characteristic zero; i.e., when
the underlying field of computation is of characteristic zero, 
say $\Q$ or $\C$.  The additional problems that
need to be addressed when the underlying field of computation is finite
would be discussed in  GCT11. 

The nonuniform (characteristic zero) version of the $\#P$ vs. $NC$ problem
is also referred to as the permanent vs. determinant problem \cite{valiant}. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented 
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$; cf. Figure~\ref{fig:matrices}. 
By linear representation, we mean
the  entries  $y_{ij}$'s of $Y$ are affine (i.e., possibly nonhomogeneous) 
linear combinations 
of the entries $x_{lk}$'s of $X$. %; i.e., 
%\[ y_{i j} = \sum_{l,k\le n} a_{i,j}^{l,k} x_{l,k} + a_{i,j}^{n+1,n+1}, \]
%for some complex 
%$a_{i,j}^{l,k}$, $l,k \le n+1$, $i,j \le m$.
There is an analogous characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.


The main results of GCT hold for the characteristic zero versions 
of both of these problems. But we shall 
concentrate here on only the characteristic zero,  nonuniform
version of the $\#P$ vs. $NC$ problem, since this illustrates all the basic
ideas. In this lecture we outline  the GCT approach to this 
problem via algebraic geometry and representation theory, and
elaborate it further in the next two lectures.

\ignore{
\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes}
      \label{fig:complexityclasses}
\end{figure} 
}

\begin{figure}
\begin{center}
\psfragscanon
\psfrag{X}{$X$}
\psfrag{Y}{$Y$}
\psfrag{n}{$n$}
\psfrag{m}{$m$}
\psfrag{xlk}{$x_{l k}$}
\psfrag{yij}{$y_{i j}$}
\psfrag{barX}{$\bar X$}
\epsfig{file=matrices.eps, scale=.6}
\end{center}
      \caption{Linear representation $Y$ of a matrix $X$}
      \label{fig:matrices}
\end{figure} 


\section*{Why is algebraic geometry needed?}
But first we have to  explain  why algebraic 
geometry is even needed, when the statements of these problems are 
purely elementary.

It would be helpful to review the development
of GCT in this context. It  began with a  concrete
lower bound result, namely, the special case of the $P \not = NC$ conjecture
 \cite{GCTpram}, which says that 
the $P$-complete max-flow problem
cannot be solved in $\polylog(n)$ parallel time using $\poly(n)$ 
processors in the PRAM model without bit operations, which
includes virtually all known parallel algorithms for algebraic 
and weighted optimization problems;  here $n$ denotes
the total bit length of the input (not just the number of input parameters).
We shall refer to this result
 as the {\em weak  form} of the $P$ vs. $NC$ problem. Its  proof is
based on classical algebraic geometry, and as such, this may be regarded  
as  the first unconditional lower bound result to come out of GCT. 
Since it is a formal implication of the usual $P \not = NC$ conjecture,
it can be stated in purely elementary, combinatorial terms. And yet 
no elementary combinatorial proof of  this result is known so far. 
This suggested that geometry may be indipensible for
the deeper study of the fundamental lower bound problems.



Another evidence is provided by the following 
weak form of the $\#P$ vs. $NC$ problem. 
To define it, we have to first give an equivalent 
homogeneous restatement of the permanent vs. determinant problem. 
Let $\bar X$ be an $(n+1)\times (n+1)$ variable matrix. 
We identify $X$ with the $n \times n$ principal top-left minor of $\bar X$.
Let $z=\bar x_{n+1,n+1}$ be the bottom-right entry of $\bar X$, which is
not in $X$; we will use it as a homogenizing variable; 
cf. Figure~\ref{fig:matrices}.
The problem now is to show that, 
when $n$ is large enough, there does not exist an $m\times m$ matrix $Y$,
whose entries $y_{ij}$'s are homogeneous linear combinations of the entries 
$\bar x_{l,k}$'s  of $\bar X$,  such that, 
$\perm(X)z^{m-n}=\det (Y)$, with  $m$ as above. 
By homogeneous linear combination, we mean
\[ y_{i j} = \sum_{l,k\le n+1} a_{i,j}^{l,k} \bar x_{l,k}, \] 
for some complex $a_{i,j}^{l,k}$, $l,k \le n+1$, 
$i,j \le m$.
It is easy to check that this homogeneous form 
of the permanent vs. determinant problem is equivalent to the nonhomogeneous 
form given before.  

By the classical theorem of symmetric functions, 
$\det(Y)$ can be written explicitly as a polynomial 
$e(w_0, \ldots, w_{m})$, where $w_i =\trace(Y^i)$. 
Hence, the following can be thought of as 
a weaker  homogeneous  form of the $\#P$ vs. $NC$ problem:

\begin{theorem} (The weak form of the $\#P$ vs. $NC$ problem)  \label{tweak}

There do not exist complex numbers $b_i^l, c_j^k$, $l,k \le n+1$, $i,j \le m$,
and a polynomial $e(w_0,\ldots, w_m)$, 
such that, with 
\[ y_{i j} = \sum_{l,k\le n} b_i^l c_j^k  \bar x_{l,k}, \]
$\perm(X)z^{m-n}=g(Y)$, where  $g(Y)=e(\trace(Y^0),\ldots, \trace(Y^m))$, 
and  $m$ is as above. In fact, this holds
for any $m\ge n$. 
\end{theorem} 


%That this holds for any $m \ge n$ indicates that this weak form is
%too weak from the complexity theoretic perspective (unlike the 
%weak form of the $P$ vs. $NC$ result above); it is  a mathematical 
%result rather than complexity-theoretic.
This   can be easily proved  using  classical algebraic geometry 
\cite{GCT2append}, though no 
elementary proof, which  does not need  any nontrivial
algebraic geometry, is known so far   \footnote{There seems to be 
a serious gap in an  elementary 
proof proposed earlier by two  attendees of  the IAS lectures}. 

But   the classical algebraic geometry does not seem sufficient
for proving the general forms of the fundamental lower bound problems for
the following reasons. 
First, the classical results 
used in \cite{GCTpram} are all degree-based; e.g. Bezout, Milnor-Thom etc.
As was pointed out in the last of chapter 
of \cite{GCTpram}, such low-degree techniques would not work in the context
of the fundamental lower bound problems;
the recent  algebrization barrier \cite{aaronson} 
also says  something similar. 
The classical results used for proving the weak form of the
$\#P$ vs. $NC$ problem  are not degree-based. But this proof too has
a serious limitation: namely, it is naturalizable; i.e., cannot cross the
natural proof barrier in \cite{rudich}, because  it works for most
functions in place of the permanent. 

This suggests that something much more than classical geometry may be  needed 
for going further.
During the course of these lectures, we shall instantiate the 
basic plan of GCT for the general form to provide a ``correct'' 
proof of the weak form of the $\#P$ vs. $NC$ result,
which does not have the   limitations of the ``wrong'' proof above.


\section*{Basic plan} 
We now outline the basic  plan of GCT focussing on
the general permanent vs. determinant problem in characteristic zero. 
The weak form will  be  used only as a simple   test of 
the basic ideas as they are developed.

The first  step (GCT1,2) is to reduce this nonexistence problem 
to an existence problem--specifically, to the problem of proving 
existence of a family $\{O_n\}$ of obstructions; 
cf. Figure~\ref{fig:firststep}.
Here an {\em obstruction} $O_n$ is a proof-certificate of
hardness of $\perm(X)$, $X$ an $n\times n$ variable matrix,
just as the Kurotowski minor is a proof-certificate of nonplanarity of a 
graph.  Specifically,  it is some 
algebro-geometric-representation-theoretic gadget, 
whose existence for every $n$,  serves as a 
guarantee that $\perm(X)$ cannot be represented linearly as $\det(Y)$,
when $m=2^{\log^a n}$, $a>0$ fixed, $n\rightarrow \infty$. 

\begin{figure} 
\begin{center}\psfragscanon
\psfrag{on}{$\{O_n\}$}
\epsfig{file=firststep.eps, scale=.8}
\end{center}
      \caption{Reduction from nonexistence to existence}
      \label{fig:firststep}
\end{figure}


This reduction to existence is carried out as follows.
First, we associate (GCT1) with 
the complexity class $\#P$ a family $\{X_{\#P}(n,m)\}$ of (group-theoretic)
class varieties, and with the complexity class $NC$ a family of 
$\{X_{NC}(n,m)\}$ of (group-theoretic) class varieties such that: 
if $\perm(X)$, $\dim(X)=n$, can be represented linearly 
as $\det(Y)$, $\dim(Y)=m>n$, then 

\begin{equation} \label{eqembed} 
X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation} 

Each  class variety is a  (projective) algebraic variety, by which
we mean the zero set of  a system of mutivariate 
homogeneous polynomials with coefficients in $\C$  (akin to the 
usual curves  and surfaces). It is  group-theoretic in the 
sense that it is  constructed using group-theoretic operations 
and the general linear group $G=GL_l(\C)$, $l=m^2$, of $l\times l$ invertible
complex matrices acts on it. Here action means moving the points 
of the class variety around, just as $G$ moves the points of $\C^l$ around 
by the standard action via invertible linear transformations.
The goal is to show that the inclusion (\ref{eqembed}) is impossible;
cf. Figure~\ref{fig:class}. 

\begin{figure} 
\begin{center} \psfragscanon
\psfrag{xsharp}{$X_{\#P}(n,m)$}
      \psfrag{xnc}{$X_{NC}(n,m)$}
      \psfrag{g}{$G=GL_l(\C)$, $l=m^2$}
      \psfrag{Obstruction}{\mbox{Obstruction}}
\epsfig{file=class.eps, scale=.5}
\end{center}
      \caption{Class varieties}
      \label{fig:class}
\end{figure} 



Since each class variety has a $G$-action, the space of polynomial functions 
on each class variety has a  representation-theoretic structure, which 
puts constraints on which  representations of $G$ can live on that variety
(i.e. in the space of polynomial  functions on that variety).
Informally, an obstruction is an irreducible (minimal)  representation of $G$
that can live on $X_{\#P}(n,m)$ but not on $X_{NC}(n,m)$; 
cf. Figure~\ref{fig:class}.
Existence of  an obstruction $O_n$, for every $n$, assuming
$m=2^{\log^a n}$, $a>1$ fixed, implies  that the inclusion (\ref{eqembed}) 
is not possible, since  $O_n$ cannot live  on $X_{NC}(n,m)$.
Thus  an obstruction blocks the inclusion (\ref{eqembed}).


To define an obstruction formally, we need to recall some basic representation
theory.  By a classical result of Weyl, the irreducible 
(polynomial) representations of $G=GL_l(\C)$ are in one-to-one correspondence 
with the partitions  $\lambda$ of length at most $l$, by which we mean 
integral sequences $\lambda_1 \ge 
\lambda_2 \cdots \ge \lambda_k > 0$, $k\le l$, where  $k$ is called the  length
of $\lambda$. The irreducible 
representation of $G$ in correpsondence with $\lambda$ is denoted 
by $V_\lambda(G)$, and is called the {\em Weyl module} of $G$ indexed by 
$\lambda$. Symbolically:

\[\mbox{Irreducible representations of } G \stackrel{\mbox{Weyl}}{\Longleftrightarrow} \quad \mbox{partitions} \ \lambda. \]  

\[\mbox{Weyl module  } V_\lambda(G)  \longleftrightarrow \lambda. \] 


Now suppose $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$. 
Suppose to the contrary that 

\begin{equation} \label{eqembed2}   X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation}

Let $R_{\#P}(n,m)$ denote the homogeneous coordinate ring of 
$X_{\#P}(n,m)$; i.e., the ring of polynomial functions on $X_{\#P}(n.m)$
(though the  functions here are not functions in usual sense;
but let us  not worry about this). 
Let $X_{\#P}(n,m)_d$ be the degree-$d$-component of $X_{\#P}(n, m)$ consisting
of functions of degree $d$. We define $R_{NC}(n,m)$ and $R_{NC}(n,m)_d$
similarly. Since $X_{\#P}(n,m)$ has the action of $G$, $R_{\#P}(n,m)$ 
also has an action of $G$; i.e., it is a representation of $G$. Hence,
$R_{\#P}(n,m)_d$ is a finite dimensional representation of $G$. 
Similarly, $R_{NC}(n,m)$ is a representation of $G$, and $R_{NC}(n,m)_d$
a finite dimensional representation of $G$. 



If (\ref{eqembed2} holds, then we get a natural map from $R_{NC}(n,m)$ to
$R_{\#P}(n,m)$ obtained by restriction of a function on $X_{NC}(n,m)$ to
$X_{\#P}(n,m)$. %; cf. Figure~\ref{fig:restriction}.
By basic algebraic geometry, this map
is surjective and is a $G$-homomorphism.
Furthermore, it is degree-preserving. This means there
is a surjective $G$-homomorphism from $R_{NC}(n,m)_d$ to 
$R_{\#P}(n,m)_d$. Symbolically: 

\begin{equation} \label{eqsurjection}
R_{\#}(n,m)_d \leftarrow  R_{NC}(n,m)_d.
\end{equation}

\ignore{
\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{Xp}{\small $X_{\#P}(n,m)$}
\psfrag{Xnc}{\small $X_{NC}(n,m)$}
\epsfig{file=restriction.eps, scale=.6}
\end{center}
      \caption{Restriction}
      \label{fig:restriction}
\end{figure}
}

Let $R_{\#P}(n,m)_d^*$ denote the dual of $R_{\#P}(n,m)_d$; i.e., the 
set of linear maps from $R_{\#P}(n,m)_d$ to $\C$. Then (\ref{eqsurjection})
implies that there is an injective $G$-homomorphism from 
$R_{\#P}(n,m)^*$ to $R_{NC}(n,m)^*$. Symbolically: 

\begin{equation} \label{eqinclusion}
R_{\#}(n,m)_d^*  \hookrightarrow {NC}(n,m)_d^*.
\end{equation}

\begin{defn} (GCT2)
An obstruction $O_n$ is a Weyl module $V_\lambda(G)$ that 
occurs as a subrepresentation 
in $R_{\#P}(n,m)_d^*$  but not in $R_{NC}(n,m)_d^*$, for some $d$. 
We call $\lambda$ an {\em obstruction label}, and sometimes,
by abuse of notation, an obstruction as well.
\end{defn}

\begin{prop} (GCT2)
Existence of an obstruction $O_n$, for all $n\rightarrow \infty$, 
with $m=2^{\log^a n}$, $a>1$ fixed, implies $\perm(X)$, $\dim(X)=n$, 
cannnot be represented linearly as 
$\det(Y)$, $\dim(Y)=m$. 
\end{prop}

This follows just from the definition of an obstruction, and 
leads to:

\begin{goal} 
Prove existence of an obstruction family $\{O_n\}$ using 
the {\em exceptional} nature of $\perm(X)$ and $\det(Y)$. 
\end{goal} 

Exceptional here means completely characterized by the symmetries 
in the following sense. 
Let  $Y$ be a variable $m\times m$ matrix.
Let $\sym^m(Y)$ be the space of homogeneous forms of degree $m$ 
in the $m^2$ variable entries of $Y$. Then, by the  classical
representation theory,  $\det(Y)$ is the only form in $\sym^m(Y)$ 
such that, for any $A,B \in GL_m(\C)$ with $\det(A)\det(B)=1$, 
\[ \det(Y)=\det(A Y^* B), \] 
where $Y^*=Y$ or $Y^t$. 
Thus $\det(Y)$ is completely characterized 
by its symmetries, and hence, is  exceptional.

Simlarly, $\perm(X)$ is the only form 
in the space of forms of degree $n$ in the entries of $X$ such that, 
for any diagonal or permutation matrices $A,B$, 
\[ \perm(X)=\perm(AX^*B), \]
where $X^*=X$ or $X^t$. 
Thus $\perm(X)$ is also
completely characterized   by its symmetries, and hence, is
exceptional.


\subsection*{The weak case}
\begin{theorem} \cite{GCT2append} \label{tgct2append}
There exists a family  $\{O_n\}$ of obstructions in the weak form of 
the $\#P$ vs. $NC$ problem in characteristic zero.
\end{theorem}

(The class varieties and obstructions are defined in a similar fashion 
in the weak form--we omit their formal definitions). This result 
implies Theorem~\ref{tweak}, and provides its 
 ``correct'' proof. We shall outline it briefly in the next lecture.
It involves a detailed study of the $G$-action on class varieties
based on:
\begin{enumerate} 
\item The work on stability in geometric invariant theory by 
Hilbert, Mumford, Kempf and others \cite{mumford}. 
\item Peter-Weyl theorem for $G=GL_l(\C)$, which is the algebraic form 
of the (noncommutative) harmonic analysis on the unitary group 
$U_l(\C)$, and 
\item An extension of an induction technique 
in the Borel-Weil theorem of geometric representation theory.
\end{enumerate}

\subsection*{The general case} 
Now we proceed to the general case, our  main interest. 

Towards that end, we  associate with the class varieties 
certain representation-theoretic {\em stretching} functions. 
Let $F_{\lambda,n,m}(k)$ denote the number of occurences (multiplicity)  of
the Weyl module $V_{k\lambda}(G)$ in $R_{\#P}(n,m)$ as a subrepresentation,
and $G_{\lambda,n,m}(k)$ the number of occurences of 
$V_{k\lambda}(G)$ in $R_{NC}(n,m)$. These are statistical functions
associated with the class varieties, where the statistics associates 
with every number (stretching parameter) $k$  
the multiplicity of the corresponding
Weyl module $V_{k\lambda}(G)$; cf. Figure~\ref{fig:statistics}.

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{l}{$\lambda$}
\psfrag{2l}{$2 \lambda$}
\psfrag{3l}{$3 \lambda$}
\psfrag{v1}{$V_\lambda(G)$}
\psfrag{v2}{$V_{2 \lambda}(G)$}
\psfrag{v3}{$V_{3\lambda}(G)$}
\epsfig{file=statistics.eps, scale=1}
\end{center}
      \caption{statistics}
      \label{fig:statistics}
\end{figure}

%We will also need a definition.
Let us  call a function $f(k)$ quasipolynomial, if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k)$ for all nonnegative integral $k=i$ modulo $l$; $l$ is
called the period of the quasi-polynomial. Thus  quasi-polynomials
are hybrids of  polynomial and periodic functions. 

A fundamental example of a quasi-polynomial is the Ehrhart quasi-polynomial
$f_P(k)$ of a polytope $P$ with rational vertices. It is defined
to be the number of integer points in the dilated polytope $kP$. By the 
classical result of Ehrhart, it is known to be a quasi-polynomial.




\begin{theorem} (GCT6) \label{tquasi}
The functions $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ 
are quasi-polynomials assumming that the singularities of the class varieties
$X_{\#P}(n,m)$ and $X_{NC}(n,m)$ are rational. 

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem} 

Here rational singulary means a singularity that is nice in
a certain algebro-geometric sense that we shall not elaborate.

The proof of this result follows from a detailed study of the behaviour
of the singularities of class varieties under the action of the 
group $G$. This is based on
\begin{enumerate} 
\item The 
resolutions of singularities in characteristic zero, as per 
Hironaka \cite{hironaka}: 
this  roughly says 
that the singularities of any algebraic variety in characteristic zero
can be untangled (resolved) nicely in a systematic fashion; cf.
 Figure~\ref{fig:resolution}.
\item Cohomological works of Boutot, Brion,  Flenner, Kempf  and others
bases on this resolution; cf.  \cite{boutot} and GCT6 for other references.
\end{enumerate} 


\begin{figure} 
\begin{center} 
\epsfig{file=resolution.eps, scale=.5}
      \caption{Resolution}
      \label{fig:resolution}
\end{center}
\end{figure}


As such, this proof is highly nonconstructive. It gives no effective
bound on the period $l$--it just says that $l$  is finite.
It is a recurrent phenomenon in geometric representation theory that 
whenvever the  stretching function associated with a fundamental
multiplicity is a quasi-polynomial, it turns out to be an Ehrhart
quasi-polynomial of some polytope. This and other evidence given 
in GCT6 leads to:

\begin{hypo} {\bf (PH) [Positivity Hypothesis]} \label{hph}
For every $\lambda,n,m\ge n$, 
there exist polytopes $P=P_{\lambda,n,m}$ and $Q=Q_{\lambda,n,m}$ 
such that 
\begin{equation} 
\begin{array}{l}
F_{\lambda,n,m}(k)=f_P(k), \\
G_{\lambda,n,m}(k)=f_Q(k).
\end{array}
\end{equation}
It is also assumed here that there exists for $P_{\lambda,n,m}$ a specification
of the form $A x \le b$, where $A$ is independent of $\lambda$, and $b$ is 
a piecewise homogeneous linear function of $\lambda$, so that
$P_{k\lambda,n,m}=k P_{\lambda,n,m}$. Similarly for $Q_{\lambda,n,m}$.
If such $P$ and $Q$ exist, their dimensions are guaranteed to be
polynomial in $n$ and the length of $\lambda$
by the proof of Theorem~\ref{tquasi}.

Analogous positivity hypothesis for the $P$ vs. $NP$ problem in characteristic
zero.
\end{hypo} 

When PH holds, we say that $F_{\lambda,n,m}(k)$ and 
$G_{\lambda,n,m}(k)$ have {\em positive convex representations}. 
Here positivity refers to the fact that the Ehhart quasipolynomial 
$f_P(k)$ is a positive expression:
\[ f_P(k)=\sum_{v} 1,\] 
where $v$ ranges over all integer points in $kP$--there are no 
alternating signs in this expression.
Convexity refers to the  convexity of the polytopes $P$ and $Q$. 

\begin{theorem} (GCT6)
There exists a family $\{O_n\}$ of obstructions 
for the general $\#P$ vs. $NC$ problem in characteristic zero, 
for $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$, 
assuming, 

\begin{enumerate} 
\item PH, and
\item OH (Obstruction Hypothesis): 

For all $n\rightarrow \infty$,  there exists $\lambda$ such that 
$P_{\lambda,n,m}\not = \emptyset$ and $Q_{\lambda,n,m}=\emptyset$.
\end{enumerate}

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem}

We call  $\lambda$ a {\em relaxed obstruction}
(or rather, relaxed obstruction-label)
if it satisfies OH. In this case, $k\lambda$, for some integer $k\ge 1$ is
an obstruction--we just have to choose $k$ so that the scaled polytope 
$P_{k\lambda,n,m}=k P_{\lambda,n,m}$ contains an integer point 
($Q_{k \lambda,n,m}=k Q_{\lambda,n,m}$  continues to be empty). 
Henceforth, whenever we say obstruction, we actually mean relaxed 
obstruction.




\subsection*{The flip: Explicit construction of obstructions (GCT6,GCTflip)} 
In principle PH may have a nonconstructive proof, like that
of Theorem~\ref{tquasi}, which only tells  that such polytopes 
exist without explicitly constructing them. But proving OH may not be feasible
unless the polytopes $P$ and $Q$ in PH are given explicitly.
This  suggests the following strategy for proving 
existence of obstructions.


\noindent (1) Prove the following stronger explicit form 
of PH:

\begin{hypo} {\bf (PH1)} 
There exist {\em explicit} 
polytopes $P_{\lambda,n,m}$ and $Q_{\lambda,n,m}$ satisfying PH.
Explicit means: 

\begin{enumerate}
\item  The polytopes are specified by explicit systems of linear constraints,
each constraint of bitlength $\poly(n,\bitlength{\lambda}, \bitlength{m})$
(note occurence of  $\bitlength{m}$  instead of $m$). 


\item  The membership problems for the polytopes
$P_{\lambda,n,m}$ and $Q_{\lambda,n,m}$ belong to the complexity class $P$.
That is,  given a point $x$, whether it belongs to $P_{\lambda,n,m}$ 
or $Q_{\lambda,n,m}$ can be decided in time that is polynomial in
$n$, the bitlength $\bitlength{\lambda}$ of $\lambda$, the 
bitlength $\bitlength{x}$ of $x$ and $\bitlength{m}$. 
Furthermore, we assume that if $x$ does not belong to the polytope,
then the membership algorithm also gives a hyperplane separating 
$x$ from the polytope in the spirit of \cite{lovasz}. 
\end{enumerate} 
\end{hypo}

In particular, PH1 implies that the functions $F_{\lambda,n,m}(k)$ and
$G_{\lambda,n,m}(k)$ belong to the complexity class $\#P$. 


\noindent (2a) {\bf [The flip]}

Let $m=2^{\log ^a n}$, for a fixed $a>1$. 
Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
show existence of  an {\em explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of obstructions  satisfying OH. 
We say that an obstruction (proof-certificate) 
$\lambda_n$ is {\em explicit} if is ``short'' and ``easy to verify'':


\begin{enumerate} 
\item  Short: This means its bitlength $\bitlength{\lambda_n}$ 
is $\poly(n)$,
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  

\item Easy to verify: given $n, m \le 2^{\log^a n}$ and 
$\lambda_n$, whether 
$\lambda_n$ is a valid obstruction 
can be verified 
in $\poly(n,\bitlength{\lambda})$ time. In particular, this is
$\poly(n)$ when $\bitlength{\lambda}=\poly(n)$. 
\end{enumerate}

Existence of an explicit family of obstructions is equivalent to saying
that the problem of deciding existence of obstructions belongs to $NP$.
This definition of explicitness is quite natural since the class $NP$ 
is a class of problems whose proof-certificates (witnesses) are 
short and easy to verify. As such, the flip--going for 
explicit  obstructions--is
a proof-strategy that is literally given to us on a platter 
by the $P$ vs. $NP$ 
problem itself. Why it is called flip would be explained later.


It should be stressed that we are primarily interested in only proving 
existence of obstructions. Whether they are explicit or not 
does not really matter in the original statement of the problem.
But we need to know the polytopes $P$ and
$Q$ explicitly (PH1)  so that proving OH is feasible. 
%In other words,   if we do not
%even know what the polytopes $P$ and $Q$ look like, 
%it seems unlikely that anything  could be said regarding OH. 
But once  PH1 is proved, existence of an explicit family follows
automatically,   as a bonus, whether we care for it or not. 

To see why, let us observe that 
the second condition above  (ease of verification) follows directly
from PH1 and the polynomial time algorithm for 
linear programming on  polytopes given by separation oracles \cite{lovasz}. 
Shortness  also follows from PH1. 

Thus it is as if the $P$ vs. $NP$ problem is forcing us to go
for explicit obstructions.


\noindent (2b) {\bf [The strong flip (optional)]} 

Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
construct (rather than just show existence of) 
a {\em strongly explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of obstructions  satisfying OH. We say that an explict family 
of obstructions is strongly explicit if,
for each $n$, a valid obstruction-label
$\lambda_n$ can be constructed in $\poly(n)$ time.
In particular, the height and the bitlength of
 $\lambda$ is $\poly(n)$ (short) 
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  


For the purposes of the lower bound problems that we are interested in, the
flip (just explicit  
existence) would suffice and the stronger flip (explicit construction)
is optional. But the stronger flip can give us deeper insight into these
lower bound problems; cf. GCTflip for more on this.

Now we turn to a few obvious questions.

\subsection*{Why should PH, PH1,  and OH hold?} 

Mathematical evidence for this is given in GCT2,4,6,7,8.
We shall discuss this a bit in the third lecture.


\subsection*{What has been achieved by all this?: The meaning of the flip} 
Let us now see what has been achieved so far
in the context of the 
$\#P\not = NC$ conjecture in the nonuniform setting (characteristic zero),
the argument for the $P$ vs. $NP$ problem in characteristic zero
being  similar. The goal of this conjecture is to prove that 
$\perm(X)$ cannot be computed by an arithmetic circuit $C$ over $X$ with
coefficients in $\C$ of size $m=\poly(n)$, or more generally,
$m \le 2^{\log^a n}$, for some fixed $a>1$, and depth $O(\log^a n)$.
Or in symbols:

\begin{equation} \label{eqioh} 
 {\bf (IOH):}  \forall n  \forall C \exists X:
\perm(X)\not = f_C(X),
\end{equation} 

where $f_C(X)$ denotes the function computed by $C$, and $n$ is supposed
to be sufficiently large.
For given $X$ and $C$ of $\poly(n)$ size, the problem 
of deciding if  $\perm(X) = f_C(X)$ belongs to $\#P$ (or rather, $P^{\#P}$). 
Since there are two alternating layers of quantifiers in (\ref{eqioh}),
the problem of verifying it belongs to $\Pi^2 \#P$, 
which is very high in the complexity hierarchy
(cf. Figure~\ref{fig:IOHcomplexity}).
Hence, we  refer to the original hypothesis (\ref{eqioh}) 
to be proven  as IOH 
(Infeasible Obstruction Hypothesis). Of course, IOH is expected to 
be a tautology, and hence is expected to  be verifiable in $O(1)$ time--but
we do not know that as yet. 



\begin{sidewaysfigure} 
\begin{center}
\psfragscanon
\psfrag{sigma2p}{{\small $\Pi^2 \#P$}}
\psfrag{sigma1p}{$\Sigma^1 \#P$}
\psfrag{P}{{\small $P$}}
\psfrag{NP}{{\small $NP$}}
\psfrag{T}{$T$}
\psfrag{#P}{$\# P$}
\psfrag{inNP}{$\in NP$}
\psfrag{inP}{$\in P$}
\psfrag{insigma2p}{$\in \Pi^2 \#P$}
\psfrag{PHplus}{PH1}
\psfrag{PHtil}{$PH^\dagger$}
\epsfig{file=IOHcomplexity.eps, scale=.8}
\end{center}
      \caption{Positivity as a means to eliminate the quantifiers and 
reduce the complexity of the  obstruction hypothesis}
      \label{fig:IOHcomplexity}
\end{sidewaysfigure}



Equivalently, the goal is to prove existence of a {\em trivial obstruction},
which is a table that lists for each $C$ as above a counterexample  $X$ so that
$\perm(X)\not = f_C(X)$; cf. Figure~\ref{fig:trivial}.
The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$ and depth
$O(\log^a n)$. Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. 
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time to decide if such a table exists and construct 
one (optional) for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. So
we call  this trivial, brute force 
strategy of proving IOH, based on existence of trivial obstructions,
 an {\em infeasible strategy}. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{eq}{$\perm(X)\not = f_C(X)$}
\epsfig{file=trivial.eps, scale=.5}
\end{center}
      \caption{A trivial obstruction}
      \label{fig:trivial}
\end{figure}


In contrast, assuming PH1, the problem  of verifying OH belongs 
to $NP$ as we have already observed. Thus, assuming PH1, we have 
transformed the original infeasible obstruction 
hypothesis $IOH \in \Pi^2 \#P$ to a new  obstuction hypothesis 
$OH \in NP$, in the process bringing down the time to verify an obstruction
from the exponential (for the original trivial obstruction) to polynomial
(for the new obstruction); cf. Figure~\ref{fig:IOHcomplexity}.  
%Intuitively, the new obstruction captures  the essence of the old obstruction
%in short space.
The task of verifying  an obstruction has also been 
transformed from the infeasible (exponential-time) to the feasible 
(polynomial-time), hence the name of this strategy: the flip,
from the infeasible to the feasible.
Positivity (PH1) is used in the flip as a means  to
eliminate the quantifying variables in IOH and bring down the 
 complexity of the obstruction hypothesis;
cf. Figure~\ref{fig:IOHcomplexity}. 




This process can be extended further. Assuming an additional
positivity hypothesis PH4 to be specified below,
$OH \in NP$ can be transformed 
to POH (Positivity Obstruction Hypothesis) that belongs to $P$; i.e.,
which can be verified in polynomial time, and an obstruction,
if it exists, can also be constructed in polynomial time; 
cf. Figure~\ref{fig:IOHcomplexity}. (The hypothesis is called PH4 instead
of PH2, because PH2 and PH3 are some other positivity hypotheses in GCT6
that complement PH1). 
Once this final positivity hypothesis POH is proven, the obstruction
hypothesis is reduced to a tautology, which can be verified in
$O(1)$ time. This  would then give us 
the final $O(1)$-size  proof. 

Thus the basic idea of the flip is to use positivity systematically
as a means to elminate the quantifiers  and reduce the complexity 
of the  obstruction hypothesis until it is finally
reduced to  an $O(1)$-time verifiable  tautology;
cf. Figure~\ref{fig:IOHcomplexity}. 

Now let us specify PH4 and POH.
Towards that end, let  $k \le l=m^2$ be the length of $\lambda$.
Define 

\begin{equation} 
\begin{array}{l}
\bar P_{n,m}= \{ \lambda: P_{\lambda,n,m} \not = \emptyset \} \subseteq \C^k, \\
\bar Q_{n,m}= \{ \lambda: Q_{\lambda,n,m} \not = \emptyset \} \subseteq \C^k.
\end{array}
\end{equation}

Then: 

\begin{hypo}  {\bf PH4} 

The sets $\bar P_{n,m}$ and $\bar Q_{n,m}$ are convex polytopes in $\C^k$.
Furthermore, the membership problems for these problems belong to 
$P$ and so also the problem of deciding if $\mbox{vol}(\bar P_{n,m}
\setminus \bar Q_{n,m})$, the volume of the relative complement 
$\bar P_{n,m} \setminus \bar Q_{n,m}$, is nonzero (positive);
i.e. if $\bar P_{n,m} \subseteq \bar Q_{n,m}$. By polynomial time,
we mean $\poly(n,l,\bitlength{m})$ time. This is $\poly(n)$,
if $m\le 2^{o(n)}$ and $l =\poly(n)$. 
\end{hypo}

\begin{hypo} {\bf (POH)}

For all $n\rightarrow \infty$, assuming $m=2^{\log^a n}$, $a>1$ fixed, 

\[ \mbox{vol}(\bar P_{n,m} \setminus \bar Q_{n,m}) > 0, \] 

for $k=(n+1)^2$. 
\end{hypo} 

\ignore{
Thus POH says that  the line-shaded area in Figure~\ref{fig:POH} has positive
volume for all large enough $n$. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{P}{$\bar P_{n,m}$}
\psfrag{Q}{$\bar Q_{n,m}$}
\epsfig{file=POH.eps, scale=1}
\end{center}
      \caption{POH}
      \label{fig:POH}
\end{figure}
}

\subsection*{How to prove PH?} 
The goal is to extend the proof of the weak 
PH needed to prove Theorem~\ref{tgct2append}
to that of the general PH in  Hypothesis~\ref{hph}.
One crucial ingradient of the weak  PH is the classical
positive convex interpretation for the Littlewood-Richardson (LR) coefficient
$c_{\alpha,\beta}^\lambda$, which is defined to be 
the number of occurences of the Weyl module $V_{\lambda(G)}$ in the 
tensor product of $V_{\alpha}(G)$ and $V_\beta(G)$; we  refer to
it as LR PH.   What is needed to prove the general PH 
is a similar positive convex interpretation for the
so-called plethysm constants in representation theory, of which the 
Littlewood-Richardson coefficient is a very special case--we shall refer to
this as Plethysm PH; cf. Lecture 3.
This  happens to be a fundamental open problem of
representation theory, older than the $P$ vs. $NP$ problem itself. It 
has been studied intensively in the last century, and is known to be
formidable. And now,  it also turns out to 
be  the heart of this approach towards the $P$ vs $NP$, the
$\#P$ vs. $NC$ problems.



A basic plan to prove Plethysm PH is given in (GCT6).
It is partially 
implemented in GCT4,6,7,8. See Figure~\ref{fig:lift} for a pictorial
depiction of the plan. It strives  to extend the  proof of LR PH based 
on the theory of the  standard quantum group \cite{drinfeld}. There it
comes out as a consequence of a  (proof of a) deep positivity result
\cite{kazhdan,lusztig}, which
we shall refer to as LR PH0. It says that   the 
tensor product of two representations of the standard quantum group 
has a canonical basis whose structure coefficients are all positive 
polynomials (i.e., polynomials with nonnegative coefficients).
The only known proof of this
result is based on the Riemann Hypothesis over finite fields (RHf) 
proved in \cite{weil2},  and the related works \cite{beilinson}. 
The Riemann Hypothesis is  itself a deep positivity statement in mathematics,
from which   LR PH can  thus be 
deduced, as shown on the bottom row of Figure~\ref{fig:lift}.

If one were only interested in LR PH, one  does not 
need this  powerful machinery, because it has a  much simpler 
algebraic-combinatorical  proof. 
But the plan to extend the
proof of LR PH to Plethysm PH in GCT6,7,8 is like a huge
inductive spiral. To  make it work,  one  needs a 
stronger inductive hypothesis than PH--this is precisely  PH0.
Thus what is needed now 
is a systematic lifting  of the bottom arrow in Figure~\ref{fig:lift}
to the top, so as to complete the  commutative diagram, so to speak. 

Initial  steps in this direction have been taken in GCT7,8. 
First, GCT7 constructs a {\em nonstandard quantumg group}, which
generalizes the notion of a standard quantum group, and plays the
same role in the plethysm setting that the standard quantum group plays
in the LR setting. Second, GCT8 gives an algorithm to construct 
a canonical basis for a representation of the nonstandard quantum group
that is conjecturally correct and has the property Plethysm PH0,
which is a   generalization of LR PH0  supported by experimental
evidence.
Now what is needed to complete  the 
commutative digram in Figure~\ref{fig:lift} is an appropriate nonstandard 
extension of the Riemann hypothesis over finite fields and the related work
from which  Plethysm PH0 can be deduced. This--the top-right corner 
of the diagram--is the big open problem,
far beyound our personal expertize. But it is 
our hope that the field of mathematics would have something to say about it.


\subsection*{How to prove OH or POH?} 
We have nothing to say on this at this point,
since the  proof of OH and POH 
would really depend on the explicit forms of the
polytopes $P$ and $Q$ that arise in   PH1. 


\subsection*{Is all this necessary?} 
Finally, one may  ask: if the positivity problems are so formidable, can
they not be avoided somehow? Unfortunately, there is a formidable 
barrier towards the $P$ vs. $NP$ and related problems, called the
{\em feasibility barrier}, which seems universal in the sense that
any approach towards these problems would have to tackle it, not just GCT. 
The existing mathematical evidence suggests that any natural approach
to cross this barrier would have to say  something deep regarding 
Plethysm PH  either explicitly or {\em implicitly}, even if
the approach does not utter a word about algebraic geometry or
representation theory.
That is,  Plethysm PH and PH0   may indeed be 
the heart of the  fundamental lower bound problems in complexity theory;
cf \cite{} for a detailed story and a precise meaning of the key 
phrase {\em implicit}.










































 

































\begin{sidewaysfigure} 
\begin{center} 
\epsfig{file=lift.eps, scale=.8}
\end{center}
      \caption{A commutativie diagram}
      \label{fig:lift}
\end{sidewaysfigure} 



\ignore{\begin{figure} 
\psfragscanon
\psfrag{P}{$P\not = NP$ and $\#P\not = NC$ conjectures (characteristic zero)}
\epsfig{file=barriers.eps, scale=1}
      \caption{The feasibility barrier towards $P$ vs. $NP$}
      \label{fig:barriers}
\end{figure}}



==> lecture1_3.tex <==
\section{{\bf \LARGE Lecture 1 (Overview)}}

The goal of this lecture is to give a high level overview of 
geometric complexity theory (GCT), an 
approach towards the fundamental lower bounds in complexity theory; 
specifically
\ignore{The complexity classes that we are concerned with 
are the well known ones: $P$, the class of problems that can be solved 
in polynomial time,  $NP$, the class of problems whose solutions can be
verified in polynomial time,  $\#P$, the counting class
associated with $NP$,  and 
$NC$, the class of problems that can be solved 
in polylogarithmic time using polynomial number of processors.
The  fundamental lower bound problems that we are concerned with are:}

\noindent (1) 
The $P$ vs. $NP$ problem \cite{cook,karp,levin}: 
 show that $P \not = NP$;


\noindent (2) 
The  $\#P$ vs. $NC$ problem \cite{valiant}: show that 
$\#P \not = NC$.

We shall be dealing with the  
nonuniform versions of these problems 
in characteristic zero; i.e., when
the underlying field of computation is of characteristic zero, 
say $\Q$ or $\C$.  The additional problems that
need to be addressed when the underlying field of computation is finite
would be discussed in  GCT11. 

The nonuniform (characteristic zero) version of the $\#P$ vs. $NC$ problem
is also referred to as the permanent vs. determinant problem \cite{valiant}. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented 
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$; cf. Figure~\ref{fig:matrices}. 
By linear representation, we mean
the  entries  $y_{ij}$'s of $Y$ are affine (i.e., possibly nonhomogeneous) 
linear combinations 
of the entries $x_{lk}$'s of $X$. %; i.e., 
%\[ y_{i j} = \sum_{l,k\le n} a_{i,j}^{l,k} x_{l,k} + a_{i,j}^{n+1,n+1}, \]
%for some complex 
%$a_{i,j}^{l,k}$, $l,k \le n+1$, $i,j \le m$.
There is an analogous characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.


The main results of GCT hold for the characteristic zero versions 
of both of these problems. But we shall 
concentrate here on only the characteristic zero,  nonuniform
version of the $\#P$ vs. $NC$ problem, since this illustrates all the basic
ideas. In this lecture we outline  the GCT approach to this 
problem via algebraic geometry and representation theory, and
elaborate it further in the next two lectures.

\ignore{
\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes}
      \label{fig:complexityclasses}
\end{figure} 
}

\begin{figure}
\begin{center}
\psfragscanon
\psfrag{X}{$X$}
\psfrag{Y}{$Y$}
\psfrag{n}{$n$}
\psfrag{m}{$m$}
\psfrag{xlk}{$x_{l k}$}
\psfrag{yij}{$y_{i j}$}
\psfrag{barX}{$\bar X$}
\epsfig{file=matrices.eps, scale=.6}
\end{center}
      \caption{Linear representation $Y$ of a matrix $X$}
      \label{fig:matrices}
\end{figure} 


\section*{Why is algebraic geometry needed?}
But first we have to  explain  why algebraic 
geometry is even needed, when the statements of these problems are 
purely elementary.

It would be helpful to review the development
of GCT in this context. It  began with a  concrete
lower bound result, namely, the special case of the $P \not = NC$ conjecture
 \cite{GCTpram}, which says that 
the $P$-complete max-flow problem
cannot be solved in $\polylog(n)$ parallel time using $\poly(n)$ 
processors in the PRAM model without bit operations, which
includes virtually all known parallel algorithms for algebraic 
and weighted optimization problems;  here $n$ denotes
the total bit length of the input (not just the number of input parameters).
We shall refer to this result
 as the {\em weak  form} of the $P$ vs. $NC$ problem. Its  proof is
based on classical algebraic geometry, and as such, this may be regarded  
as  the first unconditional lower bound result to come out of GCT. 
Since it is a formal implication of the usual $P \not = NC$ conjecture,
it can be stated in purely elementary, combinatorial terms. And yet 
no elementary combinatorial proof of  this result is known so far. 
This suggested that geometry may be indipensible for
the deeper study of the fundamental lower bound problems.



Another evidence is provided by the following 
weak form of the $\#P$ vs. $NC$ problem. 
To define it, we have to first give an equivalent 
homogeneous restatement of the permanent vs. determinant problem. 
Let $\bar X$ be an $(n+1)\times (n+1)$ variable matrix. 
We identify $X$ with the $n \times n$ principal top-left minor of $\bar X$.
Let $z=\bar x_{n+1,n+1}$ be the bottom-right entry of $\bar X$, which is
not in $X$; we will use it as a homogenizing variable; 
cf. Figure~\ref{fig:matrices}.
The problem now is to show that, 
when $n$ is large enough, there does not exist an $m\times m$ matrix $Y$,
whose entries $y_{ij}$'s are homogeneous linear combinations of the entries 
$\bar x_{l,k}$'s  of $\bar X$,  such that, 
$\perm(X)z^{m-n}=\det (Y)$, with  $m$ as above. 
By homogeneous linear combination, we mean
\[ y_{i j} = \sum_{l,k\le n+1} a_{i,j}^{l,k} \bar x_{l,k}, \] 
for some complex $a_{i,j}^{l,k}$, $l,k \le n+1$, 
$i,j \le m$.
It is easy to check that this homogeneous form 
of the permanent vs. determinant problem is equivalent to the nonhomogeneous 
form given before.  

By the classical theorem of symmetric functions, 
$\det(Y)$ can be written explicitly as a polynomial 
$e(w_0, \ldots, w_{m})$, where $w_i =\trace(Y^i)$. 
Hence, the following can be thought of as 
a weaker  homogeneous  form of the $\#P$ vs. $NC$ problem:

\begin{theorem}   \label{tweak}

\noindent (a) [The weak form of the $\#P$ vs. $NC$ problem]: 
There do not exist complex numbers $b_i^l, c_j^k$, $l,k \le n+1$, $i,j \le m$,
and a polynomial $e(w_0,\ldots, w_m)$, 
such that, with 
\[ y_{i j} = \sum_{l,k\le n} b_i^l c_j^k  \bar x_{l,k}, \]
$\perm(X)z^{m-n}=g(Y)$, where  $g(Y)=e(\trace(Y^0),\ldots, \trace(Y^m))$, 
and  $m$ is as above. In fact, this holds
for any $m\ge n$. 

\noindent (b) Analogous  weak form of generalized $\#P$ vs. $NC$ problem,
obtained by replacing the  the permanent and
the trace by their suitable generalizations (cf. Lecture3), also holds.
\end{theorem} 


The part (a) has an elementary algebraic-geometric proof \cite{GCT2append}  and
also an elementary linear algebraic proof \cite{boris}.
But these do not extend to (b) and have
a serious limitation: they  work for most functions in place of the permanent.
That is, they  cannot cross the
natural proof barrier in \cite{rudich}, and hence,  such  
proof strategies cannot   work for the general problem. 
During the course of these lectures, we shall instantiate the 
basic plan of GCT for the general form to provide a ``correct'' 
geometric proof for both (a) and (b) 
that  does not have such limitations and has a right  structure 
for the general problem.  We do not have  such  an elementary 
proof for (a), and for  (b), we do not have any elementary proof,
``correct'' or ``incorrect'', though it has an elementary statement just
like (a).

The weak form, which was not mentioned in the earlier GCT papers,
is   used here only as a test example  to illustrate 
the basic ideas of the proof technique; it cannot be considered as 
a lower bound result since it holds for any $m\ge n$. 




\section*{Basic plan} 
We now outline the basic  plan of GCT focussing on
the general permanent vs. determinant problem in characteristic zero. 


The first  step (GCT1,2) is to reduce this nonexistence problem 
to an existence problem--specifically, to the problem of proving 
existence of a family $\{O_n\}$ of obstructions; 
cf. Figure~\ref{fig:firststep}.
Here an {\em obstruction} $O_n$ is a proof-certificate of
hardness of $\perm(X)$, $X$ an $n\times n$ variable matrix,
just as the Kurotowski minor is a proof-certificate of nonplanarity of a 
graph.  Specifically,  it is some 
algebro-geometric-representation-theoretic gadget, 
whose existence for every $n$,  serves as a 
guarantee that $\perm(X)$ cannot be represented linearly as $\det(Y)$,
when $m=2^{\log^a n}$, $a>0$ fixed, $n\rightarrow \infty$. 

\begin{figure} 
\begin{center}\psfragscanon
\psfrag{on}{$\{O_n\}$}
\epsfig{file=firststep.eps, scale=.8}
\end{center}
      \caption{Reduction from nonexistence to existence}
      \label{fig:firststep}
\end{figure}


This reduction to existence is carried out as follows.
First, we associate (GCT1) with 
the complexity class $\#P$ a family $\{X_{\#P}(n,m)\}$ of (group-theoretic)
class varieties, and with the complexity class $NC$ a family of 
$\{X_{NC}(n,m)\}$ of (group-theoretic) class varieties such that: 
if $\perm(X)$, $\dim(X)=n$, can be represented linearly 
as $\det(Y)$, $\dim(Y)=m>n$, then 

\begin{equation} \label{eqembed} 
X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation} 

Each  class variety is a  (projective) algebraic variety, by which
we mean the zero set of  a system of mutivariate 
homogeneous polynomials with coefficients in $\C$  (akin to the 
usual curves  and surfaces). It is  group-theoretic in the 
sense that it is  constructed using group-theoretic operations 
and the general linear group $G=GL_l(\C)$, $l=m^2$, of $l\times l$ invertible
complex matrices acts on it. Here action means moving the points 
of the class variety around, just as $G$ moves the points of $\C^l$ around 
by the standard action via invertible linear transformations.
The goal is to show that the inclusion (\ref{eqembed}) is impossible;
cf. Figure~\ref{fig:class}. 

\begin{figure} 
\begin{center} \psfragscanon
\psfrag{xsharp}{$X_{\#P}(n,m)$}
      \psfrag{xnc}{$X_{NC}(n,m)$}
      \psfrag{g}{$G=GL_l(\C)$, $l=m^2$}
      \psfrag{Obstruction}{\mbox{Obstruction}}
\epsfig{file=class.eps, scale=.5}
\end{center}
      \caption{Class varieties}
      \label{fig:class}
\end{figure} 



Since each class variety has a $G$-action, the space of polynomial functions 
on each class variety has a  representation-theoretic structure, which 
puts constraints on which  representations of $G$ can live on that variety
(i.e. in the space of polynomial  functions on that variety).
Informally, an obstruction is an irreducible (minimal)  representation of $G$
that can live on $X_{\#P}(n,m)$ but not on $X_{NC}(n,m)$; 
cf. Figure~\ref{fig:class}.
Existence of  an obstruction $O_n$, for every $n$, assuming
$m=2^{\log^a n}$, $a>1$ fixed, implies  that the inclusion (\ref{eqembed}) 
is not possible, since  $O_n$ cannot live  on $X_{NC}(n,m)$.
Thus  an obstruction blocks the inclusion (\ref{eqembed}).


To define an obstruction formally, we need to recall some basic representation
theory.  By a classical result of Weyl, the irreducible 
(polynomial) representations of $G=GL_l(\C)$ are in one-to-one correspondence 
with the partitions  $\lambda$ of length at most $l$, by which we mean 
integral sequences $\lambda_1 \ge 
\lambda_2 \cdots \ge \lambda_k > 0$, $k\le l$, where  $k$ is called the  length
of $\lambda$. The irreducible 
representation of $G$ in correpsondence with $\lambda$ is denoted 
by $V_\lambda(G)$, and is called the {\em Weyl module} of $G$ indexed by 
$\lambda$. Symbolically:

\[\mbox{Irreducible representations of } G \stackrel{\mbox{Weyl}}{\Longleftrightarrow} \quad \mbox{partitions} \ \lambda. \]  

\[\mbox{Weyl module  } V_\lambda(G)  \longleftrightarrow \lambda. \] 
Weyl also proved that every finite dimensional representation of $G$ 
can be decomposed into irreducible representations--i.e.,
can be written as a direct sum of Weyl modules. Thus Weyl modules 
are basic building blocks of the representation theory of 
$G$, and every finite dimensional representation of $G$ can be thought
of as a complex building made out of these blocks. 


Now suppose $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$. 
Suppose to the contrary that 

\begin{equation} \label{eqembed2}   X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation}

Let $R_{\#P}(n,m)$ denote the homogeneous coordinate ring of 
$X_{\#P}(n,m)$; i.e., the ring of polynomial functions on $X_{\#P}(n.m)$
(though the  functions here are not functions in usual sense;
but let us  not worry about this). 
Let $X_{\#P}(n,m)_d$ be the degree-$d$-component of $X_{\#P}(n, m)$ consisting
of functions of degree $d$. We define $R_{NC}(n,m)$ and $R_{NC}(n,m)_d$
similarly. Since $X_{\#P}(n,m)$ has the action of $G$, $R_{\#P}(n,m)$ 
also has an action of $G$; i.e., it is a representation of $G$. Hence,
$R_{\#P}(n,m)_d$ is a finite dimensional representation of $G$. 
Similarly, $R_{NC}(n,m)$ is a representation of $G$, and $R_{NC}(n,m)_d$
a finite dimensional representation of $G$. 



If (\ref{eqembed2} holds, then we get a natural map from $R_{NC}(n,m)$ to
$R_{\#P}(n,m)$ obtained by restriction of a function on $X_{NC}(n,m)$ to
$X_{\#P}(n,m)$. %; cf. Figure~\ref{fig:restriction}.
By basic algebraic geometry, this map
is surjective and is a $G$-homomorphism.
Furthermore, it is degree-preserving. This means there
is a surjective $G$-homomorphism from $R_{NC}(n,m)_d$ to 
$R_{\#P}(n,m)_d$. Symbolically: 

\begin{equation} \label{eqsurjection}
R_{\#}(n,m)_d \leftarrow  R_{NC}(n,m)_d.
\end{equation}

\ignore{
\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{Xp}{\small $X_{\#P}(n,m)$}
\psfrag{Xnc}{\small $X_{NC}(n,m)$}
\epsfig{file=restriction.eps, scale=.6}
\end{center}
      \caption{Restriction}
      \label{fig:restriction}
\end{figure}
}

Let $R_{\#P}(n,m)_d^*$ denote the dual of $R_{\#P}(n,m)_d$; i.e., the 
set of linear maps from $R_{\#P}(n,m)_d$ to $\C$. Then (\ref{eqsurjection})
implies that there is an injective $G$-homomorphism from 
$R_{\#P}(n,m)^*$ to $R_{NC}(n,m)^*$. Symbolically: 

\begin{equation} \label{eqinclusion}
R_{\#}(n,m)_d^*  \hookrightarrow {NC}(n,m)_d^*.
\end{equation}

\begin{defn} (GCT2)
An obstruction $O_n$ is a Weyl module $V_\lambda(G)$ that 
occurs as a subrepresentation 
in $R_{\#P}(n,m)_d^*$  but not in $R_{NC}(n,m)_d^*$, for some $d$. 
We call $\lambda$ an {\em obstruction label}, and sometimes,
by abuse of notation, an obstruction as well.
\end{defn}

\begin{prop} (GCT2)
Existence of an obstruction $O_n$, for all $n\rightarrow \infty$, 
with $m=2^{\log^a n}$, $a>1$ fixed, implies $\perm(X)$, $\dim(X)=n$, 
cannnot be represented linearly as 
$\det(Y)$, $\dim(Y)=m$. 
\end{prop}

This follows just from the definition of an obstruction, and 
leads to:

\begin{goal} 
Prove existence of an obstruction family $\{O_n\}$ using 
the {\em exceptional} nature of $\perm(X)$ and $\det(Y)$. 
\end{goal} 

Exceptional here means completely characterized by the symmetries 
in the following sense. 
Let  $Y$ be a variable $m\times m$ matrix.
Let $\sym^m(Y)$ be the space of homogeneous forms of degree $m$ 
in the $m^2$ variable entries of $Y$. Then, by the  classical
representation theory,  $\det(Y)$ is the only form in $\sym^m(Y)$ 
such that, for any $A,B \in GL_m(\C)$ with $\det(A)\det(B)=1$, 
\[ \det(Y)=\det(A Y^* B), \] 
where $Y^*=Y$ or $Y^t$. 
Thus $\det(Y)$ is completely characterized 
by its symmetries, and hence, is  exceptional.

Simlarly, $\perm(X)$ is the only form 
in the space of forms of degree $n$ in the entries of $X$ such that, 
for any diagonal or permutation matrices $A,B$, 
\[ \perm(X)=\perm(AX^*B), \]
where $X^*=X$ or $X^t$. 
Thus $\perm(X)$ is also
completely characterized   by its symmetries, and hence, is
exceptional.


\subsection*{The weak case}
\begin{theorem} \cite{GCT2append} \label{tgct2append}
There exists a family  $\{O_n\}$ of obstructions in the weak form of 
the generalized $\#P$ vs. $NC$ problem in characteristic zero.
\end{theorem}

(The class varieties and obstructions are defined in a similar fashion 
in the weak form--we omit their formal definitions). This result 
implies Theorem~\ref{tweak}. %, and provides its 
% ``correct'' proof. 
We shall outline it briefly in the next lecture.
It involves a detailed study of the $G$-action on class varieties
based on:
\begin{enumerate} 
\item The work on stability in geometric invariant theory by 
Hilbert, Mumford, Kempf and others \cite{mumford}. 
\item Peter-Weyl theorem for $G=GL_l(\C)$, which is the algebraic form 
of the (noncommutative) harmonic analysis on the unitary group 
$U_l(\C)$, and 
\item An extension of an induction technique 
in the Borel-Weil theorem of geometric representation theory.
\end{enumerate}

\subsection*{The general case} 
Now we proceed to the general case, our  main interest. 

Towards that end, we  associate with the class varieties 
certain representation-theoretic {\em stretching} functions. 
Let $F_{\lambda,n,m}(k)$ denote the number of occurences (multiplicity)  of
the Weyl module $V_{k\lambda}(G)$ in $R_{\#P}(n,m)$ as a subrepresentation,
and $G_{\lambda,n,m}(k)$ the number of occurences of 
$V_{k\lambda}(G)$ in $R_{NC}(n,m)$. These are statistical functions
associated with the class varieties, where the statistics associates 
with every number (stretching parameter) $k$  
the multiplicity of the corresponding
Weyl module $V_{k\lambda}(G)$; cf. Figure~\ref{fig:statistics}.

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{l}{$\lambda$}
\psfrag{2l}{$2 \lambda$}
\psfrag{3l}{$3 \lambda$}
\psfrag{v1}{$V_\lambda(G)$}
\psfrag{v2}{$V_{2 \lambda}(G)$}
\psfrag{v3}{$V_{3\lambda}(G)$}
\epsfig{file=statistics.eps, scale=1}
\end{center}
      \caption{statistics}
      \label{fig:statistics}
\end{figure}

%We will also need a definition.
Let us  call a function $f(k)$ quasipolynomial, if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k)$ for all nonnegative integral $k=i$ modulo $l$; $l$ is
called the period of the quasi-polynomial. Thus  quasi-polynomials
are hybrids of  polynomial and periodic functions. 

A fundamental example of a quasi-polynomial is the Ehrhart quasi-polynomial
$f_P(k)$ of a polytope $P$ with rational vertices. It is defined
to be the number of integer points in the dilated polytope $kP$. By the 
classical result of Ehrhart, it is known to be a quasi-polynomial.




\begin{theorem} (GCT6) \label{tquasi}
The functions $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ 
are quasi-polynomials assumming that the singularities of the class varieties
$X_{\#P}(n,m)$ and $X_{NC}(n,m)$ are rational. 

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem} 

Here rational singulary means a singularity that is nice in
a certain algebro-geometric sense that we shall not elaborate.

The proof of this result follows from a detailed study of the behaviour
of the singularities of class varieties under the action of the 
group $G$. This is based on
\begin{enumerate} 
\item The 
resolutions of singularities in characteristic zero, as per 
Hironaka \cite{hironaka}: 
this  roughly says 
that the singularities of any algebraic variety in characteristic zero
can be untangled (resolved) nicely in a systematic fashion; cf.
 Figure~\ref{fig:resolution}.
\item Cohomological works of Boutot, Brion,  Flenner, Kempf  and others
bases on this resolution; cf.  \cite{boutot} and GCT6 for other references.
\end{enumerate} 


\begin{figure} 
\begin{center} 
\epsfig{file=resolution.eps, scale=.5}
      \caption{Resolution}
      \label{fig:resolution}
\end{center}
\end{figure}


As such, this proof is highly nonconstructive. It gives no effective
bound on the period $l$--it just says that $l$  is finite.
It is a recurrent phenomenon in geometric representation theory that 
whenvever the  stretching function associated with a fundamental
multiplicity is a quasi-polynomial, it turns out to be an Ehrhart
quasi-polynomial of some polytope. This and other evidence given 
in GCT6 leads to:

\begin{hypo} {\bf (PH) [Positivity Hypothesis]} \label{hph}
For every $\lambda,n,m\ge n$, 
there exist polytopes $P=P_{\lambda,n,m}$ and $Q=Q_{\lambda,n,m}$ 
such that 
\begin{equation} 
\begin{array}{l}
F_{\lambda,n,m}(k)=f_P(k), \\
G_{\lambda,n,m}(k)=f_Q(k).
\end{array}
\end{equation}
It is also assumed here that there exists for $P_{\lambda,n,m}$ a specification
of the form $A x \le b$, where $A$ is independent of $\lambda$, and $b$ is 
a piecewise homogeneous linear function of $\lambda$, so that
$P_{k\lambda,n,m}=k P_{\lambda,n,m}$. Similarly for $Q_{\lambda,n,m}$.
If such $P$ and $Q$ exist, their dimensions are guaranteed to be
polynomial in $n$ and the length of $\lambda$
by the proof of Theorem~\ref{tquasi}.

Analogous positivity hypothesis for the $P$ vs. $NP$ problem in characteristic
zero.
\end{hypo} 

When PH holds, we say that $F_{\lambda,n,m}(k)$ and 
$G_{\lambda,n,m}(k)$ have {\em positive convex representations}. 
Here positivity refers to the fact that the Ehhart quasipolynomial 
$f_P(k)$ is a positive expression:
\[ f_P(k)=\sum_{v} 1,\] 
where $v$ ranges over all integer points in $kP$--there are no 
alternating signs in this expression.
Convexity refers to the  convexity of the polytopes $P$ and $Q$. 

\begin{theorem} (GCT6)
There exists a family $\{O_n\}$ of obstructions 
for the general $\#P$ vs. $NC$ problem in characteristic zero, 
for $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$, 
assuming, 

\begin{enumerate} 
\item PH, and
\item OH (Obstruction Hypothesis): 

For all $n\rightarrow \infty$,  there exists $\lambda$ such that 
$P_{\lambda,n,m}\not = \emptyset$ and $Q_{\lambda,n,m}=\emptyset$.
\end{enumerate}

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem}

We call  $\lambda$ a {\em relaxed obstruction}
(or rather, relaxed obstruction-label)
if it satisfies OH. In this case, $k\lambda$, for some integer $k\ge 1$ is
an obstruction--we just have to choose $k$ so that the scaled polytope 
$P_{k\lambda,n,m}=k P_{\lambda,n,m}$ contains an integer point 
($Q_{k \lambda,n,m}=k Q_{\lambda,n,m}$  continues to be empty). 
Henceforth, whenever we say obstruction, we actually mean relaxed 
obstruction.




\subsection*{The flip: Explicit construction of obstructions (GCT6,GCTflip)} 
In principle PH may have a nonconstructive proof, like that
of Theorem~\ref{tquasi}, which only tells  that such polytopes 
exist without explicitly constructing them. But proving OH may not be feasible
unless the polytopes $P$ and $Q$ in PH are given explicitly.
This  suggests the following strategy for proving 
existence of obstructions.


\noindent (1) Prove the following stronger explicit form 
of PH, which is reasonable since the polytopes $P$ and $Q$, if they exist,
are already guaranteed to be of small (polynomial) dimension:

\begin{hypo} {\bf (PH1)} 
There exist {\em explicit} 
polytopes $P_{\lambda,n,m}$ and $Q_{\lambda,n,m}$ satisfying PH.
Explicit means: 

\begin{enumerate}
\item  The polytopes are specified by explicit systems of linear constraints,
each constraint of bitlength $\poly(n,\bitlength{\lambda}, \bitlength{m})$
(note occurence of  $\bitlength{m}$  instead of $m$), such that given 
a point $x$, whether it satisfies a given constraint can be decided 
in polynomial time; i.e., in time polynomial in
$n$, the bitlength $\bitlength{\lambda}$ of $\lambda$, the 
bitlength $\bitlength{x}$ of $x$ and $\bitlength{m}$. 


\item  The membership problems for the polytopes
$P_{\lambda,n,m}$ and $Q_{\lambda,n,m}$ also 
belong to the complexity class $P$.
That is,  given a point $x$, whether it belongs to $P_{\lambda,n,m}$ 
or $Q_{\lambda,n,m}$ can also be decided in polynomial time.
Furthermore, we assume that if $x$ does not belong to the polytope,
then the membership algorithm also gives a hyperplane separating 
$x$ from the polytope in the spirit of \cite{lovasz}. 
\end{enumerate} 
\end{hypo}


In particular, PH1 implies that the functions $F_{\lambda,n,m}(k)$ and
$G_{\lambda,n,m}(k)$ belong to the complexity class $\#P$. 


\noindent (2a) {\bf [The flip]}

Let $m=2^{\log ^a n}$, for a fixed $a>1$. 
Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
show existence of  an {\em explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of obstructions  satisfying OH. 
We say that an obstruction (proof-certificate) 
$\lambda_n$ is {\em explicit} if is ``short'' and ``easy to verify'':


\begin{enumerate} 
\item  Short: This means its bitlength $\bitlength{\lambda_n}$ 
is $\poly(n)$,
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  

\item Easy to verify: given $n, m \le 2^{\log^a n}$ and 
$\lambda_n$, whether 
$\lambda_n$ is a valid obstruction 
can be verified 
in $\poly(n,\bitlength{\lambda})$ time. In particular, this is
$\poly(n)$ when $\bitlength{\lambda}=\poly(n)$. 
\end{enumerate}

Existence of an explicit family of obstructions is equivalent to saying
that the problem of deciding existence of obstructions belongs to $NP$.
This definition of explicitness is quite natural since the class $NP$ 
is a class of problems whose proof-certificates (witnesses) are 
short and easy to verify. As such, the flip--going for 
explicit  obstructions--is
a proof-strategy that is literally given to us on a platter 
by the $P$ vs. $NP$ 
problem itself. Why it is called flip would be explained later.


It should be stressed that we are primarily interested in only proving 
existence of obstructions. Whether they are explicit or not 
does not really matter in the original statement of the problem.
But we need to know the polytopes $P$ and
$Q$ explicitly (PH1)  so that proving OH is feasible. 
%In other words,   if we do not
%even know what the polytopes $P$ and $Q$ look like, 
%it seems unlikely that anything  could be said regarding OH. 
But once  PH1 is proved, existence of an explicit family follows
automatically,   as a bonus, whether we care for it or not. 

To see why, let us observe that 
the second condition above  (ease of verification) follows directly
from PH1 and the polynomial time algorithm for 
linear programming on  polytopes given by separation oracles \cite{lovasz}. 
Shortness  also follows from PH1. 

Thus it is as if the $P$ vs. $NP$ problem is forcing us to go
for explicit obstructions.


\noindent (2b) {\bf [The strong flip (optional)]} 

Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
construct (rather than just show existence of) 
a {\em strongly explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of obstructions  satisfying OH. We say that an explict family 
of obstructions is strongly explicit if,
for each $n$, a valid obstruction-label
$\lambda_n$ can be constructed in $\poly(n)$ time.
In particular, the height and the bitlength of
 $\lambda$ is $\poly(n)$ (short) 
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  


For the purposes of the lower bound problems that we are interested in, the
flip (just explicit  
existence) would suffice and the stronger flip (explicit construction)
is optional. But the stronger flip can give us deeper insight into these
lower bound problems; cf. GCTflip for more on this.

Now we turn to a few obvious questions.

\subsection*{Why should PH, PH1,  and OH hold?} 

Mathematical evidence for this is given in GCT2,4,6,7,8.
We shall discuss this a bit in the third lecture.


\subsection*{What has been achieved by all this?: The meaning of the flip} 
Let us now see what has been achieved so far
in the context of the 
$\#P\not = NC$ conjecture in the nonuniform setting (characteristic zero),
the argument for the $P$ vs. $NP$ problem in characteristic zero
being  similar. The goal of this conjecture is to prove that 
$\perm(X)$ cannot be computed by an arithmetic circuit $C$ over $X$ with
coefficients in $\C$ of size $m=\poly(n)$, or more generally,
$m \le 2^{\log^a n}$, for some fixed $a>1$, and depth $O(\log^a n)$.
Or in symbols:

\begin{equation} \label{eqioh} 
 {\bf (IOH):}  \forall n  \forall C \exists X:
\perm(X)\not = f_C(X),
\end{equation} 

where $f_C(X)$ denotes the function computed by $C$, and $n$ is supposed
to be sufficiently large.
For given $X$ and $C$ of $\poly(n)$ size, the problem 
of deciding if  $\perm(X) = f_C(X)$ belongs to $\#P$ (or rather, $P^{\#P}$). 
Since there are two alternating layers of quantifiers in (\ref{eqioh}),
the problem of verifying it belongs to $\Pi^2 \#P$, 
which is very high in the complexity hierarchy
(cf. Figure~\ref{fig:IOHcomplexity}).
Hence, we  refer to the original hypothesis (\ref{eqioh}) 
to be proven  as IOH 
(Infeasible Obstruction Hypothesis). Of course, IOH is expected to 
be a tautology, and hence is expected to  be verifiable in $O(1)$ time--but
we do not know that as yet. 



\begin{sidewaysfigure} 
\begin{center}
\psfragscanon
\psfrag{sigma2p}{{\small $\Pi^2 \#P$}}
\psfrag{sigma1p}{$\Sigma^1 \#P$}
\psfrag{P}{{\small $P$}}
\psfrag{NP}{{\small $NP$}}
\psfrag{T}{$T$}
\psfrag{#P}{$\# P$}
\psfrag{inNP}{$\in NP$}
\psfrag{inP}{$\in P$}
\psfrag{insigma2p}{$\in \Pi^2 \#P$}
\psfrag{PHplus}{PH1}
\psfrag{PHtil}{$PH^\dagger$}
\epsfig{file=IOHcomplexity.eps, scale=.8}
\end{center}
      \caption{Positivity as a means to eliminate the quantifiers and 
reduce the complexity of the  obstruction hypothesis}
      \label{fig:IOHcomplexity}
\end{sidewaysfigure}



Equivalently, the goal is to prove existence of a {\em trivial obstruction},
which is a table that lists for each $C$ as above a counterexample  $X$ so that
$\perm(X)\not = f_C(X)$; cf. Figure~\ref{fig:trivial}.
The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$ and depth
$O(\log^a n)$. Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. 
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time to decide if such a table exists and construct 
one (optional) for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. So
we call  this trivial, brute force 
strategy of proving IOH, based on existence of trivial obstructions,
 an {\em infeasible strategy}. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{eq}{$\perm(X)\not = f_C(X)$}
\epsfig{file=trivial.eps, scale=.5}
\end{center}
      \caption{A trivial obstruction}
      \label{fig:trivial}
\end{figure}


In contrast, assuming PH1, the problem  of verifying OH belongs 
to $NP$ as we have already observed. Thus, assuming PH1, we have 
transformed the original infeasible obstruction 
hypothesis $IOH \in \Pi^2 \#P$ to a new  obstuction hypothesis 
$OH \in NP$, in the process bringing down the time to verify an obstruction
from the exponential (for the original trivial obstruction) to polynomial
(for the new obstruction); cf. Figure~\ref{fig:IOHcomplexity}.  
%Intuitively, the new obstruction captures  the essence of the old obstruction
%in short space.
The task of verifying  an obstruction has also been 
transformed from the infeasible (exponential-time) to the feasible 
(polynomial-time), hence the name of this strategy: the flip,
from the infeasible to the feasible.
Positivity (PH1) is used in the flip as a means  to
eliminate the quantifying variables in IOH and bring down the 
 complexity of the obstruction hypothesis;
cf. Figure~\ref{fig:IOHcomplexity}. 




This process can be extended further. Assuming an additional
positivity hypothesis PH4 to be specified below,
$OH \in NP$ can be transformed 
to POH (Positivity Obstruction Hypothesis) that belongs to $P$; i.e.,
which can be verified in polynomial time, and an obstruction,
if it exists, can also be constructed in polynomial time; 
cf. Figure~\ref{fig:IOHcomplexity}. (The hypothesis is called PH4 instead
of PH2, because PH2 and PH3 are some other positivity hypotheses in GCT6
that complement PH1). 
Once this final positivity hypothesis POH is proven, the obstruction
hypothesis is reduced to a tautology, which can be verified in
$O(1)$ time. This  would then give us 
the final $O(1)$-size  proof. 

Thus the basic idea of the flip is to use positivity systematically
as a means to elminate the quantifiers  and reduce the complexity 
of the  obstruction hypothesis until it is finally
reduced to  an $O(1)$-time verifiable  tautology;
cf. Figure~\ref{fig:IOHcomplexity}. 

Now let us specify PH4 and POH.
Towards that end, let  $k \le l=m^2$ be the length of $\lambda$.
Define 

\begin{equation} 
\begin{array}{l}
\bar P_{n,m}= \{ \lambda: P_{\lambda,n,m} \not = \emptyset \} \subseteq \C^k, \\
\bar Q_{n,m}= \{ \lambda: Q_{\lambda,n,m} \not = \emptyset \} \subseteq \C^k.
\end{array}
\end{equation}

Then: 

\begin{hypo}  {\bf PH4} 

The sets $\bar P_{n,m}$ and $\bar Q_{n,m}$ are convex polytopes in $\C^k$.
Furthermore, the membership problems for these problems belong to 
$P$ and so also the problem of deciding if $\mbox{vol}(\bar P_{n,m}
\setminus \bar Q_{n,m})$, the volume of the relative complement 
$\bar P_{n,m} \setminus \bar Q_{n,m}$, is nonzero (positive);
i.e. if $\bar P_{n,m} \subseteq \bar Q_{n,m}$. By polynomial time,
we mean $\poly(n,l,\bitlength{m})$ time. This is $\poly(n)$,
if $m\le 2^{o(n)}$ and $l =\poly(n)$. 
\end{hypo}

\begin{hypo} {\bf (POH)}

For all $n\rightarrow \infty$, assuming $m=2^{\log^a n}$, $a>1$ fixed, 

\[ \mbox{vol}(\bar P_{n,m} \setminus \bar Q_{n,m}) > 0, \] 

for $k=(n+1)^2$. 
\end{hypo} 

\ignore{
Thus POH says that  the line-shaded area in Figure~\ref{fig:POH} has positive
volume for all large enough $n$. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{P}{$\bar P_{n,m}$}
\psfrag{Q}{$\bar Q_{n,m}$}
\epsfig{file=POH.eps, scale=1}
\end{center}
      \caption{POH}
      \label{fig:POH}
\end{figure}
}

\subsection*{How to prove PH?} 
The goal is to extend the proof of the weak 
PH needed to prove Theorem~\ref{tgct2append}
to that of the general PH in  Hypothesis~\ref{hph}.
One crucial ingradient of the weak  PH is the classical
positive convex interpretation for the Littlewood-Richardson (LR) coefficient
$c_{\alpha,\beta}^\lambda$, which is defined to be 
the number of occurences of the Weyl module $V_{\lambda(G)}$ in the 
tensor product of $V_{\alpha}(G)$ and $V_\beta(G)$; we  refer to
it as LR PH.   What is needed to prove the general PH 
is a similar positive convex interpretation for the
so-called plethysm constants in representation theory, of which the 
Littlewood-Richardson coefficient is a very special case--we shall refer to
this as Plethysm PH; cf. Lecture 3.
This  happens to be a fundamental open problem of
representation theory, older than the $P$ vs. $NP$ problem itself. It 
has been studied intensively in the last century, and is known to be
formidable. And now,  it also turns out to 
be  the heart of this approach towards the $P$ vs $NP$, the
$\#P$ vs. $NC$ problems.



A basic plan to prove Plethysm PH is given in (GCT6).
It is partially 
implemented in GCT4,6,7,8. See Figure~\ref{fig:lift} for a pictorial
depiction of the plan. It strives  to extend the  proof of LR PH based 
on the theory of the  standard quantum group \cite{drinfeld}. There it
comes out as a consequence of a  (proof of a) deep positivity result
\cite{kazhdan,lusztig}, which
we shall refer to as LR PH0. It says that   the 
tensor product of two representations of the standard quantum group 
has a canonical basis whose structure coefficients are all positive 
polynomials (i.e., polynomials with nonnegative coefficients).
The only known proof of this
result is based on the Riemann Hypothesis over finite fields (RHf) 
proved in \cite{weil2},  and the related works \cite{beilinson}. 
The Riemann Hypothesis is  itself a deep positivity statement in mathematics,
from which   LR PH can  thus be 
deduced, as shown on the bottom row of Figure~\ref{fig:lift}.

If one were only interested in LR PH, one  does not 
need this  powerful machinery, because it has a  much simpler 
algebraic-combinatorical  proof. 
But the plan to extend the
proof of LR PH to Plethysm PH in GCT6,7,8 is like a huge
inductive spiral. To  make it work,  one  needs a 
stronger inductive hypothesis than PH--this is precisely  PH0.
Thus what is needed now 
is a systematic lifting  of the bottom arrow in Figure~\ref{fig:lift}
to the top, so as to complete the  commutative diagram, so to speak. 

Initial  steps in this direction have been taken in GCT7,8. 
First, GCT7 constructs a {\em nonstandard quantumg group}, which
generalizes the notion of a standard quantum group, and plays the
same role in the plethysm setting that the standard quantum group plays
in the LR setting. Second, GCT8 gives an algorithm to construct 
a canonical basis for a representation of the nonstandard quantum group
that is conjecturally correct and has the property Plethysm PH0,
which is a   generalization of LR PH0  supported by experimental
evidence.
Now what is needed to complete  the 
commutative digram in Figure~\ref{fig:lift} is an appropriate nonstandard 
extension of the Riemann hypothesis over finite fields and the related work
from which  Plethysm PH0 can be deduced. This--the top-right corner 
of the diagram--is the big open problem,
far beyound our personal expertize. But it is 
our hope that the field of mathematics would have something to say about it.


\subsection*{How to prove OH or POH?} 
We have nothing to say on this at this point,
since the  proof of OH and POH 
would really depend on the explicit forms of the
polytopes $P$ and $Q$ that arise in   PH1. 


\subsection*{Is all this necessary?} 
Finally, one may  ask: if the positivity problems are so formidable, can
they not be avoided somehow? Unfortunately, there is a formidable 
barrier towards the $P$ vs. $NP$ and related problems, called the
{\em feasibility barrier}, which seems universal in the sense that
any approach towards these problems would have to tackle it, not just GCT. 
The existing mathematical evidence suggests that any natural approach
to cross this barrier would have to say  something deep regarding 
Plethysm PH  either explicitly or {\em implicitly}, even if
the approach does not utter a word about algebraic geometry or
representation theory.
That is,  Plethysm PH and PH0   may indeed be 
the heart of the  fundamental lower bound problems in complexity theory;
cf \cite{} for a detailed story and a precise meaning of the key 
phrase {\em implicit}.










































 

































\begin{sidewaysfigure} 
\begin{center} 
\epsfig{file=lift.eps, scale=.8}
\end{center}
      \caption{A commutativie diagram}
      \label{fig:lift}
\end{sidewaysfigure} 



\ignore{\begin{figure} 
\psfragscanon
\psfrag{P}{$P\not = NP$ and $\#P\not = NC$ conjectures (characteristic zero)}
\epsfig{file=barriers.eps, scale=1}
      \caption{The feasibility barrier towards $P$ vs. $NP$}
      \label{fig:barriers}
\end{figure}}



==> lecture1_4.tex <==
\section{{\bf \LARGE Lecture 1}}

The goal of this lecture is to give a short overview of 
geometric complexity theory (GCT), a  geometric 
approach  towards the fundamental lower bound problems  in complexity theory, 
such as (Figure~\ref{fig:complexityclasses}):

\noindent (1) 
The $P$ vs. $NP$ problem \cite{cook,karp,levin}: 
 show that $P \not = NP$;


\noindent (2) 
The  $\#P$ vs. $NC$ problem \cite{valiant}: show that 
$\#P \not = NC$.

\noindent (3) The $P$ vs. $NC$ problem: show that $P \not = NC$.

We  focus here on only the nonuniform versions of these problems 
in characteristic zero; i.e., when
the underlying field of computation is of characteristic zero, 
say $\Q$ or $\C$.  
The nonuniform (characteristic zero) version of the $\#P$ vs. $NC$ problem
is also referred to as the permanent vs. determinant problem \cite{valiant}. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented 
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$. %; cf. Figure~\ref{fig:matrices}. 
By linear representation, we mean
the  entries   of $Y$ are  (possibly nonhomogeneous) 
linear functions 
of the entries of $X$. 
There is an analogous characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.
The nonuniform
characteristic zero version of the $P\not = NC$ conjecture (in fact,
something stronger) was already proved  in \cite{GCTpram}. It will be
discussed briefly below. 


The main results of GCT for the characteristic zero 
$\#P$ vs. $NC$ problem also extend to the characteristic zero $P$ vs. $NP$
problem. But we shall 
concentrate here on only the characteristic zero (nonuniform)
$\#P$ vs. $NC$ problem, since this illustrates all the basic
ideas. In this lecture we outline  the GCT   approach 
to this problem and elaborate it further in the next two lectures.



\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes}
      \label{fig:complexityclasses}
\end{figure} 

\ignore{
\begin{figure}
\begin{center}
\psfragscanon
\psfrag{X}{$X$}
\psfrag{Y}{$Y$}
\psfrag{n}{$n$}
\psfrag{m}{$m$}
\psfrag{xlk}{$x_{l k}$}
\psfrag{yij}{$y_{i j}$}
\psfrag{barX}{$\bar X$}
\epsfig{file=matrices.eps, scale=.6}
\end{center}
      \caption{Linear representation $Y$ of a matrix $X$}
      \label{fig:matrices}
\end{figure} 
}

\noindent {\em Remark 1}: The first IAS lecture also mentioned 
a certain weak form of the $\#P$ vs. $NC$ problem. Actually, the proof
technique here leads to a substantially stronger result.
It will be discussed in Section~\ref{} of  Lecture 3.

\ignore{\noindent {\em Remark 2}: The sections marked * in this article
were not covered in the original lectures. They briefly 
address the important questions that were raised 
after the lectures, and may be skipped, if the reader wishes. 
}




\section*{Is  geometry really necessary?*}
Before we proceed further,  we have to  explain  why 
geometry is even needed to study  the problems 
under consideration, when their statements are purely elementary and
discrete.

It would be helpful to review the development
of GCT in this context. It  began with a  concrete
lower bound, namely, the special case of the $P \not = NC$ conjecture
 \cite{GCTpram}, which says that 
the $P$-complete max-flow problem
cannot be solved in $\polylog(N)$ parallel time using $\poly(N)$ 
processors in the PRAM model without bit operations, which
includes virtually all known parallel algorithms for algebraic 
and weighted optimization problems.  Here $N$ denotes
the total bit length of the input (not just the number of input parameters).
We shall refer to this result as 
{\em the characteristic zero (nonuniform) version of the $P$ vs. $NC$ problem},
though, unlike the characteristic zero versions of the $P$ vs. $NP$ and
$\#P$ vs. $NC$ problems, this one does address the issue of bitlengths.
Its  proof is
based on classical (algebraic) geometry, and as such, this may be regarded  
as  the first unconditional lower bound  to come out of GCT. 
Since it is a formal implication of the usual $P \not = NC$ conjecture 
(because the bitlengths are taken into account),
it can be stated in purely elementary, combinatorial terms. And yet, 
we do not have any  elementary combinatorial proof of  this result  so far. 

At present, this is the only analogue  of any of
the three fundamental lower bound 
problems in Figure~\ref{fig:complexityclasses}--namely, 
$P$ vs. $NP$, $\#P$ vs. $NC$ or $P$ vs. $NC$--that
we can prove unconditionally in a natural and realistic model of computation. 
Ultimately, any approach towards these  problems 
has to prove  some such 
natural and realistic analogue, though 
not necessarily this specific one, to demonstrate its effectiveness. 
That we cannot do so at present without 
geometry  seems to suggest that it may  be indipensible in their study. 

But classical (algebraic) geometry may not suffice 
in view of the  barrier towards these  problems 
pointed out  in \cite{GCTpram} (cf. its  last chapter). We shall
refer to it as the {\em algebraic degree barrier}, though it was not
given any name there. This  says that 
any low-degree proof technique, such as the one there,
which associates with a computation algebraic 
objects (polynomials, varieties, etc.) 
and then reasons solely on the basis of the degrees of those 
objects would not work.
The recent  algebrization barrier \cite{aaronson}
also says  something similar.

The article \cite{GCTpram} also suggested a plan  for bypassing the
algebraic degree barrier: namely, associate with the complexity classes 
algebraic varieties with group action, which   intuitively 
captures the symmetries of computation, and then reason on the basis of
the deeper representation theoretic structure of these
varieties, instead of just  their degrees.
This led to the construction of such varieties in \cite{GCT1}. 
The approach based on their analysis  (cf. GCT1, GCT2)
automatically bypasses the algebraic degree  barrier along with
the natural proof \cite{rudich} and relativization \cite{solovay} barriers
in characteristic zero (cf. \cite{GCTflip}). But that is
not enough. Because soon after GCT2,
this approach ran into a really formidable barrier, namely the
feasibility ($P$) barrier (cf.  GCTflip1 and \cite{GCTbarriers}), which may
be the main barrier towards  the $P$ vs. $NP$ and related problems.



The main result of GCT (cf. GCT6) says that 
this  barrier can be crossed using 
the basic strategy of GCT called  the flip (cf. GCTflip)  assuming certain
mathematical positivity hypotheses; cf. Section~\ref{}. 
It also suggests a plan for proving them, partially implemented in GCT4,7,8. 
Thus deeper geometry, along with 
algebraic geometry, representation theory, (nonstandard) quantum groups
and so forth, comes in  essentially towards crossing this
barrier. And it seems so formidable that realistically there may 
not be much  chance of crossing it without first settling some
positivity questions requiring deep geometry in one way or the other. 

This barrier is not discussed in these lectures except in passing towards
their ends; cf. GCTflip and \cite{GCTbarriers} for their detailed discussion.
The goal here is just to present the basic idea of the approach 
without worrying  about such philosophical issues.








\section*{Basic plan} 
We now outline the basic  plan of GCT focussing on
the  permanent vs. determinant problem in characteristic zero. 


The first  step (GCT1,2) is to reduce this nonexistence problem 
to an existence problem--specifically, to the problem of proving 
existence of a family $\{O_n\}$ of obstructions; 
cf. Figure~\ref{fig:firststep}.
Here an {\em obstruction} $O_n$ is a proof-certificate of
hardness of $\perm(X)$, $X$ an $n\times n$ variable matrix,
just as the Kurotowski minor is a proof-certificate of nonplanarity of a 
graph.  Specifically,  it is some 
algebro-geometric-representation-theoretic gadget, 
whose existence for every $n$,  serves as a 
guarantee that $\perm(X)$ cannot be represented linearly as $\det(Y)$,
when $m=2^{\log^a n}$, $a>0$ fixed, $n\rightarrow \infty$. 

\begin{figure} 
\begin{center}\psfragscanon
\psfrag{on}{$\{O_n\}$}
\epsfig{file=firststep.eps, scale=.8}
\end{center}
      \caption{Reduction from nonexistence to existence}
      \label{fig:firststep}
\end{figure}


This reduction to existence is carried out as follows.
First, we associate (GCT1) with 
the complexity class $\#P$ a family $\{X_{\#P}(n,m)\}$ of (group-theoretic)
class varieties, and with the complexity class $NC$ a family of 
$\{X_{NC}(n,m)\}$ of (group-theoretic) class varieties such that: 
if $\perm(X)$, $\dim(X)=n$, can be represented linearly 
as $\det(Y)$, $\dim(Y)=m>n$, then 

\begin{equation} \label{eqembed} 
X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation} 

Each  class variety is a  (projective) algebraic variety, by which
we mean the zero set of  a system of mutivariate 
homogeneous polynomials with coefficients in $\C$  (akin to the 
usual curves  and surfaces). It is  group-theoretic in the 
sense that it is  constructed using group-theoretic operations 
and the general linear group $G=GL_l(\C)$, $l=m^2$, of $l\times l$ invertible
complex matrices acts on it. Here action means moving the points 
of the class variety around, just as $G$ moves the points of $\C^l$ around 
by the standard action via invertible linear transformations.
The goal is to show that the inclusion (\ref{eqembed}) is impossible;
cf. Figure~\ref{fig:class}. 

\begin{figure} 
\begin{center} \psfragscanon
\psfrag{xsharp}{$X_{\#P}(n,m)$}
      \psfrag{xnc}{$X_{NC}(n,m)$}
      \psfrag{g}{$G=GL_l(\C)$, $l=m^2$}
      \psfrag{Obstruction}{\mbox{Obstruction}}
\epsfig{file=class.eps, scale=.5}
\end{center}
      \caption{Class varieties}
      \label{fig:class}
\end{figure} 



Since each class variety has a $G$-action, the space of polynomial functions 
on each class variety has a  representation-theoretic structure, which 
puts constraints on which  representations of $G$ can live on that variety
(i.e. in the space of polynomial  functions on that variety).
Informally, an obstruction is an irreducible (minimal)  representation of $G$
that can live on $X_{\#P}(n,m)$ but not on $X_{NC}(n,m)$; 
cf. Figure~\ref{fig:class}.
Existence of  an obstruction $O_n$, for every $n$, assuming
$m=2^{\log^a n}$, $a>1$ fixed, implies  that the inclusion (\ref{eqembed}) 
is not possible, since  $O_n$ cannot live  on $X_{NC}(n,m)$.
Thus  an obstruction blocks the inclusion (\ref{eqembed}).


To define an obstruction formally, we need to recall some basic representation
theory.  By a classical result of Weyl, the irreducible 
(polynomial) representations of $G=GL_l(\C)$ are in one-to-one correspondence 
with the partitions  $\lambda$ of length at most $l$, by which we mean 
integral sequences $\lambda_1 \ge 
\lambda_2 \cdots \ge \lambda_k > 0$, $k\le l$, where  $k$ is called the  length
of $\lambda$. The irreducible 
representation of $G$ in correpsondence with $\lambda$ is denoted 
by $V_\lambda(G)$, and is called the {\em Weyl module} of $G$ indexed by 
$\lambda$. Symbolically:

\[\mbox{Irreducible representations of } G \stackrel{\mbox{Weyl}}{\Longleftrightarrow} \quad \mbox{partitions} \ \lambda. \]  

\[\mbox{Weyl module  } V_\lambda(G)  \longleftrightarrow \lambda. \] 
Weyl also proved that every finite dimensional representation of $G$ 
can be decomposed into irreducible representations--i.e.,
can be written as a direct sum of Weyl modules. Thus Weyl modules 
are basic building blocks of the representation theory of 
$G$, and every finite dimensional representation of $G$ can be thought
of as a complex building made out of these blocks. 


Now suppose $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$. 
Suppose to the contrary that 

\begin{equation} \label{eqembed2}   X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation}

Let $R_{\#P}(n,m)$ denote the homogeneous coordinate ring of 
$X_{\#P}(n,m)$; i.e., the ring of polynomial functions on $X_{\#P}(n.m)$
(though the  functions here are not functions in usual sense;
but let us  not worry about this). 
Let $X_{\#P}(n,m)_d$ be the degree-$d$-component of $X_{\#P}(n, m)$ consisting
of functions of degree $d$. We define $R_{NC}(n,m)$ and $R_{NC}(n,m)_d$
similarly. Since $X_{\#P}(n,m)$ has the action of $G$, $R_{\#P}(n,m)$ 
also has an action of $G$; i.e., it is a representation of $G$. Hence,
$R_{\#P}(n,m)_d$ is a finite dimensional representation of $G$. 
Similarly, $R_{NC}(n,m)$ is a representation of $G$, and $R_{NC}(n,m)_d$
a finite dimensional representation of $G$. 



If (\ref{eqembed2} holds, then we get a natural map from $R_{NC}(n,m)$ to
$R_{\#P}(n,m)$ obtained by restriction of a function on $X_{NC}(n,m)$ to
$X_{\#P}(n,m)$. %; cf. Figure~\ref{fig:restriction}.
By basic algebraic geometry, this map
is surjective and is a $G$-homomorphism.
Furthermore, it is degree-preserving. This means there
is a surjective $G$-homomorphism from $R_{NC}(n,m)_d$ to 
$R_{\#P}(n,m)_d$. Symbolically: 

\begin{equation} \label{eqsurjection}
R_{\#}(n,m)_d \leftarrow  R_{NC}(n,m)_d.
\end{equation}

\ignore{
\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{Xp}{\small $X_{\#P}(n,m)$}
\psfrag{Xnc}{\small $X_{NC}(n,m)$}
\epsfig{file=restriction.eps, scale=.6}
\end{center}
      \caption{Restriction}
      \label{fig:restriction}
\end{figure}
}

Let $R_{\#P}(n,m)_d^*$ denote the dual of $R_{\#P}(n,m)_d$; i.e., the 
set of linear maps from $R_{\#P}(n,m)_d$ to $\C$. Then (\ref{eqsurjection})
implies that there is an injective $G$-homomorphism from 
$R_{\#P}(n,m)^*$ to $R_{NC}(n,m)^*$. Symbolically: 

\begin{equation} \label{eqinclusion}
R_{\#}(n,m)_d^*  \hookrightarrow {NC}(n,m)_d^*.
\end{equation}

\begin{defn} (GCT2)
An obstruction $O_n$ is a Weyl module $V_\lambda(G)$ that 
occurs as a subrepresentation 
in $R_{\#P}(n,m)_d^*$  but not in $R_{NC}(n,m)_d^*$, for some $d$. 
We call $\lambda$ an {\em obstruction label}, and sometimes,
by abuse of notation, an obstruction as well.
\end{defn}

\begin{prop} (GCT2)
Existence of an obstruction $O_n$, for all $n\rightarrow \infty$, 
with $m=2^{\log^a n}$, $a>1$ fixed, implies $\perm(X)$, $\dim(X)=n$, 
cannnot be represented linearly as 
$\det(Y)$, $\dim(Y)=m$. 
\end{prop}

This follows just from the definition of an obstruction, and 
leads to:

\begin{goal} \label{gobs}
Prove existence of an obstruction family $\{O_n\}$ using 
the {\em exceptional} nature of $\perm(X)$ and $\det(Y)$. 
\end{goal} 

Exceptional here means completely characterized by the symmetries 
in the following sense. 
Let  $Y$ be a variable $m\times m$ matrix.
Let $\sym^m(Y)$ be the space of homogeneous forms of degree $m$ 
in the $m^2$ variable entries of $Y$. Then, by the  classical
representation theory,  $\det(Y)$ is the only form in $\sym^m(Y)$ 
such that, for any $A,B \in GL_m(\C)$ with $\det(A)\det(B)=1$, 
\[ \det(Y)=\det(A Y^* B), \] 
where $Y^*=Y$ or $Y^t$. 
Thus $\det(Y)$ is completely characterized 
by its symmetries, and hence, is  exceptional.

Simlarly, $\perm(X)$ is the only form 
in the space of forms of degree $n$ in the entries of $X$ such that, 
for any diagonal or permutation matrices $A,B$, 
\[ \perm(X)=\perm(AX^*B), \]
where $X^*=X$ or $X^t$. 
Thus $\perm(X)$ is also
completely characterized   by its symmetries, and hence, is
exceptional.

We now proceed to describe the main result of GCT in the context of
Goal~\ref{gobs}. 
Towards that end, we  associate with the class varieties 
certain representation-theoretic {\em stretching} functions. 
Let $F_{\lambda,n,m}(k)$ denote the number of occurences (multiplicity)  of
the Weyl module $V_{k\lambda}(G)$ in $R_{\#P}(n,m)$ as a subrepresentation,
and $G_{\lambda,n,m}(k)$ the number of occurences of 
$V_{k\lambda}(G)$ in $R_{NC}(n,m)$. These are statistical functions
associated with the class varieties, where the statistics associates 
with every number (stretching parameter) $k$  
the multiplicity of the corresponding
Weyl module $V_{k\lambda}(G)$; cf. Figure~\ref{fig:statistics}.

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{l}{$\lambda$}
\psfrag{2l}{$2 \lambda$}
\psfrag{3l}{$3 \lambda$}
\psfrag{v1}{$V_\lambda(G)$}
\psfrag{v2}{$V_{2 \lambda}(G)$}
\psfrag{v3}{$V_{3\lambda}(G)$}
\epsfig{file=statistics.eps, scale=1}
\end{center}
      \caption{statistics}
      \label{fig:statistics}
\end{figure}

%We will also need a definition.
Let us  call a function $f(k)$ quasipolynomial, if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k)$ for all nonnegative integral $k=i$ modulo $l$; $l$ is
called the period of the quasi-polynomial. Thus  quasi-polynomials
are hybrids of  polynomial and periodic functions. 

A fundamental example of a quasi-polynomial is the Ehrhart quasi-polynomial
$f_P(k)$ of a polytope $P$ with rational vertices. It is defined
to be the number of integer points in the dilated polytope $kP$. By the 
classical result of Ehrhart, it is known to be a quasi-polynomial.




\begin{theorem} (GCT6) \label{tquasi}
The functions $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ 
are quasi-polynomials assumming that the singularities of the class varieties
$X_{\#P}(n,m)$ and $X_{NC}(n,m)$ are rational. 

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem} 

Here rational singulary means a singularity that is nice in
a certain algebro-geometric sense that we shall not elaborate.

The proof of this result follows from a detailed study of the behaviour
of the singularities of class varieties under the action of the 
group $G$. This is based on
\begin{enumerate} 
\item The 
resolutions of singularities in characteristic zero, as per 
Hironaka \cite{hironaka}: 
this  roughly says 
that the singularities of any algebraic variety in characteristic zero
can be untangled (resolved) nicely in a systematic fashion; cf.
 Figure~\ref{fig:resolution}.
\item Cohomological works of Boutot, Brion,  Flenner, Kempf  and others
bases on this resolution; cf.  \cite{boutot,dehy} and
GCT6 for the history and other references.
\end{enumerate} 


\begin{figure} 
\begin{center} 
\epsfig{file=resolution.eps, scale=.5}
      \caption{Resolution}
      \label{fig:resolution}
\end{center}
\end{figure}


As such, this proof is highly nonconstructive. It gives no effective
bound on the period $l$--it just says that $l$  is finite.
It is a recurrent phenomenon in geometric representation theory that 
whenvever the  stretching function associated with a fundamental
multiplicity is a quasi-polynomial, it turns out to be an Ehrhart
quasi-polynomial of some polytope. This and other evidence given 
in GCT6 leads to:

\begin{hypo} {\bf (PH) [Positivity Hypothesis]} \label{hph}

\noindent (a) For every $\lambda,n,m\ge n$, 
there exist a  polytope $P=P_{\lambda,n,m}$ 
such that 
\begin{equation} \label{eqP}
F_{\lambda,n,m}(k)=f_P(k).
\end{equation} 
It is also assumed here that there exists for $P_{\lambda,n,m}$ a specification
of the form $A x \le b$, where $A$ is independent of $\lambda$, and $b$ is 
a piecewise homogeneous linear function of $\lambda$, so that
$P_{k\lambda,n,m}=k P_{\lambda,n,m}$. 

\noindent (b) There exists a similar polytope  $Q=Q_{\lambda,n,m}$ 
for the function $G_{\lambda,n,m}$ such that
\begin{equation} \label{eqQ}
G_{\lambda,n,m}(k)=f_Q(k).
\end{equation}

If such $P$ and $Q$ exist, their dimensions are guaranteed to be
polynomial in $n$ and the length of $\lambda$
by the proof of Theorem~\ref{tquasi}.


Analogous positivity hypothesis also holds 
for the $P$ vs. $NP$ problem in characteristic zero.
\end{hypo} 

When PH holds, we say that $F_{\lambda,n,m}(k)$ and 
$G_{\lambda,n,m}(k)$ have {\em positive convex representations}. 
Here positivity refers to the fact that the Ehhart quasipolynomial 
$f_P(k)$ is a positive expression:
\[ f_P(k)=\sum_{v} 1,\] 
where $v$ ranges over all integer points in $kP$--there are no 
alternating signs in this expression.
Convexity refers to the  convexity of the polytopes $P$ and $Q$. 

\begin{theorem} (GCT6) \label{tgct6}
There exists a family $\{O_n\}$ of obstructions 
for the general $\#P$ vs. $NC$ problem in characteristic zero, 
for $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$, 
assuming, 

\begin{enumerate} 
\item PH, and
\item OH (Obstruction Hypothesis): 

For all $n\rightarrow \infty$,  there exists $\lambda$ such that 
$P_{\lambda,n,m}\not = \emptyset$ and $Q_{\lambda,n,m}=\emptyset$.
\end{enumerate}

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem}

We call  $\lambda$ a {\em relaxed obstruction}
(or rather, relaxed obstruction-label)
if it satisfies OH. In this case, $k\lambda$, for some integer $k\ge 1$ is
an obstruction--we just have to choose $k$ so that the scaled polytope 
$P_{k\lambda,n,m}=k P_{\lambda,n,m}$ contains an integer point 
($Q_{k \lambda,n,m}=k Q_{\lambda,n,m}$  continues to be empty). 
Henceforth, whenever we say obstruction, we actually mean relaxed 
obstruction.




\subsection*{The flip: Explicit construction of obstructions (GCT6,GCTflip)} 
In principle PH may have a nonconstructive proof, like that
of Theorem~\ref{tquasi}, which only tells  that such polytopes 
exist without explicitly constructing them. But proving OH may not be feasible
unless the polytopes $P$ and $Q$ in PH are given explicitly.
This  suggests the following strategy for proving 
existence of obstructions.


\noindent (1) Prove the following stronger explicit form 
of PH, which is reasonable since the polytopes $P$ and $Q$, if they exist,
are already guaranteed to be of small (polynomial) dimension:

\begin{hypo} {\bf (PH1)} 

\noindent (a) There exist an {\em explicit} 
polytope $P_{\lambda,n,m}$ 
as in  PH (a).
Explicit means: 

\begin{enumerate}
\item  The polytope is specified by an explicit system of linear constraints,
each constraint of bitlength $\poly(n,\bitlength{\lambda}, \bitlength{m})$
(note occurence of  $\bitlength{m}$  instead of $m$), such that given 
a point $x$, whether it satisfies a given constraint can be decided 
in polynomial time; i.e., in time polynomial in
$n$, the bitlength $\bitlength{\lambda}$ of $\lambda$, the 
bitlength $\bitlength{x}$ of $x$ and $\bitlength{m}$. 

\item  The membership problems for the polytop
$P_{\lambda,n,m}$ and $Q_{\lambda,n,m}$ also 
belong to the complexity class $P$.
That is,  given a point $x$, whether it belongs to $P_{\lambda,n,m}$ 
or $Q_{\lambda,n,m}$ can also be decided in polynomial time.
Furthermore, we assume that if $x$ does not belong to the polytope,
then the membership algorithm also gives a hyperplane separating 
$x$ from the polytope in the spirit of \cite{lovasz}. 
\end{enumerate} 

\noindent (b) Similarly,  there exists an explicit 
polytope $Q_{\lambda,n,m}$ satisfying a weaker form PH (b),
specified in Section~\ref{} of Lecture 3, which is enough for the
purposes Theorem~\ref{tgct6}; i.e., it can play the role of PH (b) there.
\end{hypo}



In particular, PH1 implies that the functions $F_{\lambda,n,m}(k)$ and
$G_{\lambda,n,m}(k)$ belong to the complexity class $\#P$. 


\noindent (2a) {\bf [The flip]}

Let $m=2^{\log ^a n}$, for a fixed $a>1$. 
Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
show existence of  an {\em explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of obstructions  satisfying OH. 
We say that an obstruction (proof-certificate) 
$\lambda_n$ is {\em explicit} if is ``short'' and ``easy to verify'':


\begin{enumerate} 
\item  Short: This means its bitlength $\bitlength{\lambda_n}$ 
is $\poly(n)$,
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  

\item Easy to verify: given $n, m \le 2^{\log^a n}$ and 
$\lambda_n$, whether 
$\lambda_n$ is a valid obstruction 
can be verified 
in $\poly(n,\bitlength{\lambda})$ time. In particular, this is
$\poly(n)$ when $\bitlength{\lambda}=\poly(n)$. 
\end{enumerate}

Existence of an explicit family of obstructions is equivalent to saying
that the problem of deciding existence of obstructions belongs to $NP$.
This definition of explicitness is quite natural since the class $NP$ 
is a class of problems whose proof-certificates (witnesses) are 
short and easy to verify. As such, the flip--going for 
explicit  obstructions--is
a proof-strategy that is literally given to us on a platter 
by the $P$ vs. $NP$ 
problem itself. Why it is called flip would be explained later.


It should be stressed that we are primarily interested in only proving 
existence of obstructions. Whether they are explicit or not 
does not really matter in the original statement of the problem.
But we need to know the polytopes $P$ and
$Q$ explicitly (PH1)  so that proving OH is feasible. 
%In other words,   if we do not
%even know what the polytopes $P$ and $Q$ look like, 
%it seems unlikely that anything  could be said regarding OH. 
But once  PH1 is proved, existence of an explicit family follows
automatically,   as a bonus, whether we care for it or not. 

To see why, let us observe that 
the second condition above  (ease of verification) follows directly
from PH1 and the polynomial time algorithm for 
linear programming on  polytopes given by separation oracles \cite{lovasz}. 
Shortness  also follows from PH1. 

Thus it is as if the $P$ vs. $NP$ problem is forcing us to go
for explicit obstructions.


\noindent (2b) {\bf [The strong flip (optional)]} 

Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
construct (rather than just show existence of) 
a {\em strongly explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of obstructions  satisfying OH. We say that an explict family 
of obstructions is strongly explicit if,
for each $n$, a valid obstruction-label
$\lambda_n$ can be constructed in $\poly(n)$ time.
In particular, the height and the bitlength of
 $\lambda$ is $\poly(n)$ (short) 
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  


For the purposes of the lower bound problems that we are interested in, the
flip (just explicit  
existence) would suffice and the stronger flip (explicit construction)
is optional. But the stronger flip can give us deeper insight into these
lower bound problems; cf. GCTflip for more on this.

Now we turn to a few obvious questions.

\subsection*{Why should PH1  and OH hold?} 

Mathematical evidence for this is given in GCT2,4,6,7,8.
We shall discuss this a bit  in the third lecture.


\subsection*{What has been achieved by all this?: The meaning of the flip} 
Let us now see what has been achieved so far
in the context of the 
$\#P\not = NC$ conjecture in the nonuniform setting (characteristic zero),
the argument for the $P$ vs. $NP$ problem in characteristic zero
being  similar. The goal of this conjecture is to prove that 
$\perm(X)$ cannot be computed by an arithmetic circuit $C$ over $X$ with
coefficients in $\C$ of size $m=\poly(n)$, or more generally,
$m \le 2^{\log^a n}$, for some fixed $a>1$, and depth $O(\log^a n)$.
Or in symbols:

\begin{equation} \label{eqioh} 
 {\bf (IOH):}  \forall n  \forall C \exists X:
\perm(X)\not = f_C(X),
\end{equation} 

where $f_C(X)$ denotes the function computed by $C$, and $n$ is supposed
to be sufficiently large.
For given $X$ and $C$ of $\poly(n)$ size, the problem 
of deciding if  $\perm(X) = f_C(X)$ belongs to $\#P$ (or rather, $P^{\#P}$). 
Since there are two alternating layers of quantifiers in (\ref{eqioh}),
the problem of verifying it belongs to $\Pi^2 \#P$, 
which is very high in the complexity hierarchy
(cf. Figure~\ref{fig:IOHcomplexity}).
Hence, we  refer to the original hypothesis (\ref{eqioh}) 
to be proven  as IOH 
(Infeasible Obstruction Hypothesis). Of course, IOH is expected to 
be a tautology, and hence is expected to  be verifiable in $O(1)$ time--but
we do not know that as yet. 



\begin{sidewaysfigure} 
\begin{center}
\psfragscanon
\psfrag{sigma2p}{{\small $\Pi^2 \#P$}}
\psfrag{sigma1p}{$\Sigma^1 \#P$}
\psfrag{P}{{\small $P$}}
\psfrag{NP}{{\small $NP$}}
\psfrag{T}{$T$}
\psfrag{#P}{$\# P$}
\psfrag{inNP}{$\in NP$}
\psfrag{inP}{$\in P$}
\psfrag{insigma2p}{$\in \Pi^2 \#P$}
\psfrag{PHplus}{PH1}
\psfrag{PHtil}{$PH^\dagger$}
\epsfig{file=IOHcomplexity.eps, scale=.8}
\end{center}
      \caption{Positivity as a means to eliminate the quantifiers and 
reduce the complexity of the  obstruction hypothesis}
      \label{fig:IOHcomplexity}
\end{sidewaysfigure}



Equivalently, the goal is to prove existence of a {\em trivial obstruction},
which is a table that lists for each $C$ as above a counterexample  $X$ so that
$\perm(X)\not = f_C(X)$; cf. Figure~\ref{fig:trivial}.
The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$ and depth
$O(\log^a n)$. Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. 
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time to decide if such a table exists and construct 
one (optional) for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. So
we call  this trivial, brute force 
strategy of proving IOH, based on existence of trivial obstructions,
 an {\em infeasible strategy}. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{eq}{$\perm(X)\not = f_C(X)$}
\epsfig{file=trivial.eps, scale=.5}
\end{center}
      \caption{A trivial obstruction}
      \label{fig:trivial}
\end{figure}


In contrast, assuming PH1, the problem  of verifying OH belongs 
to $NP$ as we have already observed. Thus, assuming PH1, we have 
transformed the original infeasible obstruction 
hypothesis $IOH \in \Pi^2 \#P$ to a new  obstuction hypothesis 
$OH \in NP$, in the process bringing down the time to verify an obstruction
from the exponential (for the original trivial obstruction) to polynomial
(for the new obstruction); cf. Figure~\ref{fig:IOHcomplexity}.  
%Intuitively, the new obstruction captures  the essence of the old obstruction
%in short space.
The task of verifying  an obstruction has also been 
transformed from the infeasible (exponential-time) to the feasible 
(polynomial-time), hence the name of this strategy: the flip,
from the infeasible to the feasible.
Positivity (PH1) is used in the flip as a means  to
eliminate the quantifying variables in IOH and bring down the 
 complexity of the obstruction hypothesis;
cf. Figure~\ref{fig:IOHcomplexity}. 




This process can be extended further. Assuming an additional
positivity hypothesis PH4 to be specified below,
$OH \in NP$ can be transformed 
to POH (Positivity Obstruction Hypothesis) that belongs to $P$; i.e.,
which can be verified in polynomial time, and an obstruction,
if it exists, can also be constructed in polynomial time; 
cf. Figure~\ref{fig:IOHcomplexity}. (The hypothesis is called PH4 instead
of PH2, because PH2 and PH3 are some other positivity hypotheses in GCT6
that complement PH1). 
Once this final positivity hypothesis POH is proven, the obstruction
hypothesis is reduced to a tautology (FOH), which can be verified in
$O(1)$ time. This  would then give us 
the final $O(1)$-size  proof. 

Thus the basic idea of the flip is to use positivity systematically
as a means to elminate the quantifiers  and reduce the complexity 
of the  obstruction hypothesis until it is finally
reduced to  an $O(1)$-time verifiable  tautology;
cf. Figure~\ref{fig:IOHcomplexity}. 

Now let us specify PH4 and POH.
Towards that end, let  $k \le l=m^2$ be the length of $\lambda$.
Define 

\begin{equation} 
\begin{array}{l}
\bar P_{n,m}= \{ \lambda: P_{\lambda,n,m} \not = \emptyset \} \subseteq \C^k, \\
\bar Q_{n,m}= \{ \lambda: Q_{\lambda,n,m} \not = \emptyset \} \subseteq \C^k.
\end{array}
\end{equation}

Then: 

\begin{hypo}  {\bf PH4} 

The sets $\bar P_{n,m}$ and $\bar Q_{n,m}$ are convex polytopes in $\C^k$.
Furthermore, the membership problems for these problems belong to 
$P$ and so also the problem of deciding if $\mbox{vol}(\bar P_{n,m}
\setminus \bar Q_{n,m})$, the volume of the relative complement 
$\bar P_{n,m} \setminus \bar Q_{n,m}$, is nonzero (positive);
i.e. if $\bar P_{n,m} \subseteq \bar Q_{n,m}$. By polynomial time,
we mean $\poly(n,l,\bitlength{m})$ time. This is $\poly(n)$,
if $m\le 2^{o(n)}$ and $l =\poly(n)$. 
\end{hypo}

\begin{hypo} {\bf (POH)}

For all $n\rightarrow \infty$, assuming $m=2^{\log^a n}$, $a>1$ fixed, 

\[ \mbox{vol}(\bar P_{n,m} \setminus \bar Q_{n,m}) > 0, \] 

for $k=(n+1)^2$. 
\end{hypo} 

\ignore{
Thus POH says that  the line-shaded area in Figure~\ref{fig:POH} has positive
volume for all large enough $n$. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{P}{$\bar P_{n,m}$}
\psfrag{Q}{$\bar Q_{n,m}$}
\epsfig{file=POH.eps, scale=1}
\end{center}
      \caption{POH}
      \label{fig:POH}
\end{figure}
}

\subsection*{How to prove PH?} 
There is  a basic prototype of PH in representation theory,
which will be described in detail in Lecture 3. We shall
refer to it  as Plethysm PH. It says that the stretching functions 
akin to $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$
associated with  fundamental  multiplicities 
in representation theory called plethysm constants also have analogous 
positive convex representations. 

This  is   known for a very special case of the plethysm constant 
called the  Littlewood-Richardson (LR) coefficient
$c_{\alpha,\beta}^\lambda$. It is  defined to be 
the number of occurences of the Weyl module $V_{\lambda}(G)$ in the 
tensor product of $V_{\alpha}(G)$ and $V_\beta(G)$. 
The classical Littlewood-Richardson rule, which we shall refer to as LR PH,
implies that the stretching function 
$\tilde c_{\alpha,\beta}^\lambda (k) = c_{k \alpha, k \beta}^{k \lambda}$
associated with the Littlewood-Richardson coefficient has a
positive convex representation.

Plethysm PH   happens to be a fundamental open problem of
representation theory, older than the $P$ vs. $NP$ problem itself. It 
has been studied intensively in the last century, and is known to be
formidable. And  now,  as explained the third lecture, it also turns out to 
be  the heart of this approach towards the $P$ vs $NP$, the
$\#P$ vs. $NC$ problems.



A basic plan to prove Plethysm PH is given in (GCT6).
It is partially 
implemented in GCT4,6,7,8. See Figure~\ref{fig:lift} for a pictorial
depiction of the plan. It strives  to extend the  proof of LR PH based 
on the theory of the  standard quantum group \cite{drinfeld}. There it
comes out as a consequence of a  (proof of a) deep positivity result
\cite{kazhdan,lusztig}, which
we shall refer to as LR PH0. It says that   the 
tensor product of two representations of the standard quantum group 
has a canonical basis whose structure coefficients are all positive 
polynomials (i.e., polynomials with nonnegative coefficients).
The only known proof of this
result is based on the Riemann Hypothesis over finite fields (RHf) 
proved in \cite{weil2},  and the related works \cite{beilinson}. 
The Riemann Hypothesis is  itself a deep positivity statement in mathematics,
from which   LR PH can  thus be 
deduced, as shown on the bottom row of Figure~\ref{fig:lift}.

If one were only interested in LR PH, one  does not 
need this  powerful machinery, because it has a  much simpler 
algebraic-combinatorical  proof. 
But the plan to extend the
proof of LR PH to Plethysm PH in GCT6,7,8 is like a huge
inductive spiral. To  make it work,  one  needs a 
stronger inductive hypothesis than PH--this is precisely  PH0.
Thus what is needed now 
is a systematic lifting  of the bottom arrow in Figure~\ref{fig:lift}
to the top, so as to complete the  commutative diagram, so to speak. 

Initial  steps in this direction have been taken in GCT7,8. 
First, GCT7 constructs a {\em nonstandard quantumg group}, which
generalizes the notion of a standard quantum group, and plays the
same role in the plethysm setting that the standard quantum group plays
in the LR setting. Second, GCT8 gives an algorithm to construct 
a canonical basis for a representation of the nonstandard quantum group
that is conjecturally correct and has the property Plethysm PH0,
which is a   generalization of LR PH0  supported by experimental
evidence.
Now what is needed to complete  the 
commutative digram in Figure~\ref{fig:lift} is an appropriate nonstandard 
extension of the Riemann hypothesis over finite fields and the related work
from which  Plethysm PH0 can be deduced. This--the top-right corner 
of the diagram--is the   main  open problem at the heart of this approach. 

\subsection*{How to prove OH or POH?} 
We have nothing to say on this at this point,
since the  proof of OH and POH 
would really depend on the explicit forms of the
polytopes $P$ and $Q$ that arise in   PH1. 


\subsection*{Is all this necessary?} 
Finally, one may  ask: if the positivity problems are so formidable, can
they not be avoided somehow? Unfortunately, there is a formidable 
barrier towards the $P$ vs. $NP$ and related problems, called the
{\em feasibility barrier}, which seems universal in the sense that
any approach towards these problems would have to tackle it, not just GCT. 
The existing mathematical evidence suggests that any natural approach
to cross this barrier would have to say  something deep regarding 
Plethysm PH  either explicitly or {\em implicitly}, even if
the approach does not utter a word about algebraic geometry or
representation theory.
That is,  Plethysm PH and PH0   may indeed be 
the heart of the  fundamental lower bound problems in complexity theory;
cf \cite{GCTbarriers} for a detailed story and a precise meaning of the key 
phrase {\em implicit}.










































 

































\begin{sidewaysfigure} 
\begin{center} 
\epsfig{file=lift.eps, scale=.8}
\end{center}
      \caption{A commutativie diagram}
      \label{fig:lift}
\end{sidewaysfigure} 



\ignore{\begin{figure} 
\psfragscanon
\psfrag{P}{$P\not = NP$ and $\#P\not = NC$ conjectures (characteristic zero)}
\epsfig{file=barriers.eps, scale=1}
      \caption{The feasibility barrier towards $P$ vs. $NP$}
      \label{fig:barriers}
\end{figure}}



==> lecture1_5.tex <==
\section*{Introduction}

This article   gives an overview of the basic plan of 
geometric complexity theory (GCT), an
approach  towards the fundamental lower bound problems  in complexity theory, 
such as (Figure~\ref{fig:complexityclasses}):

\noindent (1) 
The $P$ vs. $NP$ problem \cite{cook,karp,levin}: 
 show that $P \not = NP$;


\noindent (2) 
The  $\#P$ vs. $NC$ problem \cite{valiant}: show that 
$\#P \not = NC$.

\noindent (3) The $P$ vs. $NC$ problem: show that $P \not = NC$.

We  focus here on only the nonuniform versions of these problems 
in characteristic zero; i.e., when
the underlying field of computation is of characteristic zero, 
say $\Q$ or $\C$.  The additional problems that
need to be addressed when the underlying field of computation is finite
would be discussed in  GCT11. 
The nonuniform
characteristic zero version of the $P\not = NC$ conjecture (in fact,
something stronger) was already proved  in GCTweak.
It may be considered to be the first unconditional lower bound result of
GCT, because, though it can be stated in purely elementary combinatorial
terms, being a formal implication of the $P\not = NC$ conjecture, its
proof is intrinsically geometric, and no elementary proof is known so far. 
Furthermore, its proof  technique may be considered to be a weak form 
of the {\em flip}, the basic guiding strategy of GCT, which  was 
refined and formalized much later in GCTflip. 
Hence we shall refer to this lower bound result
as the {\em weak form of the $P\not = NC$ 
conjecture}, and its proof technique as {\em weak GCT}. 
This  was the begining of  this  geometric approach in complexity theory.
The later work in GCT-- the subject of this overview--focusses on the other 
two problems above, namely
the $P$ vs. $NP$ and $\#P$ vs. $NC$ problems. 


The nonuniform (characteristic zero) version of the $\#P$ vs. $NC$ problem
is also known as the permanent vs. determinant problem \cite{valiant}. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented 
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$. %; cf. Figure~\ref{fig:matrices}. 
By linear representation, we mean
the  entries   of $Y$ are  (possibly nonhomogeneous) 
linear functions 
of the entries of $X$. 
There is an analogous characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.
The main results of GCT for the $\#P$ vs. $NC$ problem in 
characteristic zero also extend to the $P$ vs. $NP$ problem in characteristic
zero. But here we shall 
concentrate  on only the former problem,
%the
%$\#P$ vs. $NC$ problem in  characteristic zero (nonuniform),
since this illustrates all the basic ideas. 

The rest of this article is organized in the form of three chapters,
one per  lecture. The first gives an overview of the basic plan
of GCT, which is elaborated in the next two lectures. 
Original  lectures also mentioned 
a certain weak form of the $\#P$ vs. $NC$ problem. Actually, the proof
technique here leads to a much more nontrivial result.
It is discussed in the second section of  the third lecture.


\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes}
      \label{fig:complexityclasses}
\end{figure} 




The author is grateful to 
Avi Wigderson for arranging the lectures and the hospitality.


\chapter{Basic plan} 
We now outline the basic  plan of GCT focussing on
the  permanent vs. determinant problem in characteristic zero. 

\section{From nonexistence to existence}
The first  step (GCT1,2) is to reduce this nonexistence problem 
to an existence problem--specifically, to the problem of proving 
existence of a family $\{O_n\}$ of obstructions; 
cf. Figure~\ref{fig:firststep}.
Here an {\em obstruction} $O_n$ is a proof-certificate of
hardness of $\perm(X)$, $X$ an $n\times n$ variable matrix,
just as the Kurotowoski minor is a proof-certificate of nonplanarity of a 
graph.  Specifically,  it is some 
algebro-geometric-representation-theoretic gadget, 
whose existence for every $n$,  serves as a 
guarantee that $\perm(X)$ cannot be represented linearly as $\det(Y)$,
when $m=2^{\log^a n}$, $a>0$ fixed, $n\rightarrow \infty$ (i.e., for
$n$ greater than a large enough constant depending on $a$). 

\begin{figure} 
\begin{center}\psfragscanon
\psfrag{on}{$\{O_n\}$}
\epsfig{file=firststep.eps, scale=.8}
\end{center}
      \caption{Reduction from nonexistence to existence}
      \label{fig:firststep}
\end{figure}


This reduction to existence is carried out as follows; cf. lecture 2 for its
details.
First, we associate (GCT1) with 
the complexity class $\#P$ a family $\{X_{\#P}(n,m)\}$ of (group-theoretic)
class varieties, and with the complexity class $NC$ a family of 
$\{X_{NC}(n,m)\}$ of (group-theoretic) class varieties such that: 
if $\perm(X)$, $\dim(X)=n$, can be represented linearly 
as $\det(Y)$, $\dim(Y)=m>n$, then 

\begin{equation} \label{eqembed} 
X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation} 

Each  class variety is a  (projective) algebraic variety, by which
we mean the zero set of  a system of multivariate 
homogeneous polynomials with coefficients in $\C$  (akin to the 
usual curves  and surfaces). It is  group-theoretic in the 
sense that it is  constructed using group-theoretic operations 
and the general linear group $G=GL_l(\C)$, $l=m^2$, of $l\times l$ invertible
complex matrices acts on it. Here action means moving the points 
of the class variety around, just as $G$ moves the points of $\C^l$ around 
by the standard action via invertible linear transformations.
The goal is to show that the inclusion (\ref{eqembed}) is impossible;
cf. Figure~\ref{fig:class}. 

\begin{figure} 
\begin{center} \psfragscanon
\psfrag{xsharp}{$X_{\#P}(n,m)$}
      \psfrag{xnc}{$X_{NC}(n,m)$}
      \psfrag{g}{$G=GL_l(\C)$, $l=m^2$}
      \psfrag{Obstruction}{\mbox{Obstruction}}
\epsfig{file=class.eps, scale=.5}
\end{center}
      \caption{Class varieties}
      \label{fig:class}
\end{figure} 



Since each class variety has a $G$-action, the space of polynomial functions 
on each class variety has a  representation-theoretic structure, which 
puts constraints on which  representations of $G$ can live on that variety
(i.e., in the space of polynomial  functions on that variety).
Informally, an obstruction is an irreducible (minimal)  representation of $G$
that can live on $X_{\#P}(n,m)$ but not on $X_{NC}(n,m)$; 
cf. Figure~\ref{fig:class}.
Existence of  an obstruction $O_n$, for every $n$, assuming
$m=2^{\log^a n}$, $a>1$ fixed, implies  that the inclusion (\ref{eqembed}) 
is not possible, since  $O_n$ cannot live  on $X_{NC}(n,m)$.
Thus  an obstruction blocks the inclusion (\ref{eqembed}).


To define an obstruction formally, we need to recall some basic representation
theory.  By a classical result of Weyl, the irreducible 
(polynomial) representations of $G=GL_l(\C)$ are in one-to-one correspondence 
with the partitions  $\lambda$ of length at most $l$, by which we mean 
integral sequences $\lambda_1 \ge 
\lambda_2 \cdots \ge \lambda_k > 0$, $k\le l$, where  $k$ is called the  length
of $\lambda$. The irreducible 
representation of $G$ in correspondence with $\lambda$ is denoted 
by $V_\lambda(G)$, and is called the {\em Weyl module} of $G$ indexed by 
$\lambda$. Symbolically:

\[\mbox{Irreducible representations of } G \stackrel{\mbox{Weyl}}{\Longleftrightarrow} \quad \mbox{partitions} \ \lambda. \]  

\[\mbox{Weyl module  } V_\lambda(G)  \longleftrightarrow \lambda. \] 
Weyl also proved that every finite dimensional representation of $G$ 
can be decomposed into irreducible representations--i.e.,
can be written as a direct sum of Weyl modules. Thus Weyl modules 
are the basic building blocks of the representation theory of 
$G$, and every finite dimensional representation of $G$ can be thought
of as a complex building made out of these blocks. 


Now suppose $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$. 
Suppose to the contrary that 

\begin{equation} \label{eqembed2}   X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation}

Let $R_{\#P}(n,m)$ denote the homogeneous coordinate ring of 
$X_{\#P}(n,m)$; i.e., the ring of polynomial functions on $X_{\#P}(n.m)$
(though the  functions here are not functions in usual sense;
but let us  not worry about this). 
Let $R_{\#P}(n,m)_d$ be the degree-$d$-component of $R_{\#P}(n, m)$ consisting
of functions of degree $d$. We define $R_{NC}(n,m)$ and $R_{NC}(n,m)_d$
similarly. Since $X_{\#P}(n,m)$ has the action of $G$, $R_{\#P}(n,m)$ 
also has an action of $G$; i.e., it is a representation of $G$. Hence,
$R_{\#P}(n,m)_d$ is a finite dimensional representation of $G$. 
Similarly, $R_{NC}(n,m)$ is a representation of $G$, and $R_{NC}(n,m)_d$
a finite dimensional representation of $G$. 



If (\ref{eqembed2}) holds, then we get a natural map from $R_{NC}(n,m)$ to
$R_{\#P}(n,m)$ obtained by restricting a function on $X_{NC}(n,m)$ to
$X_{\#P}(n,m)$. %; cf. Figure~\ref{fig:restriction}.
By basic algebraic geometry, this map
is surjective and is a $G$-homomorphism.
Furthermore, it is degree-preserving. This means there
is a surjective $G$-homomorphism from $R_{NC}(n,m)_d$ to 
$R_{\#P}(n,m)_d$. Symbolically: 

\begin{equation} \label{eqsurjection}
R_{\#}(n,m)_d \leftarrow  R_{NC}(n,m)_d.
\end{equation}

\ignore{
\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{Xp}{\small $X_{\#P}(n,m)$}
\psfrag{Xnc}{\small $X_{NC}(n,m)$}
\epsfig{file=restriction.eps, scale=.6}
\end{center}
      \caption{Restriction}
      \label{fig:restriction}
\end{figure}
}

Let $R_{\#P}(n,m)_d^*$ denote the dual of $R_{\#P}(n,m)_d$; i.e., the 
set of linear maps from $R_{\#P}(n,m)_d$ to $\C$. Then (\ref{eqsurjection})
implies that there is an injective $G$-homomorphism from 
$R_{\#P}(n,m)^*_d$ to $R_{NC}(n,m)^*_d$. Symbolically: 

\begin{equation} \label{eqinclusion}
R_{\#}(n,m)_d^*  \hookrightarrow {NC}(n,m)_d^*.
\end{equation}

\begin{defn} (GCT2)
An obstruction $O_n$ is a Weyl module $V_\lambda(G)$ that 
occurs as a subrepresentation 
in $R_{\#P}(n,m)_d^*$  but not in $R_{NC}(n,m)_d^*$, for some $d$. 
We call $\lambda$ an {\em obstruction label}, and sometimes,
by abuse of notation, an obstruction as well.
\end{defn}

\begin{prop} (GCT2)
Existence of an obstruction $O_n$, for all $n\rightarrow \infty$, 
with $m=2^{\log^a n}$, $a>1$ fixed, implies $\perm(X)$, $\dim(X)=n$, 
cannot be represented linearly as 
$\det(Y)$, $\dim(Y)=m$. 
\end{prop}

This follows just from the definition of an obstruction, and 
leads to:

\begin{goal} \label{gobs} (GCT2)
Prove existence of an obstruction family $\{O_n\}$ using 
the {\em exceptional} nature of $\perm(X)$ and $\det(Y)$. 
\end{goal} 

Exceptional here means completely characterized by the symmetries 
in the following sense. 
Let  $Y$ be a variable $m\times m$ matrix.
Let $\sym^m(Y)$ be the space of homogeneous forms of degree $m$ 
in the $m^2$ variable entries of $Y$. Then, by the  classical
representation theory,  $\det(Y)$ is the only form in $\sym^m(Y)$ 
such that, for any $A,B \in GL_m(\C)$ with $\det(A)\det(B)=1$, 
\[ \det(Y)=\det(A Y^* B), \] 
where $Y^*=Y$ or $Y^t$. 
Thus $\det(Y)$ is completely characterized 
by its symmetries, and hence, is  exceptional.

Similarly, $\perm(X)$ is the only form 
in the space of forms of degree $n$ in the entries of $X$ such that, 
for any diagonal or permutation matrices $A,B$, 
\[ \perm(X)=\perm(AX^*B), \]
where $X^*=X$ or $X^t$ and the product of the diagonal entries of $A$ and $B$
is one. 
Thus $\perm(X)$ is also
completely characterized   by its symmetries, and hence, is
exceptional.

\section{Towards existence via positivity}
We now proceed to describe the main results of GCT in the context of
Goal~\ref{gobs}. 
Towards that end, we  associate with the class varieties 
certain representation-theoretic {\em stretching} functions. 
Let $F_{\lambda,n,m}(k)$ denote the number of occurances (multiplicity)  of
the Weyl module $V_{k\lambda}(G)$ in $R_{\#P}(n,m)^*$ (i.e. 
$R_{\#P}(n,m)^*_d$, for some $d$)  as a subrepresentation,
and $G_{\lambda,n,m}(k)$ the number of occurances of 
$V_{k\lambda}(G)$ in $R_{NC}(n,m)^*$. These are statistical functions
associated with the class varieties, where the statistics associates 
with every number (stretching parameter) $k$  
the multiplicity of the corresponding
Weyl module $V_{k\lambda}(G)$; cf. Figure~\ref{fig:statistics}.

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{l}{$\lambda$}
\psfrag{2l}{$2 \lambda$}
\psfrag{3l}{$3 \lambda$}
\psfrag{v1}{$V_\lambda(G)$}
\psfrag{v2}{$V_{2 \lambda}(G)$}
\psfrag{v3}{$V_{3\lambda}(G)$}
\epsfig{file=statistics.eps, scale=1}
\end{center}
      \caption{statistics}
      \label{fig:statistics}
\end{figure}


Let us  call a function $f(k)$ {\em quasipolynomial}, if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k)$ for all nonnegative integral $k=i$ modulo $l$;
here  $l$ is
called the period of the  quasi-polynomial. 
Thus  quasi-polynomials
are hybrids of  polynomial and periodic functions. 
We say that $f(k)$ is an 
{\em asymptotic quasipolynomial} if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k)$ for all nonnegative integral $k=i$ modulo $l$ for 
$k\ge a(f)$, for 
some nonnegative integer depending on $f$. The minimum 
$a(f)$ for which this holds is called the {\em deviation from 
quasipolynomiality}. Thus $f(k)$ is a (strict) quasipolynomial when this
deviation is zero.

A fundamental example of a quasi-polynomial is the Ehrhart quasi-polynomial
$f_P(k)$ of a polytope $P$ with rational vertices. It is defined
to be the number of integer points in the dilated polytope $kP$. By the 
classical result of Ehrhart, it is known to be a quasi-polynomial.
More generally, let $P(k)$ be a polytope parametrized by nonnegative
integral $k$: i.e., 
defined by a linear system of the form: 
\begin{equation} \label{eqpara}
A x \le k b + c,
\end{equation}
where $A$ is an $m \times n$ matrix, $x$ a variable $n$-vector, and 
$b$ and $c$ some constant $m$-vectors. Let $f_P(k)$ be the number 
of integer points in $P(k)$. We shall call it the Ehrhart function of
$P(k)$.  It is known to be  an asymptotic quasi-polynomial.
In what follows, we  denote a parametrized polytope $P(k)$ by 
just $P$. 




\begin{theorem} (GCT6) \label{tquasi}
The functions $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ 
are asymptotic quasi-polynomials. Furthermore, they 
are (strict) 
quasi-polynomials assuming that the singularities of the class varieties
$X_{\#P}(n,m)$ and $X_{NC}(n,m)$ are rational and normal. 

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem} 

Here a rational and normal  singularity means a singularity that is nice in
an algebro-geometric sense that we shall not elaborate here.
At present, we do not know if the singularities of the class varieties 
are indeed  rational and normal. A conservative conjecture would be  that 
they are not too bad, even if they are not strictly rational and normal,
because of the exceptional nature of the 
determinant and the permanent; 
i.e.,  the deviation from quasipolynomiality
of $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ is 
small in a sense to be made precise 
later (cf. the remarks after Hypothesis~\ref{hph1}).

The proof of Theorem~\ref{tquasi}
follows from a detailed study of the behaviour
of the singularities of class varieties under the action of the 
group $G$. This is based on
\begin{enumerate} 
\item The 
resolutions of singularities in characteristic zero
\cite{hironaka}: 
this  roughly says 
that the singularities of any algebraic variety in characteristic zero
can be untangled (resolved) nicely in a systematic fashion; cf.
 Figure~\ref{fig:resolution}.
\item Cohomological works of Boutot, Brion,  Flenner, Kempf  and others
bases on this resolution; cf.  \cite{boutot,dehy} and
GCT6 for the history and other references.
\end{enumerate} 


\begin{figure} 
\begin{center} 
\epsfig{file=resolution.eps, scale=.5}
      \caption{Resolution}
      \label{fig:resolution}
\end{center}
\end{figure}


As such, this proof is highly nonconstructive. It gives no effective
bound on the period $l$--it just says that $l$  is finite.





The following hypothesis 
says that $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ 
can be realized as the Ehrhart functions  of parametrized  polytopes.

\begin{hypo} {\bf (PH) [Positivity Hypothesis]} \label{hph} (GCT6)

\noindent (a) For every $\lambda,n,m\ge n$, 
there exists   a parametrized  polytope $P=P_{\lambda,n,m}$ 
such that 
\begin{equation} \label{eqP}
F_{\lambda,n,m}(k)=f_P(k).
\end{equation} 
It is also assumed here that there exists for $P_{\lambda,n,m}$ a specification
of the form (\ref{eqpara}),
 where $A$ is independent of $\lambda$, and $b$ and $c$ 
are  piecewise homogeneous linear functions of $\lambda$.


\noindent (b) There exists a similar parametrized 
 polytope  $Q=Q_{\lambda,n,m}$  such that
\begin{equation} \label{eqQ}
G_{\lambda,n,m}(k)=f_Q(k).
\end{equation}


Analogous positivity hypothesis also holds 
for the $P$ vs. $NP$ problem in characteristic zero.
\end{hypo} 


If such $P$ and $Q$ exist, their dimensions are guaranteed to be
small by the proof of Theorem~\ref{tquasi}: specifically,
the dimension $P$ is guaranteed to be bounded by a 
polynomial in $n$, and the dimension of $Q$ 
by a polynomial in $m$.
There is a variant of PH (b), which is good enough for our purposes (cf.
Lecture 3, Hypothesis~\ref{hphvariant}),
wherein  the dimension of $Q$ is also guaranteed
to be bounded by a polynomial in $n$ (but independent 
of $m$), if the length of $\lambda$ is $\poly(n)$ (as it would be in 
our applications).






When PH holds, we say that $F_{\lambda,n,m}(k)$ and 
$G_{\lambda,n,m}(k)$ have  {\em positive convex representations}. 
Here positivity refers to the fact that the Ehhart function 
$f_P(k)$ is a positive expression:
\[ f_P(k)=\sum_{v} 1,\] 
where $v$ ranges over all integer points in $P(k)$--there are no 
alternating signs in this expression.
Convexity refers to the  convexity of the polytopes $P(k)$ and $Q(k)$. 


But, a  priori, it is not at all clear why PH should  even hold. 
Because many numerical functions in algebraic geometry are 
asymptotic quasi-polynomials (e.g., the Hilbert function 
\footnote {Hilbert function $h_Z(k)$ of a projective algebraic variety $Z$
is defined to be $\dim(R(Z)_k)$, where $R(Z)$ is the homogeneous coordinate 
ring of $Z$ and $R(Z)_k$ its degree $k$-component.} of any projective
variety), but they rarely have positive convex representations.
PH is expected to hold for $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ 
because of the exceptional nature of the determinant and the permanent. 
For a mathematical evidence and justification
in support of PH, see  GCT6,7, and 8.







\begin{theorem} (GCT6) \label{tgct6}
There exists a family $\{O_n\}$ of obstructions 
for the  $\#P$ vs. $NC$ problem in characteristic zero, 
for $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$, 
assuming, 

\begin{enumerate} 
\item PH, and
\item OH (Obstruction Hypothesis): 

For all $n\rightarrow \infty$,  there exists $\lambda$ such that 
$P_{\lambda,n,m}(\infty)=\mbox{lim}_{k\rightarrow \infty} P(k) 
\not = \emptyset$ and $Q_{\lambda,n,m}(k)=\emptyset$ for all (large enough)
$k$.
\end{enumerate}

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem}

Mathematical evidence and arguments in support of OH are given in GCT6.

We call  $\lambda$ a {\em relaxed obstruction}
(or rather, relaxed obstruction-label)
if it satisfies OH. In this case, $k\lambda$, for some integer $k\ge 1$ is
an obstruction--we just have to choose $k$ large enough 
so that 
$P_{\lambda,n,m}(k)$ contains an integer point
but $Q_{\lambda,n,m}(k)$ does not.
Henceforth, whenever we say obstruction, we actually mean relaxed 
obstruction.

There is a fundamental difference between the nature of PH and OH.
PH is a {\em mathematical hypothesis}, because there is no 
constraint on what $m$ should be in comparison to $n$ in its statement.
In contrast, OH is a {\em complexity theoretic hypothesis}, because 
$m$ needs to be small in comparison to $n$ for it to hold.


%\subsection{Why should PH  and OH hold?} 

%Mathematical evidence for this is given in GCT2,4,6,7,8.
%We shall discuss some of this  in the third lecture.


\section{The flip: Explicit construction of obstructions} 
\label{sflip}
In principle PH may have a nonconstructive proof (like that
of Theorem~\ref{tquasi})  which only tells  that such polytopes 
exist without explicitly constructing them. But proving OH may not be feasible
unless the polytopes $P$ and $Q$ in PH are given explicitly.
This  suggests the following strategy for proving 
existence of obstructions proposed in  GCT6 and  GCTflip.


\noindent (1) Prove the following stronger explicit form 
of PH, which is reasonable since the polytopes $P$ and $Q$, if they exist,
are already guaranteed to be of small (polynomial) dimension:

\begin{hypo} {\bf (PH1)}  \label{hph1} (GCT6)

\noindent (a) There exist an {\em explicit} 
polytope $P_{\lambda,n,m}$ 
as in  PH (a).
Explicit means: 

\begin{enumerate}
\item  The polytope is specified by an explicit system of linear constraints,
where the bitlength of (the description of) 
each constraint is  $\poly(n,\bitlength{\lambda}, \bitlength{m})$.
Here and in what follows, $\bitlength{z}$ denotes the bitlength of the 
description of $z$.

\item  The membership problem for the polytope
$P_{\lambda,n,m}(k)$  also 
belongs to the complexity class $P$.
That is,  given a point $x$, whether it belongs to $P_{\lambda,n,m}(k)$ 
can also be decided in $\poly(\bitlength{x},\bitlength{\lambda},
n,\bitlength{m})$
time.
Furthermore, we assume that if $x$ does not belong to the polytope,
then the membership algorithm also gives a hyperplane separating 
$x$ from the polytope in the spirit of \cite{lovasz}. 
\end{enumerate} 

\noindent (b) There exists a similar  explicit 
polytope $Q_{\lambda,n,m}$  satisfying   PH (b). 
\end{hypo}

Note the occurance of  $\bitlength{m}$  instead of $m$ in the polynomial
bounds in (a); 
the reasons for this would be explained in Lecture 3 
(cf. remarks after Hypothesis~\ref{hph1restatement}). 
In contrast, the polynomial bounds for the polytope in (b)  depend on 
$m$, not $\bitlength{m}$. 
But there are  variants of PH (b) and PH1 (b), 
(cf. Hypotheses~\ref{hphvariant} and \ref{hph1tilde} in  Lecture 3), 
which are enough for our purposes, 
wherein the polynomial bounds depend on the bitlength of $\lambda$,
but not on $m$.
In what follows, we assume that PH (b) and PH1 (b) have been replaced 
with these variants.

 


In particular, PH1 implies that the functions $F_{\lambda,n,m}(k)$ and
$G_{\lambda,n,m}(k)$ belong to the complexity class $\#P$. 
It also implies that the deviation from quasipolynomiality 
of $F_{\lambda,n,m}(k)$ is small, specifically, 
$2^{O(\poly(\bitlength{\lambda},n,\bitlength{m}))}$--thus the bitlength
of the deviation is polynomial. In other words, this says
that the deviation from rationality and normality of the singularities
of the class variety $X_{\#P}(n,m)$ is small (cf. Theorem~\ref{tquasi}).
Similarly for $Q_{\lambda,n,m}(k)$ and $X_{NC}(n,m)$. 

Like PH, PH1 is also a mathematical hypothesis in the sense that
it puts  no constraint on what $m$ should be in comparison to $n$. 
Of course, unlike PH, there is some complexity theoretic aspect to it, 
but it is secondary in comparison to the complexity-theoretic aspect of 
of OH, since smallness  of $m$ with respect to  $n$ is the 
crux of the lower bound  problems under consideration. 





\noindent (2a) {\bf [The flip]}

Let $m=2^{\log ^a n}$, for a fixed $a>1$. 
Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
show existence of  an {\em explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of (relaxed) obstructions  satisfying OH. 
We say that an obstruction (proof-certificate) 
$\lambda_n$ is {\em explicit} if is ``short'' and ``easy to verify'':


\begin{enumerate} 
\item  Short: This means its bitlength $\bitlength{\lambda_n}$ 
is $\poly(n)$,
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  

\item Easy to verify: given $n, m \le 2^{\log^a n}$ and 
$\lambda_n$, whether 
$\lambda_n$ is a valid obstruction 
can be verified 
in $\poly(n,\bitlength{\lambda})$ time. In particular, this is
$\poly(n)$ when $\bitlength{\lambda}=\poly(n)$. 
\end{enumerate}

Existence of an explicit family of obstructions is equivalent to saying
that the problem of deciding existence of obstructions belongs to $NP$.
This definition of explicitness is quite natural since the class $NP$ 
is a class of problems whose proof-certificates (witnesses) are 
short and easy to verify. As such, the flip--going for 
explicit  obstructions--is
a proof-strategy that is literally given to us on a platter 
by the $P$ vs. $NP$ 
problem itself. Why it is called flip would be explained later.


It should be stressed that we are primarily interested in only proving 
existence of obstructions. Whether they are explicit or not 
does not really matter in the original statement of the problem.
But we need to know the polytopes $P$ and
$Q$ explicitly (as in PH1)  so that proving OH is feasible. 
%In other words,   if we do not
%even know what the polytopes $P$ and $Q$ look like, 
%it seems unlikely that anything  could be said regarding OH. 
But once  PH1 is proved, existence of an explicit family follows
automatically,   as a bonus, whether we care for it or not. 

To see why, let us observe that 
the second condition above  (ease of verification) follows directly
from PH1 and the polynomial time algorithm for 
linear programming on  polytopes given by separation oracles \cite{lovasz}. 
Shortness  also follows from PH1. 

Thus it is as if the $P$ vs. $NP$ problem is forcing us to go
for explicit obstructions.


\noindent (2b) {\bf [The strong flip (optional)]} 

Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
construct (rather than just show existence of) 
a {\em strongly explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of obstructions  satisfying OH. We say that an explicit family 
of obstructions is strongly explicit if,
for each $n$, a valid obstruction-label
$\lambda_n$ can be constructed in $\poly(n)$ time.
In particular, the height and the bitlength of
 $\lambda$ is $\poly(n)$ (short) 
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  


For the purposes of the lower bound problems that we are interested in, the
flip (just explicit  
existence) would suffice and the stronger flip (explicit construction)
is optional. But the stronger flip can give us deeper insight into these
lower bound problems; cf. GCTflip for more on this.

Now we turn to a few obvious questions.



\section{What has been achieved by all this?: The meaning of the flip} 
\label{smeaning}
Let us now see what has been achieved so far
in the context of the 
$\#P\not = NC$ conjecture in the nonuniform setting (characteristic zero),
the argument for the $P$ vs. $NP$ problem in characteristic zero
being  similar. The goal of this conjecture is to prove that 
$\perm(X)$ cannot be computed by an arithmetic circuit $C$
of size $m=\poly(n)$, or more generally,
$m \le 2^{\log^a n}$, for some fixed $a>1$, and depth $O(\log^a n)$.
Or in symbols:

\begin{equation} \label{eqioh} 
 {\bf (IOH):}  \forall n  \forall C \exists X:
\perm(X)\not = f_C(X),
\end{equation} 

where $f_C(X)$ denotes the function computed by $C$, and $n$ is supposed
to be sufficiently large.
For given $X$ and $C$ of $\poly(n)$ size, the problem 
of deciding if  $\perm(X) = f_C(X)$ belongs to $\#P$ (or rather, $P^{\#P}$). 
Since there are two alternating layers of quantifiers in (\ref{eqioh}),
the problem of verifying it belongs to $\Pi^2 \#P$, 
which is very high in the complexity hierarchy
(cf. Figure~\ref{fig:IOHcomplexity}).
Hence, we  refer to the original hypothesis (\ref{eqioh}) 
to be proven  as IOH 
(Infeasible Obstruction Hypothesis). Of course, IOH is expected to 
be a tautology, and hence is expected to  be verifiable in $O(1)$ time--but
we do not know that as yet. 



\begin{sidewaysfigure} 
\begin{center}
\psfragscanon
\psfrag{sigma2p}{{\small $\Pi^2 \#P$}}
\psfrag{sigma1p}{$\Sigma^1 \#P$}
\psfrag{P}{{\small $P$}}
\psfrag{NP}{{\small $NP$}}
\psfrag{T}{$T$}
\psfrag{#P}{$\# P$}
\psfrag{inNP}{$\in NP$}
\psfrag{inP}{$\in P$}
\psfrag{insigma2p}{$\in \Pi^2 \#P$}
\psfrag{PHplus}{PH1}
\psfrag{PHtil}{$PH^\dagger$}
\epsfig{file=IOHcomplexity.eps, scale=.8}
\end{center}
      \caption{Positivity as a means to eliminate the quantifiers and 
reduce the complexity of the  obstruction hypothesis}
      \label{fig:IOHcomplexity}
\end{sidewaysfigure}



Equivalently, the goal is to prove existence of a {\em trivial obstruction},
which is a table that lists for each $C$ as above a counterexample  $X$ so that
$\perm(X)\not = f_C(X)$; cf. Figure~\ref{fig:trivial}.
The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$ and depth
$O(\log^a n)$. Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. 
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time to decide if such a table exists and construct 
one (optional) for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. So
we call  this trivial, brute force 
strategy of proving IOH, based on existence of trivial obstructions,
 an {\em infeasible strategy}. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{eq}{$\perm(X)\not = f_C(X)$}
\epsfig{file=trivial.eps, scale=.5}
\end{center}
      \caption{A trivial obstruction}
      \label{fig:trivial}
\end{figure}


In contrast, assuming PH1, the problem  of verifying OH belongs 
to $NP$ as we have already observed. Thus, assuming PH1, we have 
transformed the original infeasible obstruction 
hypothesis $IOH \in \Pi^2 \#P$ to a new  obstruction hypothesis 
$OH \in NP$, in the process bringing down the time to verify an obstruction
from the exponential (for the original trivial obstruction) to polynomial
(for the new obstruction); cf. Figure~\ref{fig:IOHcomplexity}.  
It is crucial here that PH1, the main tool for this reduction, is a 
mathematical hypothesis,  not complexity-theoretic (cf. the remarks
after Theorem~\ref{tgct6} and Hypothesis~\ref{hph1}).
The task of verifying  an obstruction has also been 
transformed from the infeasible (exponential-time) to the feasible 
(polynomial-time). Hence the name of this strategy: the flip,
from the infeasible to the feasible.
Positivity (PH1) is used in the flip as a means  to
eliminate the quantifying variables in IOH and bring down the 
 complexity of the obstruction hypothesis;
cf. Figure~\ref{fig:IOHcomplexity}. 




This process can be extended further. Assuming an additional
positivity hypothesis PH4 specified below,
$OH \in NP$ can be transformed 
to POH (Positivity Obstruction Hypothesis) that belongs to $P$; i.e.,
which can be verified in polynomial time, and an obstruction,
if it exists, can also be constructed in polynomial time; 
cf. Figure~\ref{fig:IOHcomplexity}. (The hypothesis is called PH4 instead
of PH2, because PH2 and PH3 are some other positivity hypotheses in GCT6
that complement PH1). 
Once this final positivity hypothesis POH is proven, the obstruction
hypothesis is reduced to a tautology (FOH: Final Obstruction Hypothesis),
which can be verified in
$O(1)$ time. This  would then give us 
the final $O(1)$-size  proof. 

Thus the basic idea of the flip is to use positivity systematically
as a means to eliminate the quantifiers  and reduce the complexity 
of the  obstruction hypothesis until it is finally
reduced to  an $O(1)$-time verifiable  tautology;
cf. Figure~\ref{fig:IOHcomplexity}. 

Now let us specify PH4 and POH.
Towards that end, let  $k \le l=m^2$ be the length of $\lambda$.
Define 

\begin{equation} 
\begin{array}{l}
\bar P_{n,m}= \{ \lambda: P_{\lambda,n,m} \not = \emptyset \} \subseteq \C^k, \\
\bar Q_{n,m}= \{ \lambda: Q_{\lambda,n,m} \not = \emptyset \} \subseteq \C^k.
\end{array}
\end{equation}

Then: 

\begin{hypo}  {\bf PH4} (GCT6)

The sets $\bar P_{n,m}$ and $\bar Q_{n,m}$ are convex polytopes in $\C^k$.
Furthermore, the membership problems for these polytopes belong to 
$P$ and so also the problem of deciding if $\mbox{vol}(\bar P_{n,m}
\setminus \bar Q_{n,m})$, the volume of the relative complement 
$\bar P_{n,m} \setminus \bar Q_{n,m}$, is nonzero (positive);
i.e. if $\bar P_{n,m} \not \subseteq \bar Q_{n,m}$. By polynomial time,
we mean $\poly(n,l,\bitlength{m})$ time. This is $\poly(n)$,
if $m\le 2^{o(n)}$ and $l =\poly(n)$. 
\end{hypo}

\begin{hypo} {\bf (POH)}

For all $n\rightarrow \infty$, assuming $m=2^{\log^a n}$, $a>1$ fixed, 

\[ \mbox{vol}(\bar P_{n,m} \setminus \bar Q_{n,m}) > 0, \] 

for $k=(n+1)^2$. 
\end{hypo} 

\ignore{
Thus POH says that  the line-shaded area in Figure~\ref{fig:POH} has positive
volume for all large enough $n$. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{P}{$\bar P_{n,m}$}
\psfrag{Q}{$\bar Q_{n,m}$}
\epsfig{file=POH.eps, scale=1}
\end{center}
      \caption{POH}
      \label{fig:POH}
\end{figure}
}

\section{How to prove PH?}  \label{sphprove}
There is  a basic prototype of PH in representation theory,
which will be described in detail towards the end of Lecture 3. We shall
refer to it  as Plethysm PH. It says that the stretching functions 
akin to $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$
associated with  fundamental  multiplicities 
in representation theory called plethysm constants also have analogous 
positive convex representations. 

This  is   known for a very special case of the plethysm constant 
called the  Littlewood-Richardson (LR) coefficient
$c_{\alpha,\beta}^\lambda$. It is  defined to be 
the number of occurances of the Weyl module $V_{\lambda}(G)$ in the 
tensor product of $V_{\alpha}(G)$ and $V_\beta(G)$. 
The classical Littlewood-Richardson rule, which we shall refer to as LR PH,
implies that the stretching function 
$\tilde c_{\alpha,\beta}^\lambda (k) = c_{k \alpha, k \beta}^{k \lambda}$
associated with the Littlewood-Richardson coefficient has a
positive convex representation.

Plethysm PH   happens to be a fundamental open problem of
representation theory, older than the $P$ vs. $NP$ problem itself. It 
has been studied intensively in the last century, and is known to be
formidable. And  now,  as explained the third lecture, it also turns out to 
be  the heart of this approach towards the $P$ vs $NP$, the
$\#P$ vs. $NC$ problems.



A basic plan to prove Plethysm PH is given in GCT6.
It is partially 
implemented in GCT7 and 8. See Figure~\ref{fig:lift} for a pictorial
depiction of the plan. It strives  to extend the  proof of LR PH based 
on the theory of the  standard quantum group \cite{drinfeld,kashiwara,lusztig}.
There it
comes out as a consequence of a  (proof of a) deep positivity result
\cite{kazhdan,lusztig}, which
we shall refer to as LR PH0. It says that   the 
tensor product of two representations of the standard quantum group 
has a canonical basis \cite{kashiwara,lusztig} 
whose structure coefficients are all positive \cite{lusztig}
polynomials (i.e., polynomials with nonnegative coefficients).
The only known proof of this
result is based on the Riemann Hypothesis over finite fields 
proved in \cite{weil2},  and the related works \cite{beilinson}. 
This Riemann Hypothesis is  itself a deep positivity statement in mathematics,
from which   LR PH can  thus be 
deduced, as shown on the bottom row of Figure~\ref{fig:lift}.

If one were only interested in LR PH, one  does not 
need this  powerful machinery, because it has a  much simpler 
algebraic-combinatorial  proof. 
But the plan to extend the
proof of LR PH to Plethysm PH in GCT6,7,8 is like a huge
inductive spiral. To  make it work,  one  needs a 
stronger inductive hypothesis than Plethysm PH--this is precisely  Plethysm 
PH0 (which  will be
described in the third lecture; cf. Hypothesis~\ref{hplph0}).
Thus what is needed now 
is a systematic lifting  of the bottom arrow in Figure~\ref{fig:lift}
to the top, so as to complete the  commutative diagram, so to speak. 

Initial  steps in this direction have been taken in GCT7,8. 
First, GCT7 constructs a {\em nonstandard quantum group}, which
generalizes the notion of a standard quantum group \cite{drinfeld},
 and plays the
same role in the plethysm setting that the standard quantum group plays
in the LR setting. Second, GCT8 gives an algorithm to construct 
a canonical basis for a representation of the nonstandard quantum group
that is conjecturally correct and has the property Plethysm PH0,
which is a   generalization of LR PH0  supported by experimental
evidence.
Now what is needed to complete  the 
commutative digram in Figure~\ref{fig:lift} is an appropriate nonstandard 
extension of the Riemann hypothesis over finite fields and the related works
\cite{beilinson,weil2,kazhdan,lusztig}
from which  Plethysm PH0 can be deduced. This--the top-right corner 
of the diagram--is the   main  open problem at the heart of this approach. 

\section{How to prove OH or POH?} 
We do not  know, 
since the  proof of OH and POH 
would really depend on the explicit forms of the
polytopes that arise in   PH1/PH4, and we have no idea about them
at this point.
But GCT does suggest  that proving OH/POH  should be feasible 
``in theory''
since OH/POH  belong to NP/P, assuming PH1/4, and polynomial-time
is complexity theory stands for feasible ``in theory''. In other words,
GCT suggests that proving the $P\not =  NP$ conjecture 
should now be  feasible ``in theory''. Even this  was  always  doubted in
the field of complexity theory so far 
in view of the universal nature of the $P$ vs. $NP$ problem. So, at least,
there is a reason to believe now that the $P\not = NP$ conjecture is provable.
But, as we also know by now, 
there is a huge gap between the theory and the practice--e.g., 
just because  some problem is in $P$ does not 
necessarily mean that it is feasible in practice. Similarly,
the actual implementation of the GCT flip via positivity is expected to be 
immensely difficult ``in practice'', as Figure~\ref{fig:lift} suggests. 







\section{Is positivity  necessary?} 
But if the positivity problems are so hard,  one may  finally ask: can 
they not be avoided somehow? Unfortunately, there is a formidable 
barrier towards the $P$ vs. $NP$ and related problems, called the
{\em feasibility ($P$) barrier} (GCT6,GCTflip),
which seems universal in the sense that
any approach towards these problems would have to tackle it, not just GCT. 
The existing mathematical evidence suggests that any natural approach
to cross this barrier would have to say  something deep regarding positivity
(Plethysm PH/PH0)  either explicitly or {\em implicitly}, even if
the approach does not utter a word about algebraic geometry or
representation theory.
That is,  Plethysm PH and PH0   may indeed be 
the heart of the  fundamental lower bound problems in complexity theory;
a detailed story and a precise meaning of the key 
phrase {\em implicit} would appear in the revised version of GCTflip.

%\input{feasibility}









































 

































\begin{sidewaysfigure} 
\begin{center} 
\epsfig{file=lift.eps, scale=.8}
\end{center}
      \caption{A commutative diagram}
      \label{fig:lift}
\end{sidewaysfigure} 



\ignore{\begin{figure} 
\psfragscanon
\psfrag{P}{$P\not = NP$ and $\#P\not = NC$ conjectures (characteristic zero)}
\epsfig{file=barriers.eps, scale=1}
      \caption{The feasibility barrier towards $P$ vs. $NP$}
      \label{fig:barriers}
\end{figure}}



==> lecture1_6.tex <==
\section*{Introduction}

This article   gives a mathematical  overview of
geometric complexity theory (GCT), an
approach  towards the fundamental lower bound problems  in complexity theory, 
such as (Figure~\ref{fig:complexityclasses}):

\noindent (1) 
The $P$ vs. $NP$ problem \cite{cook,karp,levin}: 
 show that $P \not = NP$;


\noindent (2) 
The  $\#P$ vs. $NC$ problem \cite{valiant}: show that 
$\#P \not = NC$.

\noindent (3) The $P$ vs. $NC$ problem: show that $P \not = NC$.


The complementary article \cite{gctexplicit} gives a complexity-theoretic
overview. It describes   the main complexity theoretic
barrier towards these problems 
called the {\em feasibility barrier} and the basic 
strategy of GCT for crossing it called the flip: which is to go 
for {\em explicit proofs}. By an explicit proof 
we mean a proof that provides proof certificates of hardness  for the 
hard function under consideration that are short (of polynomial size) 
and easy to verify (in polynomial time). This barrier turns out to be
extremely formidable and is the root cause of all difficulties 
in these problems. Nonnelementary techniques are brought into GCT precisely
to cross this barrier. This barrier is not discussed in these lectures. 
The goal here is to describe the basic ideas of GCT at a concrete mathematical
level without getting into such meta issues. The readers who wish
to know the root cause of all difficulties encountered in GCT and
the need for the nonelementary techniques in GCT before getting
into any mathematics   may wish to read that
article before this one. On the other hand, the readers who would rather avoid 
meta issues before getting a concrete mathematical
picture  may wish to read this article first. We will leave the
exact choice to the readers.




We  focus here on only the nonuniform versions of these problems 
in characteristic zero; i.e., when
the underlying field of computation is of characteristic zero, 
say $\Q$ or $\C$.  The additional problems that
need to be addressed when the underlying field of computation is finite
would be discussed in  GCT11. 


The nonuniform
characteristic zero version of the $P\not = NC$ conjecture (in fact,
something stronger) was already proved  in GCTlocal. We shall refer
to it as the $P\not = NC$ result without bit operations.
It says that the max flow problem cannot be solved in the 
PRAM model without bit operations in $\polylog(N)$ time using 
$\poly(N)$ processors where $N$ is the bitlength of the input.
This  may be considered to be the first unconditional lower bound result of
GCT, because, though it can be stated in purely elementary combinatorial
terms, being a formal implication of the $P\not = NC$ conjecture, its
proof is intrinsically geometric, and no elementary proof is known so far. 
Furthermore, its proof  technique may be considered to be a weaker (local)
form of the {\em flip}, the basic guiding strategy of GCT, which  was 
refined and formalized much later in GCTflip. 
This  was the begining of  this  geometric approach in complexity theory.
The later work in GCT-- the subject of this overview--focusses on the other 
two problems above, namely
the $P$ vs. $NP$ and $\#P$ vs. $NC$ problems. 


The nonuniform (characteristic zero) version of the $\#P$ vs. $NC$ problem
is also known as the permanent vs. determinant problem \cite{valiant}. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented %(cf. Figure~\ref{fig:matrices})
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$. %; the best known lower bound on $m$ at present is 
% quadratic \cite{ressayre}.
By linear representation, we mean
the  entries   of $Y$ are  (possibly nonhomogeneous) 
linear functions of the entries of $X$. 
There is an analogous characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.
The main results of GCT for the $\#P$ vs. $NC$ problem in 
characteristic zero also extend to the $P$ vs. $NP$ problem in characteristic
zero. But here we shall 
concentrate  on only the former problem,
since this illustrates all the basic ideas. 

The original  lectures   stated a lower bound called 
a weak form of the $\#P$ vs. $NC$ problem. It  turned out 
to be too weak because it has an elementary proof \cite{} that does
not cross the natural proof barrier \cite{rudich}. 
This weak form  is actually a special case of a far more general   result,
called  a {\em mathematical form of the $\#P\not = NC$ conjecture} [GCT6],
which was not stated in the original lectures, but is stated here
(Section~\ref{}).  It is the second unconditional lower bound result 
of GCT. 
We cannot prove this result  by such elementary naturalizable 
techniques for the reasons explained in Section~\ref{}. 



The rest of this article is organized in the form of three chapters,
one per  lecture. The first gives a short mathematical 
overview of the basic plan of GCT,  
which is elaborated in the next two lectures. 


\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes}
      \label{fig:complexityclasses}
\end{figure} 




\noindent {\em Acknowledgement:} The author is grateful to 
Avi Wigderson for arranging the lectures and the hospitality.




\chapter{Basic plan} 
We now outline the basic  plan of GCT focussing on
the  permanent vs. determinant problem in characteristic zero. 

\section{Characterization by symmetries} \label{scharsym}
We begin by observing that 
the permanent and the determinant are 
{\em exceptional} polynomial functions. By exceptional we mean
that they are  completely characterized by the symmetries in the 
following sense.


Let  $Y$ be a variable $m\times m$ matrix.
Let $\sym^m(Y)$ be the space of homogeneous forms of degree $m$ 
in the $m^2$ variable entries of $Y$. Then, by the  classical
representation theory,  $\det(Y)$ is the only form in $\sym^m(Y)$ 
such that, for any $A,B \in GL_m(\C)$ with $\det(A)\det(B)=1$, 

\noindent  {\bf (D):} $\det(Y)=\det(A Y^* B)$,

where $Y^*=Y$ or $Y^t$. 
Thus $\det(Y)$ is completely characterized 
by its symmetries, and hence, is  exceptional. We shall refer 
to this characteristic property of the determinant as property (D)
henceforth.

Similarly, $\perm(X)$ is the only form 
in the space of forms of degree $n$ in the entries of $X$ such that, 
for any diagonal or permutation matrices $A,B$, 

\noindent  {\bf (P):} $\perm(X)=\perm(AX^*B)$, 

where $X^*=X$ or $X^t$ and the product of the (nonzero) 
diagonal entries of $A$ and $B$ is one.
Thus $\perm(X)$ is also
completely characterized   by its symmetries, and hence, is
exceptional.
We shall refer 
to this characteristic property of the permanent as property P
henceforth.





Any proof technique for the permanent vs. the determinant problem
has to ultimately make a nontrivial use of these  symmetries
  which characterize them. Indeed, one can say that 
these characteristic  properties 
lie at the heart of the permanent vs. determinant problem, and until
a proof technique has made a nontrivial use of them, it has
not entered the heart of the problem.
The most obvious interpretation of the phrase 
nontrivial here is the following: 

\begin{defn} \label{dnontrivial}
We say that a proof technique for the permanent vs. determinant 
problem makes a {\em nontrivial use of symmetries} if it does not work
for any functions (in place of the permanent or the determinant)
which do not have
nontrivial symmetries.
\end{defn}

Since symmetries is a fundamental geometric concept, we define
a  {\em geometric} approach to the permanent vs. determinant problem as
any  approach based on nontrivial use of the symmetry properties
(P) and (D) in this sense.
The meanining of the phrase geometric in the 
$P$ vs. $NP$ problem is
similar, since the  permanent and the determinant
can be replaced with   (co)-NP
and $P$ complete functions which are similarly
characterized by symmetries [GCT1]
(in a weaker sense that is good enough for our purposes).

GCT is a geometric approach in this sense.
Representation theory and 
algebraic geometry enter inevitably into  it, because
to understand symmetries, representation theory (of groups of symmetries)
becomes indispensible, and to understand  deeper properties 
of representations,  algebraic geometry becomes indispensible. 


\section{A mathematical form of the  $\#P \not = NC$ conjecture} 
\label{sweaklec1}
Before going any further, we now state one concrete application of 
GCT in the form of a concrete lower bound result--namely a 
mathematical form of the 
$\#P \not = NC$ conjecture (Theorem~\ref{tgenweaklec1} below).

We begin by observing that 
the permanent vs. determinant conjecture clearly implies  that 
$\perm(X)$ of any $n \times n$ variable matrix $X$ can not be represented 
as an $NC$-computable polynomial in the traces of $\bar X^j$, $j \ge 0$,
$\bar X=B X C$
for any (possibly singular) $n\times n$ matrices $B$ and $C$, since
$X^j$ can be computed fast in parallel. This can be proved unconditionally.
In fact, something stronger.

\begin{prop}  \label{pweaklec1}
There do not exist (possibly singular) $n\times n$ complex
matrices $B$ and $C$  and a polynomial 
$e(w_0,\ldots, w_n)$ such that $\perm(X) = g(BXC)$, 
where $g(X)=e(\trace(X^0), \trace(X), \ldots, \trace(X^n))$. 
\end{prop}
This was referred to as 
the weak form of the $\#P$ vs. $NC$ problem in the original IAS lecture. 
The article \cite{boris} showed that this is too  weak 
by giving an  elementary
proof \cite{boris} for it that is naturalizable, i.e.,
which cannot cross the
natural proof barrier \cite{rudich} because it works for most functions in
place of the permanent. The proof technique of
the quadratic lower bound \cite{ressayre}
for the permanent is also naturalizable.

We now state a much more general lower bound, which
was not stated in the IAS lecture, and which does not have such 
a naturalizable proof. For that we need a definition.

\begin{defn} \label{dgenperm}
A polynomial function $p(X_1,\ldots,X_k)$ (of any degree)
in the entries of $k$ $n\times n$ variable matrices 
is called a  {\em generalized permanent} if it has exactly 
the same symmetries as that of the permanent; i.e.,
for all nonsingular $n\times n$ matrices $U$ and $V$, 
\[ p(U X_1 V,\ldots, U X_k V)=p(X_1,\ldots,X_k) 
\mbox{\ iff\ } \perm(U X V)=\perm (X).\] 
\end{defn}

A precise description of the symmetries of the permanent  is given
by the property (P). Hence, $U$ and $V$ above have to be permutation
or diagonal matrices (with product of the nonzero  diagonal entries being
one), or 
product of such matrices.
When $k=1$ and $n$ is arbitrary,
there is just one generalized permanent of degree $n$, namely
the usual permanent itself. But for general degrees, 
the dimension of the 
space spanned by  generalized permanents can be  exponential
in $n$; cf. Section~\ref{sweak}. At the other extreme, 
when $n=1$ and $k$ is arbitrary, every function in $k$ variables 
is a generalized permanent. 
In general,  the space of generalized permanents has a highly nontrivial
structure that  is intimately linked  to some
fundamental problems of representation theory;
cf. Section~\ref{sweak} and  [GCT6].


The original nonuniform 
$\#P$ vs. $NC$  conjecture
implies the following. 

\noindent {\bf Implication of the nonuniform $\#P \not = NC$ conjecture:}

Any $\#P$-complete generalized permanent  $p(X_1,\ldots,X_k)$ of $\poly(n,k)$ 
degree cannot be expressed as an $NC$-computable polynomial function of the 
traces of arbitrary  monomials of polynomial length 
in $\bar X_i$, $1 \le i \le k$, where 
$\bar X_i=B X_i C$,  $i \le k$,  for any $n\times n$ complex (possibly
singular) matrices $B$ and $C$. Here by a monomial 
in $\bar X_i$ we mean
any matrix product  of the form $\bar X_{i_1}\ldots \bar X_{i_r}$, 
$1 \le i_1, \ldots  i_r \le k$.
We say that it is of polynomial length if 
$r=\poly(n,k)$ (it is then clearly $NC$-computable).

When $n=1$ and $k$ is arbitrary, this is  equivalent 
to the original nonuniform $\#P \not = NC$ conjecture,
since then any polynomial in $x_1,\ldots, x_k$ is a generalized permanent,
and a polynomial function of  the traces of monomials in $x_i$'s means any
polynomial in $x_1,\ldots,x_k$. This cannot be proved at present.
But the next case,  $n>1$ and $k$ arbitrary, can be:

\begin{theorem}[GCT6]

\noindent {\bf (A mathematical form of the  $\#P \not = NC$ conjecture)}
 \label{tgenweaklec1}

The implication above holds unconditionally for any $n>1$ and arbitrary $k$.

In fact, something stronger then holds. Namely, 
when  $n>1$ and $k$ is arbitrary, no generalized permanent $p(X_1,\ldots,X_k)$
can be expressed as a polynomial function of the traces of 
arbitrary  monomials in $\bar X_i$, $1 \le i \le k$, where 
$\bar X_i=B X_i C$,  $i \le k$,  for any $n\times n$ complex (possibly
singular) matrices $B$ and $C$.
\end{theorem}

When  $k=1$ and $p(X)$, $X=X_1$, is the usual permanent, this specializes to
Proposition~\ref{pweaklec1}.


We are calling this a mathematical form for two reasons. 
First, it is a mathematical
lower bound rather than a complexity theoretic lower bound in the sense
that it needs  no restriction on the computational complexity of
$p(X_1,\ldots,X_k)$ or the polynomial in the traces.
Thus it is rather in the spirit of the classical result of Galois theory 
which says that a general polynomial of degree $>5$ 
cannot be solved by any number of
radical operations, without any restriction on the number of such
operations. 
Second, observe that 
the permanent has two characteristic properties: 1) the property 
P (mathematical), and 2) $\#P$-completeness (complexity-theoretic). 
The usual complexity theoretic form of the $\#P\not = NC$ conjecture
is a lower bound for  all polynomial functions with 
the  $\#P$-completenes property, whereas the mathematical form 
is  a lower bound for all polynomial functions with the 
property (P).  In other words,  the complexity theoretic form
is associated with the $\#P$-completeness property of the
permanent and the mathematical form with 
the property (P). 




The result indicates that there is thus a chasm
between the two adjacent cases: $n=1$, $k$ arbitrary (the usual nonuniform
complexity theoretic $\#P \not = NC$ conjecture), and 
$n=2$, $k$ arbitrary (its mathematical form above). 
The complexity theoretic form is   much harder than the mathematical
form, and  a proof technique for the easier mathematical form
can be expected to give us a crucial insight into what is needed to prove 
the harder  complexity theoretic form.


For some specific
generalized permanents (cf. Section~\ref{sweak}), this result again has
an elementary naturalizable proof as in \cite{boris}.
It also has an elementary naturalizable proof for a generic 
generalized permanent, just as the fact that a generic polynomial is
hard to compute has an elementary naturalizable proof.
The nontrivial part of this 
result (which needs nonelementary proof) 
is that it holds for any generalized permanent.
Indeed the basic difference between the complexity theoretic 
and the mathematical  settings is
the following. The complexity theoretic  (i.e. the usual) $\#P \not = NC$
conjecture 
is universal in the sense 
that if it is proved for one $\#P$-complete function (say
the permanent), it automatically 
holds for all $\#P$-completeness functions (because
of the theory of $\#P$-completeness). But there is no such completeness
theory at the mathematical level. Hence, a mathematical
lower bound  for a specific 
generalized permanent, e.g., the permanent,
does not say anything about all (even $\#P$-complete)
generalized permanents. To get 
 similar universality,   the  mathematical
form of the $\#P\not = NC$ conjecture above  covers up this lack of 
completeness theory
at the mathematical level by proving a result for all polynomial functions
with property (P), not just a specific one. 
The articles \cite{boris,ressayre} suggest that without such universality
a restricted weaker form of the $\#P\not =NC$ conjecture
may be  provable by  a naturalizable proof technique. 



In contrast, it may be conjectured that Theorem~\ref{tgenweaklec1} cannot 
be proved by a naturalizable technique. This is because 
the only thing that is common among  all generalized permanents is the
property (P).  Hence any proof of this result would be 
essentially  forced
to rely only on  this property like  its GCT proof (cf. Section~\ref{sweak}).
Any such proof automatically passes the natural proof 
barrier since it is easy to show that most functions do not
have property $P$ when $n>1$ and $k$ is arbitrary.
It may be remarked that the algebraic degree barrier is not 
applicable in the permanent vs. determinant problem because both
permanent and determinant have the same degree. It is not applicable
in the context of Theorem~\ref{tgenweaklec1} as well for the same reasons.
Similarly, the relativization barrier is not applicable in the context
of the permanent vs. determinant problem because the $NC$-computation 
has been algebrized in it in the form of the determinant, and the
relativization barrier does not apply to such algebraic techniques 
(just as it does not apply to the proof of the 
$IP=PSPACE$ result).
The relativization barrier does not apply in the context of 
Theorem~\ref{tgenweaklec1} 
for the same reason. Thus it can be said that the proof technique of
Theorem~\ref{tgenweaklec1} crosses the
natural proof, algebraic degree (algebrization)
and relativization barriers simultanesouly.

Ultimately, any approach to the $\#P \not = NC$ conjecture
is expected to prove some restricted
form of this conjecture, not necessarily Theorem~\ref{tgenweaklec1},
whose proof crosses these barriers simultaneously.
At present, we do not have any other lower bound  result of this kind.



Though the statement of Theorem~\ref{tgenweaklec1} is elementary, its proof 
is nonelementary and is based on  some fundamental results 
in geometric invariant theory \cite{mumford} and the results in GCT1 and 2 
based on these results. These nonelementary techniques
are needed to cope up with a highly nontrivial 
structure of the space of generalized permanents as 
explained in Section~\ref{sweak}. 




\section{From nonexistence to existence}
The rest of this lecture  outlines  the GCT approach to 
the general  permanent vs. determinant problem,
and then  points out 
the crucial steps in this plan which can be completely executed
for the weaker  mathematical form  of the $\#P\not = NC$ conjecture above,
but which are conjectural at present for 
the general permanent vs. determinant problem. 

The first  step 
(GCT1,2) is to reduce this nonexistence problem--i.e., that there is no
small linear representation  of the permanent as a determinant--to
an existence problem--specifically, to the problem of proving 
existence of a family $\{O_n\}$ of obstructions; 
cf. Figure~\ref{fig:firststep}.
Here an {\em obstruction} $O_n$ is a proof-certificate of
hardness of $\perm(X)$, $X$ an $n\times n$ variable matrix,
just as the Kuratowski minor is a proof-certificate of the nonplanarity of a 
graph.  Specifically,  it is some 
algebro-geometric-representation-theoretic gadget
whose existence for every $n$  serves as a 
guarantee that $\perm(X)$ cannot be represented linearly as $\det(Y)$,
when $m=2^{\log^a n}$, $a>0$ fixed, $n\rightarrow \infty$ (i.e., for
$n$ greater than a large enough constant depending on $a$). 



\begin{figure} 
\begin{center}\psfragscanon
\psfrag{on}{$\{O_n\}$}
\epsfig{file=firststep.eps, scale=.8}
\end{center}
      \caption{Reduction from nonexistence to existence}
      \label{fig:firststep}
\end{figure}



This reduction to existence is carried out as follows (cf. lecture 2 for 
details).


First, we associate (GCT1) with 
the complexity class $\#P$ a family $\{X_{\#P}(n,m)\}$ of (group-theoretic)
class varieties (what this means is explained below),
and with the complexity class $NC$ a family of 
$\{X_{NC}(n,m)\}$ of (group-theoretic) class varieties such that: 
if $\perm(X)$, $\dim(X)=n$, can be represented linearly 
as $\det(Y)$, $\dim(Y)=m>n$, then 

\begin{equation} \label{eqembed} 
X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation} 

Each  class variety is a  (projective) algebraic variety, by which
we mean that it is the zero set of  a system of multivariate 
homogeneous polynomials with coefficients in $\C$  (akin to the 
usual curves  and surfaces). It is  group-theoretic in the 
sense that it is  constructed using group-theoretic operations 
and the general linear group $G=GL_l(\C)$, $l=m^2$, of $l\times l$ invertible
complex matrices acts on it. Here action means moving the points 
of the class variety around, just as $G$ moves the points of $\C^l$ around 
by the standard action via invertible linear transformations.
The goal is to show that the inclusion (\ref{eqembed}) is impossible
(obstructions are meant to ensure this);
cf. Figure~\ref{fig:class}. 

\begin{figure} 
\begin{center} \psfragscanon
\psfrag{xsharp}{$X_{\#P}(n,m)$}
      \psfrag{xnc}{$X_{NC}(n,m)$}
      \psfrag{g}{$G=GL_l(\C)$, $l=m^2$}
      \psfrag{Obstruction}{\mbox{Obstruction}}
\epsfig{file=class.eps, scale=.5}
\end{center}
      \caption{Class varieties}
      \label{fig:class}
\end{figure} 



Since each class variety has a $G$-action, the space of polynomial functions 
on each class variety has a  representation-theoretic structure, which 
puts constraints on which  representations of $G$ can live on that variety
(i.e., in the space of polynomial  functions on that variety).
Informally, an obstruction is an irreducible (minimal)  representation of $G$
that can live on $X_{\#P}(n,m)$ but not on $X_{NC}(n,m)$; 
cf. Figure~\ref{fig:class}.
Existence of  an obstruction $O_n$, for every $n$, assuming
$m=2^{\log^a n}$, $a>1$ fixed, implies  that the inclusion (\ref{eqembed}) 
is not possible, since  $O_n$ cannot live  on $X_{NC}(n,m)$.
Thus  an obstruction blocks the inclusion (\ref{eqembed}).


To define an obstruction formally, we need to recall some basic representation
theory.  By a classical result of Weyl, the irreducible 
(polynomial) representations of $G=GL_l(\C)$ are in one-to-one correspondence 
with the partitions  $\lambda$ of length at most $l$, by which we mean 
integral sequences $\lambda_1 \ge 
\lambda_2 \cdots \ge \lambda_k > 0$, $k\le l$, where  $k$ is called the  length
of $\lambda$. The irreducible 
representation of $G$ in correspondence with $\lambda$ is denoted 
by $V_\lambda(G)$, and is called the {\em Weyl module} of $G$ indexed by 
$\lambda$. Symbolically:

\[\mbox{Irreducible representations of } G \stackrel{\mbox{Weyl}}{\Longleftrightarrow} \quad \mbox{partitions} \ \lambda. \]  

\[\mbox{Weyl module  } V_\lambda(G)  \longleftrightarrow \lambda. \] 
Weyl also proved that every finite dimensional representation of $G$ 
can be decomposed into irreducible representations--i.e.,
can be written as a direct sum of Weyl modules. Thus Weyl modules 
are the basic building blocks of the representation theory of 
$G$, and every finite dimensional representation of $G$ can be thought
of as a complex building made out of these blocks. 


Now suppose $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$. 
Suppose to the contrary that 

\begin{equation} \label{eqembed2}   X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation}

Let $R_{\#P}(n,m)$ denote the homogeneous coordinate ring of 
$X_{\#P}(n,m)$; i.e., the ring of polynomial functions 
\footnote{Though the  functions here are not functions in usual sense;
but let us  not worry about this} on $X_{\#P}(n.m)$. 
Let $R_{\#P}(n,m)_d$ be the degree-$d$-component of $R_{\#P}(n, m)$ consisting
of functions of degree $d$. We define $R_{NC}(n,m)$ and $R_{NC}(n,m)_d$
similarly. Since $X_{\#P}(n,m)$ has the action of $G$, $R_{\#P}(n,m)$ 
also has an action of $G$; i.e., it is a representation of $G$. Hence,
$R_{\#P}(n,m)_d$ is a finite dimensional representation of $G$. 
Similarly, $R_{NC}(n,m)$ is a representation of $G$, and $R_{NC}(n,m)_d$
a finite dimensional representation of $G$. 



If (\ref{eqembed2}) holds, then we get a natural map from $R_{NC}(n,m)$ to
$R_{\#P}(n,m)$ obtained by restricting a function on $X_{NC}(n,m)$ to
$X_{\#P}(n,m)$. %; cf. Figure~\ref{fig:restriction}.
By basic algebraic geometry, this map
is surjective and is a $G$-homomorphism.
Furthermore, it is degree-preserving. This means there
is a surjective $G$-homomorphism from $R_{NC}(n,m)_d$ to 
$R_{\#P}(n,m)_d$. Symbolically: 

\begin{equation} \label{eqsurjection}
R_{\#}(n,m)_d \leftarrow  R_{NC}(n,m)_d.
\end{equation}

\ignore{
\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{Xp}{\small $X_{\#P}(n,m)$}
\psfrag{Xnc}{\small $X_{NC}(n,m)$}
\epsfig{file=restriction.eps, scale=.6}
\end{center}
      \caption{Restriction}
      \label{fig:restriction}
\end{figure}
}

Let $R_{\#P}(n,m)_d^*$ denote the dual of $R_{\#P}(n,m)_d$; i.e., the 
set of linear maps from $R_{\#P}(n,m)_d$ to $\C$. Then (\ref{eqsurjection})
implies that there is an injective $G$-homomorphism from 
$R_{\#P}(n,m)^*_d$ to $R_{NC}(n,m)^*_d$. Symbolically: 

\begin{equation} \label{eqinclusion}
R_{\#}(n,m)_d^*  \hookrightarrow {NC}(n,m)_d^*.
\end{equation}

\begin{defn} (GCT2)
An obstruction $O_n$ is a Weyl module $V_\lambda(G)$ that 
occurs as a subrepresentation 
in $R_{\#P}(n,m)_d^*$  but not in $R_{NC}(n,m)_d^*$, for some $d$. 
We call $\lambda$ an {\em obstruction label}, and sometimes,
by abuse of notation, an obstruction as well.
\end{defn}

\begin{prop} (GCT2)
Existence of an obstruction $O_n$, for all $n\rightarrow \infty$, 
with $m=2^{\log^a n}$, $a>1$ fixed, implies $\perm(X)$, $\dim(X)=n$, 
cannot be represented linearly as 
$\det(Y)$, $\dim(Y)=m$. 
\end{prop}

This follows just from the definition of an obstruction, and 
leads to:

\begin{goal} \label{gobs} (GCT2)
Prove existence of an obstruction family $\{O_n=V_{\lambda_n}(G)\}$ using 
the  exceptional 
nature of $\perm(X)$ and $\det(Y)$, i.e., using the 
properties (P) and (D) in  Section~\ref{scharsym}).
\end{goal} 

\section{Obstructions for the mathematical form} \label{sobsweak}

The following result achieves this goal for the mathematical form
(Theorem~\ref{tgenweaklec1}).
\begin{theorem} 
There exists an obstruction family $\{O_n\}$ for the mathematical
form  of the $\#P \not = NC$ conjecture.
\end{theorem}

This implies Theorem~\ref{tgenweaklec1}.
The notion of obstructions here is similar 
to the one in the general case. 

The proof of this result  based on the results of GCT1 and 2 in
geometric invariant theory \cite{mumford} is outlined in the third lecture.
It produces  a {\em strongly  explicit} 
family $\{O_n=V_\lambda(G)\}$ of obstructions, with a different $G$
than in the general complexity theoretic case.
This is strongly explicit in the sense (cf. Introduction) that 
the specification $\lambda_n$ of each $O_n$
has polynomial, in fact,  $O(n)$ bitlength, and  
can be constructed in polynomial, in fact, $O(n)$ time (regardless of the 
complexity  of the polynomial in the traces in the statement of 
Theorem~\ref{tgenweaklec1}).

\noindent {\em Remark:}
There is also a second noncostructive proof of this result 
(cf. Section~\ref{sweak}).
This gives a concrete evidence 
that explicit construction is not needed to cross the 
natural proof   barrier. Because 
any proof that relies only on the property (P) automatically
bypasses this barrier, as remarked before.
But   this nonconstructive
proof is not any easier than the explicit proof, in fact, a bit harder.
Indeed, the whole proof
structure  here is such that its easiest implementation  yields 
obstructions explicitly 
whether one cares for them or not. We shall see the same pheonomenon
in the general case in what follows.


\section{Towards existence of obstructions in general via positivity}
We now proceed to describe the main results of GCT for the general
(complexity-theoretic)
permanent vs. determinant problem in the context of
Goal~\ref{gobs}. 



Towards that end, we  associate with the class varieties 
certain representation-theoretic {\em stretching} functions. 
Let $F_{\lambda,n,m}(k)$ denote the number of occurances (multiplicity)  of
the Weyl module $V_{k\lambda}(G)$ in $R_{\#P}(n,m)^*$ (i.e. 
$R_{\#P}(n,m)^*_d$, for some $d$)  as a subrepresentation,
and $G_{\lambda,n,m}(k)$ the number of occurances of 
$V_{k\lambda}(G)$ in $R_{NC}(n,m)^*$. These are statistical functions
associated with the class varieties, where the statistics associates 
with every number (stretching parameter) $k$  
the multiplicity of the corresponding
Weyl module $V_{k\lambda}(G)$; cf. Figure~\ref{fig:statistics}.

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{l}{$\lambda$}
\psfrag{2l}{$2 \lambda$}
\psfrag{3l}{$3 \lambda$}
\psfrag{v1}{$V_\lambda(G)$}
\psfrag{v2}{$V_{2 \lambda}(G)$}
\psfrag{v3}{$V_{3\lambda}(G)$}
\epsfig{file=statistics.eps, scale=1}
\end{center}
      \caption{statistics}
      \label{fig:statistics}
\end{figure}


Let us  call a function $f(k)$ {\em quasipolynomial}, if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k)$ for all nonnegative integral $k=i$ modulo $l$;
here  $l$ is
called the period of the  quasi-polynomial. 
Thus  quasi-polynomials
are hybrids of  polynomial and periodic functions. 
We say that $f(k)$ is an 
{\em asymptotic quasipolynomial} if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k)$ for all nonnegative integral $k=i$ modulo $l$ for 
$k\ge a(f)$, for 
some nonnegative integer depending on $f$. The minimum 
$a(f)$ for which this holds is called the {\em deviation from 
quasipolynomiality}. Thus $f(k)$ is a (strict) quasipolynomial when this
deviation is zero.

A fundamental example of a quasi-polynomial is the Ehrhart quasi-polynomial
$f_P(k)$ of a polytope $P$ with rational vertices. It is defined
to be the number of integer points in the dilated polytope $kP$. By the 
classical result of Ehrhart, it is known to be a quasi-polynomial.
More generally, let $P(k)$ be a polytope parametrized by nonnegative
integral $k$: i.e., 
defined by a linear system of the form: 
\begin{equation} \label{eqpara}
A x \le k b + c,
\end{equation}
where $A$ is an $m \times n$ matrix, $x$ a variable $n$-vector, and 
$b$ and $c$ some constant $m$-vectors. Let $f_P(k)$ be the number 
of integer points in $P(k)$. We shall call it the Ehrhart function of
$P(k)$.  It is known to be  an asymptotic quasi-polynomial.
In what follows, we  denote a parametrized polytope $P(k)$ by 
just $P$. 




\begin{theorem} (GCT6) \label{tquasi}
The functions $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ 
are asymptotic quasi-polynomials. Furthermore, they 
are (strict) 
quasi-polynomials assuming that the singularities of the class varieties
$X_{\#P}(n,m)$ and $X_{NC}(n,m)$ are rational and normal. 

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem} 

Here a rational and normal  singularity means a singularity that is nice in
an algebro-geometric sense that we shall not elaborate here.
At present, we do not know if the singularities of the class varieties 
are indeed  rational and normal. A conservative conjecture would be  that 
they are not too bad, even if they are not strictly rational and normal,
because of the exceptional nature of the 
determinant and the permanent; 
i.e.,  the deviation from quasipolynomiality
of $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ is 
small in a sense to be made precise 
later (cf. the remarks after Hypothesis~\ref{hph1}).

The proof of Theorem~\ref{tquasi}
follows from a detailed study of the behaviour
of the singularities of class varieties under the action of the 
group $G$. This is based on
\begin{enumerate} 
\item The 
resolutions of singularities in characteristic zero
\cite{hironaka}: 
this  roughly says 
that the singularities of any algebraic variety in characteristic zero
can be untangled (resolved) nicely in a systematic fashion; cf.
 Figure~\ref{fig:resolution}.
\item Cohomological works of Boutot, Brion,  Flenner, Kempf  and others
based on this resolution; cf.  \cite{boutot,dehy} and
GCT6 for the history and other references.
\end{enumerate} 


\begin{figure} 
\begin{center} 
\epsfig{file=resolution.eps, scale=.5}
      \caption{Resolution}
      \label{fig:resolution}
\end{center}
\end{figure}


As such, this proof is highly nonconstructive. It gives no effective
bound on the period $l$--it just says that $l$  is finite.





The following hypothesis 
says that $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ 
can be realized as the Ehrhart functions  of parametrized  polytopes.

\begin{hypo} {\bf (PH) [Positivity Hypothesis]} \label{hph} (GCT6)

\noindent (a) For every $\lambda,n,m\ge n$, 
there exists   a parametrized  polytope $P=P_{\lambda,n,m}$ 
such that 
\begin{equation} \label{eqP}
F_{\lambda,n,m}(k)=f_P(k).
\end{equation} 
It is also assumed here that there exists for $P_{\lambda,n,m}$ a specification
of the form (\ref{eqpara}),
 where $A$ is independent of $\lambda$, and $b$ and $c$ 
are  piecewise homogeneous linear functions of $\lambda$.


\noindent (b) There exists a similar parametrized 
 polytope  $Q=Q_{\lambda,n,m}$  such that
\begin{equation} \label{eqQ}
G_{\lambda,n,m}(k)=f_Q(k).
\end{equation}


Analogous positivity hypothesis also holds 
for the $P$ vs. $NP$ problem in characteristic zero.
\end{hypo} 


If such $P$ and $Q$ exist, their dimensions are guaranteed to be
small by the proof of Theorem~\ref{tquasi}: specifically,
the dimension $P$ is guaranteed to be bounded by a 
polynomial in $n$, and the dimension of $Q$ 
by a polynomial in $m$.
There is a variant of PH (b), which is good enough for our purposes (cf.
Lecture 3, Hypothesis~\ref{hphvariant}),
wherein  the dimension of $Q$ is also guaranteed
to be bounded by a polynomial in $n$ (but independent 
of $m$), if the length of $\lambda$ is $\poly(n)$ (as it would be in 
our applications).






When PH holds, we say that $F_{\lambda,n,m}(k)$ and 
$G_{\lambda,n,m}(k)$ have  {\em positive convex representations}. 
Here positivity refers to the fact that the Ehhart function 
$f_P(k)$ is a positive expression:
\[ f_P(k)=\sum_{v} 1,\] 
where $v$ ranges over all integer points in $P(k)$--there are no 
alternating signs in this expression.
Convexity refers to the  convexity of the polytopes $P(k)$ and $Q(k)$. 


But, a  priori, it is not at all clear why PH should  even hold. 
Many numerical functions in algebraic geometry are 
asymptotic quasi-polynomials (e.g., the Hilbert function 
\footnote {Hilbert function $h_Z(k)$ of a projective algebraic variety $Z$
is defined to be $\dim(R(Z)_k)$, where $R(Z)$ is the homogeneous coordinate 
ring of $Z$ and $R(Z)_k$ its degree $k$-component.} of any projective
variety), but they rarely have positive convex representations.
PH is expected to hold for $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ 
because of the exceptional nature of the determinant and the permanent. 
One concrete evidence is provided by the proof of the weak form 
(Thoerem~\ref{tgenweaklec1}).
Analogous PH that arises in this weak setting can 
proven unconditionally.
For  mathematical evidence and justification
in support of  general PH, see  GCT6,7, and 8. 


The hypothesis 
PH alone is not sufficient to prove the existence of obstructions.
The precise statement of a sufficient condition is given in 
the theorem below.




\begin{theorem} (GCT6) \label{tgct6}
There exists a family $\{O_n\}$ of obstructions 
for the  $\#P$ vs. $NC$ problem in characteristic zero, 
for $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$, 
assuming, 

\begin{enumerate} 
\item PH, and
\item OH (Obstruction Hypothesis): 

For all $n\rightarrow \infty$,  there exists $\lambda$ such that 
$P_{\lambda,n,m}(\infty)=\mbox{lim}_{k\rightarrow \infty} P(k) 
\not = \emptyset$ and $Q_{\lambda,n,m}(k)=\emptyset$ for all (large enough)
$k$.
\end{enumerate}

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem}

Mathematical evidence and arguments in support of OH are given in GCT6.
The analogous weak OH that arises in the context of the generalized 
weak form can be  proven unconditionally.

We call  $\lambda$ a {\em relaxed obstruction}
(or rather, relaxed obstruction-label)
if it satisfies OH. In this case, $k\lambda$, for some integer $k\ge 1$ is
an obstruction--we just have to choose $k$ large enough 
so that 
$P_{\lambda,n,m}(k)$ contains an integer point
but $Q_{\lambda,n,m}(k)$ does not.
Henceforth, whenever we say obstruction, we actually mean relaxed 
obstruction.

There is a fundamental difference between the nature of PH and OH.
PH is a {\em mathematical hypothesis}, because there is no 
constraint on what $m$ should be in comparison to $n$ in its statement.
In contrast, OH is a {\em complexity theoretic hypothesis}, because 
$m$ needs to be small in comparison to $n$ for it to hold.


%\subsection{Why should PH  and OH hold?} 

%Mathematical evidence for this is given in GCT2,4,6,7,8.
%We shall discuss some of this  in the third lecture.


\section{The flip: Explicit construction of obstructions} 
\label{sflip}
In principle PH may have a nonconstructive proof (like that
of Theorem~\ref{tquasi})  which only tells  that such polytopes 
exist without explicitly constructing them. But proving OH may not be feasible
unless the polytopes $P$ and $Q$ in PH are given explicitly.
This  suggests the following strategy for proving 
existence of obstructions proposed in  GCT6 and  GCTflip.


\noindent (1) Prove the following stronger explicit form 
of PH, which is reasonable since the polytopes $P$ and $Q$, if they exist,
are already guaranteed to be of small (polynomial) dimension:

\begin{hypo} {\bf (PH1)}  \label{hph1} (GCT6)

\noindent (a) There exists an {\em explicit} 
polytope $P_{\lambda,n,m}$ 
as in  PH (a).
Explicit means: 

\begin{enumerate}
\item  The polytope is specified by an explicit system of linear constraints,
where the bitlength of (the description of) 
each constraint is  $\poly(n,\bitlength{\lambda}, \bitlength{m})$.
Here and in what follows, $\bitlength{z}$ denotes the bitlength of the 
description of $z$.

\item  The membership problem for the polytope
$P_{\lambda,n,m}(k)$  also 
belongs to the complexity class $P$.
That is,  given a point $x$, whether it belongs to $P_{\lambda,n,m}(k)$ 
can also be decided in $\poly(\bitlength{x},\bitlength{\lambda},
n,\bitlength{m})$
time.
Furthermore, we assume that if $x$ does not belong to the polytope,
then the membership algorithm also gives a hyperplane separating 
$x$ from the polytope in the spirit of \cite{lovasz}. 
\end{enumerate} 

\noindent (b) There exists a similar  explicit 
polytope $Q_{\lambda,n,m}$  satisfying   PH (b). 
\end{hypo}

\noindent {\em Remark 1:} 
Note the occurence of  $\bitlength{m}$  instead of $m$ in the polynomial
bounds in (a) (which implies that the bounds here become $\poly(n)$
when $m<2^n$ and $\bitlength{\lambda}=\poly(n)$). 
The reasons for this will be explained in Lecture 3 
(cf. remarks after Hypothesis~\ref{hph1restatement}). 
In contrast, the polynomial bounds for the polytope in (b)  depend on 
$m$, not $\bitlength{m}$. 
But there are  variants of PH (b) and PH1 (b), 
(cf. Hypotheses~\ref{hphvariant} and \ref{hph1tilde} in  Lecture 3), 
which are enough for our purposes, 
wherein the polynomial bounds depend on the bitlength of $\lambda$,
but not on $m$.
In what follows, we assume that PH (b) and PH1 (b) have been replaced 
with these variants.

 


\noindent {\em Remark 2:} 
In particular, PH1 implies that the functions $F_{\lambda,n,m}(k)$ and
$G_{\lambda,n,m}(k)$ belong to the complexity class $\#P$. 
It can be shown that it 
also implies that the deviation from quasipolynomiality 
of $F_{\lambda,n,m}(k)$ is small, specifically, 
$2^{O(\poly(\bitlength{\lambda},n,\bitlength{m}))}$--thus the bitlength
of the deviation is polynomial. This says
that the deviation from rationality and normality of the singularities
of the class variety $X_{\#P}(n,m)$ is small (cf. Theorem~\ref{tquasi}).
Similarly for $Q_{\lambda,n,m}(k)$ and $X_{NC}(n,m)$. 

Like PH, PH1 is also a mathematical hypothesis in the sense that
it puts  no constraint on what $m$ should be in comparison to $n$. 
Of course, unlike PH, there is some complexity theoretic aspect to it, 
but it is secondary in comparison to the complexity-theoretic aspect of 
 OH, since smallness  of $m$ with respect to  $n$ is the 
crux of the lower bound  problems under consideration. 





\noindent (2a) {\bf [The flip]}

Let $m=2^{\log ^a n}$, for a fixed $a>1$. 
Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
show existence of  an {\em explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of (relaxed) obstructions  satisfying OH. 
We say that an obstruction (proof-certificate) 
$\lambda_n$ is {\em explicit} if is ``short'' and ``easy to verify'':


\begin{enumerate} 
\item  Short: This means its bitlength $\bitlength{\lambda_n}$ 
is $\poly(n)$,
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  

\item Easy to verify: given $n, m \le 2^{n}$ and 
$\lambda_n$, whether 
$\lambda_n$ is a valid obstruction 
can be verified 
in $\poly(n,\bitlength{\lambda})$ time. In particular, this is
$\poly(n)$ when $\bitlength{\lambda}=\poly(n)$. 
\end{enumerate}

Existence of an explicit family of obstructions is equivalent to saying
that the problem of deciding existence of obstructions belongs to $NP$.
This definition of explicitness is quite natural since the class $NP$ 
is a class of problems whose proof-certificates (witnesses) are 
short and easy to verify. As such, the flip--going for 
explicit  obstructions--is
a proof-strategy that is literally given to us on a platter 
by the $P$ vs. $NP$ 
problem itself. Why it is called flip will be explained later.


It should be stressed that we are primarily interested in only proving 
existence of obstructions. Whether they are explicit or not 
does not really matter in the original statement of the problem.
But we need to know the polytopes $P$ and
$Q$ explicitly (as in PH1)  so that proving OH is feasible. 
%In other words,   if we do not
%even know what the polytopes $P$ and $Q$ look like, 
%it seems unlikely that anything  could be said regarding OH. 
But once  PH1 is proved, existence of an explicit family follows
automatically,   as a bonus, whether we care for it or not. 

To see why, let us observe that 
the second condition above  (ease of verification) follows directly
from PH1 and the polynomial time algorithm for 
linear programming on  polytopes given by separation oracles \cite{lovasz}. 
Shortness  also follows from PH1. 

Thus it is as if the $P$ vs. $NP$ problem is forcing us to go
for explicit obstructions.


\noindent (2b) {\bf [The strong flip (optional)]} 

Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
construct (rather than just show existence of) 
a {\em strongly explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of obstructions  satisfying OH. We say that an explicit family 
of obstructions is strongly explicit if,
for each $n$, a valid obstruction-label
$\lambda_n$ can be constructed in $\poly(n)$ time.
In particular, the height and the bitlength of
 $\lambda$ is $\poly(n)$ (short) 
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  


For the purposes of the lower bound problems that we are interested in, the
flip (just explicit  
existence) would suffice and the stronger flip (explicit construction)
is optional. But the stronger flip can give us deeper insight into these
lower bound problems; cf. GCTflip for more on this.

Now we turn to a few obvious questions.



\section{What has been achieved by all this?: The meaning of the flip} 
\label{smeaning}
Let us now see what has been achieved so far
in the context of the 
$\#P\not = NC$ conjecture in the nonuniform setting (characteristic zero),
the argument for the $P$ vs. $NP$ problem in characteristic zero
being  similar. 
At  first glance,
it may seem that all that GCT has achieved 
is to exchange a known difficult problem of 
complexity theory with a new very difficult problem of algebraic geoemtry.
In order to see that something is gained in exchange let us reexamine the 
original question.

The goal of the original  conjecture is to prove that 
$\perm(X)$, $\dim(X)=n$,  cannot be computed by an arithmetic circuit $C$
of size $m=\poly(n)$, or more generally,
$m \le 2^{\log^a n}$, for some fixed $a>1$, and depth $O(\log^a n)$.
Symbolically, 
let  $f_C(X)$ denote the function computed by $C$. Then we want to prove that
\begin{equation} \label{eqioh} 
 {\bf (IOH):}  \forall n \ge n_0 \forall C \exists X:
\perm(X)\not = f_C(X),
\end{equation} 
where $n_0$ is a sufficiently large constant.
For given $X$ and $C$ of $\poly(n)$ size, the problem 
of deciding if  $\perm(X) \not = f_C(X)$
belongs to $\#P$ (or rather, $P^{\#P}$). 
Since there are two alternating layers of quantifiers in (\ref{eqioh}),
the problem of verifying it belongs to $\Pi_2^{\#P}$, 
which is very high in the complexity hierarchy
(cf. Figure~\ref{fig:IOHcomplexity}).
Hence, we  refer to the original hypothesis (\ref{eqioh}) 
to be proven  as IOH 
(Infeasible Obstruction Hypothesis). Of course, IOH is expected to 
be a tautology, and hence is expected to  be verifiable in $O(1)$ time--but
we do not know that as yet. 



\begin{sidewaysfigure} 
\begin{center}
\psfragscanon
\psfrag{sigma2p}{{\small $\Pi^2 \#P$}}
\psfrag{sigma1p}{$\Sigma^1 \#P$}
\psfrag{P}{{\small $P$}}
\psfrag{NP}{{\small $NP$}}
\psfrag{T}{$T$}
\psfrag{#P}{$\# P$}
\psfrag{inNP}{$\in NP$}
\psfrag{inP}{$\in P$}
\psfrag{insigma2p}{$\in \Pi^2 \#P$}
\psfrag{PHplus}{PH1}
\psfrag{PHtil}{$PH^\dagger$}
\epsfig{file=IOHcomplexity.eps, scale=.8}
\end{center}
      \caption{Positivity as a means to eliminate the quantifiers and 
reduce the complexity of the  obstruction hypothesis}
      \label{fig:IOHcomplexity}
\end{sidewaysfigure}



Equivalently, the goal of IOH 
is to prove existence of a {\em trivial obstruction},
which is a table that lists for each $C$ as above a counterexample  $X$ so that
$\perm(X)\not = f_C(X)$; cf. Figure~\ref{fig:trivial}.
The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$ and depth
$O(\log^a n)$. Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. (Well, only
if the underlying field of computation is finite. For infinite fields, 
such as $\Q$ or $\C$ in this paper, 
there is another notion of a trivial obstruction (cf. 
GCT6). But let us imagine that the underlying
field is finite for this argument.)
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time to decide if such a table exists and construct 
one (optional) for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. That is why we 
call  this trivial, brute force 
strategy of proving IOH, based on existence of trivial obstructions,
an {\em infeasible strategy}. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{eq}{$\perm(X)\not = f_C(X)$}
\epsfig{file=trivial.eps, scale=.5}
\end{center}
      \caption{A trivial obstruction}
      \label{fig:trivial}
\end{figure}


In contrast, assuming PH1, the problem  of verifying OH belongs 
to $NP$ as we have already observed. Thus, assuming PH1, we have 
transformed the original infeasible obstruction 
hypothesis $IOH \in \Pi_2^{\#P}$ to a new  obstruction hypothesis 
$OH \in NP$, in the process bringing down the time to verify an obstruction
from  exponential (for the original trivial obstruction) to polynomial
(for the new obstruction); cf. Figure~\ref{fig:IOHcomplexity}.  
It is crucial here that PH1, the main tool for this reduction, is a 
mathematical hypothesis,  not complexity-theoretic (cf. the remarks
after Theorem~\ref{tgct6} and Hypothesis~\ref{hph1}).
The task of verifying  an obstruction has also been 
transformed from the infeasible (exponential-time) to the feasible 
(polynomial-time). Hence the name of this strategy: the flip,
from the infeasible to the feasible.
Positivity (PH1) is used in the flip as a means  to
eliminate the quantifying variables in IOH and bring down the 
 complexity of the obstruction hypothesis;
cf. Figure~\ref{fig:IOHcomplexity}. 




This process can be extended further. Assuming an additional
positivity hypothesis PH4 specified below,
$OH \in NP$ can be transformed 
to POH (Positivity Obstruction Hypothesis) that belongs to $P$; i.e.,
which can be verified in polynomial time, and an obstruction,
if it exists, can also be constructed in polynomial time; 
cf. Figure~\ref{fig:IOHcomplexity}. (The hypothesis is called PH4 instead
of PH2, because PH2 and PH3 are some other positivity hypotheses in GCT6
that complement PH1). 
Once this final positivity hypothesis POH is proven, the obstruction
hypothesis is reduced to a tautology (FOH: Final Obstruction Hypothesis),
which can be verified in
$O(1)$ time. This  would then give us 
the final $O(1)$-size  proof. 

Thus the basic idea of the flip is to use positivity systematically
as a means to eliminate the quantifiers  and reduce the complexity 
of the  obstruction hypothesis until it is finally
reduced to  an $O(1)$-time verifiable  tautology;
cf. Figure~\ref{fig:IOHcomplexity}. 

Now let us specify PH4 and POH.
Towards that end, let  $k \le l=m^2$ be the length of $\lambda$.
Define 

\begin{equation} 
\begin{array}{l}
\bar P_{n,m}= \{ \lambda: P_{\lambda,n,m} \not = \emptyset \} \subseteq \C^k, \\
\bar Q_{n,m}= \{ \lambda: Q_{\lambda,n,m} \not = \emptyset \} \subseteq \C^k.
\end{array}
\end{equation}

\begin{theorem} 
The sets $\bar P_{n,m}$ and $\bar Q_{n,m}$ are convex polytopes in $\C^k$.
\end{theorem} 
This follows from some fundamental results in geometric invariant theory
\cite{mumford}. 

Then: 

\begin{hypo}  {\bf PH4} (GCT6)
The membership problems for these polytopes belong to 
$P$ and so also the problem of deciding if $\mbox{vol}(\bar P_{n,m}
\setminus \bar Q_{n,m})$, the volume of the relative complement 
$\bar P_{n,m} \setminus \bar Q_{n,m}$, is nonzero (positive);
i.e. if $\bar P_{n,m} \not \subseteq \bar Q_{n,m}$. By polynomial time,
we mean $\poly(n,l,\bitlength{m})$ time. This is $\poly(n)$,
if $m\le 2^{o(n)}$ and $l =\poly(n)$. 
\end{hypo}

\begin{hypo} {\bf (POH)}

For all $n\rightarrow \infty$, assuming $m=2^{\log^a n}$, $a>1$ fixed, 

\[ \mbox{vol}(\bar P_{n,m} \setminus \bar Q_{n,m}) > 0, \] 

for $k=(n+1)^2$. 
\end{hypo} 

\ignore{
Thus POH says that  the line-shaded area in Figure~\ref{fig:POH} has positive
volume for all large enough $n$. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{P}{$\bar P_{n,m}$}
\psfrag{Q}{$\bar Q_{n,m}$}
\epsfig{file=POH.eps, scale=1}
\end{center}
      \caption{POH}
      \label{fig:POH}
\end{figure}
}

\section{How to prove PH?}  \label{sphprove}
There is  a basic prototype of PH in representation theory,
which will be described in detail towards the end of Lecture 3. We shall
refer to it  as Plethysm PH. It says that the stretching functions 
akin to $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$
associated with  fundamental  multiplicities 
in representation theory called plethysm constants also have analogous 
positive convex representations. 

This  is   known for a very special case of the plethysm constant 
called the  Littlewood-Richardson (LR) coefficient
$c_{\alpha,\beta}^\lambda$. It is  defined to be 
the number of occurances of the Weyl module $V_{\lambda}(G)$ in the 
tensor product of $V_{\alpha}(G)$ and $V_\beta(G)$. 
The classical Littlewood-Richardson rule, which we shall refer to as LR PH,
implies that the stretching function 
$\tilde c_{\alpha,\beta}^\lambda (k) = c_{k \alpha, k \beta}^{k \lambda}$
associated with the Littlewood-Richardson coefficient has a
positive convex representation.

Plethysm PH   happens to be a fundamental open problem of
representation theory, older than the $P$ vs. $NP$ problem itself. It 
has been studied intensively in the last century, and is known to be
formidable. And  now,  as explained the third lecture, it also turns out to 
be  the heart of this approach towards the $P$ vs $NP$, the
$\#P$ vs. $NC$ problems.



A basic plan to prove Plethysm PH is given in GCT6.
It is partially 
implemented in GCT7 and 8. See Figure~\ref{fig:lift} for a pictorial
depiction of the plan. It strives  to extend the  proof of LR PH based 
on the theory of the  standard quantum group \cite{drinfeld,kashiwara,lusztig}.
There it
comes out as a consequence of a  (proof of a) deep positivity result
\cite{kazhdan,lusztig}, which
we shall refer to as LR PH0. It says that   the 
tensor product of two representations of the standard quantum group 
has a canonical basis \cite{kashiwara,lusztig} 
whose structure coefficients are all positive \cite{lusztig}
polynomials (i.e., polynomials with nonnegative coefficients).
The only known proof of this
result is based on the Riemann Hypothesis over finite fields 
proved in \cite{weil2},  and the related works \cite{beilinson}. 
This Riemann Hypothesis over finite fields 
is  itself a deep positivity statement in mathematics,
from which   LR PH can  thus be 
deduced, as shown on the bottom row of Figure~\ref{fig:lift}.

If one were only interested in LR PH, one  does not 
need this  powerful machinery, because it has a  much simpler 
algebraic-combinatorial  proof. 
But the plan to extend the
proof of LR PH to Plethysm PH in GCT6,7,8 is like a huge
inductive spiral. To  make it work,  one  needs a 
stronger inductive hypothesis than Plethysm PH--this is precisely  Plethysm 
PH0 (which  will be
described in the third lecture; cf. Hypothesis~\ref{hplph0}).
Thus what is needed now 
is a systematic lifting  of the bottom arrow in Figure~\ref{fig:lift}
to the top, so as to complete the  commutative diagram, so to speak. 

Initial  steps in this direction have been taken in GCT7,8. 
First, GCT7 constructs a {\em nonstandard quantum group}, which
generalizes the notion of a standard quantum group \cite{drinfeld},
 and plays the
same role in the plethysm setting that the standard quantum group plays
in the LR setting. Second, GCT8 gives an algorithm to construct 
a canonical basis for a representation of the nonstandard quantum group
that is conjecturally correct and has the property Plethysm PH0,
which is a   generalization of LR PH0  supported by experimental
evidence.
Now what is needed to complete  the 
commutative diagram in Figure~\ref{fig:lift} is an appropriate nonstandard 
extension of the Riemann hypothesis over finite fields and the related works
\cite{beilinson,weil2,kazhdan,lusztig}
from which  Plethysm PH0 can be deduced. This--the top-right corner 
of the diagram--is the   main  open problem at the heart of this approach. 

\section{How to prove OH or POH?} 
We do not  know, 
since the  proof of OH and POH 
would really depend on the explicit forms of the
polytopes that arise in   PH1/PH4, and we have no idea about them
at this point.
\ignore{GCT does suggest  that proving OH/POH  should be feasible 
``in theory''
since OH/POH  belong to NP/P, assuming PH1/4, and polynomial-time
is complexity theory stands for feasible ``in theory''. 
In other words,
GCT gives a reason to believe now that proving 
the  $P\not = NP$ conjecture should be feasible in theory. Even this
was  always questioned  in the field of complexity theory so far, because 
the $P$ vs. $NP$ problem is a universal statement regarding all of mathematics
(that says theorems cannot be proven automatically).
But, as we also know by now, 
there is a huge gap between  theory and  practice--e.g., 
just because  some problem is in $P$ does not 
necessarily mean that it is feasible in practice. Similarly,
the actual implementation of the GCT flip via positivity is expected to be 
immensely difficult ``in practice'', as Figure~\ref{fig:lift} suggests. 
}






\section{Is positivity  necessary?} \label{sposnece}
\ignore{
Though the statement of this result is elementary, its proof is nonelementary,
as expected,  since the generalized permanents are highly nontrivial
and mathematically formidable objects. Specifically, the problem
of finding a $\#P$-basis for the space of generalized permanents 
is intimately related to some formidable problems of representation
theory and algebraic geometry,
and the  simplest analogue of this problem 
which can be solved at present  \cite{}
requires the deep Riemann Hypothesis over finite fields \cite{} for its
proof; cf. Section~\ref{}.
The proof of Theorem~\ref{} proceeds at an abstract level 
through algebraic geometry and representation theory without
having to know anything about such a basis.
At present, it is open if there is any alternative 
weaker form of the $\#P \not = NC$  conjecture,
which cannot be proved by relativizable, low-degree or 
naturalizable  techniques, but which can still be proved by elementary 
or not so  nonelementary techniques; that is, whether the earlier known
barriers mentioned above can 
be simultaneously bypassed in an elementary way in the context of 
the $\#P$ vs. $NC$ (or $P$ vs. $NC$  or $P$ vs. $NP$) problem.


\section{Why are we going for explicit obstructions?}
In a sense, the proof of the weak form turns out to be nonelementary
because of the difficulty of explicit construction. Specifically, algorithm 
to construct an obstruction $O_n$ for each $n$ is very simple, but to
show that it is correct requires nontrivial algebraic geometry,
just as the construction 
of an explcit family of Ramanujan graphs in \cite{} is very simple,
but to show that it is correct requires nontrivial algebraic geometry.
We already know, e.g. from this example of Ramanujan graphs, that 
explicit constructions can require highly nonelementary techniques.
So the question now arises: why are we going for such difficult explicit
constructions? Can they not be avoided somehow? 
After all, to solve the original problem we only need to show existence
of obstructions. We do not have to construct them explicitly.

Furthermore,  explicit construction is not needed to 
cross any of the barriers mentioned above (e.g. the natural-proof-barrier).
This is because {\em any} proof technique which uses symmetries of the
permanent would automatically bypass the natural-proof barrier
in the context of the permanent vs. determinant problem,
even if it does not utter a word about explicit construction, since
most functions have no symmetries. Indeed, the weak form of 
the generalized $\#P$ vs. $NC$ problem itself has two proofs, one
purely nonconstructive and one through explicit construction--the major 
chunk of both proofs being  the same, except for the last step,
which is carried out via a counting argument in the former proof and via
explicit construction in the latter. Since the nonconstructive proof too
is based on symmetries, it also crosses the natural-proof barrier.
This provides a concrete evidence that explicit construction is not 
necessary for crossing the earlier known  barriers.

Then why are we still going for explicit construction? 
Before we go any further, we wish to briefly state  the motivation
behind  going for the flip (explicit construction),
since this is an important issue. 
}

Finally,  if the positivity problems are so hard,  one may ask if 
they can not be avoided somehow. Unfortunately, there is a formidable 
barrier towards the $P$ vs. $NP$ and related problems, called the
{\em feasibility ($P$) barrier} (GCT6,GCTflip),
which seems universal in the sense that
any approach towards these problems would have to tackle it, not just GCT. 
The flip, i.e., explicit construction of obstructions, is the most natural
and obvious way to cross this barrier, and it also seems to be 
among the easiest. The 
existing mathematical evidence suggests that any such natural approach
to cross this barrier would have to say  something deep regarding positivity
(Plethysm PH/PH0)  either explicitly or {\em implicitly}, even if
the approach does not utter a word about algebraic geometry or
representation theory.
That is,  Plethysm PH and PH0   may indeed be 
the heart of the  fundamental lower bound problems in complexity theory;
a detailed story and a precise meaning of the key 
phrase {\em implicit} would appear in the revised version of GCTflip.

%\input{feasibility}









































 

































\begin{sidewaysfigure} 
\begin{center} 
\epsfig{file=lift.eps, scale=.8}
\end{center}
      \caption{A commutative diagram}
      \label{fig:lift}
\end{sidewaysfigure} 



\ignore{\begin{figure} 
\psfragscanon
\psfrag{P}{$P\not = NP$ and $\#P\not = NC$ conjectures (characteristic zero)}
\epsfig{file=barriers.eps, scale=1}
      \caption{The feasibility barrier towards $P$ vs. $NP$}
      \label{fig:barriers}
\end{figure}}


%\input{lecture1_maintext}


==> lecture1_7.tex <==
\section*{Preface}

This article   gives a mathematical overview of 
geometric complexity theory (GCT), an
approach  towards the fundamental lower bound problems  in complexity theory, 
such as (Figure~\ref{fig:complexityclasses}):

\noindent (1) 
The $P$ vs. $NP$ problem \cite{cook,karp,levin}: 
 show that $P \not = NP$;


\noindent (2) 
The  $\#P$ vs. $NC$ problem \cite{valiant}: show that 
$\#P \not = NC$.

\noindent (3) The $P$ vs. $NC$ problem: show that $P \not = NC$.

We shall be interested 
in  the stronger  nonuniform versions of these problems.

\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes (no proper containments are known)}
      \label{fig:complexityclasses}
\end{figure} 


The basic strategy of GCT, called the
{\em flip} [GCT6,GCTflip],  is to search for  {\em explicit obstructions} $O_n$
to efficient computation 
of the (judiciously chosen) hard function $f(X)=f(x_1,\ldots,x_n)$
under consideration (cf. Section~\ref{smeaning} for the reasons behind 
the terminology flip).  Here each $O_n$ is  meant to be some  
(algebro-geometric-representation-theoretic) object
whose existence serves as
a guarantee that $f(X)$ cannot be computed efficiently; in the 
context of the $P$ vs. $NP$ problem this means by a circuit of
size $m=\poly(n)$. In other words,
obstruction is a proof-certificate of hardness. 
We say that an obstruction family is {\em explicit}, if it contains
obstructions that are  {\em short} and {\em easy-to-verify}.
Here short  means: for given $n$ and $m\le 2^n$, if there 
exists such an obstruction to computation of $f(X)$ by circuits of size $m$,
then  there exists a short one whose 
specification has $\poly(n)$  bitlength (the bound does not depend on $m$), 
and furthermore, a short obstruction exists if $m=\poly(n)$, or more generally,
 $m=2^{\log ^a n}$
(say), for some fixed $a>0$. Easy to verify means:
for any $n$ and $m \le 2^n$, whether a given object 
is a valid obstruction for this $n$ and $m$ can be verified 
in time polynomial in $n$ and the bitlength of the specification of the object
(again the bound does not depend on $m$). In
particular, this is $\poly(n)$ if the bitlength of the specification
of the object  is $\poly(n)$.
We say that the family is strongly explicit if, in addition, obstructions are
{\em easy to discover}.  This means, for given $n$ and $m$, whether 
there exists such an obstruction can be decided in $\poly(n)$ time, 
and if so, the specification of one can also be constructed in
this much time.  Finally, we say that the obstruction 
family is {\em extremely explicit}
if, in addition, there is a polynomial time {\em decoding algorithm}, 
which, given a specification of an obstruction $O_n$ and a small circuit $C$,
produces  a counter-example $X$
such that the value $f_C(X)$ of $C$ on $X$ is different from $f(X)$.
Thus we can think of an extremely explicit obstruction as a short 
and easily verifiable encoding of a {\em trivial obstruction}, 
 by which we mean the 
exponential size table that lists for every small circuit the 
counter example produced by the decoding algorithm.
It may be conjectured that there exist extremely 
explicit families of obstructions for the $P$ vs. $NP$ problem
(for any $NP$-complete $f(X)$) with 
exponentially  many such small obstructions for every $n$. Indeed, it 
may be conjectured that the obstructions that GCT goes for are extremely
explicit; i.e., there exists such a polynomial time 
decoding algorithm. We do not
need extreme explicitness, at least not at this stage. That is, it
is enough for us if the existence of an obstruction implies that there exists
some  trivial obstruction, even if we cannot get one such easily.
But  intuitively
it may help to imagine (as conjectured) 
that the obstructions we are going for in GCT are extremely explicit,
i.e., some such polynomial time decoding algorithm exists.



The basic idea of the flip is to first come up with 
a theoretically ``easy'' (feasible) 
algorithm for the discovery of an obstruction for given $n$ and $m$
(if one exists),
and then show that for each large enough $n$,
if $m=\poly(n)$, this ``easy'' algorithm 
terminates successfully with discovery. We shall
refer to this as the discovery-program-correctness step. 
Of course, for the strategy to be feasible practically, and not just 
theoretically, it is 
also necessary that this discovery algorithm should  have 
a simple enough structure that  can be used to prove this program 
correctness. If not, it has to be made simpler and simpler until this
becomes practically feasible.

The flip in the context of  other problems is analogous.


The flip is the defining strategy of GCT. Indeed, GCT may be abstractly
defined as any (geometric) approach to the $P$ vs. $NP$ and related 
problems based on the flip, i.e., explicit construction of obstructions
(for a precise meaning of the phrase geometric see Section~\ref{scharsym}).
The present (concrete) GCT is one such  approach. 
We focus here on characteristic zero. That is we only consider computations
performed by algebraic circuits, where each gate can perform an algebraic
operation of the underlying ring or field   of characteristic zero, 
say $Z$, $\Q$ or $\C$ \footnote{The characteristic zero version
of the $P$ vs. $NC$ obtained this way 
is not very interesting. The more nontrivial 
version solved in GCTweak will be considered below.}. This is because
the nonuniform lower bounds over $Z$ are weaker implications of the
corresponding ones over a finite field (the usual case), and hence
easier. The additional problems that
need to be addressed when the underlying field of computation is finite
will be discussed in  GCT11. 

But first we need to explain why we are going 
for explicit construction
of obstructions, since to solve the original problems we only need to
demonstrate their existence, which, in principle, could be
done  nonconstructively. Hence, 
in this preface we briefly explain the motivation behind the flip by
reviewing   two concrete lower bounds 
of GCT based on the (weaker form of) this paradigm,
namely, {\em the weak form of the $P \not = NC$ conjecture} [GCTweak],
and {\em the generalized weak form of the $\#P\not = NC$ conjecture} [GCT6]
(which is a much more nontrivial generalization of the weak form
in the original IAS lecture).
After this, we  briefly explain how the 
the conjectural scheme  for  implementing the flip in
characteristic zero [GCT6,7,8]  is supported by these concrete lower bounds.



We  begin with 
the  special case of the $P \not = NC$ conjecture [GCTweak],
which we are calling
its {\em weak form}, and which can be considered to be the
first concrete lower bound result of GCT. It  says that 
the $P$-complete max-flow problem
cannot be solved in $\polylog(N)$ parallel time using $\poly(N)$
processors in the PRAM model without bit operations,
where $N$ denotes
the total bit length of the input, not just the number of input parameters.
This model  is quite realistic and natural
since it includes virtually all known parallel algorithms for algebraic 
and weighted optimization problems.
The proof technique of this result can be considered to be {\em locally
explicit}, i.e.,  a weaker form
of the flip,  in the sense that  for each branching program $C$  (i.e. 
a circuit with arithmetic, branching and comparison operations) 
of depth $\log^a N$ and size $\poly(N)$ (or even 
$2^{\log^a N}$, for some positive constant $a$),
it produces in $\log ^b N$ time using $2^{\log ^b N}$ 
processors, $b=O(a)$, 
an explicit   counter example  $X$ such that the output of $C$
on $X$ is different from what is expected in the maxflow (decision) problem.
This counter example $X$ is then a proof-certificate of hardness (obstruction)
against $C$.
We are calling this kind of explicitness local 
because the obstruction   here is
a short and easily-verifiable  proof 
certificate of hardness against a specific circuit   rather than 
a short and easily-verifiable {\em global obstruction} 
against  the
whole class of circuits of small depth and size, which is far harder to
achieve, and which was what the full flip eventually goes far
in the context of the harder lower bound problems.

Local explicitness here  may seem counterintuitve at the surface,
since max-flow is $P$-complete, and hence, it may seem that we may not
even be able to verify if a given $X$ is a counter-example in 
polylogarithmic parallel time. But this is still possible,
because  the proof technique in
GCTweak produces for a given $C$ an explicit 
counter example $X$ for which 
max-flow can be computed in polylogarithmic time
nevertheless.


\noindent Remark:
Local explicitness was not  specifically mentioned 
in GCTweak. But it is easy to see \cite{GCTpramappend}  that 
the proof technique there actually
produces a locally
explicit proof certificate of hardness, though the goal was only
to prove its existence (which is why explicitness was not mentioned).
In other words, the proof technique produces a locally
explicit proof-certificate of hardness  whether one cares for it or not.


Local explicitness of the proof technique is the fundamental difference between
this lower bound result and the earlier ones, such as 
the lower bounds for constant depth circuits \cite{sipser}, monotone circuits 
\cite{monotone}, or 
algebraic decision trees \cite{benor}, whose proof techniques are inherently 
nonconstructive. For example, the random restriction method \cite{sipser}
for proving lower bounds for  constant depth circuits gives a randomized 
fast parallel algorithm to produce  for each such
circuit $C$ a local counter example $X$ on which it differs from
the parity function. But the best determistic algorithm to produce 
such a counter example, based on  derandomization of the switching
lemma \cite{agarwal},
takes sequential polynomial time. Locally explicit in this
setting would mean computable by a constant depth circuit. Again, at the
surface this may seem counterintuitive, since it may appear that 
even to verify if a given $X$ is a counter example against a given
$C$ may necessarily
require $NC$-computation, given that parity is not in $AC^0$. 
But this should still be possible in view 
of the weak form of the $P\not = NC$ conjecture above. 
Similarly, the proof of the lower bound for sorting in
the  algebraic-decision-tree 
model \cite{benor}  inherently requires
exponential time  to produce a counter example, 
so also the proof of the lower bound for monotone circuits \cite{monotone}.
It may be conjectured that there are
(locally) explicit proofs 
for the constant-depth or  monotone circuit lower bounds. 
At present this is  open. But the main point is that such  explicit 
proofs are not  required to prove these lower bounds,
whereas,
the only way we can prove the weak form of the $P \not = NC$ conjecture
at present is via locally explicit construction. 

As per the natural-proof barrier \cite{rudich},
the nonconstructive proof techniques of 
the kind used to prove constant-depth-circuit lower bounds
would not work in the context of the $P$ vs. $NP$ problem.
Hence it should not be 
surprising that the proof of the weak form of the $P\not = NC$ 
conjecture should require something fundamentally different, since the
$P \not = NC$ conjecture is generally
regarded as a smaller version of the $P \not = NP$ conjecture.
Though, admitedly,  the natural proof barrier itself does not suggest that 
we should go for anything explicit (cf. Section~\ref{sobsweak}).

Another  feature of the proof of the weak form is that  it
is based on classical algebraic geometry, though 
the lower bound result itself can be stated in purely 
elementary and combinatorial terms.  No elementary or combinatorial 
proof of this result is known so far.
At present, this weak form of the $P\not = NC$ conjecture seems to be the
only known  special case of any
of the fundamental separation  problems in 
Figure~\ref{fig:complexityclasses} that  holds unconditionally (and 
superpolynomially) in a realistic and 
natural model of computation. That its only known proof needs 
geometry and explicit construction   provides  the first
concrete  support for the
geometric approach based on  explicit construction (GCT), 
albeit only in the weak setting, and
hence, in retrospect, we shall refer to its proof technique as {\em weak GCT}.

But the weak  GCT turns out to be too weak for going ahead 
for two reasons.
First, GCTweak (towards the end of its Chapter 7) 
pointed out a barrier (other than the earlier natural-proof
and relativization barriers), which we shall 
refer to  as the {\em algebraic degree barrier}, though it was not
given any name there. This  says that 
any low-degree proof technique, such as the one there,
which associates with a computation algebraic 
objects (polynomials, varieties, etc.) 
and then reasons solely on the basis of the degrees of those 
objects would not work in the context of the fundamental problems 
such as the $P$ vs. $NC$ problem.
The recent  algebrization barrier \cite{aaronson}
also says  something similar, but with different  motivation and framework.
Second, as we already pointed out before, the obstructions in weak GCT are 
short and easily-verifiable 
locally as against globally, which is what seems to be needed in 
the much harder lower bound problems in Figure~\ref{fig:complexityclasses}.

GCTweak also suggested an idea  for bypassing the
algebraic degree barrier: namely, associate with complexity classes 
algebraic varieties with group action, as studied in geometric invariant theory
\cite{mumford}, which   intuitively 
capture the symmetries among the  computations in  that class,
and then reason on the basis of
the deeper representation theoretic structure of these
varieties, instead of just  their degrees.

This then was the motivation behind the 
approach to the fundamental lower bound problems via geometric 
invariant theory that was initiated in GCT1 and 2. 
The focus here is on the 
characteristic zero versions of the other 
two problems in Figure~\ref{fig:complexityclasses}, namely
the $P$ vs. $NP$ and $\#P$ vs. $NC$ problems (weak GCT is too weak in
this context too). 
The nonuniform (characteristic zero) version of the $\#P$ vs. $NC$ problem
is also known as the permanent vs. determinant problem \cite{valiant}. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented 
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$. %; the best known lower bound on $m$ at present is 
%quadratic \cite{ressayre}.
By linear representation, we mean
the  entries   of $Y$ are  (possibly nonhomogeneous) 
linear functions 
of the entries of $X$. 
There is an analogous characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.
The main results of GCT for the $\#P$ vs. $NC$ problem in 
characteristic zero also extend to the $P$ vs. $NP$ problem in characteristic
zero. But for the sake of completeness,   we shall mainly
concentrate in this article 
on only the former problem, since it illustrates all the
basic ideas.


In GCT1, and 2  certain algebraic varieties with group action, 
called the {\em class varieties}, are associated with the fundamental 
complexity classes, and the $\#P$ vs. $NC$ and $P$ vs. $NP$ problems in
characteristic zero are reduced to showing existence of 
certain representation-theoretic {\em obstructions} to embeddings
amongs such varieties. Furthermore, some results in geometric invariant
theory are also proved to justify why such obstructions should exist and
why they should be mathematically well behaved.



Using these
results and the notion of an obstruction
in GCT1 and 2, GCT6 then proves a second concrete 
lower bound result of GCT, namely the {\em generalized 
weak form of the $\#P$ vs. $NC$ problem} in characteristic zero.
%(which is much more nontrivial than the weak form in the original
%IAS lecture.)  
A special case of this result
says that any generalized permanent of an 
$n\times n$ variable matrix $X$ cannot be 
represented as a polynomial in the traces of $\bar X^j$, $j\ge 0$, where 
 $\bar X= B X C$, for any (possibly singular) $n\times n$
complex 
matrices $B$ and $C$. Here by a generalized permanent, we mean a function
$p(X)$ 
which has exactly the same symmetries as that of the permanent: i.e.,
for all nonsingular $n\times n$ complex matrices
$U$ and $V$, $p(U X V)=p(X)$
iff $\perm(U X V)=\perm(X)$. The proof technique of this result 
produces a strongly explicit family $\{O_n\}$ of (global) obstructions, 
where each $O_n$ has a specification of $O(n)$ size that can verified
and constructed in $O(n)$ time. It also  bypasses 
the natural-proof, relativization
and algebraic degree (algebrization) barriers (or rather their analogues)
simultaneously 
in this setting.



The main result of GCT is a conjectural scheme [GCT6,7,8] 
for explicit construction 
of obstructions (i.e. for the implementation of the flip) 
for the general $\#P$ vs. $NC$ and $P$ vs. $NP$ 
problems in characteristic zero. 
At the heart of this scheme lies a certain positivity hypothesis called PH1,
which   says that 
certain  representation-theoretic counting  functions
associated with the class  varieties in GCT1 and 2 
have positive  convex formulae,
by which we mean  positive convex
representations as the number of integer points in  explicitly 
specified polytopes, like the one for the permanent of a $0-1$-matrix 
as the number of integer points in the perfect matching polytope, which
is both positive (since each integer point is counted 
with a positive sign) and convex. 
Furthermore, GCT6,7,and 8   provide an evidence in support of validity
of PH1, and suggest  an approach for proving it via the theory of
nonstandard quantum groups, which are generalizations of
standard quantum groups \cite{drinfeld}. At the heart of this approach,
in turn,  lie certain conjectural positivity hypotheses [GCT8] in the theory
of these nonstandard quantum groups, which are  generalizations of the
known positivity results \cite{kazhdan,lusztig} for the standard quantum group.
The only known proofs of these positivity results relie on the 
Riemann hypothesis over finite fields \cite{weil2}, which is
itself a profound  positivity result in mathematics. 
Thus the proposed scheme for explicit construction of obstructions 
in GCT6,7,8  seems to need  as yet unknown nonstandard
extension of the work surrounding this central positivity theorem,
which encompasses several areas of mathematics, such as algebraic geometry,
representation theory, quantum groups and so forth.

This should not be too surprising, given that 
the difficulty of explicit construction is by now well recognized 
in complexiy theory.
For example, the explicit construction of Ramanujan graphs \cite{sarnak},
which are the best (optimal) expanders,  also 
needs the Riemann hypothesis over finite fields (for curves).
But explicit expanders  cannot be used to prove a lower bound result.
Explicit constructions that yield hard lower bound results are bound
to be  more difficult. Hence, if a nontrivial  extension 
of the work surrounding the Riemann Hypothesis over finite fields 
is needed for explicit constructions in GCT, that is only to be expected.


If explicit construction is thus the root cause of all difficulties in
GCT, one may finally ask: can they not be avoided somehow?
After all, for the original lower bound problems we only need to 
prove existence of some obstructions. Furthermore, as pointed out
in Section~\ref{sobsweak}, explicit constructions are also not needed 
to cross the natural-proof, relativization,
algebraic-degree or algebrization barriers. Why are then we going for
explicit constructions? 

Because of the {\em feasibility barrier} (to be described in the
revised version of [GCTflip]), which is encountered after 
bypassing the  barriers mentioned above, and which 
seems to be the main barrier towards the $P$ vs. $NP$ and related problems.
Explicit constructions seems to be the easiest way to cross this barrier,
for mysterious reasons that we do not understand, though there 
there may be nonconstructive ways to cross  it as well. 
In GCT, this barrier takes  the form of  the $P$ barrier
[GCTflip] mentioned briefly towards the end of the second lecture.
We do not discuss the feasiblity
barrier in these lectures, since the goal here is to
stick to  concrete mathematics, without getting into such philosophical
issues. At the concrete level, all one can say  is that GCT goes 
for explicit constructions for the lack of any better alternative. 
After all, any approach to the $P$ vs. $NP$ and related problems has 
to yield at least:
\begin{enumerate} 
\item[A] Some weak form of any of the separation problems in
Figure~\ref{fig:complexityclasses}
that  gives
a concrete superpolynomial lower bound
in a realistic and natural model of computation, by which
we mean a model that is actually used in practice and is
not defined for the sake of the lower bound, and
\item[B] Some  weak form  whose 
proof technique bypasses 
the relativization, natural proof,  algebraic degree, and 
algebrization barriers simultaneously, and which makes nontrivial use 
of the symmetries in the underlying problem (in the $\#P$ vs. $NC$ problem
this refers to the symmetries of the permanent). 
\end{enumerate}
The weak form of the $P\not = NC$ conjecture in GCT meets criterion (A),
and the generalized weak form of
the $\#P \not = NC$ conjecture meets criterion (B). 
These are the weak forms specific only to  this concrete form
of GCT. Other  approaches (GCT or nonGCT) may lead to other
comparable weak forms which are more suitable to them.
But, at present, these are the only such lower bounds that 
we can prove unconditionally in the context of the $P$ vs. $NP$, $P$ vs. $NC$
or $\#P$ vs. $NC$ problems.
And the only way we can prove them is via explicit constructions based on
geometry.  The situation is summarized in Figure~\ref{fig:summary}.
Here it can be
seen that as the circuit lower bounds start moving in the 
direction of the $P$ vs. $NP$ problem, the proof techniques, for some
mysterious reasons, become more and more geometric and explicit.
This sugests that there may be after all something inevitable 
about a geometric approach based  explicit constructions, 
which is what GCT means.

\begin{figure} 
\begin{center}
\psfragscanon
\psfrag{pvsnc}{$P\not = NC$}
\psfrag{#pvsnc}{$\#P\not = NC$}
\psfrag{pvsnp}{$P\not = NP$}
\epsfig{file=summary.eps, scale=1}
\end{center}
      \caption{Circuit lower bounds vs. proof techniques}
      \label{fig:summary}
\end{figure} 



The rest of this article is organized in the form of three chapters,
one per  lecture. The first gives a short overview of the basic plan
of GCT for implementing the flip (explicit constructions),
which is elaborated in the next two lectures. 






\noindent {\em Acknowledgement:} The author is grateful to 
Avi Wigderson for arranging the lectures and the hospitality in IAS.


\chapter{Basic plan} 
We now outline the basic  plan of GCT focussing on
the  permanent vs. determinant problem in characteristic zero. Recall that
this  says  $\perm(X)$  cannot be represented 
linearly  as the determinant of a polynomial size 
matrix.

%\input{weak}
\input{lecture1_maintext}


==> lecture1_8.tex <==
\section*{Introduction}

This article   gives a mathematical  overview of
geometric complexity theory (GCT), an
approach  towards the fundamental lower bound problems  in complexity theory, 
such as (Figure~\ref{fig:complexityclasses}):

\noindent (1) 
The $P$ vs. $NP$ problem \cite{cook,karp,levin}: 
 show that $P \not = NP$;


\noindent (2) 
The  $\#P$ vs. $NC$ problem \cite{valiant}: show that 
$\#P \not = NC$.

\noindent (3) The $P$ vs. $NC$ problem: show that $P \not = NC$.



We  focus here on only the nonuniform versions of the above problems 
in characteristic zero; i.e., when
the underlying field of computation is of characteristic zero, 
say $\Q$ or $\C$.  The additional problems that
need to be addressed when the underlying field of computation is finite
would be discussed in  GCT11. 


The nonuniform
characteristic zero version of the $P\not = NC$ conjecture (in fact,
something stronger) was already proved  in GCTlocal. We shall refer
to it as the $P\not = NC$ result without bit operations.
It says that the max flow problem cannot be solved in the 
PRAM model without bit operations in $\polylog(N)$ time using 
$\poly(N)$ processors where $N$ is the bitlength of the input.
This  may be considered to be the first unconditional lower bound result of
GCT, because, though it can be stated in purely elementary combinatorial
terms, being a formal implication of the $P\not = NC$ conjecture, its
proof is intrinsically geometric, and no elementary proof is known so far. 
Furthermore, its proof  technique may be considered to be a weaker (local)
form of the {\em flip}, the basic guiding strategy of GCT, which  was 
refined and formalized much later in GCTflip. 
This  was the begining of  this  geometric approach in complexity theory.
The later work in GCT-- the subject of this overview--focusses on the other 
two problems above, namely
the $P$ vs. $NP$ and $\#P$ vs. $NC$ problems. 


The nonuniform (characteristic zero) version of the $\#P$ vs. $NC$ problem
is also known as the permanent vs. determinant problem \cite{valiant}. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented %(cf. Figure~\ref{fig:matrices})
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$. %; the best known lower bound on $m$ at present is 
% quadratic \cite{ressayre}.
By linear representation, we mean
the  entries   of $Y$ are  (possibly nonhomogeneous) 
linear functions of the entries of $X$. 
There is an analogous characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.
The main results of GCT for the $\#P$ vs. $NC$ problem in 
characteristic zero also extend to the $P$ vs. $NP$ problem in characteristic
zero. But here we shall 
concentrate  on only the former problem,
since this illustrates all the basic ideas. 



The original  lectures   stated a lower bound called 
a weak form of the $\#P$ vs. $NC$ problem. It  turned out 
to be too weak because it has an elementary proof \cite{} that does
not cross the natural proof barrier \cite{rudich}. 
This weak form  is actually a special case of a far more general   result,
called  a {\em mathematical form of the $\#P\not = NC$ conjecture} [GCT6],
which was not stated in the original lectures, but is stated here
(Section~\ref{}).  It is the second unconditional lower bound result 
of GCT. 
We cannot prove this result  by such elementary naturalizable 
techniques for the reasons explained in Section~\ref{}. 


The complementary article \cite{gctexplicit} gives a complexity-theoretic
overview of GCT. It describes   the main complexity theoretic
barrier towards these problems 
called the {\em feasibility barrier} and the basic 
strategy of GCT for crossing it called the flip: which is to go 
for {\em explicit proofs}. By an explicit proof 
we mean a proof that provides proof certificates of hardness  for the 
hard function under consideration that are short (of polynomial size) 
and easy to verify (in polynomial time). This barrier turns out to be
extremely formidable and is the root cause of all difficulties 
in these problems. Nonnelementary techniques are brought into GCT precisely
to cross this barrier. This barrier is not discussed in these lectures. 
The goal here is to describe the basic ideas of GCT at a concrete mathematical
level without getting into such meta issues. The readers who wish
to know the root cause of all difficulties encountered in GCT and
the need for the nonelementary techniques in GCT before getting
into any mathematics   may wish to read that
article before this one. On the other hand, the readers who would rather avoid 
meta issues before getting a concrete mathematical
picture  may wish to read this article first. We will leave the
exact choice to the readers.





The rest of this article is organized in the form of three chapters,
one per  lecture. The first gives a short mathematical 
overview of the basic plan of GCT,  
which is elaborated in the next two lectures. 


\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes}
      \label{fig:complexityclasses}
\end{figure} 




\noindent {\em Acknowledgement:} The author is grateful to 
Avi Wigderson for arranging the lectures and the hospitality.




\chapter{Basic plan} 
We now outline the basic  plan of GCT focussing on
the  permanent vs. determinant problem in characteristic zero. 

\section{Characterization by symmetries} \label{scharsym}
We begin by observing that 
the permanent and the determinant are 
{\em exceptional} polynomial functions. By exceptional we mean
that they are  completely characterized by the symmetries in the 
following sense.


Let  $Y$ be a variable $m\times m$ matrix.
Let $\sym^m(Y)$ be the space of homogeneous forms of degree $m$ 
in the $m^2$ variable entries of $Y$. Then, by the  classical
representation theory,  $\det(Y)$ is the only form in $\sym^m(Y)$ 
such that, for any $A,B \in GL_m(\C)$ with $\det(A)\det(B)=1$, 

\noindent  {\bf (D):} $\det(Y)=\det(A Y^* B)$,

where $Y^*=Y$ or $Y^t$. 
Thus $\det(Y)$ is completely characterized 
by its symmetries, and hence, is  exceptional. We shall refer 
to this characteristic property of the determinant as property (D)
henceforth.

Similarly, $\perm(X)$ is the only form 
in the space of forms of degree $n$ in the entries of $X$ such that, 
for any diagonal or permutation matrices $A,B$, 

\noindent  {\bf (P):} $\perm(X)=\perm(AX^*B)$, 

where $X^*=X$ or $X^t$ and the product of the (nonzero) 
diagonal entries of $A$ and $B$ is one.
Thus $\perm(X)$ is also
completely characterized   by its symmetries, and hence, is
exceptional.
We shall refer 
to this characteristic property of the permanent as property P
henceforth.





Any proof technique for the permanent vs. the determinant problem
has to ultimately make a nontrivial use of these  symmetries
  which characterize them. Indeed, one can say that 
these characteristic  properties 
lie at the heart of the permanent vs. determinant problem, and until
a proof technique has made a nontrivial use of them, it has
not entered the heart of the problem.
The most obvious interpretation of the phrase 
nontrivial here is the following: 

\begin{defn} \label{dnontrivial}
We say that a proof technique for the permanent vs. determinant 
problem makes a {\em nontrivial use of symmetries} if it does not work
for any functions (in place of the permanent or the determinant)
which do not have
nontrivial symmetries.
\end{defn}

Since symmetries is a fundamental geometric concept, we define
a  {\em geometric} approach to the permanent vs. determinant problem as
any  approach based on nontrivial use of the symmetry properties
(P) and (D) in this sense.
The meanining of the phrase geometric in the 
$P$ vs. $NP$ problem is
similar, since the  permanent and the determinant
can be replaced with   (co)-NP
and $P$ complete functions which are similarly
characterized by symmetries [GCT1]
(in a weaker sense that is good enough for our purposes).

GCT is a geometric approach in this sense.
Representation theory and 
algebraic geometry enter inevitably into  it, because
to understand symmetries, representation theory (of groups of symmetries)
becomes indispensible, and to understand  deeper properties 
of representations,  algebraic geometry becomes indispensible. 


\section{A mathematical form of the  $\#P \not = NC$ conjecture} 
\label{sweaklec1}
Before going any further, we now state one concrete application of 
GCT in the form of a concrete lower bound result--namely a 
mathematical form of the 
$\#P \not = NC$ conjecture (Theorem~\ref{tgenweaklec1} below).

We begin by observing that 
the permanent vs. determinant conjecture clearly implies  that 
$\perm(X)$ of any $n \times n$ variable matrix $X$ can not be represented 
as an $NC$-computable polynomial in the traces of $\bar X^j$, $j \ge 0$,
$\bar X=B X C$
for any (possibly singular) $n\times n$ matrices $B$ and $C$, since
$X^j$ can be computed fast in parallel. This can be proved unconditionally.
In fact, something stronger.

\begin{prop}  \label{pweaklec1}
There do not exist (possibly singular) $n\times n$ complex
matrices $B$ and $C$  and a polynomial 
$e(w_0,\ldots, w_n)$ such that $\perm(X) = g(BXC)$, 
where $g(X)=e(\trace(X^0), \trace(X), \ldots, \trace(X^n))$. 
\end{prop}
This was referred to as 
the weak form of the $\#P$ vs. $NC$ problem in the original IAS lecture. 
The article \cite{boris} showed that this is too  weak 
by giving an  elementary
proof \cite{boris} for it that is naturalizable, i.e.,
which cannot cross the
natural proof barrier \cite{rudich} because it works for most functions in
place of the permanent. The proof technique of
the quadratic lower bound \cite{ressayre}
for the permanent is also naturalizable.

We now state a much more general lower bound, which
was not stated in the IAS lecture, and which does not have such 
a naturalizable proof. For that we need a definition.

\begin{defn} \label{dgenperm}
A polynomial function $p(X_1,\ldots,X_k)$ (of any degree)
in the entries of $k$ $n\times n$ variable matrices 
is called a  {\em generalized permanent} if it has exactly 
the same symmetries as that of the permanent; i.e.,
for all nonsingular $n\times n$ matrices $U_i$ and $_V$, $i \le k$, 
\[ p(U_1 X_1 V_1,\ldots, U_k X_k V_k)=p(X_1,\ldots,X_k) 
\mbox{\ iff\ } \perm(U_i X V_i)=\perm (X) \mbox{\quad for all $i$}.\] 
\end{defn}

A precise description of the symmetries of the permanent  is given
by the property (P). Hence, $U_i$ and $V_i$ above have to be permutation
or diagonal matrices (with product of the nonzero  diagonal entries being
one), or 
product of such matrices.
When $k=1$ and $n$ is arbitrary,
there is just one generalized permanent of degree $n$, namely
the usual permanent itself. 
At the other extreme, 
when $n=1$ and $k$ is arbitrary, every function in $k$ variables 
is a generalized permanent. 
For general  $n$ and $k$, almost any polynomial 
in $\perm(X_i)$'s, $i \le k$, is  a generalized permanent, but 
there are many others besides these.
For general degrees, 
the dimension of the 
space spanned by  generalized permanents can be  exponential
in $n$; cf. Section~\ref{sweak}. 
In general,  the space of generalized permanents has a highly nontrivial
structure that  is intimately linked  to some
fundamental problems of representation theory;
cf. Section~\ref{sweak} and  [GCT6].


The original nonuniform 
$\#P$ vs. $NC$  conjecture
implies the following. 

\noindent {\bf Implication of the nonuniform $\#P \not = NC$ conjecture:}

Any $\#P$-complete generalized permanent  $p(X_1,\ldots,X_k)$ of $\poly(n,k)$ 
degree cannot be expressed as an $NC$-computable polynomial function of the 
traces of  $\bar X_i^j$, $1 \le i \le k$, $j=\poly(n,k)$, where 
$\bar X_i=B_i X_i C_i$,  $i \le k$,  for any $n\times n$ complex (possibly
singular) matrices $B_i$ and $C_i$.

(Here $X_i^j$ are  clearly $NC$-computable).

When $n=1$ and $k$ is arbitrary, this is  equivalent 
to the original nonuniform $\#P \not = NC$ conjecture,
since then any polynomial in $x_1,\ldots, x_k$ is a generalized permanent,
and a polynomial function of  the traces of  $x_i$'s means any
polynomial in $x_1,\ldots,x_k$. This cannot be proved at present.
But the next case,  $n>1$ and $k$ arbitrary, can be:

\begin{theorem}[GCT6]

\noindent {\bf (A mathematical form of the  $\#P \not = NC$ conjecture)}
 \label{tgenweaklec1}

The implication above holds unconditionally for any $n>1$ and arbitrary $k$.

In fact, something stronger then holds. Namely, 
when  $n>1$ and $k$ is arbitrary, no generalized permanent $p(X_1,\ldots,X_k)$
can be expressed as a polynomial function of the traces of 
$\bar X_i^j$, $1 \le i \le k$, $j \ge 0$,  where 
$\bar X_i=B_i X_i C_i$,  $i \le k$,  for any $n\times n$ complex (possibly
singular) matrices $B_i$ and $C_i$.
\end{theorem}

When  $k=1$ and $p(X)$, $X=X_1$, is the usual permanent, this specializes to
Proposition~\ref{pweaklec1}.


We are calling this a mathematical form for two reasons. 
First, it needs  no restriction on the computational complexity of
$p(X_1,\ldots,X_k)$ or the polynomial in the traces.
Thus it is rather in the spirit of the classical result of Galois theory 
which says that a general polynomial of degree $>5$ 
cannot be solved by any number of
radical operations, without any restriction on the number of such
operations. 
Second, observe that 
the permanent has two characteristic properties: 1) the property 
P (mathematical), and 2) $\#P$-completeness (complexity-theoretic). 
The usual complexity theoretic form of the $\#P\not = NC$ conjecture
is a lower bound for  all polynomial functions with 
the  $\#P$-completenes property, whereas the mathematical form 
is  a lower bound for all polynomial functions with the 
property (P).  In other words,  the complexity theoretic form
is associated with the $\#P$-completeness property of the
permanent and the mathematical form with 
the property (P). 




The result indicates that there is thus a chasm
between the two adjacent cases: $n=1$, $k$ arbitrary (the usual nonuniform
complexity theoretic $\#P \not = NC$ conjecture), and 
$n=2$, $k$ arbitrary (its mathematical form above). 
The complexity theoretic form is   much harder than the mathematical
form, and  a proof technique for the easier mathematical form
can be expected to give us a crucial insight into what is needed to prove 
the harder  complexity theoretic form.


For some specific
generalized permanents (cf. Section~\ref{sweak}), this result again has
an elementary naturalizable proof as in \cite{boris}.
It also has an elementary naturalizable proof for a generic 
generalized permanent, just as the fact that a generic polynomial is
hard to compute has an elementary naturalizable proof.
The nontrivial part of this 
result (which needs nonelementary proof) 
is that it holds for any generalized permanent.
Indeed the basic difference between the complexity theoretic 
and the mathematical  settings is
the following. The complexity theoretic  (i.e. the usual) $\#P \not = NC$
conjecture 
is complete in the sense 
that if it is proved for one $\#P$-complete function (say
the permanent), it automatically 
holds for all $\#P$-completeness functions (because
of the theory of $\#P$-completeness). But there is no such completeness
theory at the mathematical level. Hence, a mathematical
lower bound  for a specific 
generalized permanent, e.g., the permanent,
does not say anything about all (even $\#P$-complete)
generalized permanents. To get 
 similar completeness,   the  mathematical
form of the $\#P\not = NC$ conjecture above  covers up this lack of 
completeness theory
at the mathematical level by proving a result for all polynomial functions
with property (P), not just a specific one. 
The articles \cite{boris,ressayre} suggest that without such completeness
a restricted weaker form of the $\#P\not =NC$ conjecture
may be  provable by  a naturalizable proof technique. 



In contrast, it may be conjectured that Theorem~\ref{tgenweaklec1} cannot 
be proved by a naturalizable technique. This is because 
the only thing that is common among  all generalized permanents is the
property (P).  Hence any proof of this result would be 
essentially  forced
to rely only on  this property like  its GCT proof (cf. Section~\ref{sweak}).
Any such proof automatically passes the natural proof 
barrier since it is easy to show that most functions do not
have property $P$ when $n>1$ and $k$ is arbitrary.
\ignore{It may be remarked that the algebraic degree barrier is not 
applicable in the permanent vs. determinant problem because both
permanent and determinant have the same degree. It is not applicable
in the context of Theorem~\ref{tgenweaklec1} as well for the same reasons.
Similarly, the relativization barrier is not applicable in the context
of the permanent vs. determinant problem because the $NC$-computation 
has been algebrized in it in the form of the determinant, and the
relativization barrier does not apply to such algebraic techniques 
(just as it does not apply to the proof of the 
$IP=PSPACE$ result).
The relativization barrier does not apply in the context of 
Theorem~\ref{tgenweaklec1} 
for the same reason. Thus it can be said that the proof technique of
Theorem~\ref{tgenweaklec1} crosses the
natural proof, algebraic degree (algebrization)
and relativization barriers simultanesouly.

Ultimately, any approach to the $\#P \not = NC$ conjecture
is expected to prove some restricted
form of this conjecture, not necessarily Theorem~\ref{tgenweaklec1},
whose proof crosses these barriers simultaneously.
At present, we do not have any other lower bound  result of this kind.}



Though the statement of Theorem~\ref{tgenweaklec1} is elementary, its proof 
is nonelementary and is based on  some fundamental results 
in geometric invariant theory \cite{mumford} and the results in GCT1 and 2 
based on these results. These nonelementary techniques
are needed to cope up with a highly nontrivial 
structure of the space of generalized permanents as 
explained in Section~\ref{sweak}. 




\section{From nonexistence to existence}
The rest of this lecture  outlines  the GCT approach to 
the general  permanent vs. determinant problem,
and then  points out 
the crucial steps in this plan which can be completely executed
for the   mathematical form  of the $\#P\not = NC$ conjecture above,
but which are conjectural at present for 
the general (i.e. complexity theoretic) permanent vs. determinant problem. 

The first  step 
(GCT1,2) is to reduce this nonexistence problem--i.e., that there is no
small linear representation  of the permanent as a determinant--to
an existence problem--specifically, to the problem of proving 
existence of a family $\{O_n\}$ of obstructions; 
cf. Figure~\ref{fig:firststep}.
Here an {\em obstruction} $O_n$ is a proof-certificate of
hardness of $\perm(X)$, $X$ an $n\times n$ variable matrix,
just as the Kuratowski minor is a proof-certificate of the nonplanarity of a 
graph.  Specifically,  it is some 
algebro-geometric-representation-theoretic gadget
whose existence for every $n$  serves as a 
guarantee that $\perm(X)$ cannot be represented linearly as $\det(Y)$,
when $m=2^{\log^a n}$, $a>0$ fixed, $n\rightarrow \infty$ (i.e., for
$n$ greater than a large enough constant depending on $a$). 



\begin{figure} 
\begin{center}\psfragscanon
\psfrag{on}{$\{O_n\}$}
\epsfig{file=firststep.eps, scale=.8}
\end{center}
      \caption{Reduction from nonexistence to existence}
      \label{fig:firststep}
\end{figure}



This reduction to existence is carried out as follows (cf. lecture 2 for 
details).


First, we associate (GCT1) with 
the complexity class $\#P$ a family $\{X_{\#P}(n,m)\}$ of (group-theoretic)
class varieties (what this means is explained below),
and with the complexity class $NC$ a family of 
$\{X_{NC}(n,m)\}$ of (group-theoretic) class varieties such that: 
if $\perm(X)$, $\dim(X)=n$, can be represented linearly 
as $\det(Y)$, $\dim(Y)=m>n$, then 

\begin{equation} \label{eqembed} 
X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation} 

Each  class variety is a  (projective) algebraic variety, by which
we mean that it is the zero set of  a system of multivariate 
homogeneous polynomials with coefficients in $\C$  (akin to the 
usual curves  and surfaces). It is  group-theoretic in the 
sense that it is  constructed using group-theoretic operations 
and the special linear group $G=SL_l(\C)$, $l=m^2$, of $l\times l$ invertible
complex matrices acts on it, and furthermore the groups of
symmetries of the permanent and the determinant are embedded in this group
in some way. Here action means moving the points 
of the class variety around, just as $G$ moves the points of $\C^l$ around 
by the standard action via invertible linear transformations.
The goal is to show that the inclusion (\ref{eqembed}) is impossible
(obstructions are meant to ensure this);
cf. Figure~\ref{fig:class}. 

\begin{figure} 
\begin{center} \psfragscanon
\psfrag{xsharp}{$X_{\#P}(n,m)$}
      \psfrag{xnc}{$X_{NC}(n,m)$}
      \psfrag{g}{$G=SL_l(\C)$, $l=m^2$}
      \psfrag{Obstruction}{\mbox{Obstruction}}
\epsfig{file=class.eps, scale=.5}
\end{center}
      \caption{Class varieties}
      \label{fig:class}
\end{figure} 



Since each class variety has a $G$-action, the space of polynomial functions 
on each class variety has a  representation-theoretic structure, which 
puts constraints on which  representations of $G$ can live on that variety
(i.e., in the space of polynomial  functions on that variety).
Informally, an obstruction is an irreducible (minimal)  representation of $G$
that can live on $X_{\#P}(n,m)$ but not on $X_{NC}(n,m)$; 
cf. Figure~\ref{fig:class}.
Existence of  an obstruction $O_n$, for every $n$, assuming
$m=2^{\log^a n}$, $a>1$ fixed, implies  that the inclusion (\ref{eqembed}) 
is not possible, since  $O_n$ cannot live  on $X_{NC}(n,m)$.
Thus  an obstruction blocks the inclusion (\ref{eqembed}).


To define an obstruction formally, we need to recall some basic representation
theory.  By a classical result of Weyl, the irreducible 
(polynomial) representations of $G=SL_l(\C)$ are in one-to-one correspondence 
with the partitions  $\lambda$ of length  $<l$, by which we mean 
integral sequences $\lambda_1 \ge 
\lambda_2 \cdots \ge \lambda_k > 0$, $k < l$, where  $k$ is called the  length
of $\lambda$. The irreducible 
representation of $G$ in correspondence with $\lambda$ is denoted 
by $V_\lambda(G)$, and is called the {\em Weyl module} of $G$ indexed by 
$\lambda$. Symbolically:

\[\mbox{Irreducible representations of } G \stackrel{\mbox{Weyl}}{\Longleftrightarrow} \quad \mbox{partitions} \ \lambda. \]  

\[\mbox{Weyl module  } V_\lambda(G)  \longleftrightarrow \lambda. \] 
Weyl also proved that every finite dimensional representation of $G$ 
can be decomposed into irreducible representations--i.e.,
can be written as a direct sum of Weyl modules. Thus Weyl modules 
are the basic building blocks of the representation theory of 
$G$, and every finite dimensional representation of $G$ can be thought
of as a complex building made out of these blocks. 


Now suppose $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$. 
Suppose to the contrary that 

\begin{equation} \label{eqembed2}   X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation}

Let $R_{\#P}(n,m)$ denote the homogeneous coordinate ring of 
$X_{\#P}(n,m)$; i.e., the ring of polynomial functions 
\footnote{Though the  functions here are not functions in usual sense;
but let us  not worry about this} on $X_{\#P}(n.m)$. 
Let $R_{\#P}(n,m)_d$ be the degree-$d$-component of $R_{\#P}(n, m)$ consisting
of functions of degree $d$. We define $R_{NC}(n,m)$ and $R_{NC}(n,m)_d$
similarly. Since $X_{\#P}(n,m)$ has the action of $G$, $R_{\#P}(n,m)$ 
also has an action of $G$; i.e., it is a representation of $G$. Hence,
$R_{\#P}(n,m)_d$ is a finite dimensional representation of $G$. 
Similarly, $R_{NC}(n,m)$ is a representation of $G$, and $R_{NC}(n,m)_d$
a finite dimensional representation of $G$. 



If (\ref{eqembed2}) holds, then we get a natural map from $R_{NC}(n,m)$ to
$R_{\#P}(n,m)$ obtained by restricting a function on $X_{NC}(n,m)$ to
$X_{\#P}(n,m)$. %; cf. Figure~\ref{fig:restriction}.
By basic algebraic geometry, this map
is surjective and is a $G$-homomorphism.
Furthermore, it is degree-preserving. This means there
is a surjective $G$-homomorphism from $R_{NC}(n,m)_d$ to 
$R_{\#P}(n,m)_d$. Symbolically: 

\begin{equation} \label{eqsurjection}
R_{\#}(n,m)_d \leftarrow  R_{NC}(n,m)_d.
\end{equation}

\ignore{
\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{Xp}{\small $X_{\#P}(n,m)$}
\psfrag{Xnc}{\small $X_{NC}(n,m)$}
\epsfig{file=restriction.eps, scale=.6}
\end{center}
      \caption{Restriction}
      \label{fig:restriction}
\end{figure}
}

Let $R_{\#P}(n,m)_d^*$ denote the dual of $R_{\#P}(n,m)_d$; i.e., the 
set of linear maps from $R_{\#P}(n,m)_d$ to $\C$. Then (\ref{eqsurjection})
implies that there is an injective $G$-homomorphism from 
$R_{\#P}(n,m)^*_d$ to $R_{NC}(n,m)^*_d$. Symbolically: 

\begin{equation} \label{eqinclusion}
R_{\#}(n,m)_d^*  \hookrightarrow {NC}(n,m)_d^*.
\end{equation}

\begin{defn} (GCT2)
An obstruction $O_n$ is a Weyl module $V_\lambda(G)$ that 
occurs as a subrepresentation 
in $R_{\#P}(n,m)_d^*$  but not in $R_{NC}(n,m)_d^*$, for some $d$. 
We call $\lambda$ an {\em obstruction label}, and sometimes,
by abuse of notation, an obstruction as well.

A strong obstruction $O_n$ is a Weyl module $V_\lambda(G)$ 
that occurs as a subrepresentation in $R_{\#P}(n,m)_d^*$ but 
does not contain a nonzero 
invariant (fix point) of the group of the symmetries 
of the determinant.
\end{defn}

Here recall that the group of the symmetries of the determinant 
is embedded in $G$ as its subgroup, which we shall refer to as $G_{det}$.
By an invariant we mean a point in $V_{\lambda}(G)$ 
which is fixed (does not move) with respect to the action of this subgroup
$G_{det} \subseteq G$ of symmetries.

\begin{prop} (GCT2)

\noindent (a) 
Existence of an obstruction $O_n$, for all $n\rightarrow \infty$, 
with $m=2^{\log^a n}$, $a>1$ fixed, implies $\perm(X)$, $\dim(X)=n$, 
cannot be represented linearly as 
$\det(Y)$, $\dim(Y)=m$. 

\noindent (b) A strong obstruction is an obstruction. Hence (a) 
also holds for a strong obstruction.
\end{prop}

Here (a)  follows just from the definition of an obstruction, and 
leads to:

\begin{goal} \label{gobs} (GCT2)
Prove existence of a (strong) 
obstruction family $\{O_n=V_{\lambda_n}(G)\}$ using 
the  exceptional 
nature of $\perm(X)$ and $\det(Y)$, i.e., using the 
properties (P) and (D) in  Section~\ref{scharsym}).
\end{goal} 

\section{Obstructions for the mathematical form} \label{sobsweak}

The following result achieves this goal for the mathematical form
(Theorem~\ref{tgenweaklec1}).
\begin{theorem} 
There exists a (strong)  obstruction family $\{O_n\}$ for the mathematical
form  of the $\#P \not = NC$ conjecture.
\end{theorem}

This implies Theorem~\ref{tgenweaklec1}.
The notion of obstructions here is similar 
to the one in the general case. 

The proof of this result  based on the results of GCT1 and 2 in
geometric invariant theory \cite{mumford} is outlined in the third lecture.
It produces  a 
family $\{O_n=V_\lambda(G)\}$ of (strong) obstructions, with a different $G$
than in the general complexity theoretic case.
Furthemore this family  is {\em strongly explicit} in the sense  that 
the specification $\lambda_n$ of each $O_n$
has polynomial, in fact,  $O(n)$ bitlength, and  
can be constructed in polynomial, in fact, $O(n)$ time (regardless of the 
complexity  of the polynomial in the traces in the statement of 
Theorem~\ref{tgenweaklec1}).

\noindent {\em Remark:}
There is also a second noncostructive proof of this result 
(cf. Section~\ref{sweak}).
This gives a concrete evidence 
that explicit construction is not needed to cross the 
natural proof   barrier. Because 
any proof that relies only on the property (P) automatically
bypasses this barrier, as remarked before.
But   this nonconstructive
proof is not any easier than the explicit proof.
Indeed, the whole proof
structure  here is such that its easiest implementation  yields 
obstructions explicitly 
whether one cares for them or not. We shall see the same pheonomenon
in the general case in what follows.


\section{Towards existence of obstructions in general via positivity}
We now proceed to describe the main results of GCT for the general
(complexity-theoretic)
permanent vs. determinant problem in the context of
Goal~\ref{gobs}. 



Towards that end, we  define 
certain representation-theoretic {\em stretching} functions. 
Let $F_{\lambda,n,m}(k)$ denote the number of occurances (multiplicity)  of
the Weyl module $V_{k\lambda}(G)$ in $R_{\#P}(n,m)^*$ (i.e. 
$R_{\#P}(n,m)^*_d$, for some $d$)  as a subrepresentation.
Let $G_{\lambda,m}(k)$ denote the multiplicity of the trivial one dimensional
representation (invariant) of $G_{det} \subgroup G$ in 
$V_{k\lambda}(G)$. In other words, $G_{\lambda,m}(k)$ is the dimension
of the subspace of invariants of $G_{det}$ in $V_{k \lmbda}(G)$.
These are statistical functions
associated with the class variety $X_{\#P}(n,m)$ 
and the subgroup embedding  $G_{det} \hookrightarrow  G$.
In the first case,  the statistics associates 
with every number (stretching parameter) $k$  
the multiplicity of the corresponding
Weyl module $V_{k\lambda}(G)$ in $R_{\#P}(n,m)^*$;
cf. Figure~\ref{fig:statistics}.

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{l}{$\lambda$}
\psfrag{2l}{$2 \lambda$}
\psfrag{3l}{$3 \lambda$}
\psfrag{v1}{$V_\lambda(G)$}
\psfrag{v2}{$V_{2 \lambda}(G)$}
\psfrag{v3}{$V_{3\lambda}(G)$}
\epsfig{file=statistics.eps, scale=1}
\end{center}
      \caption{statistics}
      \label{fig:statistics}
\end{figure}


Let us  call a function $f(k)$ {\em quasipolynomial}, if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k)$ for all nonnegative integral $k=i$ modulo $l$;
here  $l$ is
called the period of the  quasi-polynomial. 
Thus  quasi-polynomials
are hybrids of  polynomial and periodic functions. 
We say that $f(k)$ is an 
{\em asymptotic quasipolynomial} if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k)$ for all nonnegative integral $k=i$ modulo $l$ for 
$k\ge a(f)$, for 
some nonnegative integer depending on $f$. The minimum 
$a(f)$ for which this holds is called the {\em deviation from 
quasipolynomiality}. Thus $f(k)$ is a (strict) quasipolynomial when this
deviation is zero.

A fundamental example of a quasi-polynomial is the Ehrhart quasi-polynomial
$f_P(k)$ of a polytope $P$ with rational vertices. It is defined
to be the number of integer points in the dilated polytope $kP$. By the 
classical result of Ehrhart, it is known to be a quasi-polynomial.
More generally, let $P(k)$ be a polytope parametrized by nonnegative
integral $k$: i.e., 
defined by a linear system of the form: 
\begin{equation} \label{eqpara}
A x \le k b + c,
\end{equation}
where $A$ is an $m \times n$ matrix, $x$ a variable $n$-vector, and 
$b$ and $c$ some constant $m$-vectors. Let $f_P(k)$ be the number 
of integer points in $P(k)$.  It is known to be  an asymptotic
 quasi-polynomial. We shall call it the asymptotic 
Ehrhart quasi-polynomial  of the parametrized polytope $P(k)$. 
In what follows, we  denote a parametrized polytope $P(k)$ by 
just $P$. 
From the context it should be clear whether $P$ is a usual nonparametrized 
polytope or a parametrized polytope.









\begin{theorem} (GCT6) \label{tquasi}

\noindent (a) The  function $G_{\lambda,m}(k)$ is a quasi-polynomial.


\noindent (b) The function $F_{\lambda,n,m}(k)$ is 
an asymptotic quasi polynomial.

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem} 

\ignore{Here a rational and normal  singularity means a singularity that is nice in
an algebro-geometric sense that we shall not elaborate here.
At present, we do not know if the singularities of the class varieties 
are indeed  rational and normal. A conservative conjecture would be  that 
they are not too bad, even if they are not strictly rational and normal,
because of the exceptional nature of the 
determinant and the permanent; 
i.e.,  the deviation from quasipolynomiality
of $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ is 
small in a sense to be made precise 
later (cf. the remarks after Hypothesis~\ref{hph1}).}

The proof of Theorem~\ref{tquasi} is based on:
\begin{enumerate} 
\item The classical work of Hilbert in invariant theory, 
\item The 
resolutions of singularities in characteristic zero
\cite{hironaka}: 
this  roughly says 
that the singularities of any algebraic variety in characteristic zero
can be untangled (resolved) nicely in a systematic fashion; cf.
 Figure~\ref{fig:resolution}.
\item Cohomological works of Boutot, Brion,  Flenner, Kempf  and others
based on this resolution; cf.  \cite{boutot,dehy} and
GCT6 for the history and other references.
\end{enumerate} 


\begin{figure} 
\begin{center} 
\epsfig{file=resolution.eps, scale=.5}
      \caption{Resolution}
      \label{fig:resolution}
\end{center}
\end{figure}


As such, this proof is highly nonconstructive. It gives no effective
bound on the period $l$--it just says that $l$  is finite.





The following hypothesis 
says that $G_{\lambda,m}(k)$  can be realized as the Ehrhart quasi-polynomial
of a polytope, and 
$F_{\lambda,n,m}(k)$ 
can be realized as the asymptotic Ehrhart quasi-polynomial 
of a parametrized  polytope.

\begin{hypo} {\bf (PH) [Positivity Hypothesis]} \label{hph} (GCT6)

\noindent (a) For every $\lambda,n,m\ge n$, 
there exists   a parametrized  polytope $P=P_{\lambda,n,m}(k)$ 
such that 
\begin{equation} \label{eqP}
F_{\lambda,n,m}(k)=f_P(k).
\end{equation} 
It is also assumed here that there exists for $P_{\lambda,n,m}$ a specification
of the form (\ref{eqpara}),
 where $A$ is independent of $\lambda$, and $b$ and $c$ 
are  piecewise homogeneous linear functions of $\lambda$.


\noindent (b) There exists a (usual nonparametrized) 
polytope  $Q=Q_{\lambda,n,m}$  such that
\begin{equation} \label{eqQ}
G_{\lambda,m}(k)=f_Q(k).
\end{equation}


Analogous positivity hypothesis also holds 
for the $P$ vs. $NP$ problem in characteristic zero.
\end{hypo} 


If such $P$ and $Q$ exist, their dimensions are guaranteed to be
small by the proof of Theorem~\ref{tquasi}: specifically,
the dimension $P$ is guaranteed to be bounded by a 
polynomial in $n$, and the dimension of $Q$ 
by a polynomial in $m$.
There is a variant of PH (b), which is good enough for our purposes (cf.
Lecture 3, Hypothesis~\ref{hphvariant}),
wherein  the dimension of $Q$ is also guaranteed
to be bounded by a polynomial in $n$ (but independent 
of $m$), if the length of $\lambda$ is $\poly(n)$ (as it would be in 
our applications).






When PH holds, we say that $F_{\lambda,n,m}(k)$ and 
$G_{\lambda,n,m}(k)$ have  {\em positive convex representations}. 
Here positivity refers to the fact that the Ehhart function 
$f_P(k)$ is a positive expression:
\[ f_P(k)=\sum_{v} 1,\] 
where $v$ ranges over all integer points in $P(k)$--there are no 
alternating signs in this expression.
Convexity refers to the  convexity of the polytopes $P(k)$ and $Q(k)$. 


But, a  priori, it is not at all clear why PH should  even hold. 
Many numerical functions in algebraic geometry are 
asymptotic quasi-polynomials (e.g., the Hilbert function 
\footnote {Hilbert function $h_Z(k)$ of a projective algebraic variety $Z$
is defined to be $\dim(R(Z)_k)$, where $R(Z)$ is the homogeneous coordinate 
ring of $Z$ and $R(Z)_k$ its degree $k$-component.} of any projective
variety), but they rarely have positive convex representations.
PH is expected to hold for $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ 
because of the exceptional nature of the determinant and the permanent. 
One concrete evidence is provided by the proof of the weak form 
(Thoerem~\ref{tgenweaklec1}).
Analogous PH that arises in this weak setting can 
proven unconditionally.
For  mathematical evidence and justification
in support of  general PH, see  GCT6,7, and 8. 


The hypothesis 
PH alone is not sufficient to prove the existence of obstructions.
The precise statement of a sufficient condition is given in 
the theorem below.




\begin{theorem} (GCT6) \label{tgct6}
There exists a family $\{O_n\}$ of obstructions 
for the  $\#P$ vs. $NC$ problem in characteristic zero, 
for $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$, 
assuming, 

\begin{enumerate} 
\item PH, and
\item OH (Obstruction Hypothesis): 

For all $n\rightarrow \infty$,  there exists $\lambda$ such that 
$P_{\lambda,n,m}(\infty)=\mbox{lim}_{k\rightarrow \infty} P(k) 
\not = \emptyset$ and $Q_{\lambda,n,m}(k)=\emptyset$ for all (large enough)
$k$.
\end{enumerate}

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem}

Mathematical evidence and arguments in support of OH are given in GCT6.
The analogous weak OH that arises in the context of the generalized 
weak form can be  proven unconditionally.

We call  $\lambda$ a {\em relaxed obstruction}
(or rather, relaxed obstruction-label)
if it satisfies OH. In this case, $k\lambda$, for some integer $k\ge 1$ is
an obstruction--we just have to choose $k$ large enough 
so that 
$P_{\lambda,n,m}(k)$ contains an integer point
but $Q_{\lambda,n,m}(k)$ does not.
Henceforth, whenever we say obstruction, we actually mean relaxed 
obstruction.

There is a fundamental difference between the nature of PH and OH.
PH is a {\em mathematical hypothesis}, because there is no 
constraint on what $m$ should be in comparison to $n$ in its statement.
In contrast, OH is a {\em complexity theoretic hypothesis}, because 
$m$ needs to be small in comparison to $n$ for it to hold.


%\subsection{Why should PH  and OH hold?} 

%Mathematical evidence for this is given in GCT2,4,6,7,8.
%We shall discuss some of this  in the third lecture.


\section{The flip: Explicit construction of obstructions} 
\label{sflip}
In principle PH may have a nonconstructive proof (like that
of Theorem~\ref{tquasi})  which only tells  that such polytopes 
exist without explicitly constructing them. But proving OH may not be feasible
unless the polytopes $P$ and $Q$ in PH are given explicitly.
This  suggests the following strategy for proving 
existence of obstructions proposed in  GCT6 and  GCTflip.


\noindent (1) Prove the following stronger explicit form 
of PH, which is reasonable since the polytopes $P$ and $Q$, if they exist,
are already guaranteed to be of small (polynomial) dimension:

\begin{hypo} {\bf (PH1)}  \label{hph1} (GCT6)

\noindent (a) There exists an {\em explicit} 
polytope $P_{\lambda,n,m}$ 
as in  PH (a).
Explicit means: 

\begin{enumerate}
\item  The polytope is specified by an explicit system of linear constraints,
where the bitlength of (the description of) 
each constraint is  $\poly(n,\bitlength{\lambda}, \bitlength{m})$.
Here and in what follows, $\bitlength{z}$ denotes the bitlength of the 
description of $z$.

\item  The membership problem for the polytope
$P_{\lambda,n,m}(k)$  also 
belongs to the complexity class $P$.
That is,  given a point $x$, whether it belongs to $P_{\lambda,n,m}(k)$ 
can also be decided in $\poly(\bitlength{x},\bitlength{\lambda},
n,\bitlength{m})$
time.
Furthermore, we assume that if $x$ does not belong to the polytope,
then the membership algorithm also gives a hyperplane separating 
$x$ from the polytope in the spirit of \cite{lovasz}. 
\end{enumerate} 

\noindent (b) There exists a similar  explicit 
polytope $Q_{\lambda,n,m}$  satisfying   PH (b). 
\end{hypo}

\noindent {\em Remark 1:} 
Note the occurence of  $\bitlength{m}$  instead of $m$ in the polynomial
bounds in (a) (which implies that the bounds here become $\poly(n)$
when $m<2^n$ and $\bitlength{\lambda}=\poly(n)$). 
The reasons for this will be explained in Lecture 3 
(cf. remarks after Hypothesis~\ref{hph1restatement}). 
In contrast, the polynomial bounds for the polytope in (b)  depend on 
$m$, not $\bitlength{m}$. 
But there are  variants of PH (b) and PH1 (b), 
(cf. Hypotheses~\ref{hphvariant} and \ref{hph1tilde} in  Lecture 3), 
which are enough for our purposes, 
wherein the polynomial bounds depend on the bitlength of $\lambda$,
but not on $m$.
In what follows, we assume that PH (b) and PH1 (b) have been replaced 
with these variants.

 


\noindent {\em Remark 2:} 
In particular, PH1 implies that the functions $F_{\lambda,n,m}(k)$ and
$G_{\lambda,n,m}(k)$ belong to the complexity class $\#P$. 
It can be shown that it 
also implies that the deviation from quasipolynomiality 
of $F_{\lambda,n,m}(k)$ is small, specifically, 
$2^{O(\poly(\bitlength{\lambda},n,\bitlength{m}))}$--thus the bitlength
of the deviation is polynomial. This says
that the deviation from rationality and normality of the singularities
of the class variety $X_{\#P}(n,m)$ is small (cf. Theorem~\ref{tquasi}).
Similarly for $Q_{\lambda,n,m}(k)$ and $X_{NC}(n,m)$. 

Like PH, PH1 is also a mathematical hypothesis in the sense that
it puts  no constraint on what $m$ should be in comparison to $n$. 
Of course, unlike PH, there is some complexity theoretic aspect to it, 
but it is secondary in comparison to the complexity-theoretic aspect of 
 OH, since smallness  of $m$ with respect to  $n$ is the 
crux of the lower bound  problems under consideration. 





\noindent (2a) {\bf [The flip]}

Let $m=2^{\log ^a n}$, for a fixed $a>1$. 
Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
show existence of  an {\em explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of (relaxed) obstructions  satisfying OH. 
We say that an obstruction (proof-certificate) 
$\lambda_n$ is {\em explicit} if is ``short'' and ``easy to verify'':


\begin{enumerate} 
\item  Short: This means its bitlength $\bitlength{\lambda_n}$ 
is $\poly(n)$,
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  

\item Easy to verify: given $n, m \le 2^{n}$ and 
$\lambda_n$, whether 
$\lambda_n$ is a valid obstruction 
can be verified 
in $\poly(n,\bitlength{\lambda})$ time. In particular, this is
$\poly(n)$ when $\bitlength{\lambda}=\poly(n)$. 
\end{enumerate}

Existence of an explicit family of obstructions is equivalent to saying
that the problem of deciding existence of obstructions belongs to $NP$.
This definition of explicitness is quite natural since the class $NP$ 
is a class of problems whose proof-certificates (witnesses) are 
short and easy to verify. As such, the flip--going for 
explicit  obstructions--is
a proof-strategy that is literally given to us on a platter 
by the $P$ vs. $NP$ 
problem itself. Why it is called flip will be explained later.


It should be stressed that we are primarily interested in only proving 
existence of obstructions. Whether they are explicit or not 
does not really matter in the original statement of the problem.
But we need to know the polytopes $P$ and
$Q$ explicitly (as in PH1)  so that proving OH is feasible. 
%In other words,   if we do not
%even know what the polytopes $P$ and $Q$ look like, 
%it seems unlikely that anything  could be said regarding OH. 
But once  PH1 is proved, existence of an explicit family follows
automatically,   as a bonus, whether we care for it or not. 

To see why, let us observe that 
the second condition above  (ease of verification) follows directly
from PH1 and the polynomial time algorithm for 
linear programming on  polytopes given by separation oracles \cite{lovasz}. 
Shortness  also follows from PH1. 

Thus it is as if the $P$ vs. $NP$ problem is forcing us to go
for explicit obstructions.


\noindent (2b) {\bf [The strong flip (optional)]} 

Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
construct (rather than just show existence of) 
a {\em strongly explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of obstructions  satisfying OH. We say that an explicit family 
of obstructions is strongly explicit if,
for each $n$, a valid obstruction-label
$\lambda_n$ can be constructed in $\poly(n)$ time.
In particular, the height and the bitlength of
 $\lambda$ is $\poly(n)$ (short) 
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  


For the purposes of the lower bound problems that we are interested in, the
flip (just explicit  
existence) would suffice and the stronger flip (explicit construction)
is optional. But the stronger flip can give us deeper insight into these
lower bound problems; cf. GCTflip for more on this.

Now we turn to a few obvious questions.



\section{What has been achieved by all this?: The meaning of the flip} 
\label{smeaning}
Let us now see what has been achieved so far
in the context of the 
$\#P\not = NC$ conjecture in the nonuniform setting (characteristic zero),
the argument for the $P$ vs. $NP$ problem in characteristic zero
being  similar. 
At  first glance,
it may seem that all that GCT has achieved 
is to exchange a known difficult problem of 
complexity theory with a new very difficult problem of algebraic geoemtry.
In order to see that something is gained in exchange let us reexamine the 
original question.

The goal of the original  conjecture is to prove that 
$\perm(X)$, $\dim(X)=n$,  cannot be computed by an arithmetic circuit $C$
of size $m=\poly(n)$, or more generally,
$m \le 2^{\log^a n}$, for some fixed $a>1$, and depth $O(\log^a n)$.
Symbolically, 
let  $f_C(X)$ denote the function computed by $C$. Then we want to prove that
\begin{equation} \label{eqioh} 
 {\bf (IOH):}  \forall n \ge n_0 \forall C \exists X:
\perm(X)\not = f_C(X),
\end{equation} 
where $n_0$ is a sufficiently large constant.
For given $X$ and $C$ of $\poly(n)$ size, the problem 
of deciding if  $\perm(X) \not = f_C(X)$
belongs to $\#P$ (or rather, $P^{\#P}$). 
Since there are two alternating layers of quantifiers in (\ref{eqioh}),
the problem of verifying it belongs to $\Pi_2^{\#P}$, 
which is very high in the complexity hierarchy
(cf. Figure~\ref{fig:IOHcomplexity}).
Hence, we  refer to the original hypothesis (\ref{eqioh}) 
to be proven  as IOH 
(Infeasible Obstruction Hypothesis). Of course, IOH is expected to 
be a tautology, and hence is expected to  be verifiable in $O(1)$ time--but
we do not know that as yet. 



\begin{sidewaysfigure} 
\begin{center}
\psfragscanon
\psfrag{sigma2p}{{\small $\Pi^2 \#P$}}
\psfrag{sigma1p}{$\Sigma^1 \#P$}
\psfrag{P}{{\small $P$}}
\psfrag{NP}{{\small $NP$}}
\psfrag{T}{$T$}
\psfrag{#P}{$\# P$}
\psfrag{inNP}{$\in NP$}
\psfrag{inP}{$\in P$}
\psfrag{insigma2p}{$\in \Pi^2 \#P$}
\psfrag{PHplus}{PH1}
\psfrag{PHtil}{$PH^\dagger$}
\epsfig{file=IOHcomplexity.eps, scale=.8}
\end{center}
      \caption{Positivity as a means to eliminate the quantifiers and 
reduce the complexity of the  obstruction hypothesis}
      \label{fig:IOHcomplexity}
\end{sidewaysfigure}



Equivalently, the goal of IOH 
is to prove existence of a {\em trivial obstruction},
which is a table that lists for each $C$ as above a counterexample  $X$ so that
$\perm(X)\not = f_C(X)$; cf. Figure~\ref{fig:trivial}.
The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$ and depth
$O(\log^a n)$. Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. (Well, only
if the underlying field of computation is finite. For infinite fields, 
such as $\Q$ or $\C$ in this paper, 
there is another notion of a trivial obstruction (cf. 
GCT6). But let us imagine that the underlying
field is finite for this argument.)
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time to decide if such a table exists and construct 
one (optional) for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. That is why we 
call  this trivial, brute force 
strategy of proving IOH, based on existence of trivial obstructions,
an {\em infeasible strategy}. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{eq}{$\perm(X)\not = f_C(X)$}
\epsfig{file=trivial.eps, scale=.5}
\end{center}
      \caption{A trivial obstruction}
      \label{fig:trivial}
\end{figure}


In contrast, assuming PH1, the problem  of verifying OH belongs 
to $NP$ as we have already observed. Thus, assuming PH1, we have 
transformed the original infeasible obstruction 
hypothesis $IOH \in \Pi_2^{\#P}$ to a new  obstruction hypothesis 
$OH \in NP$, in the process bringing down the time to verify an obstruction
from  exponential (for the original trivial obstruction) to polynomial
(for the new obstruction); cf. Figure~\ref{fig:IOHcomplexity}.  
It is crucial here that PH1, the main tool for this reduction, is a 
mathematical hypothesis,  not complexity-theoretic (cf. the remarks
after Theorem~\ref{tgct6} and Hypothesis~\ref{hph1}).
The task of verifying  an obstruction has also been 
transformed from the infeasible (exponential-time) to the feasible 
(polynomial-time). Hence the name of this strategy: the flip,
from the infeasible to the feasible.
Positivity (PH1) is used in the flip as a means  to
eliminate the quantifying variables in IOH and bring down the 
 complexity of the obstruction hypothesis;
cf. Figure~\ref{fig:IOHcomplexity}. 




This process can be extended further. Assuming an additional
positivity hypothesis PH4 specified below,
$OH \in NP$ can be transformed 
to POH (Positivity Obstruction Hypothesis) that belongs to $P$; i.e.,
which can be verified in polynomial time, and an obstruction,
if it exists, can also be constructed in polynomial time; 
cf. Figure~\ref{fig:IOHcomplexity}. (The hypothesis is called PH4 instead
of PH2, because PH2 and PH3 are some other positivity hypotheses in GCT6
that complement PH1). 
Once this final positivity hypothesis POH is proven, the obstruction
hypothesis is reduced to a tautology (FOH: Final Obstruction Hypothesis),
which can be verified in
$O(1)$ time. This  would then give us 
the final $O(1)$-size  proof. 

Thus the basic idea of the flip is to use positivity systematically
as a means to eliminate the quantifiers  and reduce the complexity 
of the  obstruction hypothesis until it is finally
reduced to  an $O(1)$-time verifiable  tautology;
cf. Figure~\ref{fig:IOHcomplexity}. 

Now let us specify PH4 and POH.
Towards that end, let  $k \le l=m^2$ be the length of $\lambda$.
Define 

\begin{equation} 
\begin{array}{l}
\bar P_{n,m}= \{ \lambda: P_{\lambda,n,m} \not = \emptyset \} \subseteq \C^k, \\
\bar Q_{n,m}= \{ \lambda: Q_{\lambda,n,m} \not = \emptyset \} \subseteq \C^k.
\end{array}
\end{equation}

\begin{theorem} 
The sets $\bar P_{n,m}$ and $\bar Q_{n,m}$ are convex polytopes in $\C^k$.
\end{theorem} 
This follows from some fundamental results in geometric invariant theory
\cite{mumford}. 

Then: 

\begin{hypo}  {\bf PH4} (GCT6)
The membership problems for these polytopes belong to 
$P$ and so also the problem of deciding if $\mbox{vol}(\bar P_{n,m}
\setminus \bar Q_{n,m})$, the volume of the relative complement 
$\bar P_{n,m} \setminus \bar Q_{n,m}$, is nonzero (positive);
i.e. if $\bar P_{n,m} \not \subseteq \bar Q_{n,m}$. By polynomial time,
we mean $\poly(n,l,\bitlength{m})$ time. This is $\poly(n)$,
if $m\le 2^{o(n)}$ and $l =\poly(n)$. 
\end{hypo}

\begin{hypo} {\bf (POH)}

For all $n\rightarrow \infty$, assuming $m=2^{\log^a n}$, $a>1$ fixed, 

\[ \mbox{vol}(\bar P_{n,m} \setminus \bar Q_{n,m}) > 0, \] 

for $k=(n+1)^2$. 
\end{hypo} 

\ignore{
Thus POH says that  the line-shaded area in Figure~\ref{fig:POH} has positive
volume for all large enough $n$. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{P}{$\bar P_{n,m}$}
\psfrag{Q}{$\bar Q_{n,m}$}
\epsfig{file=POH.eps, scale=1}
\end{center}
      \caption{POH}
      \label{fig:POH}
\end{figure}
}

\section{How to prove PH?}  \label{sphprove}
There is  a basic prototype of PH in representation theory,
which will be described in detail towards the end of Lecture 3. We shall
refer to it  as Plethysm PH. It says that the stretching functions 
akin to $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$
associated with  fundamental  multiplicities 
in representation theory called plethysm constants also have analogous 
positive convex representations. 

This  is   known for a very special case of the plethysm constant 
called the  Littlewood-Richardson (LR) coefficient
$c_{\alpha,\beta}^\lambda$. It is  defined to be 
the number of occurances of the Weyl module $V_{\lambda}(G)$ in the 
tensor product of $V_{\alpha}(G)$ and $V_\beta(G)$. 
The classical Littlewood-Richardson rule, which we shall refer to as LR PH,
implies that the stretching function 
$\tilde c_{\alpha,\beta}^\lambda (k) = c_{k \alpha, k \beta}^{k \lambda}$
associated with the Littlewood-Richardson coefficient has a
positive convex representation.

Plethysm PH   happens to be a fundamental open problem of
representation theory, older than the $P$ vs. $NP$ problem itself. It 
has been studied intensively in the last century, and is known to be
formidable. And  now,  as explained the third lecture, it also turns out to 
be  the heart of this approach towards the $P$ vs $NP$, the
$\#P$ vs. $NC$ problems.



A basic plan to prove Plethysm PH is given in GCT6.
It is partially 
implemented in GCT7 and 8. See Figure~\ref{fig:lift} for a pictorial
depiction of the plan. It strives  to extend the  proof of LR PH based 
on the theory of the  standard quantum group \cite{drinfeld,kashiwara,lusztig}.
There it
comes out as a consequence of a  (proof of a) deep positivity result
\cite{kazhdan,lusztig}, which
we shall refer to as LR PH0. It says that   the 
tensor product of two representations of the standard quantum group 
has a canonical basis \cite{kashiwara,lusztig} 
whose structure coefficients are all positive \cite{lusztig}
polynomials (i.e., polynomials with nonnegative coefficients).
The only known proof of this
result is based on the Riemann Hypothesis over finite fields 
proved in \cite{weil2},  and the related works \cite{beilinson}. 
This Riemann Hypothesis over finite fields 
is  itself a deep positivity statement in mathematics,
from which   LR PH can  thus be 
deduced, as shown on the bottom row of Figure~\ref{fig:lift}.

If one were only interested in LR PH, one  does not 
need this  powerful machinery, because it has a  much simpler 
algebraic-combinatorial  proof. 
But the plan to extend the
proof of LR PH to Plethysm PH in GCT6,7,8 is like a huge
inductive spiral. To  make it work,  one  needs a 
stronger inductive hypothesis than Plethysm PH--this is precisely  Plethysm 
PH0 (which  will be
described in the third lecture; cf. Hypothesis~\ref{hplph0}).
Thus what is needed now 
is a systematic lifting  of the bottom arrow in Figure~\ref{fig:lift}
to the top, so as to complete the  commutative diagram, so to speak. 

Initial  steps in this direction have been taken in GCT7,8. 
First, GCT7 constructs a {\em nonstandard quantum group}, which
generalizes the notion of a standard quantum group \cite{drinfeld},
 and plays the
same role in the plethysm setting that the standard quantum group plays
in the LR setting. Second, GCT8 gives an algorithm to construct 
a canonical basis for a representation of the nonstandard quantum group
that is conjecturally correct and has the property Plethysm PH0,
which is a   generalization of LR PH0  supported by experimental
evidence.
Now what is needed to complete  the 
commutative diagram in Figure~\ref{fig:lift} is an appropriate nonstandard 
extension of the Riemann hypothesis over finite fields and the related works
\cite{beilinson,weil2,kazhdan,lusztig}
from which  Plethysm PH0 can be deduced. This--the top-right corner 
of the diagram--is the   main  open problem at the heart of this approach. 

\section{How to prove OH or POH?} 
We do not  know, 
since the  proof of OH and POH 
would really depend on the explicit forms of the
polytopes that arise in   PH1/PH4, and we have no idea about them
at this point.
\ignore{GCT does suggest  that proving OH/POH  should be feasible 
``in theory''
since OH/POH  belong to NP/P, assuming PH1/4, and polynomial-time
is complexity theory stands for feasible ``in theory''. 
In other words,
GCT gives a reason to believe now that proving 
the  $P\not = NP$ conjecture should be feasible in theory. Even this
was  always questioned  in the field of complexity theory so far, because 
the $P$ vs. $NP$ problem is a universal statement regarding all of mathematics
(that says theorems cannot be proven automatically).
But, as we also know by now, 
there is a huge gap between  theory and  practice--e.g., 
just because  some problem is in $P$ does not 
necessarily mean that it is feasible in practice. Similarly,
the actual implementation of the GCT flip via positivity is expected to be 
immensely difficult ``in practice'', as Figure~\ref{fig:lift} suggests. 
}






\section{Is positivity  necessary?} \label{sposnece}
\ignore{
Though the statement of this result is elementary, its proof is nonelementary,
as expected,  since the generalized permanents are highly nontrivial
and mathematically formidable objects. Specifically, the problem
of finding a $\#P$-basis for the space of generalized permanents 
is intimately related to some formidable problems of representation
theory and algebraic geometry,
and the  simplest analogue of this problem 
which can be solved at present  \cite{}
requires the deep Riemann Hypothesis over finite fields \cite{} for its
proof; cf. Section~\ref{}.
The proof of Theorem~\ref{} proceeds at an abstract level 
through algebraic geometry and representation theory without
having to know anything about such a basis.
At present, it is open if there is any alternative 
weaker form of the $\#P \not = NC$  conjecture,
which cannot be proved by relativizable, low-degree or 
naturalizable  techniques, but which can still be proved by elementary 
or not so  nonelementary techniques; that is, whether the earlier known
barriers mentioned above can 
be simultaneously bypassed in an elementary way in the context of 
the $\#P$ vs. $NC$ (or $P$ vs. $NC$  or $P$ vs. $NP$) problem.


\section{Why are we going for explicit obstructions?}
In a sense, the proof of the weak form turns out to be nonelementary
because of the difficulty of explicit construction. Specifically, algorithm 
to construct an obstruction $O_n$ for each $n$ is very simple, but to
show that it is correct requires nontrivial algebraic geometry,
just as the construction 
of an explcit family of Ramanujan graphs in \cite{} is very simple,
but to show that it is correct requires nontrivial algebraic geometry.
We already know, e.g. from this example of Ramanujan graphs, that 
explicit constructions can require highly nonelementary techniques.
So the question now arises: why are we going for such difficult explicit
constructions? Can they not be avoided somehow? 
After all, to solve the original problem we only need to show existence
of obstructions. We do not have to construct them explicitly.

Furthermore,  explicit construction is not needed to 
cross any of the barriers mentioned above (e.g. the natural-proof-barrier).
This is because {\em any} proof technique which uses symmetries of the
permanent would automatically bypass the natural-proof barrier
in the context of the permanent vs. determinant problem,
even if it does not utter a word about explicit construction, since
most functions have no symmetries. Indeed, the weak form of 
the generalized $\#P$ vs. $NC$ problem itself has two proofs, one
purely nonconstructive and one through explicit construction--the major 
chunk of both proofs being  the same, except for the last step,
which is carried out via a counting argument in the former proof and via
explicit construction in the latter. Since the nonconstructive proof too
is based on symmetries, it also crosses the natural-proof barrier.
This provides a concrete evidence that explicit construction is not 
necessary for crossing the earlier known  barriers.

Then why are we still going for explicit construction? 
Before we go any further, we wish to briefly state  the motivation
behind  going for the flip (explicit construction),
since this is an important issue. 
}

Finally,  if the positivity problems are so hard,  one may ask if 
they can not be avoided somehow. Unfortunately, there is a formidable 
barrier towards the $P$ vs. $NP$ and related problems, called the
{\em feasibility ($P$) barrier} (GCT6,GCTflip),
which seems universal in the sense that
any approach towards these problems would have to tackle it, not just GCT. 
The flip, i.e., explicit construction of obstructions, is the most natural
and obvious way to cross this barrier, and it also seems to be 
among the easiest. The 
existing mathematical evidence suggests that any such natural approach
to cross this barrier would have to say  something deep regarding positivity
(Plethysm PH/PH0)  either explicitly or {\em implicitly}, even if
the approach does not utter a word about algebraic geometry or
representation theory.
That is,  Plethysm PH and PH0   may indeed be 
the heart of the  fundamental lower bound problems in complexity theory;
a detailed story and a precise meaning of the key 
phrase {\em implicit} would appear in the revised version of GCTflip.

%\input{feasibility}









































 

































\begin{sidewaysfigure} 
\begin{center} 
\epsfig{file=lift.eps, scale=.8}
\end{center}
      \caption{A commutative diagram}
      \label{fig:lift}
\end{sidewaysfigure} 



\ignore{\begin{figure} 
\psfragscanon
\psfrag{P}{$P\not = NP$ and $\#P\not = NC$ conjectures (characteristic zero)}
\epsfig{file=barriers.eps, scale=1}
      \caption{The feasibility barrier towards $P$ vs. $NP$}
      \label{fig:barriers}
\end{figure}}


%\input{lecture1_maintext}


==> lecture1_9.tex <==
\section*{Introduction}

This article   gives a mathematical  overview of
geometric complexity theory (GCT), an
approach  towards the fundamental lower bound problems  in complexity theory, 
such as (Figure~\ref{fig:complexityclasses}):

\noindent (1) 
The $P$ vs. $NP$ problem \cite{cook,karp,levin}: 
 show that $P \not = NP$;


\noindent (2) 
The  $\#P$ vs. $NC$ problem \cite{valiant}: show that 
$\#P \not = NC$.

\noindent (3) The $P$ vs. $NC$ problem: show that $P \not = NC$.



We  focus here on only the nonuniform versions of the above problems 
in characteristic zero; i.e., when
the underlying field of computation is of characteristic zero, 
say $\Q$ or $\C$.  The additional problems that
need to be addressed when the underlying field of computation is finite
would be discussed in  GCT11. 


The nonuniform
characteristic zero version of the $P\not = NC$ conjecture (in fact,
something stronger) was already proved  in GCTlocal. We shall refer
to it as the $P\not = NC$ result without bit operations.
It says that the max flow problem cannot be solved in the 
PRAM model without bit operations in $\polylog(N)$ time using 
$\poly(N)$ processors where $N$ is the bitlength of the input.
This  may be considered to be the first unconditional lower bound result of
GCT, because, though it can be stated in purely elementary combinatorial
terms, being a formal implication of the $P\not = NC$ conjecture, its
proof is intrinsically geometric, and no elementary proof is known so far. 
Furthermore, its proof  technique may be considered to be a weaker (local)
form of the {\em flip}, the basic guiding strategy of GCT, which  was 
refined and formalized much later in GCTflip. 
This  was the begining of  this  geometric approach in complexity theory.
The later work in GCT-- the subject of this overview--focusses on the other 
two problems above, namely
the $P$ vs. $NP$ and $\#P$ vs. $NC$ problems. 


The nonuniform (characteristic zero) version of the $\#P$ vs. $NC$ problem
is also known as the permanent vs. determinant problem \cite{valiant}. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented %(cf. Figure~\ref{fig:matrices})
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$. %; the best known lower bound on $m$ at present is 
% quadratic \cite{ressayre}.
By linear representation, we mean
the  entries   of $Y$ are  (possibly nonhomogeneous) 
linear functions of the entries of $X$. 
There is an analogous characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.
The main results of GCT for the $\#P$ vs. $NC$ problem in 
characteristic zero also extend to the $P$ vs. $NP$ problem in characteristic
zero. But here we shall 
concentrate  on only the former problem,
since this illustrates all the basic ideas. 



The complementary article \cite{GCTexplicit} gives a complexity-theoretic
overview of GCT. It describes   the main complexity theoretic
barrier towards these problems 
called the {\em feasibility barrier} and the defining
strategy of GCT for crossing it called the {\em flip} [GCT6,GCTflip]: 
which is to go 
for {\em explicit proofs}. By an explicit proof 
we mean a proof that provides proof certificates of hardness  for the 
hard function under consideration that are short (of polynomial size) 
and easy to verify (in polynomial time). This barrier turns out to be
extremely formidable and is the root cause of all difficulties 
in these problems. Nonelementary techniques are brought into GCT precisely
to cross this barrier. This barrier is not discussed in these lectures. 
The goal here is to describe the basic ideas of GCT at a concrete mathematical
level without getting into such meta issues. But the readers who wish
to know the need for the nonelementary techniques in GCT before getting
into any mathematics   may wish to read that
article before this one. On the other hand, the readers who would rather avoid 
meta issues before getting a concrete mathematical
picture  may wish to read this article first. We will leave the
exact choice to the readers.

The original IAS lectures stated a lower bound called a 
{\em weak form  of the $\#P$ vs. $NC$
problem}. This is a special case of a far more general result of 
GCT, which may be considered its second unconditional lower bound result, and 
which we shall call {\em a mathematical form of the $\#P \not = NC$ 
conjecture}.  It is essentially a direct consequence of the general 
results in GCT1 and 2 in conjunction with a fundamental result \cite{kempf} 
of geometric invariant theory \cite{mumford} that were used there, though
the lower bound was not stated there. It would appear in revised GCT6
with an explicit proof.
The article \cite{boris} showed that the weak form  stated in the IAS 
lectures is  too weak because it has a direct elementary proof 
which is naturalizable, i.e., which  does not cross the natural proof barrier
\cite{rudich}. Hence in this article it has been replaced with the 
mathematical form of the $\#P\not = NC$ conjecture mentioned above; cf. 
Section~\ref{sweaklec1}. 
We cannot prove this  mathematical form by such elementary naturalizable 
proof techniques for the reasons given in Sections~\ref{sweaklec1} and 
\ref{sweak}. 





The rest of this article is organized in the form of three chapters,
one per  lecture. The first gives a short mathematical 
overview of the basic plan of GCT,  
which is elaborated in the next two lectures. 


\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes}
      \label{fig:complexityclasses}
\end{figure} 




\noindent {\em Acknowledgement:} The author is grateful to 
Avi Wigderson for arranging the lectures and the hospitality,
to the authors of \cite{boris} for pointing out weakness of the 
lower bound stated during the lectures, and to Shrawan Kumar for
bringing the reference \cite{ariki} to his attention.




\chapter{Basic plan} 
We now outline the basic  plan of GCT focussing on
the  permanent vs. determinant problem in characteristic zero. 

\section{Characterization by symmetries} \label{scharsym}
We begin by observing that 
the permanent and the determinant are 
{\em exceptional} polynomial functions. By exceptional we mean
that they are  completely characterized by the symmetries in the 
following sense.


Let  $Y$ be a variable $m\times m$ matrix.
Let $\sym^m(Y)$ be the space of homogeneous forms of degree $m$ 
in the $m^2$ variable entries of $Y$. Then, by the  classical
representation theory,  $\det(Y)$ is the only form in $\sym^m(Y)$ 
such that, for any $A,B \in GL_m(\C)$ with $\det(A)\det(B)=1$, 

\noindent  {\bf (D):} $\det(Y)=\det(A Y^* B)$,

where $Y^*=Y$ or $Y^t$. 
Thus $\det(Y)$ is completely characterized 
by its symmetries, and hence, is  exceptional. We shall refer 
to this characteristic property of the determinant as property (D)
henceforth.

Similarly, $\perm(X)$ is the only form 
in the space of forms of degree $n$ in the entries of $X$ such that, 
for any diagonal or permutation matrices $A,B$,

\noindent  {\bf (P):} $\perm(X)=\perm(AX^*B)$, 

where $X^*=X$ or $X^t$  with obvious constraints 
on the product of the diagonal entries of $A$ and $B$ when they are diagonal.
Thus $\perm(X)$ is also
completely characterized   by its symmetries, and hence, is
exceptional.
We shall refer 
to this characteristic property of the permanent as property P
henceforth.





Any proof technique for the permanent vs. the determinant problem
has to ultimately make a nontrivial use of these  symmetries
  which characterize them. Indeed, one can say that 
these characteristic  properties 
lie at the heart of the permanent vs. determinant problem, and until
a proof technique has made a nontrivial use of them, it has
not entered the heart of the problem.
The most obvious interpretation of the phrase 
nontrivial here is the following: 

\begin{defn} \label{dnontrivial}
We say that a proof technique for the permanent vs. determinant 
problem makes a {\em nontrivial use of symmetries} if it does not work
for any functions (in place of the permanent or the determinant)
which do not have
nontrivial symmetries.
\end{defn}

Since symmetries is a fundamental geometric concept, we define
a  {\em geometric} approach to the permanent vs. determinant problem as
any  approach based on nontrivial use of the symmetry properties
(P) and (D) in this sense.
The meaning of the phrase geometric in the 
$P$ vs. $NP$ problem is
similar, since the  permanent and the determinant
can be replaced with   (co)-NP
and $P$ complete functions which are similarly
characterized by symmetries [GCT1]
(in a weaker sense that is good enough for our purposes).

GCT is a geometric approach in this sense.
Representation theory and 
algebraic geometry enter inevitably into  it, because
to understand symmetries, representation theory (of groups of symmetries)
becomes indispensible, and to understand  deeper properties 
of representations,  algebraic geometry becomes indispensible. 


\section{A mathematical form of the  $\#P \not = NC$ conjecture} 
\label{sweaklec1}
Before going any further, we now state one concrete application of 
GCT in the form of a concrete lower bound result--namely a 
mathematical form of the 
$\#P \not = NC$ conjecture (Theorem~\ref{tgenweaklec1} below).

We begin by observing that 
the permanent vs. determinant conjecture clearly implies  that 
$\perm(X)$ of any $n \times n$ variable matrix $X$ can not be represented 
as an $NC$-computable polynomial in the traces of $\bar X^j$, $j \ge 0$,
$\bar X=B X C$
for any (possibly singular) $n\times n$ matrices $B$ and $C$, since
$X^j$ can be computed fast in parallel. This can be proved unconditionally.
In fact, something stronger.

\begin{prop}  \label{pweaklec1}
There do not exist (possibly singular) $n\times n$ complex
matrices $B$ and $C$  and a polynomial 
$e(w_0,\ldots, w_n)$ such that $\perm(X) = g(BXC)$, 
where $g(X)=e(\trace(X^0), \trace(X), \ldots, \trace(X^n))$. 
\end{prop}
This was referred to as 
the weak form of the $\#P$ vs. $NC$ problem in the original IAS lecture. 
The article \cite{boris} showed that this is too  weak 
by giving an  elementary
proof \cite{boris} for it that is naturalizable, i.e.,
which cannot cross the
natural proof barrier \cite{rudich} because it works for most functions in
place of the permanent. The proof technique of
the quadratic lower bound \cite{ressayre}
for the permanent is also naturalizable.

We now state a much more general lower bound, which
was not stated in the IAS lecture, and which does not have such 
a naturalizable proof. For that we need a definition.

\begin{defn} \label{dgenperm}
A polynomial function $p(X_1,\ldots,X_k)$ (of any degree)
in the entries of $k$ $n\times n$ variable matrices 
is called a  {\em generalized permanent} if it has exactly 
the same symmetries as that of the permanent; i.e.,
for all nonsingular $n\times n$ matrices $U_i$ and $V_i$, $i \le k$, 
\[ p(U_1 X_1 V_1,\ldots, U_k X_k V_k)=p(X_1,\ldots,X_k) 
\mbox{\ iff\ } \perm(U_i X V_i)=\perm (X) \quad \forall i.\] 
\end{defn}

A precise description of the symmetries of the permanent  is given
by the property (P). Hence, $U_i$ and $V_i$ above have to be permutation
or diagonal matrices (with obvious constraints on the product of their 
diagonal entries), or 
product of such matrices.
When $k=1$ and $n$ is arbitrary,
there is just one generalized permanent of degree $n$, namely
the usual permanent itself. 
At the other extreme, 
when $n=1$ and $k$ is arbitrary, every function in $k$ variables 
is a generalized permanent. 
For general  $n$ and $k$, almost any polynomial 
in $\perm(X_i)$'s, $i \le k$, is  a generalized permanent, but 
there are many others besides these.
For general degrees, 
the dimension of the 
space spanned by  generalized permanents can be  exponential
in $n$; cf. Section~\ref{sweak}. 
In general,  the space of generalized permanents has a highly nontrivial
structure that  is intimately linked  to some
fundamental problems of representation theory;
cf. Section~\ref{sweak} and  [GCT6].


The original nonuniform 
$\#P$ vs. $NC$  conjecture
implies the following. 

\noindent {\bf Implication of the nonuniform $\#P \not = NC$ conjecture:}

Any $\#P$-complete generalized permanent  $p(X_1,\ldots,X_k)$ of $\poly(n,k)$ 
degree cannot be expressed as an $NC$-computable polynomial function of the 
traces of  $\bar X_i^j$, $1 \le i \le k$, $j=\poly(n,k)$, where 
$\bar X_i=B_i X_i C_i$,  $i \le k$,  for any $n\times n$ complex (possibly
singular) matrices $B_i$ and $C_i$.

(Here $X_i^j$ are  clearly $NC$-computable).

When $n=1$ and $k$ is arbitrary, this is  equivalent 
to the original nonuniform $\#P \not = NC$ conjecture,
since then any polynomial in $x_1,\ldots, x_k$ is a generalized permanent,
and a polynomial function of  the traces of  $x_i$'s means any
polynomial in $x_1,\ldots,x_k$. This cannot be proved at present.
But the next case,  $n>1$ and $k$ arbitrary, can be:

\begin{theorem}[GCT1,2,6]

\noindent {\bf (A mathematical form of the  $\#P \not = NC$ conjecture)}
 \label{tgenweaklec1}

The implication above holds unconditionally for any $n>1$ and arbitrary $k$.

In fact, something stronger then holds. Namely, 
when  $n>1$ and $k$ is arbitrary, no generalized permanent $p(X_1,\ldots,X_k)$
can be expressed as a polynomial function of the traces of 
$\bar X_i^j$, $1 \le i \le k$, $j \ge 0$,  where 
$\bar X_i=B_i X_i C_i$,  $i \le k$,  for any $n\times n$ complex (possibly
singular) matrices $B_i$ and $C_i$.
\end{theorem}

When  $k=1$ and $p(X)$, $X=X_1$, is the usual permanent, this specializes to
Proposition~\ref{pweaklec1}.


We are calling this a mathematical form for two reasons. 
First, it needs  no restriction on the computational complexity of
$p(X_1,\ldots,X_k)$ or the polynomial in the traces.
Thus it is rather in the spirit of the classical result of Galois theory 
which says that a  polynomial  whose Galois group is not
solvable cannot be solved by any number of
radical operations, without any restriction on the number of such
operations. 
Second, observe that 
the permanent has two characteristic properties: 1) the property 
P (mathematical), and 2) $\#P$-completeness (complexity-theoretic). 
The usual complexity theoretic form of the $\#P\not = NC$ conjecture
is a lower bound for  all polynomial functions with 
the  $\#P$-completeness property, whereas the mathematical form 
is  a lower bound for all polynomial functions with the 
property (P).  In other words,  the complexity theoretic form
is associated with the $\#P$-completeness property of the
permanent and the mathematical form with 
the property (P). 




The result indicates that there is thus a chasm
between the two adjacent cases: $n=1$, $k$ arbitrary (the usual nonuniform
complexity theoretic $\#P \not = NC$ conjecture), and 
$n=2$, $k$ arbitrary (its mathematical form above). 
The complexity theoretic form is   much harder than the mathematical
form, and  a proof technique for the easier mathematical form
can be expected to give us a crucial insight into what is needed to prove 
the harder  complexity theoretic form.


For some specific
generalized permanents (cf. Section~\ref{sweak}), this result again has
an elementary naturalizable proof as in \cite{boris}.
It also has an elementary naturalizable proof for a generic 
generalized permanent, just as the fact that a generic polynomial is
hard to compute has an elementary naturalizable proof.
The nontrivial part of this 
result (which needs nonelementary proof) 
is that it holds for any generalized permanent.
Indeed the basic difference between the complexity theoretic 
and the mathematical  settings is
the following. The complexity theoretic  (i.e. the usual) $\#P \not = NC$
conjecture 
is complete in the sense 
that if it is proved for one $\#P$-complete function (say
the permanent), it automatically 
holds for all $\#P$-completeness functions (because
of the theory of $\#P$-completeness). But there is no such completeness
theory at the mathematical level. Hence, a mathematical
lower bound  for a specific 
generalized permanent, e.g., the permanent,
does not say anything about all (even $\#P$-complete)
generalized permanents. To get 
similar completeness,   the  mathematical
form of the $\#P\not = NC$ conjecture above  covers up this lack of 
completeness theory
at the mathematical level by proving a result for all polynomial functions
with property (P), not just a specific one. 
The articles \cite{boris,ressayre} suggest that without such completeness
a restricted weaker form of the $\#P\not =NC$ conjecture
may be  provable by  a naturalizable proof technique. 



In contrast, it may be conjectured that Theorem~\ref{tgenweaklec1} cannot 
be proved by a naturalizable technique. This is because 
the only thing that is common among  all generalized permanents is the
property (P).  Hence any proof of this result would be 
essentially  forced
to rely only on  this property like  its GCT proof (cf. Section~\ref{sweak}).
Any such proof automatically passes the natural proof 
barrier since it is easy to show that most functions do not
have property $P$ when $n>1$ and $k$ is arbitrary.
\ignore{It may be remarked that the algebraic degree barrier is not 
applicable in the permanent vs. determinant problem because both
permanent and determinant have the same degree. It is not applicable
in the context of Theorem~\ref{tgenweaklec1} as well for the same reasons.
Similarly, the relativization barrier is not applicable in the context
of the permanent vs. determinant problem because the $NC$-computation 
has been algebrized in it in the form of the determinant, and the
relativization barrier does not apply to such algebraic techniques 
(just as it does not apply to the proof of the 
$IP=PSPACE$ result).
The relativization barrier does not apply in the context of 
Theorem~\ref{tgenweaklec1} 
for the same reason. Thus it can be said that the proof technique of
Theorem~\ref{tgenweaklec1} crosses the
natural proof, algebraic degree (algebrization)
and relativization barriers simultaneously.

Ultimately, any approach to the $\#P \not = NC$ conjecture
is expected to prove some restricted
form of this conjecture, not necessarily Theorem~\ref{tgenweaklec1},
whose proof crosses these barriers simultaneously.
At present, we do not have any other lower bound  result of this kind.}



Though the statement of Theorem~\ref{tgenweaklec1} is elementary, its proof 
is nonelementary and is based on  some fundamental results 
in geometric invariant theory \cite{kempf,mumford} and
the results in GCT1 and 2 
based on these results. These nonelementary techniques
are needed to cope up with a highly nontrivial 
structure of the space of generalized permanents as 
explained in Section~\ref{sweak}. 




\section{From nonexistence to existence}
The rest of this lecture  outlines  the GCT approach to 
the general  permanent vs. determinant problem,
and then  points out 
the crucial steps in this plan which can be completely executed
for the   mathematical form  of the $\#P\not = NC$ conjecture above,
but which are conjectural at present for 
the general (i.e. complexity theoretic) permanent vs. determinant problem. 

The first  step 
(GCT1,2) is to reduce this nonexistence problem--i.e., that there is no
small linear representation  of the permanent as a determinant--to
an existence problem--specifically, to the problem of proving 
existence of a family $\{O_n\}$ of obstructions; 
cf. Figure~\ref{fig:firststep}.
Here an {\em obstruction} $O_n$ is a proof-certificate of
hardness of $\perm(X)$, $X$ an $n\times n$ variable matrix,
just as the Kurotowski minor is a proof-certificate of the nonplanarity of a 
graph.  Specifically,  it is some 
algebro-geometric-representation-theoretic gadget
whose existence for every $n$  serves as a 
guarantee that $\perm(X)$ cannot be represented linearly as $\det(Y)$,
when $m=2^{\log^a n}$, $a>0$ fixed, $n\rightarrow \infty$ (i.e., for
$n$ greater than a large enough constant depending on $a$). 



\begin{figure} 
\begin{center}\psfragscanon
\psfrag{on}{$\{O_n\}$}
\epsfig{file=firststep.eps, scale=.8}
\end{center}
      \caption{Reduction from nonexistence to existence}
      \label{fig:firststep}
\end{figure}



This reduction to existence is carried out as follows (cf. lecture 2 for 
details).


First, we associate (GCT1) with 
the complexity class $\#P$ a family $\{X_{\#P}(n,m)\}$ of (group-theoretic)
class varieties (what this means is explained below),
and with the complexity class $NC$ a family of 
$\{X_{NC}(n,m)\}$ of (group-theoretic) class varieties such that: 
if $\perm(X)$, $\dim(X)=n$, can be represented linearly 
as $\det(Y)$, $\dim(Y)=m>n$, then 

\begin{equation} \label{eqembed} 
X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation} 

Each  class variety is a  (projective) algebraic variety, by which
we mean that it is the zero set of  a system of multivariate 
homogeneous polynomials with coefficients in $\C$  (akin to the 
usual curves  and surfaces). It is  group-theoretic in the 
sense that it is  constructed using group-theoretic operations 
and the general linear group $G=GL_l(\C)$, $l=m^2$, of $l\times l$ invertible
complex matrices acts on it, and furthermore the groups of
symmetries of the permanent and the determinant are embedded in this group
in some way. Here action means moving the points 
of the class variety around, just as $G$ moves the points of $\C^l$ around 
by the standard action via invertible linear transformations.
The goal is to show that the inclusion (\ref{eqembed}) is impossible
(obstructions are meant to ensure this);
cf. Figure~\ref{fig:class}. 

\begin{figure} 
\begin{center} \psfragscanon
\psfrag{xsharp}{$X_{\#P}(n,m)$}
      \psfrag{xnc}{$X_{NC}(n,m)$}
      \psfrag{g}{$G=GL_l(\C)$, $l=m^2$}
      \psfrag{Obstruction}{\mbox{Obstruction}}
\epsfig{file=class.eps, scale=.5}
\end{center}
      \caption{Class varieties}
      \label{fig:class}
\end{figure} 



Since each class variety has a $G$-action, the space of polynomial functions 
on each class variety has a  representation-theoretic structure, which 
puts constraints on which  representations of $G$ can live on that variety
(i.e., in the space of polynomial  functions on that variety).
Informally, an obstruction is an irreducible (minimal)  representation of $G$
that can live on $X_{\#P}(n,m)$ but not on $X_{NC}(n,m)$; 
cf. Figure~\ref{fig:class}.
Existence of  an obstruction $O_n$, for every $n$, assuming
$m=2^{\log^a n}$, $a>1$ fixed, implies  that the inclusion (\ref{eqembed}) 
is not possible, since  $O_n$ cannot live  on $X_{NC}(n,m)$.
Thus  an obstruction blocks the inclusion (\ref{eqembed}).


To define an obstruction formally, we need to recall some basic representation
theory.  By a classical result of Weyl, the irreducible 
(polynomial) representations of $G=GL_l(\C)$ are in one-to-one correspondence 
with the partitions  $\lambda$ of length  at most $l$, by which we mean 
integral sequences $\lambda_1 \ge 
\lambda_2 \cdots \ge \lambda_k > 0$, $k \le l$,
where  $k$ is called the  length
of $\lambda$. The irreducible 
representation of $G$ in correspondence with $\lambda$ is denoted 
by $V_\lambda(G)$, and is called the {\em Weyl module} of $G$ indexed by 
$\lambda$. Symbolically:

\[\mbox{Irreducible representations of } G \stackrel{\mbox{Weyl}}{\Longleftrightarrow} \quad \mbox{partitions} \ \lambda. \]  

\[\mbox{Weyl module  } V_\lambda(G)  \longleftrightarrow \lambda. \] 
Weyl also proved that every finite dimensional representation of $G$ 
can be decomposed into irreducible representations--i.e.,
can be written as a direct sum of Weyl modules. Thus Weyl modules 
are the basic building blocks of the representation theory of 
$G$, and every finite dimensional representation of $G$ can be thought
of as a complex building made out of these blocks. 


Now suppose $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$. 
Suppose to the contrary that 

\begin{equation} \label{eqembed2}   X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation}

Let $R_{\#P}(n,m)$ denote the homogeneous coordinate ring of 
$X_{\#P}(n,m)$; i.e., the ring of polynomial functions 
\footnote{Though the  functions here are not functions in usual sense;
but let us  not worry about this} on $X_{\#P}(n.m)$. 
Let $R_{\#P}(n,m)_d$ be the degree-$d$-component of $R_{\#P}(n, m)$ consisting
of functions of degree $d$. We define $R_{NC}(n,m)$ and $R_{NC}(n,m)_d$
similarly. Since $X_{\#P}(n,m)$ has the action of $G$, $R_{\#P}(n,m)$ 
also has an action of $G$; i.e., it is a representation of $G$. Hence,
$R_{\#P}(n,m)_d$ is a finite dimensional representation of $G$. 
Similarly, $R_{NC}(n,m)$ is a representation of $G$, and $R_{NC}(n,m)_d$
a finite dimensional representation of $G$. 



If (\ref{eqembed2}) holds, then we get a natural map from $R_{NC}(n,m)$ to
$R_{\#P}(n,m)$ obtained by restricting a function on $X_{NC}(n,m)$ to
$X_{\#P}(n,m)$. %; cf. Figure~\ref{fig:restriction}.
By basic algebraic geometry, this map
is surjective and is a $G$-homomorphism.
Furthermore, it is degree-preserving. This means there
is a surjective $G$-homomorphism from $R_{NC}(n,m)_d$ to 
$R_{\#P}(n,m)_d$. Symbolically: 

\begin{equation} \label{eqsurjection}
R_{\#}(n,m)_d \leftarrow  R_{NC}(n,m)_d.
\end{equation}

\ignore{
\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{Xp}{\small $X_{\#P}(n,m)$}
\psfrag{Xnc}{\small $X_{NC}(n,m)$}
\epsfig{file=restriction.eps, scale=.6}
\end{center}
      \caption{Restriction}
      \label{fig:restriction}
\end{figure}
}

Let $R_{\#P}(n,m)_d^*$ denote the dual of $R_{\#P}(n,m)_d$; i.e., the 
set of linear maps from $R_{\#P}(n,m)_d$ to $\C$. Then (\ref{eqsurjection})
implies that there is an injective $G$-homomorphism from 
$R_{\#P}(n,m)^*_d$ to $R_{NC}(n,m)^*_d$. Symbolically: 

\begin{equation} \label{eqinclusion}
R_{\#}(n,m)_d^*  \hookrightarrow {NC}(n,m)_d^*.
\end{equation}

\begin{defn} (GCT2)
An obstruction $O_n$ is a Weyl module $V_\lambda(G)$ that 
occurs as a subrepresentation 
in $R_{\#P}(n,m)_d^*$  but not in $R_{NC}(n,m)_d^*$, for some $d$. 
We call $\lambda$ an {\em obstruction label}, and sometimes,
by abuse of notation, an obstruction as well.

A strong obstruction $O_n$ is a Weyl module $V_\lambda(G)$ 
that occurs as a subrepresentation in $R_{\#P}(n,m)_d^*$ but 
does not contain a nonzero 
invariant (fix point) of the group of the symmetries 
of the determinant.
\end{defn}

Here recall that the group of the symmetries of the determinant 
is embedded in $G$ as its subgroup, which we shall refer to as $G_{det}$.
By an invariant we mean a point in $V_{\lambda}(G)$ 
which is fixed (does not move) with respect to the action of this subgroup
$G_{det} \subseteq G$ of symmetries.

\begin{prop} (GCT2)

\noindent (a) 
Existence of an obstruction $O_n$, for all $n\rightarrow \infty$, 
with $m=2^{\log^a n}$, $a>1$ fixed, implies $\perm(X)$, $\dim(X)=n$, 
cannot be represented linearly as 
$\det(Y)$, $\dim(Y)=m$. 

\noindent (b) A strong obstruction is an obstruction. Hence (a) 
also holds for a strong obstruction.
\end{prop}

Here (a)  follows just from the definition of an obstruction, and 
leads to:

\begin{goal} \label{gobs} (GCT2)
Prove existence of a (strong) 
obstruction family $\{O_n=V_{\lambda_n}(G)\}$ using 
the  exceptional 
nature of $\perm(X)$ and $\det(Y)$, i.e., using the 
properties (P) and (D) in  Section~\ref{scharsym}).
\end{goal} 

\section{Obstructions for the mathematical form} \label{sobsweak}

The following result achieves this goal for the mathematical form
(Theorem~\ref{tgenweaklec1}).
\begin{theorem} 
There exists a (strong)  obstruction family $\{O_n\}$ for the mathematical
form  of the $\#P \not = NC$ conjecture.
\end{theorem}

This implies Theorem~\ref{tgenweaklec1}.
The notion of obstructions here is similar 
to the one in the general case. 

The proof of this result  based on the results of GCT1 and 2 in
geometric invariant theory \cite{mumford} is outlined in the third lecture.
It produces  a 
family $\{O_n=V_\lambda(G)\}$ of (strong) obstructions, with a different $G$
than in the general complexity theoretic case.
Furthermore this family  is {\em strongly explicit} in the sense  that 
the specification $\lambda_n$ of each $O_n$
has polynomial, in fact,  $O(n)$ bitlength, and  
can be constructed in polynomial, in fact, $O(n)$ time (regardless of the 
complexity  of the polynomial in the traces in the statement of 
Theorem~\ref{tgenweaklec1}).

\noindent {\em Remark:}
There is also a second nonconstructive proof of this result 
(cf. Section~\ref{sweak}).
This gives a concrete evidence 
that explicit construction is not needed to cross the 
natural proof   barrier. Because 
any proof that relies only on the property (P) automatically
bypasses this barrier, as remarked before.
But   this nonconstructive
proof is not any easier than the explicit proof.
Indeed, the whole proof
structure  here is such that its easiest implementation  yields 
obstructions explicitly 
whether one cares for them or not. We shall see the same phenomenon
in the general case in what follows.


\section{Towards existence of obstructions in general via positivity}
We now proceed to describe the main results of GCT for the general
(complexity-theoretic)
permanent vs. determinant problem in the context of
Goal~\ref{gobs}. 



Towards that end, we  define 
certain representation-theoretic {\em stretching} functions. 
Let $F_{\lambda,n,m}(k)$ denote the number of occurences (multiplicity)  of
the Weyl module $V_{k\lambda}(G)$ in $R_{\#P}(n,m)^*$ (i.e. 
$R_{\#P}(n,m)^*_d$, for some $d$)  as a subrepresentation.
Let $G_{\lambda,m}(k)$ denote the multiplicity of the trivial one dimensional
representation (invariant) of $G_{det} \subset G$ in 
$V_{k\lambda}(G)$. In other words, $G_{\lambda,m}(k)$ is the dimension
of the subspace of invariants of $G_{det}$ in $V_{k \lambda}(G)$.
These are statistical functions
associated with the class variety $X_{\#P}(n,m)$ 
and the subgroup embedding  $G_{det} \hookrightarrow  G$.
In the first case,  the statistics associates 
with every number (stretching parameter) $k$  
the multiplicity of the corresponding
Weyl module $V_{k\lambda}(G)$ in $R_{\#P}(n,m)^*$;
cf. Figure~\ref{fig:statistics}.

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{l}{$\lambda$}
\psfrag{2l}{$2 \lambda$}
\psfrag{3l}{$3 \lambda$}
\psfrag{v1}{$V_\lambda(G)$}
\psfrag{v2}{$V_{2 \lambda}(G)$}
\psfrag{v3}{$V_{3\lambda}(G)$}
\epsfig{file=statistics.eps, scale=1}
\end{center}
      \caption{statistics}
      \label{fig:statistics}
\end{figure}


Let us  call a function $f(k)$ {\em quasipolynomial}, if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k)$ for all nonnegative integral $k=i$ modulo $l$;
here  $l$ is
called the period of the  quasi-polynomial. 
Thus  quasi-polynomials
are hybrids of  polynomial and periodic functions. 
We say that $f(k)$ is an 
{\em asymptotic quasipolynomial} if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k)$ for all nonnegative integral $k=i$ modulo $l$ for 
$k\ge a(f)$, for 
some nonnegative integer depending on $f$. The minimum 
$a(f)$ for which this holds is called the {\em deviation from 
quasipolynomiality}. Thus $f(k)$ is a (strict) quasipolynomial when this
deviation is zero.

A fundamental example of a quasi-polynomial is the Ehrhart quasi-polynomial
$f_P(k)$ of a polytope $P$ with rational vertices. It is defined
to be the number of integer points in the dilated polytope $kP$. By the 
classical result of Ehrhart, it is known to be a quasi-polynomial.
More generally, let $P(k)$ be a polytope parametrized by nonnegative
integral $k$: i.e., 
defined by a linear system of the form: 
\begin{equation} \label{eqpara}
A x \le k b + c,
\end{equation}
where $A$ is an $m \times n$ matrix, $x$ a variable $n$-vector, and 
$b$ and $c$ some constant $m$-vectors. Let $f_P(k)$ be the number 
of integer points in $P(k)$.  It is known to be  an asymptotic
 quasi-polynomial. We shall call it the asymptotic 
Ehrhart quasi-polynomial  of the parametrized polytope $P(k)$. 
In what follows, we  denote a parametrized polytope $P(k)$ by 
just $P$. 
From the context it should be clear whether $P$ is a usual nonparametrized 
polytope or a parametrized polytope.









\begin{theorem} (GCT6) \label{tquasi}

\noindent (a) The  function $G_{\lambda,m}(k)$ is a quasi-polynomial.


\noindent (b) The function $F_{\lambda,n,m}(k)$ is 
an asymptotic quasi polynomial.

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem} 


The proof of Theorem~\ref{tquasi} is based on:
\begin{enumerate} 
\item The classical work of Hilbert in invariant theory, 
\item The 
resolutions of singularities in characteristic zero
\cite{hironaka}: 
this  roughly says 
that the singularities of any algebraic variety in characteristic zero
can be untangled (resolved) nicely in a systematic fashion; cf.
 Figure~\ref{fig:resolution}.
\item Cohomological works of Boutot, Brion,  Flenner, Kempf  and others
based on this resolution; cf.  \cite{boutot,dehy} and
GCT6 for the history and other references.
\end{enumerate} 


\begin{figure} 
\begin{center} 
\epsfig{file=resolution.eps, scale=.5}
      \caption{Resolution}
      \label{fig:resolution}
\end{center}
\end{figure}


As such, this proof is highly nonconstructive. It gives no effective
bound on the period $l$--it just says that $l$  is finite.

\noindent {\em Remark:} 
The original IAS lecture   stated a conditional form of (b),
which said that $F_{\lambda,n,m}(k)$ is a quasi-polynomial if the
singularities of the class variety $X_{\#P}(n,m)$ are rational and normal 
(in some algebro-geometric sense). 
Recently, Shrawan Kumar  \cite{shrawan}  has shown that 
the singularities of $X_{\#P}(n,m)$ are not normal in general. This means 
$F_{\lambda,n,m}(k)$ in general need not be  a quasi-polynomial and 
asymptotic quasi-polynomiality as in  (b) is all that we can expect.
Though this complicates the situation mathematically, 
it makes no essential difference  in the complexity theoretic sense 
as long as the singularities of $R_{\#P,m}$ are not too bad 
in the sense described in Remark 3  after Hypothesis~\ref{hph1} below.

The following hypothesis 
says that $G_{\lambda,m}(k)$  can be realized as the Ehrhart quasi-polynomial
of a polytope, and 
$F_{\lambda,n,m}(k)$ 
can be realized as the asymptotic Ehrhart quasi-polynomial 
of a parametrized  polytope.

\begin{hypo} {\bf (PH) [Positivity Hypothesis]} \label{hph} (GCT6)

\noindent (a) For every $\lambda,n,m\ge n$, 
there exists   a parametrized  polytope $P=P_{\lambda,n,m}(k)$ 
such that 
\begin{equation} \label{eqP}
F_{\lambda,n,m}(k)=f_P(k).
\end{equation} 
It is also assumed here that there exists for $P_{\lambda,n,m}$ a specification
of the form (\ref{eqpara}),
 where $A$ is independent of $\lambda$, and $b$ and $c$ 
are  piecewise homogeneous linear functions of $\lambda$.


\noindent (b) For every $m$, there exists a (usual nonparametrized) 
polytope  $Q=Q_{\lambda,m}$  such that
\begin{equation} \label{eqQ}
G_{\lambda,m}(k)=f_Q(k).
\end{equation}
It is assumed here that there exists for $Q_{\lambda,m}$ a specification
of the form (\ref{eqpara}),
 where $A$ is independent of $\lambda$, and $b$ is 
is a  piecewise homogeneous linear function of $\lambda$ 
(since $Q$ is nonparametrized $c=0$.).



Analogous positivity hypothesis also holds 
for the $P$ vs. $NP$ problem in characteristic zero.
\end{hypo} 



If such $P$ and $Q$ exist, their dimensions are guaranteed to be
small by the proof of Theorem~\ref{tquasi}: specifically,
the dimension $P$ is guaranteed to be bounded by a 
polynomial in $n$, and the dimension of $Q$ 
by a polynomial in $n$ (but independent 
of $m$), if the length of $\lambda$ is $\poly(n)$ (as it would be in 
our applications).






When PH holds, we say that $F_{\lambda,n,m}(k)$ and 
$G_{\lambda,m}(k)$ have  {\em positive convex representations}. 
Here positivity refers to the fact that the Ehhart function 
$f_P(k)$ is a positive expression:
\[ f_P(k)=\sum_{v} 1,\] 
where $v$ ranges over all integer points in $P(k)$--there are no 
alternating signs in this expression.
Convexity refers to the  convexity of the polytopes $P(k)$ and $Q$. 


But, a  priori, it is not at all clear why PH should  even hold. 
Many numerical functions in mathematics are quasi-polynomials 
or asymptotic quasi-polynomials (e.g., the Hilbert function 
\footnote {Hilbert function $h_Z(k)$ of a projective algebraic variety $Z$
is defined to be $\dim(R(Z)_k)$, where $R(Z)$ is the homogeneous coordinate 
ring of $Z$ and $R(Z)_k$ its degree $k$-component.} of any projective
variety), but they rarely have positive convex representations.
PH is expected to hold 
because of the exceptional nature of the determinant and the permanent. 
For concrete  mathematical evidence and justification, see  GCT6,7, and 8. 


The hypothesis 
PH alone is not sufficient to prove the existence of obstructions.
The precise statement of a sufficient condition is given in 
the theorem below.




\begin{theorem} (GCT6) \label{tgct6}
There exists a family $\{O_n\}$ of (strong) obstructions 
for the  $\#P$ vs. $NC$ problem in characteristic zero, 
for $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$, 
assuming, 

\begin{enumerate} 
\item PH, and
\item OH (Obstruction Hypothesis): 

For all $n\rightarrow \infty$,  there exists $\lambda$ such that 
$P_{\lambda,n,m}(k) \not = \emptyset$ for all large enough $k$ and
$Q_{\lambda,m}=\emptyset$.
\end{enumerate}

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem}

Mathematical evidence and arguments in support of OH are given in GCT6.
The analogous OH that arises in the context of the mathematical form
of the $\#P\not = NC$ conjecture can be  proven unconditionally.

We call  $\lambda$ a {\em polyhedral  obstruction}
(or rather, polyhedral  obstruction-label)
if it satisfies OH. In this case, $k\lambda$, for some integer $k\ge 1$ is
a (strong)  obstruction--we just have to choose $k$ large enough 
so that 
$P_{\lambda,n,m}(k)$ contains an integer point.
Henceforth, whenever we say obstruction, we actually mean polyhedral
obstruction.

There is a fundamental difference between the nature of PH and OH.
PH is a {\em mathematical hypothesis}, because there is no 
constraint on what $m$ should be in comparison to $n$ in its statement.
In contrast, OH is a {\em complexity theoretic hypothesis}, because 
$m$ needs to be small in comparison to $n$ for it to hold.


%\subsection{Why should PH  and OH hold?} 

%Mathematical evidence for this is given in GCT2,4,6,7,8.
%We shall discuss some of this  in the third lecture.


\section{The flip: Explicit construction of obstructions} 
\label{sflip}
In principle PH may have a nonconstructive proof (like that
of Theorem~\ref{tquasi})  which only tells  that such polytopes 
exist without explicitly constructing them. But proving OH may not be feasible
unless the polytopes $P$ and $Q$ in PH are given explicitly.
This  suggests the following strategy for proving 
existence of obstructions proposed in  GCT6 and  GCTflip.


\noindent (1) Prove the following stronger explicit form 
of PH, which is reasonable since the polytopes $P$ and $Q$, if they exist,
are already guaranteed to be of small (polynomial) dimension:

\begin{hypo} {\bf (PH1)}  \label{hph1} (GCT6)

\noindent (a) There exists an {\em explicit} 
parametrized polytope $P_{\lambda,n,m}=P_{\lambda,n,m}(k)$ 
as in  PH (a).
Explicit means: 

\begin{enumerate}
\item  The polytope is specified by an explicit system of linear constraints,
where the bitlength of (the description of) 
each constraint is  $\poly(n,\bitlength{\lambda}, \bitlength{m})$.
Here and in what follows, $\bitlength{z}$ denotes the bitlength of the 
description of $z$.

\item  The membership problem for the polytope
$P_{\lambda,n,m}(k)$  also 
belongs to the complexity class $P$.
That is,  given a point $x$, whether it belongs to $P_{\lambda,n,m}(k)$ 
can also be decided in $\poly(\bitlength{x},\bitlength{\lambda},
n,\bitlength{m})$
time.
Furthermore, we assume that if $x$ does not belong to the polytope,
then the membership algorithm also gives a hyperplane separating 
$x$ from the polytope in the spirit of \cite{lovasz}. 
\end{enumerate} 

\noindent (b) There exists a similar  explicit 
(nonparametrized) polytope $Q_{\lambda,m}$  satisfying   PH (b)
with the polynomial bounds that 
depend on $n$ and the bitlength of $\lambda$, but not on $m$.
\end{hypo}

\noindent {\em Remark 1:} 
Note the occurrence of  $\bitlength{m}$  instead of $m$ in the polynomial
bounds in (a) (which implies that the bounds here become $\poly(n)$
when $m<2^n$ and $\bitlength{\lambda}=\poly(n)$), and the absence 
of $m$ in the polynomial bounds in (b), which means they again are 
$\poly(n)$ when  $\bitlength{\lambda}=\poly(n)$).
The reasons for this will be explained in Lecture 3 
(cf. remarks after Hypothesis~\ref{hph1restatement}). 



\noindent {\em Remark 2:} 
In particular, PH1 implies that the functions $F_{\lambda,n,m}(k)$ and
$G_{\lambda,m}(k)$ belong to the complexity class $\#P$. 

\noindent {\em Remark 3:} PH1 
also implies that the deviation from quasipolynomiality 
of $F_{\lambda,n,m}(k)$ is small, specifically, 
$2^{O(\poly(\bitlength{\lambda},n,\bitlength{m}))}$, i.e.,  the bitlength
of the deviation is polynomial.  As remarked after Theorem~\ref{tquasi},
this deviation would have been zero, i.e., $F_{\lambda,n,m}(k)$ would
have been a (strict) quasi-polynomial, if the singularities of the class
variety $X_{\#P}(n,m)$ were all normal and rational, which, as we know now,
is not the case \cite{shrawan}). So small deviation from quasi-polynomiality
implied by PH1 
basically means that the deviation from rationality and normality of
the singularities
of the class variety $X_{\#P}(n,m)$ is small (cf. Theorem~\ref{tquasi}).
This is the basic minimum that is required by PH1.


Like PH, PH1 is also a mathematical hypothesis in the sense that
it puts  no constraint on what $m$ should be in comparison to $n$. 
Of course, unlike PH, there is some complexity theoretic aspect to it, 
but it is secondary in comparison to the complexity-theoretic aspect of 
OH, since smallness  of $m$ with respect to  $n$ is the 
crux of the lower bound  problems under consideration. 





\noindent (2a) {\bf [The flip]}

Let $m=2^{\log ^a n}$, for a fixed $a>1$. 
Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
show existence of  an {\em explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of (polyhedral) obstructions  satisfying OH. 
We say that an obstruction (proof-certificate) 
$\lambda_n$ is {\em explicit} if is ``short'' and ``easy to verify'':


\begin{enumerate} 
\item  Short: This means its bitlength $\bitlength{\lambda_n}$ 
is $\poly(n)$,
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  

\item Easy to verify: given $n, m \le 2^{n}$ and 
$\lambda_n$, whether 
$\lambda_n$ is a valid obstruction 
can be verified 
in $\poly(n,\bitlength{\lambda})$ time. In particular, this is
$\poly(n)$ when $\bitlength{\lambda}=\poly(n)$. 
\end{enumerate}

Existence of an explicit family of obstructions is equivalent to saying
that the problem of deciding existence of polyhedral obstructions
for given $n$ and $m$ (in unary) 
belongs to $NP$--we shall refer to this decision problem as $DP(OH)$.
This definition of explicitness is quite natural since the class $NP$ 
is a class of problems whose proof-certificates (witnesses) are 
short and easy to verify. As such, the flip--going for 
explicit  obstructions--is
a proof-strategy that is literally given to us on a platter 
by the $P$ vs. $NP$ 
problem itself. Why it is called flip will be explained later.


It should be stressed that we are primarily interested in only proving 
existence of obstructions. Whether they are explicit or not 
does not really matter in the original statement of the problem.
But we need to know the polytopes $P$ and
$Q$ explicitly (as in PH1)  so that proving OH is feasible. 
%In other words,   if we do not
%even know what the polytopes $P$ and $Q$ look like, 
%it seems unlikely that anything  could be said regarding OH. 
But once  PH1 is proved, existence of an explicit family follows
automatically,   as a bonus, whether we care for it or not. 

To see why, let us observe that 
the second condition above  (ease of verification) follows directly
from PH1 and the polynomial time algorithm for 
linear programming on  polytopes given by separation oracles \cite{lovasz}. 
Shortness  also follows from PH1. 

Thus it is as if the $P$ vs. $NP$ problem is forcing us to go
for explicit obstructions.


\noindent (2b) {\bf [The strong flip (optional)]} 

Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
construct (rather than just show existence of) 
a {\em strongly explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of obstructions  satisfying OH. We say that an explicit family 
of obstructions is strongly explicit if,
for each $n$, a valid obstruction-label
$\lambda_n$ can be constructed in $\poly(n)$ time.
In particular, the height and the bitlength of
 $\lambda$ is $\poly(n)$ (short) 
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  


For the purposes of the lower bound problems that we are interested in, the
flip (just explicit  
existence) would suffice and the stronger flip (explicit construction)
is optional. But the stronger flip can give us deeper insight into these
lower bound problems; cf. GCTflip for more on this.

Now we turn to a few obvious questions.



\section{What has been achieved by all this?: The meaning of the flip} 
\label{smeaning}
Let us now see what has been achieved so far
in the context of the 
$\#P\not = NC$ conjecture in the nonuniform setting (characteristic zero),
the argument for the $P$ vs. $NP$ problem in characteristic zero
being  similar. 
At  first glance,
it may seem that all that GCT has achieved 
is to exchange a known difficult problem of 
complexity theory with a new very difficult problem of algebraic geometry.
In order to see that something is gained in exchange let us reexamine the 
original question.

The goal of the original  conjecture is to prove that 
$\perm(X)$, $\dim(X)=n$,  cannot be computed by an arithmetic circuit $C$
of size $m=\poly(n)$, or more generally,
$m \le 2^{\log^a n}$, for some fixed $a>1$, and depth $O(\log^a n)$.
Symbolically, 
let  $f_C(X)$ denote the function computed by $C$. Then we want to prove that
\begin{equation} \label{eqioh} 
 {\bf (IOH):}  \forall n \ge n_0 \forall C \exists X:
\perm(X)\not = f_C(X),
\end{equation} 
where $n_0$ is a sufficiently large constant.
For given $X$ and $C$ of $\poly(n)$ size, the problem 
of deciding if  $\perm(X) \not = f_C(X)$
belongs to  $P^{\#P}$.  Let $DP(IOH)$ denote the decision problem 
of deciding for given $n$ and $m$ (in unary) whether 
(\ref{eqioh}) holds.
Since there are two alternating layers of quantifiers in (\ref{eqioh}), it
belongs to $\Pi_2^{\#P}$, which is very high in the complexity hierarchy
(cf. Figure~\ref{fig:IOHcomplexity}).
Hence, we  refer to the original hypothesis (\ref{eqioh}) 
to be proven  as IOH 
(Infeasible Obstruction Hypothesis). Of course, IOH is expected to 
be a tautology, and hence (\ref{eqioh})
is expected to  be verifiable for small  $m=\poly(n)$ 
in $O(1)$ time--but
we do not know that as yet. 



\begin{sidewaysfigure} 
\begin{center}
\psfragscanon
\psfrag{sigma2p}{{\small $\Pi^2 \#P$}}
\psfrag{sigma1p}{$\Sigma^1 \#P$}
\psfrag{P}{{\small $P$}}
\psfrag{NP}{{\small $NP$}}
\psfrag{T}{$T$}
\psfrag{#P}{$\# P$}
\psfrag{inNP}{$DP(OH) \in NP$}
\psfrag{inP}{$DP(POH) \in P$}
\psfrag{insigma2p}{$DP(IOH) \in \Pi^2 \#P$}
\psfrag{PHplus}{PH1}
\psfrag{PHtil}{$PH^\dagger$}
\epsfig{file=IOHcomplexity.eps, scale=.8}
\end{center}
      \caption{Positivity as a means to eliminate the quantifiers and 
reduce the complexity of the  decision problem associated 
with the obstruction hypothesis}
      \label{fig:IOHcomplexity}
\end{sidewaysfigure}



Equivalently, the goal of IOH 
is to prove existence of a {\em trivial obstruction},
which is a table that lists for each $C$ as above a counterexample  $X$ so that
$\perm(X)\not = f_C(X)$; cf. Figure~\ref{fig:trivial}.
The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$ and depth
$O(\log^a n)$. Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. (Well, only
if the underlying field of computation is finite. For infinite fields, 
such as $\Q$ or $\C$ in this paper, 
there is another notion of a trivial obstruction (cf. 
GCT6). But let us imagine that the underlying
field is finite for this argument.)
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time to decide if such a table exists and construct 
one (optional) for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. That is why we 
call  this trivial, brute force 
strategy of proving IOH, based on existence of trivial obstructions,
an {\em infeasible strategy}. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{eq}{$\perm(X)\not = f_C(X)$}
\epsfig{file=trivial.eps, scale=.5}
\end{center}
      \caption{A trivial obstruction}
      \label{fig:trivial}
\end{figure}


In contrast, assuming PH1, $DP(OH)$, the decision 
problem  of deciding if a new polyhedral obstruction exists, belongs 
to $NP$ as we have already observed. Thus, assuming PH1, we have 
transformed the original decision problem for trivial obstructions
$DP(IOH) \in \Pi_2^{\#P}$ to the  decision problem for the  new polyhedral 
obstructions $DP(OH) \in NP$,
in the process bringing down the time to verify an obstruction
from  exponential (for the original trivial obstruction) to polynomial
(for the new polyhedral obstruction); cf. Figure~\ref{fig:IOHcomplexity}.  
It is crucial here that PH1, the main tool for this reduction, is a 
mathematical hypothesis,  not complexity-theoretic (cf. the remarks
after Theorem~\ref{tgct6} and Hypothesis~\ref{hph1}).
The task of verifying  an obstruction has also been 
transformed from the infeasible (exponential-time) to the feasible 
(polynomial-time). Hence the name of this strategy: the flip,
from the infeasible to the feasible.
Positivity (PH1) is used in the flip as a means  to
eliminate the quantifying variables in IOH and bring down the 
complexity of the decision problem associated with the obstruction hypothesis;
cf. Figure~\ref{fig:IOHcomplexity}. 




This process can be extended further. Assuming an additional
positivity hypothesis PH4 specified below,
$OH$, whose associated decision problem  $DP(OH)$ belongs to $NP$,
can be transformed 
to POH (Positivity Obstruction Hypothesis),  whose associated
decision problem $DP(POH) \in P$; i.e.,  whether a new obstruction 
exists can then be decided in polynomial time,
and if so, it can also be constructed in polynomial time; 
cf. Figure~\ref{fig:IOHcomplexity}. (The hypothesis is called PH4 instead
of PH2, because PH2 and PH3 are some other positivity hypotheses in GCT6
that complement PH1). 
Once this final positivity hypothesis POH is proven, the obstruction
hypothesis is reduced to a tautology (FOH: Final Obstruction Hypothesis),
which can be verified and constructed in
$O(1)$ time--i.e., the associated decision problem $DP(FOH)$ 
is $O(1)$-time solvable. This  would then give us 
the final $O(1)$-size  proof. 

Thus the basic idea of the flip is to use positivity systematically
as a means to eliminate the quantifiers  and reduce the complexity 
of the decision problem associated with 
the  obstruction hypothesis until 
the obstruction hypothesis  is finally 
reduced to  an $O(1)$-time verifiable  tautology;
cf. Figure~\ref{fig:IOHcomplexity}. 

Now let us specify PH4 and POH.
Towards that end, let  $k \le l=m^2$ be the length of $\lambda$.
Define 

\begin{equation} 
\begin{array}{l}
\bar P_{n,m}= \{ \lambda: P_{\lambda,n,m} \not = \emptyset \} \subseteq \C^k, \\
\bar Q_{m}= \{ \lambda: Q_{\lambda,m} \not = \emptyset \} \subseteq \C^k.
\end{array}
\end{equation}

\begin{theorem} 
The sets $\bar P_{n,m}$ and $\bar Q_{m}$ are convex polytopes in $\C^k$.
\end{theorem} 
This follows from some fundamental results in geometric invariant theory
\cite{mumford}. 

Then: 

\begin{hypo}  {\bf PH4} (GCT6)
The membership problems for these polytopes belong to 
$P$ and so also the problem of deciding if $\mbox{vol}(\bar P_{n,m}
\setminus \bar Q_{m})$, the volume of the relative complement 
$\bar P_{n,m} \setminus \bar Q_{m}$, is nonzero (positive);
i.e. if $\bar P_{n,m} \not \subseteq \bar Q_{m}$. By polynomial time,
we mean $\poly(n,l,\bitlength{m})$ time. This is $\poly(n)$,
if $m\le 2^{o(n)}$ and $l =\poly(n)$. 
\end{hypo}

\begin{hypo} {\bf (POH)}

For all $n\rightarrow \infty$, assuming $m=2^{\log^a n}$, $a>1$ fixed, 

\[ \mbox{vol}(\bar P_{n,m} \setminus \bar Q_{m}) > 0, \] 

for $k=(n+1)^2$. 
\end{hypo} 

\ignore{
Thus POH says that  the line-shaded area in Figure~\ref{fig:POH} has positive
volume for all large enough $n$. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{P}{$\bar P_{n,m}$}
\psfrag{Q}{$\bar Q_{n,m}$}
\epsfig{file=POH.eps, scale=1}
\end{center}
      \caption{POH}
      \label{fig:POH}
\end{figure}
}

\section{How to prove PH?}  \label{sphprove}
There is  a basic prototype of PH in representation theory,
which will be described in detail towards the end of Lecture 3. We shall
refer to it  as Plethysm PH. It says that the stretching functions 
akin to $F_{\lambda,n,m}(k)$ and $G_{\lambda,m}(k)$
associated with  fundamental  multiplicities 
in representation theory called plethysm constants also have analogous 
positive convex representations. 

This  is   known for a very special case of the plethysm constant 
called the  Littlewood-Richardson (LR) coefficient
$c_{\alpha,\beta}^\lambda$. It is  defined to be 
the number of occurences of the Weyl module $V_{\lambda}(G)$ in the 
tensor product of $V_{\alpha}(G)$ and $V_\beta(G)$. 
The classical Littlewood-Richardson rule, which we shall refer to as LR PH,
implies that the stretching function 
$\tilde c_{\alpha,\beta}^\lambda (k) = c_{k \alpha, k \beta}^{k \lambda}$
associated with the Littlewood-Richardson coefficient has a
positive convex representation.

Plethysm PH   happens to be a fundamental open problem of
representation theory, older than the $P$ vs. $NP$ problem itself. It 
has been studied intensively in the last century, and is known to be
formidable. And  now,  as explained the third lecture, it also turns out to 
be  the heart of this approach towards the $P$ vs $NP$, the
$\#P$ vs. $NC$ problems.



A basic plan to prove Plethysm PH is given in GCT6.
It is partially 
implemented in GCT7 and 8. See Figure~\ref{fig:lift} for a pictorial
depiction of the plan. It strives  to extend the  proof of LR PH based 
on the theory of the  standard quantum group \cite{drinfeld,kashiwara,lusztig}.
There it
comes out as a consequence of a  (proof of a) deep positivity result
\cite{kazhdan,lusztig}, which
we shall refer to as LR PH0. It says that   the 
tensor product of two representations of the standard quantum group 
has a canonical basis \cite{kashiwara,lusztig} 
whose structure coefficients are all positive \cite{lusztig}
polynomials (i.e., polynomials with nonnegative coefficients).
The only known proof of this
result is based on the Riemann Hypothesis over finite fields 
proved in \cite{weil2},  and the related works \cite{beilinson}. 
This Riemann Hypothesis over finite fields 
is  itself a deep positivity statement in mathematics,
from which   LR PH can  thus be 
deduced, as shown on the bottom row of Figure~\ref{fig:lift}.

If one were only interested in LR PH, one  does not 
need this  powerful machinery, because it has a  much simpler 
algebraic-combinatorial  proof. 
But the plan to extend the
proof of LR PH to Plethysm PH in GCT6,7,8 is like a huge
inductive spiral. To  make it work,  one  needs a 
stronger inductive hypothesis than Plethysm PH--this is precisely  Plethysm 
PH0 (which  will be
described in the third lecture; cf. Hypothesis~\ref{hplph0}).
Thus what is needed now 
is a systematic lifting  of the bottom arrow in Figure~\ref{fig:lift}
to the top, so as to complete the  commutative diagram, so to speak. 

Initial  steps in this direction have been taken in GCT7,8. 
First, GCT7 constructs a {\em nonstandard quantum group}, which
generalizes the notion of a standard quantum group \cite{drinfeld},
 and plays the
same role in the plethysm setting that the standard quantum group plays
in the LR setting. Second, GCT8 gives an algorithm to construct 
a canonical basis for a representation of the nonstandard quantum group
that is conjecturally correct and has the property Plethysm PH0,
which is a   generalization of LR PH0  supported by experimental
evidence.
Now what is needed to complete  the 
commutative diagram in Figure~\ref{fig:lift} is an appropriate nonstandard 
extension of the Riemann hypothesis over finite fields and the related works
\cite{beilinson,weil2,kazhdan,lusztig}
from which  Plethysm PH0 can be deduced. This--the top-right corner 
of the diagram--is the   main  open problem at the heart of this approach. 

\section{How to prove OH or POH?} 
We do not  know, 
since the  proof of OH and POH 
would really depend on the explicit forms of the
polytopes that arise in   PH1/PH4, and we have no idea about them
at this point.
GCT does suggest  that proving OH/POH  should be feasible 
``in theory'', i.e., {\em theoretically feasible}, 
since DP(OH)/DP(POH)  belong to NP/P, assuming PH1/4, and polynomial-time
is complexity theory stands for feasible ``in theory''. 
In other words,
GCT gives a reason to believe now that proving 
the  $P\not = NP$ conjecture should be theoretically feasible. Even this
was  always questioned  in the field of complexity theory so far, because 
the $P$ vs. $NP$ problem is a universal statement regarding all of mathematics
(that says theorems cannot be proven automatically).
But, as we also know by now, 
there is a huge gap between  theory and  practice--e.g., 
just because  some problem is in $P$ does not 
necessarily mean that it is feasible in practice. Similarly,
the actual implementation of the GCT flip via positivity is expected to be 
immensely difficult ``in practice'', as Figure~\ref{fig:lift} suggests. 







\section{Is positivity  necessary?} \label{sposnece}
\ignore{
Though the statement of this result is elementary, its proof is nonelementary,
as expected,  since the generalized permanents are highly nontrivial
and mathematically formidable objects. Specifically, the problem
of finding a $\#P$-basis for the space of generalized permanents 
is intimately related to some formidable problems of representation
theory and algebraic geometry,
and the  simplest analogue of this problem 
which can be solved at present  \cite{}
requires the deep Riemann Hypothesis over finite fields \cite{} for its
proof; cf. Section~\ref{}.
The proof of Theorem~\ref{} proceeds at an abstract level 
through algebraic geometry and representation theory without
having to know anything about such a basis.
At present, it is open if there is any alternative 
weaker form of the $\#P \not = NC$  conjecture,
which cannot be proved by relativizable, low-degree or 
naturalizable  techniques, but which can still be proved by elementary 
or not so  nonelementary techniques; that is, whether the earlier known
barriers mentioned above can 
be simultaneously bypassed in an elementary way in the context of 
the $\#P$ vs. $NC$ (or $P$ vs. $NC$  or $P$ vs. $NP$) problem.


\section{Why are we going for explicit obstructions?}
In a sense, the proof of the weak form turns out to be nonelementary
because of the difficulty of explicit construction. Specifically, algorithm 
to construct an obstruction $O_n$ for each $n$ is very simple, but to
show that it is correct requires nontrivial algebraic geometry,
just as the construction 
of an explicit family of Ramanujan graphs in \cite{} is very simple,
but to show that it is correct requires nontrivial algebraic geometry.
We already know, e.g. from this example of Ramanujan graphs, that 
explicit constructions can require highly nonelementary techniques.
So the question now arises: why are we going for such difficult explicit
constructions? Can they not be avoided somehow? 
After all, to solve the original problem we only need to show existence
of obstructions. We do not have to construct them explicitly.

Furthermore,  explicit construction is not needed to 
cross any of the barriers mentioned above (e.g. the natural-proof-barrier).
This is because {\em any} proof technique which uses symmetries of the
permanent would automatically bypass the natural-proof barrier
in the context of the permanent vs. determinant problem,
even if it does not utter a word about explicit construction, since
most functions have no symmetries. Indeed, the weak form of 
the generalized $\#P$ vs. $NC$ problem itself has two proofs, one
purely nonconstructive and one through explicit construction--the major 
chunk of both proofs being  the same, except for the last step,
which is carried out via a counting argument in the former proof and via
explicit construction in the latter. Since the nonconstructive proof too
is based on symmetries, it also crosses the natural-proof barrier.
This provides a concrete evidence that explicit construction is not 
necessary for crossing the earlier known  barriers.

Then why are we still going for explicit construction? 
Before we go any further, we wish to briefly state  the motivation
behind  going for the flip (explicit construction),
since this is an important issue. 
}

Finally,  if the positivity problems are so hard,  one may ask if 
they can not be avoided somehow. Unfortunately, there is a formidable 
barrier towards the $P$ vs. $NP$ and related problems, called the
{\em feasibility  barrier} \cite{GCTexplicit,GCTflip}
which is universal in the sense that
any approach towards these problems would have to tackle it, not just GCT. 
The flip, i.e., explicit construction of obstructions, is the most natural
and obvious way to cross this barrier, and it may well be 
among the easiest. The 
existing mathematical evidence suggests that any such natural approach
to cross this barrier would have to say  something deep regarding positivity
(Plethysm PH/PH0)  either explicitly or {\em implicitly}, even if
the approach does not utter a word about algebraic geometry or
representation theory.
That is,  Plethysm PH and PH0   may indeed be 
the heart of the  fundamental lower bound problems in complexity theory;
a detailed story and a precise meaning of the key 
phrase {\em implicit} would appear in the revised version of GCTflip.

%\input{feasibility}









































 

































\begin{sidewaysfigure} 
\begin{center} 
\epsfig{file=lift.eps, scale=.8}
\end{center}
      \caption{A commutative diagram}
      \label{fig:lift}
\end{sidewaysfigure} 



\ignore{\begin{figure} 
\psfragscanon
\psfrag{P}{$P\not = NP$ and $\#P\not = NC$ conjectures (characteristic zero)}
\epsfig{file=barriers.eps, scale=1}
      \caption{The feasibility barrier towards $P$ vs. $NP$}
      \label{fig:barriers}
\end{figure}}


%\input{lecture1_maintext}


==> lecture1_abs.tex <==
\section{Introduction}

This article   gives an overview of the basic plan of
geometric complexity theory (GCT), an
approach  towards the fundamental lower bound problems  in complexity theory, 
such as (Figure~\ref{fig:complexityclasses}):

\noindent (1) 
The $P$ vs. $NP$ problem \cite{cook,karp,levin}: 
 show that $P \not = NP$;


\noindent (2) 
The  $\#P$ vs. $NC$ problem \cite{valiant}: show that 
$\#P \not = NC$.

\noindent (3) The $P$ vs. $NC$ problem: show that $P \not = NC$.

We  focus here on only the nonuniform versions of these problems 
in characteristic zero; i.e., when
the underlying field of computation is of characteristic zero, 
say $\Q$ or $\C$.  The additional problems that
need to be addressed when the underlying field of computation is finite
would be discussed in  GCT11. 
The nonuniform
characteristic zero version of the $P\not = NC$ conjecture (in fact,
something stronger) was already proved  in GCTweak.
It may be considered to be the first unconditional lower bound result of
GCT, because, though it can be stated in purely elementary combinatorial
terms, being a formal implication of the $P\not = NC$ conjecture, its
proof is intrinsically geometric, and no elementary proof is known so far. 
Furthermore, its proof  technique may be considered to be a weak form 
of the {\em flip}, the basic guiding strategy of GCT, which  was 
refined and formalized much later in GCTflip. 
Hence we shall refer to this lower bound result
as the {\em weak form of the $P\not = NC$ 
conjecture}, and its proof technique as {\em weak GCT}. 
This  was the begining of  this  geometric approach in complexity theory.
The later work in GCT-- the subject of this overview--focusses on the other 
two problems above, namely
the $P$ vs. $NP$ and $\#P$ vs. $NC$ problems. 


The nonuniform (characteristic zero) version of the $\#P$ vs. $NC$ problem
is also known as the permanent vs. determinant problem \cite{valiant}. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented 
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$; 
the best known lower bound on $m$ at present is 
 quadratic \cite{ressayre}. %; cf. Figure~\ref{fig:matrices}. 
By linear representation, we mean
the  entries   of $Y$ are  (possibly nonhomogeneous) 
linear functions 
of the entries of $X$. 
There is an analogous characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.
The main results of GCT for the $\#P$ vs. $NC$ problem in 
characteristic zero also extend to the $P$ vs. $NP$ problem in characteristic
zero. But here we shall 
concentrate  on only the former problem,
%the
%$\#P$ vs. $NC$ problem in  characteristic zero (nonuniform),
since this illustrates all the basic ideas. 


\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes}
      \label{fig:complexityclasses}
\end{figure} 






%\chapter{Basic plan} 

\noindent {\em Remark:} The original  lectures also mentioned 
a certain weak form of the $\#P$ vs. $NC$ problem. Actually, the proof
technique here leads to a much more nontrivial result.
It is discussed in the second section of  the third lecture.

\noindent {\em Acknowledgement:} The author is grateful to 
Avi Wigderson for arranging the lectures and the hospitality.


In the rest of this article we  outline the basic  plan of GCT focussing on
the  permanent vs. determinant problem in characteristic zero. 
It is elaborated further 
in the next two lectures which can be found in the full overview.


\input{lecture1_maintext}

==> lecture1_maintext.tex <==
\chapter{Basic plan} 
We now outline the basic  plan of GCT focussing on
the  permanent vs. determinant problem in characteristic zero. Recall that
this  says  $\perm(X)$  cannot be represented 
linearly  as the determinant of a polynomial size 
matrix.


\section{Characterization by symmetries} \label{scharsym}
We begin by observing that 
the permanent and the determinant are 
{\em exceptional} polynomial functions. By exceptional we mean
that they are  completely characterized by the symmetries in the 
following sense.


Let  $Y$ be a variable $m\times m$ matrix.
Let $\sym^m(Y)$ be the space of homogeneous forms of degree $m$ 
in the $m^2$ variable entries of $Y$. Then, by the  classical
representation theory,  $\det(Y)$ is the only form in $\sym^m(Y)$ 
such that, for any $A,B \in GL_m(\C)$ with $\det(A)\det(B)=1$, 

\noindent  {\bf (D):} $\det(Y)=\det(A Y^* B)$,

where $Y^*=Y$ or $Y^t$. 
Thus $\det(Y)$ is completely characterized 
by its symmetries, and hence, is  exceptional. We shall refer 
to this characteristic property of the determinant as property (D)
henceforth.

Similarly, $\perm(X)$ is the only form 
in the space of forms of degree $n$ in the entries of $X$ such that, 
for any diagonal or permutation matrices $A,B$, 

\noindent  {\bf (P):} $\perm(X)=\perm(AX^*B)$, 

where $X^*=X$ or $X^t$ and the product of the (nonzero) 
diagonal entries of $A$ and $B$ is one.
Thus $\perm(X)$ is also
completely characterized   by its symmetries, and hence, is
exceptional.
We shall refer 
to this characteristic property of the permanent as property P
henceforth.





Any proof technique for the permanent vs. the determinant problem
has to ultimately make a nontrivial use of these  symmetries
  which characterize them. Indeed, one can say that 
these characteristic  properties 
lie at the heart of the permanent vs. determinant problem, and until
a proof technique has made a nontrivial use of them, it has
not entered the heart of the problem.
The most obvious interpretation of the phrase 
nontrivial here is the following: 

\begin{defn} \label{dnontrivial}
We say that a proof technique for the permanent vs. determinant 
problem makes a {\em nontrivial use of symmetries} if it does not work
for any functions (in place of the permanent or the determinant)
which do not have
nontrivial symmetries.
\end{defn}

Since symmetries is a fundamental geometric concept, we define
a  {\em geometric} approach to the permanent vs. determinant problem as
any  approach based on nontrivial use of the symmetry properties
(P) and (D) in this sense.
The meanining of the phrase geometric in the 
$P$ vs. $NP$ problem is
similar, since the  permanent and the determinant
can be replaced with   (co)-NP
and $P$ complete functions which are similarly
characterized by symmetries [GCT1]
(in a weaker sense that is good enough for our purposes).

GCT is a geometric approach in this sense.
Representation theory and 
algebraic geometry enter inevitably into  it, because
to understand symmetries, representation theory (of groups of symmetries)
becomes indispensible, and to understand  deeper properties 
of representations,  algebraic geometry becomes indispensible. 


\section{A mathematical form of the  $\#P \not = NC$ conjecture} 
\label{sweaklec1}
Before going any further, we now state one concrete application of 
GCT in the form of a concrete lower bound result--namely a 
mathematical form of the 
$\#P \not = NC$ conjecture (Theorem~\ref{tgenweaklec1} below).

We begin by observing that 
the permanent vs. determinant conjecture clearly implies  that 
$\perm(X)$ of any $n \times n$ variable matrix $X$ can not be represented 
as an $NC$-computable polynomial in the traces of $\bar X^j$, $j \ge 0$,
$\bar X=B X C$
for any (possibly singular) $n\times n$ matrices $B$ and $C$, since
$X^j$ can be computed fast in parallel. This can be proved unconditionally.
In fact, something stronger.

\begin{prop}  \label{pweaklec1}
There do not exist (possibly singular) $n\times n$ complex
matrices $B$ and $C$  and a polynomial 
$e(w_0,\ldots, w_n)$ such that $\perm(X) = g(BXC)$, 
where $g(X)=e(\trace(X^0), \trace(X), \ldots, \trace(X^n))$. 
\end{prop}
This was referred to as 
the weak form of the $\#P$ vs. $NC$ problem in the original IAS lecture. 
The article \cite{boris} showed that this is too  weak 
by giving an  elementary
proof \cite{boris} for it that is naturalizable, i.e.,
which cannot cross the
natural proof barrier \cite{rudich} because it works for most functions in
place of the permanent. The proof technique of
the quadratic lower bound \cite{ressayre}
for the permanent is also naturalizable.

We now state a much more general lower bound, which
was not stated in the IAS lecture, and which does not have such 
a naturalizable proof. For that we need a definition.

\begin{defn} \label{dgenperm}
A polynomial function $p(X_1,\ldots,X_k)$ (of any degree)
in the entries of $k$ $n\times n$ variable matrices 
is called a  {\em generalized permanent} if it has exactly 
the same symmetries as that of the permanent; i.e.,
for all nonsingular $n\times n$ matrices $U$ and $V$, 
\[ p(U X_1 V,\ldots, U X_k V)=p(X_1,\ldots,X_k) 
\mbox{\ iff\ } \perm(U X V)=\perm (X).\] 
\end{defn}

A precise description of the symmetries of the permanent  is given
by the property (P). Hence, $U$ and $V$ above have to be permutation
or diagonal matrices (with product of the nonzero  diagonal entries being
one), or 
product of such matrices.
When $k=1$ and $n$ is arbitrary,
there is just one generalized permanent of degree $n$, namely
the usual permanent itself. But for general degrees, 
the dimension of the 
space spanned by  generalized permanents can be  exponential
in $n$; cf. Section~\ref{sweak}. At the other extreme, 
when $n=1$ and $k$ is arbitrary, every function in $k$ variables 
is a generalized permanent. 
In general,  the space of generalized permanents has a highly nontrivial
structure that  is intimately linked  to some
fundamental problems of representation theory;
cf. Section~\ref{sweak} and  [GCT6].


The original nonuniform 
$\#P$ vs. $NC$  conjecture
implies the following. 

\noindent {\bf Implication of the nonuniform $\#P \not = NC$ conjecture:}

Any $\#P$-complete generalized permanent  $p(X_1,\ldots,X_k)$ of $\poly(n,k)$ 
degree cannot be expressed as an $NC$-computable polynomial function of the 
traces of arbitrary  monomials of polynomial length 
in $\bar X_i$, $1 \le i \le k$, where 
$\bar X_i=B X_i C$,  $i \le k$,  for any $n\times n$ complex (possibly
singular) matrices $B$ and $C$. Here by a monomial 
in $\bar X_i$ we mean
any matrix product  of the form $\bar X_{i_1}\ldots \bar X_{i_r}$, 
$1 \le i_1, \ldots  i_r \le k$.
We say that it is of polynomial length if 
$r=\poly(n,k)$ (it is then clearly $NC$-computable).

When $n=1$ and $k$ is arbitrary, this is  equivalent 
to the original nonuniform $\#P \not = NC$ conjecture,
since then any polynomial in $x_1,\ldots, x_k$ is a generalized permanent,
and a polynomial function of  the traces of monomials in $x_i$'s means any
polynomial in $x_1,\ldots,x_k$. This cannot be proved at present.
But the next case,  $n>1$ and $k$ arbitrary, can be:

\begin{theorem}[GCT6]

\noindent {\bf (A mathematical form of the  $\#P \not = NC$ conjecture)}
 \label{tgenweaklec1}

The implication above holds unconditionally for any $n>1$ and arbitrary $k$.

In fact, something stronger then holds. Namely, 
when  $n>1$ and $k$ is arbitrary, no generalized permanent $p(X_1,\ldots,X_k)$
can be expressed as a polynomial function of the traces of 
arbitrary  monomials in $\bar X_i$, $1 \le i \le k$, where 
$\bar X_i=B X_i C$,  $i \le k$,  for any $n\times n$ complex (possibly
singular) matrices $B$ and $C$.
\end{theorem}

When  $k=1$ and $p(X)$, $X=X_1$, is the usual permanent, this specializes to
Proposition~\ref{pweaklec1}.


We are calling this a mathematical form for two reasons. 
First, it is a mathematical
lower bound rather than a complexity theoretic lower bound in the sense
that it needs  no restriction on the computational complexity of
$p(X_1,\ldots,X_k)$ or the polynomial in the traces.
Thus it is rather in the spirit of the classical result of Galois theory 
which says that a general polynomial of degree $>5$ 
cannot be solved by any number of
radical operations, without any restriction on the number of such
operations. 
Second, observe that 
the permanent has two characteristic properties: 1) the property 
P (mathematical), and 2) $\#P$-completeness (complexity-theoretic). 
The usual complexity theoretic form of the $\#P\not = NC$ conjecture
is a lower bound for  all polynomial functions with 
the  $\#P$-completenes property, whereas the mathematical form 
is  a lower bound for all polynomial functions with the 
property (P).  In other words,  the complexity theoretic form
is associated with the $\#P$-completeness property of the
permanent and the mathematical form with 
the property (P). 




The result indicates that there is thus a chasm
between the two adjacent cases: $n=1$, $k$ arbitrary (the usual nonuniform
complexity theoretic $\#P \not = NC$ conjecture), and 
$n=2$, $k$ arbitrary (its mathematical form above). 
The complexity theoretic form is   much harder than the mathematical
form, and  a proof technique for the easier mathematical form
can be expected to give us a crucial insight into what is needed to prove 
the harder  complexity theoretic form.


For some specific
generalized permanents (cf. Section~\ref{sweak}), this result again has
an elementary naturalizable proof as in \cite{boris}.
It also has an elementary naturalizable proof for a generic 
generalized permanent, just as the fact that a generic polynomial is
hard to compute has an elementary naturalizable proof.
The nontrivial part of this 
result (which needs nonelementary proof) 
is that it holds for any generalized permanent.
Indeed the basic difference between the complexity theoretic 
and the mathematical  settings is
the following. The complexity theoretic  (i.e. the usual) $\#P \not = NC$
conjecture 
is universal in the sense 
that if it is proved for one $\#P$-complete function (say
the permanent), it automatically 
holds for all $\#P$-completeness functions (because
of the theory of $\#P$-completeness). But there is no such completeness
theory at the mathematical level. Hence, a mathematical
lower bound  for a specific 
generalized permanent, e.g., the permanent,
does not say anything about all (even $\#P$-complete)
generalized permanents. To get 
 similar universality,   the  mathematical
form of the $\#P\not = NC$ conjecture above  covers up this lack of 
completeness theory
at the mathematical level by proving a result for all polynomial functions
with property (P), not just a specific one. 
The articles \cite{boris,ressayre} suggest that without such universality
a restricted weaker form of the $\#P\not =NC$ conjecture
may be  provable by  a naturalizable proof technique. 



In contrast, it may be conjectured that Theorem~\ref{tgenweaklec1} cannot 
be proved by a naturalizable technique. This is because 
the only thing that is common among  all generalized permanents is the
property (P).  Hence any proof of this result would be 
essentially  forced
to rely only on  this property like  its GCT proof (cf. Section~\ref{sweak}).
Any such proof automatically passes the natural proof 
barrier since it is easy to show that most functions do not
have property $P$ when $n>1$ and $k$ is arbitrary.
It may be remarked that the algebraic degree barrier is not 
applicable in the permanent vs. determinant problem because both
permanent and determinant have the same degree. It is not applicable
in the context of Theorem~\ref{tgenweaklec1} as well for the same reasons.
Similarly, the relativization barrier is not applicable in the context
of the permanent vs. determinant problem because the $NC$-computation 
has been algebrized in it in the form of the determinant, and the
relativization barrier does not apply to such algebraic techniques 
(just as it does not apply to the proof of the 
$IP=PSPACE$ result).
The relativization barrier does not apply in the context of 
Theorem~\ref{tgenweaklec1} 
for the same reason. Thus it can be said that the proof technique of
Theorem~\ref{tgenweaklec1} crosses the
natural proof, algebraic degree (algebrization)
and relativization barriers simultanesouly.

Ultimately, any approach to the $\#P \not = NC$ conjecture
is expected to prove some restricted
form of this conjecture, not necessarily Theorem~\ref{tgenweaklec1},
whose proof crosses these barriers simultaneously.
At present, we do not have any other lower bound  result of this kind.



Though the statement of Theorem~\ref{tgenweaklec1} is elementary, its proof 
is nonelementary and is based on  some fundamental results 
in geometric invariant theory \cite{mumford} and the results in GCT1 and 2 
based on these results. These nonelementary techniques
are needed to cope up with a highly nontrivial 
structure of the space of generalized permanents as 
explained in Section~\ref{sweak}. 




\section{From nonexistence to existence}
The rest of this lecture  outlines  the GCT approach to 
the general  permanent vs. determinant problem,
and then  points out 
the crucial steps in this plan which can be completely executed
for the weaker  mathematical form  of the $\#P\not = NC$ conjecture above,
but which are conjectural at present for 
the general permanent vs. determinant problem. 

The first  step 
(GCT1,2) is to reduce this nonexistence problem--i.e., that there is no
small linear representation  of the permanent as a determinant--to
an existence problem--specifically, to the problem of proving 
existence of a family $\{O_n\}$ of obstructions; 
cf. Figure~\ref{fig:firststep}.
Here an {\em obstruction} $O_n$ is a proof-certificate of
hardness of $\perm(X)$, $X$ an $n\times n$ variable matrix,
just as the Kuratowski minor is a proof-certificate of the nonplanarity of a 
graph.  Specifically,  it is some 
algebro-geometric-representation-theoretic gadget
whose existence for every $n$  serves as a 
guarantee that $\perm(X)$ cannot be represented linearly as $\det(Y)$,
when $m=2^{\log^a n}$, $a>0$ fixed, $n\rightarrow \infty$ (i.e., for
$n$ greater than a large enough constant depending on $a$). 



\begin{figure} 
\begin{center}\psfragscanon
\psfrag{on}{$\{O_n\}$}
\epsfig{file=firststep.eps, scale=.8}
\end{center}
      \caption{Reduction from nonexistence to existence}
      \label{fig:firststep}
\end{figure}



This reduction to existence is carried out as follows (cf. lecture 2 for 
details).


First, we associate (GCT1) with 
the complexity class $\#P$ a family $\{X_{\#P}(n,m)\}$ of (group-theoretic)
class varieties (what this means is explained below),
and with the complexity class $NC$ a family of 
$\{X_{NC}(n,m)\}$ of (group-theoretic) class varieties such that: 
if $\perm(X)$, $\dim(X)=n$, can be represented linearly 
as $\det(Y)$, $\dim(Y)=m>n$, then 

\begin{equation} \label{eqembed} 
X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation} 

Each  class variety is a  (projective) algebraic variety, by which
we mean that it is the zero set of  a system of multivariate 
homogeneous polynomials with coefficients in $\C$  (akin to the 
usual curves  and surfaces). It is  group-theoretic in the 
sense that it is  constructed using group-theoretic operations 
and the general linear group $G=GL_l(\C)$, $l=m^2$, of $l\times l$ invertible
complex matrices acts on it. Here action means moving the points 
of the class variety around, just as $G$ moves the points of $\C^l$ around 
by the standard action via invertible linear transformations.
The goal is to show that the inclusion (\ref{eqembed}) is impossible
(obstructions are meant to ensure this);
cf. Figure~\ref{fig:class}. 

\begin{figure} 
\begin{center} \psfragscanon
\psfrag{xsharp}{$X_{\#P}(n,m)$}
      \psfrag{xnc}{$X_{NC}(n,m)$}
      \psfrag{g}{$G=GL_l(\C)$, $l=m^2$}
      \psfrag{Obstruction}{\mbox{Obstruction}}
\epsfig{file=class.eps, scale=.5}
\end{center}
      \caption{Class varieties}
      \label{fig:class}
\end{figure} 



Since each class variety has a $G$-action, the space of polynomial functions 
on each class variety has a  representation-theoretic structure, which 
puts constraints on which  representations of $G$ can live on that variety
(i.e., in the space of polynomial  functions on that variety).
Informally, an obstruction is an irreducible (minimal)  representation of $G$
that can live on $X_{\#P}(n,m)$ but not on $X_{NC}(n,m)$; 
cf. Figure~\ref{fig:class}.
Existence of  an obstruction $O_n$, for every $n$, assuming
$m=2^{\log^a n}$, $a>1$ fixed, implies  that the inclusion (\ref{eqembed}) 
is not possible, since  $O_n$ cannot live  on $X_{NC}(n,m)$.
Thus  an obstruction blocks the inclusion (\ref{eqembed}).


To define an obstruction formally, we need to recall some basic representation
theory.  By a classical result of Weyl, the irreducible 
(polynomial) representations of $G=GL_l(\C)$ are in one-to-one correspondence 
with the partitions  $\lambda$ of length at most $l$, by which we mean 
integral sequences $\lambda_1 \ge 
\lambda_2 \cdots \ge \lambda_k > 0$, $k\le l$, where  $k$ is called the  length
of $\lambda$. The irreducible 
representation of $G$ in correspondence with $\lambda$ is denoted 
by $V_\lambda(G)$, and is called the {\em Weyl module} of $G$ indexed by 
$\lambda$. Symbolically:

\[\mbox{Irreducible representations of } G \stackrel{\mbox{Weyl}}{\Longleftrightarrow} \quad \mbox{partitions} \ \lambda. \]  

\[\mbox{Weyl module  } V_\lambda(G)  \longleftrightarrow \lambda. \] 
Weyl also proved that every finite dimensional representation of $G$ 
can be decomposed into irreducible representations--i.e.,
can be written as a direct sum of Weyl modules. Thus Weyl modules 
are the basic building blocks of the representation theory of 
$G$, and every finite dimensional representation of $G$ can be thought
of as a complex building made out of these blocks. 


Now suppose $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$. 
Suppose to the contrary that 

\begin{equation} \label{eqembed2}   X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation}

Let $R_{\#P}(n,m)$ denote the homogeneous coordinate ring of 
$X_{\#P}(n,m)$; i.e., the ring of polynomial functions 
\footnote{Though the  functions here are not functions in usual sense;
but let us  not worry about this} on $X_{\#P}(n.m)$. 
Let $R_{\#P}(n,m)_d$ be the degree-$d$-component of $R_{\#P}(n, m)$ consisting
of functions of degree $d$. We define $R_{NC}(n,m)$ and $R_{NC}(n,m)_d$
similarly. Since $X_{\#P}(n,m)$ has the action of $G$, $R_{\#P}(n,m)$ 
also has an action of $G$; i.e., it is a representation of $G$. Hence,
$R_{\#P}(n,m)_d$ is a finite dimensional representation of $G$. 
Similarly, $R_{NC}(n,m)$ is a representation of $G$, and $R_{NC}(n,m)_d$
a finite dimensional representation of $G$. 



If (\ref{eqembed2}) holds, then we get a natural map from $R_{NC}(n,m)$ to
$R_{\#P}(n,m)$ obtained by restricting a function on $X_{NC}(n,m)$ to
$X_{\#P}(n,m)$. %; cf. Figure~\ref{fig:restriction}.
By basic algebraic geometry, this map
is surjective and is a $G$-homomorphism.
Furthermore, it is degree-preserving. This means there
is a surjective $G$-homomorphism from $R_{NC}(n,m)_d$ to 
$R_{\#P}(n,m)_d$. Symbolically: 

\begin{equation} \label{eqsurjection}
R_{\#}(n,m)_d \leftarrow  R_{NC}(n,m)_d.
\end{equation}

\ignore{
\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{Xp}{\small $X_{\#P}(n,m)$}
\psfrag{Xnc}{\small $X_{NC}(n,m)$}
\epsfig{file=restriction.eps, scale=.6}
\end{center}
      \caption{Restriction}
      \label{fig:restriction}
\end{figure}
}

Let $R_{\#P}(n,m)_d^*$ denote the dual of $R_{\#P}(n,m)_d$; i.e., the 
set of linear maps from $R_{\#P}(n,m)_d$ to $\C$. Then (\ref{eqsurjection})
implies that there is an injective $G$-homomorphism from 
$R_{\#P}(n,m)^*_d$ to $R_{NC}(n,m)^*_d$. Symbolically: 

\begin{equation} \label{eqinclusion}
R_{\#}(n,m)_d^*  \hookrightarrow {NC}(n,m)_d^*.
\end{equation}

\begin{defn} (GCT2)
An obstruction $O_n$ is a Weyl module $V_\lambda(G)$ that 
occurs as a subrepresentation 
in $R_{\#P}(n,m)_d^*$  but not in $R_{NC}(n,m)_d^*$, for some $d$. 
We call $\lambda$ an {\em obstruction label}, and sometimes,
by abuse of notation, an obstruction as well.
\end{defn}

\begin{prop} (GCT2)
Existence of an obstruction $O_n$, for all $n\rightarrow \infty$, 
with $m=2^{\log^a n}$, $a>1$ fixed, implies $\perm(X)$, $\dim(X)=n$, 
cannot be represented linearly as 
$\det(Y)$, $\dim(Y)=m$. 
\end{prop}

This follows just from the definition of an obstruction, and 
leads to:

\begin{goal} \label{gobs} (GCT2)
Prove existence of an obstruction family $\{O_n=V_{\lambda_n}(G)\}$ using 
the  exceptional 
nature of $\perm(X)$ and $\det(Y)$, i.e., using the 
properties (P) and (D) in  Section~\ref{scharsym}).
\end{goal} 

\section{Obstructions for the mathematical form} \label{sobsweak}

The following result achieves this goal for the mathematical form
(Theorem~\ref{tgenweaklec1}).
\begin{theorem} 
There exists an obstruction family $\{O_n\}$ for the mathematical
form  of the $\#P \not = NC$ conjecture.
\end{theorem}

This implies Theorem~\ref{tgenweaklec1}.
The notion of obstructions here is similar 
to the one in the general case. 

The proof of this result  based on the results of GCT1 and 2 in
geometric invariant theory \cite{mumford} is outlined in the third lecture.
It produces  a {\em strongly  explicit} 
family $\{O_n=V_\lambda(G)\}$ of obstructions, with a different $G$
than in the general complexity theoretic case.
This is strongly explicit in the sense (cf. Introduction) that 
the specification $\lambda_n$ of each $O_n$
has polynomial, in fact,  $O(n)$ bitlength, and  
can be constructed in polynomial, in fact, $O(n)$ time (regardless of the 
complexity  of the polynomial in the traces in the statement of 
Theorem~\ref{tgenweaklec1}).

\noindent {\em Remark:}
There is also a second noncostructive proof of this result 
(cf. Section~\ref{sweak}).
This gives a concrete evidence 
that explicit construction is not needed to cross the 
natural proof   barrier. Because 
any proof that relies only on the property (P) automatically
bypasses this barrier, as remarked before.
But   this nonconstructive
proof is not any easier than the explicit proof, in fact, a bit harder.
Indeed, the whole proof
structure  here is such that its easiest implementation  yields 
obstructions explicitly 
whether one cares for them or not. We shall see the same pheonomenon
in the general case in what follows.


\section{Towards existence of obstructions in general via positivity}
We now proceed to describe the main results of GCT for the general
(complexity-theoretic)
permanent vs. determinant problem in the context of
Goal~\ref{gobs}. 



Towards that end, we  associate with the class varieties 
certain representation-theoretic {\em stretching} functions. 
Let $F_{\lambda,n,m}(k)$ denote the number of occurances (multiplicity)  of
the Weyl module $V_{k\lambda}(G)$ in $R_{\#P}(n,m)^*$ (i.e. 
$R_{\#P}(n,m)^*_d$, for some $d$)  as a subrepresentation,
and $G_{\lambda,n,m}(k)$ the number of occurances of 
$V_{k\lambda}(G)$ in $R_{NC}(n,m)^*$. These are statistical functions
associated with the class varieties, where the statistics associates 
with every number (stretching parameter) $k$  
the multiplicity of the corresponding
Weyl module $V_{k\lambda}(G)$; cf. Figure~\ref{fig:statistics}.

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{l}{$\lambda$}
\psfrag{2l}{$2 \lambda$}
\psfrag{3l}{$3 \lambda$}
\psfrag{v1}{$V_\lambda(G)$}
\psfrag{v2}{$V_{2 \lambda}(G)$}
\psfrag{v3}{$V_{3\lambda}(G)$}
\epsfig{file=statistics.eps, scale=1}
\end{center}
      \caption{statistics}
      \label{fig:statistics}
\end{figure}


Let us  call a function $f(k)$ {\em quasipolynomial}, if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k)$ for all nonnegative integral $k=i$ modulo $l$;
here  $l$ is
called the period of the  quasi-polynomial. 
Thus  quasi-polynomials
are hybrids of  polynomial and periodic functions. 
We say that $f(k)$ is an 
{\em asymptotic quasipolynomial} if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k)$ for all nonnegative integral $k=i$ modulo $l$ for 
$k\ge a(f)$, for 
some nonnegative integer depending on $f$. The minimum 
$a(f)$ for which this holds is called the {\em deviation from 
quasipolynomiality}. Thus $f(k)$ is a (strict) quasipolynomial when this
deviation is zero.

A fundamental example of a quasi-polynomial is the Ehrhart quasi-polynomial
$f_P(k)$ of a polytope $P$ with rational vertices. It is defined
to be the number of integer points in the dilated polytope $kP$. By the 
classical result of Ehrhart, it is known to be a quasi-polynomial.
More generally, let $P(k)$ be a polytope parametrized by nonnegative
integral $k$: i.e., 
defined by a linear system of the form: 
\begin{equation} \label{eqpara}
A x \le k b + c,
\end{equation}
where $A$ is an $m \times n$ matrix, $x$ a variable $n$-vector, and 
$b$ and $c$ some constant $m$-vectors. Let $f_P(k)$ be the number 
of integer points in $P(k)$. We shall call it the Ehrhart function of
$P(k)$.  It is known to be  an asymptotic quasi-polynomial.
In what follows, we  denote a parametrized polytope $P(k)$ by 
just $P$. 




\begin{theorem} (GCT6) \label{tquasi}
The functions $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ 
are asymptotic quasi-polynomials. Furthermore, they 
are (strict) 
quasi-polynomials assuming that the singularities of the class varieties
$X_{\#P}(n,m)$ and $X_{NC}(n,m)$ are rational and normal. 

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem} 

Here a rational and normal  singularity means a singularity that is nice in
an algebro-geometric sense that we shall not elaborate here.
At present, we do not know if the singularities of the class varieties 
are indeed  rational and normal. A conservative conjecture would be  that 
they are not too bad, even if they are not strictly rational and normal,
because of the exceptional nature of the 
determinant and the permanent; 
i.e.,  the deviation from quasipolynomiality
of $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ is 
small in a sense to be made precise 
later (cf. the remarks after Hypothesis~\ref{hph1}).

The proof of Theorem~\ref{tquasi}
follows from a detailed study of the behaviour
of the singularities of class varieties under the action of the 
group $G$. This is based on
\begin{enumerate} 
\item The 
resolutions of singularities in characteristic zero
\cite{hironaka}: 
this  roughly says 
that the singularities of any algebraic variety in characteristic zero
can be untangled (resolved) nicely in a systematic fashion; cf.
 Figure~\ref{fig:resolution}.
\item Cohomological works of Boutot, Brion,  Flenner, Kempf  and others
based on this resolution; cf.  \cite{boutot,dehy} and
GCT6 for the history and other references.
\end{enumerate} 


\begin{figure} 
\begin{center} 
\epsfig{file=resolution.eps, scale=.5}
      \caption{Resolution}
      \label{fig:resolution}
\end{center}
\end{figure}


As such, this proof is highly nonconstructive. It gives no effective
bound on the period $l$--it just says that $l$  is finite.





The following hypothesis 
says that $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ 
can be realized as the Ehrhart functions  of parametrized  polytopes.

\begin{hypo} {\bf (PH) [Positivity Hypothesis]} \label{hph} (GCT6)

\noindent (a) For every $\lambda,n,m\ge n$, 
there exists   a parametrized  polytope $P=P_{\lambda,n,m}$ 
such that 
\begin{equation} \label{eqP}
F_{\lambda,n,m}(k)=f_P(k).
\end{equation} 
It is also assumed here that there exists for $P_{\lambda,n,m}$ a specification
of the form (\ref{eqpara}),
 where $A$ is independent of $\lambda$, and $b$ and $c$ 
are  piecewise homogeneous linear functions of $\lambda$.


\noindent (b) There exists a similar parametrized 
 polytope  $Q=Q_{\lambda,n,m}$  such that
\begin{equation} \label{eqQ}
G_{\lambda,n,m}(k)=f_Q(k).
\end{equation}


Analogous positivity hypothesis also holds 
for the $P$ vs. $NP$ problem in characteristic zero.
\end{hypo} 


If such $P$ and $Q$ exist, their dimensions are guaranteed to be
small by the proof of Theorem~\ref{tquasi}: specifically,
the dimension $P$ is guaranteed to be bounded by a 
polynomial in $n$, and the dimension of $Q$ 
by a polynomial in $m$.
There is a variant of PH (b), which is good enough for our purposes (cf.
Lecture 3, Hypothesis~\ref{hphvariant}),
wherein  the dimension of $Q$ is also guaranteed
to be bounded by a polynomial in $n$ (but independent 
of $m$), if the length of $\lambda$ is $\poly(n)$ (as it would be in 
our applications).






When PH holds, we say that $F_{\lambda,n,m}(k)$ and 
$G_{\lambda,n,m}(k)$ have  {\em positive convex representations}. 
Here positivity refers to the fact that the Ehhart function 
$f_P(k)$ is a positive expression:
\[ f_P(k)=\sum_{v} 1,\] 
where $v$ ranges over all integer points in $P(k)$--there are no 
alternating signs in this expression.
Convexity refers to the  convexity of the polytopes $P(k)$ and $Q(k)$. 


But, a  priori, it is not at all clear why PH should  even hold. 
Many numerical functions in algebraic geometry are 
asymptotic quasi-polynomials (e.g., the Hilbert function 
\footnote {Hilbert function $h_Z(k)$ of a projective algebraic variety $Z$
is defined to be $\dim(R(Z)_k)$, where $R(Z)$ is the homogeneous coordinate 
ring of $Z$ and $R(Z)_k$ its degree $k$-component.} of any projective
variety), but they rarely have positive convex representations.
PH is expected to hold for $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ 
because of the exceptional nature of the determinant and the permanent. 
One concrete evidence is provided by the proof of the weak form 
(Thoerem~\ref{tgenweaklec1}).
Analogous PH that arises in this weak setting can 
proven unconditionally.
For  mathematical evidence and justification
in support of  general PH, see  GCT6,7, and 8. 


The hypothesis 
PH alone is not sufficient to prove the existence of obstructions.
The precise statement of a sufficient condition is given in 
the theorem below.




\begin{theorem} (GCT6) \label{tgct6}
There exists a family $\{O_n\}$ of obstructions 
for the  $\#P$ vs. $NC$ problem in characteristic zero, 
for $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$, 
assuming, 

\begin{enumerate} 
\item PH, and
\item OH (Obstruction Hypothesis): 

For all $n\rightarrow \infty$,  there exists $\lambda$ such that 
$P_{\lambda,n,m}(\infty)=\mbox{lim}_{k\rightarrow \infty} P(k) 
\not = \emptyset$ and $Q_{\lambda,n,m}(k)=\emptyset$ for all (large enough)
$k$.
\end{enumerate}

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem}

Mathematical evidence and arguments in support of OH are given in GCT6.
The analogous weak OH that arises in the context of the generalized 
weak form can be  proven unconditionally.

We call  $\lambda$ a {\em relaxed obstruction}
(or rather, relaxed obstruction-label)
if it satisfies OH. In this case, $k\lambda$, for some integer $k\ge 1$ is
an obstruction--we just have to choose $k$ large enough 
so that 
$P_{\lambda,n,m}(k)$ contains an integer point
but $Q_{\lambda,n,m}(k)$ does not.
Henceforth, whenever we say obstruction, we actually mean relaxed 
obstruction.

There is a fundamental difference between the nature of PH and OH.
PH is a {\em mathematical hypothesis}, because there is no 
constraint on what $m$ should be in comparison to $n$ in its statement.
In contrast, OH is a {\em complexity theoretic hypothesis}, because 
$m$ needs to be small in comparison to $n$ for it to hold.


%\subsection{Why should PH  and OH hold?} 

%Mathematical evidence for this is given in GCT2,4,6,7,8.
%We shall discuss some of this  in the third lecture.


\section{The flip: Explicit construction of obstructions} 
\label{sflip}
In principle PH may have a nonconstructive proof (like that
of Theorem~\ref{tquasi})  which only tells  that such polytopes 
exist without explicitly constructing them. But proving OH may not be feasible
unless the polytopes $P$ and $Q$ in PH are given explicitly.
This  suggests the following strategy for proving 
existence of obstructions proposed in  GCT6 and  GCTflip.


\noindent (1) Prove the following stronger explicit form 
of PH, which is reasonable since the polytopes $P$ and $Q$, if they exist,
are already guaranteed to be of small (polynomial) dimension:

\begin{hypo} {\bf (PH1)}  \label{hph1} (GCT6)

\noindent (a) There exists an {\em explicit} 
polytope $P_{\lambda,n,m}$ 
as in  PH (a).
Explicit means: 

\begin{enumerate}
\item  The polytope is specified by an explicit system of linear constraints,
where the bitlength of (the description of) 
each constraint is  $\poly(n,\bitlength{\lambda}, \bitlength{m})$.
Here and in what follows, $\bitlength{z}$ denotes the bitlength of the 
description of $z$.

\item  The membership problem for the polytope
$P_{\lambda,n,m}(k)$  also 
belongs to the complexity class $P$.
That is,  given a point $x$, whether it belongs to $P_{\lambda,n,m}(k)$ 
can also be decided in $\poly(\bitlength{x},\bitlength{\lambda},
n,\bitlength{m})$
time.
Furthermore, we assume that if $x$ does not belong to the polytope,
then the membership algorithm also gives a hyperplane separating 
$x$ from the polytope in the spirit of \cite{lovasz}. 
\end{enumerate} 

\noindent (b) There exists a similar  explicit 
polytope $Q_{\lambda,n,m}$  satisfying   PH (b). 
\end{hypo}

\noindent {\em Remark 1:} 
Note the occurence of  $\bitlength{m}$  instead of $m$ in the polynomial
bounds in (a) (which implies that the bounds here become $\poly(n)$
when $m<2^n$ and $\bitlength{\lambda}=\poly(n)$). 
The reasons for this will be explained in Lecture 3 
(cf. remarks after Hypothesis~\ref{hph1restatement}). 
In contrast, the polynomial bounds for the polytope in (b)  depend on 
$m$, not $\bitlength{m}$. 
But there are  variants of PH (b) and PH1 (b), 
(cf. Hypotheses~\ref{hphvariant} and \ref{hph1tilde} in  Lecture 3), 
which are enough for our purposes, 
wherein the polynomial bounds depend on the bitlength of $\lambda$,
but not on $m$.
In what follows, we assume that PH (b) and PH1 (b) have been replaced 
with these variants.

 


\noindent {\em Remark 2:} 
In particular, PH1 implies that the functions $F_{\lambda,n,m}(k)$ and
$G_{\lambda,n,m}(k)$ belong to the complexity class $\#P$. 
It can be shown that it 
also implies that the deviation from quasipolynomiality 
of $F_{\lambda,n,m}(k)$ is small, specifically, 
$2^{O(\poly(\bitlength{\lambda},n,\bitlength{m}))}$--thus the bitlength
of the deviation is polynomial. This says
that the deviation from rationality and normality of the singularities
of the class variety $X_{\#P}(n,m)$ is small (cf. Theorem~\ref{tquasi}).
Similarly for $Q_{\lambda,n,m}(k)$ and $X_{NC}(n,m)$. 

Like PH, PH1 is also a mathematical hypothesis in the sense that
it puts  no constraint on what $m$ should be in comparison to $n$. 
Of course, unlike PH, there is some complexity theoretic aspect to it, 
but it is secondary in comparison to the complexity-theoretic aspect of 
 OH, since smallness  of $m$ with respect to  $n$ is the 
crux of the lower bound  problems under consideration. 





\noindent (2a) {\bf [The flip]}

Let $m=2^{\log ^a n}$, for a fixed $a>1$. 
Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
show existence of  an {\em explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of (relaxed) obstructions  satisfying OH. 
We say that an obstruction (proof-certificate) 
$\lambda_n$ is {\em explicit} if is ``short'' and ``easy to verify'':


\begin{enumerate} 
\item  Short: This means its bitlength $\bitlength{\lambda_n}$ 
is $\poly(n)$,
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  

\item Easy to verify: given $n, m \le 2^{n}$ and 
$\lambda_n$, whether 
$\lambda_n$ is a valid obstruction 
can be verified 
in $\poly(n,\bitlength{\lambda})$ time. In particular, this is
$\poly(n)$ when $\bitlength{\lambda}=\poly(n)$. 
\end{enumerate}

Existence of an explicit family of obstructions is equivalent to saying
that the problem of deciding existence of obstructions belongs to $NP$.
This definition of explicitness is quite natural since the class $NP$ 
is a class of problems whose proof-certificates (witnesses) are 
short and easy to verify. As such, the flip--going for 
explicit  obstructions--is
a proof-strategy that is literally given to us on a platter 
by the $P$ vs. $NP$ 
problem itself. Why it is called flip will be explained later.


It should be stressed that we are primarily interested in only proving 
existence of obstructions. Whether they are explicit or not 
does not really matter in the original statement of the problem.
But we need to know the polytopes $P$ and
$Q$ explicitly (as in PH1)  so that proving OH is feasible. 
%In other words,   if we do not
%even know what the polytopes $P$ and $Q$ look like, 
%it seems unlikely that anything  could be said regarding OH. 
But once  PH1 is proved, existence of an explicit family follows
automatically,   as a bonus, whether we care for it or not. 

To see why, let us observe that 
the second condition above  (ease of verification) follows directly
from PH1 and the polynomial time algorithm for 
linear programming on  polytopes given by separation oracles \cite{lovasz}. 
Shortness  also follows from PH1. 

Thus it is as if the $P$ vs. $NP$ problem is forcing us to go
for explicit obstructions.


\noindent (2b) {\bf [The strong flip (optional)]} 

Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
construct (rather than just show existence of) 
a {\em strongly explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of obstructions  satisfying OH. We say that an explicit family 
of obstructions is strongly explicit if,
for each $n$, a valid obstruction-label
$\lambda_n$ can be constructed in $\poly(n)$ time.
In particular, the height and the bitlength of
 $\lambda$ is $\poly(n)$ (short) 
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  


For the purposes of the lower bound problems that we are interested in, the
flip (just explicit  
existence) would suffice and the stronger flip (explicit construction)
is optional. But the stronger flip can give us deeper insight into these
lower bound problems; cf. GCTflip for more on this.

Now we turn to a few obvious questions.



\section{What has been achieved by all this?: The meaning of the flip} 
\label{smeaning}
Let us now see what has been achieved so far
in the context of the 
$\#P\not = NC$ conjecture in the nonuniform setting (characteristic zero),
the argument for the $P$ vs. $NP$ problem in characteristic zero
being  similar. 
At  first glance,
it may seem that all that GCT has achieved 
is to exchange a known difficult problem of 
complexity theory with a new very difficult problem of algebraic geoemtry.
In order to see that something is gained in exchange let us reexamine the 
original question.

The goal of the original  conjecture is to prove that 
$\perm(X)$, $\dim(X)=n$,  cannot be computed by an arithmetic circuit $C$
of size $m=\poly(n)$, or more generally,
$m \le 2^{\log^a n}$, for some fixed $a>1$, and depth $O(\log^a n)$.
Symbolically, 
let  $f_C(X)$ denote the function computed by $C$. Then we want to prove that
\begin{equation} \label{eqioh} 
 {\bf (IOH):}  \forall n \ge n_0 \forall C \exists X:
\perm(X)\not = f_C(X),
\end{equation} 
where $n_0$ is a sufficiently large constant.
For given $X$ and $C$ of $\poly(n)$ size, the problem 
of deciding if  $\perm(X) \not = f_C(X)$
belongs to $\#P$ (or rather, $P^{\#P}$). 
Since there are two alternating layers of quantifiers in (\ref{eqioh}),
the problem of verifying it belongs to $\Pi_2^{\#P}$, 
which is very high in the complexity hierarchy
(cf. Figure~\ref{fig:IOHcomplexity}).
Hence, we  refer to the original hypothesis (\ref{eqioh}) 
to be proven  as IOH 
(Infeasible Obstruction Hypothesis). Of course, IOH is expected to 
be a tautology, and hence is expected to  be verifiable in $O(1)$ time--but
we do not know that as yet. 



\begin{sidewaysfigure} 
\begin{center}
\psfragscanon
\psfrag{sigma2p}{{\small $\Pi^2 \#P$}}
\psfrag{sigma1p}{$\Sigma^1 \#P$}
\psfrag{P}{{\small $P$}}
\psfrag{NP}{{\small $NP$}}
\psfrag{T}{$T$}
\psfrag{#P}{$\# P$}
\psfrag{inNP}{$\in NP$}
\psfrag{inP}{$\in P$}
\psfrag{insigma2p}{$\in \Pi^2 \#P$}
\psfrag{PHplus}{PH1}
\psfrag{PHtil}{$PH^\dagger$}
\epsfig{file=IOHcomplexity.eps, scale=.8}
\end{center}
      \caption{Positivity as a means to eliminate the quantifiers and 
reduce the complexity of the  obstruction hypothesis}
      \label{fig:IOHcomplexity}
\end{sidewaysfigure}



Equivalently, the goal of IOH 
is to prove existence of a {\em trivial obstruction},
which is a table that lists for each $C$ as above a counterexample  $X$ so that
$\perm(X)\not = f_C(X)$; cf. Figure~\ref{fig:trivial}.
The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$ and depth
$O(\log^a n)$. Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. (Well, only
if the underlying field of computation is finite. For infinite fields, 
such as $\Q$ or $\C$ in this paper, 
there is another notion of a trivial obstruction (cf. 
GCT6). But let us imagine that the underlying
field is finite for this argument.)
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time to decide if such a table exists and construct 
one (optional) for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. That is why we 
call  this trivial, brute force 
strategy of proving IOH, based on existence of trivial obstructions,
an {\em infeasible strategy}. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{eq}{$\perm(X)\not = f_C(X)$}
\epsfig{file=trivial.eps, scale=.5}
\end{center}
      \caption{A trivial obstruction}
      \label{fig:trivial}
\end{figure}


In contrast, assuming PH1, the problem  of verifying OH belongs 
to $NP$ as we have already observed. Thus, assuming PH1, we have 
transformed the original infeasible obstruction 
hypothesis $IOH \in \Pi_2^{\#P}$ to a new  obstruction hypothesis 
$OH \in NP$, in the process bringing down the time to verify an obstruction
from  exponential (for the original trivial obstruction) to polynomial
(for the new obstruction); cf. Figure~\ref{fig:IOHcomplexity}.  
It is crucial here that PH1, the main tool for this reduction, is a 
mathematical hypothesis,  not complexity-theoretic (cf. the remarks
after Theorem~\ref{tgct6} and Hypothesis~\ref{hph1}).
The task of verifying  an obstruction has also been 
transformed from the infeasible (exponential-time) to the feasible 
(polynomial-time). Hence the name of this strategy: the flip,
from the infeasible to the feasible.
Positivity (PH1) is used in the flip as a means  to
eliminate the quantifying variables in IOH and bring down the 
 complexity of the obstruction hypothesis;
cf. Figure~\ref{fig:IOHcomplexity}. 




This process can be extended further. Assuming an additional
positivity hypothesis PH4 specified below,
$OH \in NP$ can be transformed 
to POH (Positivity Obstruction Hypothesis) that belongs to $P$; i.e.,
which can be verified in polynomial time, and an obstruction,
if it exists, can also be constructed in polynomial time; 
cf. Figure~\ref{fig:IOHcomplexity}. (The hypothesis is called PH4 instead
of PH2, because PH2 and PH3 are some other positivity hypotheses in GCT6
that complement PH1). 
Once this final positivity hypothesis POH is proven, the obstruction
hypothesis is reduced to a tautology (FOH: Final Obstruction Hypothesis),
which can be verified in
$O(1)$ time. This  would then give us 
the final $O(1)$-size  proof. 

Thus the basic idea of the flip is to use positivity systematically
as a means to eliminate the quantifiers  and reduce the complexity 
of the  obstruction hypothesis until it is finally
reduced to  an $O(1)$-time verifiable  tautology;
cf. Figure~\ref{fig:IOHcomplexity}. 

Now let us specify PH4 and POH.
Towards that end, let  $k \le l=m^2$ be the length of $\lambda$.
Define 

\begin{equation} 
\begin{array}{l}
\bar P_{n,m}= \{ \lambda: P_{\lambda,n,m} \not = \emptyset \} \subseteq \C^k, \\
\bar Q_{n,m}= \{ \lambda: Q_{\lambda,n,m} \not = \emptyset \} \subseteq \C^k.
\end{array}
\end{equation}

\begin{theorem} 
The sets $\bar P_{n,m}$ and $\bar Q_{n,m}$ are convex polytopes in $\C^k$.
\end{theorem} 
This follows from some fundamental results in geometric invariant theory
\cite{mumford}. 

Then: 

\begin{hypo}  {\bf PH4} (GCT6)
The membership problems for these polytopes belong to 
$P$ and so also the problem of deciding if $\mbox{vol}(\bar P_{n,m}
\setminus \bar Q_{n,m})$, the volume of the relative complement 
$\bar P_{n,m} \setminus \bar Q_{n,m}$, is nonzero (positive);
i.e. if $\bar P_{n,m} \not \subseteq \bar Q_{n,m}$. By polynomial time,
we mean $\poly(n,l,\bitlength{m})$ time. This is $\poly(n)$,
if $m\le 2^{o(n)}$ and $l =\poly(n)$. 
\end{hypo}

\begin{hypo} {\bf (POH)}

For all $n\rightarrow \infty$, assuming $m=2^{\log^a n}$, $a>1$ fixed, 

\[ \mbox{vol}(\bar P_{n,m} \setminus \bar Q_{n,m}) > 0, \] 

for $k=(n+1)^2$. 
\end{hypo} 

\ignore{
Thus POH says that  the line-shaded area in Figure~\ref{fig:POH} has positive
volume for all large enough $n$. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{P}{$\bar P_{n,m}$}
\psfrag{Q}{$\bar Q_{n,m}$}
\epsfig{file=POH.eps, scale=1}
\end{center}
      \caption{POH}
      \label{fig:POH}
\end{figure}
}

\section{How to prove PH?}  \label{sphprove}
There is  a basic prototype of PH in representation theory,
which will be described in detail towards the end of Lecture 3. We shall
refer to it  as Plethysm PH. It says that the stretching functions 
akin to $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$
associated with  fundamental  multiplicities 
in representation theory called plethysm constants also have analogous 
positive convex representations. 

This  is   known for a very special case of the plethysm constant 
called the  Littlewood-Richardson (LR) coefficient
$c_{\alpha,\beta}^\lambda$. It is  defined to be 
the number of occurances of the Weyl module $V_{\lambda}(G)$ in the 
tensor product of $V_{\alpha}(G)$ and $V_\beta(G)$. 
The classical Littlewood-Richardson rule, which we shall refer to as LR PH,
implies that the stretching function 
$\tilde c_{\alpha,\beta}^\lambda (k) = c_{k \alpha, k \beta}^{k \lambda}$
associated with the Littlewood-Richardson coefficient has a
positive convex representation.

Plethysm PH   happens to be a fundamental open problem of
representation theory, older than the $P$ vs. $NP$ problem itself. It 
has been studied intensively in the last century, and is known to be
formidable. And  now,  as explained the third lecture, it also turns out to 
be  the heart of this approach towards the $P$ vs $NP$, the
$\#P$ vs. $NC$ problems.



A basic plan to prove Plethysm PH is given in GCT6.
It is partially 
implemented in GCT7 and 8. See Figure~\ref{fig:lift} for a pictorial
depiction of the plan. It strives  to extend the  proof of LR PH based 
on the theory of the  standard quantum group \cite{drinfeld,kashiwara,lusztig}.
There it
comes out as a consequence of a  (proof of a) deep positivity result
\cite{kazhdan,lusztig}, which
we shall refer to as LR PH0. It says that   the 
tensor product of two representations of the standard quantum group 
has a canonical basis \cite{kashiwara,lusztig} 
whose structure coefficients are all positive \cite{lusztig}
polynomials (i.e., polynomials with nonnegative coefficients).
The only known proof of this
result is based on the Riemann Hypothesis over finite fields 
proved in \cite{weil2},  and the related works \cite{beilinson}. 
This Riemann Hypothesis over finite fields 
is  itself a deep positivity statement in mathematics,
from which   LR PH can  thus be 
deduced, as shown on the bottom row of Figure~\ref{fig:lift}.

If one were only interested in LR PH, one  does not 
need this  powerful machinery, because it has a  much simpler 
algebraic-combinatorial  proof. 
But the plan to extend the
proof of LR PH to Plethysm PH in GCT6,7,8 is like a huge
inductive spiral. To  make it work,  one  needs a 
stronger inductive hypothesis than Plethysm PH--this is precisely  Plethysm 
PH0 (which  will be
described in the third lecture; cf. Hypothesis~\ref{hplph0}).
Thus what is needed now 
is a systematic lifting  of the bottom arrow in Figure~\ref{fig:lift}
to the top, so as to complete the  commutative diagram, so to speak. 

Initial  steps in this direction have been taken in GCT7,8. 
First, GCT7 constructs a {\em nonstandard quantum group}, which
generalizes the notion of a standard quantum group \cite{drinfeld},
 and plays the
same role in the plethysm setting that the standard quantum group plays
in the LR setting. Second, GCT8 gives an algorithm to construct 
a canonical basis for a representation of the nonstandard quantum group
that is conjecturally correct and has the property Plethysm PH0,
which is a   generalization of LR PH0  supported by experimental
evidence.
Now what is needed to complete  the 
commutative diagram in Figure~\ref{fig:lift} is an appropriate nonstandard 
extension of the Riemann hypothesis over finite fields and the related works
\cite{beilinson,weil2,kazhdan,lusztig}
from which  Plethysm PH0 can be deduced. This--the top-right corner 
of the diagram--is the   main  open problem at the heart of this approach. 

\section{How to prove OH or POH?} 
We do not  know, 
since the  proof of OH and POH 
would really depend on the explicit forms of the
polytopes that arise in   PH1/PH4, and we have no idea about them
at this point.
\ignore{GCT does suggest  that proving OH/POH  should be feasible 
``in theory''
since OH/POH  belong to NP/P, assuming PH1/4, and polynomial-time
is complexity theory stands for feasible ``in theory''. 
In other words,
GCT gives a reason to believe now that proving 
the  $P\not = NP$ conjecture should be feasible in theory. Even this
was  always questioned  in the field of complexity theory so far, because 
the $P$ vs. $NP$ problem is a universal statement regarding all of mathematics
(that says theorems cannot be proven automatically).
But, as we also know by now, 
there is a huge gap between  theory and  practice--e.g., 
just because  some problem is in $P$ does not 
necessarily mean that it is feasible in practice. Similarly,
the actual implementation of the GCT flip via positivity is expected to be 
immensely difficult ``in practice'', as Figure~\ref{fig:lift} suggests. 
}






\section{Is positivity  necessary?} \label{sposnece}
\ignore{
Though the statement of this result is elementary, its proof is nonelementary,
as expected,  since the generalized permanents are highly nontrivial
and mathematically formidable objects. Specifically, the problem
of finding a $\#P$-basis for the space of generalized permanents 
is intimately related to some formidable problems of representation
theory and algebraic geometry,
and the  simplest analogue of this problem 
which can be solved at present  \cite{}
requires the deep Riemann Hypothesis over finite fields \cite{} for its
proof; cf. Section~\ref{}.
The proof of Theorem~\ref{} proceeds at an abstract level 
through algebraic geometry and representation theory without
having to know anything about such a basis.
At present, it is open if there is any alternative 
weaker form of the $\#P \not = NC$  conjecture,
which cannot be proved by relativizable, low-degree or 
naturalizable  techniques, but which can still be proved by elementary 
or not so  nonelementary techniques; that is, whether the earlier known
barriers mentioned above can 
be simultaneously bypassed in an elementary way in the context of 
the $\#P$ vs. $NC$ (or $P$ vs. $NC$  or $P$ vs. $NP$) problem.


\section{Why are we going for explicit obstructions?}
In a sense, the proof of the weak form turns out to be nonelementary
because of the difficulty of explicit construction. Specifically, algorithm 
to construct an obstruction $O_n$ for each $n$ is very simple, but to
show that it is correct requires nontrivial algebraic geometry,
just as the construction 
of an explcit family of Ramanujan graphs in \cite{} is very simple,
but to show that it is correct requires nontrivial algebraic geometry.
We already know, e.g. from this example of Ramanujan graphs, that 
explicit constructions can require highly nonelementary techniques.
So the question now arises: why are we going for such difficult explicit
constructions? Can they not be avoided somehow? 
After all, to solve the original problem we only need to show existence
of obstructions. We do not have to construct them explicitly.

Furthermore,  explicit construction is not needed to 
cross any of the barriers mentioned above (e.g. the natural-proof-barrier).
This is because {\em any} proof technique which uses symmetries of the
permanent would automatically bypass the natural-proof barrier
in the context of the permanent vs. determinant problem,
even if it does not utter a word about explicit construction, since
most functions have no symmetries. Indeed, the weak form of 
the generalized $\#P$ vs. $NC$ problem itself has two proofs, one
purely nonconstructive and one through explicit construction--the major 
chunk of both proofs being  the same, except for the last step,
which is carried out via a counting argument in the former proof and via
explicit construction in the latter. Since the nonconstructive proof too
is based on symmetries, it also crosses the natural-proof barrier.
This provides a concrete evidence that explicit construction is not 
necessary for crossing the earlier known  barriers.

Then why are we still going for explicit construction? 
Before we go any further, we wish to briefly state  the motivation
behind  going for the flip (explicit construction),
since this is an important issue. 
}

Finally,  if the positivity problems are so hard,  one may ask if 
they can not be avoided somehow. Unfortunately, there is a formidable 
barrier towards the $P$ vs. $NP$ and related problems, called the
{\em feasibility ($P$) barrier} (GCT6,GCTflip),
which seems universal in the sense that
any approach towards these problems would have to tackle it, not just GCT. 
The flip, i.e., explicit construction of obstructions, is the most natural
and obvious way to cross this barrier, and it also seems to be 
among the easiest. The 
existing mathematical evidence suggests that any such natural approach
to cross this barrier would have to say  something deep regarding positivity
(Plethysm PH/PH0)  either explicitly or {\em implicitly}, even if
the approach does not utter a word about algebraic geometry or
representation theory.
That is,  Plethysm PH and PH0   may indeed be 
the heart of the  fundamental lower bound problems in complexity theory;
a detailed story and a precise meaning of the key 
phrase {\em implicit} would appear in the revised version of GCTflip.

%\input{feasibility}









































 

































\begin{sidewaysfigure} 
\begin{center} 
\epsfig{file=lift.eps, scale=.8}
\end{center}
      \caption{A commutative diagram}
      \label{fig:lift}
\end{sidewaysfigure} 



\ignore{\begin{figure} 
\psfragscanon
\psfrag{P}{$P\not = NP$ and $\#P\not = NC$ conjectures (characteristic zero)}
\epsfig{file=barriers.eps, scale=1}
      \caption{The feasibility barrier towards $P$ vs. $NP$}
      \label{fig:barriers}
\end{figure}}



==> lecture1_maintext2.tex <==

The first  step 
(GCT1,2) is to reduce this nonexistence problem 
to an existence problem--specifically, to the problem of proving 
existence of a family $\{O_n\}$ of obstructions; 
cf. Figure~\ref{fig:firststep}.
Here an {\em obstruction} $O_n$ is a proof-certificate of
hardness of $\perm(X)$, $X$ an $n\times n$ variable matrix,
just as the Kurotowoski minor is a proof-certificate of nonplanarity of a 
graph.  Specifically,  it is some 
algebro-geometric-representation-theoretic gadget, 
whose existence for every $n$,  serves as a 
guarantee that $\perm(X)$ cannot be represented linearly as $\det(Y)$,
when $m=2^{\log^a n}$, $a>0$ fixed, $n\rightarrow \infty$ (i.e., for
$n$ greater than a large enough constant depending on $a$). 

\begin{figure} 
\begin{center}\psfragscanon
\psfrag{on}{$\{O_n\}$}
\epsfig{file=firststep.eps, scale=.8}
\end{center}
      \caption{Reduction from nonexistence to existence}
      \label{fig:firststep}
\end{figure}


\section{Weak form of the (generalized) $\#P$ vs. $NC$ problem} 
We will also illustrate the GCT approach by applying it to prove a concrete 
lower bound result --namely a weak of form of the (generalized) 
$\#P$ vs. $NC$ problem. 
To begin with:

\begin{prop}  \label{pweak}
Then there do not exist (possibly singular) $n\times n$ complex
matrices $B$ and $C$  and a polynomial 
$e(w_0,\ldots, w_n)$ such that $\perm(X) = g(BXC)$, 
where $g(X)=e(\trace(X^0), \trace(X), \ldots, \trace(X^n))$. 
\end{prop}
This was referred to as 
the weak form of the $\#P$ vs. $NC$ problem in the original lecture. 
It has a surprisingly simple elementary proof \cite{}. But the 
proof is naturalizable in the terminology of \cite{}--i.e. does not
cross the natural-proof barrier therein--because it works for 
most functions in place of the permanent. The proof technique of
the quadratic lower bound \cite{} for the permanent is also naturalizable.
Hence, the  first goal in this context 
is to prove some weaker form of the $\#P \not = NC$ conjecture (nonuniform)
which cannot be proved by naturalizable proof techniques. 

We shall now describe such a weaker form. 
For that we need a definition.
A function $p(X)$ is called a {\em generalized permanent} if it has exactly 
the same symmetries as that of the permanent; i.e.,
for all nonsingular $n\times n$ matrices $U$ and $V$, 
\[ p(U X V)=p(X) \mbox{\ iff\ } \perm(U X V)=\perm (X).\] 
For a precise description of the symmetries of the permanent,
see Section~\ref{} (basically $U$ and $V$ above have to be permutation
or diagonal matrices (with product of the diagonal entries one), or 
product of such matrices.) 
It may be conjectured that any generalized permanent of $\poly(n)$ 
degree cannot be linearly represented in terms of the determinant 
of a matrix of $\poly(n)$ dimension--we shall refer to this as 
the generalized $\#P$ vs. $NC$ problem. It may be conjectured 
that the space of of generalized permanents has a $\#P$-basis, by which
we mean a basis  whose 
elements represent $P^{\#P$-computable functions.
Hence, this is essentially (and conjecturally) 
equivalent to the original conjecture (though a bit stronger).
The following is its weaker form:

\begin{theorem}[The weak form of the generalized $\#P$ vs. $NC$ problem]
Let $p(X)$ be any nonzero generalized permanent function.
Then there do not exist (possibly singular) $n\times n$ complex
matrices $B$ and $C$  and a polynomial 
$e(w_0,\ldots, w_n)$ such that $p(X) = g(BXC)$, 
where $g(X)=e(\trace(X^0), \trace(X), \ldots, \trace(X^n))$. 
\end{theorem}

The only thing that is common to all generalized permanents is that
they have the same symmetries. Hence any proof of this result can
rely only on these symmetries, and thus is essentially forced to
cross the natural-proof barrier, since most functions have no symmetries.
The classical relativization barrier is also automatically bypassed 
in this problem (and also in the original permanent vs. determinant problem)
because of its algbraic nature. So also 
the algebraic-degree [GCTweak] (algebrization
\cite{}) barrier, since 
$p(X)$ and $g(X)$ (like the 
permanent and the determinant)  have the same degree, 
and hence, (low) degree-based 
techniques would not work either.  Thus, the main significance 
of this result from the complexity-theoretic view point is that 
it cannot be proved by relativizable, low-degree, or naturalizable 
proof techniques, i.e. any proof of this result
is essentially forced to bypass all the 
earlier known barriers--namely, relativization, natural-proof, and
algebraic-degree/algebrization. In particular, it illustrates that
GCT bypasses all these barriers simultaneously.


But we are still referring to it as weak because it is a mathematical
lower bound rather than a complexity theoretic lower bound in the sense
that there is no restriction on the computational complexity of the 
polynomial $e(w_0, \ldots, w_n)$ in this result. If $e(w_0,\ldots,w_n)$
were $NC$-computable, then so would be $g(X)$ and $g(BXC)$, since traces are 
$NC$-computable. But the result does not require this. In that sense,
it is rather in the spirit of the classical result of Galois theory 
which says that a general prolynomial cannot be solved by any number of
radical operations, without any restriction on the number of radical
operations.

Though the statement of this result is elementary, its proof is nonelementary.
This is to be expected, since the generalized permanents are highly nontrivial
and mathematically formidable objects. Specifically, the problem
of finding a $\#P$-basis for the space of generalized permanents 
is intimately related to some formidable problems of representation
theory and algebraic geometry,
and the far simpler anlogues of this problem 
which can be solved at present (e.g. \cite{}) 
all require the deep Riemann Hypothesis over finite fields \cite{} for their 
proofs; cf. Section~\ref{}.
The proof of Theorem~\ref{} proceeds at an abstract level 
through algebraic geometry and representation theory without
having to know anything about such a basis.
At present, it is open if there is any alternative 
weaker form of the $\#P \not = NC$  conjecture,
which cannot be proved by relativizable, low-degree or 
naturalizable  techniques, but which can still be proved by elementary 
or not so  nonelementary techniques; that is, whether the earlier known
barriers mentioned above can 
be simultaneously bypassed in an elementary way in the context of 
the $\#P$ vs. $NC$ (or $P$ vs. $NC$  or $P$ vs. $NP$) problem.













\section{From nonexistence to existence}
This reduction to existence is carried out as follows; cf. lecture 2 for its
details.
First, we associate (GCT1) with 
the complexity class $\#P$ a family $\{X_{\#P}(n,m)\}$ of (group-theoretic)
class varieties, and with the complexity class $NC$ a family of 
$\{X_{NC}(n,m)\}$ of (group-theoretic) class varieties such that: 
if $\perm(X)$, $\dim(X)=n$, can be represented linearly 
as $\det(Y)$, $\dim(Y)=m>n$, then 

\begin{equation} \label{eqembed} 
X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation} 

Each  class variety is a  (projective) algebraic variety, by which
we mean the zero set of  a system of multivariate 
homogeneous polynomials with coefficients in $\C$  (akin to the 
usual curves  and surfaces). It is  group-theoretic in the 
sense that it is  constructed using group-theoretic operations 
and the general linear group $G=GL_l(\C)$, $l=m^2$, of $l\times l$ invertible
complex matrices acts on it. Here action means moving the points 
of the class variety around, just as $G$ moves the points of $\C^l$ around 
by the standard action via invertible linear transformations.
The goal is to show that the inclusion (\ref{eqembed}) is impossible;
cf. Figure~\ref{fig:class}. 

\begin{figure} 
\begin{center} \psfragscanon
\psfrag{xsharp}{$X_{\#P}(n,m)$}
      \psfrag{xnc}{$X_{NC}(n,m)$}
      \psfrag{g}{$G=GL_l(\C)$, $l=m^2$}
      \psfrag{Obstruction}{\mbox{Obstruction}}
\epsfig{file=class.eps, scale=.5}
\end{center}
      \caption{Class varieties}
      \label{fig:class}
\end{figure} 



Since each class variety has a $G$-action, the space of polynomial functions 
on each class variety has a  representation-theoretic structure, which 
puts constraints on which  representations of $G$ can live on that variety
(i.e., in the space of polynomial  functions on that variety).
Informally, an obstruction is an irreducible (minimal)  representation of $G$
that can live on $X_{\#P}(n,m)$ but not on $X_{NC}(n,m)$; 
cf. Figure~\ref{fig:class}.
Existence of  an obstruction $O_n$, for every $n$, assuming
$m=2^{\log^a n}$, $a>1$ fixed, implies  that the inclusion (\ref{eqembed}) 
is not possible, since  $O_n$ cannot live  on $X_{NC}(n,m)$.
Thus  an obstruction blocks the inclusion (\ref{eqembed}).


To define an obstruction formally, we need to recall some basic representation
theory.  By a classical result of Weyl, the irreducible 
(polynomial) representations of $G=GL_l(\C)$ are in one-to-one correspondence 
with the partitions  $\lambda$ of length at most $l$, by which we mean 
integral sequences $\lambda_1 \ge 
\lambda_2 \cdots \ge \lambda_k > 0$, $k\le l$, where  $k$ is called the  length
of $\lambda$. The irreducible 
representation of $G$ in correspondence with $\lambda$ is denoted 
by $V_\lambda(G)$, and is called the {\em Weyl module} of $G$ indexed by 
$\lambda$. Symbolically:

\[\mbox{Irreducible representations of } G \stackrel{\mbox{Weyl}}{\Longleftrightarrow} \quad \mbox{partitions} \ \lambda. \]  

\[\mbox{Weyl module  } V_\lambda(G)  \longleftrightarrow \lambda. \] 
Weyl also proved that every finite dimensional representation of $G$ 
can be decomposed into irreducible representations--i.e.,
can be written as a direct sum of Weyl modules. Thus Weyl modules 
are the basic building blocks of the representation theory of 
$G$, and every finite dimensional representation of $G$ can be thought
of as a complex building made out of these blocks. 


Now suppose $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$. 
Suppose to the contrary that 

\begin{equation} \label{eqembed2}   X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation}

Let $R_{\#P}(n,m)$ denote the homogeneous coordinate ring of 
$X_{\#P}(n,m)$; i.e., the ring of polynomial functions on $X_{\#P}(n.m)$
(though the  functions here are not functions in usual sense;
but let us  not worry about this). 
Let $R_{\#P}(n,m)_d$ be the degree-$d$-component of $R_{\#P}(n, m)$ consisting
of functions of degree $d$. We define $R_{NC}(n,m)$ and $R_{NC}(n,m)_d$
similarly. Since $X_{\#P}(n,m)$ has the action of $G$, $R_{\#P}(n,m)$ 
also has an action of $G$; i.e., it is a representation of $G$. Hence,
$R_{\#P}(n,m)_d$ is a finite dimensional representation of $G$. 
Similarly, $R_{NC}(n,m)$ is a representation of $G$, and $R_{NC}(n,m)_d$
a finite dimensional representation of $G$. 



If (\ref{eqembed2}) holds, then we get a natural map from $R_{NC}(n,m)$ to
$R_{\#P}(n,m)$ obtained by restricting a function on $X_{NC}(n,m)$ to
$X_{\#P}(n,m)$. %; cf. Figure~\ref{fig:restriction}.
By basic algebraic geometry, this map
is surjective and is a $G$-homomorphism.
Furthermore, it is degree-preserving. This means there
is a surjective $G$-homomorphism from $R_{NC}(n,m)_d$ to 
$R_{\#P}(n,m)_d$. Symbolically: 

\begin{equation} \label{eqsurjection}
R_{\#}(n,m)_d \leftarrow  R_{NC}(n,m)_d.
\end{equation}

\ignore{
\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{Xp}{\small $X_{\#P}(n,m)$}
\psfrag{Xnc}{\small $X_{NC}(n,m)$}
\epsfig{file=restriction.eps, scale=.6}
\end{center}
      \caption{Restriction}
      \label{fig:restriction}
\end{figure}
}

Let $R_{\#P}(n,m)_d^*$ denote the dual of $R_{\#P}(n,m)_d$; i.e., the 
set of linear maps from $R_{\#P}(n,m)_d$ to $\C$. Then (\ref{eqsurjection})
implies that there is an injective $G$-homomorphism from 
$R_{\#P}(n,m)^*_d$ to $R_{NC}(n,m)^*_d$. Symbolically: 

\begin{equation} \label{eqinclusion}
R_{\#}(n,m)_d^*  \hookrightarrow {NC}(n,m)_d^*.
\end{equation}

\begin{defn} (GCT2)
An obstruction $O_n$ is a Weyl module $V_\lambda(G)$ that 
occurs as a subrepresentation 
in $R_{\#P}(n,m)_d^*$  but not in $R_{NC}(n,m)_d^*$, for some $d$. 
We call $\lambda$ an {\em obstruction label}, and sometimes,
by abuse of notation, an obstruction as well.
\end{defn}

\begin{prop} (GCT2)
Existence of an obstruction $O_n$, for all $n\rightarrow \infty$, 
with $m=2^{\log^a n}$, $a>1$ fixed, implies $\perm(X)$, $\dim(X)=n$, 
cannot be represented linearly as 
$\det(Y)$, $\dim(Y)=m$. 
\end{prop}

This follows just from the definition of an obstruction, and 
leads to:

\begin{goal} \label{gobs} (GCT2)
Prove existence of an obstruction family $\{O_n\}$ using 
the {\em exceptional} nature of $\perm(X)$ and $\det(Y)$. 
\end{goal} 

Exceptional here means completely characterized by the symmetries 
in the following sense. 
Let  $Y$ be a variable $m\times m$ matrix.
Let $\sym^m(Y)$ be the space of homogeneous forms of degree $m$ 
in the $m^2$ variable entries of $Y$. Then, by the  classical
representation theory,  $\det(Y)$ is the only form in $\sym^m(Y)$ 
such that, for any $A,B \in GL_m(\C)$ with $\det(A)\det(B)=1$, 
\[ \det(Y)=\det(A Y^* B), \] 
where $Y^*=Y$ or $Y^t$. 
Thus $\det(Y)$ is completely characterized 
by its symmetries, and hence, is  exceptional.

Similarly, $\perm(X)$ is the only form 
in the space of forms of degree $n$ in the entries of $X$ such that, 
for any diagonal or permutation matrices $A,B$, 
\[ \perm(X)=\perm(AX^*B), \]
where $X^*=X$ or $X^t$ and the product of the diagonal entries of $A$ and $B$
is one. 
Thus $\perm(X)$ is also
completely characterized   by its symmetries, and hence, is
exceptional.

\section{Towards existence via positivity}
We now proceed to describe the main results of GCT in the context of
Goal~\ref{gobs}. 
Towards that end, we  associate with the class varieties 
certain representation-theoretic {\em stretching} functions. 
Let $F_{\lambda,n,m}(k)$ denote the number of occurances (multiplicity)  of
the Weyl module $V_{k\lambda}(G)$ in $R_{\#P}(n,m)^*$ (i.e. 
$R_{\#P}(n,m)^*_d$, for some $d$)  as a subrepresentation,
and $G_{\lambda,n,m}(k)$ the number of occurances of 
$V_{k\lambda}(G)$ in $R_{NC}(n,m)^*$. These are statistical functions
associated with the class varieties, where the statistics associates 
with every number (stretching parameter) $k$  
the multiplicity of the corresponding
Weyl module $V_{k\lambda}(G)$; cf. Figure~\ref{fig:statistics}.

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{l}{$\lambda$}
\psfrag{2l}{$2 \lambda$}
\psfrag{3l}{$3 \lambda$}
\psfrag{v1}{$V_\lambda(G)$}
\psfrag{v2}{$V_{2 \lambda}(G)$}
\psfrag{v3}{$V_{3\lambda}(G)$}
\epsfig{file=statistics.eps, scale=1}
\end{center}
      \caption{statistics}
      \label{fig:statistics}
\end{figure}


Let us  call a function $f(k)$ {\em quasipolynomial}, if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k)$ for all nonnegative integral $k=i$ modulo $l$;
here  $l$ is
called the period of the  quasi-polynomial. 
Thus  quasi-polynomials
are hybrids of  polynomial and periodic functions. 
We say that $f(k)$ is an 
{\em asymptotic quasipolynomial} if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k)$ for all nonnegative integral $k=i$ modulo $l$ for 
$k\ge a(f)$, for 
some nonnegative integer depending on $f$. The minimum 
$a(f)$ for which this holds is called the {\em deviation from 
quasipolynomiality}. Thus $f(k)$ is a (strict) quasipolynomial when this
deviation is zero.

A fundamental example of a quasi-polynomial is the Ehrhart quasi-polynomial
$f_P(k)$ of a polytope $P$ with rational vertices. It is defined
to be the number of integer points in the dilated polytope $kP$. By the 
classical result of Ehrhart, it is known to be a quasi-polynomial.
More generally, let $P(k)$ be a polytope parametrized by nonnegative
integral $k$: i.e., 
defined by a linear system of the form: 
\begin{equation} \label{eqpara}
A x \le k b + c,
\end{equation}
where $A$ is an $m \times n$ matrix, $x$ a variable $n$-vector, and 
$b$ and $c$ some constant $m$-vectors. Let $f_P(k)$ be the number 
of integer points in $P(k)$. We shall call it the Ehrhart function of
$P(k)$.  It is known to be  an asymptotic quasi-polynomial.
In what follows, we  denote a parametrized polytope $P(k)$ by 
just $P$. 




\begin{theorem} (GCT6) \label{tquasi}
The functions $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ 
are asymptotic quasi-polynomials. Furthermore, they 
are (strict) 
quasi-polynomials assuming that the singularities of the class varieties
$X_{\#P}(n,m)$ and $X_{NC}(n,m)$ are rational and normal. 

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem} 

Here a rational and normal  singularity means a singularity that is nice in
an algebro-geometric sense that we shall not elaborate here.
At present, we do not know if the singularities of the class varieties 
are indeed  rational and normal. A conservative conjecture would be  that 
they are not too bad, even if they are not strictly rational and normal,
because of the exceptional nature of the 
determinant and the permanent; 
i.e.,  the deviation from quasipolynomiality
of $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ is 
small in a sense to be made precise 
later (cf. the remarks after Hypothesis~\ref{hph1}).

The proof of Theorem~\ref{tquasi}
follows from a detailed study of the behaviour
of the singularities of class varieties under the action of the 
group $G$. This is based on
\begin{enumerate} 
\item The 
resolutions of singularities in characteristic zero
\cite{hironaka}: 
this  roughly says 
that the singularities of any algebraic variety in characteristic zero
can be untangled (resolved) nicely in a systematic fashion; cf.
 Figure~\ref{fig:resolution}.
\item Cohomological works of Boutot, Brion,  Flenner, Kempf  and others
bases on this resolution; cf.  \cite{boutot,dehy} and
GCT6 for the history and other references.
\end{enumerate} 


\begin{figure} 
\begin{center} 
\epsfig{file=resolution.eps, scale=.5}
      \caption{Resolution}
      \label{fig:resolution}
\end{center}
\end{figure}


As such, this proof is highly nonconstructive. It gives no effective
bound on the period $l$--it just says that $l$  is finite.





The following hypothesis 
says that $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ 
can be realized as the Ehrhart functions  of parametrized  polytopes.

\begin{hypo} {\bf (PH) [Positivity Hypothesis]} \label{hph} (GCT6)

\noindent (a) For every $\lambda,n,m\ge n$, 
there exists   a parametrized  polytope $P=P_{\lambda,n,m}$ 
such that 
\begin{equation} \label{eqP}
F_{\lambda,n,m}(k)=f_P(k).
\end{equation} 
It is also assumed here that there exists for $P_{\lambda,n,m}$ a specification
of the form (\ref{eqpara}),
 where $A$ is independent of $\lambda$, and $b$ and $c$ 
are  piecewise homogeneous linear functions of $\lambda$.


\noindent (b) There exists a similar parametrized 
 polytope  $Q=Q_{\lambda,n,m}$  such that
\begin{equation} \label{eqQ}
G_{\lambda,n,m}(k)=f_Q(k).
\end{equation}


Analogous positivity hypothesis also holds 
for the $P$ vs. $NP$ problem in characteristic zero.
\end{hypo} 


If such $P$ and $Q$ exist, their dimensions are guaranteed to be
small by the proof of Theorem~\ref{tquasi}: specifically,
the dimension $P$ is guaranteed to be bounded by a 
polynomial in $n$, and the dimension of $Q$ 
by a polynomial in $m$.
There is a variant of PH (b), which is good enough for our purposes (cf.
Lecture 3, Hypothesis~\ref{hphvariant}),
wherein  the dimension of $Q$ is also guaranteed
to be bounded by a polynomial in $n$ (but independent 
of $m$), if the length of $\lambda$ is $\poly(n)$ (as it would be in 
our applications).






When PH holds, we say that $F_{\lambda,n,m}(k)$ and 
$G_{\lambda,n,m}(k)$ have  {\em positive convex representations}. 
Here positivity refers to the fact that the Ehhart function 
$f_P(k)$ is a positive expression:
\[ f_P(k)=\sum_{v} 1,\] 
where $v$ ranges over all integer points in $P(k)$--there are no 
alternating signs in this expression.
Convexity refers to the  convexity of the polytopes $P(k)$ and $Q(k)$. 


But, a  priori, it is not at all clear why PH should  even hold. 
Because many numerical functions in algebraic geometry are 
asymptotic quasi-polynomials (e.g., the Hilbert function 
\footnote {Hilbert function $h_Z(k)$ of a projective algebraic variety $Z$
is defined to be $\dim(R(Z)_k)$, where $R(Z)$ is the homogeneous coordinate 
ring of $Z$ and $R(Z)_k$ its degree $k$-component.} of any projective
variety), but they rarely have positive convex representations.
PH is expected to hold for $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ 
because of the exceptional nature of the determinant and the permanent. 
For a mathematical evidence and justification
in support of PH, see  GCT6,7, and 8.







\begin{theorem} (GCT6) \label{tgct6}
There exists a family $\{O_n\}$ of obstructions 
for the  $\#P$ vs. $NC$ problem in characteristic zero, 
for $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$, 
assuming, 

\begin{enumerate} 
\item PH, and
\item OH (Obstruction Hypothesis): 

For all $n\rightarrow \infty$,  there exists $\lambda$ such that 
$P_{\lambda,n,m}(\infty)=\mbox{lim}_{k\rightarrow \infty} P(k) 
\not = \emptyset$ and $Q_{\lambda,n,m}(k)=\emptyset$ for all (large enough)
$k$.
\end{enumerate}

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem}

Mathematical evidence and arguments in support of OH are given in GCT6.

We call  $\lambda$ a {\em relaxed obstruction}
(or rather, relaxed obstruction-label)
if it satisfies OH. In this case, $k\lambda$, for some integer $k\ge 1$ is
an obstruction--we just have to choose $k$ large enough 
so that 
$P_{\lambda,n,m}(k)$ contains an integer point
but $Q_{\lambda,n,m}(k)$ does not.
Henceforth, whenever we say obstruction, we actually mean relaxed 
obstruction.

There is a fundamental difference between the nature of PH and OH.
PH is a {\em mathematical hypothesis}, because there is no 
constraint on what $m$ should be in comparison to $n$ in its statement.
In contrast, OH is a {\em complexity theoretic hypothesis}, because 
$m$ needs to be small in comparison to $n$ for it to hold.


%\subsection{Why should PH  and OH hold?} 

%Mathematical evidence for this is given in GCT2,4,6,7,8.
%We shall discuss some of this  in the third lecture.


\section{The flip: Explicit construction of obstructions} 
\label{sflip}
In principle PH may have a nonconstructive proof (like that
of Theorem~\ref{tquasi})  which only tells  that such polytopes 
exist without explicitly constructing them. But proving OH may not be feasible
unless the polytopes $P$ and $Q$ in PH are given explicitly.
This  suggests the following strategy for proving 
existence of obstructions proposed in  GCT6 and  GCTflip.


\noindent (1) Prove the following stronger explicit form 
of PH, which is reasonable since the polytopes $P$ and $Q$, if they exist,
are already guaranteed to be of small (polynomial) dimension:

\begin{hypo} {\bf (PH1)}  \label{hph1} (GCT6)

\noindent (a) There exist an {\em explicit} 
polytope $P_{\lambda,n,m}$ 
as in  PH (a).
Explicit means: 

\begin{enumerate}
\item  The polytope is specified by an explicit system of linear constraints,
where the bitlength of (the description of) 
each constraint is  $\poly(n,\bitlength{\lambda}, \bitlength{m})$.
Here and in what follows, $\bitlength{z}$ denotes the bitlength of the 
description of $z$.

\item  The membership problem for the polytope
$P_{\lambda,n,m}(k)$  also 
belongs to the complexity class $P$.
That is,  given a point $x$, whether it belongs to $P_{\lambda,n,m}(k)$ 
can also be decided in $\poly(\bitlength{x},\bitlength{\lambda},
n,\bitlength{m})$
time.
Furthermore, we assume that if $x$ does not belong to the polytope,
then the membership algorithm also gives a hyperplane separating 
$x$ from the polytope in the spirit of \cite{lovasz}. 
\end{enumerate} 

\noindent (b) There exists a similar  explicit 
polytope $Q_{\lambda,n,m}$  satisfying   PH (b). 
\end{hypo}

Note the occurance of  $\bitlength{m}$  instead of $m$ in the polynomial
bounds in (a); 
the reasons for this would be explained in Lecture 3 
(cf. remarks after Hypothesis~\ref{hph1restatement}). 
In contrast, the polynomial bounds for the polytope in (b)  depend on 
$m$, not $\bitlength{m}$. 
But there are  variants of PH (b) and PH1 (b), 
(cf. Hypotheses~\ref{hphvariant} and \ref{hph1tilde} in  Lecture 3), 
which are enough for our purposes, 
wherein the polynomial bounds depend on the bitlength of $\lambda$,
but not on $m$.
In what follows, we assume that PH (b) and PH1 (b) have been replaced 
with these variants.

 


In particular, PH1 implies that the functions $F_{\lambda,n,m}(k)$ and
$G_{\lambda,n,m}(k)$ belong to the complexity class $\#P$. 
It also implies that the deviation from quasipolynomiality 
of $F_{\lambda,n,m}(k)$ is small, specifically, 
$2^{O(\poly(\bitlength{\lambda},n,\bitlength{m}))}$--thus the bitlength
of the deviation is polynomial. In other words, this says
that the deviation from rationality and normality of the singularities
of the class variety $X_{\#P}(n,m)$ is small (cf. Theorem~\ref{tquasi}).
Similarly for $Q_{\lambda,n,m}(k)$ and $X_{NC}(n,m)$. 

Like PH, PH1 is also a mathematical hypothesis in the sense that
it puts  no constraint on what $m$ should be in comparison to $n$. 
Of course, unlike PH, there is some complexity theoretic aspect to it, 
but it is secondary in comparison to the complexity-theoretic aspect of 
of OH, since smallness  of $m$ with respect to  $n$ is the 
crux of the lower bound  problems under consideration. 





\noindent (2a) {\bf [The flip]}

Let $m=2^{\log ^a n}$, for a fixed $a>1$. 
Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
show existence of  an {\em explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of (relaxed) obstructions  satisfying OH. 
We say that an obstruction (proof-certificate) 
$\lambda_n$ is {\em explicit} if is ``short'' and ``easy to verify'':


\begin{enumerate} 
\item  Short: This means its bitlength $\bitlength{\lambda_n}$ 
is $\poly(n)$,
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  

\item Easy to verify: given $n, m \le 2^{\log^a n}$ and 
$\lambda_n$, whether 
$\lambda_n$ is a valid obstruction 
can be verified 
in $\poly(n,\bitlength{\lambda})$ time. In particular, this is
$\poly(n)$ when $\bitlength{\lambda}=\poly(n)$. 
\end{enumerate}

Existence of an explicit family of obstructions is equivalent to saying
that the problem of deciding existence of obstructions belongs to $NP$.
This definition of explicitness is quite natural since the class $NP$ 
is a class of problems whose proof-certificates (witnesses) are 
short and easy to verify. As such, the flip--going for 
explicit  obstructions--is
a proof-strategy that is literally given to us on a platter 
by the $P$ vs. $NP$ 
problem itself. Why it is called flip would be explained later.


It should be stressed that we are primarily interested in only proving 
existence of obstructions. Whether they are explicit or not 
does not really matter in the original statement of the problem.
But we need to know the polytopes $P$ and
$Q$ explicitly (as in PH1)  so that proving OH is feasible. 
%In other words,   if we do not
%even know what the polytopes $P$ and $Q$ look like, 
%it seems unlikely that anything  could be said regarding OH. 
But once  PH1 is proved, existence of an explicit family follows
automatically,   as a bonus, whether we care for it or not. 

To see why, let us observe that 
the second condition above  (ease of verification) follows directly
from PH1 and the polynomial time algorithm for 
linear programming on  polytopes given by separation oracles \cite{lovasz}. 
Shortness  also follows from PH1. 

Thus it is as if the $P$ vs. $NP$ problem is forcing us to go
for explicit obstructions.


\noindent (2b) {\bf [The strong flip (optional)]} 

Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
construct (rather than just show existence of) 
a {\em strongly explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of obstructions  satisfying OH. We say that an explicit family 
of obstructions is strongly explicit if,
for each $n$, a valid obstruction-label
$\lambda_n$ can be constructed in $\poly(n)$ time.
In particular, the height and the bitlength of
 $\lambda$ is $\poly(n)$ (short) 
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  


For the purposes of the lower bound problems that we are interested in, the
flip (just explicit  
existence) would suffice and the stronger flip (explicit construction)
is optional. But the stronger flip can give us deeper insight into these
lower bound problems; cf. GCTflip for more on this.

Now we turn to a few obvious questions.



\section{What has been achieved by all this?: The meaning of the flip} 
\label{smeaning}
Let us now see what has been achieved so far
in the context of the 
$\#P\not = NC$ conjecture in the nonuniform setting (characteristic zero),
the argument for the $P$ vs. $NP$ problem in characteristic zero
being  similar. The goal of this conjecture is to prove that 
$\perm(X)$ cannot be computed by an arithmetic circuit $C$
of size $m=\poly(n)$, or more generally,
$m \le 2^{\log^a n}$, for some fixed $a>1$, and depth $O(\log^a n)$.
Or in symbols:

\begin{equation} \label{eqioh} 
 {\bf (IOH):}  \forall n  \forall C \exists X:
\perm(X)\not = f_C(X),
\end{equation} 

where $f_C(X)$ denotes the function computed by $C$, and $n$ is supposed
to be sufficiently large.
For given $X$ and $C$ of $\poly(n)$ size, the problem 
of deciding if  $\perm(X) = f_C(X)$ belongs to $\#P$ (or rather, $P^{\#P}$). 
Since there are two alternating layers of quantifiers in (\ref{eqioh}),
the problem of verifying it belongs to $\Pi^2 \#P$, 
which is very high in the complexity hierarchy
(cf. Figure~\ref{fig:IOHcomplexity}).
Hence, we  refer to the original hypothesis (\ref{eqioh}) 
to be proven  as IOH 
(Infeasible Obstruction Hypothesis). Of course, IOH is expected to 
be a tautology, and hence is expected to  be verifiable in $O(1)$ time--but
we do not know that as yet. 



\begin{sidewaysfigure} 
\begin{center}
\psfragscanon
\psfrag{sigma2p}{{\small $\Pi^2 \#P$}}
\psfrag{sigma1p}{$\Sigma^1 \#P$}
\psfrag{P}{{\small $P$}}
\psfrag{NP}{{\small $NP$}}
\psfrag{T}{$T$}
\psfrag{#P}{$\# P$}
\psfrag{inNP}{$\in NP$}
\psfrag{inP}{$\in P$}
\psfrag{insigma2p}{$\in \Pi^2 \#P$}
\psfrag{PHplus}{PH1}
\psfrag{PHtil}{$PH^\dagger$}
\epsfig{file=IOHcomplexity.eps, scale=.8}
\end{center}
      \caption{Positivity as a means to eliminate the quantifiers and 
reduce the complexity of the  obstruction hypothesis}
      \label{fig:IOHcomplexity}
\end{sidewaysfigure}



Equivalently, the goal is to prove existence of a {\em trivial obstruction},
which is a table that lists for each $C$ as above a counterexample  $X$ so that
$\perm(X)\not = f_C(X)$; cf. Figure~\ref{fig:trivial}.
The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$ and depth
$O(\log^a n)$. Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. (Well, only
if the underlying field of computation is finite. For infinite fields, 
such as $\Q$ or $\C$ in this paper, 
there is another notion of a trivial obstruction (cf. 
GCT6). But let us imagine that the underlying
field is finite for this argument.)
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time to decide if such a table exists and construct 
one (optional) for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. So
we call  this trivial, brute force 
strategy of proving IOH, based on existence of trivial obstructions,
 an {\em infeasible strategy}. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{eq}{$\perm(X)\not = f_C(X)$}
\epsfig{file=trivial.eps, scale=.5}
\end{center}
      \caption{A trivial obstruction}
      \label{fig:trivial}
\end{figure}


In contrast, assuming PH1, the problem  of verifying OH belongs 
to $NP$ as we have already observed. Thus, assuming PH1, we have 
transformed the original infeasible obstruction 
hypothesis $IOH \in \Pi^2 \#P$ to a new  obstruction hypothesis 
$OH \in NP$, in the process bringing down the time to verify an obstruction
from the exponential (for the original trivial obstruction) to polynomial
(for the new obstruction); cf. Figure~\ref{fig:IOHcomplexity}.  
It is crucial here that PH1, the main tool for this reduction, is a 
mathematical hypothesis,  not complexity-theoretic (cf. the remarks
after Theorem~\ref{tgct6} and Hypothesis~\ref{hph1}).
The task of verifying  an obstruction has also been 
transformed from the infeasible (exponential-time) to the feasible 
(polynomial-time). Hence the name of this strategy: the flip,
from the infeasible to the feasible.
Positivity (PH1) is used in the flip as a means  to
eliminate the quantifying variables in IOH and bring down the 
 complexity of the obstruction hypothesis;
cf. Figure~\ref{fig:IOHcomplexity}. 




This process can be extended further. Assuming an additional
positivity hypothesis PH4 specified below,
$OH \in NP$ can be transformed 
to POH (Positivity Obstruction Hypothesis) that belongs to $P$; i.e.,
which can be verified in polynomial time, and an obstruction,
if it exists, can also be constructed in polynomial time; 
cf. Figure~\ref{fig:IOHcomplexity}. (The hypothesis is called PH4 instead
of PH2, because PH2 and PH3 are some other positivity hypotheses in GCT6
that complement PH1). 
Once this final positivity hypothesis POH is proven, the obstruction
hypothesis is reduced to a tautology (FOH: Final Obstruction Hypothesis),
which can be verified in
$O(1)$ time. This  would then give us 
the final $O(1)$-size  proof. 

Thus the basic idea of the flip is to use positivity systematically
as a means to eliminate the quantifiers  and reduce the complexity 
of the  obstruction hypothesis until it is finally
reduced to  an $O(1)$-time verifiable  tautology;
cf. Figure~\ref{fig:IOHcomplexity}. 

Now let us specify PH4 and POH.
Towards that end, let  $k \le l=m^2$ be the length of $\lambda$.
Define 

\begin{equation} 
\begin{array}{l}
\bar P_{n,m}= \{ \lambda: P_{\lambda,n,m} \not = \emptyset \} \subseteq \C^k, \\
\bar Q_{n,m}= \{ \lambda: Q_{\lambda,n,m} \not = \emptyset \} \subseteq \C^k.
\end{array}
\end{equation}

Then: 

\begin{hypo}  {\bf PH4} (GCT6)

The sets $\bar P_{n,m}$ and $\bar Q_{n,m}$ are convex polytopes in $\C^k$.
Furthermore, the membership problems for these polytopes belong to 
$P$ and so also the problem of deciding if $\mbox{vol}(\bar P_{n,m}
\setminus \bar Q_{n,m})$, the volume of the relative complement 
$\bar P_{n,m} \setminus \bar Q_{n,m}$, is nonzero (positive);
i.e. if $\bar P_{n,m} \not \subseteq \bar Q_{n,m}$. By polynomial time,
we mean $\poly(n,l,\bitlength{m})$ time. This is $\poly(n)$,
if $m\le 2^{o(n)}$ and $l =\poly(n)$. 
\end{hypo}

\begin{hypo} {\bf (POH)}

For all $n\rightarrow \infty$, assuming $m=2^{\log^a n}$, $a>1$ fixed, 

\[ \mbox{vol}(\bar P_{n,m} \setminus \bar Q_{n,m}) > 0, \] 

for $k=(n+1)^2$. 
\end{hypo} 

\ignore{
Thus POH says that  the line-shaded area in Figure~\ref{fig:POH} has positive
volume for all large enough $n$. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{P}{$\bar P_{n,m}$}
\psfrag{Q}{$\bar Q_{n,m}$}
\epsfig{file=POH.eps, scale=1}
\end{center}
      \caption{POH}
      \label{fig:POH}
\end{figure}
}

\section{How to prove PH?}  \label{sphprove}
There is  a basic prototype of PH in representation theory,
which will be described in detail towards the end of Lecture 3. We shall
refer to it  as Plethysm PH. It says that the stretching functions 
akin to $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$
associated with  fundamental  multiplicities 
in representation theory called plethysm constants also have analogous 
positive convex representations. 

This  is   known for a very special case of the plethysm constant 
called the  Littlewood-Richardson (LR) coefficient
$c_{\alpha,\beta}^\lambda$. It is  defined to be 
the number of occurances of the Weyl module $V_{\lambda}(G)$ in the 
tensor product of $V_{\alpha}(G)$ and $V_\beta(G)$. 
The classical Littlewood-Richardson rule, which we shall refer to as LR PH,
implies that the stretching function 
$\tilde c_{\alpha,\beta}^\lambda (k) = c_{k \alpha, k \beta}^{k \lambda}$
associated with the Littlewood-Richardson coefficient has a
positive convex representation.

Plethysm PH   happens to be a fundamental open problem of
representation theory, older than the $P$ vs. $NP$ problem itself. It 
has been studied intensively in the last century, and is known to be
formidable. And  now,  as explained the third lecture, it also turns out to 
be  the heart of this approach towards the $P$ vs $NP$, the
$\#P$ vs. $NC$ problems.



A basic plan to prove Plethysm PH is given in GCT6.
It is partially 
implemented in GCT7 and 8. See Figure~\ref{fig:lift} for a pictorial
depiction of the plan. It strives  to extend the  proof of LR PH based 
on the theory of the  standard quantum group \cite{drinfeld,kashiwara,lusztig}.
There it
comes out as a consequence of a  (proof of a) deep positivity result
\cite{kazhdan,lusztig}, which
we shall refer to as LR PH0. It says that   the 
tensor product of two representations of the standard quantum group 
has a canonical basis \cite{kashiwara,lusztig} 
whose structure coefficients are all positive \cite{lusztig}
polynomials (i.e., polynomials with nonnegative coefficients).
The only known proof of this
result is based on the Riemann Hypothesis over finite fields 
proved in \cite{weil2},  and the related works \cite{beilinson}. 
This Riemann Hypothesis is  itself a deep positivity statement in mathematics,
from which   LR PH can  thus be 
deduced, as shown on the bottom row of Figure~\ref{fig:lift}.

If one were only interested in LR PH, one  does not 
need this  powerful machinery, because it has a  much simpler 
algebraic-combinatorial  proof. 
But the plan to extend the
proof of LR PH to Plethysm PH in GCT6,7,8 is like a huge
inductive spiral. To  make it work,  one  needs a 
stronger inductive hypothesis than Plethysm PH--this is precisely  Plethysm 
PH0 (which  will be
described in the third lecture; cf. Hypothesis~\ref{hplph0}).
Thus what is needed now 
is a systematic lifting  of the bottom arrow in Figure~\ref{fig:lift}
to the top, so as to complete the  commutative diagram, so to speak. 

Initial  steps in this direction have been taken in GCT7,8. 
First, GCT7 constructs a {\em nonstandard quantum group}, which
generalizes the notion of a standard quantum group \cite{drinfeld},
 and plays the
same role in the plethysm setting that the standard quantum group plays
in the LR setting. Second, GCT8 gives an algorithm to construct 
a canonical basis for a representation of the nonstandard quantum group
that is conjecturally correct and has the property Plethysm PH0,
which is a   generalization of LR PH0  supported by experimental
evidence.
Now what is needed to complete  the 
commutative digram in Figure~\ref{fig:lift} is an appropriate nonstandard 
extension of the Riemann hypothesis over finite fields and the related works
\cite{beilinson,weil2,kazhdan,lusztig}
from which  Plethysm PH0 can be deduced. This--the top-right corner 
of the diagram--is the   main  open problem at the heart of this approach. 

\section{How to prove OH or POH?} 
We do not  know, 
since the  proof of OH and POH 
would really depend on the explicit forms of the
polytopes that arise in   PH1/PH4, and we have no idea about them
at this point.
But GCT does suggest  that proving OH/POH  should be feasible 
``in theory''
since OH/POH  belong to NP/P, assuming PH1/4, and polynomial-time
is complexity theory stands for feasible ``in theory''. In other words,
GCT gives a reason to believe now that proving 
the  $P\not = NP$ conjecture should be feasible in theory, which 
was  always  doubted in the field of complexity theory so far, because 
the $P$ vs. $NP$ problem is a universal statement regarding all of mathematics
(that says theorems cannot be proven automatically). 
But, as we also know by now, 
there is a huge gap between  theory and  practice--e.g., 
just because  some problem is in $P$ does not 
necessarily mean that it is feasible in practice. Similarly,
the actual implementation of the GCT flip via positivity is expected to be 
immensely difficult ``in practice'', as Figure~\ref{fig:lift} suggests. 







\section{Is positivity  necessary?} \label{sposnece}
Finally,  if the positivity problems are so hard,  one may ask if 
they can not be avoided somehow. Unfortunately, there is a formidable 
barrier towards the $P$ vs. $NP$ and related problems, called the
{\em feasibility ($P$) barrier} (GCT6,GCTflip),
which seems universal in the sense that
any approach towards these problems would have to tackle it, not just GCT. 
The existing mathematical evidence suggests that any natural approach
to cross this barrier would have to say  something deep regarding positivity
(Plethysm PH/PH0)  either explicitly or {\em implicitly}, even if
the approach does not utter a word about algebraic geometry or
representation theory.
That is,  Plethysm PH and PH0   may indeed be 
the heart of the  fundamental lower bound problems in complexity theory;
a detailed story and a precise meaning of the key 
phrase {\em implicit} would appear in the revised version of GCTflip.

%\input{feasibility}









































 

































\begin{sidewaysfigure} 
\begin{center} 
\epsfig{file=lift.eps, scale=.8}
\end{center}
      \caption{A commutative diagram}
      \label{fig:lift}
\end{sidewaysfigure} 



\ignore{\begin{figure} 
\psfragscanon
\psfrag{P}{$P\not = NP$ and $\#P\not = NC$ conjectures (characteristic zero)}
\epsfig{file=barriers.eps, scale=1}
      \caption{The feasibility barrier towards $P$ vs. $NP$}
      \label{fig:barriers}
\end{figure}}



==> lecture1_maintext3.tex <==
\chapter{Basic plan} 
We now outline the basic  plan of GCT focussing on
the  permanent vs. determinant problem in characteristic zero. Recall that
this  says  $\perm(X)$  cannot be represented 
linearly  as the determinant of a polynomial size 
matrix.


\section{Characterization by symmetries} \label{scharsym}
We begin by observing that 
the permanent and the determinant are 
{\em exceptional} polynomial functions. By exceptional we mean
that they are  completely characterized by the symmetries in the 
following sense.


Let  $Y$ be a variable $m\times m$ matrix.
Let $\sym^m(Y)$ be the space of homogeneous forms of degree $m$ 
in the $m^2$ variable entries of $Y$. Then, by the  classical
representation theory,  $\det(Y)$ is the only form in $\sym^m(Y)$ 
such that, for any $A,B \in GL_m(\C)$ with $\det(A)\det(B)=1$, 

\noindent  {\bf (D):} $\det(Y)=\det(A Y^* B)$,

where $Y^*=Y$ or $Y^t$. 
Thus $\det(Y)$ is completely characterized 
by its symmetries, and hence, is  exceptional. We shall refer 
to this characteristic property of the determinant as property D
henceforth.

Similarly, $\perm(X)$ is the only form 
in the space of forms of degree $n$ in the entries of $X$ such that, 
for any diagonal or permutation matrices $A,B$, 

\noindent  {\bf (P):} $\perm(X)=\perm(AX^*B)$, 

where $X^*=X$ or $X^t$ and the product of the diagonal entries of $A$ (and $B$)
is one when it is diagonal. 
Thus $\perm(X)$ is also
completely characterized   by its symmetries, and hence, is
exceptional.
We shall refer 
to this characteristic property of the permanent as property P
henceforth.





Any proof technique for the permanent vs. the determinant problem
has to ultimately make a nontrivial use of these  symmetries
  which characterize them. Indeed, one can say that 
these characteristic  properties 
lie at the heart of the permanent vs. determinant problem, and until
a proof technique has made a nontrivial use of them, it has
not entered the heart of the problem.
The most obvious interpretation of the phrase 
nontrivial here is the following: 

\begin{defn} \label{dnontrivial}
We say that a proof technique for the permanent vs. determinant 
problem makes a {\em nontrivial use of symmetries} if it does not work
for any functions (in place of the permanent or the determinant)
which do not have
nontrivial symmetries.
\end{defn}

Since symmetries is a fundamental geometric concept, we define
a  {\em geometric} approach to the permanent vs. determinant problem as
any  approach based on nontrivial use of the symmetry properties
P and D in this sense.
The meanining of the phrase geometric in the 
$P$ vs. $NP$ problem is
similar, since the  permanent and the determinant
can be replaced with   (co)-NP
and $P$ complete functions which are similarly
characterized by symmetries [GCT1]
(in a weaker sense that is good enough for our purposes).

GCT is a geometric approach in this sense.
Representation theory and 
algebraic geometry enter inevitably into  it, because
to understand symmetries, representation theory (of groups of symmetries)
becomes indispensible, and to understand  deeper properties 
of representations,  algebraic geometry becomes indispensible. 




\section{Mathematical form of the  $\#P \not = NC$ conjecture} 
\label{sweaklec1}
Before going any further, we now state one concrete application of 
GCT in the form of a concrete lower bound result--namely a 
mathematical form of the 
$\#P \not = NC$ conjecture (Theorem~\ref{tgenweaklec1} below).

We begin by observing that 
the permanent vs. determinant conjecture clearly implies  that 
$\perm(X)$ of any $n \times n$ variable matrix $X$ can not be represented 
as an $NC$-computable polynomial in the traces of $\bar X^j$, $j \ge 0$,
$\bar X=B X C$
for any (possibly singular) $n\times n$ matrices $B$ and $C$, since
$X^j$ can be computed fast in parallel. This can be proved unconditionally.
In fact, something stronger.

\begin{prop}  \label{pweaklec1}
There do not exist (possibly singular) $n\times n$ complex
matrices $B$ and $C$  and a polynomial 
$e(w_0,\ldots, w_n)$ such that $\perm(X) = g(BXC)$, 
where $g(X)=e(\trace(X^0), \trace(X), \ldots, \trace(X^n))$. 
\end{prop}
This was referred to as 
the weak form of the $\#P$ vs. $NC$ problem in the original IAS lecture. 
The article \cite{} showed that this is indeed  weak 
by giving an  elementary
proof \cite{boris} for this result that is naturalizable, i.e.,
which cannot cross the
natural proof barrier \cite{} because it works for most functions in
place of the permanent. By weak we now mean provable by naturalizable 
techniques. The proof technique of
the quadratic lower bound \cite{ressayre}
for the permanent is also naturalizable.

We now state the much more nontrivial lower bound of GCT, which
was not stated in the IAS lecture, and which cannot be proved by
such naturalizable technqiues.
Hence, the  first goal in this context 
is to prove some weaker form of the $\#P \not = NC$ conjecture (nonuniform)
which cannot be proved by naturalizable proof techniques. 

For that, let us analyze why the proof techniques in \cite{boris,ressayre} 
are naturalizable. It is because they do not make nontrivial 
(Definition~\ref{dnontrivial}) use of the symmetries, which, as
we have already pointed out, is the heart of this problem. The moral of the 
story is that unless a proof technique makes a nontrivial use of the
symmetries, the natural proof  barrier would stand in the way. 
In a sense, this barrier 
forces a proof technique to enter into the heart of the problem.



So the basic idea is
to formulate a generalized weak form of the $\#P$ vs. $NC$ conjecture
whose proof  would essentially be forced to rely 
only on  the characteristic property P of the 
permanent, and thereby enter into the heart of the problem.  Any such
proof technique would automatically bypass the natural proof barrier
since most functions have no symmetries.  
Furthermore, it would
also automatically bypass the relativization \cite{solovay}
and the algebraic-degree 
[GCTweak]
 (algebrization \cite{aaronson}) barriers--the first because the symmetries are
algebraic/geometric, and the second because they  are  not  degree-based.
\ignore{Ultimately any proof technique for the permanent vs. determinant
conjecture has to prove some weaker 
form of this conjecture unconditionally to demonstrate that:
\begin{description} 
\item[A] It can bypass the relativization, natural-proof and algebraic-degree
(algebrization) barriers simultaneously, and that
\item[B] It has made a nontrivial use of the symmetry property P,
and thereby has entered into the heart of the problem.
\end{description}
By nontrivial, we mean  the proof technique does not work for
any function (in place of the permanent) if it does not have nontrivial
symmetries. 
%With the interpretation of the phrase nontrivial, 
%(B) implies (A) since most functions have no symmetries.


We  now describe one such  weak form which can be proved unconditionally
via GCT, and which thus shows that GCT meets criteria (A) and (B).}

To formulate the weak form,  we need a definition.

\begin{defn} 
A function $p(X)$ (of any degree) is called a  {\em generalized permanent} if it has exactly 
the same symmetries as that of the permanent; i.e.,
for all nonsingular $n\times n$ matrices $U$ and $V$, 
\[ p(U X V)=p(X) \mbox{\ iff\ } \perm(U X V)=\perm (X).\] 
\end{defn}

The precise description of the symmetries of the permanent  is given
by the property P. Hence, $U$ and $V$ above have to be permutation
or diagonal matrices (with product of the diagonal entries one if they
are diagonal), or 
product of such matrices.
There is just one generalized permanent of degree $n$, namely
the permanent itself. But in general (i.e., with no restriction on 
the degree) the space of generalized permanents has a highly nontrivial
structure that  is intimately linked  to some
fundamental problems of representation theory;
cf. Section{sweak} and  [GCT6].

The original nonuniform 
$\#P$ vs. $NC$  conjecture
implies that  any $\#P$-complete generalized permanent $p(X)$ of $\poly(n)$ 
degree cannot be expressed as an $NC$-computable polynomial of the 
traces of $\bar X^j$, $\bar X=B X C$, for any $n\times n$ complex
matrices $B$ and $C$, since $X^j$ is  $NC$-computable.
This implication of the nonuniform $\#P\not = NC$ conjecture can be proven 
unconditionally. In fact, something stronger:

\begin{theorem}[GCT6]

\noindent {\bf (The generalized weak form of the  $\#P$ vs. $NC$ problem)}

 \label{tgenweaklec1}
\noindent (a) Let $p(X)$ be any  generalized permanent.
Then there do not exist (possibly singular) $n\times n$ complex
matrices $B$ and $C$  and a polynomial 
$e(w_0,\ldots, w_n)$ such that 
\[p(X) = e(\trace(\bar X^0), \trace(\bar X), \ldots, \trace(\bar X^n))\] 
where $\bar X=B X C$.

\noindent (b) 
More generally, no generalized permanent of  $k$ $n\times n$ variable
matrices $X_1,\ldots,X_k$ (defined similarly)
can be expressed as a polynomial in 
the traces of  monomials in $\bar X_i$, $1\le i \le k$, $\bar X_i=B X_i C$,
for any $B$ and $C$. 
\end{theorem}

For some specific
generalized permanents (cf. Section~\ref{sweak}), this result again has
an elementary proof as in \cite{boris}. The nontrivial part of this 
result (which needs nonelementary proof) 
is that it holds for any generalized permanent.
Indeed the basic difference between the general and the weak setting is
the following. The general (i.e. the usual) $\#P$ vs. $NC$ conjecture
is such that if it is proved for one $\#P$-complete function (say
the permanent), it automatically 
holds for all $\#P$-completeness functions (because
of the theory of $\#P$-completeness). But there is no such completeness
theory at the weak level. Hence, a weak result for a specific 
generalized permanent, e.g. the permanent,
does not say anything about all (even $\#P$-complete)
generalized permanents. The generalized weak form is essentially meant 
to cover up this lack of completeness theory at the weak level.





The only thing that is common among  all generalized permanents is the
property P.  Hence a proof of this result is 
essentially  forced
to rely only on  this property,  and 
thereby bypass the natural proof, relativization, algebraic-degree and
algebrization barriers simultaneously.



This result is a mathematical
lower bound rather than a complexity theoretic lower bound in the sense
that it puts  no restriction on the computational complexity of $p(X)$ or
the polynomial $e(w_0, \ldots, w_n)$. If $e(w_0,\ldots,w_n)$
were $NC$-computable, then so would be $g(X)$ and $g(BXC)$, since traces are 
$NC$-computable. But the result does not require this. Nor does it
require $\#P$-completeness of $p(X)$. In that sense,
it is rather in the spirit of the classical result of Galois theory 
which says that a general polynomial cannot be solved by any number of
radical operations, without any restriction on the number of such
operations. Its complexity theoretic content  is that 
it demonstrates that GCT bypasses the barriers mentioned above.


\section{From nonexistence to existence}
The rest of this lecture  outlines  the GCT approach to 
the general permanent vs. determinant problem,
and then  points out 
the crucial steps in this plan which can be completely excecuted
in the weak case, but are conjectural at present in  the general case.

The first  step 
(GCT1,2) is to reduce this nonexistence problem--i.e., that there is no
small linear representation  of the permanent as a determinant--to
an existence problem--specifically, to the problem of proving 
existence of a family $\{O_n\}$ of obstructions; 
cf. Figure~\ref{fig:firststep}.
Here an {\em obstruction} $O_n$ is a proof-certificate of
hardness of $\perm(X)$, $X$ an $n\times n$ variable matrix,
just as the Kuratowski minor is a proof-certificate of the nonplanarity of a 
graph.  Specifically,  it is some 
algebro-geometric-representation-theoretic gadget
whose existence for every $n$  serves as a 
guarantee that $\perm(X)$ cannot be represented linearly as $\det(Y)$,
when $m=2^{\log^a n}$, $a>0$ fixed, $n\rightarrow \infty$ (i.e., for
$n$ greater than a large enough constant depending on $a$). 



\begin{figure} 
\begin{center}\psfragscanon
\psfrag{on}{$\{O_n\}$}
\epsfig{file=firststep.eps, scale=.8}
\end{center}
      \caption{Reduction from nonexistence to existence}
      \label{fig:firststep}
\end{figure}



This reduction to existence is carried out as follows (cf. lecture 2 for 
details).


First, we associate (GCT1) with 
the complexity class $\#P$ a family $\{X_{\#P}(n,m)\}$ of (group-theoretic)
class varieties (what this means is explained below),
and with the complexity class $NC$ a family of 
$\{X_{NC}(n,m)\}$ of (group-theoretic) class varieties such that: 
if $\perm(X)$, $\dim(X)=n$, can be represented linearly 
as $\det(Y)$, $\dim(Y)=m>n$, then 

\begin{equation} \label{eqembed} 
X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation} 

Each  class variety is a  (projective) algebraic variety, by which
we mean that it is the zero set of  a system of multivariate 
homogeneous polynomials with coefficients in $\C$  (akin to the 
usual curves  and surfaces). It is  group-theoretic in the 
sense that it is  constructed using group-theoretic operations 
and the general linear group $G=GL_l(\C)$, $l=m^2$, of $l\times l$ invertible
complex matrices acts on it. Here action means moving the points 
of the class variety around, just as $G$ moves the points of $\C^l$ around 
by the standard action via invertible linear transformations.
The goal is to show that the inclusion (\ref{eqembed}) is impossible
(obstructions are meant to ensure this);
cf. Figure~\ref{fig:class}. 

\begin{figure} 
\begin{center} \psfragscanon
\psfrag{xsharp}{$X_{\#P}(n,m)$}
      \psfrag{xnc}{$X_{NC}(n,m)$}
      \psfrag{g}{$G=GL_l(\C)$, $l=m^2$}
      \psfrag{Obstruction}{\mbox{Obstruction}}
\epsfig{file=class.eps, scale=.5}
\end{center}
      \caption{Class varieties}
      \label{fig:class}
\end{figure} 



Since each class variety has a $G$-action, the space of polynomial functions 
on each class variety has a  representation-theoretic structure, which 
puts constraints on which  representations of $G$ can live on that variety
(i.e., in the space of polynomial  functions on that variety).
Informally, an obstruction is an irreducible (minimal)  representation of $G$
that can live on $X_{\#P}(n,m)$ but not on $X_{NC}(n,m)$; 
cf. Figure~\ref{fig:class}.
Existence of  an obstruction $O_n$, for every $n$, assuming
$m=2^{\log^a n}$, $a>1$ fixed, implies  that the inclusion (\ref{eqembed}) 
is not possible, since  $O_n$ cannot live  on $X_{NC}(n,m)$.
Thus  an obstruction blocks the inclusion (\ref{eqembed}).


To define an obstruction formally, we need to recall some basic representation
theory.  By a classical result of Weyl, the irreducible 
(polynomial) representations of $G=GL_l(\C)$ are in one-to-one correspondence 
with the partitions  $\lambda$ of length at most $l$, by which we mean 
integral sequences $\lambda_1 \ge 
\lambda_2 \cdots \ge \lambda_k > 0$, $k\le l$, where  $k$ is called the  length
of $\lambda$. The irreducible 
representation of $G$ in correspondence with $\lambda$ is denoted 
by $V_\lambda(G)$, and is called the {\em Weyl module} of $G$ indexed by 
$\lambda$. Symbolically:

\[\mbox{Irreducible representations of } G \stackrel{\mbox{Weyl}}{\Longleftrightarrow} \quad \mbox{partitions} \ \lambda. \]  

\[\mbox{Weyl module  } V_\lambda(G)  \longleftrightarrow \lambda. \] 
Weyl also proved that every finite dimensional representation of $G$ 
can be decomposed into irreducible representations--i.e.,
can be written as a direct sum of Weyl modules. Thus Weyl modules 
are the basic building blocks of the representation theory of 
$G$, and every finite dimensional representation of $G$ can be thought
of as a complex building made out of these blocks. 


Now suppose $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$. 
Suppose to the contrary that 

\begin{equation} \label{eqembed2}   X_{\#P}(n,m) \subseteq X_{NC}(n,m).
\end{equation}

Let $R_{\#P}(n,m)$ denote the homogeneous coordinate ring of 
$X_{\#P}(n,m)$; i.e., the ring of polynomial functions 
\footnote{Though the  functions here are not functions in usual sense;
but let us  not worry about this} on $X_{\#P}(n.m)$. 
Let $R_{\#P}(n,m)_d$ be the degree-$d$-component of $R_{\#P}(n, m)$ consisting
of functions of degree $d$. We define $R_{NC}(n,m)$ and $R_{NC}(n,m)_d$
similarly. Since $X_{\#P}(n,m)$ has the action of $G$, $R_{\#P}(n,m)$ 
also has an action of $G$; i.e., it is a representation of $G$. Hence,
$R_{\#P}(n,m)_d$ is a finite dimensional representation of $G$. 
Similarly, $R_{NC}(n,m)$ is a representation of $G$, and $R_{NC}(n,m)_d$
a finite dimensional representation of $G$. 



If (\ref{eqembed2}) holds, then we get a natural map from $R_{NC}(n,m)$ to
$R_{\#P}(n,m)$ obtained by restricting a function on $X_{NC}(n,m)$ to
$X_{\#P}(n,m)$. %; cf. Figure~\ref{fig:restriction}.
By basic algebraic geometry, this map
is surjective and is a $G$-homomorphism.
Furthermore, it is degree-preserving. This means there
is a surjective $G$-homomorphism from $R_{NC}(n,m)_d$ to 
$R_{\#P}(n,m)_d$. Symbolically: 

\begin{equation} \label{eqsurjection}
R_{\#}(n,m)_d \leftarrow  R_{NC}(n,m)_d.
\end{equation}

\ignore{
\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{Xp}{\small $X_{\#P}(n,m)$}
\psfrag{Xnc}{\small $X_{NC}(n,m)$}
\epsfig{file=restriction.eps, scale=.6}
\end{center}
      \caption{Restriction}
      \label{fig:restriction}
\end{figure}
}

Let $R_{\#P}(n,m)_d^*$ denote the dual of $R_{\#P}(n,m)_d$; i.e., the 
set of linear maps from $R_{\#P}(n,m)_d$ to $\C$. Then (\ref{eqsurjection})
implies that there is an injective $G$-homomorphism from 
$R_{\#P}(n,m)^*_d$ to $R_{NC}(n,m)^*_d$. Symbolically: 

\begin{equation} \label{eqinclusion}
R_{\#}(n,m)_d^*  \hookrightarrow {NC}(n,m)_d^*.
\end{equation}

\begin{defn} (GCT2)
An obstruction $O_n$ is a Weyl module $V_\lambda(G)$ that 
occurs as a subrepresentation 
in $R_{\#P}(n,m)_d^*$  but not in $R_{NC}(n,m)_d^*$, for some $d$. 
We call $\lambda$ an {\em obstruction label}, and sometimes,
by abuse of notation, an obstruction as well.
\end{defn}

\begin{prop} (GCT2)
Existence of an obstruction $O_n$, for all $n\rightarrow \infty$, 
with $m=2^{\log^a n}$, $a>1$ fixed, implies $\perm(X)$, $\dim(X)=n$, 
cannot be represented linearly as 
$\det(Y)$, $\dim(Y)=m$. 
\end{prop}

This follows just from the definition of an obstruction, and 
leads to:

\begin{goal} \label{gobs} (GCT2)
Prove existence of an obstruction family $\{O_n=V_{\lambda_n}(G)\}$ using 
the  exceptional 
nature of $\perm(X)$ and $\det(Y)$, i.e., using the 
properties P and D in  Section~\ref{scharsym}).
\end{goal} 

\section{Obstructions in the weak case} \label{sobsweak}

The following result achieves this goal in the weak case 
(Theorem~\ref{tgenweaklec1}).
\begin{theorem} 
There exists an obstruction family $\{O_n\}$ in the generalized 
weak form of the $\#P$ vs. $NC$ problem.
\end{theorem}

This implies Theorem~\ref{tgenweaklec1}.
The notion of obstructions here is similar 
to the one in the general case. 

The proof of this result is based on the results of GCT1 and 2 in
geometric invariant theory \cite{mumford} and is outlined in the third lecture.
It produces  a {\em strongly  explicit} 
family $\{O_n=V_\lambda(G)\}$ of obstructions, with a different $G$
than in the general case.
This is strongly explicit in the sense (as explained in
the preface) that 
the specification $\lambda_n$ of each $O_n$
has polynomial, in fact,  $O(n)$ bitlength, and  
can be constructed in polynomial, in fact, $O(n)$ time (regardless of the 
complexity  of the polynomial $e$ in the statement of 
Theorem~\ref{tgenweaklec1}).

\noindent {\em Remark:}
There is also a second noncostructive proof of this result.
This gives a concrete evidence 
that explicit construction is not needed to cross the 
natural proof   barrier. Because 
any proof, even a nonconstructive one as this,
which makes nontrivial
use (cf. Definition~\ref{dnontrivial})
of the symmetry property P would automatically
bypass this barrier, since most 
functions have no symmetries, and also
the relativization and algebraic degree (algebrization) barriers.
But for some mysterious reasons  this nonconstructive
proof is harder than the explicit proof. Indeed, the whole proof
structure  here is such that its easiest implementation  yields 
obstructions explicitly 
whether one cares for them or not. We shall see the same pheonomenon
in the general case in what follows.


\section{Towards existence of obstructions in general via positivity}
We now proceed to describe the main results of GCT for the general
permanent vs. determinant problem in the context of
Goal~\ref{gobs}. 



Towards that end, we  associate with the class varieties 
certain representation-theoretic {\em stretching} functions. 
Let $F_{\lambda,n,m}(k)$ denote the number of occurances (multiplicity)  of
the Weyl module $V_{k\lambda}(G)$ in $R_{\#P}(n,m)^*$ (i.e. 
$R_{\#P}(n,m)^*_d$, for some $d$)  as a subrepresentation,
and $G_{\lambda,n,m}(k)$ the number of occurances of 
$V_{k\lambda}(G)$ in $R_{NC}(n,m)^*$. These are statistical functions
associated with the class varieties, where the statistics associates 
with every number (stretching parameter) $k$  
the multiplicity of the corresponding
Weyl module $V_{k\lambda}(G)$; cf. Figure~\ref{fig:statistics}.

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{l}{$\lambda$}
\psfrag{2l}{$2 \lambda$}
\psfrag{3l}{$3 \lambda$}
\psfrag{v1}{$V_\lambda(G)$}
\psfrag{v2}{$V_{2 \lambda}(G)$}
\psfrag{v3}{$V_{3\lambda}(G)$}
\epsfig{file=statistics.eps, scale=1}
\end{center}
      \caption{statistics}
      \label{fig:statistics}
\end{figure}


Let us  call a function $f(k)$ {\em quasipolynomial}, if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k)$ for all nonnegative integral $k=i$ modulo $l$;
here  $l$ is
called the period of the  quasi-polynomial. 
Thus  quasi-polynomials
are hybrids of  polynomial and periodic functions. 
We say that $f(k)$ is an 
{\em asymptotic quasipolynomial} if there exist 
$l$ polynomials $f_i(k)$, $1\le i \le l$, for some $l$, such that
$f(k)=f_i(k)$ for all nonnegative integral $k=i$ modulo $l$ for 
$k\ge a(f)$, for 
some nonnegative integer depending on $f$. The minimum 
$a(f)$ for which this holds is called the {\em deviation from 
quasipolynomiality}. Thus $f(k)$ is a (strict) quasipolynomial when this
deviation is zero.

A fundamental example of a quasi-polynomial is the Ehrhart quasi-polynomial
$f_P(k)$ of a polytope $P$ with rational vertices. It is defined
to be the number of integer points in the dilated polytope $kP$. By the 
classical result of Ehrhart, it is known to be a quasi-polynomial.
More generally, let $P(k)$ be a polytope parametrized by nonnegative
integral $k$: i.e., 
defined by a linear system of the form: 
\begin{equation} \label{eqpara}
A x \le k b + c,
\end{equation}
where $A$ is an $m \times n$ matrix, $x$ a variable $n$-vector, and 
$b$ and $c$ some constant $m$-vectors. Let $f_P(k)$ be the number 
of integer points in $P(k)$. We shall call it the Ehrhart function of
$P(k)$.  It is known to be  an asymptotic quasi-polynomial.
In what follows, we  denote a parametrized polytope $P(k)$ by 
just $P$. 




\begin{theorem} (GCT6) \label{tquasi}
The functions $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ 
are asymptotic quasi-polynomials. Furthermore, they 
are (strict) 
quasi-polynomials assuming that the singularities of the class varieties
$X_{\#P}(n,m)$ and $X_{NC}(n,m)$ are rational and normal. 

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem} 

Here a rational and normal  singularity means a singularity that is nice in
an algebro-geometric sense that we shall not elaborate here.
At present, we do not know if the singularities of the class varieties 
are indeed  rational and normal. A conservative conjecture would be  that 
they are not too bad, even if they are not strictly rational and normal,
because of the exceptional nature of the 
determinant and the permanent; 
i.e.,  the deviation from quasipolynomiality
of $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ is 
small in a sense to be made precise 
later (cf. the remarks after Hypothesis~\ref{hph1}).

The proof of Theorem~\ref{tquasi}
follows from a detailed study of the behaviour
of the singularities of class varieties under the action of the 
group $G$. This is based on
\begin{enumerate} 
\item The 
resolutions of singularities in characteristic zero
\cite{hironaka}: 
this  roughly says 
that the singularities of any algebraic variety in characteristic zero
can be untangled (resolved) nicely in a systematic fashion; cf.
 Figure~\ref{fig:resolution}.
\item Cohomological works of Boutot, Brion,  Flenner, Kempf  and others
based on this resolution; cf.  \cite{boutot,dehy} and
GCT6 for the history and other references.
\end{enumerate} 


\begin{figure} 
\begin{center} 
\epsfig{file=resolution.eps, scale=.5}
      \caption{Resolution}
      \label{fig:resolution}
\end{center}
\end{figure}


As such, this proof is highly nonconstructive. It gives no effective
bound on the period $l$--it just says that $l$  is finite.





The following hypothesis 
says that $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ 
can be realized as the Ehrhart functions  of parametrized  polytopes.

\begin{hypo} {\bf (PH) [Positivity Hypothesis]} \label{hph} (GCT6)

\noindent (a) For every $\lambda,n,m\ge n$, 
there exists   a parametrized  polytope $P=P_{\lambda,n,m}$ 
such that 
\begin{equation} \label{eqP}
F_{\lambda,n,m}(k)=f_P(k).
\end{equation} 
It is also assumed here that there exists for $P_{\lambda,n,m}$ a specification
of the form (\ref{eqpara}),
 where $A$ is independent of $\lambda$, and $b$ and $c$ 
are  piecewise homogeneous linear functions of $\lambda$.


\noindent (b) There exists a similar parametrized 
 polytope  $Q=Q_{\lambda,n,m}$  such that
\begin{equation} \label{eqQ}
G_{\lambda,n,m}(k)=f_Q(k).
\end{equation}


Analogous positivity hypothesis also holds 
for the $P$ vs. $NP$ problem in characteristic zero.
\end{hypo} 


If such $P$ and $Q$ exist, their dimensions are guaranteed to be
small by the proof of Theorem~\ref{tquasi}: specifically,
the dimension $P$ is guaranteed to be bounded by a 
polynomial in $n$, and the dimension of $Q$ 
by a polynomial in $m$.
There is a variant of PH (b), which is good enough for our purposes (cf.
Lecture 3, Hypothesis~\ref{hphvariant}),
wherein  the dimension of $Q$ is also guaranteed
to be bounded by a polynomial in $n$ (but independent 
of $m$), if the length of $\lambda$ is $\poly(n)$ (as it would be in 
our applications).






When PH holds, we say that $F_{\lambda,n,m}(k)$ and 
$G_{\lambda,n,m}(k)$ have  {\em positive convex representations}. 
Here positivity refers to the fact that the Ehhart function 
$f_P(k)$ is a positive expression:
\[ f_P(k)=\sum_{v} 1,\] 
where $v$ ranges over all integer points in $P(k)$--there are no 
alternating signs in this expression.
Convexity refers to the  convexity of the polytopes $P(k)$ and $Q(k)$. 


But, a  priori, it is not at all clear why PH should  even hold. 
Many numerical functions in algebraic geometry are 
asymptotic quasi-polynomials (e.g., the Hilbert function 
\footnote {Hilbert function $h_Z(k)$ of a projective algebraic variety $Z$
is defined to be $\dim(R(Z)_k)$, where $R(Z)$ is the homogeneous coordinate 
ring of $Z$ and $R(Z)_k$ its degree $k$-component.} of any projective
variety), but they rarely have positive convex representations.
PH is expected to hold for $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$ 
because of the exceptional nature of the determinant and the permanent. 
One concrete evidence is provided by the proof of the weak form 
(Thoerem~\ref{tgenweaklec1}).
Analogous PH that arises in this weak setting can 
proven unconditionally.
For  mathematical evidence and justification
in support of  general PH, see  GCT6,7, and 8. 


The hypothesis 
PH alone is not sufficient to prove the existence of obstructions.
The precise statement of a sufficient condition is given in 
the theorem below.




\begin{theorem} (GCT6) \label{tgct6}
There exists a family $\{O_n\}$ of obstructions 
for the  $\#P$ vs. $NC$ problem in characteristic zero, 
for $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$, 
assuming, 

\begin{enumerate} 
\item PH, and
\item OH (Obstruction Hypothesis): 

For all $n\rightarrow \infty$,  there exists $\lambda$ such that 
$P_{\lambda,n,m}(\infty)=\mbox{lim}_{k\rightarrow \infty} P(k) 
\not = \emptyset$ and $Q_{\lambda,n,m}(k)=\emptyset$ for all (large enough)
$k$.
\end{enumerate}

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem}

Mathematical evidence and arguments in support of OH are given in GCT6.
The analogous weak OH that arises in the context of the generalized 
weak form can be  proven unconditionally.

We call  $\lambda$ a {\em relaxed obstruction}
(or rather, relaxed obstruction-label)
if it satisfies OH. In this case, $k\lambda$, for some integer $k\ge 1$ is
an obstruction--we just have to choose $k$ large enough 
so that 
$P_{\lambda,n,m}(k)$ contains an integer point
but $Q_{\lambda,n,m}(k)$ does not.
Henceforth, whenever we say obstruction, we actually mean relaxed 
obstruction.

There is a fundamental difference between the nature of PH and OH.
PH is a {\em mathematical hypothesis}, because there is no 
constraint on what $m$ should be in comparison to $n$ in its statement.
In contrast, OH is a {\em complexity theoretic hypothesis}, because 
$m$ needs to be small in comparison to $n$ for it to hold.


%\subsection{Why should PH  and OH hold?} 

%Mathematical evidence for this is given in GCT2,4,6,7,8.
%We shall discuss some of this  in the third lecture.


\section{The flip: Explicit construction of obstructions} 
\label{sflip}
In principle PH may have a nonconstructive proof (like that
of Theorem~\ref{tquasi})  which only tells  that such polytopes 
exist without explicitly constructing them. But proving OH may not be feasible
unless the polytopes $P$ and $Q$ in PH are given explicitly.
This  suggests the following strategy for proving 
existence of obstructions proposed in  GCT6 and  GCTflip.


\noindent (1) Prove the following stronger explicit form 
of PH, which is reasonable since the polytopes $P$ and $Q$, if they exist,
are already guaranteed to be of small (polynomial) dimension:

\begin{hypo} {\bf (PH1)}  \label{hph1} (GCT6)

\noindent (a) There exists an {\em explicit} 
polytope $P_{\lambda,n,m}$ 
as in  PH (a).
Explicit means: 

\begin{enumerate}
\item  The polytope is specified by an explicit system of linear constraints,
where the bitlength of (the description of) 
each constraint is  $\poly(n,\bitlength{\lambda}, \bitlength{m})$.
Here and in what follows, $\bitlength{z}$ denotes the bitlength of the 
description of $z$.

\item  The membership problem for the polytope
$P_{\lambda,n,m}(k)$  also 
belongs to the complexity class $P$.
That is,  given a point $x$, whether it belongs to $P_{\lambda,n,m}(k)$ 
can also be decided in $\poly(\bitlength{x},\bitlength{\lambda},
n,\bitlength{m})$
time.
Furthermore, we assume that if $x$ does not belong to the polytope,
then the membership algorithm also gives a hyperplane separating 
$x$ from the polytope in the spirit of \cite{lovasz}. 
\end{enumerate} 

\noindent (b) There exists a similar  explicit 
polytope $Q_{\lambda,n,m}$  satisfying   PH (b). 
\end{hypo}

\noindent {\em Remark 1:} 
Note the occurence of  $\bitlength{m}$  instead of $m$ in the polynomial
bounds in (a) (which implies that the bounds here become $\poly(n)$
when $m<2^n$ and $\bitlength{\lambda}=\poly(n)$). 
The reasons for this will be explained in Lecture 3 
(cf. remarks after Hypothesis~\ref{hph1restatement}). 
In contrast, the polynomial bounds for the polytope in (b)  depend on 
$m$, not $\bitlength{m}$. 
But there are  variants of PH (b) and PH1 (b), 
(cf. Hypotheses~\ref{hphvariant} and \ref{hph1tilde} in  Lecture 3), 
which are enough for our purposes, 
wherein the polynomial bounds depend on the bitlength of $\lambda$,
but not on $m$.
In what follows, we assume that PH (b) and PH1 (b) have been replaced 
with these variants.

 


\noindent {\em Remark 2:} 
In particular, PH1 implies that the functions $F_{\lambda,n,m}(k)$ and
$G_{\lambda,n,m}(k)$ belong to the complexity class $\#P$. 
It can be shown that it 
also implies that the deviation from quasipolynomiality 
of $F_{\lambda,n,m}(k)$ is small, specifically, 
$2^{O(\poly(\bitlength{\lambda},n,\bitlength{m}))}$--thus the bitlength
of the deviation is polynomial. This says
that the deviation from rationality and normality of the singularities
of the class variety $X_{\#P}(n,m)$ is small (cf. Theorem~\ref{tquasi}).
Similarly for $Q_{\lambda,n,m}(k)$ and $X_{NC}(n,m)$. 

Like PH, PH1 is also a mathematical hypothesis in the sense that
it puts  no constraint on what $m$ should be in comparison to $n$. 
Of course, unlike PH, there is some complexity theoretic aspect to it, 
but it is secondary in comparison to the complexity-theoretic aspect of 
 OH, since smallness  of $m$ with respect to  $n$ is the 
crux of the lower bound  problems under consideration. 





\noindent (2a) {\bf [The flip]}

Let $m=2^{\log ^a n}$, for a fixed $a>1$. 
Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
show existence of  an {\em explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of (relaxed) obstructions  satisfying OH. 
We say that an obstruction (proof-certificate) 
$\lambda_n$ is {\em explicit} if is ``short'' and ``easy to verify'':


\begin{enumerate} 
\item  Short: This means its bitlength $\bitlength{\lambda_n}$ 
is $\poly(n)$,
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  

\item Easy to verify: given $n, m \le 2^{n}$ and 
$\lambda_n$, whether 
$\lambda_n$ is a valid obstruction 
can be verified 
in $\poly(n,\bitlength{\lambda})$ time. In particular, this is
$\poly(n)$ when $\bitlength{\lambda}=\poly(n)$. 
\end{enumerate}

Existence of an explicit family of obstructions is equivalent to saying
that the problem of deciding existence of obstructions belongs to $NP$.
This definition of explicitness is quite natural since the class $NP$ 
is a class of problems whose proof-certificates (witnesses) are 
short and easy to verify. As such, the flip--going for 
explicit  obstructions--is
a proof-strategy that is literally given to us on a platter 
by the $P$ vs. $NP$ 
problem itself. Why it is called flip will be explained later.


It should be stressed that we are primarily interested in only proving 
existence of obstructions. Whether they are explicit or not 
does not really matter in the original statement of the problem.
But we need to know the polytopes $P$ and
$Q$ explicitly (as in PH1)  so that proving OH is feasible. 
%In other words,   if we do not
%even know what the polytopes $P$ and $Q$ look like, 
%it seems unlikely that anything  could be said regarding OH. 
But once  PH1 is proved, existence of an explicit family follows
automatically,   as a bonus, whether we care for it or not. 

To see why, let us observe that 
the second condition above  (ease of verification) follows directly
from PH1 and the polynomial time algorithm for 
linear programming on  polytopes given by separation oracles \cite{lovasz}. 
Shortness  also follows from PH1. 

Thus it is as if the $P$ vs. $NP$ problem is forcing us to go
for explicit obstructions.


\noindent (2b) {\bf [The strong flip (optional)]} 

Using the explicit forms of the polytopes $P$ and $Q$ in PH1,
construct (rather than just show existence of) 
a {\em strongly explicit} family $\{O_n=V_{\lambda_n}(G)\}$ 
of obstructions  satisfying OH. We say that an explicit family 
of obstructions is strongly explicit if,
for each $n$, a valid obstruction-label
$\lambda_n$ can be constructed in $\poly(n)$ time.
In particular, the height and the bitlength of
 $\lambda$ is $\poly(n)$ (short) 
regardless what $m$ is, as long as it is $\le 2^{\log^a n}$, for some fixed
$a>1$.  


For the purposes of the lower bound problems that we are interested in, the
flip (just explicit  
existence) would suffice and the stronger flip (explicit construction)
is optional. But the stronger flip can give us deeper insight into these
lower bound problems; cf. GCTflip for more on this.

Now we turn to a few obvious questions.



\section{What has been achieved by all this?: The meaning of the flip} 
\label{smeaning}
Let us now see what has been achieved so far
in the context of the 
$\#P\not = NC$ conjecture in the nonuniform setting (characteristic zero),
the argument for the $P$ vs. $NP$ problem in characteristic zero
being  similar. 
At  first glance,
it may seem that all that GCT has achieved 
is to exchange a known difficult problem of 
complexity theory with a new very difficult problem of algebraic geoemtry.
In order to see that something is gained in exchange let us reexamine the 
original question.

The goal of the original  conjecture is to prove that 
$\perm(X)$, $\dim(X)=n$,  cannot be computed by an arithmetic circuit $C$
of size $m=\poly(n)$, or more generally,
$m \le 2^{\log^a n}$, for some fixed $a>1$, and depth $O(\log^a n)$.
Symbolically, 
let  $f_C(X)$ denote the function computed by $C$. Then we want to prove that
\begin{equation} \label{eqioh} 
 {\bf (IOH):}  \forall n \ge n_0 \forall C \exists X:
\perm(X)\not = f_C(X),
\end{equation} 
where $n_0$ is a sufficiently large constant.
For given $X$ and $C$ of $\poly(n)$ size, the problem 
of deciding if  $\perm(X) \not = f_C(X)$
belongs to $\#P$ (or rather, $P^{\#P}$). 
Since there are two alternating layers of quantifiers in (\ref{eqioh}),
the problem of verifying it belongs to $\Pi_2^{\#P}$, 
which is very high in the complexity hierarchy
(cf. Figure~\ref{fig:IOHcomplexity}).
Hence, we  refer to the original hypothesis (\ref{eqioh}) 
to be proven  as IOH 
(Infeasible Obstruction Hypothesis). Of course, IOH is expected to 
be a tautology, and hence is expected to  be verifiable in $O(1)$ time--but
we do not know that as yet. 



\begin{sidewaysfigure} 
\begin{center}
\psfragscanon
\psfrag{sigma2p}{{\small $\Pi^2 \#P$}}
\psfrag{sigma1p}{$\Sigma^1 \#P$}
\psfrag{P}{{\small $P$}}
\psfrag{NP}{{\small $NP$}}
\psfrag{T}{$T$}
\psfrag{#P}{$\# P$}
\psfrag{inNP}{$\in NP$}
\psfrag{inP}{$\in P$}
\psfrag{insigma2p}{$\in \Pi^2 \#P$}
\psfrag{PHplus}{PH1}
\psfrag{PHtil}{$PH^\dagger$}
\epsfig{file=IOHcomplexity.eps, scale=.8}
\end{center}
      \caption{Positivity as a means to eliminate the quantifiers and 
reduce the complexity of the  obstruction hypothesis}
      \label{fig:IOHcomplexity}
\end{sidewaysfigure}



Equivalently, the goal of IOH 
is to prove existence of a {\em trivial obstruction},
which is a table that lists for each $C$ as above a counterexample  $X$ so that
$\perm(X)\not = f_C(X)$; cf. Figure~\ref{fig:trivial}.
The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$ and depth
$O(\log^a n)$. Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. (Well, only
if the underlying field of computation is finite. For infinite fields, 
such as $\Q$ or $\C$ in this paper, 
there is another notion of a trivial obstruction (cf. 
GCT6). But let us imagine that the underlying
field is finite for this argument.)
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time to decide if such a table exists and construct 
one (optional) for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. That is why we 
call  this trivial, brute force 
strategy of proving IOH, based on existence of trivial obstructions,
an {\em infeasible strategy}. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{eq}{$\perm(X)\not = f_C(X)$}
\epsfig{file=trivial.eps, scale=.5}
\end{center}
      \caption{A trivial obstruction}
      \label{fig:trivial}
\end{figure}


In contrast, assuming PH1, the problem  of verifying OH belongs 
to $NP$ as we have already observed. Thus, assuming PH1, we have 
transformed the original infeasible obstruction 
hypothesis $IOH \in \Pi_2^{\#P}$ to a new  obstruction hypothesis 
$OH \in NP$, in the process bringing down the time to verify an obstruction
from  exponential (for the original trivial obstruction) to polynomial
(for the new obstruction); cf. Figure~\ref{fig:IOHcomplexity}.  
It is crucial here that PH1, the main tool for this reduction, is a 
mathematical hypothesis,  not complexity-theoretic (cf. the remarks
after Theorem~\ref{tgct6} and Hypothesis~\ref{hph1}).
The task of verifying  an obstruction has also been 
transformed from the infeasible (exponential-time) to the feasible 
(polynomial-time). Hence the name of this strategy: the flip,
from the infeasible to the feasible.
Positivity (PH1) is used in the flip as a means  to
eliminate the quantifying variables in IOH and bring down the 
 complexity of the obstruction hypothesis;
cf. Figure~\ref{fig:IOHcomplexity}. 




This process can be extended further. Assuming an additional
positivity hypothesis PH4 specified below,
$OH \in NP$ can be transformed 
to POH (Positivity Obstruction Hypothesis) that belongs to $P$; i.e.,
which can be verified in polynomial time, and an obstruction,
if it exists, can also be constructed in polynomial time; 
cf. Figure~\ref{fig:IOHcomplexity}. (The hypothesis is called PH4 instead
of PH2, because PH2 and PH3 are some other positivity hypotheses in GCT6
that complement PH1). 
Once this final positivity hypothesis POH is proven, the obstruction
hypothesis is reduced to a tautology (FOH: Final Obstruction Hypothesis),
which can be verified in
$O(1)$ time. This  would then give us 
the final $O(1)$-size  proof. 

Thus the basic idea of the flip is to use positivity systematically
as a means to eliminate the quantifiers  and reduce the complexity 
of the  obstruction hypothesis until it is finally
reduced to  an $O(1)$-time verifiable  tautology;
cf. Figure~\ref{fig:IOHcomplexity}. 

Now let us specify PH4 and POH.
Towards that end, let  $k \le l=m^2$ be the length of $\lambda$.
Define 

\begin{equation} 
\begin{array}{l}
\bar P_{n,m}= \{ \lambda: P_{\lambda,n,m} \not = \emptyset \} \subseteq \C^k, \\
\bar Q_{n,m}= \{ \lambda: Q_{\lambda,n,m} \not = \emptyset \} \subseteq \C^k.
\end{array}
\end{equation}

\begin{theorem} 
The sets $\bar P_{n,m}$ and $\bar Q_{n,m}$ are convex polytopes in $\C^k$.
\end{theorem} 
This follows from some fundamental results in geometric invariant theory
\cite{mumford}. 

Then: 

\begin{hypo}  {\bf PH4} (GCT6)
The membership problems for these polytopes belong to 
$P$ and so also the problem of deciding if $\mbox{vol}(\bar P_{n,m}
\setminus \bar Q_{n,m})$, the volume of the relative complement 
$\bar P_{n,m} \setminus \bar Q_{n,m}$, is nonzero (positive);
i.e. if $\bar P_{n,m} \not \subseteq \bar Q_{n,m}$. By polynomial time,
we mean $\poly(n,l,\bitlength{m})$ time. This is $\poly(n)$,
if $m\le 2^{o(n)}$ and $l =\poly(n)$. 
\end{hypo}

\begin{hypo} {\bf (POH)}

For all $n\rightarrow \infty$, assuming $m=2^{\log^a n}$, $a>1$ fixed, 

\[ \mbox{vol}(\bar P_{n,m} \setminus \bar Q_{n,m}) > 0, \] 

for $k=(n+1)^2$. 
\end{hypo} 

\ignore{
Thus POH says that  the line-shaded area in Figure~\ref{fig:POH} has positive
volume for all large enough $n$. 

\begin{figure} 
\begin{center} 
\psfragscanon
\psfrag{P}{$\bar P_{n,m}$}
\psfrag{Q}{$\bar Q_{n,m}$}
\epsfig{file=POH.eps, scale=1}
\end{center}
      \caption{POH}
      \label{fig:POH}
\end{figure}
}

\section{How to prove PH?}  \label{sphprove}
There is  a basic prototype of PH in representation theory,
which will be described in detail towards the end of Lecture 3. We shall
refer to it  as Plethysm PH. It says that the stretching functions 
akin to $F_{\lambda,n,m}(k)$ and $G_{\lambda,n,m}(k)$
associated with  fundamental  multiplicities 
in representation theory called plethysm constants also have analogous 
positive convex representations. 

This  is   known for a very special case of the plethysm constant 
called the  Littlewood-Richardson (LR) coefficient
$c_{\alpha,\beta}^\lambda$. It is  defined to be 
the number of occurances of the Weyl module $V_{\lambda}(G)$ in the 
tensor product of $V_{\alpha}(G)$ and $V_\beta(G)$. 
The classical Littlewood-Richardson rule, which we shall refer to as LR PH,
implies that the stretching function 
$\tilde c_{\alpha,\beta}^\lambda (k) = c_{k \alpha, k \beta}^{k \lambda}$
associated with the Littlewood-Richardson coefficient has a
positive convex representation.

Plethysm PH   happens to be a fundamental open problem of
representation theory, older than the $P$ vs. $NP$ problem itself. It 
has been studied intensively in the last century, and is known to be
formidable. And  now,  as explained the third lecture, it also turns out to 
be  the heart of this approach towards the $P$ vs $NP$, the
$\#P$ vs. $NC$ problems.



A basic plan to prove Plethysm PH is given in GCT6.
It is partially 
implemented in GCT7 and 8. See Figure~\ref{fig:lift} for a pictorial
depiction of the plan. It strives  to extend the  proof of LR PH based 
on the theory of the  standard quantum group \cite{drinfeld,kashiwara,lusztig}.
There it
comes out as a consequence of a  (proof of a) deep positivity result
\cite{kazhdan,lusztig}, which
we shall refer to as LR PH0. It says that   the 
tensor product of two representations of the standard quantum group 
has a canonical basis \cite{kashiwara,lusztig} 
whose structure coefficients are all positive \cite{lusztig}
polynomials (i.e., polynomials with nonnegative coefficients).
The only known proof of this
result is based on the Riemann Hypothesis over finite fields 
proved in \cite{weil2},  and the related works \cite{beilinson}. 
This Riemann Hypothesis over finite fields 
is  itself a deep positivity statement in mathematics,
from which   LR PH can  thus be 
deduced, as shown on the bottom row of Figure~\ref{fig:lift}.

If one were only interested in LR PH, one  does not 
need this  powerful machinery, because it has a  much simpler 
algebraic-combinatorial  proof. 
But the plan to extend the
proof of LR PH to Plethysm PH in GCT6,7,8 is like a huge
inductive spiral. To  make it work,  one  needs a 
stronger inductive hypothesis than Plethysm PH--this is precisely  Plethysm 
PH0 (which  will be
described in the third lecture; cf. Hypothesis~\ref{hplph0}).
Thus what is needed now 
is a systematic lifting  of the bottom arrow in Figure~\ref{fig:lift}
to the top, so as to complete the  commutative diagram, so to speak. 

Initial  steps in this direction have been taken in GCT7,8. 
First, GCT7 constructs a {\em nonstandard quantum group}, which
generalizes the notion of a standard quantum group \cite{drinfeld},
 and plays the
same role in the plethysm setting that the standard quantum group plays
in the LR setting. Second, GCT8 gives an algorithm to construct 
a canonical basis for a representation of the nonstandard quantum group
that is conjecturally correct and has the property Plethysm PH0,
which is a   generalization of LR PH0  supported by experimental
evidence.
Now what is needed to complete  the 
commutative diagram in Figure~\ref{fig:lift} is an appropriate nonstandard 
extension of the Riemann hypothesis over finite fields and the related works
\cite{beilinson,weil2,kazhdan,lusztig}
from which  Plethysm PH0 can be deduced. This--the top-right corner 
of the diagram--is the   main  open problem at the heart of this approach. 

\section{How to prove OH or POH?} 
We do not  know, 
since the  proof of OH and POH 
would really depend on the explicit forms of the
polytopes that arise in   PH1/PH4, and we have no idea about them
at this point.
\ignore{GCT does suggest  that proving OH/POH  should be feasible 
``in theory''
since OH/POH  belong to NP/P, assuming PH1/4, and polynomial-time
is complexity theory stands for feasible ``in theory''. 
In other words,
GCT gives a reason to believe now that proving 
the  $P\not = NP$ conjecture should be feasible in theory. Even this
was  always questioned  in the field of complexity theory so far, because 
the $P$ vs. $NP$ problem is a universal statement regarding all of mathematics
(that says theorems cannot be proven automatically).
But, as we also know by now, 
there is a huge gap between  theory and  practice--e.g., 
just because  some problem is in $P$ does not 
necessarily mean that it is feasible in practice. Similarly,
the actual implementation of the GCT flip via positivity is expected to be 
immensely difficult ``in practice'', as Figure~\ref{fig:lift} suggests. 
}






\section{Is positivity  necessary?} \label{sposnece}
\ignore{
Though the statement of this result is elementary, its proof is nonelementary,
as expected,  since the generalized permanents are highly nontrivial
and mathematically formidable objects. Specifically, the problem
of finding a $\#P$-basis for the space of generalized permanents 
is intimately related to some formidable problems of representation
theory and algebraic geometry,
and the  simplest analogue of this problem 
which can be solved at present  \cite{}
requires the deep Riemann Hypothesis over finite fields \cite{} for its
proof; cf. Section~\ref{}.
The proof of Theorem~\ref{} proceeds at an abstract level 
through algebraic geometry and representation theory without
having to know anything about such a basis.
At present, it is open if there is any alternative 
weaker form of the $\#P \not = NC$  conjecture,
which cannot be proved by relativizable, low-degree or 
naturalizable  techniques, but which can still be proved by elementary 
or not so  nonelementary techniques; that is, whether the earlier known
barriers mentioned above can 
be simultaneously bypassed in an elementary way in the context of 
the $\#P$ vs. $NC$ (or $P$ vs. $NC$  or $P$ vs. $NP$) problem.


\section{Why are we going for explicit obstructions?}
In a sense, the proof of the weak form turns out to be nonelementary
because of the difficulty of explicit construction. Specifically, algorithm 
to construct an obstruction $O_n$ for each $n$ is very simple, but to
show that it is correct requires nontrivial algebraic geometry,
just as the construction 
of an explcit family of Ramanujan graphs in \cite{} is very simple,
but to show that it is correct requires nontrivial algebraic geometry.
We already know, e.g. from this example of Ramanujan graphs, that 
explicit constructions can require highly nonelementary techniques.
So the question now arises: why are we going for such difficult explicit
constructions? Can they not be avoided somehow? 
After all, to solve the original problem we only need to show existence
of obstructions. We do not have to construct them explicitly.

Furthermore,  explicit construction is not needed to 
cross any of the barriers mentioned above (e.g. the natural-proof-barrier).
This is because {\em any} proof technique which uses symmetries of the
permanent would automatically bypass the natural-proof barrier
in the context of the permanent vs. determinant problem,
even if it does not utter a word about explicit construction, since
most functions have no symmetries. Indeed, the weak form of 
the generalized $\#P$ vs. $NC$ problem itself has two proofs, one
purely nonconstructive and one through explicit construction--the major 
chunk of both proofs being  the same, except for the last step,
which is carried out via a counting argument in the former proof and via
explicit construction in the latter. Since the nonconstructive proof too
is based on symmetries, it also crosses the natural-proof barrier.
This provides a concrete evidence that explicit construction is not 
necessary for crossing the earlier known  barriers.

Then why are we still going for explicit construction? 
Before we go any further, we wish to briefly state  the motivation
behind  going for the flip (explicit construction),
since this is an important issue. 
}

Finally,  if the positivity problems are so hard,  one may ask if 
they can not be avoided somehow. Unfortunately, there is a formidable 
barrier towards the $P$ vs. $NP$ and related problems, called the
{\em feasibility ($P$) barrier} (GCT6,GCTflip),
which seems universal in the sense that
any approach towards these problems would have to tackle it, not just GCT. 
The flip, i.e., explicit construction of obstructions, is the most natural
and obvious way to cross this barrier, and it also seems to be 
among the easiest. The 
existing mathematical evidence suggests that any such natural approach
to cross this barrier would have to say  something deep regarding positivity
(Plethysm PH/PH0)  either explicitly or {\em implicitly}, even if
the approach does not utter a word about algebraic geometry or
representation theory.
That is,  Plethysm PH and PH0   may indeed be 
the heart of the  fundamental lower bound problems in complexity theory;
a detailed story and a precise meaning of the key 
phrase {\em implicit} would appear in the revised version of GCTflip.

%\input{feasibility}









































 

































\begin{sidewaysfigure} 
\begin{center} 
\epsfig{file=lift.eps, scale=.8}
\end{center}
      \caption{A commutative diagram}
      \label{fig:lift}
\end{sidewaysfigure} 



\ignore{\begin{figure} 
\psfragscanon
\psfrag{P}{$P\not = NP$ and $\#P\not = NC$ conjectures (characteristic zero)}
\epsfig{file=barriers.eps, scale=1}
      \caption{The feasibility barrier towards $P$ vs. $NP$}
      \label{fig:barriers}
\end{figure}}



==> lecture3_2.tex <==
\chapter{Positivity}
In this lecture, we study   positivity  hypotheses in mathematics 
in the context of the problem of showing  existence of obstructions 
(Conjecture~\ref{cgct2obs}) and the $P$-barrier (Section~\ref{spbarrier}). 

Henceforth, we let 
$G=SL(Y)$ instead of $GL(Y)$ and  $H=SL(X)$ instead of $GL(X)$. This makes
no essential difference since our ambient space is $P(V)$, and two points in
$V$ differing by a nonzero scalar correspond to the same point in $P(V)$.
Thus everything discussed in the first two lectures goes through for this $G$ 
and $H$ as well.
This lecture assumes  more familiarity 
with representation theory that in the previous lectures;   Appendix
covers  the additional concepts needed here. 



\section{On the $G$-module structure of the homogeneous coordinate rings
of the class varieties} \label{sgmodule}

Given $v \in P(V)$, let $\hat v$ denote any nonzero point on the line
corresponding to $v$ in $P(V)$. Let $\hat g= \det(Y) \in V$ (not $P(V)$),
and $\hat h = \perm(X) \in W$ (not $P(W))$. Let $G_{\hat g} \subseteq G$
and $H_{\hat h}$ be their stabilizers. 


\begin{theorem} (GCT2) \label{tgct2first}

\noindent (1) $V_\lambda(G)$ occurs in $R_V[g]^*$ (i.e., in $R_V[g]_d^*$, for
some $d$) iff it contains a $G_{\hat g}$-invariant (i.e, a trivial 
subrepresentation--a fix point). 

\noindent (2) $V_\pi(H)$ occurs in $R_W[h]^*$ iff $V_\pi(H)$ contains an
$H_{\hat h}$-invariant. 
\end{theorem} 

This reduces some questions concerning  algebraic geometry of the class 
varieties to those concerning representation theory of the associated
group  triples (cf. Observation~\ref{obstriple} and the remarks after 
it)--or rather,
the  associated primary 
couples in this case--in keeping with the basic plan 
discussed in  Section~\ref{sonexi}.

It is easy to see that $G_{\hat g}$ is reductive (Definition~\ref{dreductive})
from its description in 
the proof of Proposition~\ref{pchar}. Hence 
$V_\lambda(G)$ contains a $G_{\hat g}$-invariant iff
the dual $V_\lambda(G)^*$ does. Thus, this theorem also holds if we replace
$V_\lambda(G)$ and $V_\pi(H)$ by $V_\lambda(G)^*$ and $V_\pi(H)^*$,
respectively. 


\proof We will only prove (1), (2) being similar. 
Let $\hat \Delta_V[g,m] \subseteq V$ denote the affine cone of $\Delta_V[g,m]
\subseteq P(V)$. This is the union of all lines in $V$ corresponding to the
points in $\Delta_V[g,m]$. Thus $R_V[g,m]$, the homogeneous coordinate ring
of $\Delta_V[g,m]$, can also be thought of as the coordinate ring of 
$\hat \Delta_V[g,m]$. 

\noindent (A) [The trivial part]: Suppose $V_\lambda(G)$ occurs in
$R_V[g,m]$.  The goal is  to show that $V_\lambda(G)$ contains 
a $G_{\hat g}$-invariant.

 Fix any copy $S$ of $V_\lambda(G)$ in 
$R_V[g,m]$. 

\begin{claim} Not all functions in $S$ can vanish at $\hat g$. 
\end{claim} 

Suppose to the contrary. Then, since $S$ is a $G$-module, 
all functions in $S$ vanish on the orbit $G \hat g \subseteq V$ as well.
By homogeneity of the functions in $S$, then vanish on the 
cone of $G \hat g$ in $V$. But this cone is dense in $\hat \Delta_V[g,m]$,
since $G g$ is dense in $\Delta_V[g,m]$. 
Thus all functions in $S$ vanish on $\hat \Delta_V[g,m]$, and hence, $S$ 
cannot occur in $R_V[g,m]$; a contradiction.  This proves the claim.

Now consider the evaluation map at $\hat g$: 

\[ \psi: S \rightarrow \C,\] 
which maps every function in $S$ to its value at $\hat g$. 
It belongs to $S^*$, the dual of $S$. It is $G_{\hat g}$-invariant
since $\hat g$ is fixed by $G_{\hat g}$. 
Thus $S^*$, and hence $S$,  contains a nonzero $G_{\hat g}$-invariant. 
This proves (A).


\noindent (B) [The nontrivial part]: Suppose $V_\lambda(G)$ contains 
a $G_{\hat g}$-invariant. The goal is to show that it occurs in
$R_V[g,m]$. 

For this we need the notion of stability in geometric invariant theory
\cite{mumford},
which we now recall.

Let $Z$ be a finite dimensional $G$-representation, $G=SL_l(\C)$. 

\begin{defn} \cite{mumford} \label{dstable}
A point $z \in Z$ is called stable with respect to the $G$-action if 
the orbit $G z$ is closed in $Z$ in the complex (equivalently, Zariski) 
topology on $Z$. 
\end{defn}

\noindent Example: Let $Z=M_l(\C)$, the space of $l \times l$ complex
matrices, with the adjoint action of $G$ given by: 

\[ z \rightarrow \sigma z \sigma^{-1},\] 
for any $z \in Z$ and $\sigma \in G$. 
Then it can be shown that $z \in Z$ is stable iff $z$ is diagonalizable. 
For example, under the action of 
\[\sigma = \left[ \begin{array}{ll} t&0 \\ 0 & t^{-1} \end{array} \right], \] 
we have: 

\[ 
z=\left[ \begin{array}{ll} 1& a \\ 0 & 1 \end{array} \right]
\stackrel{\longrightarrow}{\sigma}
\left[ \begin{array}{ll} 1& a t^2  \\ 0 & 1 \end{array} \right] 
\stackrel{\longrightarrow}{t\rightarrow 0}
\left[ \begin{array}{ll} 1& 0  \\ 0 & 1 \end{array} \right].
\] 
Thus the orbit of the nondiagonalizable $z$ contains a  diagonalizable 
limit point,  which cannot be contained in the orbit. Hence  $z$ is
not stable.

Most points in any representation $Z$ of $G$ are stable \cite{mumford}.
The nontrivial
problem is  to show that a specific $z \in Z$ is stable.
For this, there is a very useful Hilbert-Mumford-Kempf criterion of
stability \cite{mumford}, using which can be proved:


\begin{theorem} (GCT1)
The point $\hat g=\det(Y) \in V=\sym^m(Y)$ is stable with respect to
the action of $G=SL(Y)$. That is, the orbit $G {\hat g} \subseteq V$ is
closed in $V$. 
\end{theorem}

Now let us get back to (B). 
Since $\hat g$ is stable, the orbit $G \hat g$ is closed in $V$,
and hence in $\hat \Delta_V[g]=\hat \Delta_V[g,m] \subseteq V$. 
That is, the orbit $G \hat g$  is a closed affine subvariety of 
$\hat \Delta_V[g,m]$. Hence, there is a surjective 
$G$-homomorphism from the coordinate ring $R_V[g,m]$ of $\hat \Delta_V[g,m]$
to the coordinate ring $\C[G \hat g]$ of $G \hat g$. 

It suffices to show that $S=V_\lambda(G)$ occurs in $\C[G \hat g]$. 
Now $G \hat g \cong G/L$, where $L=G_{\hat g}$ is stabilizer of $\hat g$.
By the algebraic form of the Peter-Weyl theorem \cite{fultonrepr}, 
the coordinate ring $\C[G]$ of $G$ (considered as an affine variety) 
decomposes as a $G$-module:
\[ \C[G] \cong \oplus_\alpha V_\alpha(G) \otimes V_\alpha(G)^*.\] 

Now 
\[ \C[G/L] = \C[G]^L,\] 
the ring of $L$-invariants in $\C[G]$. 
Thus, 

\[\C[G \hat g]= 
\C[G/L] = \C[G]^L = \oplus_\alpha V_\alpha(G) \otimes [V_\alpha(G)^*]^L.\]

Therefore $V_\alpha(G)$ occurs in $\C[G \hat g]$ iff 
$V_{\alpha}(G)^*$ contains an $L$-variant. Since $L$ is reductive, this
is so iff $V_{\alpha}(G)$ contains an $L$-invariant. 
Thus $S=V_\lambda(G)$ occurs in $\C[G \hat g]$. 

This implies (B), and proves Theorem~\ref{tgct2first}. 

We now wish to state a similar result 
for the coordinate ring $R_V[f,n,m]$, $f=h^\phi=\perm^\phi$.
For that, we need a few definitions. 
Let $W=\sym^n(X)$ and $V=\sym^m(Y)$ be as above.
Furthermore, let $\bar W=\sym^m(\bar X)$, where $\bar X$ is the 
$(n+1)\times (n+1)$ bottom-right
submatrix of $Y$ containing $X$ and $z$ in Figure~\ref{fig:matrix2}. Let 
$\bar H=SL(\bar X)$.  Thus we have 
\[ H=SL(X) \subseteq \bar H =SL(\bar X) \subseteq G=SL(Y).\] 
Let $h(X)=\perm(X)$,  and $\bar h(\bar X)= z^{m-n} h(X) \in P(\bar W)$. 
Let \[ \Delta_{\bar W}[\bar h]= \Delta_{\bar W}[\bar h,n,m] \subseteq 
P(\bar W)\] 
be the closure of the orbit $\bar H \bar h$.
Let $R_{\bar W}[\bar h]=R_{\bar W}[\bar h,n,m]$ be its homogeneous 
coordinate ring.


\begin{theorem} (GCT2) \label{tgct2second}

\noindent (a) $V_\lambda(G)$ occurs in $R_V[f,n,m]^*$ iff
the length of $\lambda$ is at most $(n+1)^2$ and $V_{\lambda}(\bar H)$ 
occurs in $R_{\bar W}[\bar h,n,m]^*$.


\noindent (b) If $V_\lambda(\bar H)$ occurs in $R_{\bar W}[\bar h,n,m]^*$, 
then it  contains as a subrepresentation
an $H$-module $V_\alpha(H)$ containing an  $H_{\hat h}$-invariant, where
$H_{\hat h} \subseteq H$ is the stabilizer of $\hat h$.

\noindent (c) Conversely, if $V_\alpha(H)$ contains an $H_{\hat h}$-invariant,
there exists a $\lambda$ lying over $\alpha$ such that 
$V_\lambda(\bar H)$ occurs in $R_{\bar W}[\bar h,n,m]^*$, and hence,
$V_\lambda(G)$ occurs in $R_V[f,n,m]^*$. Here lying over means 
(a) the length of $\lambda$ is $\le (n+1)^2$, and (b) 
$V_\alpha(H)$ occurs in $V_\lambda(\bar H)$, considered as an $H$-module
via the natural embedding $H=SL(X)  \subseteq \bar H=SL(\bar X)$. 
\end{theorem} 


\section{A mathematical form of the  $\#P \not = NC$ conjecture} 
 \label{sweak}
We now  apply  GCT to prove 
Theorem~\ref{tmathobs} stated in
the first lecture.
In fact, the same proof technique yields a  more general result.


To state it, we need a few definitions.
Let $H=SL(X)=SL_{n^2}(\C)$ as before, and 
let $\tilde H=SL_n(\C) \times SL_n(\C)$ be embedded naturally in 
$SL(X)=SL(\C^n \otimes \C^n)$ (each $SL_n$ factor acts on the
corresponding $\C^n$). Thus the representation $\sym^n(X)$ for 
$H$ can also be considered to be a representation of $\tilde H$.

Let $\hat t=\trace(X^n) \in \sym^n(X)$ and
$\tilde H_{\hat t} \subseteq \tilde H$ its stabilizer.
It consists of all linear transformations of the form:

\begin{equation}  \label{eqstabtrace}
X \rightarrow A X A^{-1}, 
\end{equation} 
for all $A \in SL_{n}$. Thus $\tilde H_{\hat t} = SL_n$,  embedded 
in $SL_n \times SL_n$ naturally: 
\[ \sigma \rightarrow (\sigma, (\sigma^{-1})^t),\] 
for all $\sigma \in SL_n$. 
Let  $h=\perm \in P(\sym^n(X))$ as before,
$\hat h$  the corresponding point in $\sym^n(X)$, and 
$\tilde H_{\hat h} \subseteq \tilde H$
its stabilizer; it is esentially  the
stabilizer  described in the proof of Proposition~\ref{pchar}.

Let $W$  be any  polynomial 
representation of $\tilde H ^k= \tilde H \times \cdots \times \tilde H $
($k$ copies of $\tilde H$).
Let $w\in P(W)$ be a point, and $\hat w  \in W$ any nonzero point on the line
corresponding to $w$. 
We say that  $w$ is a {\em generalized trace-like} point
if $\hat w$  is an invariant of 
$\tilde H^k_{\hat t} = \tilde H_{\hat t} \times \cdots \times \tilde
 H_{\hat t}$ ($k$ copies of $\tilde H_{\hat t}$); i.e., 
$\tilde H^k_{\hat t} \subseteq \tilde H^k_{\hat w}$. 
We  say it is a 
{\em generalized permanent-like} point  if similarly
$\tilde H^k_{\hat w} \subseteq \tilde H^k_{\hat h}$.
We say that it is a {\em generalized
permanent} if $\tilde H^k_{\hat w} = \tilde H^k_{\hat h}$.


As an example, let $\C[X]$ be the ring  of polynomial functions in
the entries $x_{ij}$ of $X$, with the natural 
action of $\tilde H=SL_n \times SL_n$ (one factor acting on the left
and the other on the right), the case of the 
more general  ring $\C[X_1,\ldots,X_k]$ being similar.
Let $\C[X]^{\tilde H_{\hat t}} \subseteq \C[X]$ be the subring 
of the invariants of $\tilde H_{\hat t}$; i.e., 
the subring of generalized trace-like points in 
$\C[X]$. It 
is generated by $\trace(X^j)$, $j\ge 0$, by (a variant of) the first 
fundamental theorem of invariant theory \cite{fultonrepr}.
A generalized permanent in $\C[X]$ is essentially the 
same as a generalized permanent  in Definition~\ref{dgenperm}
(for $k=1$). There is a slight difference between two definitions. 
In Definition~\ref{dgenperm} we let $U_i$ and $V_i$ be any matrices in
$GL_n(\C)$, whereas here we are taking them to be in $SL_n(\C)$.
Thus as per  the definition in this section $\det(X)$ is a 
generalized permanent-like function, but not a generalized permanent.
Everything  in this section holds for a generalized
permanent in Definition~\ref{dgenperm} as well.
In what follows, we shall assume that a generalized permanent is as 
defined in this section.


Let
$\C[X]^{\tilde H_{\hat h}} \subseteq \C[X]$ be the  subring of 
invariants of $\tilde H_{\hat h}$; i.e., the subring of
generalized permanent-like functions.
By the classical result of Hilbert, it
is finitely generated.
No finite explicit set of generators for this ring is known
(unlike for the ring of generalized-trace like functions). 
But an explicit basis for this ring is known. It is as follows.
To every $n \times n$ magic square $A$ of weight $r$--i.e. 
a matrix of nonnegative
integers whose each row and column sums to $r$--assign a
{\em basic generalized permanent-like function} 
\[ p_A(X)=\sum_{A'} x_{A'},\]
where $A'$ ranges over all matrices obtained by permuting the rows 
and/or columns of $A$, and $x_{A'}=\prod_{i j} x_{ij}^{a'_{ij}}$,
$a'_{ij}$ the entries of $A'$, denotes the monomial associated with
$A'$. This is a $\#P$-computable and $\#P$-complete
function of $A$ and $X$. Furthermore,
the basic generalized permanent-like functions form a basis of 
$\C[X]^{\tilde H_{\hat h}}$.
Not all   generalized permanent-like functions are 
generalized permanents. For example, $p_A(X)$, when
every entry of $A$ is one, is not a generalized permanent, since it has more
symmetries than that of the permanent.
But most generalized permanent-like functions would be generalized 
permanents.


Now let $W$ be any   polynomial representation of $\tilde H^k$,
$\tilde H= SL_n(\C) \times SL_n(\C)$.
Given any $\sigma \in \tilde H^k$
and $w \in P(W)$, 
let $w^\sigma=\rho(\sigma) (w)$,
where $\rho: \tilde H \rightarrow GL(W)$ is the representation
map. Since this map is polynomial, $w^\sigma$ is well defined 
for any $\sigma \in (M_{n}(\C) \times M_n(\C))^k$.
Let $\tilde \Delta_W[w] \subseteq P(W)$
denote the orbit closure of $w$ with  respect
to the $\tilde H^k$ action; i.e., the closure of the orbit $\tilde H^k w$.


\begin{theorem}  \label{tweak}
Let $w$ be any generalized trace-like point in $W$, and 
and $h$ any generalized permanent in $W$. 
Then, for any $\sigma \in (M_{n}(\C) \times M_{n}(\C))^k$, $w^\sigma \not = h$.
More generally,  $\tilde \Delta_W[w]$ does not contain $h$.
\end{theorem} 

This reduces to Theorem~\ref{tgenweaklec1}  when $W=\C[X_1,\ldots,X_k]$.
The proof in \cite{GCT2appnedix} based on basic geoemtric invariant
theory also works in this case. But we are more interested 
here in testing the general proof strategy of GCT based on obstructions 
in this nontrivial special case. 





\ignore{We do not have  any elementary proof for this result like the
one for Proposition~\ref{pweaklec1}. 
The main difficulty is the following.
Let $W^{\tilde H^k_{\hat h}} \subseteq W$
be the subspace of $\tilde H^k_{\hat h}$-invariants 
(i.e. generalized  permanent-like elements) in $W$. 
When $W=\sym^n(X)$, $W^{\tilde H_{\hat h}}$ 
consists of just constant  multiples of 
the usual permanent, and hence, its dimension is one.
But  when $W$ is a general  irreducible representation of $\tilde H^k$, 
finding a positive formula for $\dim(W^{\tilde H^k_{\hat h}})$ is 
is a nontrivial special case of the fundamental
plethysm problem of representation theory
(cf. Section~\ref{splethysm}).
Thus even finding the dimension of the space of 
permanent-like elements is very hard, let alone having any understanding
of its structure.  Though Theorem~\ref{tgenweaklec1} looks 
elementary at the surface,
it has similar difficulties hidden underneath \cite{GCT6}.



We shall sketch the proof of 
Theorem~\ref{tweak} only for $W=\C[X]$. The details for 
the general case can be found in GCT6.
For $W=\C[X]$, Theorem~\ref{tweak}  follows from:

\begin{theorem} 
There exists a family $\{O_n\}$ of obstructions in this case.
\end{theorem}

\proof 
Let  $h\in \C[X]$ be any generalized permanent,
and $w \in \C[X]$ any generalized trace-like point.
The class varieties $\tilde \Delta_W[w], \tilde \Delta_W[h] \subseteq
P(W)$ are now defined with respect to the $\tilde H$-action
and the obstructions are $\tilde H$-Weyl-modules defined similarly.
Let $\tilde R_W[h]$ and $\tilde R_W[w]$ be the homogeneous coordinate 
rings of $\tilde \Delta_W[w]$ and $\tilde \Delta_W[h]$.

It can be using shown using  Kempf's criterion of stability \cite{mumford}
that $\hat h$ is stable with respect to the $\tilde H$ action--the proof
of this fact is  similar to the stability related proofs in GCT1. 
Specifically, in this setting Kempf's criterion in a concrete form says
that $\hat h$ is stable if the standard irreducible 
representation $\C^n \otimes \C^n$
of $\tilde H=SL_n(\C) \times SL_m(\c)$ is also an irreducible representation of
its subgroup $\tilde H_{\hat h}$, which is easy to check.
The crucial point here is that this proof needs to know only about 
the stabilizer of $\hat h$ and nothing else.
Using stability of $\hat h$  it then follows from the general 
results in GCT2  that the analogue of
Theorem~\ref{tgct2first}  (2) holds for this $h$.

The stabilizer $\tilde H_{\hat w}$ contains 
the stabilizer $\tilde H_{\hat t} \subseteq \tilde 
H$ of $\hat t=\trace(X^n) \in \sym^n(X)$ as described in (\ref{eqstabtrace}). 

We need the following two facts.

\noindent (a) Any
irreducible $\tilde H$-module is  of the form 
$V_\alpha(SL_n) \otimes V_\beta(SL_n)$. 
By the classical Schur's lemma it contains a 
$\tilde H_{\hat t}$-invariant iff $\alpha=\beta$;.
Hence, it does not contain a $\tilde H_{\hat w}$-invariant if 
$\alpha \not = \beta$.

\noindent (b) (Cf. \cite{ariki})
An irreducible representation of $\tilde H$
of the form $1 \otimes V_{\gamma}(SL_n)$,
where $1$ stands for the trivial representation of $SL_n$ 
and $|\gamma|=2n$, contains a $\tilde H_{\hat h}$-invariant
iff $\gamma$ is even--if 
$\gamma =(\gamma_1, \gamma_2, \cdots)$, 
this means every $\gamma_i$ is divisible by $2$.
Here $|\gamma|=\sum_i \gamma_i$
denotes the size of $\gamma$. 



Let $\gamma$ be any even partition with $|\gamma|=2n$.
By (b) and Theorem~\ref{tgct2first} (2)
(or rather its analogue in this case mentioned above), 
$1 \otimes V_\gamma(SL_n)$ occurs in $\tilde R_W[h]^*$.
By (a), it 
does not contain a $\tilde H_{\hat w}$-invariant.
By Theorem~\ref{tgct2first} (2) again (or rather its analogue in this case),
it cannot occur in $\tilde R_W[w]^*$. 
Therefore, $1 \otimes V_\gamma(SL_n)$ is an obstruction. \qed

The proof above shows that 
any $1 \otimes V_\gamma(SL_n)$, $|\gamma| >0$, 
which contains an $\tilde H_{\hat h}$-invariant 
is an obstruction. One can  show nonconstructively, i.e., without
using \cite{ariki}, that there is such $\gamma$ for every $n$.
This then yields a nonconstructive proof of this result (whose 
major part is the same as in the explicit proof). 





\section{From the mathematical towards the  general complexity theoretic
form} \label{sweaktogeneral}
We now discuss what is needed to lift the proof of the mathematical
form of the $\#P \not = NC$ conjecture
to the general complexity theoretic form.
There are two issues.

(1) There is a serious leak in Theorem~\ref{tgct2second},
because there can be
several $\lambda$ lying over $\alpha$, and that result does not tell us
exactly which one of them would occur in $R_{\bar W}[\bar h,n,m]$ or 
$R_V[f,n,m]^*$, nor does it
tell us which $V_\lambda(G)$'s occur in $R_{\bar W}[\bar h,n,m]_d$
or $R_V[f,n,m]^*_d$, for a fixed
$d$. Such refined information can be obtained from 
a general positivity hypothesis 
(PH: Hypothesis~\ref{hph}) for $R_V[f,n,m]$ 
(which was  denoted  by $R_{\#P}(n,m)$ in Lecture 1).
We will discuss this  issue  in Section~\ref{sposgeneral}.

(2) To use Theorem~\ref{tgct2first} and Theorem~\ref{tgct2second}
we need an effective criteria for: 

\begin{problem} \label{pinvariant}

\noindent (a) Does $V_\lambda(G)$ contain a $G_{\hat g}$-invariant? 

\noindent (b) Does $V_\pi(H)$ contain an $H_{\hat h}$-invariant? 

\end{problem} 

These are special cases of the general subgroup restriction problem 
which we discuss next in the following section. 

\section{The subgroup restriction problem} 


Let $H$ be a reductive subgroup of $G=GL(V)$, where $V$ is an explicitly
given finite dimensional representation of $H$. Symbolically:

\begin{equation}  H \stackrel{\rho} \hookrightarrow G=GL(V), 
\end{equation} 

where $\rho$ denotes the representation map. 
For example, we can have $H=GL_n(\C)$, and $V=V_\mu(H)$, 
the Weyl module of $H$. Then $\mu$ specifies the representation
map $\rho$ completely, and hence, we shall also use $\mu$ in place of 
$\rho$ in this case--called the {\em plethysm} case. Symbolically: 

\begin{equation}  \label{eqplethysm}
H \stackrel{\mu} \hookrightarrow G=GL(V), \quad V=V_\mu(H).
\end{equation} 


Given any partition $\lambda$, the Weyl module $V_\lambda(G)$ of 
of $G$ can be considered an $H$-module via 
the representation map $\rho$.
 Since $H$ is reductive, 
it is completely reducible as an $H$-module:

\begin{equation} 
V_\lambda(G)= \bigoplus_\pi a^\lambda_{\pi,\rho} V_\pi(H),
\end{equation}

where $a^\lambda_{\pi,\rho}$ denotes the multiplicity of $V_\pi(H)$
in $V_\lambda(G)$. In the plethysm case, we also denote $a^\lambda_{\pi,\rho}$ 
by $a^\lambda_{\pi,\mu}$, and call it the {\em plethysm constant}. 


\begin{problem} [Subgroup restriction  problem]

\noindent (1) Given partitions $\lambda,\pi$ and $\rho$,
does $V_\pi(H)$ occur as a subrepresentation of $V_\lambda(G)$? That is,
is $a^\lambda_{\pi,\rho}$  positive? 

\noindent (2) Find a good positive  formula for 
$a^\lambda_{\pi,\rho}$ akin to the usual positive formula for the permanent 
which does not have any alternating signs. What 
good and positive means would be elaborated later
(cf. Hypothesis~\ref{hphple}).
\end{problem} 

\begin{problem}[Plethysm problem]  \label{pplethysm}
The special case of the subgroup restriction problem for the
representation map (\ref{eqplethysm}), obtained by replacing $\rho$ by $\mu$.
\end{problem}

The two special cases that arise in the context of Problem~\ref{pinvariant}
are: 

\noindent (1) Let $\hat g= \det(Y) \in \sym^m(Y)$,
$G=GL(Y)=GL_{m^2}(\C)$, and $H=G_{\hat g} \subseteq G$,
the stabilizer of $\hat g$; cf. the proof of Proposition~\ref{pchar} for
its description. 
If we ignore the discrete (and torus) part of the stabilizer, then 
the subgroup restriction problem here is for the embedding:

\[ GL_m\times GL_m \hookrightarrow GL(\C^m \otimes \C^m).\] 

\noindent (2) Let $\hat h =\perm(X) \in \sym^n(X)$, and $H=GL(X)$, and
$H_{\hat h}$ the stabilizer of $\hat h$; cf. the proof of 
Proposition~\ref{pchar} for its description.
If we ignore the continuous part of the stabilizer, then 
the subgroup restriction problem here is for the embedding:

\[ S_n \times S_n \hookrightarrow GL(\C^n \otimes \C^n), \]

where $S_n$ is the symmetric group on $n$ letters.

It is a classical result of representation theory that (1) can
be reduced to the plethysm problem. 
By \cite{ariki}, (2) can also be reduced to the plethysm problem. So
the plethysm problem is the fundamental special case of the 
subgroup restriction problem that we will be interested in
(though the following results also hold for the general subgroup 
restriction problem).

\section{Littlewood-Richardson problem} 

One completely understood special case of the subgroup restriction problem
is  the Littlewood-Richardson (LR) problem. This arises when 
 $H=GL_n(\C)$ embedded  in $G=H \times H$ diagonally:

\begin{equation} \label{eqdiagonallr}
\begin{array}{lcl}
H &\rightarrow & G= H \times H \\
\sigma &\rightarrow&  (\sigma,\sigma).
\end{array}
\end{equation}

Then every irreducible representation of $G$ is of the form
$V_\alpha(H) \otimes V_\beta(H)$. Considered as an $H$-module via the 
above diagonal embedding, it
decomposes:

\[ V_\alpha(H) \otimes V_\beta(H) = \oplus_\lambda c_{\alpha,\beta}^\lambda
V_\lambda(H).\] 
The multiplicities $c_{\alpha,\beta}^\lambda$ are called 
Littlewood-Richardson coefficients. Let $\tilde c_{\alpha,\beta}^\lambda(k)
= c_{k \alpha, k \beta}^{k \lambda}$ be the associated stretching functions.

\begin{theorem}  \label{tlr}

\  

\begin{enumerate} 
\item {\bf [LR PH1]} 
There exists a polytope of $P_{\alpha,\beta}^\lambda$ with description of
$\poly(\bitlength{\alpha},\bitlength{\beta},\bitlength{\lambda})$ bitlength
such that:
\[ c_{\alpha,\beta}^\lambda= \#(P^\lambda_{\alpha,\beta}),\]  the
number of integer points in $P^\lambda_{\alpha,\beta}$, and 
\[ \tilde c_{\alpha,\beta}^\lambda (k) = c_{k \alpha,k \beta}^{k \lambda}
= \# (k P^\lambda_{\alpha,\beta}) = f_{P^\lambda_{\alpha,\beta}}(k),\] 
the Ehrhart quasipolynomial of $P^\lambda_{\alpha,\beta}$. 
This provides a good positive formula for the Littlewood-Richardson 
coefficients. 

\item {\bf [Saturation Theorem]} \cite{knutson}: 
$c_{\alpha,\beta}^\lambda \not = 0$ iff $P_{\alpha,\beta}^\lambda \not 
= \emptyset$. 

\item (GCT3,\cite{knutson}) 
Given $\alpha,\beta,\lambda$, whether $c_{\alpha,\beta}^\lambda$ is nonzero
(i.e. positive) can be decided in 
$\poly(\bitlength{\alpha},\bitlength{\beta},\bitlength{\lambda})$ time.
\end{enumerate} 
\end{theorem}

Here the third statement follows from the first two by 
a polynomial time algorithm for linear programming \cite{lovasz}. 

\section{Plethysm problem}  \label{splethysm}
Let us now focus on the plethysm problem (Problem~\ref{pplethysm}). 
Let $\tilde a_{\pi,\mu}^\lambda(k) = a_{k \pi,\mu}^{k \lambda}$ be
the stretching function associated with the plethysm constant 
$a_{\pi,\mu}^{\lambda}$.  Let 
\[ A^\lambda_{\pi,\mu}(t) = \sum_{k \ge 0} \tilde a^\lambda_{\pi,\mu}(k)\]
be the associated generating function. 
It was asked in \cite{kirillov} if it is a rational function. 
The following result shows something stronger:

\begin{theorem}  \label{tplethysmqausi} (GCT6)
The stretching function $\tilde a_{\pi,\mu}^\lambda(k)$ is 
a quasi-polynomial. 
\end{theorem}
This implies, in particular, that $A^\lambda_{\pi,\mu}$ is rational
by a standard  result of enumerative combinatorics \cite{stanleyenu}. 

The proof below is motivated by Brion's proof \cite{dehy} of quasipolynomiality
of the stretching functions associated with the Littlewood-Richardson
coefficients (of arbitrary type). 

\proof 

Let $H=GL_n(\C)$, and $V=V_\pi(H)$. Let $U \subseteq H$ be 
the subgroup of  lower triangular matrices with $1$'s on the diagonal.
Then it is known (cf.
 Appendix) that there is a unique (up to constant multiple) 
nonzero point 
$\hat v = \hat v_\pi \in V$ that is stabilized by $U$; i.e., such that
$u \hat v= \hat v$ for all $u \in U$. The point $\hat v$ is called 
the highest weight vector of $V_\pi(H)$. Let $v=v_\pi$ be the corresponding
point in $P(V)=P(V_\pi(H))$. 
Then it is known that the orbit $H v \subseteq P(V)$ is already closed.
That is, the orbit closure $\Delta_V[v]$ (with respect to the $H$ action)
is just the orbit $H v$ itself. Furthermore, by Borel-Weil \cite{fultonrepr}, 
the homogeneous coordinate ring $R_V[v]$ of $\Delta_V[v]= H v$ has the
following decomposition as an $H$-module: 

\begin{equation} \label{eqrvv}
R_V[v]=\oplus_k V_{k \pi}(H)^*,
\end{equation}

where the superscript $*$ denotes the dual. 
We can also think of $R_V[v]$ as the coordinate ring of 
$\hat \Delta_V[v]$, the affine cone of $\Delta_V[v]$. 
It is known that 
the  singularities of $\hat \Delta_V[v]$ are rational 
and normal; e.g., see \cite{smith}. 

\noindent {\em Remark:} 
By normal, we mean that for each $x \in X= \hat \Delta_V[v]$, 
there exists a  (classical)
neighbourhood  $U \subseteq X$ of $x$, such that
$U \setminus (U \cap \mbox{sing}(X))$
is connected; where $\mbox{sing}(X)$ is the subvariety of $X$ consisting
of all its singular points. Rational is much more difficult to define. 
Roughly it means the following. By Hironaka \cite{hironaka}, 
all singularities of $X$ can be resolved (untangled)--cf. 
Figure~\ref{fig:resolution}.
With each singularity of $X$, one can associate a cohomological object 
that measures the difficulty of this resolution. A singularity is called
rational if this cohomological object vanishes. This means the
singularity is sufficiently nice. 

By abuse of terminology, we say that the ring $R_V[v]$ in (\ref{eqrvv})
is normal and rational. Similarly, 
it can be shown that the ring

\begin{equation} \label{eqS}
S=\oplus_\pi V_{k \pi}(H)^* \otimes V_{k \lambda} (G)
\end{equation}

is normal and rational. (Formally, this means the singularities
of the variety, or rather the
scheme, which  can be associated with this ring, are rational
and normal.)

Let $S^H$ denote the ring of $H$-invariants in $S$: 

\[ S^H= \{ s \in S \ | \ h s = s, \quad \forall h \in H \}. \] 

By (\ref{eqS}), 

\begin{equation} 
S^H= \oplus_k [ V_{k \pi}(H)^* \otimes V_{k \lambda}(G)]^H,
\end{equation}

where the superscript $H$ on the right hand side again denotes the operation
of taking $H$-invariants. 

By a classical result of Hilbert \cite{popov},
$S^H$  is  a finitely generated ring (since $S$ is finitely generated). 
Furthermore, since $S$ is normal and rational, it follows by 
Boutot \cite{boutot} that $S^H$ is normal and rational (this is the crux 
of the argument). 

Let $h_{S^H}(k)=\dim(S^H_k)$ denote the Hilbert function of $S^H$,
where $S^H_k$ denotes the degree-$k$ component of $S^H$. 

By Schur's lemma \cite{fultonrepr}, 

\[ 
\dim ([V_{k \pi}(H)^* \otimes V_{k \lambda}(G)]^H) = a_{k \pi, \mu}^{k \lambda}
=\tilde a^\lambda_{\pi,\mu}(k),
\] 
the multiplicity of $V_{k \pi}(H)$ in $V_{k \lambda}(G)$. 
Hence, 
\[ h_{S^H}(k)= \tilde a_{\pi,\mu}^\lambda(k). \] 

By  Flenner \cite{flenner}, $h_{S^H}(k)$ 
 is a quasi-polynomial, since $S^H$ is rational and
normal. 
Thus it follows that $\tilde a_{\pi,\mu}^\lambda(k)$ is also a 
quasi-polynomial. \qed


\begin{hypo} [Plethysm PH] \label{hphple} (GCT6)

There exists a polytope of $P=P^\lambda_{\pi,\mu}$ with description of 
$\poly(\bitlength{\lambda},\bitlength{\pi},\bitlength{\mu})$ bitlength
such that 

\begin{equation} 
\tilde a_{\pi,\mu}^\lambda(k) = f_P(k),
\end{equation}
the Ehrhart quasi-polynomial of $P$. In particular,

\begin{equation} 
a_{\pi,\mu}^\lambda(k) = \#(P),
\end{equation}
the number of integer points in $P$. 

This would provide the sought good positive formula for the plethysm 
constant $a_{\pi,\mu}^\lambda$ (cf. Problem~\ref{pplethysm})
\end{hypo}

Here it is assumed that the polytope is presented by a separation 
oracle as in \cite{lovasz},
and the bitlength $\bitlength{P}$ of the description
of $P$ is defined to be $l+s$, where $l$ is the dimension of the ambient 
space in which  $P$ is defined by linear constraints,
and $s$ the maximum bitlength of any defining constraint. 
Notice that the polytope $P$ here 
depends only on $\lambda,\pi$ and $\mu$ but not on 
$H$, just like the  plethysm constant $a^\lambda_{\pi,\mu}$ itself.



\begin{theorem} \label{tlinear} (GCT6)
Assuming Plethysm PH, whether $a_{k \pi,\mu}^{k \lambda} > 0$ for some
$k \ge 1$ can be decided in $\poly(\bitlength{\lambda}, \bitlength{\pi},
\bitlength{\mu})$ time. If so, one such $k$ can also be found in
polynomial time.
\end{theorem}

\proof By linear programming \cite{lovasz}. One has to just decide if
$P^\lambda_{\pi,\mu}$ is nonempty, and if so, find a vertex $v$ of $P$ and
choose  $k$ such that $k v$ has integral coordinates. 
\qed 

\section{Positivity and the existence of obstructions in  the general case} 
\label{sposgeneral}
Now we describe how positivity can help in proving the existence of
obstructions in the general case of the $\#P$ vs. $NC$ problem.


Towards that end, first we introduce a stronger notion of obstructions.
We follow the same notation as in Section~\ref{sgmodule}. Thus 
$G=SL(Y)=SL_{m^2}(\C)$ as there. 

\begin{defn} (GCT2)
A Weyl module $V_\lambda(G)$ is called a {\em strong obstruction} 
for the pair $(f,g)$, if $V_\lambda(G)$ occurs in $R_V[f,n,m]^*$,
i.e. in $R_V[f,n,m]_d^*$ for some $d$,  but does not contain a nonzero
$G_{\hat g}$-invariant.
\end{defn} 


It follows from Theorem~\ref{tgct2first} (1) that a strong obstruction is also
an obstruction as per Definition~\ref{dobstru}. 
Furthermore, by Theorem~\ref{tgct2second}, we have:


\begin{prop} \label{pgct2uni}
A Weyl module $V_\lambda(G)$ is a {\em strong obstruction} 
for the pair $(f,g)$, iff 
\begin{enumerate} 
\item The length of $\lambda$ is at most 
$(n+1)^2$,
\item  $V_\lambda(\bar H)$ occurs in $R_{\bar W}[\bar h,n,m]^*$,
i.e., in $R_{\bar W}[\bar h,n,m]_d^*$ for some $d$ 
(which has to be $|\lambda|/m$). 
\item  $V_\lambda(G)$  does not contain a nonzero
$G_{\hat g}$-invariant.
\end{enumerate}
\end{prop}

Now let $G_\lambda(k)= 
 G_{\lambda,m}(k)$ 
denote the multiplicity of the trivial representation of $G_{\hat g}$  in
$V_{k \lambda}(G)$. 

\begin{theorem} \label{tplethysm2} (GCT6)
The stretching function $G_{\lambda,m}(k)$ is a quasi-polynomial.
\end{theorem}

This is proved like Theorem~\ref{tplethysmqausi};
in fact, this is essentially its special case. 

The following is a 
precise form  Hypothesis~\ref{hph} (b).
It is essentially a special case of Plethysm PH: 


\begin{hypo} [PH] \label{hphvariant} (GCT6)

There exists a polytope of $Q_{\lambda}$ 
such that 

\begin{equation} 
 G_{\lambda,m}(k) = f_{ Q_{\lambda}}(k),
\end{equation}
for every $m$.
\end{hypo}

Here  the polytope $ Q_\lambda$ does not depend on $G$ or its 
dimension $m=\dim(G)$, 
for the same reasons that  the polytope $P$ in the Plethysm PH 
does  not depend on $H$ there; cf. the remark after the  Plethysm PH.
Furthermore, if $ Q_\lambda$ exists, its dimension is guaranteed 
to be polynomial in the length of $\lambda$ by the proof of
Theorem~\ref{tplethysm2}. 


The following  is a precise form of 
Hypothesis~\ref{hph1} (b).




\begin{hypo} {\bf (PH1)} \label{hph1tilde} (GCT6)

There exists an
explicit polytope $ Q_{\lambda}$ satisfying  PH 
in Hypothesis~\ref{hphvariant}. 
Here explicit means:

\begin{enumerate}
\item  The polytope is specified by an explicit system of linear constraints,
each constraint of bitlength $\poly(\bitlength{\lambda})$
(note no dependence on $m$).

\item  The membership problem for the polytope
$ Q_{\lambda}$  also 
belongs to the complexity class $P$.
That is,  given a point $x$, whether it belongs to $ Q_{\lambda}$ 
can also be decided in $\poly(\bitlength{x},\bitlength{\lambda})$  time.
Furthermore, we assume that if $x$ does not belong to the polytope,
then the membership algorithm also gives a hyperplane separating 
$x$ from the polytope in the spirit of \cite{lovasz}. 
\end{enumerate} 
\end{hypo}

The following  addresses a relaxed form of Problem~\ref{pinvariant},
which is enough for our purposes: 

\begin{theorem} \label{tverify1}

\noindent (1)  Assuming PH1 above (Hypothesis~\ref{hph1tilde}),
 whether $V_{k \lambda}(G)$ contains a $G_{\hat g}$-invariant,
for some $k \ge 1$,
can be decided in $\poly(\bitlength{\lambda})$ time.
By Theorem~\ref{tgct2first}, this is equivalent to deciding 
whether $V_{k \lambda}(G)$ occurs in $R_V[g,m]^*$ for some $k \ge 1$. 

\noindent (2) Assuming an analogous PH1 for the subgroup 
restriction problem for $H_{\hat h} \subseteq H$,
whether $V_{k \pi}(H)$ contains an $H_{\hat h}$-invariant, for some
$k \ge 1$, can also be decided in $\poly(\bitlength{\pi},n)$ time.
By Theorem~\ref{tgct2first}, this is equivalent to deciding 
whether $V_{k \pi}(H)$ occurs in $R_W[h,n]^*$ for some $k \ge 1$. 

\end{theorem} 

\proof Similar to that of  Theorem~\ref{tlinear}. \qed 

A similar result for $R_V[f,n,m]$ or $R_{\bar W}[\bar h,n,m]$ 
would not follow from the Plethysm PH 
(or more generally, the subgroup restriction PH) 
because of the serious 
leak in Theorem\ref{tgct2second} that we discussed in 
Section~\ref{sweaktogeneral}. 
One needs a more general PH for this.
We turn to this issue next.


For any $\lambda$ of length $\le (n+1)^2$, 
let $F_{\lambda,n,m}(k)$ be the multiplicity of 
$V_{k \lambda}(\bar H)$ in $R_{\bar W}[\bar h,n,m]^*$, which 
by Theorem~\ref{tgct2second},
coincides with the multiplicity of $V_{k \lambda}(G)$
in $R_V[f,n,m]^*$. Thus $F_{\lambda,n,m}(k)$ is the same as the function 
with the same notation in Theorem~\ref{tquasi} (b). The following 
is  its restatement.

\begin{theorem} \label{tquasiaymptotic}
The function $F_{\lambda,n,m}(k)$ is an asymptotic quasi-polynomial.
\end{theorem}


The singularities of the class variety $\Delta_{\bar W}[\bar h,n,m]$ 
here are not 
normal \cite{shrawan} when $m>n$. But 
in view of the exceptional nature of the class variety
and Theorems~\ref{tplethysmqausi} and \ref{tplethysm2}, 
it may be conjectured that the deviation from
rationality and normality is small; cf. the remarks after 
Hypothesis~\ref{hph1restatement} 
below.

The following is a restatement  of Hypothesis~\ref{hph} (a).

\begin{hypo} {\bf (PH) [Positivity Hypothesis]} \label{hph2}
For every $\lambda,n,m\ge n$, 
there exists a parametrized (cf. (\ref{eqpara}))  polytope 
$P=P_{\lambda,n,m}=P_{\lambda,n,m}(k)$ 
such that 
\begin{equation} 
F_{\lambda,n,m}(k)=f_P(k)
\end{equation} 
It is also assumed that $P_{\lambda,n,m}$ has a specification as in
Hypothesis~\ref{hph} (a). 
\end{hypo} 




If such $P$ exists, its  dimension is  guaranteed to be
polynomial in $n$
(by the proof of Theorem~\ref{tquasiaymptotic}) 
essentially because the dimension
of $\bar H$ is  $O(n^2)$ and does not depend on
$m$. 

The following is a restatement of Hypothesis~\ref{hph1} (a). 

\begin{hypo} {\bf (PH1)}  \label{hph1restatement}

There exists an {\em explicit} 
parametrized polytope $P_{\lambda,n,m}=P_{\lambda,n,m}(k)$ 
as in Hypothesis~\ref{hph2}.
\end{hypo} 

The meaning of explicit  here is as 
in Hypothesis~\ref{hph1}. In particular, the  polynomial bounds are
meant to be polynomial in $\bitlength{\lambda},n$ and $\bitlength{m}$,
instead of $m$. Because
$F_{\lambda,n,m}(k)$ is the multiplicity of 
$V_{k \lambda}(\bar H)$ in $R_{\bar W}[\bar h,n,m]^*$, 
$\dim(\bar H)=(n+1)^2$, which does not depend on $m$,  and $m$ occurs
only in the definition of $\bar h(\bar X)=z^{m-n} h(X)$ as a numeric parameter 
akin to the numeric parameters $\lambda_i$'s. 

Furthermore, PH1 above
implies that the deviation from quasipolynomiality of 
$F_{\lambda,n,m}(k)$ is small, specifically, 
$O(2^{O(\poly(\bitlength{\lambda},n,\bitlength{m}))})$, so that the bitlength
of the deviation is polynomial. This would mean that the deviation from
rationality and normality of the singularities of the class variety 
$\Delta_{\bar W}[\bar h,n,m]$ is also small; 
 cf.  Theorem~\ref{tquasiaymptotic} and the remarks after it.




\begin{theorem} \label{tverify2}
Assuming general  PH1  (Hypothesis~\ref{hph1restatement}), 
whether $V_{k \lambda}(G)$ occurs in $R_V[f,n,m]^*$--or
equivalently, whether $V_{k \lambda}(\bar H)$ 
occurs in  $R_{\bar W}[\bar h,n,m]^*$--for some
$k \ge 1$, can be 
decided in $\poly(\bitlength{\lambda},n,\bitlength{m})$ time.
\end{theorem} 




The following is a  refined version of Theorem~\ref{tgct6}: 

\begin{theorem} (GCT6) \label{tgct6refined}
There exists a family $\{O_n=V_{\lambda_n}(G)\}$ of strong obstructions 
for the general $\#P$ vs. $NC$ problem in characteristic zero, 
for $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$, 
assuming, 

\begin{enumerate} 
\item PH above (Hypotheses~\ref{hphvariant} and \ref{hph2}) , and
\item OH (Obstruction Hypothesis): 

For all $n\rightarrow \infty$,  there exists $\lambda$ such that 
$P_{\lambda,n,m}(k) \not = \emptyset$ for all sufficiently large $k$ and 
$Q_{\lambda}=\emptyset$.
\end{enumerate}


For an analogous result  for the $P$ vs. $NP$ problem, see GCT6.
\end{theorem}


We define $\lambda$ to be a polyhedral  obstruction (label) if it satisfies OH
here. 
In this case it is easy to see that $k \lambda$, for some $k \ge 1$,
is a strong  obstruction. 


\section{Positivity and the $P$-barrier} 

Theorem~\ref{tverify1}   and \ref{tverify2} imply: 

\begin{theorem} 
Given $\lambda,n,m$, whether $\lambda$ is a polyhedral obstruction (label) 
can be decided in $\poly(\bitlength{\lambda},n,\bitlength{m})$ time
assuming PH1 (Hypotheses~\ref{hph1tilde}
 and \ref{hph1restatement}). In other words, 
the $P$-barrier for verification of obstructions
(Section~\ref{spbarrier}) can be crossed assuming
PH1. 
\end{theorem}

In conjunction with Theorem~\ref{tgct6refined}, this implies 
its stronger form:

\begin{theorem} (GCT6)
There exists an explicit (cf. Section~\ref{sflip}) 
family $\{\lambda_n\}$ of polyhedral obstructions,
for the general $\#P$ vs. $NC$ problem in characteristic zero, 
for $m=2^{\log^a n}$, $a>1$ fixed, $n\rightarrow \infty$, 
assuming PH1 and OH above. 

Analogous result holds for the $P$ vs. $NP$ problem in characteristic zero.
\end{theorem}

The strategy now is to prove PH, or rather PH1, first, and then 
prove OH using the explicit forms of the polytopes in PH1. 
GCT2,6,7,8 together give an evidence for why PH/PH1 and OH should hold. 
As far as proving OH is concerned, there is nothing that we can say at this
point since it depends on the explicit forms of the polytopes 
in PH/PH1. The remaining  question is the following.

\section{How to prove  PH1 and why should it hold?}
We now briefly describe the plan in GCT6 
to prove PH1 by generalizing the proof of LR PH1
(Theorem~\ref{tlr}) based on  the theory of standard quantum groups
 \cite{drinfeld,kashiwara,lusztig}. 

For that we need a definition.

\begin{defn} 
Let $H$ be a connected reductive subgroup of a connected reductive $G$. 
A basis $B$ of a representation $V$ of $G$ 
is called {\em positive} with respect to the $H$-action if: 

\begin{enumerate}  
\item If it $H$-compatible. This means there exists a filtration of $B$:
\[ B=B_0 \supset B_1 \supset \cdots \] 
such that $\langle B_i \rangle / \langle B_{i+1} \rangle$, where 
$\langle B_i \rangle$ denote the linear span of $B_i$, is 
isomorphic to an irreducible $H$-module. In other words, this filtration
gives a Jordan-Holder series of $V$.

\item For each standard generator $h$ of (the Lie algebra of) $H$ and
each $b \in B$, 
\[ h b = \sum_{b' \in B} c^h_{b,b'} b, \] 
where each $c^h_{b,b'}$ is a nonnegative rational. 
\end{enumerate} 
\end{defn} 

LR PH1 is  a 
consequence of the proof of a much deeper positivity result:

\begin{theorem} [LR PH0] \cite{lusztig,beilinson}
Let $H=GL_n(\C)$ embedded in $G=H\times H$ diagonally as in 
(\ref{eqdiagonallr}).
Then each irreducible 
representation of $G$ has a positive basis with respect to the $H$ action.
\end{theorem}

The proof of this result goes via the theory of the standard quantum group.
Specifically, the diagonal embedding (\ref{eqdiagonallr}) is first 
quantized \cite{drinfeld} in the form
\begin{equation}  \label{eqqdi}
H_q \rightarrow H_q \times H_q,
\end{equation}
where $H_q$ is the standard quantum group, a quantization of $H$ that
plays the same role
in quantum mechanics that the standard group $H$ plays in classical 
mechanics. (Well, (\ref{eqqdi}) is not really accurate, because what is 
quantized in \cite{drinfeld} is not $H$ but rather its universal 
enveloping algebra. We shall ignore this technicality here.) 
It is then shown that the irreducible representations of $H_q$ and 
$H_q \times H_q$ have extremely rigid {\em canonical} bases 
\cite{kashiwara,lusztig},
which are positive \cite{lusztig},
and have many other remarkable properties.
The only known proof of this
positivity 
\cite{lusztig} is based on the Riemann hypothesis over finite fields 
and the related works 
\cite{weil2,beilinson}

\begin{goal} 
Lift this LR story to the  plethysm problem (and the more general
subgroup restriction problem).
\end{goal}

In this context:

\begin{hypo} [Plethysm PH0] \label{hplph0}
Let 
\begin{equation} \label{eqpl2}
H=GL_n(\C) \rightarrow GL(V), V=V_\mu(H),
\end{equation}
be the plethysm homomorphism (\ref{eqplethysm}).
The each Weyl module $V_\lambda(G)$ has a positive basis with respect
to the $H$-action.
\end{hypo}

\begin{theorem} (GCT7)
The plethysm map (\ref{eqpl2}) can be quantized in the form 
\begin{equation} 
H_q \rightarrow G^H_q,
\end{equation}
where $H_q$ is the standard quantum group associated with 
$H$ and $G^H_q$ is a new nonstandard quantization of $G$.

A similar result holds for general connected reductive $H$ as well.
\end{theorem}

Furthermore, GCT8 gives a conjecturally correct algorithm to construct 
canonical bases of 
irreducible representations $G^H_q$ with  conjectural positivity
and other properties from which Plethysm PH0 would follow. 
Experimental evidence for 
positivity of the conjectural canonical bases in GCT8 constitutes 
the main evidence  for Plethysm PH0, and hence Plethysm PH1/PH.



The general PH1 (Hypothesis~\ref{hph1restatement})  can be regarded as a
generalization  of the Plethysm PH1 for    the triple
(cf. Observation~\ref{obstriple})
\begin{equation} \label{eqtri}
\bar H_{\hat h} \rightarrow \bar H=SL(\bar X) \rightarrow L=GL(\bar W)
\end{equation}
associated 
with the class variety $\Delta_{\bar W}[\bar h]$,
rather than the plethysm couple (\ref{eqpl2}).
To go from the Plethysm PH1 to the general PH1, one has to similarly
quantize the triple (\ref{eqtri}) and develop an analogous theory of 
canonical bases for this quantized triple. 
But first, we have to understand the couples. Hence the Plethysm PH0/PH1
can be regarded as the heart of GCT. 
To prove the nonstandard quantum group  conjectures in GCT7,8 that arise
in this context, 
a substantial nonstandard  extension of the work 
\cite{weil2,beilinson,kazhdan,lusztig} surrounding 
the standard Riemann hypothesis over finite fields may 
be necessary; cf. Figure~\ref{fig:lift}. 
Thus the ultimate goal of GCT would be  to deduce the ultimate 
negative hypothesis of mathematics, $P \not = NP$ conjecture (in characteristic
 zero), 
from the ultimate positive hypotheses--namely, as yet unknown,
nonstandard Riemann
hypotheses (over finite fields); cf. Figure~\ref{fig:finalgoal}.


\begin{figure} 
\begin{center}
\psfragscanon
\epsfig{file=finalgoal.eps, scale=.6}
\end{center}
      \caption{The ultimate goal of GCT}
      \label{fig:finalgoal}
\end{figure}


























































































==> preface.tex <==
\section*{Introduction} 
Geometric complexity
theory (GCT) is an approach to the  fundamental problems of
complexity theory, such as the (nonuniform) $P$ vs. $NP$
\cite{cook,karp,levin},
$P$ vs. $NC$ and $\#P$ vs. $NC$ \cite{valiant} problems
(Figure~\ref{fig:complexityclasses}). 
The main barrier 
towards these problems is   the {\em   feasibility
barrier} described here (Section~\ref{})   and  the basic strategy
of GCT for crossing this barrier is called the flip [GCT6,GCTflip].
The main result of  GCT [GCT6,7,8,GCT11] is conjectural scheme for
the implementation of the flip.
Its  final goal
is to prove the {\em explicit proof conjecture} (Section~\ref{}),
which says that
the $P\not = NP$ conjecture has an {\em extremely explicit proof}, by 
which we mean a proof  
that shows existence of  proof certificates
of hardness for the $NP$-complete function under consideration 
that are short (of polynomial size), easy to verify, discover and decode 
(in polynomial time); cf. Section~\ref{}.
This  is supported by 
two concrete lower bounds of GCT based on weaker forms of the flip: namely
the  $P \not = NC$ result without bit operations [GCTlocal] (Section~\ref{})
and a mathematical  form of the $\#P\not = NC$ conjecture in characteristic
zero (Section~\ref{}).
This introduction gives a short overview  of GCT outlining these developments.


The original lectures did not describe the 
the  feasiblity   barrier  and the explicit proof conjecture.
But all the mathematical effort in   GCT as described in these lectures 
goes towards crossing this barrier and  producing such an explicit proof.
Hence, we describe  them   here so that the root cause of 
all difficulties encountered in GCT and the need for nonelementary techniques
to cross this formidable barrier
becomes clear  at a high level before we get into any mathematics. 


The original IAS lectures did not state the first lower bound and
only stated   a special case of the second 
lower bound called  the weak form of the $\#P$ vs.
$NC$ problem. The article \cite{boris} showed that this weak form 
is too weak; i.e., it can be proved    by an elementary  technique
that  cannot cross the natural-proof barrier \cite{rudich}.
We cannot prove the full mathematical form by such
techniques for the reasons given in Sections~\ref{}.
Its  proof here 
is based on the results of GCT1,2 and geometric invariant theory 
\cite{mumford}. It crosses the relativization \cite{solovay}, 
natural proof \cite{rudich}, 
algebraic degree \cite{GCTlocal}, and algebrization \cite{aaronson} 
barriers simultaneously  and is (strongly) explicit. 
These two lower bound results  provide a concrete support  for 
the GCT approach.









\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes (no proper containments are known)}
      \label{fig:complexityclasses}
\end{figure} 




\section{The  feasibility barrier} \label{sfeasibility}
The  feasibility barrier is {\em universal} in 
the sense that it has to be crossed by every approach towards the $P$ vs. 
$NP$ problem, not just GCT, regardless of which areas of mathematics it goes
through. In contrast, the other known barriers 
such as the relativization \cite{solovay}, natural-proof \cite{rudich},
algebraic-degree [GCTlocal],  and algebrization  \cite{aaronson} barriers
are {\em local} in the
sense that they are only applicable to specific areas of mathematical
techniques and hence can simply  be bypassed, as in GCT. 
In other words, a local barrier is like a guiding post which tells 
us what must not be done, and hence must  be bypassed,  whereas 
a universal barrier cannot be bypassed no matter what, because it tells us
what must be done, i.e., it has to be crossed.
Due its universality, the feasibility barrier
captures the root cause of all the 
difficulties in the $P$ vs. $NP$ and related  problems, and it turns 
out to quiet formidable, as expected. 

Before we describe it, let us  remark  that the 
presence of such a universal barrier should not be surprising,
because the $P \not = NP$ conjecture    is itself a {\em universal} statement
regarding all of mathematics. Namely, 
if this conjecture fails to hold,
every theorem in mathematics that has a proof of reasonable 
length  can be proved  efficiently by a computer in 
time polynomial in the length of its shortest proof. No other known
conjecture in mathematics has such stunning mathematical sweep. 
Given the universal nature of this problem, it then stands to reason that
the main  barrier towards this problem--the root cause of its 
difficulty--should also be
{\em universal}. The  feasibility barrier is this universal barrier.
Due to its universal nature, it 
cannot be  fully formalized like the local barriers, because any barrier
that can be fully formalized would tend to be local.  But since it is the 
root cause of the difficulty of the $P$ vs. $NP$ problem, 
we wish to  state it as clearly as possible. 

Towards that end,  let us 
fix an appropriate $NP$-complete function $f(X)=f(x_1,\ldots,x_n)$. 
The goal of the nonuniform $P$ vs. $NP$ problem  is to show that 
there does not exist a circuit $C=C(X)$ of size 
$m=\poly(n)$  that computes $f(X)$, $n\rightarrow \infty$. 
Symbolically, let  $f_C(X)$ denote the function computed by $C$. 
Then we want to prove that
\begin{equation} \label{eqiohp}
\forall n, m=\poly(n) \ \forall C \exists x : f(X)\not = f_C(X). 
\end{equation}

Equivalently, the goal is to prove:

\noindent {\bf (IOH)}: For every large enough $n$, and $m=\poly(n)$,
there  exists a {\em trivial obstruction
(i.e. a ``proof-certificate'' of hardness)} to efficient computation of
$f(X)$. Here by a trivial obstruction we mean
a table (cf. Figure~\ref{fig:trivialtonew}) that lists for every small 
$C$  a counterexample  $X$ such that $f(X)\not = f_C(X)$.



The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$.
Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. 
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time to decide if such a table exists for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. So
we call  this trivial, brute force 
strategy of proving the nonuniform $P$ vs. $NP$ conjecture,
based on existence of trivial obstructions,  a {\em theoretically
infeasible strategy}. Also because
it is really just a restatement of the original problem.
Hence, the terminology  IOH (Infeasible Obstruction Hypothesis)--we also
call it {\em theoretically infeasible}. 


Any approach to the  $P$ vs. $NP$ problem has to 
answer the following question: 

\begin{question} \label{qfeasible} {\bf (Feasibility Barrier)} 
Why should the approach be    feasible (i.e., lead to a proof) 
even theoretically?
That is, in what sense is it fundamentally 
different from the  trivial, infeasible approach above, 
and not just a restatement of the original problem? 
\end{question}

This question is  natural and not new, 
because,  in view of the universality 
of the $P \not =  NP$ conjecture, it has always been questioned right from
the begining  why it
should even be provable. For example,  why can it not be 
independent of the formal axioms of mathematics? This was studied 
in some early works; cf. \cite{aaronsonformal} for their  survey. It 
was also the 
motivation behind identifying  the fundamental 
barriers towards this problem,
such as the relativization \cite{solovay} and natural-proof 
\cite{rudich} barriers.
The latter barrier  roughly says that the proof techniques akin to
the ones used for proving the lower bounds for constant depth circuits
would not work for the $P$ vs. $NP$ problem
in a sense because the problem itself
stands in their way, rendering them theoretically infeasible, so to say.
Admittedly, such proof techniques constitute  only  a very specific 
subarea of mathematics, which is why this  barrier can be considered 
local,  and we cannot conclude anything about the proof techniques
which go through other areas of mathematics on the basis of such a local
barrier (for the reasons explained in more detail in Section~\ref{sexp}).
But one can still wonder if the $P$ vs. $NP$ problem could not
stand in the way of every proof technique like this, rendering it
theoretically infeasible, and thereby precluding its own proof. This
does not seem inconceivable since the problem itself says that the discovery
is hard, and so, why could it not make the discovery of its own proof hard?
Hence arises the question:
why should a given proof technique 
be even theoretically feasible as per some 
reasonable notion of theoretical feasibility. 
The feasibility barrier is simply the task of answering this 
fundamental question, which has been lurking in the background of the $P$ vs.
$NP$ problem right from the begining.
It is universal in the sense that every approach has to answer
Question~\ref{qfeasible}, and
until it is answered clearly,
however sophisticated an approach may be, it cannot be
considered to be more than a  restatement of the original problem.

Now we have specify what is meant by answering
Question~\ref{qfeasible} clearly. Let us assume that the approach
is nonuniform unlike the uniform approaches used to prove the 
classical hierarachy theorems, 
since the relativization barrier \cite{solovay} 
suggest such  approaches 
have a fundamental limitation in the context of the $P$ vs. $NP$ problem.
%If there exists a nonrelativizable uniform approach, we
%leave the task of answering Question~\ref{qfeasible} to that approach. 
By  a nonuniform approach, we mean 
it shows existence of some obstruction $O_{n,m}$ 
(proof-certificate of hardness as per that approach) depending on 
$n$ for every $n$ and $m=\poly(n)$.
All proofs of nonuniform lower bounds so far,
e.g. \cite{sipser,razborov,GCTlocal}, prove existence of such obstructions
that are better than the trivial obstructions in the lower  bound problems
under consideration.
For example, in the proof of the lower bound for constant depth 
circuits   an obstruction is a  table that lists 
of every constant depth small size circuit 
a counter example that could  be potentially produced by the derandomized 
polynomial time  version \cite{} of the random restriction procedure 
\cite{sipser}.
This obstruction  is better than the brute force  trivial obstruction in the
sense that its each row can be constructed in polynomial time instead 
of  exponential time as in   the brute force method. 

Formally:

\begin{defn} \label{dobst}
We say that a family ${\cal O}=\cup_{n,m} {\cal O}_{n,m}$ of mathematical
objects is an {\em obstruction family} to efficient computation of 
$f(X)=f(x_1,\ldots,x_n)$ if
\begin{enumerate} 
\item Each object $O$ in ${\cal O}$ called an {\em obstruction} has 
a specification (a bit string)  denoted by $[O]$. 
An object $O_{n,m} \in {\cal O}_{n,m}$ is called an obstruction to
computation of $f(X)$ by circuits of size $m$.
\item  Nonemptyness of ${\cal O}_{n,m}$, i.e.,
existence of an obstruction $O_{n,m}$ serves as a
guarantee that $f(X)$ cannot be computed by circuits of size $m$.
Specifically, there is a decidable decoding algorithm that given $n,m$ 
and the specification $[O]=[O_{n,m}]$
of an obstruction  $O=O_{n,m}  \in {\cal O}_{n,m}$ 
produces a trivial obstruction to computation of $f(X)$ by circuits 
of size $m$, i.e., a table that gives for each circuit $\C$ of size 
$m$ a counter example $X$ so that $f_C(X)\not = f(X)$. 
This decoding algorithm must be guaranteed to be correct. 
That is, it must produce such a trivial obstruction correctly 
for every obstruction. But we put no restriction on the computational
complexity of the algorithm.
\end{enumerate}
Given an obstruction $O \in {\cal O}$, we let $\bitlength{O}$ denote
the bitlength of its description $[O]$.
We say that an obstruction family is uniform if $\bitlength{O}$ is $O(1)$
for every obstruction $O$.
\end{defn}

In principle, we do not need a decoding algorithm here. All we 
need is a guarantee than nonemptyness of ${\cal O}_{n,m}$ implies
that $f(X)$ cannot be computed by circuits of size $m$. But decoding 
algorithm makes everything concrete, so we will assume that it is there.

The most important  obstruction is a final proof of the $P \not = NP$ 
conjecture. It has  $O(1)$ length and can be verified in $O(1)$ time.
We call it the final obstruction.
For this obstruction there is a {\em trivial
deconding algorithm}, namely, for each circuit $C$ of size $m=\poly(n)$,
just compute $f_C$ and $f$ on all $X$ of length $n$ in any order and produce 
the first  $X$ on which they differ. A final proof of the $P \not = NP$ 
conjecture guarantees that this algorithm is correct, but it is not until then.
Once there is a final proof, an $O(1)$-size program for $f(X)$,
or far that matter any NP-complete function,
also becomes an obstruction with a trivial decoding algorithm,
but not until then.
Other well known $O(1)$-size obstructions in the $P$ vs. $NP$ 
problem are polynomial time  one way functions 
or  pseudo random generators.  But the problem of proving existence 
of such obstructions is  believed to be 
even harder than the $P$ vs. $NP$ problem.
Alternatively, we can consider an $O(1)$-size program for an explicitly given
conjectural one way function or pseudo random generator. This
is  an obstruction only 
after it is proved that the  function under consideration
is indeed a one-way function or a pseudo random generator,  but 
proving that  is again believed to be   harder than the original 
$P$ vs. $NP$ problem. Thus it can be seen that 
any argument based on such  uniform, i.e., $O(1)$-size objects is bound to be
circular, which is what has to be avoided to cross the feasibility barrier,
and furthermore,
the relativization barrier \cite{solovay} 
also suggests that arguments based on uniform
objects may have fundamental limitations.
Hence, our  interest   is primarily in the
intermediate obstructions that are meant to be a vehicle in 
a given nonuniform approach  to reach 
a final proof (i.e. a final obstruction)
in the spirit of the intermediate  obstructions that are 
used to prove the earlier nonuniform lower bound results 
\cite{sipser,razborov,GCTlocal}. Hence,
whenever we say obstructions  we have in mind intermediate 
nonunifrom obstructions
which lie on the way from the trivial to the final obstruction.


To answer Question~\ref{qfeasible}, 
a nonuniform approach has to:
\begin{description}
\item[I] Come up with a new notion of (nonuniform) obstruction which
is fundamentally different from the trivial obstruction, and thus 
precisely formulate the new Obstruction Hypothesis (OH), which says 
that such obstructions should exist when $m=\poly(n)$, and which provably 
implies the old IOH. The approach 
must  provide an unconditional  proof  here that the 
decoding algorithm associated with the obstructions is correct, i.e., 
each  object $O_{n,m}$ is indeed an  obstruction whenever it exists
(but we allow an approach to work
over  an arbitrary base field of computation, 
not necessarily boolean or finite, as 
we are doing here for simplicity).
This is meant to  rule out circular arguments, like the ones  based on uniform 
objects which are obstructions   only assuming a result that is at least 
as strong or stronger  than the original lower bound problem.
The main issue that has 
to be settled then is:  do  these new obstructions 
really exist when $m=\poly(n)$, and even if they do, why is the
problem of proving their existence fundamentally different or better than the 
original problem of proving existence of trivial obstructions? 
This is to be justified in the next steps.

\item [II] As a first step towards that end, 
precisely formulate the notion of theoretical feasibility, 
and  justify why it is a reasonable notion, i.e., why does a theoretically
feasible problem as per this notion means a problem that can be solved 
by a technique that is fundamentally better than the brute-force search,
just as the literature in complexity theory justifies that 
a problem in $P$ can be solved by a technique that is fundamentally 
better than a brute force search.
\item [III] 
Prove that the problem (OH) of proving existence of  such obstructions
is  theoretically feasible as per this notion
in contrast to the theoretically infeasible problem of proving
existence of trivial obstructions (IOH).
One possible way to do this is to prove that  the problem of 
recognizing (verifying) an obstruction is 
theoretically feasible as per this notion. After all,  every 
approach is in a sense a search for obstructions. It is possible 
that the approach may seek 
to prove existence of obstructions by a nonconstructive 
method, without exhibiting any obstruction explicitly. But if it is not
theoretically feasible for the approach to even recognize (verify) 
what is searching for,
then there is a serious problem with the approach.
\item [IV] Justify why it is plausible
that the task of proving OH should
become practically feasible once it  is  theoretically feasible
by proving concrete nontrivial lower bounds 
in restricted  settings using the approach; i.e., 
by showing that theoretical 
feasibility can lead to practical feasiblity in nontrivial cases.
\end{description}

We will say that the {\em the feasibility barrier} is crossed and
that the approach is {\em theoretically feasible} once 
Question~\ref{qfeasible} has been answered clearly in this manner.
As we will see in this article, this barrier is extremely 
formidable. Its crossing  is too much to expect from any approach 
at this stage. But any   approach to the $P$ vs. $NP$ problem 
should  provide using its strategy for crossing 
this barrier at least the following:



\begin{enumerate} 
\item[A] A concrete superpolynomial lower bound that  is a 
restricted form  of any of the fundamental separation problems 
in Figure~\ref{fig:complexityclasses} 
(the center of complexity theory)
in a realistic and natural model of computation, where by natural and
realistic we mean a model that is actually used extensively in practice and is
not defined for the sake of proving  the lower bound.
\item[B] A concrete  lower bound that is a restricted  form  of
any of these separation problems   whose 
proof  demonstrates that the 
approach  bypasses the earlier 
relativization \cite{solovay}, natural-(probabilistic)-proof {rudich}, 
algebraic degree [GCTlocal], and 
algebrization \cite{aaronson} barriers simultaneously.
Here, in view of the fundamental nature of these barriers, we agree to
take them in spirit rather than letter. Because, though these barriers 
are defined only for the unrestricted $P$ vs. $NP$ problem, they make 
sense in  any reasonable restricted setting. Thus we assume that
the relativization barrier   applies to any technique that views 
computation abstractly without algebrizing it, algebraic degree or
algebrization barrier to any low degree technique,
and the natural proof barrier to any technique that works 
for most functions with the meaning of most as in \cite{rudich}. 
\item[C] A concrete mathematical support for its
theoretical feasibility  in  the general  unrestricted setting.
\end{enumerate}
We shall refer to these as the criteria A,B, and C to evaluate any approach.
Here C is really a matter of subjective interpretation 
as per the approach. But A and B are 
the criteria that all approaches can agree on given that the fundamental 
difficulty of proving any natural and realistic superpolynomial lower bound
and of crossing the earlier local barriers simultaneously has been
well recognized by now. Hence if an approach can meet the criteria
A and B, one can 
be  reasonably sure that it is not restating the original problem or 
going in circles, which is  what crossing the feasibility barrier
finally means: overcoming the  seemingly self-referential nature of the
$P$ vs. $NP$ problem.



\section{The flip: going for explicit construction}
The most obvious and natural strategy for crossing the feasibility barrier
is suggested by the $P$ vs. $NP$ problem itself. For that, 
let us see what is wrong with the trivial obstruction from the 
complexity-theoretic point view. That is quite clear. First, it is long,
i.e.,  its description takes exponential space. Second, it is hard to
verify (and also construct); i.e., this  takes exponential time.
Since $NP$ is the class of problems with ``proof-certificates'' that 
are short (of polynomial-size) and easy to verify (in polynomial-time), 
this then leads to the following strategy, called the {\em flip}
[GCT6,GCTflip],
for proving the nonuniform
$P\not = NP$ conjecture, with the obvious complexity-theoretic
interpretation of the phrase theoretically feasible.

\begin{figure} 
\begin{center}
\epsfig{file=trivialtonew.eps, scale=.6}
\end{center}
      \caption{From trivial to new obstruction}
      \label{fig:trivialtonew}
\end{figure} 


\noindent {\bf I. (The flip: theoretical feasibility of verification) :}
Formulate a new notion of a (nonuniform)
obstruction (cf. Definition~\ref{dobst})
that is {\em explicit}, by which 
we mean {\em short and easy-to-verify}.
Formally:

\begin{defn} \label{defnobstexplicit}
We say that an obstruction family ${\cal O}$ (Definition~\ref{dobst}) 
is {\em explicit} if:
\begin{enumerate}
\item {\bf Shortness:}
For any $n$ and $m< 2^n$, if there exists  an 
obstruction in ${\cal O}_{n,m}$ 
to efficient computation of $f(X)$ by circuits of size $m$,
then there also exists a short  obstruction $O_{n,m}$ in ${\cal O}_{n,m}$, 
where by short we mean 
the bitlength $\bitlength{O_{n,m}}$ of its specification is
$\poly(n)$ (note the bound does not depend on $m$).
\item {\bf Easy-to-verify:} Given $n,m$ and a bit string $x$, whether 
it is the specification $[O_{n,m}]$ of an obstruction  
$O_{n,m} \in {\cal O}_{n,m}$ can be decided  in $\poly(n,\bitlength{x})$
time, where $\bitlength{x}$ denotes the bitlength of $x$.
\end{enumerate}
\end{defn} 

This means that the problem of verifying (recognizing)
an obstruction (or rather its specification) belongs to $P$, and hence,
is theoretically feasible (``easy''). Thus this notion 
of an obstruction is then fundamentally better than the theoretically
infeasible trivial obstruction as far as verification is concerned.





Now, to prove $P \not = NP$ it  suffices  to show that 
${\cal O}_{n,m}$ is nonempty if $m=\poly(n)$, $n \rightarrow \infty$.
In this step, the approach should also justify on the basis of
mathematical evidence why this should be
so assuming  $P \not = NP$ (nonuniform).
This circular reasoning at this stage is only meant to convince us 
before we  plunge ahead that such obstructions should exist, i.e., there 
is no loss of essential information,  
assuming $P \not = NP$, which we take on faith, and the goal
now is to prove the existence of these obstructions.


Intuitively (cf. Figure~\ref{fig:trivialtonew}), we can think of 
the new  explicit 
obstruction as an 
encryption of a some trivial obstruction of exponential
size which is highly compressable
in the information theoretic sense--i.e., such that 
its description can be encrypted in polynomial size--and furthermore,
such that the encrypted information can also be verified fast in polynomial
time.
At the surface, it is hard to believe that 
such an obstruction can even exist. To see why, let us note that 
the problem of  verifying 
if a given $X$ is a counterexample to a given $C$ is  intractable since 
it requires evaluating the NP-complete function $f(X)$, which cannot 
be done  efficiently assuming $P \not = NP$, and furthermore
$f_C(X)$ too cannot be evaluated  in polynomial time if the size $m$ of
$C$ is superpolynomial (say $n^{\log n}$). To verify the new obstruction,
in effect, we  are 
{\em implicitly} verifying   all exponentially many  rows of some 
trivial obstruction  in polynomial time, but without 
even knowing what that trivial obstruction is, since the verification 
procedure cannot affort to decrypt the new obstruction using
the associated decoding procedure to get an exponential
size trivial obstruction.
It may seem that 
such a scheme could not possibly exist and that the $P \not = NP$ conjecture
would again stand in the way either directly or indirectly (implicitly).
Implementation of  this step of the flip
amounts to   showing that
the $P\not = NP$ conjecture
would not stand in the way--which is what crossing the feasibility barrier
essentially means.
Of course, the actual implementation 
does not have to  encrypt any trivial obstructions. The 
new obstruction could be such that its existence implies existence of
some trivial obstruction in a highly indirect way. That is,
the computational complexity of the associated decoding algorithm 
(which we are only assuming is decidable) could be extremely high. 
And for that matter, we do not even need such a decoding algorithm 
as long as there is a guarantee that existence of an obstruction implies
existence of a trivial obstruction.
But if it is possible to get a trivial obstruction from a new obstruction
easily; i.e., if the asociated {\em decoding algorithm} works in polynomial
time, by  which we mean 
given specification of 
a new obstruction $O_{n,m}$ and a small $C$ of size $m$ it
produces in $\poly(n,m, \bitlength{O_{n,m}})$ time a counter example $X$ for 
$C$--then we say that the new obstruction is {\em easy to decode}. 
Note that if $O_{n,m}$ is short, i.e., $\bitlength{O_{n,m}}=\poly(n)$,
then this running time is $\poly(n,m)$.
Though we do not need the decoding algorithm to work in
polynomial time, at least at this stage, it may intuitively
help to imagine that the new obstructions are easy to decode.


It may be noticed that a final proof of the $P \not = NP$ conjecture 
is  an explicit obstruction for every $n$ and $m=\poly(n)$ 
as per Definition~\ref{defnobstexplicit} since it can be verified 
in $O(1)$ time. That is how it ought be since a final proof is 
the most explicit obstruction to the equality  of $NP$ with $P$ that one
can imagine. Similarly, an $O(1)$-size  program  for a one 
way function is an explicit obstruction for every $n$ and $m=\poly(n)$ 
after there is a final proof 
that it is indeed a one way function, i.e., when it is accompanied by
such a final proof  (without  it it is not even an 
obstruction, as already pointed out). 
But we are assuming here that the approach has not been
so lucky as to come with a final proof right in the first step. That is, 
the new obstruction in this first step is not a 
final proof or  accompanied by a final proof
but only a vehicle towards the final proof
as in the proofs of the earlier nonuniform lower bounds. 





\noindent {\bf II. (The strong flip: theoretical feasibility of discovery) 
[optional]:} 
Give a $\poly(n)$  time algorithm for deciding,
for any given $n$ and $m< 2^n$,
if there exists such a new  obstruction, and constructing the specification of
one if one exists. This means the problem of discovering an obstruction
belongs to $P$, and hence, is theoretically feasible (``easy'').
Formally, 

\begin{defn} 
We say that an explicit family of obstructions
(Definition~\ref{defnobstexplicit})
is {\em strongly explicit} if 
there is a discovery algorithm that given any $n$ and $m < 2^n$ 
decides in $\poly(n)$ time if ${\cal O}_{n,m}$ is nonempty
and, if so, produces in this much time specification $[O_{n,m}]$ of
an obstruction $O_{n,m} \in {\cal O}_{n,m}$.

We say that a strongly explicit family is {\em extremely explicit} 
if the obstructions are easy to decode; i.e., 
given the specifcation of a new obstruction $O_{n,m} \in {\cal O}_{n,m}$
and a small $C$ of size $m$ the associated decoding algorithm 
produces in $\poly(n,m, \bitlength{O_{n,m}})$ time a counter example $X$ for 
$C$. 
\end{defn}

Again the $P\not = NP$ conjecture seems to stand in the 
way of this step, because the conjecture  says discovery is hard, whereas 
this step says  discovery (of its own proof) is easy. 




\noindent {\bf III. (Practical feasibility):} 
Using the ``easy'' criterion for recognizing an obstruction 
in step I, prove:

\noindent {\bf OH (Obstruction Hypothesis):} If 
$m=\poly(n)$, then for every sufficiently large $n$, there exists 
such a short obstruction $O_{n,m} \in {\cal O}_{n,m}$. 

%We call such an obstruction family $\{O_n\}$  {\em explicit}.


If we also have an ``easy'' procedure for discovering an obstruction 
in step II, then this amounts to  proving that this 
procedure always discovers and constructs the specification of 
an obstruction $O_{n,m}$  successfully when $m=\poly(n)$--i.e., the discovery
procedure works correctly (successfully). So this step amount to 
proving correctness of the discovery program.
%If it is correct, we 
%call such an obstruction family $\{O_n\}$ {\em strongly explicit}.

We  call a proof of the $P\not = NP$ conjecture an {\em explicit proof},
based on the given notion of obstructions, if 
it is based on the flip and carries out the step I, a {\em strongly explicit
proof} if it carries out both steps I and II, and an 
{\em extremely explicit proof} if
in addition, the obstructions are easy to decode.




We  say that OH becomes {\em theoretically feasible}
once the steps I and II have been carried out, 
since the associated problems of verifying and constructing an obstruction 
then become theoretically feasible, i.e., belong to $P$--in other words, 
the theoretically infeasible task of proving IOH is transformed 
into a theoretically feasible task of proving OH, and 
however hard the task of proving OH may be mathematically,
the $P\not = NP$ conjecture  can be expected not to stand in the way
of its proof.
Hence, the name of this strategy {\em the flip}:
from the infeasible to the feasible. 
We also say that the {\em feasibilty barrier for verification} 
is crossed once step I is carried out, and the {\em feasibility barrier
for discovery} is crossed once step II is carried out, and the 
{\em feasibility barrier is crossed} once both the barriers are 
crossed. We also say that the approach becomes {\em theoretically
feasible} once the feasibility  barrier is crossed.


Of course, theoretical 
feasibility of OH  does not automatically  imply that the task of 
actually proving it would be practically feasible.
For that, it is also necessary
that the algorithms for verifying and discovering an obstruction in
steps I and II have a simple enough structure that can be used for
proving OH in step III; i.e.,  for proving correctness of the discovery 
procedure. If not, they have to made simpler and simpler until
this becomes practically feasible.
Theoretical feasibility of the approach   basically
means that the $P\not = NP$ conjecture should 
no longer stand in the way of the 
approach, and hence, there is no philosophical barrier to 
practical feasibility, though transforming  a theoretically
feasible  approach into a practically feasible approach  can be  a challenging
mathematical problem in itself.

Step II above  has been labelled optional, because
there may exist a  proof of the $P\not = NP$ conjecture
along the  lines of the flip  that  takes substantial
short cuts in this step.
For example,  a proof technique may simply be lucky and come 
up with a right guess for the obstruction family (since it is meant to be
carried out by humans and not machines). 
But substantial short cuts in step I seem difficult. After all, as we have
already said,  if the proof
technique cannot even recognize easily what it is searching for, then
there is  a serious problem.


Here is  another way to look at the flip 
(cf. Figure~\ref{fig:IOHcomplexityintro}). 
For that let us reexamine IOH. 
The problem of deciding,  given $X$ and $C$, if  $\f(X) \not = f_C(X)$
belongs to co-$NP$.
Since there are two alternating layers of quantifiers in (\ref{eqiohp}),
the problem of verifying it--i.e. the problem of deciding 
if  a trivial obstruction exists for given $n$ and $m$ specified
in unary--belongs to $\Pi_3$. We refer to this as the decision
problem associated with IOH and denote it by $DP(IOH)$.
When $m=\poly(n)$,  IOH  is expected to be a tautology,  though
we do not know that yet, and hence, the answer to this decision
problem  would then be always yes.
But for general $m$, not just $m=\poly(n)$, it is a hard decision
problem that  lies  high in the complexity hierarchy
(cf. Figure~\ref{fig:IOHcomplexityintro}) and this is another reason for
referring to IOH as theoretically infeasible.
Let $DP(OH)$ be  the decision problem 
associated with OH, by which we mean the problem of deciding existence of 
a (new) obstruction for given $n$ and $m$ specified in unary. 
It belongs  to $NP$
after execution of the step I and to $P$ after the step II.
Once this final $P$-verifiable OH is proved, it is reduced to a tautology
(FOH: Final Obstruction Hypothesis), which can be verified in 
$O(1)$ time. This gives us the final $O(1)$-size proof.
Thus the basic idea of the flip is to systematically 
eliminate the quantifiers in IOH  and reduce the complexity of the
decision problem associated with 
the  obstruction hypothesis until the obstruction hypothesis  is finally
reduced to  an $O(1)$-time verifiable  tautology;
cf. Figure~\ref{fig:IOHcomplexityintro}. 

But this extremely simple strategy is also deeply paradoxical.
Because it may be conjectured that  $DP(IOH) \in \Pi_3$ 
above is hard, i.e., does not belong to $\Pi_2$ or $\Sigma_2$.
Though this problem may not be $\Pi_3$-complete, we can still call
it a universal problem, because the $P$ vs. $NP$ problem and 
hence IOH is a universal statement about mathematics. 
So to make the flip work, the approach has to come with a new 
notion of an obstruction so that for $m=\poly(n)$ the new OH is equivalent 
to IOH logically (both becoming tautologies),
and yet the decision problem for the 
new OH for general $m$ 
should belong to $NP$ for the flip and $P$ for the strong flip. 
Furthermore, the new OH is also a universal statement
since it is meant to imply $P \not = NP$.
Assumming that the polynomial time hierarachy does not collapse,
or more specifically, that $\Pi_3 \not = NP \not = P$, such reduction
of a universal statement in $\Pi_3$ to another in $NP$ and then
to $P$ may seem impossible.
That is, as the flip starts moving from IOH towards its final 
destination FOH through the polynomial time hierachy as shown
in Figure~\ref{},  it may seem as if  it may bring about a collapse of this 
hierarchy in its wake  thereby disproving the very conjectures 
it is meant to prove.   So once again we see the self-referential
nature of the  feasiblity barrier which is saying here 
that the main  barrier towards the $P$ vs. $NP$ problem is the problem itself.





For mathematical problems which are not universal, theoretical feasibility
can be meaningless. For example, consider 
a trivial  assertion $\forall A, B: A + B = B + A$ where $A$ and $B$ 
are $n\times n$ matrices.
The problem of brute force verification of this assertion 
belongs to $\Pi_1$, but that is no indication of its difficulty,
and we cannot say that it is a theoretically infeasible hypothesis.
Indeed, it is well known
in proof theory that the logical complexity of an assertion, i.e., the
number of alternating quantifiers in it, is in general no index of its
mathematical difficulty. In the context of the $P$ vs. $NP$ problem 
theoretical feasibility of elimination
of the quantifying variables in IOH
is  a fundamental  issue only because of its universality and because 
those alternating quantifiers are intimately related to the 
the alternating quantifiers used to define the conjecturally 
noncollapsible  polynomial time hierarchy.
For mathematical
problems that are not universal, e.g. the Riemann hypothesis,  practical 
feasibility is all that matters. Because however hard they may be, they do not
say that discovery is hard. 


The  flip can also be formulated
in the theory of pseudorandom generators. For that we  fix 
an explicit $NP$-computable pseudorandom generator 
$g$ that conjecturally fools 
small  circuits (assuming which  $P \not = NP$). We  then express 
this property as an IOH for $g$ and associate a decision problem with it.
But it will be seen that this decision problem lies even higher in
the complexity hierarachy than the IOH for the $P$ vs. $NP$ problem; 
specifically it lies  in $\Pi_3^{BPP}$. Hence
the corresponding flip, which begins at this IOH  and runs towards FOH for $g$ 
through the complexity hierarchy, is harder.
In other words,  this says  that the theory
of pseudorandom generation (derandomization)
is in general  harder than the theory of lower bounds, and hence,
hardness should be proved first  and then transformed into
pseudorandom generation  as per the hardness vs. randomness 
principle \cite{}. This is why we focus on lower bounds in GCT at present.





The flip considered so far  is {\em global} because it is 
based on a global  obstruction of $\poly(n)$ size 
that acts as a proof certificate of hardness for all small
circuits. We may also consider a  {\em local  (strong) flip}
based on a {\em local (strongly) explicit 
obstruction}, by which we mean .
a table specifying a counter example $X$ for each small circuit $C$ of size 
$m$ whose each row can be verified (constructed) in $\poly(n,m)$ time. 
\ignore{It may be conjectured that the local strong flip is possible in 
the context of the $P$ vs. $NP$ problem: i.e. for
any $NP$-complete $f(X)$, there exists an algorithm that 
produces a counter example $X$ for 
any circuit  $C$ of $m=\poly(n)$ size in $\poly(n,m)=\poly(n)$ time. 
We shall refer to this as the {\em local strong flip conjecture} for
the $P$ vs. $NP$ problem--it is evidently much stronger than the nonuniform
$P\not = NP$ conjecture.}
The local flip  crosses the  feasibility 
barrier {\em locally} in the sense that a 
locally  explicit  obstruction is fundamentally different and better 
than a trivial obstruction. Better locally but not  globally
because  verification 
of the whole locally   explicit obstruction still
takes exponential time. The same  for a local strongly explicit obstruction.
In this sense, the global flip is stronger than the local flip.
The global   flip also implies   the local  flip if there is a polynomial 
time decoding algorithm, since then 
from a  global  obstruction one can get 
a local  strongly  explicit  obstruction easily. 
The $P\not = NP$ conjecture does not stand in the way of this decoding.
Hence intuitively the global (strong) flip subsumes the local (strong) flip.
A local strong flip is used in the proof of the $P\not = NC$ result 
without bit operations described below. But for harder separation problems
it does not seem good enough to cross the feasibility barrier. 
We do not really understand why.






The feasibility barrier and the flip for other problems such as 
the $P$ vs. $NC$ and $\#P$ vs. $NC$ problems are analogous.
Though these problems  are not  universal, 
we  assume that the feasibility barrier is 
meaningful for them  because we look at them as  variants
of the $P$ vs. $NP$ problem.



So far we have been assumming that the underlying field of 
computation is the boolean field. But the $P$ vs. $NP$ and
$\#P$ vs. $NC$ problems can also be defined over an arbitrary ring or
field, and we are  specifically  interested in 
the rings and fields of characteristic zero such as $Z$, $\Q$ and $\C$. 
Let us now explain what we mean by the (nonuniform) $\#P$ vs. $NC$ and 
$P$ vs. $NP$ problems in characteristic zero. 
By the nonuniform (characteristic zero) version of the $\#P$ vs. $NC$ problem
we mean  the permanent vs. determinant problem \cite{valiant}. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented 
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$. %; the best known lower bound on $m$ at present is 
%quadratic \cite{ressayre}.
By linear representation, we mean
the  entries   of $Y$ are  (possibly nonhomogeneous) 
linear functions (over $\C$ or $Z$)
of the entries of $X$. 
There is an analogous characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.
But we shall not worry about it here because all the basic ideas of GCT
are  illustrated in the $\#P$ vs. $NC$ problem in characteristic zero.
We  focuss  on characteristic zero  in this article  because
the nonuniform lower bounds over $Z$ are weaker implications of the
corresponding ones over a finite field (the usual case), and hence
easier. The additional problems that
need to be addressed when the underlying field of computation is finite
will be discussed in  GCT11. 

The flip can also be defined for the $P$ vs. $NP$ and $\#P$ vs. $NC$ 
problems over fields of characteristic zero such as $Q$ or $\C$ and for
algebraically closed fields of positive characteristic such as $\bar F_p$, 
the algebraic closure of the finite field $F_p$, $p$ prime.
All  definitions in the flip 
can be lifted to this setting in the obvious way. We  only give
one critical definition as an illustration assuming that the underlying 
field is $Q$. In this case we say that an
obstruction family is {\em easy to decode} 
if there is a decoding algorithm which given the specification of 
an obstruction $O=O_{n,m}$ and a small circuit $C$ over $\Q$ of size $m$ 
(i.e. whose whole description is of bitlength $m$)
produces in $\poly(n,m, \bitlength{O})$ time a counter example (local
obstruction) $X$ for 
$C$ whose description has  $\poly(n,\bitlength{O})$ bitlength, 
independent of $m$ as long as it is $\le n^{\log n}$ (say). If 
$\bitlength{O}$ is $\poly(n)$ the bitlength of $X$ is then $\poly(n)$
independent of $m$. In other words, smallness
of  obstructions is to be preserved in the process of decoding.

The flip is the defining strategy of GCT. Indeed, GCT may be abstractly
defined as any (geometric) approach to the $P$ vs. $NP$ and related 
problems based on the flip, i.e., explicit construction of obstructions
(for a precise meaning of the phrase geometric see Section~\ref{scharsym}).
By based on the flip, we mean it uses the flip as a basic guiding principle
and goes for ``more or less'' explicit construction of obstructions, 
though it does not have to be completely explicit, i.e., 
some deviations and short cuts are fine and also inevitable as long as 
the spirit  is maintained.
The present (concrete) GCT is one such  approach.
It proposes  a scheme for implementing the flip for the $P$ 
vs. $NP$ and related problems via algebraic geometry, representation
theory and the theory of quantum groups.
This turns out to be a nontrivial affair, as to be expected, because of the
counterintuitive and paradoxical  nature of the flip as explained above.




But before we enter into it, let us 
ask ourselves if the flip, i.e.,  explicit construction, the root 
cause of all difficulties in GCT, is really necessary.
Because, to solve  the  lower bound problems under consideration
we only need to prove existence of obstructions, we do not have to
construct them,  and moreover,
the flip also has the following disturbing   feature.
Namely,  proving a superpolynomial 
lower bound for $f(X)$  via the flip 
is not very different from proving a superlinear 
lower bound, because the
heart of the flip, consisting of the steps I and II, is the same whether
$m$ is superpolynomial or superlinear, and only the final step III differs.
In other words, as per the flip,  modest as well as  strong lower bounds
lie on the other side of the feasibility barrier, and 
the main difficulty in getting to them--the feasibility barrier 
(steps I and II)--is the same.
One may wonder if there is any other gradual way towards the $P$ vs. $NP$
problem on which
we could meet  modest lower bounds much before strong lower bounds without
having to cross  the formidable feasibility barrier first.

After all the flip is only the most obvious and natural way to cross
the feasibility barrier. 
(Whenever we say natural in the context of GCT
we always mean explicit unlike in \cite{rudich} where it means probabilistic.) 
There may exist  nonobvious and 
unnatural (e.g. nonconstructive) ways to cross this barrier.
At present,  we only know 
that one class of nonconstructive techniques 
would not work, namely the ones with probabilistic flavour, which
are ruled out by the natural-(probabilistic)-proof-barrier \cite{rudich}. 
But the probabilistic  proofs constitute  only a 
small subarea of nonconstructive proofs, namely the ones 
which are of a  {\em nonspecific} kind, by which we mean nonconstructive
proofs which apply to most functions or structures under consideration.
Vast areas of
nonconstructive proofs in  mathematics, such as the ones  in algebraic 
geometry and representation theory, are of fundamentally different nature
than probabilistic proofs: they are nonconstructive yet 
{\em very specific};
i.e., they  apply to only very specific functions or structures
under consideration. The natural-(probabilistic)-proof-barrier 
does not apply to
such  nonconstructive but specific proof techniques. 
Indeed, one of the concrete lower bounds of GCT to be discussed below
(Section~\ref{}) has a nonconstructive   proof
which applies to only very specific  functions (generalized permanents) 
and which 
crosses  the natural-proof, relativization,
algebraic-degree (algebrization) and feasibility
barriers simultaneously  in this   setting. 
This gives a concrete evidence that
explicit constructions are  not needed to cross these barriers, and that
they may be crossed by nonconstructive proof techniques as well.


But the mathematical evidence and arguments 
in [GCTflip] sugggest that such unnatural ways to cross the feasibility barrier
may not be any easier and perhaps even harder
than  the natural ways as one may intuitively expect. 
For example, the nonconstructive proof of the lower bound mentioned above
is not much different or easier than the explicit proof (and, in fact, 
a bit harder).
We do not go any further into such  arguments  here.
At a concrete level, 
all we can say is that we are going the natural  way because there 
is no  concrete  alternative.
After all, as pointed out in Section~\ref{sfeasibility}, 
any approach to the $P$ vs. $NP$ problem has 
to meet at least the criteria A, B, and C stated there.

The $P \not = NC$ result without bit operations [GCTlocal] in GCT
(cf. Section~\ref{}) addresses (A).
The mathematical form of the $\#P\not = NC$ conjecture [GCT1,2,6] 
(cf. Section~\ref{})   addresses (B).
The main result [GCT6] of GCT  (cf. Section~\ref{})  gives a conjectural
scheme supported by mathematical evidence to cross the feasibility barrier
via the flip for  the nonuniform
$P$ vs. $NP$ and $\#P$ vs.
$NC$ problems over fields of characteristic zero;
[GCT11] does  the same for   any
field including the finite field (the usual case). This
addresses (C). 


But, at present,  we do not have any  concrete   alternative to GCT
which addresses A, B and C, or for that matter any one of them,
and hence  there is not much that we  can
do but follow  the most natural direction.


We now briefly  describe  the   concrete results of GCT 
which address A, B, and C.

\section{A: The $P\not = NC$ result without bit operations} \label{swithoutbit}
We  begin with 
a  special case of the $P \not = NC$ conjecture [GCTlocal],
which we are calling the $P\not = NC$ result without bit operations,
and which can be considered to be the
first concrete lower bound result of GCT. It was  proved using the weaker
local form of the flip much before the (global) flip was formalized
in [GCT6,GCTflip].
It  says that 
the $P$-complete max-flow problem
cannot be solved in $\polylog(N)$ parallel time using $\poly(N)$
processors in the PRAM model without bit operations,
where $N$ denotes
the total bit length of the input, not just the number of input parameters.
This model  is quite realistic and natural
since it includes virtually all known parallel algorithms for algebraic 
and weighted optimization problems. Hence, this lower bound meets 
the criterion B.
The proof technique of this result is  locally strongly
explicit, i.e.,  the   local strong form
of the flip (but a bit relaxed),  
in the sense that  for each branching program $C$  (i.e. 
a circuit with arithmetic, branching and comparison operations) 
of depth $\log^a N$ and size $\poly(N)$, or even 
$2^{\log^a N}$, for some positive constant $a$,
it produces in $\log ^b N$ time using $2^{\log ^b N}$ 
processors, $b=O(a)$, 
an explicit   counter example  $X$ such that the output of $C$
on $X$ is different from what is expected in the maxflow (decision) problem.
This counter example $X$ is then a proof-certificate of hardness (obstruction)
against $C$.

Local explicitness was not  specifically mentioned 
in GCTlocal. But it is easy to see \cite{GCTpramappend}  that 
the proof technique there actually
produces a locally
explicit proof certificate of hardness, after a little postprocessing,
though the goal was only
to prove its existence (which is why explicitness was not mentioned).
In other words, the proof technique essentially produces a locally
explicit proof-certificate of hardness  whether one cares for it or not.


Local explicitness of the proof technique is the fundamental difference between
this lower bound result and the earlier ones, such as 
the lower bounds for constant depth circuits \cite{sipser}, monotone circuits 
\cite{monotone}, or 
algebraic decision trees \cite{benor}, whose proof techniques are inherently 
nonconstructive. For example, the random restriction method \cite{sipser}
for proving lower bounds for  constant depth circuits gives a randomized 
fast parallel algorithm to produce  for each such
circuit $C$ a local counter example $X$ on which it differs from
the parity function. But the best determistic algorithm to produce 
such a counter example, based on  derandomization of the switching
lemma \cite{agarwal},
takes sequential polynomial time. Locally explicit in this
setting would mean computable by a constant depth circuit
(or in a relaxed sense, 
say $\log \log n$ depth circuit of $2^{\polylog(n)}$ size). 
Similarly, the proof of the lower bound for sorting in
the  algebraic-decision-tree 
model \cite{benor}  inherently requires
exponential time  to produce a counter example, 
so also the proof of the lower bound for monotone circuits \cite{monotone}.
It may be conjectured that there are
(locally strongly) explicit proofs 
for the constant-depth or  monotone circuit lower bounds. 
At present this is  open. But the main point is that such  explicit 
proofs are not  required to prove these lower bounds,
whereas, 
the only way we can prove the weak form of the $P \not = NC$ conjecture
at present is essentially via locally explicit construction. 


\noindent {\em Remark:} Assuming  a stronger lower bound result \cit{}  for 
constant depth circuits, it is easy to show that a counter example 
against a constant depth circuit can be found in $\polylog(N)$ time using
$2^{\polylog(N)}$ processors. And similarly assumming a stronger form
of the $P\not = NC$ result without bit operations, it is easy to show
that a counter example against a branching  circuit of $\polylog(N)$ depth
and $2^{\polylog(N)}$ size can be found by a branching circuit of
 $\polylog(N)$ depth and $2^{\polylog(N)}$ size. But what matters here is not 
how quickly obstructions can be constructed 
once  the lower bound result is proved, but rather how quickly the obstructions
that can be  used to prove the result can be constructed.


In view of the natural proof barrier, it should not be surprising 
that the proof of the  $P \not = NC$ result without bit operations  should
require something fundamentally different from the nonconstructive
techniques of the kind used to prove lower bounds for constant depth
circuits to which this barrier applies,
though, admitedly,  this barrier itself does not suggest that 
we should go for anything explicit (cf. Section~\ref{sexp}).

Another  feature of the proof of this lower bound result  is that  it
is based on classical algebraic geometry, though 
the result itself can be stated in purely 
elementary and combinatorial terms.  No elementary or combinatorial 
proof of this result is known so far.
At present,  the $P\not = NC$ result without bit operations seems to be the
only known  special case of any
of the fundamental separation  problems in 
Figure~\ref{fig:complexityclasses} that  holds unconditionally (and 
superpolynomially) in a realistic and 
natural model of computation. That its  proof needs 
geometry and explicit construction   provides  the first
concrete  support for the
geometric approach based on the flip  (explicit construction), i.e. GCT, 
albeit only in the local setting, and
hence, in retrospect, we shall refer to its proof technique as {\em local GCT}.

But the local  GCT turns out to be too weak for going ahead 
for two reasons.
First, GCTlocal (towards the end of its Chapter 7) 
pointed out a barrier (other than the earlier natural-proof
and relativization barriers), which we shall 
refer to  as the {\em algebraic degree barrier}, though it was not
given any name there. This  says that 
any low-degree proof technique, such as the one there,
which associates with a computation algebraic 
objects (polynomials, varieties, etc.) 
and then reasons solely on the basis of the degrees of those 
objects would not work in the context of the fundamental problems 
such as the $P$ vs. $NC$ problem.
The recent  algebrization barrier \cite{aaronson}
also says  something similar.%, but with different  motivation and framework.
Second, as we already pointed out before, 
the local flip does not seems good enough for the harder separation problems.
So began a search for  a proof technique that can overcome the algebraic 
degree barrier and the locality limitation of local GCT. 


\section{Geometric obstructions}
This then was the motivation behind the 
approach to the fundamental lower bound problems via geometric 
invariant theory that was initiated in GCT1 and 2. 


In GCT1, and 2  certain algebraic varieties with group action, 
called the {\em class varieties}, are associated with the fundamental 
complexity classes, and the $\#P$ vs. $NC$ and $P$ vs. $NP$ problems in
characteristic zero are reduced to showing existence of 
certain representation-theoretic {\em obstructions} to embeddings
amongs such varieties. Furthermore, some results in geometric invariant
theory are also proved to justify why such obstructions should exist 
in  the lower bound problems under consideration and
why they should be mathematically well behaved.

GCT 6 conjectures that these  new obstructions are (globally) explict; i.e., 
their specifications are easy to verify and a short obstruction
exists whenever an obstruction exists


\section{A mathematical form of the $\#P\not = NC$ conjecture}
Using  this notion of an obstruction and the geometric-invariant-theoretic
results in GCT1 and 2,  GCT6 (revised version) then proves a second concrete 
lower bound result of GCT, called a  {\em mathematical
weak form of the $\#P$ vs. $NC$ problem} in characteristic zero for the
reasons given below,
and verifies this conjecture in this special case.
This says  that for any generalized permanent of $k$
$n\times n$ variable matrices $X_1,\ldots,X_k$ 
cannot be represented as a polynomial in the traces of monomials in 
$\bar X^j$, $j\ge 0$, where 
$\bar X_i= B X_i C$, for all $i$,  for any (possibly singular) $n\times n$
complex 
matrices $B$ and $C$.
Here by a generalized permanent, we mean a function $p(X_1,\ldots,X_k)$ 
(of any degree not necessarily $n$)
which has exactly the same symmetries as that of the permanent: i.e., such
that for all nonsingular $n\times n$ complex matrices
$U$ and $V$, $p(U X_1 V,\ldots, U X_k V)=p(X_1,\ldots, X_k)$
iff $\perm(U X V)=\perm(X)$. 
It is called a {\em mathematical form} because there is no restriction here
on the complexity of the generalized permanent or the polynomial in traces.
In that sense, unlike the $P\not = NC$ result without bit operations,
this is a mathematical lower bound, rather than a 
complexity theoretic lower bound,  like the one in Galois 
theory which says that any general polynomial of degree greater than five
cannot be solved by any number of radical operations without any restriction
on the number of such operations.
The proof technique of this result 
produces a strongly explicit family $\{O_n\}$ of  (global) obstructions, 
where each $O_n$ has a specification of $O(n)$ size that can verified
and constructed in $O(n)$ time. The obstruction is global in the sense
that it is against all $B$, $C$ and polynomials in traces. 
Thus this result
provides a concrete support for the (global) flip. Its
proof technique  also  bypasses 
the natural-proof, relativization
and algebraic degree (algebrization) barriers 
simultaneously in this setting.


There is also a  nonconstructive 
proof of this result, which also bypasses these 
barriers.
It  is essentially the same as the
explicit proof, except for the last and the easiest step,
which can be carried out nonconstructively. 
Thus the situation here is again similar to the one for the
$P \not =NC$ result without bit operations. That is, the proof is such that 
it essentially (modulo a little postprocessing at the end) 
yields explicit proof certificates whether one cares for them or not.


To summarize the dicussion so far, the 
$P\not =NC$ result without bit operations in GCT is
a complexity theoretic lower bound proved using  a locally explicit  
technique, the mathematical form of the $\#P\not =NC$ conjecture is a 
mathematical lower bound  proved using a globally
explicit technique.
What is needed now to address 
the fundamental separation problems in Figure~\ref{fig:complexityclasses} 
following this line of investigation 
is  a global flip in this  complexity theoretic setting.
This is addressed next in characteristic zero.



\section{On the flip in general in characteristic zero}
The main result of GCT in this context is a conjectural scheme [GCT6,7,8] 
for explicit construction 
of obstructions (i.e. for the implementation of the global flip) 
for the general $\#P$ vs. $NC$ and $P$ vs. $NP$ 
problems in characteristic zero. 
Specifically, GCT6 shows that the feasibility barrier for verification
(and discovery) can be crossed for these problems assumming
a certain positivity hypothesis called PH1 (and its stronger form PH4).
PH1    says that 
certain  representation-theoretic counting  functions
associated with the class  varieties in GCT1 and 2 
have positive $(\#P)$  convex formulae.
By this we mean  positive convex
representations as the number of integer points in  explicitly 
specified polytopes, like the one for the permanent of a $0-1$-matrix 
as the number of integer points in the perfect matching polytope, which
is both positive (since each integer point is counted 
with a positive sign) and convex. 
Furthermore, GCT6,7,and 8   provide an evidence in support of validity
of PH1, and suggest  an approach for proving it via the theory of
nonstandard quantum groups, which are generalizations of
standard quantum groups \cite{drinfeld}. At the heart of this approach,
  lie certain conjectural positivity hypotheses [GCT8] in the theory
of these nonstandard quantum groups, which are  generalizations of the
known positivity results \cite{kazhdan,lusztig} for the standard quantum group.
The only known proofs of these positivity results are based  on the 
Riemann hypothesis over finite fields \cite{weil2}, which is
itself a profound  positivity result in mathematics. 
Thus the proposed scheme for explicit construction of obstructions 
in GCT6,7,8  seems to need  as yet unknown nonstandard
extension of the work surrounding this central positivity theorem,
which encompasses several areas of mathematics, such as algebraic geometry,
representation theory, quantum groups and so forth.

This should not be too surprising, given that 
the difficulty of explicit construction is by now well recognized 
in complexiy theory.
For example, the explicit construction of Ramanujan graphs \cite{sarnak},
which are the best (optimal) expanders,  also 
needs the Riemann hypothesis over finite fields (for curves).
But explicit expanders  cannot be used to prove a lower bound result.
Explicit constructions that yield hard lower bound results are bound
to be  more difficult. Hence, if a nontrivial  extension 
of the work surrounding the Riemann Hypothesis over finite fields 
is needed for explicit constructions in GCT, that is only to be expected.


\ignore{
If explicit construction is thus the root cause of all difficulties in
GCT, one may finally ask: can it not be avoided somehow?
The weak form of the $P\not = NC$ conjecture in GCT meets criterion (A),
and the generalized weak form of
the $\#P \not = NC$ conjecture meets criterion (B). 
These are the weak forms specific only to  this concrete form
of GCT. Other  approaches (GCT or nonGCT) may lead to other
comparable weak forms which are more suitable to them.
But, at present, these are the only such lower bounds that 
we can prove unconditionally in the context of the $P$ vs. $NP$, $P$ vs. $NC$
or $\#P$ vs. $NC$ problems, i.e., in the main testing ground 
shown in Figure~\ref{fig:complexityclasses} 
for  any approach.
And the only  way we can prove them at present 
is esentially (modulo some postprocessing at the end) 
via explicit constructions based on
geometry.  The situation is summarized in Figure~\ref{fig:summary}.
Here it can be
seen that as the circuit lower bounds start moving in the 
direction of the $P$ vs. $NP$ problem, the proof techniques, for some
mysterious reasons, become more and more geometric and explicit.
This sugests that there may be after all something inevitable 
about  geometry and   explicit constructions, 
which is what GCT means.}






\begin{figure} 
\begin{center}
\psfragscanon
\psfrag{pvsnc}{$P\not = NC$}
\psfrag{#pvsnc}{$\#P\not = NC$}
\psfrag{pvsnp}{$P\not = NP$}
\epsfig{file=summary.eps, scale=1}
\end{center}
      \caption{Circuit lower bounds vs. proof techniques}
      \label{fig:summary}
\end{figure} 



The rest of this article is organized in the form of three chapters,
one per  lecture. The first gives a short overview of the basic plan
of GCT for implementing the flip (explicit constructions) in characteristic
zero, which is elaborated in the next two lectures. 






\noindent {\em Acknowledgement:} The author is grateful to 
Avi Wigderson for arranging the lectures and the hospitality in IAS,
and to Janos Simon, Josh Grochow, and Hari Narayanan for 
the help in presentation. 









==> preface2.tex <==
\section*{Introduction} 
Geometric complexity
theory (GCT) is an approach to  fundamental problems of
complexity theory, such as the (nonuniform) $P$ vs. $NP$
\cite{cook,karp,levin},
$P$ vs. $NC$ and $\#P$ vs. $NC$ \cite{valiant} problems
(Figure~\ref{fig:complexityclasses}), 
suggested in a series of  articles we call GCTlocal \cite{GCTpram},
GCT1-8 \cite{GCT1}-\cite{GCT8}, and GCTflip
\cite{GCTflip}.
A  high level overview of this reasearch plan and the results 
obtained so far  was presented  in 
a series of three lectures in the Institute of Advanced study, Princeton,
Feb 9-11, 2009.  This article contains the material covered in
those lectures after some revision, and gives an overview of GCT.
No background in algebraic geometry, representation theory
or quantum groups is assumed. 
For those who are interested in a short overview, the preface 
and the first chapter (lecture 1) of this article provide
such a short overview.
The video lectures for this series are available at:

http://video.ias.edu/csdm/pvsnp

They may be a helpful supplement to  this article.


This article   gives an overview of the basic plan of 
geometric complexity theory (GCT), an
approach  towards the fundamental lower bound problems  in complexity theory, 
such as :

\noindent (1) 
The $P$ vs. $NP$ problem \cite{cook,karp,levin}: 
 show that $P \not = NP$;


\noindent (2) 
The  $\#P$ vs. $NC$ problem \cite{valiant}: show that 
$\#P \not = NC$.

\noindent (3) The $P$ vs. $NC$ problem: show that $P \not = NC$.

We shall be interested 
in  the stronger  nonuniform versions of these problems.


\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes (no proper containments are known)}
      \label{fig:complexityclasses}
\end{figure} 


In this introduction, we  describe  the main barrier  
towards these problems, called the {\em feasibility
barrier}, and  the basic strategy of GCT for crossing it, called 
the {\em flip} [GCT6,GCTflip], two concrete lower bounds 
of GCT based on weaker forms of the flip: namely
the  $P \not = NC$ result without bit operations [GCTlocal] and
a mathematical  form of the $\#P\not = NC$ conjecture [GCT1,2,6] (which
does not have a naturalizable \cite{rudich} proof unlike its
its weak form in the original IAS lecture which  turned out to be too weak
\cite{boris}) and a brief outline of 
the approach  for implementing the flip in  general.
The feasiblity   barrier was not explicitly described  in 
the original lectures. But 
all the mathematical effort in   GCT as described in these lectures 
in a sense goes towards crossing this barrier.
Hence, we wish
to describe  it explicitly here so that the fundamental difficulty that
GCT is trying to overcome
and the need for the nonelementary techniques that enter into GCT to 
deal with it  would be clear at a high level before we 
get into any mathematics. 



\section{The feasibility barrier and the flip} 
This barrier is {\em universal} in 
the sense that it has to be crossed by every approach towards the $P$ vs. 
$NP$ problem, not just GCT, regardless of which areas of mathematics it goes
through. In contrast, the other known barriers 
such as the relativization \cite{solovay}, natural-proof \cite{rudich},
algebraic-degree [GCTlocal],  and algebrization  \cite{aaronson} barriers
are {\em local} in the
sense that they are only applicable to specific areas of mathematical
techniques and hence can  be bypassed, as in GCT. 
In other words, a local barrier is like a guiding post which tells 
us what must not be done, and hence must  be bypassed,  whereas 
a universal barrier cannot be bypassed no matter what, because it tells us
what must be done, i.e., it has to be crossed.
Due its universality, the feasibility barrier
captures the root cause of all the 
difficulties in the $P$ vs. $NP$ and related  problems, and it turns 
out to quiet formidable, as expected. 

Before we describe it, let us  remark  that the 
presence of such a universal barrier should not be surprising,
because the $P \not = NP$ conjecture    is itself a {\em universal} statement
regarding all of mathematics. Namely, 
if this conjecture fails to hold,
every theorem in mathematics that has a proof of reasonable 
length  can be proved  efficiently by a computer in 
time polynomial in the length of its shortest proof. No other known
conjecture in mathematics has such stunning mathematical sweep. 
Given the universal nature of this problem, it then stands to reason that
the main  barrier towards this problem--the root cause of its 
difficulty--should also be
{\em universal}. The feasibility barrier is this universal barrier.
Due to its universal nature, it 
cannot be  fully formalized like the local barriers, because any barrier
that can be fully formalized would tend to be local. But since it is the 
root cause of the difficulty of the $P$ vs. $NP$ problem, 
we wish to  state it as clearly as possible. 

Towards that end,  let us 
fix an appropriate $NP$-complete function $f(X)=f(x_1,\ldots,x_n)$. 
The goal of the nonuniform $P$ vs. $NP$ problem  is to show that 
there does not exist a circuit $C=C(X)$ of size 
$m=\poly(n)$  that computes $f(X)$, $n\rightarrow \infty$. 
Symbolically, let  $f_C(X)$ denote the function computed by $C$. 
Then we want to prove that
\begin{equation} \label{eqiohp}
\forall n, m=\poly(n) \ \forall C \exists x : f(X)\not = f_C(X). 
\end{equation}

Equivalently, the goal is to prove:

\noindent {\bf (IOH)}: For every large enough $n$, and $m=\poly(n)$,
there  exists a {\em trivial obstruction
(i.e. a ``proof-certificate'' of hardness)} to efficient computation of
$f(X)$. Here by a trivial obstruction we mean
a table (cf. Figure~\ref{fig:trivialtonew}) that lists for every small 
$C$  a counterexample  $X$ such that $f(X)\not = f_C(X)$.



The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$.
Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. 
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time to decide if such a table exists for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. So
we call  this trivial, brute force 
strategy of proving the nonuniform $P$ vs. $NP$ conjecture,
based on existence of trivial obstructions,  a {\em theoretically
infeasible strategy}. Also because
it is really just a restatement of the original problem.
Hence, the terminology  IOH (Infeasible Obstruction Hypothesis)--we also
call it {\em theoretically infeasible}. 


Any approach to the  $P$ vs. $NP$ problem has to 
answer the following question: 

\begin{question} \label{qfeasible} {\bf (Feasibility Barrier)} [GCTflip,GCT6]
Why should the approach be    feasible (i.e., lead to a proof) 
even theoretically?
That is, in what sense is it fundamentally 
different from the  trivial, infeasible approach above, 
and not just a restatement of the original problem? 
\end{question}

This question is most natural and obvious
because,  in view of the universality 
of the $P \not =  NP$ conjecture, it has always been questioned right from
the begining  why it
should even be provable. For example,  why can it not be 
independent of the formal axioms of mathematics? This was studied 
in some early works; cf. \cite{aaronsonformal} for their  survey. It 
was also the 
motivation behind identifying  the fundamental 
barriers towards this problem,
such as the relativization \cite{solovay} and natural-proof 
\cite{rudich} barriers.
The latter barrier  roughly says that the proof techniques akin to
the ones used for proving the lower bounds for constant depth circuits
would not work for the $P$ vs. $NP$ problem
in a sense because the problem itself
stands in their way, rendering them theoretically infeasible, so to say.
Admittedly, such proof techniques constitute  only  a very specific 
subarea of mathematics, which is why this  barrier can be considered 
local,  and we cannot conclude anything about the proof techniques
which go through other areas of mathematics on the basis of such a local
barrier (for the reasons explained in more detail in Section~\ref{sexp}).
But one can still wonder if the $P$ vs. $NP$ problem could not
stand in the way of every proof technique like this, rendering it
theoretically infeasible, and thereby precluding its own proof. This
does not seem inconceivable since the problem itself says that the discovery
is hard, and so, why could it not make the discovery of its own proof hard?
Hence arises the question:
why should a given proof technique 
be even theoretically feasible, as per some 
reasonable notion of theoretical feasibility. 
The feasibility barrier is simply the task of answering this 
fundamental question, which has been lurking in the background of the $P$ vs.
$NP$ problem right from the begining.
It is universal in the sense that every approach has to answer
Question~\ref{qfeasible}, and
until it is answered clearly,
however sophisticated an approach may be, it cannot be
considered to be more than a  restatement of the original problem.

Now we have specify what is meant by answering
Question~\ref{qfeasible} clearly. For this,
the approach has to:
\begin{description}
\item[A] Come up with a new notion of obstruction (i.e. the cause
or proof-certificate of hardness as per that approach), which
is fundamentally different from the trivial obstruction, and thus 
precisely formulate the new Obstruction Hypothesis (OH), which says 
that such obstructions should exist when $m=\poly(n)$, and which provably 
implies the old IOH.

\item [B] Precisely formulate the notion of theoretical feasibility, 
and  justify why it is reasonable notion, i.e., why does a theoretically
feasible problem as per this notion means a problem that can be solved 
by a technique that is fundamentally better than the brute-force search.
\item [C] 
Justify on the basis of  concrete mathematical results 
why the problem (OH) of proving existence of  such obstructions
should  be considered theoretically feasible as per this notion
in contrast to the theoretically infeasible IOH.
One possible way to do this is by justifying why the problem of 
recognizing (verifying) an obstruction is 
theoretically feasible as per this notion. After all,  every 
approach is in a sense a search for obstructions. It is possible 
that the approach may seek 
to prove existence of obstructions by a nonconstructive 
method, without exhibiting any obstruction explicitly. But if it is not
theoretically feasible for the approach to even recognize (verify) 
what is searching for,
then there is a serious problem with the approach.
\item [D] Justify why it is plausible
that the task of proving OH should
become practically feasible once its theoretical feasibility is established.
One possible way is to prove concrete nontrivial lower bounds 
in weaker settings using the approach to demonstrate that theoretical
feasibility can lead to practical feasiblity in nontrivial cases.
\end{description}
By the feasibility barrier, we  mean the task of answering 
Question~\ref{qfeasible} in this manner. 

\section{The flip}
The most obvious and natural strategy for crossing the feasibility barrier
is suggested by the $P$ vs. $NP$ problem itself. For that, 
let us see what is wrong with the trivial obstruction from the 
complexity-theoretic point view. That is quite clear. First, it is long,
i.e.,  its description takes exponential space. Second, it is hard to
verify (and also construct); i.e., this  takes exponential time.
Since $NP$ is the class of problems with ``proof-certificates'' that 
are short (of polynomial-size) and easy to verify (in polynomial-time), 
this then leads to the following strategy for proving the nonuniform
$P\not = NP$ conjecture, with the obvious complexity-theoretic
interpretation of the phrase theoretically feasible.

\begin{figure} 
\begin{center}
\epsfig{file=trivialtonew.eps, scale=.6}
\end{center}
      \caption{From trivial to new obstruction}
      \label{fig:trivialtonew}
\end{figure} 


\noindent {\bf The flip  [GCT6,GCTflip]: Going for explicit construction}

\noindent {\bf I. (Theoretical feasibility of verification):}
Formulate a new notion of obstruction
(``proof-certificate of hardness'') that is {\em explicit}, by which 
we mean {\em short and easy-to-verify}: i.e., 
for any $n$ and $m< 2^n$, if there exists such an 
obstruction to efficient computation of $f(X)$ by circuits of size $m$,
then there also exists a short  obstruction with description of
$\poly(n)$ size bitlength, 
whose validity as an obstruction can be verified 
in $\poly(n)$ time.
This means that the problem of verifying (recognizing)
an obstruction belongs to $P$, 
and hence, is theoretically feasible (``easy'').

Intuitively (cf. Figure~\ref{fig:trivialtonew}), we can think of the new obstruction as an 
encryption of a some trivial obstruction of exponential
size which is highly compressable
in the information theoretic sense--i.e., such that 
its description can be encrypted in polynomial size--and furthermore,
such that the encrypted information can also be verified fast in polynomial
time.
At the surface, it is hard to believe that 
such an obstruction can even exist. To see why, let us note that 
the problem of  verifying 
if a given $X$ is a counterexample to a given $C$ is  intractable since 
it requires evaluating the NP-complete function $f(X)$, which cannot 
be done  efficiently assuming $P \not = NP$, and furthermore
$f_C(X)$ too cannot be evaluated  in polynomial time if the size $m$ of
$C$ is superpolynomial (say $n^{\log n}$). To verify the new obstruction,
in effect, we  are 
{\em implicitly} verifying   all exponentially many  rows of some 
trivial obstruction  in polynomial time (but without 
even knowing what that trivial obstruction is, since the verification 
procedure cannot affort to decrypt the new obstruction to get an exponential
size trivial obstruction).
It may seem that 
such a scheme could not possibly exist and that the $P \not = NP$ conjecture
would again stand in the way either directly or indirectly (implicitly).
Implementation of  this step of the flip
amounts to   showing that
the $P\not = NP$ conjecture
would not stand in the way--which is what crossing the feasibility barrier
essentially means.
Of course, the actual implementation 
does not have to  encrypt any trivial obstructions. The 
new obstruction could be such that its existence implies existence of
some trivial obstruction in a highly indirect way,
without actually telling how to get such a 
trivial obstruction from the new obstruction.
But if it is possble to do so
easily--i.e., if there is a polynomial time {\em decoding algorithm}, which
given a new obstruction and a small $C$ produces a counter example $X$ for 
$C$--then we say that the new obstruction is {\em easy to decode}. 
Though this is optional, at least at this stage, it may intuitively
help to imagine that the new obstructions are easy to decode.


\noindent {\bf II. (Theoretical feasibility of discovery) [optional]:} 
Give a $\poly(n)$  time algorithm for deciding,
for any given $n$ and $m< 2^n$,
if there exists such a new  obstruction, and constructing
one if one exists. This means the problem of discovering an obstruction
belongs to $P$, and hence, is theoretically feasible (``easy'').

\noindent {\bf III. (Practical feasibility):} 
Using the ``easy'' criterion for recognizing an obstruction 
in step I, prove:

\noindent {\bf OH (Obstruction Hypothesis):} If 
$m=\poly(n)$, then for every sufficiently large $n$, there exists 
such a short obstruction $O_n$. 

We call such an obstruction family $\{O_n\}$  {\em explicit}.


If we also have an ``easy'' procedure for discovering an obstruction 
in step II, then this amounts to  proving that this 
procedure always discovers and constructs
an obstruction $O_n$  successfully when $m=\poly(n)$--i.e., the discovery
procedure works correctly (successfully). So this step amount to 
proving correctness of the discovery program.
If it is correct, we 
call such an obstruction family $\{O_n\}$ {\em strongly explicit}.

We  call a proof of the $P\not = NP$ conjecture {\em explicit} if 
it is based on the flip and carries out the step I, and {\em strongly explicit}
if it carries out both steps I and II.


We  say that OH becomes {\em theoretically feasible}, as against
theoretically infeasible IOH, 
once the steps I and II have been carried out, 
since the associated problems of verifying and constructing an obstruction 
then belong to $P$; i.e., 
the theoretically infeasible task of proving IOH is transformed 
into a theoretically feasible task of proving OH.
Hence, the name of this stategy {\em the flip}:
from the infeasible to the feasible. 
We also say that the {\em feasibilty barrier for verification} 
is crossed once step I is carried out, and the {\em feasibility barrier
for discovery} is crossed once step II is carried out (these barriers
are referred to as the $P$ barriers for verification and discovery in
[GCTflip,GCT6]). We also say that the approach becomes {\em theoretically
feasible} once these two barriers are crossed.

Of course, theoretical 
feasibility of OH  does not automatically  imply that the task of 
actually proving it would be practically feasible.
For that, it is also necessary
that the algorithms for verifying and discovering an obstruction in
steps I and II have a simple enough structure that can be used for
proving OH in step III; i.e.,  for proving correctness of the discovery 
procedure. If not, they have to made simpler and simpler until
this becomes practically feasible.
Theoretical feasibility of the approach basically
means that the $P\not = NP$ conjecture  no longer stands in the way of the 
approach, and hence, there is no philosophical barrier to 
practical feasibility, though transforming  a theoretically
feasible  approach into a practically feasible approach  can be  a challenging
mathematical problem in itself.

Step II above  has been labelled optional, because
there may exist a  proof of the $P\not = NP$ conjecture
along the  lines of the flip  that  takes substantial
short cuts in this step.
For example,  a proof technique may simply be lucky and come 
up with a right guess for the obstruction family (since it is meant to be
carried out by humans and not machines). 
But substantial short cuts in step I seem difficult. After all, as we have
already said,  if the proof
technique cannot even recognize easily what it is searching for, then
there is  a serious problem.

The feasibility barrier and the flip for other problems are analogous.

The flip is the defining strategy of GCT. Indeed, GCT may be abstractly
defined as any (geometric) approach to the $P$ vs. $NP$ and related 
problems based on the flip, i.e., explicit construction of obstructions
(for a precise meaning of the phrase geometric see Section~\ref{scharsym}).



The present (concrete) GCT is one such  approach. It
proposes  a scheme for implementing the flip for the $P$ 
vs. $NP$ and related problems via algebraic geometry, representation
theory and the theory of quantum groups.
This turns out to be a massive affair, as to be expected, because of the
counterintuitive and paradoxical nature of the flip, as explained in 
the step I.
We focus here on characteristic zero. That is we only consider computations
performed by algebraic circuits, where each gate can perform an algebraic
operation of the underlying ring or field   of characteristic zero, 
say $Z$, $\Q$ or $\C$ \footnote{The characteristic zero version
of the $P$ vs. $NC$ obtained this way 
is not very interesting. The more nontrivial 
version solved in GCTlocal will be considered below.}. This is because
the nonuniform lower bounds over $Z$ are weaker implications of the
corresponding ones over a finite field (the usual case), and hence
easier. The additional problems that
need to be addressed when the underlying field of computation is finite
will be discussed in  GCT11. 



We now describe the   concrete lower bounds of GCT based on weaker
forms of the flip  and 
then briefly  the conjectural scheme  for  implementing the flip in
characteristic zero [GCT6,7,8] in general.

\section{The $P\not = NC$ result without bit operations}
We  begin with 
a  special case of the $P \not = NC$ conjecture [GCTlocal],
which we are calling the $P\not = NC$ result without bit operations,
and which can be considered to be the
first concrete lower bound result of GCT. It was  proved using a weaker
form of the flip much before the flip was formalized in [GCT6,GCTflip].
It  says that 
the $P$-complete max-flow problem
cannot be solved in $\polylog(N)$ parallel time using $\poly(N)$
processors in the PRAM model without bit operations,
where $N$ denotes
the total bit length of the input, not just the number of input parameters.
This model  is quite realistic and natural
since it includes virtually all known parallel algorithms for algebraic 
and weighted optimization problems.
The proof technique of this result can be considered to be {\em locally
explicit}, i.e.,  a weaker {\em local} form
of the flip,  in the sense that  for each branching program $C$  (i.e. 
a circuit with arithmetic, branching and comparison operations) 
of depth $\log^a N$ and size $\poly(N)$ (or even 
$2^{\log^a N}$, for some positive constant $a$),
it produces in $\log ^b N$ time using $2^{\log ^b N}$ 
processors, $b=O(a)$, 
an explicit   counter example  $X$ such that the output of $C$
on $X$ is different from what is expected in the maxflow (decision) problem.
This counter example $X$ is then a proof-certificate of hardness (obstruction)
against $C$.
We are calling this kind of explicitness local 
because the obstruction   here is
a short and easily-verifiable  proof 
certificate of hardness against a specific circuit   rather than 
a short and easily-verifiable {\em global obstruction} 
against  the
whole class of circuits of small depth and size, which is far harder to
achieve, and which was what the  flip (described earlier in this
introduction) eventually goes for in the context of the harder 
lower bound problems, and to which we shall also sometimes refer to as
the global flip for this reason. 

Local explicitness here  may seem counterintuitve at the surface,
since the max-flow problem
is $P$-complete, and hence, it may seem that we may not
even be able to verify if a given $X$ is a counter-example in 
polylogarithmic parallel time. In other words, it may seem that the
$P\not = NC$ conjecture may stand in the way of local explicitness,
just as the $P\not = NP$ conjecture seems to stand in the way
of the step I of the flip.
But local explicitness  is  possible,
because  the proof technique in
GCTlocal produces for a given $C$ an explicit 
counter example $X$ for which 
max-flow can be computed in polylogarithmic time
nevertheless. This   suggests that local 
explicitness ought to be similarly 
possible in the context of the $P$ vs. $NP$ problem
as well. In other words,
there ought to exist for this problem trivial obstructions, as in
Figure~\ref{fig:trivialtonew}, 
whose each row, specifying a counter example $X$ for a given $C$, can be
verified in $\poly(n,m)$ time, $m$ the size of $C$. That is, so
that $f(X)$ for this specific counterexample 
$X$  can be evaluated in polynomial time
in spite of  $NP$-completeness of $f(X)$ in general. Note that
$\poly(n,m)$ is $\poly(n)$ if $m=\poly(n)$.


\noindent {\em Remark}:
Local explicitness was not  specifically mentioned 
in GCTlocal. But it is easy to see \cite{GCTpramappend}  that 
the proof technique there actually
produces a locally
explicit proof certificate of hardness, after a little postprocessing,
though the goal was only
to prove its existence (which is why explicitness was not mentioned).
In other words, the proof technique essentially produces a locally
explicit proof-certificate of hardness  whether one cares for it or not.


Local explicitness of the proof technique is the fundamental difference between
this lower bound result and the earlier ones, such as 
the lower bounds for constant depth circuits \cite{sipser}, monotone circuits 
\cite{monotone}, or 
algebraic decision trees \cite{benor}, whose proof techniques are inherently 
nonconstructive. For example, the random restriction method \cite{sipser}
for proving lower bounds for  constant depth circuits gives a randomized 
fast parallel algorithm to produce  for each such
circuit $C$ a local counter example $X$ on which it differs from
the parity function. But the best determistic algorithm to produce 
such a counter example, based on  derandomization of the switching
lemma \cite{agarwal},
takes sequential polynomial time. Locally explicit in this
setting would mean computable by a constant depth circuit. Again, at the
surface this may seem counterintuitive, since it may appear that 
even to verify if a given $X$ is a counter example against a given
$C$ may necessarily
require $NC$-computation, given that parity is not in $AC^0$. 
But this should still be possible in view 
of the weak form of the $P\not = NC$ conjecture above. 
Similarly, the proof of the lower bound for sorting in
the  algebraic-decision-tree 
model \cite{benor}  inherently requires
exponential time  to produce a counter example, 
so also the proof of the lower bound for monotone circuits \cite{monotone}.
It may be conjectured that there are
(locally) explicit proofs 
for the constant-depth or  monotone circuit lower bounds. 
At present this is  open. But the main point is that such  explicit 
proofs are not  required to prove these lower bounds,
whereas,
the only way we can prove the weak form of the $P \not = NC$ conjecture
at present is essentially via locally explicit construction. 
In view of the natural proof barrier, it should not be surprising 
that the proof of  $P \not = NC$ result without bit operations  should
require something fundamentally different from the nonconstructive
techniques of the kind used to prove lower bounds for constant depth
circuits, to which this barrier applies,
though, admitedly,  this barrier itself does not suggest that 
we should go for anything explicit (cf. Section~\ref{sexp}).

Another  feature of the proof of this lower bound result  is that  it
is based on classical algebraic geometry, though 
the result itself can be stated in purely 
elementary and combinatorial terms.  No elementary or combinatorial 
proof of this result is known so far.
At present,  the $P\not = NC$ result without bit operations seems to be the
only known  special case of any
of the fundamental separation  problems in 
Figure~\ref{fig:complexityclasses} that  holds unconditionally (and 
superpolynomially) in a realistic and 
natural model of computation. That its  proof needs 
geometry and explicit construction   provides  the first
concrete  support for the
geometric approach based on the flip  (explicit construction), i.e. GCT, 
albeit only in the local setting, and
hence, in retrospect, we shall refer to its proof technique as {\em local GCT}.

But the local  GCT turns out to be too weak for going ahead 
for two reasons.
First, GCTlocal (towards the end of its Chapter 7) 
pointed out a barrier (other than the earlier natural-proof
and relativization barriers), which we shall 
refer to  as the {\em algebraic degree barrier}, though it was not
given any name there. This  says that 
any low-degree proof technique, such as the one there,
which associates with a computation algebraic 
objects (polynomials, varieties, etc.) 
and then reasons solely on the basis of the degrees of those 
objects would not work in the context of the fundamental problems 
such as the $P$ vs. $NC$ problem.
The recent  algebrization barrier \cite{aaronson}
also says  something similar, but with different  motivation and framework.
Second, as we already pointed out before, the obstructions in local GCT are 
short and easily-verifiable 
locally as against globally, i.e., the flip is local instead of global.
For reasons, which we do not understand, the local flip does not seem good
enough for the harder separation problems. 


GCTlocal also suggested an idea  for overcoming the
algebraic degree barrier and the locality limitation of local GCT:
namely, associate with complexity classes 
algebraic varieties with group action, as studied in geometric invariant theory
\cite{mumford}, which   intuitively 
capture the symmetries among the  computations in  that class,
and then reason globally on the basis of
the deeper representation theoretic structure of these
varieties, instead of just  their degrees.

\section{From local to global: new obstructions}
This then was the motivation behind the 
approach to the fundamental lower bound problems via geometric 
invariant theory that was initiated in GCT1 and 2. 
The focus here is on the 
characteristic zero versions of the other 
two problems in Figure~\ref{fig:complexityclasses}, namely
the $P$ vs. $NP$ and $\#P$ vs. $NC$ problems (weak GCT is too weak in
this context too). 
The nonuniform (characteristic zero) version of the $\#P$ vs. $NC$ problem
is also known as the permanent vs. determinant problem \cite{valiant}. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented 
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$. %; the best known lower bound on $m$ at present is 
%quadratic \cite{ressayre}.
By linear representation, we mean
the  entries   of $Y$ are  (possibly nonhomogeneous) 
linear functions 
of the entries of $X$. 
There is an analogous characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.
The main results of GCT for the $\#P$ vs. $NC$ problem in 
characteristic zero also extend to the $P$ vs. $NP$ problem in characteristic
zero. But for the sake of completeness,   we shall mainly
concentrate in this article 
on only the former problem, since it illustrates all the
basic ideas.


In GCT1, and 2  certain algebraic varieties with group action, 
called the {\em class varieties}, are associated with the fundamental 
complexity classes, and the $\#P$ vs. $NC$ and $P$ vs. $NP$ problems in
characteristic zero are reduced to showing existence of 
certain representation-theoretic {\em obstructions} to embeddings
amongs such varieties. Furthermore, some results in geometric invariant
theory are also proved to justify why such obstructions should exist 
in  the lower bound problems under consideration and
why they should be mathematically well behaved.

GCT 6 conjectures that these  new obstructions are (globally) explict; i.e., 
their specifications are easy to verify and a short obstruction
exists whenever an obstruction exists


\section{A mathematical form of the $\#P\not = NC$ conjecture}
Using  this notion of an obstruction and the geometric-invariant-theoretic
results in GCT1 and 2,  GCT6 (revised version) then proves a second concrete 
lower bound result of GCT, called a  {\em mathematical
weak form of the $\#P$ vs. $NC$ problem} in characteristic zero for the
reasons given below,
and verifies this conjecture in this special case.
This says  that for any generalized permanent of $k$
$n\times n$ variable matrices $X_1,\ldots,X_k$ 
cannot be represented as a polynomial in the traces of monomials in 
$\bar X^j$, $j\ge 0$, where 
$\bar X_i= B X_i C$, for all $i$,  for any (possibly singular) $n\times n$
complex 
matrices $B$ and $C$.
Here by a generalized permanent, we mean a function $p(X_1,\ldots,X_k)$ 
(of any degree not necessarily $n$)
which has exactly the same symmetries as that of the permanent: i.e., such
that for all nonsingular $n\times n$ complex matrices
$U$ and $V$, $p(U X_1 V,\ldots, U X_k V)=p(X_1,\ldots, X_k)$
iff $\perm(U X V)=\perm(X)$. 
It is called a {\em mathematical form} because there is no restriction here
on the complexity of the generalized permanent or the polynomial in traces.
In that sense, unlike the $P\not = NC$ result without bit operations,
this is a mathematical lower bound, rather than a 
complexity theoretic lower bound,  like the one in Galois 
theory which says that any general polynomial of degree greater than five
cannot be solved by any number of radical operations without any restriction
on the number of such operations.
The proof technique of this result 
produces a strongly explicit family $\{O_n\}$ of  (global) obstructions, 
where each $O_n$ has a specification of $O(n)$ size that can verified
and constructed in $O(n)$ time. The obstruction is global in the sense
that it is against all $B$, $C$ and polynomials in traces. 
Thus this result
provides a concrete support for the (global) flip. Its
proof technique  also  bypasses 
the natural-proof, relativization
and algebraic degree (algebrization) barriers 
simultaneously in this setting.


There is also a  nonconstructive 
proof of this result, which also bypasses these 
barriers.
It  is essentially the same as the
explicit proof, except for the last and the easiest step,
which can be carried out nonconstructively. 
Thus the situation here is again similar to the one for the
$P \not =NC$ result without bit operations. That is, the proof is such that 
it essentially (modulo a little postprocessing at the end) 
yields explicit proof certificates whether one cares for them or not.


To summarize the dicussion so far, the 
$P\not =NC$ result without bit operations in GCT is
a complexity theoretic lower bound proved using  a locally explicit  
technique, the mathematical form of the $\#P\not =NC$ conjecture is a 
mathematical lower bound  proved using a globally
explicit technique.
What is needed now to address 
the fundamental separation problems in Figure~\ref{fig:complexityclasses} 
following this line of investigation 
is  a global flip in this  complexity theoretic setting.
This is addressed next in characteristic zero.



\section{On the flip in general in characteristic zero}
The main result of GCT in this context is a conjectural scheme [GCT6,7,8] 
for explicit construction 
of obstructions (i.e. for the implementation of the global flip) 
for the general $\#P$ vs. $NC$ and $P$ vs. $NP$ 
problems in characteristic zero. 
Specifically, GCT6 shows that the feasibility barrier for verification
(and discovery) can be crossed for these problems assumming
a certain positivity hypothesis called PH1 (and its stronger form PH4).
PH1    says that 
certain  representation-theoretic counting  functions
associated with the class  varieties in GCT1 and 2 
have positive $(\#P)$  convex formulae.
By this we mean  positive convex
representations as the number of integer points in  explicitly 
specified polytopes, like the one for the permanent of a $0-1$-matrix 
as the number of integer points in the perfect matching polytope, which
is both positive (since each integer point is counted 
with a positive sign) and convex. 
Furthermore, GCT6,7,and 8   provide an evidence in support of validity
of PH1, and suggest  an approach for proving it via the theory of
nonstandard quantum groups, which are generalizations of
standard quantum groups \cite{drinfeld}. At the heart of this approach,
  lie certain conjectural positivity hypotheses [GCT8] in the theory
of these nonstandard quantum groups, which are  generalizations of the
known positivity results \cite{kazhdan,lusztig} for the standard quantum group.
The only known proofs of these positivity results are based  on the 
Riemann hypothesis over finite fields \cite{weil2}, which is
itself a profound  positivity result in mathematics. 
Thus the proposed scheme for explicit construction of obstructions 
in GCT6,7,8  seems to need  as yet unknown nonstandard
extension of the work surrounding this central positivity theorem,
which encompasses several areas of mathematics, such as algebraic geometry,
representation theory, quantum groups and so forth.

This should not be too surprising, given that 
the difficulty of explicit construction is by now well recognized 
in complexiy theory.
For example, the explicit construction of Ramanujan graphs \cite{sarnak},
which are the best (optimal) expanders,  also 
needs the Riemann hypothesis over finite fields (for curves).
But explicit expanders  cannot be used to prove a lower bound result.
Explicit constructions that yield hard lower bound results are bound
to be  more difficult. Hence, if a nontrivial  extension 
of the work surrounding the Riemann Hypothesis over finite fields 
is needed for explicit constructions in GCT, that is only to be expected.

\section{Is explicit construction necessary?} \label{sexp}
If explicit construction is thus the root cause of all difficulties in
GCT, one may finally ask: can it not be avoided somehow?
After all, for the original lower bound problems we only need to 
prove existence of some obstructions, and 
the flip is only the most obvious and natural way to cross
the feasibility barrier. There may exist  nonobvious and 
unnatural (e.g. nonconstructive) ways
to cross this barrier, perhaps several.
At present,  we only know 
that one class of nonconstructive techniques 
would not work, namely the ones with probabilistic flavour, which
are ruled out by the natural-proof-barrier \cite{rudich}. 
But the probabilistic  proofs constitute  only a 
small subarea of nonconstructive proofs, namely the ones 
which are of a  {\em nonspecific} kind, by which we mean nonconstructive
proofs which apply to most functions (or structures) under consideration.
Vast areas of
nonconstructive proofs in  mathematics, such as the ones  in algebraic 
geometry and representation theory, are of fundamentally different nature
than probabilistic proofs: they are nonconstructive yet very
{\em specific}; i.e., they  apply to only very specific functions or structures
under consideration. The natural-proof-barrier does not apply to
such  nonconstructive but specific proof techniques. 
Indeed, as we already pointed out above,
the generalized weak form of the $\#P\not = NC$ conjecture 
has a nonconstructive (but very specific)  proof (cf. Section~\ref{sweak})
which
applies to only the (generalized) permanent functions, and  
crosses (the analogues of)  the natural-proof, relativization,
algebraic-degree (algebrization) and feasibility
barriers  in this weak setting.
This gives a concrete evidence that
explicit constructions are  not needed to cross these barriers, and that
they may be crossed by nonconstructive proof techniques as well.

But the mathematical arguments  given in [GCT6,GCTflip]  suggest that 
such unnatural ways to cross the feasibility barrier
may be even harder than  the natural ways, as one may intuitively expect. 


\noindent {\em Remark:} The meaning 
of natural here (explicit)  is different from the one in \cite{rudich} 
(probabilistic). Whenever we say natural in the context of GCT, 
we always mean explicit.

The natural way  is also supported at a concrete level by the 
lower bounds of GCT discussed above.
After all, any approach to the $P$ vs. $NP$ and related problems has 
to yield at least:
\begin{enumerate} 
\item[A] Some weak form of any of the separation problems in
Figure~\ref{fig:complexityclasses}
that  gives
a concrete superpolynomial lower bound
in a realistic and natural model of computation, by which
we mean a model that is actually used in practice and is
not defined for the sake of the lower bound, and
\item[B] Some  weak form  of any of the separation problems in
Figure~\ref{fig:complexityclasses} whose 
proof technique bypasses 
the relativization, natural proof,  algebraic degree, and 
algebrization barriers simultaneously.
\end{enumerate}
The weak form of the $P\not = NC$ conjecture in GCT meets criterion (A),
and the generalized weak form of
the $\#P \not = NC$ conjecture meets criterion (B). 
These are the weak forms specific only to  this concrete form
of GCT. Other  approaches (GCT or nonGCT) may lead to other
comparable weak forms which are more suitable to them.
But, at present, these are the only such lower bounds that 
we can prove unconditionally in the context of the $P$ vs. $NP$, $P$ vs. $NC$
or $\#P$ vs. $NC$ problems, i.e., in the main testing ground 
shown in Figure~\ref{fig:complexityclasses} 
for  any approach.
And the only  way we can prove them at present 
is esentially (modulo some postprocessing at the end) 
via explicit constructions based on
geometry.  The situation is summarized in Figure~\ref{fig:summary}.
Here it can be
seen that as the circuit lower bounds start moving in the 
direction of the $P$ vs. $NP$ problem, the proof techniques, for some
mysterious reasons, become more and more geometric and explicit.
This sugests that there may be after all something inevitable 
about  geometry and   explicit constructions, 
which is what GCT means.

\begin{figure} 
\begin{center}
\psfragscanon
\psfrag{pvsnc}{$P\not = NC$}
\psfrag{#pvsnc}{$\#P\not = NC$}
\psfrag{pvsnp}{$P\not = NP$}
\epsfig{file=summary.eps, scale=1}
\end{center}
      \caption{Circuit lower bounds vs. proof techniques}
      \label{fig:summary}
\end{figure} 



The rest of this article is organized in the form of three chapters,
one per  lecture. The first gives a short overview of the basic plan
of GCT for implementing the flip (explicit constructions) in characteristic
zero, which is elaborated in the next two lectures. 






\noindent {\em Acknowledgement:} The author is grateful to 
Avi Wigderson for arranging the lectures and the hospitality in IAS.









==> preface3.tex <==
\begin{abstract}
Geometric complexity
theory (GCT) is an approach to the $P$ vs. $NP$ and related problems 
suggested in a series of  articles we call GCTlocal \cite{GCTpram},
GCT1-8 \cite{GCT1}-\cite{GCT8}, and GCTflip
\cite{GCTflip}.
A  high level overview of this reasearch plan and the results 
obtained so far  was presented  in 
a series of three lectures in the Institute of Advanced study, Princeton,
Feb 9-11, 2009.  This article contains the material covered in
those lectures after some revision, and gives an overview of GCT.
No background in algebraic geometry, representation theory
or quantum groups is assumed. 
For those who are interested in a short overview, the preface 
and the first chapter (lecture 1) of this article provide
such a short overview.
The video lectures for this series are available at \\
http://video.ias.edu/csdm/pvsnp \\
They  may be  a helpful supplement to  this article. 
\end{abstract}
\section*{Introduction} 
Geometric complexity
theory (GCT) is an approach to the  fundamental problems of
complexity theory, such as the (nonuniform) $P$ vs. $NP$
\cite{cook,karp,levin},
$P$ vs. $NC$ and $\#P$ vs. $NC$ \cite{valiant} problems
(Figure~\ref{fig:complexityclasses}). 
In this introduction, we  briefly describe  (1) the main barrier  
towards these problems called the {\em feasibility
barrier}, and  (2) the basic strategy of GCT for crossing it called 
the {\em flip} [GCT6,GCTflip], (3) the main result [GCT6] of GCT that 
says that this barrier, along with the earlier relativization \cite{solovay},
natural proof \cite{rudich}, algebraic degre [GCTlocal] and algebrization
\cite{aaronson} barriers,  can be crossed in characteristic zero, i.e.,
when the underlying field of computation is of characteristic zero 
as explained  below (cf.  [GCT11] for general fields), and (4) 
two concrete lower bounds 
of GCT based on weaker forms of the flip: namely
the  $P \not = NC$ result without bit operations [GCTlocal] and
a mathematical  form of the $\#P\not = NC$ conjecture in characteristic
zero [GCT1,2,6] (which
does not have a naturalizable \cite{rudich} proof unlike its
its weak form in the original IAS lecture which  turned out to be too weak
\cite{boris}).

\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes (no proper containments are known)}
      \label{fig:complexityclasses}
\end{figure} 



The feasiblity   barrier was not explicitly described  in 
the original lectures. But 
all the mathematical effort in   GCT as described in these lectures 
in a sense goes towards crossing this barrier.
Hence, we wish
to describe  it explicitly here so that the fundamental difficulty that
GCT is trying to overcome
and the need for the nonelementary techniques that enter into GCT to 
deal with it  would be clear at a high level before we 
get into any mathematics. 









\section{The feasibility barrier and the flip} 
This barrier is {\em universal} in 
the sense that it has to be crossed by every approach towards the $P$ vs. 
$NP$ problem, not just GCT, regardless of which areas of mathematics it goes
through. In contrast, the other known barriers 
such as the relativization \cite{solovay}, natural-proof \cite{rudich},
algebraic-degree [GCTlocal],  and algebrization  \cite{aaronson} barriers
are {\em local} in the
sense that they are only applicable to specific areas of mathematical
techniques and hence can  be bypassed, as in GCT. 
In other words, a local barrier is like a guiding post which tells 
us what must not be done, and hence must  be bypassed,  whereas 
a universal barrier cannot be bypassed no matter what, because it tells us
what must be done, i.e., it has to be crossed.
Due its universality, the feasibility barrier
captures the root cause of all the 
difficulties in the $P$ vs. $NP$ and related  problems, and it turns 
out to quiet formidable, as expected. 

Before we describe it, let us  remark  that the 
presence of such a universal barrier should not be surprising,
because the $P \not = NP$ conjecture    is itself a {\em universal} statement
regarding all of mathematics. Namely, 
if this conjecture fails to hold,
every theorem in mathematics that has a proof of reasonable 
length  can be proved  efficiently by a computer in 
time polynomial in the length of its shortest proof. No other known
conjecture in mathematics has such stunning mathematical sweep. 
Given the universal nature of this problem, it then stands to reason that
the main  barrier towards this problem--the root cause of its 
difficulty--should also be
{\em universal}. The feasibility barrier is this universal barrier.
Due to its universal nature, it 
cannot be  fully formalized like the local barriers, because any barrier
that can be fully formalized would tend to be local. But since it is the 
root cause of the difficulty of the $P$ vs. $NP$ problem, 
we wish to  state it as clearly as possible. 

Towards that end,  let us 
fix an appropriate $NP$-complete function $f(X)=f(x_1,\ldots,x_n)$. 
The goal of the nonuniform $P$ vs. $NP$ problem  is to show that 
there does not exist a circuit $C=C(X)$ of size 
$m=\poly(n)$  that computes $f(X)$, $n\rightarrow \infty$. 
Symbolically, let  $f_C(X)$ denote the function computed by $C$. 
Then we want to prove that
\begin{equation} \label{eqiohp}
\forall n, m=\poly(n) \ \forall C \exists x : f(X)\not = f_C(X). 
\end{equation}

Equivalently, the goal is to prove:

\noindent {\bf (IOH)}: For every large enough $n$, and $m=\poly(n)$,
there  exists a {\em trivial obstruction
(i.e. a ``proof-certificate'' of hardness)} to efficient computation of
$f(X)$. Here by a trivial obstruction we mean
a table (cf. Figure~\ref{fig:trivialtonew}) that lists for every small 
$C$  a counterexample  $X$ such that $f(X)\not = f_C(X)$.



The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$.
Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. 
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time to decide if such a table exists for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. So
we call  this trivial, brute force 
strategy of proving the nonuniform $P$ vs. $NP$ conjecture,
based on existence of trivial obstructions,  a {\em theoretically
infeasible strategy}. Also because
it is really just a restatement of the original problem.
Hence, the terminology  IOH (Infeasible Obstruction Hypothesis)--we also
call it {\em theoretically infeasible}. 


Any approach to the  $P$ vs. $NP$ problem has to 
answer the following question: 

\begin{question} \label{qfeasible} {\bf (Feasibility Barrier)} [GCTflip,GCT6]
Why should the approach be    feasible (i.e., lead to a proof) 
even theoretically?
That is, in what sense is it fundamentally 
different from the  trivial, infeasible approach above, 
and not just a restatement of the original problem? 
\end{question}

This question is most natural and obvious
because,  in view of the universality 
of the $P \not =  NP$ conjecture, it has always been questioned right from
the begining  why it
should even be provable. For example,  why can it not be 
independent of the formal axioms of mathematics? This was studied 
in some early works; cf. \cite{aaronsonformal} for their  survey. It 
was also the 
motivation behind identifying  the fundamental 
barriers towards this problem,
such as the relativization \cite{solovay} and natural-proof 
\cite{rudich} barriers.
The latter barrier  roughly says that the proof techniques akin to
the ones used for proving the lower bounds for constant depth circuits
would not work for the $P$ vs. $NP$ problem
in a sense because the problem itself
stands in their way, rendering them theoretically infeasible, so to say.
Admittedly, such proof techniques constitute  only  a very specific 
subarea of mathematics, which is why this  barrier can be considered 
local,  and we cannot conclude anything about the proof techniques
which go through other areas of mathematics on the basis of such a local
barrier (for the reasons explained in more detail in Section~\ref{sexp}).
But one can still wonder if the $P$ vs. $NP$ problem could not
stand in the way of every proof technique like this, rendering it
theoretically infeasible, and thereby precluding its own proof. This
does not seem inconceivable since the problem itself says that the discovery
is hard, and so, why could it not make the discovery of its own proof hard?
Hence arises the question:
why should a given proof technique 
be even theoretically feasible, as per some 
reasonable notion of theoretical feasibility. 
The feasibility barrier is simply the task of answering this 
fundamental question, which has been lurking in the background of the $P$ vs.
$NP$ problem right from the begining.
It is universal in the sense that every approach has to answer
Question~\ref{qfeasible}, and
until it is answered clearly,
however sophisticated an approach may be, it cannot be
considered to be more than a  restatement of the original problem.

Now we have specify what is meant by answering
Question~\ref{qfeasible} clearly. Let us assume that the approach
is nonuniform, i.e., it shows existence of some obstruction $O_n$
(the cause
or proof-certificate of hardness as per that approach) for every $n$,
since the relativization barrier \cite{solovay} 
suggests that uniform approaches 
may have a fundamental limitation in the context of the $P$ vs. $NP$ problem.
If there exists a nonrelativizable uniform approach, we
leave the task of answering Question~\ref{qfeasible} to that approach. 
To answer Question~\ref{qfeasible}, 
a nonuniform approach has to:
\begin{description}
\item[A] Come up with a new notion of obstruction, which
is fundamentally different from the trivial obstruction, and thus 
precisely formulate the new Obstruction Hypothesis (OH), which says 
that such obstructions should exist when $m=\poly(n)$, and which provably 
implies the old IOH.

\item [B] Precisely formulate the notion of theoretical feasibility, 
and  justify why it is reasonable notion, i.e., why does a theoretically
feasible problem as per this notion means a problem that can be solved 
by a technique that is fundamentally better than the brute-force search.
\item [C] 
Justify on the basis of  concrete mathematical results 
why the problem (OH) of proving existence of  such obstructions
should  be considered theoretically feasible as per this notion
in contrast to the theoretically infeasible IOH.
One possible way to do this is by justifying why the problem of 
recognizing (verifying) an obstruction is 
theoretically feasible as per this notion. After all,  every 
approach is in a sense a search for obstructions. It is possible 
that the approach may seek 
to prove existence of obstructions by a nonconstructive 
method, without exhibiting any obstruction explicitly. But if it is not
theoretically feasible for the approach to even recognize (verify) 
what is searching for,
then there is a serious problem with the approach.
\item [D] Justify why it is plausible
that the task of proving OH should
become practically feasible once its theoretical feasibility is established.
One possible way is to prove concrete nontrivial lower bounds 
in weaker settings using the approach to demonstrate that theoretical
feasibility can lead to practical feasiblity in nontrivial cases.
\end{description}
By the feasibility barrier, we  mean the task of answering 
Question~\ref{qfeasible} in this manner. 

\section{The flip}
The most obvious and natural strategy for crossing the feasibility barrier
is suggested by the $P$ vs. $NP$ problem itself. For that, 
let us see what is wrong with the trivial obstruction from the 
complexity-theoretic point view. That is quite clear. First, it is long,
i.e.,  its description takes exponential space. Second, it is hard to
verify (and also construct); i.e., this  takes exponential time.
Since $NP$ is the class of problems with ``proof-certificates'' that 
are short (of polynomial-size) and easy to verify (in polynomial-time), 
this then leads to the following strategy for proving the nonuniform
$P\not = NP$ conjecture, with the obvious complexity-theoretic
interpretation of the phrase theoretically feasible.

\begin{figure} 
\begin{center}
\epsfig{file=trivialtonew.eps, scale=.6}
\end{center}
      \caption{From trivial to new obstruction}
      \label{fig:trivialtonew}
\end{figure} 


\noindent {\bf The flip  [GCT6,GCTflip]: Going for explicit construction}

\noindent {\bf I. (Theoretical feasibility of verification):}
Formulate a new notion of obstruction
(``proof-certificate of hardness'') that is {\em explicit}, by which 
we mean {\em short and easy-to-verify}: i.e., 
for any $n$ and $m< 2^n$, if there exists such an 
obstruction to efficient computation of $f(X)$ by circuits of size $m$,
then there also exists a short  obstruction with description of
$\poly(n)$ size bitlength, 
whose validity as an obstruction can be verified 
in $\poly(n)$ time.
This means that the problem of verifying (recognizing)
an obstruction belongs to $P$, 
and hence, is theoretically feasible (``easy'').
Furthemore, the approach should also provide mathematical evidence
to justify  why such  obstructions should exist when $m$ is small.


Intuitively (cf. Figure~\ref{fig:trivialtonew}), we can think of the
new obstruction as an 
encryption of a some trivial obstruction of exponential
size which is highly compressable
in the information theoretic sense--i.e., such that 
its description can be encrypted in polynomial size--and furthermore,
such that the encrypted information can also be verified fast in polynomial
time.
At the surface, it is hard to believe that 
such an obstruction can even exist. To see why, let us note that 
the problem of  verifying 
if a given $X$ is a counterexample to a given $C$ is  intractable since 
it requires evaluating the NP-complete function $f(X)$, which cannot 
be done  efficiently assuming $P \not = NP$, and furthermore
$f_C(X)$ too cannot be evaluated  in polynomial time if the size $m$ of
$C$ is superpolynomial (say $n^{\log n}$). To verify the new obstruction,
in effect, we  are 
{\em implicitly} verifying   all exponentially many  rows of some 
trivial obstruction  in polynomial time (but without 
even knowing what that trivial obstruction is, since the verification 
procedure cannot affort to decrypt the new obstruction to get an exponential
size trivial obstruction).
It may seem that 
such a scheme could not possibly exist and that the $P \not = NP$ conjecture
would again stand in the way either directly or indirectly (implicitly).
Implementation of  this step of the flip
amounts to   showing that
the $P\not = NP$ conjecture
would not stand in the way--which is what crossing the feasibility barrier
essentially means.
Of course, the actual implementation 
does not have to  encrypt any trivial obstructions. The 
new obstruction could be such that its existence implies existence of
some trivial obstruction in a highly indirect way,
without actually telling how to get such a 
trivial obstruction from the new obstruction.
But if it is possble to do so
easily--i.e., if there is a polynomial time {\em decoding algorithm}, which
given a new obstruction and a small $C$ of size $m$ 
produces in $\poly(n,m)$ time a counter example $X$ for 
$C$--then we say that the new obstruction is {\em easy to decode}. 
We shall say that the trivial obstruction produced by such a decoding
algorithm--i.e. the table that gives for each $C$ the counter example
$X$ produced by the decoding algorithm--is locally explicit.
In other words, a {\em a locally explicit   obstruction} 
is a table specifying a counter example for each circuit 
whose each row can be verified in $\poly(n,m)$ time. 
Though decoding is optional, at least at this stage, it may intuitively
help to imagine that the new obstructions are easy to decode
and correspond to some locally explicit  obstructions.


\noindent {\bf II. (Theoretical feasibility of discovery) [optional]:} 
Give a $\poly(n)$  time algorithm for deciding,
for any given $n$ and $m< 2^n$,
if there exists such a new  obstruction, and constructing
one if one exists. This means the problem of discovering an obstruction
belongs to $P$, and hence, is theoretically feasible (``easy'').



\noindent {\bf III. (Practical feasibility):} 
Using the ``easy'' criterion for recognizing an obstruction 
in step I, prove:

\noindent {\bf OH (Obstruction Hypothesis):} If 
$m=\poly(n)$, then for every sufficiently large $n$, there exists 
such a short obstruction $O_n$. 

We call such an obstruction family $\{O_n\}$  {\em explicit}.


If we also have an ``easy'' procedure for discovering an obstruction 
in step II, then this amounts to  proving that this 
procedure always discovers and constructs
an obstruction $O_n$  successfully when $m=\poly(n)$--i.e., the discovery
procedure works correctly (successfully). So this step amount to 
proving correctness of the discovery program.
If it is correct, we 
call such an obstruction family $\{O_n\}$ {\em strongly explicit}.

We  call a proof of the $P\not = NP$ conjecture {\em explicit} if 
it is based on the flip and carries out the step I, and {\em strongly explicit}
if it carries out both steps I and II.


%Thus once the steps I and II have been carried out, 
%the associated problems of verifying and discovering  an obstruction 
%belong to $P$, and hence, become theoretically feasible.


We  say that the {\em feasibilty barrier for verification} 
is crossed if the step I can be  carried out assuming only
{\em theoretical feasible mathematical hypotheses} supported 
by mathematical evidence.
By a theoretically feasible  hypothesis, we mean  that
it is not based on
any hard complexity-theoretic assumption that is
equivalent to or harder than the original $P \not = NP$ conjecture, and that
there is a good justification for why
the $P\not = NP$ conjecture should not stand in the way of its
proof.  By mathematical, we mean 
it should hold for all  n
and $m$ without any restriction on $m$ (as long as it is $<2^n$) unlike 
the original  $P\not = NP$ conjecture, where 
$m$ has to be  a small function of $n$ for it to hold, and 
this smallness of $m$ with respect to $n$ is the complexity theoretic
heart of the problem.
We similarly say that 
the {\em feasibility barrier
for discovery} is crossed once the step II is carried out assuming only
theoretical feasible mathematical hypotheses supported by mathematical
evidence. 
We say that the  {\em feasibility barrier is crossed}
once the feasibility barriers for verification and discovery  are crossed. 
We  say that  OH
becomes a {\em theoretically
feasible complexity-theoretic hypothesis}
once the feasibility barrier is crossed, because
then the tasks  of verifying and discovering an obstruction become
theoretically feasible in the complexity theoretic sense (i.e. belong to $P$)
assuming the theoretically feasible
mathematical hypotheses that arise in steps I and II.
It is called complexity theoretic, because  it is necessary
that $m$ be a small function of $n$ for it to hold (just as in the $P\not = NP$
conjecture).
We also say that the approach becomes theoretically feasible once 
OH becomes theoretically feasible like this.
Hence, the name of this stategy {\em the flip}:
from the infeasible (IOH) to the feasible (OH). 


To summarize, an approach becomes theoretically feasible and the feasibilty 
barrier is crossed once it can be justified  that the $P\not = NP$ conjecture
no longer stands in the way of 
the approach; i.e., in the way of proving the basic hypotheses of the approach.



Of course, theoretical 
feasibility of the complexity theoretic 
OH  does not automatically  imply that the task of 
actually proving it would be practically feasible.
For that, it is also necessary
that the algorithms for verifying and discovering an obstruction in
steps I and II have a simple enough structure that can be used for
proving OH in step III; i.e.,  for proving correctness of the discovery 
procedure. If not, they have to made simpler and simpler until
this becomes practically feasible.
Similarly, theoretical feasibility of the mathematical hypotheses 
that arise in the implementation of the steps I and II does not 
guarantee that the mathematical task of proving them 
would be practically feasible.
%because this may require overcoming formidable mathematical
%difficulties.





Theoretical feasibility of an  approach only 
means that the $P\not = NP$ conjecture  no longer stands in its way,
and hence, there is no philosophical barrier to its
practical feasibility, though transforming  a theoretically
feasible  approach into a practically feasible approach  can be  
an immensely  formidable mathematical challenge. Hence it is to
be stressed  that there is a huge gap between theoretical feasibility
and practical feasibility. Furthermore, theoretical feasibility can
be separated from practical feasibility like this only for the
$P$ vs. $NP$ problem because of its universality. For other 
mathematical problems, e.g. Riemann hypothesis, only practical 
feasibility is the issue. Because however hard they may be, they do not
say that discovery is hard.




Step II above  has been labelled optional, because
there may exist a  proof of the $P\not = NP$ conjecture
along the  lines of the flip  that  takes substantial
short cuts in this step.
For example,  a proof technique may simply be lucky and come 
up with a right guess for the obstruction family (since it is meant to be
carried out by humans and not machines). 
But substantial short cuts in step I seem difficult. After all, as we have
already said,  if the proof
technique cannot even recognize easily what it is searching for, then
there is  a serious problem.



The feasibility barrier and the flip for other problems such as 
the $P$ vs. $NC$ and $\#P$ vs. $NC$ problems are analogous.
Though these problems  are not formally universal, 
we  assume that the feasibility barrier is 
meaningful for them  because we look at them as  brothers and sisters
of the $P$ vs. $NP$ problem.

The flip described so far  is {\em global} in the sense 
that it explicitly produces a (global) obstruction of $\poly(n)$ size 
that acts as a proof certificate of hardness for all small
circuits. We may also consider a  {\local flip}
which produces for every small circuit $C$ of size $m$ a 
counter example $X$ in $\poly(n,m)$ time; i.e., 
gives an algorithm for producing   a locally explicit 
obstruction. The local flip  crosses the  feasibility 
barrier {\em locally} in the sense that a 
locally explicit  obstruction is fundamentally different and better 
than a trivial obstruction. Better locally but not  globally
because  verification of the whole locally explicit obstruction still
takes exponential time.
The global flip is intuitively stronger than the local flip in
the sense that from a  global obstruction one can get 
a locally explicit  obstruction once we have 
a polynomial time decoding algorithm (as we are intuitively imagining)
and  the $P\not = NP$ conjecture does 
not stand in the way of this decoding.
Hence intuively we will always assume that the global flip subsumes 
the local flip.
As we shall see below (Section~\ref{swithoutbit}),
the local flip can be used to prove some restricted lower bounds.
But we can not make it work in the context of the harder problems of 
complexity theory.



The flip is the defining strategy of GCT. Indeed, GCT may be abstractly
defined as any (geometric) approach to the $P$ vs. $NP$ and related 
problems based on the flip, i.e., explicit construction of obstructions
(for a precise meaning of the phrase geometric see Section~\ref{scharsym}).
The present (concrete) GCT is one such  approach.


\section{Is explicit construction necessary?} \label{sexp}
But before we describe the concrete results of this GCT, 
let us explain  
why we are going for the flip, i.e., for explicit constructions,
in the first place.
After all, to solve  the  lower bound problems under consideration
we only need to prove existence of some obstructions, and 
the flip is only the most obvious and natural way to cross
the feasibility barrier. There may exist  nonobvious and 
unnatural (e.g. nonconstructive) ways
to cross this barrier, perhaps several.
At present,  we only know 
that one class of nonconstructive techniques 
would not work, namely the ones with probabilistic flavour, which
are ruled out by the natural-proof-barrier \cite{rudich}. 
But the probabilistic  proofs constitute  only a 
small subarea of nonconstructive proofs, namely the ones 
which are of a  {\em nonspecific} kind, by which we mean nonconstructive
proofs which apply to most functions (or structures) under consideration.
Vast areas of
nonconstructive proofs in  mathematics, such as the ones  in algebraic 
geometry and representation theory, are of fundamentally different nature
than probabilistic proofs: they are nonconstructive yet 
{\em very specific};
i.e., they  apply to only very specific functions or structures
under consideration. The natural-proof-barrier does not apply to
such  nonconstructive but specific proof techniques. 
Indeed, one of the concrete lower bounds of GCT to be discussed below
(Section~\ref{}) has a nonconstructive   proof
which applies to only very specific (permanent-like) functions and which 
crosses (the analogues of)  the natural-proof, relativization,
algebraic-degree (algebrization) and feasibility
barriers  in a restricted   setting.
This gives a concrete evidence that
explicit constructions are  not needed to cross these barriers, and that
they may be crossed by nonconstructive proof techniques as well.

But the mathematical evidence and arguments 
in [GCTflip] sugggest that such unnatural ways to cross the feasibility barrier
may be even harder than  the natural ways, as one may intuitively expect. 
We do not go into  these arguments here. At a concrete level, 
all we can say is that we are going the natural way, because there 
is no other concrete alternative.
After all, any approach to the $P$ vs. $NP$ problem has 
to provide  at least:
\begin{enumerate} 
\item[A] Concrete evidence for its theoretical feasibility; i.e., 
concrete evidence  which says  that the feasibility barrier can be
crossed in that approach. 
\item[B] Unconditional proof of a 
weaker form  of the $P$ vs. $NP$ problem or any of its two smaller
versions--namely 
the   $P$ vs. $NC$ or the $\#P$ vs. $NC$ problem
(cf. Figure~\ref{fig:complexityclasses})--that  gives
a concrete superpolynomial lower bound
in a realistic and natural model of computation, by which
we mean a model that is actually used in practice and is
not defined for the sake of the lower bound, and
\item[C] Unconditional proof of some  weaker form  of
any of the separation problems above  whose 
proof technique simultaneously bypasses the earlier 
relativization, natural proof,  algebraic degree, and 
algebrization barriers in complexity theory.
\end{enumerate}

We will say that an approach is {\concrete} if it meets the criteria 
A, B and C above.

The main result [GCT6] of GCT, which  says that the feasibility barrier 
can be crossed in characteristic zero (GCT11 says the same over any field),
addresses  (A). The
$P \not NC$ result without bit operations [GCTlocal] addresses (B).
The mathematical form of the $\#P\not = NC$ conjecture addresses (C).
Thus one may now say that GCT is a concrete approach to the $P$ vs. $NP$ 
problem.

At present,  there is a no concrete alternative to GCT
which addresses A, B and C. Finally, this is why we are going for the flip,
for the lack of any  other concrete alternative.










The weak form of the $P\not = NC$ conjecture in GCT meets criterion (A),
and the generalized weak form of
the $\#P \not = NC$ conjecture meets criterion (B). 
These are the weak forms specific only to  this concrete form
of GCT. Other  approaches (GCT or nonGCT) may lead to other
comparable weak forms which are more suitable to them.
But, at present, these are the only such lower bounds that 
we can prove unconditionally in the context of the $P$ vs. $NP$, $P$ vs. $NC$
or $\#P$ vs. $NC$ problems, i.e., in the main testing ground 
shown in Figure~\ref{fig:complexityclasses} 
for  any approach.
And the only  way we can prove them at present 
is esentially (modulo some postprocessing at the end) 
via explicit constructions based on
geometry.  The situation is summarized in Figure~\ref{fig:summary}.
Here it can be
seen that as the circuit lower bounds start moving in the 
direction of the $P$ vs. $NP$ problem, the proof techniques, for some
mysterious reasons, become more and more geometric and explicit.
This sugests that there may be after all something inevitable 
about  geometry and   explicit constructions, 
which is what GCT means.

And the concrete results of GCT mentioned above shows that this
obvious natural way is effective. We cannot get any such 
comparable results in any other way. That is finally the only reason
we are going this way because this 











It
proposes  a scheme for implementing the flip for the $P$ 
vs. $NP$ and related problems via algebraic geometry, representation
theory and the theory of quantum groups.
This turns out to be a massive affair, as to be expected, because of the
counterintuitive and paradoxical nature of the flip as explained in 
the step I.
We focus in this article  on characteristic zero. 
That is we only consider computations
performed by algebraic circuits, where each gate can perform an algebraic
operation of the underlying ring or field   of characteristic zero, 
say $Z$, $\Q$ or $\C$ \footnote{The characteristic zero version
of the $P$ vs. $NC$ obtained this way 
is not very interesting. The more nontrivial 
version solved in GCTlocal will be considered below.}. This is because
the nonuniform lower bounds over $Z$ are weaker implications of the
corresponding ones over a finite field (the usual case), and hence
easier. The additional problems that
need to be addressed when the underlying field of computation is finite
will be discussed in  GCT11. 

The nonuniform (characteristic zero) version of the $\#P$ vs. $NC$ problem
is also known as the permanent vs. determinant problem \cite{valiant}. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented 
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$. %; the best known lower bound on $m$ at present is 
%quadratic \cite{ressayre}.
By linear representation, we mean
the  entries   of $Y$ are  (possibly nonhomogeneous) 
linear functions 
of the entries of $X$. 
There is an analogous characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.
The main results of GCT for the $\#P$ vs. $NC$ problem in 
characteristic zero also extend to the $P$ vs. $NP$ problem in characteristic
zero. But for the sake of completeness,   we shall mainly
concentrate in this article 
on only the former problem, since it illustrates all the
basic ideas.









We next  describe briefly the   concrete lower bounds of GCT based on weaker
forms of the flip [GCTlocal,GCT1,2,6],
the  geometric notion of obstructions introduced in
[GCT1,2], the main result [GCT6]  of GCT that says that
the feasibility barrier can be crossed for the $P$ vs. $NP$ and $\#P$ vs.
$NC$ problems in characteristic zero using these geometric obstructions,
and an approach  [GCT7,8] to proving the theoretically
feasible mathematical hypotheses that arise during the crossing 
of this barrier.








\section{The $P\not = NC$ result without bit operations} \label{swithoutbit}
We  begin with 
a  special case of the $P \not = NC$ conjecture [GCTlocal],
which we are calling the $P\not = NC$ result without bit operations,
and which can be considered to be the
first concrete lower bound result of GCT. It was  proved using the weaker
local form of the flip much before the (global) flip was formalized
in [GCT6,GCTflip].
It  says that 
the $P$-complete max-flow problem
cannot be solved in $\polylog(N)$ parallel time using $\poly(N)$
processors in the PRAM model without bit operations,
where $N$ denotes
the total bit length of the input, not just the number of input parameters.
This model  is quite realistic and natural
since it includes virtually all known parallel algorithms for algebraic 
and weighted optimization problems.
The proof technique of this result can be considered to be {\em locally
explicit}, i.e.,  the weaker {\em local} form
of the flip,  in the sense that  for each branching program $C$  (i.e. 
a circuit with arithmetic, branching and comparison operations) 
of depth $\log^a N$ and size $\poly(N)$ (or even 
$2^{\log^a N}$, for some positive constant $a$),
it produces in $\log ^b N$ time using $2^{\log ^b N}$ 
processors, $b=O(a)$, 
an explicit   counter example  $X$ such that the output of $C$
on $X$ is different from what is expected in the maxflow (decision) problem.
This counter example $X$ is then a proof-certificate of hardness (obstruction)
against $C$.
We are calling this kind of explicitness local 
because the obstruction   here is
a short and easily-verifiable  proof 
certificate of hardness against a specific circuit   rather than 
a short and easily-verifiable {\em global obstruction} 
against  the
whole class of circuits of small depth and size, which is far harder to
achieve, and which was what the  (global) flip (described earlier in this
introduction) eventually goes for in the context of the harder 
lower bound problems.

Local explicitness here  may seem counterintuitve at the surface,
since the max-flow problem
is $P$-complete, and hence, it may seem that we may not
even be able to verify if a given $X$ is a counter-example in 
polylogarithmic parallel time. In other words, it may seem that the
$P\not = NC$ conjecture may stand in the way of local explicitness,
just as the $P\not = NP$ conjecture seems to stand in the way
of the step I of the flip.
But local explicitness  is  possible,
because  the proof technique in
GCTlocal produces for a given $C$ an explicit 
counter example $X$ for which 
max-flow can be computed in polylogarithmic time
nevertheless. This  provides a concrete evidence as to why
locally explicit trivial obstructions (Figure~\ref{fig:trivialtonew}) 
should also exist in the context of the $P$ vs. $NP$ problem.
Intuitively, it would specify for a given $C$ of size $m$ 
a counter example $X$ such that $f(X)$ can be evaluated on this specific 
$X$ in $\poly(n,m)$  time in spite of 
$NP$-completeness of $f(X)$ in general ($\poly(n,m)$
is $\poly(n)$ if $m=\poly(n)$).
Thus GCTlocal crosses the  feasibility barrier locally
in the context of the $P\not = NC$ problem without bit operations and 
provides a concrete evidence for the feasibility of 
the  local flip in the context of the fundamental problems of complexity
theory.

\noindent {\em Remark}:
Local explicitness was not  specifically mentioned 
in GCTlocal. But it is easy to see \cite{GCTpramappend}  that 
the proof technique there actually
produces a locally
explicit proof certificate of hardness, after a little postprocessing,
though the goal was only
to prove its existence (which is why explicitness was not mentioned).
In other words, the proof technique essentially produces a locally
explicit proof-certificate of hardness  whether one cares for it or not.


Local explicitness of the proof technique is the fundamental difference between
this lower bound result and the earlier ones, such as 
the lower bounds for constant depth circuits \cite{sipser}, monotone circuits 
\cite{monotone}, or 
algebraic decision trees \cite{benor}, whose proof techniques are inherently 
nonconstructive. For example, the random restriction method \cite{sipser}
for proving lower bounds for  constant depth circuits gives a randomized 
fast parallel algorithm to produce  for each such
circuit $C$ a local counter example $X$ on which it differs from
the parity function. But the best determistic algorithm to produce 
such a counter example, based on  derandomization of the switching
lemma \cite{agarwal},
takes sequential polynomial time. Locally explicit in this
setting would mean computable by a constant depth circuit. Again, at the
surface this may seem counterintuitive, since it may appear that 
even to verify if a given $X$ is a counter example against a given
$C$ may necessarily
require $NC$-computation, given that parity is not in $AC^0$. 
But this should still be possible in view 
of the weak form of the $P\not = NC$ conjecture above. 
Similarly, the proof of the lower bound for sorting in
the  algebraic-decision-tree 
model \cite{benor}  inherently requires
exponential time  to produce a counter example, 
so also the proof of the lower bound for monotone circuits \cite{monotone}.
It may be conjectured that there are
(locally) explicit proofs 
for the constant-depth or  monotone circuit lower bounds. 
At present this is  open. But the main point is that such  explicit 
proofs are not  required to prove these lower bounds,
whereas,
the only way we can prove the weak form of the $P \not = NC$ conjecture
at present is essentially via locally explicit construction. 
In view of the natural proof barrier, it should not be surprising 
that the proof of  $P \not = NC$ result without bit operations  should
require something fundamentally different from the nonconstructive
techniques of the kind used to prove lower bounds for constant depth
circuits, to which this barrier applies,
though, admitedly,  this barrier itself does not suggest that 
we should go for anything explicit (cf. Section~\ref{sexp}).
One may say that 
the proof technique of this result bypasses this barrier
in the sense that such locally explicit construction can be
carried out only for very special problems in $P$ 
such as the max flow problem, though this barrier cannot be
formally defined in the PRAM model without bit operations.
One may also say that the proof technique
bypasses the relativization barrier \cite{rudich}
since it is known that this barrier is not effective against the
proof techniques which algebrize computations.
Thus GCTlocal crosses/bypasses
the local feasibility, natural proof and  relativization
barriers simultaneously in a restricted setting. 






Another  feature of the proof of this lower bound result  is that  it
is based on classical algebraic geometry, though 
the result itself can be stated in purely 
elementary and combinatorial terms.  No elementary or combinatorial 
proof of this result is known so far.
At present,  the $P\not = NC$ result without bit operations seems to be the
only known  special case of any
of the fundamental separation  problems in 
Figure~\ref{fig:complexityclasses} that  holds unconditionally (and 
superpolynomially) in a realistic and 
natural model of computation. That its  proof needs 
geometry and explicit construction   provides  the first
concrete  support for the
geometric approach based on the flip  (explicit construction), i.e. GCT, 
albeit only in the local setting, and
hence, in retrospect, we shall refer to its proof technique as {\em local GCT}.

But the local  GCT turns out to be too weak for going ahead 
for two reasons.
First, GCTlocal (towards the end of its Chapter 7) 
pointed out a barrier (other than the earlier natural-proof
and relativization barriers), which we shall 
refer to  as the {\em algebraic degree barrier}, though it was not
given any name there. This  says that 
any low-degree proof technique, such as the one there,
which associates with a computation algebraic 
objects (polynomials, varieties, etc.) 
and then reasons solely on the basis of the degrees of those 
objects would not work in the context of the fundamental problems 
such as the $P$ vs. $NC$ problem.
The recent  algebrization barrier \cite{aaronson}
also says  something similar, but with different  motivation and framework.
Second, as we already pointed out before, 
the local flip does not seems good enough for the harder separation problems
for the reasons that we do not understand. 


GCTlocal also suggested an idea  for overcoming the
algebraic degree barrier and the locality limitation of local GCT:
namely, associate with complexity classes 
algebraic varieties with group action, as studied in geometric invariant theory
\cite{mumford}, which   intuitively 
capture the symmetries among the  computations in  that class,
and then reason globally on the basis of
the deeper representation theoretic structure of these
varieties, instead of just  their degrees.

\section{Geometric obstructions}
This then was the motivation behind the 
approach to the fundamental lower bound problems via geometric 
invariant theory that was initiated in GCT1 and 2. 


In GCT1, and 2  certain algebraic varieties with group action, 
called the {\em class varieties}, are associated with the fundamental 
complexity classes, and the $\#P$ vs. $NC$ and $P$ vs. $NP$ problems in
characteristic zero are reduced to showing existence of 
certain representation-theoretic {\em obstructions} to embeddings
amongs such varieties. Furthermore, some results in geometric invariant
theory are also proved to justify why such obstructions should exist 
in  the lower bound problems under consideration and
why they should be mathematically well behaved.

GCT 6 conjectures that these  new obstructions are (globally) explict; i.e., 
their specifications are easy to verify and a short obstruction
exists whenever an obstruction exists


\section{A mathematical form of the $\#P\not = NC$ conjecture}
Using  this notion of an obstruction and the geometric-invariant-theoretic
results in GCT1 and 2,  GCT6 (revised version) then proves a second concrete 
lower bound result of GCT, called a  {\em mathematical
weak form of the $\#P$ vs. $NC$ problem} in characteristic zero for the
reasons given below,
and verifies this conjecture in this special case.
This says  that for any generalized permanent of $k$
$n\times n$ variable matrices $X_1,\ldots,X_k$ 
cannot be represented as a polynomial in the traces of monomials in 
$\bar X^j$, $j\ge 0$, where 
$\bar X_i= B X_i C$, for all $i$,  for any (possibly singular) $n\times n$
complex 
matrices $B$ and $C$.
Here by a generalized permanent, we mean a function $p(X_1,\ldots,X_k)$ 
(of any degree not necessarily $n$)
which has exactly the same symmetries as that of the permanent: i.e., such
that for all nonsingular $n\times n$ complex matrices
$U$ and $V$, $p(U X_1 V,\ldots, U X_k V)=p(X_1,\ldots, X_k)$
iff $\perm(U X V)=\perm(X)$. 
It is called a {\em mathematical form} because there is no restriction here
on the complexity of the generalized permanent or the polynomial in traces.
In that sense, unlike the $P\not = NC$ result without bit operations,
this is a mathematical lower bound, rather than a 
complexity theoretic lower bound,  like the one in Galois 
theory which says that any general polynomial of degree greater than five
cannot be solved by any number of radical operations without any restriction
on the number of such operations.
The proof technique of this result 
produces a strongly explicit family $\{O_n\}$ of  (global) obstructions, 
where each $O_n$ has a specification of $O(n)$ size that can verified
and constructed in $O(n)$ time. The obstruction is global in the sense
that it is against all $B$, $C$ and polynomials in traces. 
Thus this result
provides a concrete support for the (global) flip. Its
proof technique  also  bypasses 
the natural-proof, relativization
and algebraic degree (algebrization) barriers 
simultaneously in this setting.


There is also a  nonconstructive 
proof of this result, which also bypasses these 
barriers.
It  is essentially the same as the
explicit proof, except for the last and the easiest step,
which can be carried out nonconstructively. 
Thus the situation here is again similar to the one for the
$P \not =NC$ result without bit operations. That is, the proof is such that 
it essentially (modulo a little postprocessing at the end) 
yields explicit proof certificates whether one cares for them or not.


To summarize the dicussion so far, the 
$P\not =NC$ result without bit operations in GCT is
a complexity theoretic lower bound proved using  a locally explicit  
technique, the mathematical form of the $\#P\not =NC$ conjecture is a 
mathematical lower bound  proved using a globally
explicit technique.
What is needed now to address 
the fundamental separation problems in Figure~\ref{fig:complexityclasses} 
following this line of investigation 
is  a global flip in this  complexity theoretic setting.
This is addressed next in characteristic zero.



\section{On the flip in general in characteristic zero}
The main result of GCT in this context is a conjectural scheme [GCT6,7,8] 
for explicit construction 
of obstructions (i.e. for the implementation of the global flip) 
for the general $\#P$ vs. $NC$ and $P$ vs. $NP$ 
problems in characteristic zero. 
Specifically, GCT6 shows that the feasibility barrier for verification
(and discovery) can be crossed for these problems assumming
a certain positivity hypothesis called PH1 (and its stronger form PH4).
PH1    says that 
certain  representation-theoretic counting  functions
associated with the class  varieties in GCT1 and 2 
have positive $(\#P)$  convex formulae.
By this we mean  positive convex
representations as the number of integer points in  explicitly 
specified polytopes, like the one for the permanent of a $0-1$-matrix 
as the number of integer points in the perfect matching polytope, which
is both positive (since each integer point is counted 
with a positive sign) and convex. 
Furthermore, GCT6,7,and 8   provide an evidence in support of validity
of PH1, and suggest  an approach for proving it via the theory of
nonstandard quantum groups, which are generalizations of
standard quantum groups \cite{drinfeld}. At the heart of this approach,
  lie certain conjectural positivity hypotheses [GCT8] in the theory
of these nonstandard quantum groups, which are  generalizations of the
known positivity results \cite{kazhdan,lusztig} for the standard quantum group.
The only known proofs of these positivity results are based  on the 
Riemann hypothesis over finite fields \cite{weil2}, which is
itself a profound  positivity result in mathematics. 
Thus the proposed scheme for explicit construction of obstructions 
in GCT6,7,8  seems to need  as yet unknown nonstandard
extension of the work surrounding this central positivity theorem,
which encompasses several areas of mathematics, such as algebraic geometry,
representation theory, quantum groups and so forth.

This should not be too surprising, given that 
the difficulty of explicit construction is by now well recognized 
in complexiy theory.
For example, the explicit construction of Ramanujan graphs \cite{sarnak},
which are the best (optimal) expanders,  also 
needs the Riemann hypothesis over finite fields (for curves).
But explicit expanders  cannot be used to prove a lower bound result.
Explicit constructions that yield hard lower bound results are bound
to be  more difficult. Hence, if a nontrivial  extension 
of the work surrounding the Riemann Hypothesis over finite fields 
is needed for explicit constructions in GCT, that is only to be expected.


If explicit construction is thus the root cause of all difficulties in
GCT, one may finally ask: can it not be avoided somehow?

\begin{figure} 
\begin{center}
\psfragscanon
\psfrag{pvsnc}{$P\not = NC$}
\psfrag{#pvsnc}{$\#P\not = NC$}
\psfrag{pvsnp}{$P\not = NP$}
\epsfig{file=summary.eps, scale=1}
\end{center}
      \caption{Circuit lower bounds vs. proof techniques}
      \label{fig:summary}
\end{figure} 



The rest of this article is organized in the form of three chapters,
one per  lecture. The first gives a short overview of the basic plan
of GCT for implementing the flip (explicit constructions) in characteristic
zero, which is elaborated in the next two lectures. 






\noindent {\em Acknowledgement:} The author is grateful to 
Avi Wigderson for arranging the lectures and the hospitality in IAS.









==> preface4.tex <==
\section*{Introduction} 
Geometric complexity
theory (GCT) is an approach to the  fundamental problems of
complexity theory, such as the (nonuniform) $P$ vs. $NP$
\cite{cook,karp,levin},
$P$ vs. $NC$ and $\#P$ vs. $NC$ \cite{valiant} problems
(Figure~\ref{fig:complexityclasses}). 
In this introduction, we  briefly describe  the main barrier  
towards these problems called the {\em   feasibility
barrier},    the basic strategy of GCT for crossing it called 
the {\em flip} [GCT6,GCTflip],  
a conjectural scheme  [GCT6,7,8,11] for implementation of the flip, 
and two concrete lower bounds of GCT based on weaker forms of the flip: namely
the  $P \not = NC$ result without bit operations [GCTlocal] and
a mathematical  form of the $\#P\not = NC$ conjecture [GCT1,2,6].

The original IAS lectures did not state the first lower bound and
only stated   a special case of the second 
lower bound, called  the weak form of the $\#P$ vs.
$NC$ problem. The article \cite{boris} showed that this weak form 
is too weak; i.e., it can be proved    by an elementary  technique
that  cannot cross the natural-proof barrier \cite{rudich}.
We cannot prove the full mathematical form stated here by such
technique; cf. Sections~\ref{}, \ref{} and \ref{}. 



\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes (no proper containments are known)}
      \label{fig:complexityclasses}
\end{figure} 


The original lectures also did not describe the 
the  feasiblity   barrier.
But all the mathematical effort in   GCT as described in these lectures 
goes towards crossing this barrier.
Hence, we describe  it explicitly here so that the root cause of 
all difficulties encountered in GCT and the need for nonelementary techniques
to overcome this formidable barrier
becomes clear  at a high level before we get into any mathematics. 


\section{The  feasibility barrier} 
The  feasibility barrier is {\em universal} in 
the sense that it has to be crossed by every approach towards the $P$ vs. 
$NP$ problem, not just GCT, regardless of which areas of mathematics it goes
through. In contrast, the other known barriers 
such as the relativization \cite{solovay}, natural-proof \cite{rudich},
algebraic-degree [GCTlocal],  and algebrization  \cite{aaronson} barriers
are {\em local} in the
sense that they are only applicable to specific areas of mathematical
techniques and hence can simply  be bypassed, as in GCT. 
In other words, a local barrier is like a guiding post which tells 
us what must not be done, and hence must  be bypassed,  whereas 
a universal barrier cannot be bypassed no matter what, because it tells us
what must be done, i.e., it has to be crossed.
Due its universality, the feasibility barrier
captures the root cause of all the 
difficulties in the $P$ vs. $NP$ and related  problems, and it turns 
out to quiet formidable, as expected. 

Before we describe it, let us  remark  that the 
presence of such a universal barrier should not be surprising,
because the $P \not = NP$ conjecture    is itself a {\em universal} statement
regarding all of mathematics. Namely, 
if this conjecture fails to hold,
every theorem in mathematics that has a proof of reasonable 
length  can be proved  efficiently by a computer in 
time polynomial in the length of its shortest proof. No other known
conjecture in mathematics has such stunning mathematical sweep. 
Given the universal nature of this problem, it then stands to reason that
the main  barrier towards this problem--the root cause of its 
difficulty--should also be
{\em universal}. The  feasibility barrier is this universal barrier.
Due to its universal nature, it 
cannot be  fully formalized like the local barriers, because any barrier
that can be fully formalized would tend to be local.  But since it is the 
root cause of the difficulty of the $P$ vs. $NP$ problem, 
we wish to  state it as clearly as possible. 

Towards that end,  let us 
fix an appropriate $NP$-complete function $f(X)=f(x_1,\ldots,x_n)$. 
The goal of the nonuniform $P$ vs. $NP$ problem  is to show that 
there does not exist a circuit $C=C(X)$ of size 
$m=\poly(n)$  that computes $f(X)$, $n\rightarrow \infty$. 
Symbolically, let  $f_C(X)$ denote the function computed by $C$. 
Then we want to prove that
\begin{equation} \label{eqiohp}
\forall n, m=\poly(n) \ \forall C \exists x : f(X)\not = f_C(X). 
\end{equation}

Equivalently, the goal is to prove:

\noindent {\bf (IOH)}: For every large enough $n$, and $m=\poly(n)$,
there  exists a {\em trivial obstruction
(i.e. a ``proof-certificate'' of hardness)} to efficient computation of
$f(X)$. Here by a trivial obstruction we mean
a table (cf. Figure~\ref{fig:trivialtonew}) that lists for every small 
$C$  a counterexample  $X$ such that $f(X)\not = f_C(X)$.



The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$.
Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. 
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time to decide if such a table exists for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. So
we call  this trivial, brute force 
strategy of proving the nonuniform $P$ vs. $NP$ conjecture,
based on existence of trivial obstructions,  a {\em theoretically
infeasible strategy}. Also because
it is really just a restatement of the original problem.
Hence, the terminology  IOH (Infeasible Obstruction Hypothesis)--we also
call it {\em theoretically infeasible}. 


Any approach to the  $P$ vs. $NP$ problem has to 
answer the following question: 

\begin{question} \label{qfeasible} {\bf (Theoretical Feasibility Barrier)} 
[GCTflip,GCT6]
Why should the approach be    feasible (i.e., lead to a proof) 
even theoretically?
That is, in what sense is it fundamentally 
different from the  trivial, infeasible approach above, 
and not just a restatement of the original problem? 
\end{question}

This question is  natural and not new, 
because,  in view of the universality 
of the $P \not =  NP$ conjecture, it has always been questioned right from
the begining  why it
should even be provable. For example,  why can it not be 
independent of the formal axioms of mathematics? This was studied 
in some early works; cf. \cite{aaronsonformal} for their  survey. It 
was also the 
motivation behind identifying  the fundamental 
barriers towards this problem,
such as the relativization \cite{solovay} and natural-proof 
\cite{rudich} barriers.
The latter barrier  roughly says that the proof techniques akin to
the ones used for proving the lower bounds for constant depth circuits
would not work for the $P$ vs. $NP$ problem
in a sense because the problem itself
stands in their way, rendering them theoretically infeasible, so to say.
Admittedly, such proof techniques constitute  only  a very specific 
subarea of mathematics, which is why this  barrier can be considered 
local,  and we cannot conclude anything about the proof techniques
which go through other areas of mathematics on the basis of such a local
barrier (for the reasons explained in more detail in Section~\ref{sexp}).
But one can still wonder if the $P$ vs. $NP$ problem could not
stand in the way of every proof technique like this, rendering it
theoretically infeasible, and thereby precluding its own proof. This
does not seem inconceivable since the problem itself says that the discovery
is hard, and so, why could it not make the discovery of its own proof hard?
Hence arises the question:
why should a given proof technique 
be even theoretically feasible as per some 
reasonable notion of theoretical feasibility. 
The feasibility barrier is simply the task of answering this 
fundamental question, which has been lurking in the background of the $P$ vs.
$NP$ problem right from the begining.
It is universal in the sense that every approach has to answer
Question~\ref{qfeasible}, and
until it is answered clearly,
however sophisticated an approach may be, it cannot be
considered to be more than a  restatement of the original problem.

Now we have specify what is meant by answering
Question~\ref{qfeasible} clearly. Let us assume that the approach
is nonuniform, i.e., it shows existence of some obstruction $O_n$
(the cause
or proof-certificate of hardness as per that approach) for every $n$,
since the relativization barrier \cite{solovay} 
suggests that uniform approaches 
may have a fundamental limitation in the context of the $P$ vs. $NP$ problem.
If there exists a nonrelativizable uniform approach, we
leave the task of answering Question~\ref{qfeasible} to that approach. 
To answer Question~\ref{qfeasible}, 
a nonuniform approach has to:
\begin{description}
\item[A] Come up with a new notion of obstruction, which
is fundamentally different from the trivial obstruction, and thus 
precisely formulate the new Obstruction Hypothesis (OH), which says 
that such obstructions should exist when $m=\poly(n)$, and which provably 
implies the old IOH.

\item [B] Precisely formulate the notion of theoretical feasibility, 
and  justify why it is reasonable notion, i.e., why does a theoretically
feasible problem as per this notion means a problem that can be solved 
by a technique that is fundamentally better than the brute-force search.
\item [C] 
Justify on the basis of  concrete mathematical results 
why the problem (OH) of proving existence of  such obstructions
should  be considered theoretically feasible as per this notion
in contrast to the theoretically infeasible IOH.
One possible way to do this is by justifying why the problem of 
recognizing (verifying) an obstruction is 
theoretically feasible as per this notion. After all,  every 
approach is in a sense a search for obstructions. It is possible 
that the approach may seek 
to prove existence of obstructions by a nonconstructive 
method, without exhibiting any obstruction explicitly. But if it is not
theoretically feasible for the approach to even recognize (verify) 
what is searching for,
then there is a serious problem with the approach.
\item [D] Justify why it is plausible
that the task of proving OH should
become practically feasible once its theoretical feasibility is established.
One possible way is to prove concrete nontrivial lower bounds 
in weaker settings using the approach to demonstrate that theoretical
feasibility can lead to practical feasiblity in nontrivial cases.
\end{description}
By the feasibility barrier, we  mean the task of answering 
Question~\ref{qfeasible} in this manner. 

\section{The flip: going for explicit construction}
The most obvious and natural strategy for crossing the feasibility barrier
is suggested by the $P$ vs. $NP$ problem itself. For that, 
let us see what is wrong with the trivial obstruction from the 
complexity-theoretic point view. That is quite clear. First, it is long,
i.e.,  its description takes exponential space. Second, it is hard to
verify (and also construct); i.e., this  takes exponential time.
Since $NP$ is the class of problems with ``proof-certificates'' that 
are short (of polynomial-size) and easy to verify (in polynomial-time), 
this then leads to the following strategy, called the {\em flip}
[GCT6,GCTflip],
for proving the nonuniform
$P\not = NP$ conjecture, with the obvious complexity-theoretic
interpretation of the phrase theoretically feasible.

\begin{figure} 
\begin{center}
\epsfig{file=trivialtonew.eps, scale=.6}
\end{center}
      \caption{From trivial to new obstruction}
      \label{fig:trivialtonew}
\end{figure} 


\noindent {\bf I. (The flip: theoretical feasibility of verification) :}
Formulate a new notion of obstruction
(``proof-certificate of hardness'') that is {\em explicit}, by which 
we mean {\em short and easy-to-verify}: i.e., 
for any $n$ and $m< 2^n$, if there exists such an 
obstruction to efficient computation of $f(X)$ by circuits of size $m$,
then there also exists a short  obstruction with description of
$\poly(n)$ size bitlength, 
whose validity as an obstruction can be verified 
in $\poly(n)$ time.
This means that the problem of verifying (recognizing)
an obstruction belongs to $P$, 
and hence, is theoretically feasible (``easy'').
Furthemore, the approach should also provide mathematical evidence
to justify  why such  obstructions should exist when $m$ is small.


Intuitively (cf. Figure~\ref{fig:trivialtonew}), we can think of the
new obstruction as an 
encryption of a some trivial obstruction of exponential
size which is highly compressable
in the information theoretic sense--i.e., such that 
its description can be encrypted in polynomial size--and furthermore,
such that the encrypted information can also be verified fast in polynomial
time.
At the surface, it is hard to believe that 
such an obstruction can even exist. To see why, let us note that 
the problem of  verifying 
if a given $X$ is a counterexample to a given $C$ is  intractable since 
it requires evaluating the NP-complete function $f(X)$, which cannot 
be done  efficiently assuming $P \not = NP$, and furthermore
$f_C(X)$ too cannot be evaluated  in polynomial time if the size $m$ of
$C$ is superpolynomial (say $n^{\log n}$). To verify the new obstruction,
in effect, we  are 
{\em implicitly} verifying   all exponentially many  rows of some 
trivial obstruction  in polynomial time (but without 
even knowing what that trivial obstruction is, since the verification 
procedure cannot affort to decrypt the new obstruction to get an exponential
size trivial obstruction).
It may seem that 
such a scheme could not possibly exist and that the $P \not = NP$ conjecture
would again stand in the way either directly or indirectly (implicitly).
Implementation of  this step of the flip
amounts to   showing that
the $P\not = NP$ conjecture
would not stand in the way--which is what crossing the feasibility barrier
essentially means.
Of course, the actual implementation 
does not have to  encrypt any trivial obstructions. The 
new obstruction could be such that its existence implies existence of
some trivial obstruction in a highly indirect way,
without actually telling how to get such a 
trivial obstruction from the new obstruction.
But if it is possble to do so
easily--i.e., if there is a polynomial time {\em decoding algorithm}, which
given a new obstruction and a small $C$ of size $m$ 
produces in $\poly(n,m)$ time a counter example $X$ for 
$C$--then we say that the new obstruction is {\em easy to decode}. 
Though this  is optional, at least at this stage, it may intuitively
help to imagine that the new obstructions are easy to decode.
and correspond to some locally explicit  obstructions.


\noindent {\bf II. (The strong flip: theoretical feasibility of discovery) 
[optional]:} 
Give a $\poly(n)$  time algorithm for deciding,
for any given $n$ and $m< 2^n$,
if there exists such a new  obstruction, and constructing
one if one exists. This means the problem of discovering an obstruction
belongs to $P$, and hence, is theoretically feasible (``easy'').
Again the $P\not = NP$ conjecture seems to stand in the 
way of this step, because the conjecture  says discovery is hard, whereas 
this step says  discovery (of its own proof) is easy. 




\noindent {\bf III. (Practical feasibility):} 
Using the ``easy'' criterion for recognizing an obstruction 
in step I, prove:

\noindent {\bf OH (Obstruction Hypothesis):} If 
$m=\poly(n)$, then for every sufficiently large $n$, there exists 
such a short obstruction $O_n$. 

We call such an obstruction family $\{O_n\}$  {\em explicit}.


If we also have an ``easy'' procedure for discovering an obstruction 
in step II, then this amounts to  proving that this 
procedure always discovers and constructs
an obstruction $O_n$  successfully when $m=\poly(n)$--i.e., the discovery
procedure works correctly (successfully). So this step amount to 
proving correctness of the discovery program.
If it is correct, we 
call such an obstruction family $\{O_n\}$ {\em strongly explicit}.

We  call a proof of the $P\not = NP$ conjecture {\em explicit} if 
it is based on the flip and carries out the step I, and {\em strongly explicit}
if it carries out both steps I and II.





We  say that the {\em feasibilty barrier for verification} 
is crossed if the step I can be  carried out assuming only
{\em theoretical feasible mathematical  hypotheses} supported 
by mathematical evidence.
By a theoretically feasible  mathematical hypothesis, we mean  that
it is not based on
any hard complexity-theoretic assumption that is
equivalent to or harder than the original $P \not = NP$ conjecture, that
it can be justified why 
the  $P\not = NP$ conjecture should  not stand in the way of its proof,
and that it holds for all  n
and $m$ without any restriction on $m$ (as long as it is $<2^n$) unlike 
the original  $P\not = NP$ conjecture, where 
$m$ has to be  a small function of $n$ for it to hold, and 
this smallness of $m$ with respect to $n$ is the main complexity theoretic
difficulty of the problem (which is gone in the mathematical hypothesis)
We  say that 
the {\em feasibility barrier
for discovery} is crossed once the step II can be carried out assuming only
theoretically feasible mathematical  hypotheses supported by mathematical
evidence. 
We say that the  {\em feasibility barrier is crossed}
once the feasibility barriers for verification and discovery  are crossed. 
We  say that  OH
becomes a {\em theoretically feasible complexity-theoretic hypothesis} 
once the feasibility barrier is crossed, because
then the tasks  of verifying and discovering an obstruction become
theoretically feasible (i.e., belong to $P$)
assuming the 
theoretically feasible  mathematical hypotheses that arise in steps I and II.
It is called complexity-theoretic because $m$ has to be a small function
of $n$ for it to hold just like in the original IOH.
We also say that the approach becomes theoretically feasible once 
the feasibility barrier is crossed; i.e., once 
the theoretically infeasible IOH is transformed into a theoretically feasible
OH. Hence, the name of this stategy {\em the flip}:
from the infeasible (IOH) to the feasible (OH). 



For another way to look at the flip (cf. Figure~\ref{fig:IOHcomplexityintro})
let us reexamine IOH. 
For given $X$ and $C$ of $\poly(n)$ size, the problem 
of deciding if  $\f(X) \not = f_C(X)$
belongs to co-$NP$.
Since there are two alternating layers of quantifiers in (\ref{}),
the problem of verifying it belongs to $\Pi_3$, 
which is  high in the complexity hierarchy
(cf. Figure~\ref{fig:IOHcomplexityintro}), and this is another reason for
referring to IOH as theoretically infeasible.
Of course, IOH is expected to 
be a tautology, and hence is expected to  be verifiable in $O(1)$ time--but
we do not know that as yet. 
After execution of the local flip, the problem of verifying OH
belongs to $\Pi_2$, since the condition $f(X)\not = f_C(X)$ for
a locally explicit obstruction can then be verified in polynomial time.
After execution of the step I of the (global) flip, the problem
of verifying OH belongs to $NP$, and after the step II to $P$.
Once this final $P$-verifiable OH is proved, it is reduced to a tautology
(FOH: Final Obstruction Hypothesis), which can be verified in 
$O(1)$ time. This gives us the final $O(1)$-size proof.
Thus the basic idea of the flip is to systematically 
eliminate the quantifiers  with the help of theoretically feasible 
mathematical hypotheses and reduce the complexity 
of the  obstruction hypothesis until it is finally
reduced to  an $O(1)$-time verifiable  tautology;
cf. Figure~\ref{fig:IOHcomplexityintro}. 

But this extremely simple strategy is also deeply paradoxical because 
assuming that the polynomial time hierachy does not collapse--or more 
specifically that $\Pi_3 \not = Pi_2 \not = NP \not = P$--it may seem
impossible   to reduce a universal $\Pi_3$ statement 
to a universal $\Pi_2$ statement  all the way  to a universal
$P$-statement and then to a tautology, where by a universal statement
we mean a statement about all of mathematics which every
statement under consideration here is
(since it would imply the universal $P \not = NP$ conjecture).
That is, as the flip starts moving from IOH towards its final 
destination FOH through the polynomial time hierachy as shown
in Figure~\ref{},  it seems as if  it may bring about a collapse of this 
hierarchy in its wake  thereby disproving the very conjectures 
it is meant to prove.   Hence the  feasiblity barrier is
self-referential barrier that says 
the main  barrier towards the $P$ vs. $NP$ problem is the problem itself.
An approach becomes theoretically feasible and this
barrier is crossed once it can be justified  that the $P\not = NP$ conjecture
no longer stands in its way; i.e.,  it is no longer a barrier to 
practical feasibility (of proving the basic hypotheses) of the approach.


Theoretical feasibility (of elimination
of the quantifying variables in IOH)
is a fundamental  issue  that 
can be separated from practical feasibility  in the context of  the
$P$ vs. $NP$ problem only 
because of its universality.
For mathematical problems which are not universal, theoretical feasibility
can be  meaningless.
For example, consider 
a trivial  assertion: 

\[ \forall x_1 \ldots x_n  \exists y_1 \ldots y_n: 
\ \sum_i x_i  + \sum_i y_i = \sum y_i + \sum_i x_i.
\]
The problem of brute force verification of this assertion 
belongs to $\Pi_2$, though that does not say anything about the 
difficulty of the problem. 
Indeed, it is well known
in proof theory that the logical complexity of an assertion, i.e., the
number of alternating quantifiers in it, is in general no index of its
mathematical difficulty. 
Hence for mathematical
problems that are not universal, e.g. the Riemann hypothesis,  practical 
feasibility is all that matters. Because however hard they may be, they do not
say that discovery is hard. 



Of course, theoretical 
feasibility of OH  does not automatically  imply that the task of 
actually proving it would be practically feasible.
For that, it is also necessary
that the polynomial time
algorithms for verifying and discovering an obstruction in
steps I and II have a simple enough structure that can be used for
proving OH in step III; i.e.,  for proving correctness of the discovery 
procedure. If not, they have to made simpler and simpler until
this becomes practically feasible.
Similarly, theoretical feasibility of the mathematical hypotheses 
that arise in the implementation of the steps I and II does not 
guarantee that the mathematical task of proving them 
would be practically feasible.


In other words,
there is a huge difference  between 
theoretical feasibility and practical feasibility. 
Theoretical feasibility of an  approach only 
says that there is no  philosophical barrier to its
practical feasibility, though transforming  a theoretically
feasible  approach into a practically feasible approach  can be  
an immensely  formidable mathematical task.   
Crossing  of the feasibility  barrier basically
exchanges hard complexity theory  with  hard mathematics.
What is gained in this exchange is that the $P$ vs. $NP$ problem does not
stand in the way of this hard  mathematics.

Step II above  has been labelled optional, because
there may exist a  proof of the $P\not = NP$ conjecture
along the  lines of the flip  that  takes substantial
short cuts in this step.
For example,  a proof technique may simply be lucky and come 
up with a right guess for the obstruction family (since it is meant to be
carried out by humans and not machines). 
But substantial short cuts in step I seem difficult. After all, as we have
already said,  if the proof
technique cannot even recognize easily what it is searching for, then
there is  a serious problem.

The flip above  is {\em global} because it is 
based on a global  obstruction of $\poly(n)$ size 
that acts as a proof certificate of hardness for all small
circuits. We may also consider a  {\em local  (strong) flip}
based on a {\em local (strongly) explicit 
obstruction}, by which we mean .
a table specifying a counter example $X$ for each small circuit $C$ of size 
$m$ whose each row can be verified (constructed) in $\poly(n,m)$ time. 
It may be conjectured that the local strong flip is possible in 
the context of the $P$ vs. $NP$ problem: i.e. for
any $NP$-complete $f(X)$, there exists an algorithm that 
produces a counter example $X$ for 
any circuit  $C$ of $m=\poly(n)$ size in $\poly(n,m)=\poly(n)$ time. 
We shall refer to this as the {\em local strong flip conjecture} for
the $P$ vs. $NP$ problem--it is evidently much stronger than the nonuniform
$P\not = NP$ conjecture.
The local flip  crosses the  feasibility 
barrier {\em locally} in the sense that a 
locally  explicit  obstruction is fundamentally different and better 
than a trivial obstruction. Better locally but not  globally
because  verification 
of the whole locally   explicit obstruction still
takes exponential time. Similarly for a local strongly explicit obstruction.
The global   flip is intuitively stronger than the local  flip in
the sense that from a  global  obstruction one can get 
a local   explicit  obstruction once we have 
a polynomial time decoding algorithm (as we are intuitively imagining)
and  the $P\not = NP$ conjecture does 
not stand in the way of this decoding.
Hence intuively the global (strong) flip subsumes the local (strong) flip.




The feasibility barrier and the flip for other problems such as 
the $P$ vs. $NC$ and $\#P$ vs. $NC$ problems are analogous.
Though these problems  are not  universal, 
we  assume that the feasibility barrier is 
meaningful for them  because we look at them as  variants
of the $P$ vs. $NP$ problem.

The flip is the defining strategy of GCT. Indeed, GCT may be abstractly
defined as any (geometric) approach to the $P$ vs. $NP$ and related 
problems based on the flip, i.e., explicit construction of obstructions
(for a precise meaning of the phrase geometric see Section~\ref{scharsym}).
The present (concrete) GCT is one such  approach.
\ignore{It proposes  a scheme for implementing the flip for the $P$ 
vs. $NP$ and related problems via algebraic geometry, representation
theory and the theory of quantum groups.
This turns out to be a massive affair, as to be expected, because of the
counterintuitive and paradoxical  nature of the flip as explained above.}




But before we describe how this  GCT crosses the feasibility barrier,
let us explain  
why we are going for the flip, i.e., for explicit constructions,
in the first place.
After all, to solve  the  lower bound problems under consideration
we only need to prove existence of some obstructions, and moreover,
the flip is only the most obvious and natural way to cross
the feasibility barrier. 
(Whenever we say natural in the context of GCT
we always mean explicit unlike in \cite{rudich} where it means probabilistic.) 
There may exist  nonobvious and 
unnatural (e.g. nonconstructive) ways
to cross this barrier, perhaps several.
At present,  we only know 
that one class of nonconstructive techniques 
would not work, namely the ones with probabilistic flavour, which
are ruled out by the natural-(probabilistic)-proof-barrier \cite{rudich}. 
But the probabilistic  proofs constitute  only a 
small subarea of nonconstructive proofs, namely the ones 
which are of a  {\em nonspecific} kind, by which we mean nonconstructive
proofs which apply to most functions or structures under consideration.
Vast areas of
nonconstructive proofs in  mathematics, such as the ones  in algebraic 
geometry and representation theory, are of fundamentally different nature
than probabilistic proofs: they are nonconstructive yet 
{\em very specific};
i.e., they  apply to only very specific functions or structures
under consideration. The natural-(probabilistic)-proof-barrier 
does not apply to
such  nonconstructive but specific proof techniques. 
Indeed, one of the concrete lower bounds of GCT to be discussed below
(Section~\ref{}) has a nonconstructive   proof
which applies to only very specific (permanent-like) functions and which 
crosses  the natural-proof, relativization,
algebraic-degree (algebrization) and feasibility
barriers simultaneously  in a restricted   setting. 
This gives a concrete evidence that
explicit constructions are  not needed to cross these barriers, and that
they may be crossed by nonconstructive proof techniques as well.


But the mathematical evidence and arguments 
in [GCTflip] sugggest that such unnatural ways to cross the feasibility barrier
may not be any easier and perhaps even harder
than  the natural ways as one may intuitively expect. 
For example, the nonconstructive proof of the lower bound mentioned above
is not much different or easier than the explicit proof (and, in fact, 
a bit harder).
We do not go any further into such  arguments  here.
At a concrete level, 
all we can say is that we are going the obvious  way because there 
is no  concrete nonobvious alternative.
After all, any approach to the $P$ vs. $NP$ problem has 
to provide  at least:
\begin{enumerate} 
\item[A] Concrete evidence for its theoretical feasibility; i.e., 
concrete evidence  which says  that the feasibility barrier can be
crossed in that approach. 
\item[B] Concrete 
weaker form  of the $P$ vs. $NP$ problem or any of its two smaller
versions--namely 
the   $P$ vs. $NC$ and the $\#P$ vs. $NC$ problems
(cf. Figure~\ref{fig:complexityclasses})--that  provides
a concrete superpolynomial lower bound
in a realistic and natural model of computation, where by natural and
realistic we mean a model that is actually used extensively in practice and is
not defined for the sake of proving  the lower bound, and
\item[C] Concrete  weaker form  of
any of the separation problems above  whose 
proof  demonstrates that the 
approach  bypasses the earlier 
relativization \cite{solovay}, natural-(probabilistic)-proof {rudich}, 
algebraic degree [GCTlocal], and 
algebrization \cite{aaronson} barriers simultaneously.
\end{enumerate}

We say that an approach is {\em concrete} if it meets the criteria 
A, B and C.

The main result [GCT6] of GCT  (cf. Section~\ref{})  says that
the feasibility barrier can be crossed for the nonuniform
$P$ vs. $NP$ and $\#P$ vs.
$NC$ problems over fields of characteristic zero (as defined below);
[GCT11] says the same for   any
field including the finite field (the usual case). This
addresses (A). The
$P \not = NC$ result without bit operations [GCTlocal] (cf. Section~\ref{})
based on the local flip  addresses (B).
The mathematical form of the $\#P\not = NC$ conjecture [GCT1,2,6] 
(cf. Section~\ref{}) based on the global flip  addresses (C).
Thus one may  say that GCT is a concrete approach to the $P$ vs. $NP$ 
problem.

At present,  there seems to be  no concrete alternative to GCT
which addresses A, B and C. And  this is why we are going for this
most obvious and natural way to cross the feasibility barrier.





Let us now explain what we mean by the (nonuniform) $\#P$ vs. $NC$ and 
$P$ vs. $NP$ problems in characteristic zero. 
The nonuniform (characteristic zero) version of the $\#P$ vs. $NC$ problem
is also known as the permanent vs. determinant problem \cite{valiant}. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented 
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$. %; the best known lower bound on $m$ at present is 
%quadratic \cite{ressayre}.
By linear representation, we mean
the  entries   of $Y$ are  (possibly nonhomogeneous) 
linear functions (over $\C$ or $Z$)
of the entries of $X$. 
There is an analogous characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.
We focus on characteristic zero  because
the nonuniform lower bounds over $Z$ are weaker implications of the
corresponding ones over a finite field (the usual case), and hence
easier. The additional problems that
need to be addressed when the underlying field of computation is finite
will be discussed in  GCT11. 
The main results of GCT for the $\#P$ vs. $NC$ problem in 
characteristic zero also extend to the $P$ vs. $NP$ problem in characteristic
zero. But for the sake of completeness,   we shall mainly
concentrate in this article 
on only the former problem, since it illustrates all the
basic ideas.

We now briefly  describe  the   concrete results of GCT 
which address A, B, and C.

\section{The $P\not = NC$ result without bit operations} \label{swithoutbit}
We  begin with 
a  special case of the $P \not = NC$ conjecture [GCTlocal],
which we are calling the $P\not = NC$ result without bit operations,
and which can be considered to be the
first concrete lower bound result of GCT. It was  proved using the weaker
local form of the flip much before the (global) flip was formalized
in [GCT6,GCTflip].
It  says that 
the $P$-complete max-flow problem
cannot be solved in $\polylog(N)$ parallel time using $\poly(N)$
processors in the PRAM model without bit operations,
where $N$ denotes
the total bit length of the input, not just the number of input parameters.
This model  is quite realistic and natural
since it includes virtually all known parallel algorithms for algebraic 
and weighted optimization problems. Hence, this lower bound meets 
the criterion B.
The proof technique of this result is {\em locally
explicit}, i.e.,  the weaker {\em local} form
of the flip,  in the sense that  for each branching program $C$  (i.e. 
a circuit with arithmetic, branching and comparison operations) 
of depth $\log^a N$ and size $\poly(N)$ (or even 
$2^{\log^a N}$, for some positive constant $a$),
it produces in $\log ^b N$ time using $2^{\log ^b N}$ 
processors, $b=O(a)$, 
an explicit   counter example  $X$ such that the output of $C$
on $X$ is different from what is expected in the maxflow (decision) problem.
This counter example $X$ is then a proof-certificate of hardness (obstruction)
against $C$.
We are calling this kind of explicitness local 
because the obstruction   here is
a short and easily-verifiable  proof 
certificate of hardness against a specific circuit   rather than 
a short and easily-verifiable {\em global obstruction} 
against  the
whole class of circuits of small depth and size, which is far harder to
achieve, and which was what the  (global) flip (described earlier in this
introduction) eventually goes for in the context of the harder 
lower bound problems.

Local explicitness here  may seem counterintuitve at the surface,
since the max-flow problem
is $P$-complete, and hence, it may seem that we may not
even be able to verify if a given $X$ is a counter-example in 
polylogarithmic parallel time. In other words, it may seem that the
$P\not = NC$ conjecture may stand in the way of local explicitness,
just as the $P\not = NP$ conjecture seems to stand in the way
of the step I of the flip.
But local explicitness  is  possible,
because  the proof technique in
GCTlocal produces for a given $C$ an explicit 
counter example $X$ for which 
max-flow can be computed in polylogarithmic time
nevertheless. This  provides a concrete evidence as to why
locally explicit trivial obstructions (Figure~\ref{fig:trivialtonew}) 
should also exist in the context of the $P$ vs. $NP$ problem.
Intuitively, it would specify for a given $C$ of size $m$ 
a counter example $X$ such that $f(X)$ can be evaluated on this specific 
$X$ in $\poly(n,m)$  time in spite of 
$NP$-completeness of $f(X)$ in general ($\poly(n,m)$
is $\poly(n)$ if $m=\poly(n)$).
Thus GCTlocal crosses the  feasibility barrier locally
in the context of the $P\not = NC$ problem without bit operations and 
provides a concrete evidence for the feasibility of 
the  local flip in the context of the fundamental problems of complexity
theory.

\noindent {\em Remark}:
Local explicitness was not  specifically mentioned 
in GCTlocal. But it is easy to see \cite{GCTpramappend}  that 
the proof technique there actually
produces a locally
explicit proof certificate of hardness, after a little postprocessing,
though the goal was only
to prove its existence (which is why explicitness was not mentioned).
In other words, the proof technique essentially produces a locally
explicit proof-certificate of hardness  whether one cares for it or not.


Local explicitness of the proof technique is the fundamental difference between
this lower bound result and the earlier ones, such as 
the lower bounds for constant depth circuits \cite{sipser}, monotone circuits 
\cite{monotone}, or 
algebraic decision trees \cite{benor}, whose proof techniques are inherently 
nonconstructive. For example, the random restriction method \cite{sipser}
for proving lower bounds for  constant depth circuits gives a randomized 
fast parallel algorithm to produce  for each such
circuit $C$ a local counter example $X$ on which it differs from
the parity function. But the best determistic algorithm to produce 
such a counter example, based on  derandomization of the switching
lemma \cite{agarwal},
takes sequential polynomial time. Locally explicit in this
setting would mean computable by a constant depth circuit. Again, at the
surface this may seem counterintuitive, since it may appear that 
even to verify if a given $X$ is a counter example against a given
$C$ may necessarily
require $NC$-computation, given that parity is not in $AC^0$. 
But this should still be possible in view 
of the weak form of the $P\not = NC$ conjecture above. 
Similarly, the proof of the lower bound for sorting in
the  algebraic-decision-tree 
model \cite{benor}  inherently requires
exponential time  to produce a counter example, 
so also the proof of the lower bound for monotone circuits \cite{monotone}.
It may be conjectured that there are
(locally) explicit proofs 
for the constant-depth or  monotone circuit lower bounds. 
At present this is  open. But the main point is that such  explicit 
proofs are not  required to prove these lower bounds,
whereas,
the only way we can prove the weak form of the $P \not = NC$ conjecture
at present is essentially via locally explicit construction. 
In view of the natural proof barrier, it should not be surprising 
that the proof of  $P \not = NC$ result without bit operations  should
require something fundamentally different from the nonconstructive
techniques of the kind used to prove lower bounds for constant depth
circuits, to which this barrier applies,
though, admitedly,  this barrier itself does not suggest that 
we should go for anything explicit (cf. Section~\ref{sexp}).
One may say that 
the proof technique of this result bypasses this barrier
in the sense that such locally explicit construction can be
carried out only for very special problems in $P$ 
such as the max flow problem, though this barrier cannot be
formally defined in the PRAM model without bit operations.
One may also say that the proof technique
bypasses the relativization barrier \cite{rudich}
since it is known that this barrier is not effective against the
proof techniques which algebrize computations.
Thus GCTlocal crosses/bypasses
the local feasibility, natural proof and  relativization
barriers simultaneously in a restricted setting. 






Another  feature of the proof of this lower bound result  is that  it
is based on classical algebraic geometry, though 
the result itself can be stated in purely 
elementary and combinatorial terms.  No elementary or combinatorial 
proof of this result is known so far.
At present,  the $P\not = NC$ result without bit operations seems to be the
only known  special case of any
of the fundamental separation  problems in 
Figure~\ref{fig:complexityclasses} that  holds unconditionally (and 
superpolynomially) in a realistic and 
natural model of computation. That its  proof needs 
geometry and explicit construction   provides  the first
concrete  support for the
geometric approach based on the flip  (explicit construction), i.e. GCT, 
albeit only in the local setting, and
hence, in retrospect, we shall refer to its proof technique as {\em local GCT}.

But the local  GCT turns out to be too weak for going ahead 
for two reasons.
First, GCTlocal (towards the end of its Chapter 7) 
pointed out a barrier (other than the earlier natural-proof
and relativization barriers), which we shall 
refer to  as the {\em algebraic degree barrier}, though it was not
given any name there. This  says that 
any low-degree proof technique, such as the one there,
which associates with a computation algebraic 
objects (polynomials, varieties, etc.) 
and then reasons solely on the basis of the degrees of those 
objects would not work in the context of the fundamental problems 
such as the $P$ vs. $NC$ problem.
The recent  algebrization barrier \cite{aaronson}
also says  something similar, but with different  motivation and framework.
Second, as we already pointed out before, 
the local flip does not seems good enough for the harder separation problems
for the reasons that we do not understand. 


GCTlocal also suggested an idea  for overcoming the
algebraic degree barrier and the locality limitation of local GCT:
namely, associate with complexity classes 
algebraic varieties with group action, as studied in geometric invariant theory
\cite{mumford}, which   intuitively 
capture the symmetries among the  computations in  that class,
and then reason globally on the basis of
the deeper representation theoretic structure of these
varieties, instead of just  their degrees.

\section{Geometric obstructions}
This then was the motivation behind the 
approach to the fundamental lower bound problems via geometric 
invariant theory that was initiated in GCT1 and 2. 


In GCT1, and 2  certain algebraic varieties with group action, 
called the {\em class varieties}, are associated with the fundamental 
complexity classes, and the $\#P$ vs. $NC$ and $P$ vs. $NP$ problems in
characteristic zero are reduced to showing existence of 
certain representation-theoretic {\em obstructions} to embeddings
amongs such varieties. Furthermore, some results in geometric invariant
theory are also proved to justify why such obstructions should exist 
in  the lower bound problems under consideration and
why they should be mathematically well behaved.

GCT 6 conjectures that these  new obstructions are (globally) explict; i.e., 
their specifications are easy to verify and a short obstruction
exists whenever an obstruction exists


\section{A mathematical form of the $\#P\not = NC$ conjecture}
Using  this notion of an obstruction and the geometric-invariant-theoretic
results in GCT1 and 2,  GCT6 (revised version) then proves a second concrete 
lower bound result of GCT, called a  {\em mathematical
weak form of the $\#P$ vs. $NC$ problem} in characteristic zero for the
reasons given below,
and verifies this conjecture in this special case.
This says  that for any generalized permanent of $k$
$n\times n$ variable matrices $X_1,\ldots,X_k$ 
cannot be represented as a polynomial in the traces of monomials in 
$\bar X^j$, $j\ge 0$, where 
$\bar X_i= B X_i C$, for all $i$,  for any (possibly singular) $n\times n$
complex 
matrices $B$ and $C$.
Here by a generalized permanent, we mean a function $p(X_1,\ldots,X_k)$ 
(of any degree not necessarily $n$)
which has exactly the same symmetries as that of the permanent: i.e., such
that for all nonsingular $n\times n$ complex matrices
$U$ and $V$, $p(U X_1 V,\ldots, U X_k V)=p(X_1,\ldots, X_k)$
iff $\perm(U X V)=\perm(X)$. 
It is called a {\em mathematical form} because there is no restriction here
on the complexity of the generalized permanent or the polynomial in traces.
In that sense, unlike the $P\not = NC$ result without bit operations,
this is a mathematical lower bound, rather than a 
complexity theoretic lower bound,  like the one in Galois 
theory which says that any general polynomial of degree greater than five
cannot be solved by any number of radical operations without any restriction
on the number of such operations.
The proof technique of this result 
produces a strongly explicit family $\{O_n\}$ of  (global) obstructions, 
where each $O_n$ has a specification of $O(n)$ size that can verified
and constructed in $O(n)$ time. The obstruction is global in the sense
that it is against all $B$, $C$ and polynomials in traces. 
Thus this result
provides a concrete support for the (global) flip. Its
proof technique  also  bypasses 
the natural-proof, relativization
and algebraic degree (algebrization) barriers 
simultaneously in this setting.


There is also a  nonconstructive 
proof of this result, which also bypasses these 
barriers.
It  is essentially the same as the
explicit proof, except for the last and the easiest step,
which can be carried out nonconstructively. 
Thus the situation here is again similar to the one for the
$P \not =NC$ result without bit operations. That is, the proof is such that 
it essentially (modulo a little postprocessing at the end) 
yields explicit proof certificates whether one cares for them or not.


To summarize the dicussion so far, the 
$P\not =NC$ result without bit operations in GCT is
a complexity theoretic lower bound proved using  a locally explicit  
technique, the mathematical form of the $\#P\not =NC$ conjecture is a 
mathematical lower bound  proved using a globally
explicit technique.
What is needed now to address 
the fundamental separation problems in Figure~\ref{fig:complexityclasses} 
following this line of investigation 
is  a global flip in this  complexity theoretic setting.
This is addressed next in characteristic zero.



\section{On the flip in general in characteristic zero}
The main result of GCT in this context is a conjectural scheme [GCT6,7,8] 
for explicit construction 
of obstructions (i.e. for the implementation of the global flip) 
for the general $\#P$ vs. $NC$ and $P$ vs. $NP$ 
problems in characteristic zero. 
Specifically, GCT6 shows that the feasibility barrier for verification
(and discovery) can be crossed for these problems assumming
a certain positivity hypothesis called PH1 (and its stronger form PH4).
PH1    says that 
certain  representation-theoretic counting  functions
associated with the class  varieties in GCT1 and 2 
have positive $(\#P)$  convex formulae.
By this we mean  positive convex
representations as the number of integer points in  explicitly 
specified polytopes, like the one for the permanent of a $0-1$-matrix 
as the number of integer points in the perfect matching polytope, which
is both positive (since each integer point is counted 
with a positive sign) and convex. 
Furthermore, GCT6,7,and 8   provide an evidence in support of validity
of PH1, and suggest  an approach for proving it via the theory of
nonstandard quantum groups, which are generalizations of
standard quantum groups \cite{drinfeld}. At the heart of this approach,
  lie certain conjectural positivity hypotheses [GCT8] in the theory
of these nonstandard quantum groups, which are  generalizations of the
known positivity results \cite{kazhdan,lusztig} for the standard quantum group.
The only known proofs of these positivity results are based  on the 
Riemann hypothesis over finite fields \cite{weil2}, which is
itself a profound  positivity result in mathematics. 
Thus the proposed scheme for explicit construction of obstructions 
in GCT6,7,8  seems to need  as yet unknown nonstandard
extension of the work surrounding this central positivity theorem,
which encompasses several areas of mathematics, such as algebraic geometry,
representation theory, quantum groups and so forth.

This should not be too surprising, given that 
the difficulty of explicit construction is by now well recognized 
in complexiy theory.
For example, the explicit construction of Ramanujan graphs \cite{sarnak},
which are the best (optimal) expanders,  also 
needs the Riemann hypothesis over finite fields (for curves).
But explicit expanders  cannot be used to prove a lower bound result.
Explicit constructions that yield hard lower bound results are bound
to be  more difficult. Hence, if a nontrivial  extension 
of the work surrounding the Riemann Hypothesis over finite fields 
is needed for explicit constructions in GCT, that is only to be expected.


\ignore{
If explicit construction is thus the root cause of all difficulties in
GCT, one may finally ask: can it not be avoided somehow?
The weak form of the $P\not = NC$ conjecture in GCT meets criterion (A),
and the generalized weak form of
the $\#P \not = NC$ conjecture meets criterion (B). 
These are the weak forms specific only to  this concrete form
of GCT. Other  approaches (GCT or nonGCT) may lead to other
comparable weak forms which are more suitable to them.
But, at present, these are the only such lower bounds that 
we can prove unconditionally in the context of the $P$ vs. $NP$, $P$ vs. $NC$
or $\#P$ vs. $NC$ problems, i.e., in the main testing ground 
shown in Figure~\ref{fig:complexityclasses} 
for  any approach.
And the only  way we can prove them at present 
is esentially (modulo some postprocessing at the end) 
via explicit constructions based on
geometry.  The situation is summarized in Figure~\ref{fig:summary}.
Here it can be
seen that as the circuit lower bounds start moving in the 
direction of the $P$ vs. $NP$ problem, the proof techniques, for some
mysterious reasons, become more and more geometric and explicit.
This sugests that there may be after all something inevitable 
about  geometry and   explicit constructions, 
which is what GCT means.}






\begin{figure} 
\begin{center}
\psfragscanon
\psfrag{pvsnc}{$P\not = NC$}
\psfrag{#pvsnc}{$\#P\not = NC$}
\psfrag{pvsnp}{$P\not = NP$}
\epsfig{file=summary.eps, scale=1}
\end{center}
      \caption{Circuit lower bounds vs. proof techniques}
      \label{fig:summary}
\end{figure} 



The rest of this article is organized in the form of three chapters,
one per  lecture. The first gives a short overview of the basic plan
of GCT for implementing the flip (explicit constructions) in characteristic
zero, which is elaborated in the next two lectures. 






\noindent {\em Acknowledgement:} The author is grateful to 
Avi Wigderson for arranging the lectures and the hospitality in IAS,
and to Janos Simon, Josh Grochow, and Hari Narayanan for 
the help in presentation. 









==> preface5.tex <==
\section*{Introduction} 
Geometric complexity
theory (GCT) is an approach to the  fundamental problems of
complexity theory, such as the (nonuniform) $P$ vs. $NP$
\cite{cook,karp,levin},
$P$ vs. $NC$ and $\#P$ vs. $NC$ \cite{valiant} problems
(Figure~\ref{fig:complexityclasses}). 
In this introduction, we  briefly describe  the main barrier  
towards these problems called the {\em   feasibility
barrier},    the basic strategy of GCT for crossing it called 
the {\em flip} [GCT6,GCTflip],  
a conjectural scheme  [GCT6,7,8,11] for implementation of the flip, 
and two concrete lower bounds of GCT based on weaker forms of the flip: namely
the  $P \not = NC$ result without bit operations [GCTlocal] and
a mathematical  form of the $\#P\not = NC$ conjecture [GCT1,2,6].

The original IAS lectures did not state the first lower bound and
only stated   a special case of the second 
lower bound, called  the weak form of the $\#P$ vs.
$NC$ problem. The article \cite{boris} showed that this weak form 
is too weak; i.e., it can be proved    by an elementary  technique
that  cannot cross the natural-proof barrier \cite{rudich}.
We cannot prove the full mathematical form stated here by such
techniques; cf. Sections~\ref{}, \ref{} and \ref{}. 



\begin{figure} 
\begin{center}
\epsfig{file=complexityclasses.eps, scale=.6}
\end{center}
      \caption{Complexity Classes (no proper containments are known)}
      \label{fig:complexityclasses}
\end{figure} 


The original lectures also did not describe the 
the  feasiblity   barrier.
But all the mathematical effort in   GCT as described in these lectures 
goes towards crossing this barrier.
Hence, we describe  it explicitly here so that the root cause of 
all difficulties encountered in GCT and the need for nonelementary techniques
to overcome this formidable barrier
becomes clear  at a high level before we get into any mathematics. 


\section{The  feasibility barrier} 
The  feasibility barrier is {\em universal} in 
the sense that it has to be crossed by every approach towards the $P$ vs. 
$NP$ problem, not just GCT, regardless of which areas of mathematics it goes
through. In contrast, the other known barriers 
such as the relativization \cite{solovay}, natural-proof \cite{rudich},
algebraic-degree [GCTlocal],  and algebrization  \cite{aaronson} barriers
are {\em local} in the
sense that they are only applicable to specific areas of mathematical
techniques and hence can simply  be bypassed, as in GCT. 
In other words, a local barrier is like a guiding post which tells 
us what must not be done, and hence must  be bypassed,  whereas 
a universal barrier cannot be bypassed no matter what, because it tells us
what must be done, i.e., it has to be crossed.
Due its universality, the feasibility barrier
captures the root cause of all the 
difficulties in the $P$ vs. $NP$ and related  problems, and it turns 
out to quiet formidable, as expected. 

Before we describe it, let us  remark  that the 
presence of such a universal barrier should not be surprising,
because the $P \not = NP$ conjecture    is itself a {\em universal} statement
regarding all of mathematics. Namely, 
if this conjecture fails to hold,
every theorem in mathematics that has a proof of reasonable 
length  can be proved  efficiently by a computer in 
time polynomial in the length of its shortest proof. No other known
conjecture in mathematics has such stunning mathematical sweep. 
Given the universal nature of this problem, it then stands to reason that
the main  barrier towards this problem--the root cause of its 
difficulty--should also be
{\em universal}. The  feasibility barrier is this universal barrier.
Due to its universal nature, it 
cannot be  fully formalized like the local barriers, because any barrier
that can be fully formalized would tend to be local.  But since it is the 
root cause of the difficulty of the $P$ vs. $NP$ problem, 
we wish to  state it as clearly as possible. 

Towards that end,  let us 
fix an appropriate $NP$-complete function $f(X)=f(x_1,\ldots,x_n)$. 
The goal of the nonuniform $P$ vs. $NP$ problem  is to show that 
there does not exist a circuit $C=C(X)$ of size 
$m=\poly(n)$  that computes $f(X)$, $n\rightarrow \infty$. 
Symbolically, let  $f_C(X)$ denote the function computed by $C$. 
Then we want to prove that
\begin{equation} \label{eqiohp}
\forall n, m=\poly(n) \ \forall C \exists x : f(X)\not = f_C(X). 
\end{equation}

Equivalently, the goal is to prove:

\noindent {\bf (IOH)}: For every large enough $n$, and $m=\poly(n)$,
there  exists a {\em trivial obstruction
(i.e. a ``proof-certificate'' of hardness)} to efficient computation of
$f(X)$. Here by a trivial obstruction we mean
a table (cf. Figure~\ref{fig:trivialtonew}) that lists for every small 
$C$  a counterexample  $X$ such that $f(X)\not = f_C(X)$.



The number of rows of this table is equal
to the number of circuits $C$'s of size $m=\poly(n)$.
Thus the size of this table is 
exponential; i.e., $2^{O(\poly(n))}$. 
The time to verify whether a given table is a trivial obstruction
is also exponential,
and so also the time to decide if such a table exists for given $n$ and $m$. 
From the complexity theoretic viewpoint, this is an infeasible 
(inefficient) task. So
we call  this trivial, brute force 
strategy of proving the nonuniform $P$ vs. $NP$ conjecture,
based on existence of trivial obstructions,  a {\em theoretically
infeasible strategy}. Also because
it is really just a restatement of the original problem.
Hence, the terminology  IOH (Infeasible Obstruction Hypothesis)--we also
call it {\em theoretically infeasible}. 


Any approach to the  $P$ vs. $NP$ problem has to 
answer the following question: 

\begin{question} \label{qfeasible} {\bf (Theoretical Feasibility Barrier)} 
[GCTflip,GCT6]
Why should the approach be    feasible (i.e., lead to a proof) 
even theoretically?
That is, in what sense is it fundamentally 
different from the  trivial, infeasible approach above, 
and not just a restatement of the original problem? 
\end{question}

This question is  natural and not new, 
because,  in view of the universality 
of the $P \not =  NP$ conjecture, it has always been questioned right from
the begining  why it
should even be provable. For example,  why can it not be 
independent of the formal axioms of mathematics? This was studied 
in some early works; cf. \cite{aaronsonformal} for their  survey. It 
was also the 
motivation behind identifying  the fundamental 
barriers towards this problem,
such as the relativization \cite{solovay} and natural-proof 
\cite{rudich} barriers.
The latter barrier  roughly says that the proof techniques akin to
the ones used for proving the lower bounds for constant depth circuits
would not work for the $P$ vs. $NP$ problem
in a sense because the problem itself
stands in their way, rendering them theoretically infeasible, so to say.
Admittedly, such proof techniques constitute  only  a very specific 
subarea of mathematics, which is why this  barrier can be considered 
local,  and we cannot conclude anything about the proof techniques
which go through other areas of mathematics on the basis of such a local
barrier (for the reasons explained in more detail in Section~\ref{sexp}).
But one can still wonder if the $P$ vs. $NP$ problem could not
stand in the way of every proof technique like this, rendering it
theoretically infeasible, and thereby precluding its own proof. This
does not seem inconceivable since the problem itself says that the discovery
is hard, and so, why could it not make the discovery of its own proof hard?
Hence arises the question:
why should a given proof technique 
be even theoretically feasible as per some 
reasonable notion of theoretical feasibility. 
The feasibility barrier is simply the task of answering this 
fundamental question, which has been lurking in the background of the $P$ vs.
$NP$ problem right from the begining.
It is universal in the sense that every approach has to answer
Question~\ref{qfeasible}, and
until it is answered clearly,
however sophisticated an approach may be, it cannot be
considered to be more than a  restatement of the original problem.

Now we have specify what is meant by answering
Question~\ref{qfeasible} clearly. Let us assume that the approach
is nonuniform, i.e., it shows existence of some obstruction $O_n$
(the cause
or proof-certificate of hardness as per that approach) for every $n$,
since the relativization barrier \cite{solovay} 
suggests that uniform approaches 
may have a fundamental limitation in the context of the $P$ vs. $NP$ problem.
If there exists a nonrelativizable uniform approach, we
leave the task of answering Question~\ref{qfeasible} to that approach. 
To answer Question~\ref{qfeasible}, 
a nonuniform approach has to:
\begin{description}
\item[A] Come up with a new notion of obstruction, which
is fundamentally different from the trivial obstruction, and thus 
precisely formulate the new Obstruction Hypothesis (OH), which says 
that such obstructions should exist when $m=\poly(n)$, and which provably 
implies the old IOH.

\item [B] Precisely formulate the notion of theoretical feasibility, 
and  justify why it is reasonable notion, i.e., why does a theoretically
feasible problem as per this notion means a problem that can be solved 
by a technique that is fundamentally better than the brute-force search.
\item [C] 
Justify on the basis of  concrete mathematical results 
why the problem (OH) of proving existence of  such obstructions
should  be considered theoretically feasible as per this notion
in contrast to the theoretically infeasible IOH.
One possible way to do this is by justifying why the problem of 
recognizing (verifying) an obstruction is 
theoretically feasible as per this notion. After all,  every 
approach is in a sense a search for obstructions. It is possible 
that the approach may seek 
to prove existence of obstructions by a nonconstructive 
method, without exhibiting any obstruction explicitly. But if it is not
theoretically feasible for the approach to even recognize (verify) 
what is searching for,
then there is a serious problem with the approach.
\item [D] Justify why it is plausible
that the task of proving OH should
become practically feasible once its theoretical feasibility is established.
One possible way is to prove concrete nontrivial lower bounds 
in weaker settings using the approach to demonstrate that theoretical
feasibility can lead to practical feasiblity in nontrivial cases.
\end{description}
By the feasibility barrier, we  mean the task of answering 
Question~\ref{qfeasible} in this manner. 

\section{The flip: going for explicit construction}
The most obvious and natural strategy for crossing the feasibility barrier
is suggested by the $P$ vs. $NP$ problem itself. For that, 
let us see what is wrong with the trivial obstruction from the 
complexity-theoretic point view. That is quite clear. First, it is long,
i.e.,  its description takes exponential space. Second, it is hard to
verify (and also construct); i.e., this  takes exponential time.
Since $NP$ is the class of problems with ``proof-certificates'' that 
are short (of polynomial-size) and easy to verify (in polynomial-time), 
this then leads to the following strategy, called the {\em flip}
[GCT6,GCTflip],
for proving the nonuniform
$P\not = NP$ conjecture, with the obvious complexity-theoretic
interpretation of the phrase theoretically feasible.

\begin{figure} 
\begin{center}
\epsfig{file=trivialtonew.eps, scale=.6}
\end{center}
      \caption{From trivial to new obstruction}
      \label{fig:trivialtonew}
\end{figure} 


\noindent {\bf I. (The flip: theoretical feasibility of verification) :}
Formulate a new notion of obstruction
(``proof-certificate of hardness'') that is {\em explicit}, by which 
we mean {\em short and easy-to-verify}: i.e., 
for any $n$ and $m< 2^n$, if there exists such an 
obstruction to efficient computation of $f(X)$ by circuits of size $m$,
then there also exists a short  obstruction with description of
$\poly(n)$ size bitlength, 
whose validity as an obstruction can be verified 
in $\poly(n)$ time.
This means that the problem of verifying (recognizing)
an obstruction belongs to $P$, 
and hence, is theoretically feasible (``easy'').
Furthemore, the approach should also provide mathematical evidence
to justify  why such  obstructions should exist when $m$ is small.


Intuitively (cf. Figure~\ref{fig:trivialtonew}), we can think of the
new obstruction as an 
encryption of a some trivial obstruction of exponential
size which is highly compressable
in the information theoretic sense--i.e., such that 
its description can be encrypted in polynomial size--and furthermore,
such that the encrypted information can also be verified fast in polynomial
time.
At the surface, it is hard to believe that 
such an obstruction can even exist. To see why, let us note that 
the problem of  verifying 
if a given $X$ is a counterexample to a given $C$ is  intractable since 
it requires evaluating the NP-complete function $f(X)$, which cannot 
be done  efficiently assuming $P \not = NP$, and furthermore
$f_C(X)$ too cannot be evaluated  in polynomial time if the size $m$ of
$C$ is superpolynomial (say $n^{\log n}$). To verify the new obstruction,
in effect, we  are 
{\em implicitly} verifying   all exponentially many  rows of some 
trivial obstruction  in polynomial time (but without 
even knowing what that trivial obstruction is, since the verification 
procedure cannot affort to decrypt the new obstruction to get an exponential
size trivial obstruction).
It may seem that 
such a scheme could not possibly exist and that the $P \not = NP$ conjecture
would again stand in the way either directly or indirectly (implicitly).
Implementation of  this step of the flip
amounts to   showing that
the $P\not = NP$ conjecture
would not stand in the way--which is what crossing the feasibility barrier
essentially means.
Of course, the actual implementation 
does not have to  encrypt any trivial obstructions. The 
new obstruction could be such that its existence implies existence of
some trivial obstruction in a highly indirect way,
without actually telling how to get such a 
trivial obstruction from the new obstruction.
But if it is possble to do so
easily--i.e., if there is a polynomial time {\em decoding algorithm}, which
given a new obstruction and a small $C$ of size $m$ 
produces in $\poly(n,m)$ time a counter example $X$ for 
$C$--then we say that the new obstruction is {\em easy to decode}. 
Though this  is optional, at least at this stage, it may intuitively
help to imagine that the new obstructions are easy to decode.



\noindent {\bf II. (The strong flip: theoretical feasibility of discovery) 
[optional]:} 
Give a $\poly(n)$  time algorithm for deciding,
for any given $n$ and $m< 2^n$,
if there exists such a new  obstruction, and constructing
one if one exists. This means the problem of discovering an obstruction
belongs to $P$, and hence, is theoretically feasible (``easy'').
Again the $P\not = NP$ conjecture seems to stand in the 
way of this step, because the conjecture  says discovery is hard, whereas 
this step says  discovery (of its own proof) is easy. 




\noindent {\bf III. (Practical feasibility):} 
Using the ``easy'' criterion for recognizing an obstruction 
in step I, prove:

\noindent {\bf OH (Obstruction Hypothesis):} If 
$m=\poly(n)$, then for every sufficiently large $n$, there exists 
such a short obstruction $O_n$. 

We call such an obstruction family $\{O_n\}$  {\em explicit}.


If we also have an ``easy'' procedure for discovering an obstruction 
in step II, then this amounts to  proving that this 
procedure always discovers and constructs
an obstruction $O_n$  successfully when $m=\poly(n)$--i.e., the discovery
procedure works correctly (successfully). So this step amount to 
proving correctness of the discovery program.
If it is correct, we 
call such an obstruction family $\{O_n\}$ {\em strongly explicit}.

We  call a proof of the $P\not = NP$ conjecture {\em explicit} if 
it is based on the flip and carries out the step I, and {\em strongly explicit}
if it carries out both steps I and II.




We  say that OH becomes {\em theoretically feasible}, as against
theoretically infeasible IOH, 
once the steps I and II have been carried out, 
since the associated problems of verifying and constructing an obstruction 
then theoretically feasible, i.e., belong to $P$--in other words, 
the theoretically infeasible task of proving IOH is transformed 
into a theoretically feasible task of proving OH.
Hence, the name of this stategy {\em the flip}:
from the infeasible to the feasible. 
We also say that the {\em feasibilty barrier for verification} 
is crossed once step I is carried out, and the {\em feasibility barrier
for discovery} is crossed once step II is carried out, and the 
{\em feasibility barrier is crossed} once both the barriers are 
crossed. We also say that the approach becomes {\em theoretically
feasible} once the feasibility  barrier is crossed.


Of course, theoretical 
feasibility of OH  does not automatically  imply that the task of 
actually proving it would be practically feasible.
For that, it is also necessary
that the algorithms for verifying and discovering an obstruction in
steps I and II have a simple enough structure that can be used for
proving OH in step III; i.e.,  for proving correctness of the discovery 
procedure. If not, they have to made simpler and simpler until
this becomes practically feasible.
Theoretical feasibility of the approach basically
means that the $P\not = NP$ conjecture  no longer stands in the way of the 
approach, and hence, there is no philosophical barrier to 
practical feasibility, though transforming  a theoretically
feasible  approach into a practically feasible approach  can be  a challenging
mathematical problem in itself.

Step II above  has been labelled optional, because
there may exist a  proof of the $P\not = NP$ conjecture
along the  lines of the flip  that  takes substantial
short cuts in this step.
For example,  a proof technique may simply be lucky and come 
up with a right guess for the obstruction family (since it is meant to be
carried out by humans and not machines). 
But substantial short cuts in step I seem difficult. After all, as we have
already said,  if the proof
technique cannot even recognize easily what it is searching for, then
there is  a serious problem.


Here is  another way to look at the flip 
(cf. Figure~\ref{fig:IOHcomplexityintro}). 
For that let us reexamine IOH. 
The problem of deciding,  given $X$ and $C$, if  $\f(X) \not = f_C(X)$
belongs to co-$NP$.
Since there are two alternating layers of quantifiers in (\ref{}),
the problem of verifying it--i.e. the problem of deciding 
if  a trivial obstruction exists for given $n$ and $m$ specified
in unary--belongs to $\Pi_3$. We refer to this as the IOH  decision
problem. When $m=\poly(n)$,  IOH  is expected to be a tautology,  though
we do not know that yet, and hence, the answer to this decision
problem  would then be always yes.
But for general $m$, not just $m=\poly(n)$, it is a hard decision
problem that  lies  high in the complexity hierarchy
(cf. Figure~\ref{fig:IOHcomplexityintro}) and this is another reason for
referring to IOH as theoretically infeasible.
After execution of the step I, the OH decision  problem,
by which we mean the problem of deciding existence of 
a (new) obstruction for given $n$ and $m$ specified in unary,
belongs to $NP$, and after the step II to  $P$.
Once this final $P$-verifiable OH is proved, it is reduced to a tautology
(FOH: Final Obstruction Hypothesis), which can be verified in 
$O(1)$ time. This gives us the final $O(1)$-size proof.
Thus the basic idea of the flip is to systematically 
eliminate the quantifiers in IOH  and reduce the complexity of the
decision problem associated with 
the  obstruction hypothesis until the obstruction hypothesis  is finally
reduced to  an $O(1)$-time verifiable  tautology;
cf. Figure~\ref{fig:IOHcomplexityintro}. 

But this extremely simple strategy is also deeply paradoxical.
Because it may be conjectured that the IOH decision problem in $\Pi_3$ 
above is hard, i.e., does not belong to $\Pi_2$ or $\Sigma_2$.
Though this problem may not be $\Pi_3$-complete, we can still call
it a universal problem, because the $P$ vs. $NP$ problem and 
hence IOH is a universal statement about mathematics. 
So to make the flip work, the approach has to come with a new 
notion of an obstruction so that for $m=\poly(n)$ the new OH is equivalent 
to IOH (both becoming tautologies), and yet the new OH decision problem
should belong to $NP$ for the flip and $P$ for the strong flip. 
Furthermore, the new OH can also be considered to be a universal statement
since it is meant to imply $P \not = NP$.
Assumming that the polynomial time hierarachy does not collapse,
or more specifically, that $\Pi_3 \not = NP \not = P$, reduction
of a universal statement in $\Pi_3$ to another in $NP$ to another in $P$ 
may seem impossible.
That is, as the flip starts moving from IOH towards its final 
destination FOH through the polynomial time hierachy as shown
in Figure~\ref{},  it may seem as if  it may bring about a collapse of this 
hierarchy in its wake  thereby disproving the very conjectures 
it is meant to prove.   So once again we see the self-referential
nature of the  feasiblity barrier, which is saying here 
that the main  barrier towards the $P$ vs. $NP$ problem is the problem itself.






For mathematical problems which are not universal, theoretical feasibility
can be a  meaningless notion. For example, consider 
a trivial  assertion: 

\[ \forall x_1 \ldots x_n  \exists y_1 \ldots y_n: 
\ \sum_i x_i  + \sum_i y_i = \sum y_i + \sum_i x_i.
\]
The problem of brute force verification of this assertion 
belongs to $\Pi_2$, but that is no indication of its difficulty,
and we cannot say that it is a theoretically infeasible hypothesis
like IOH.
Indeed, it is well known
in proof theory that the logical complexity of an assertion, i.e., the
number of alternating quantifiers in it, is in general no index of its
mathematical difficulty. In the context of the $P$ vs. $NP$ problem 
theoretical feasibility of elimination
of the quantifying variables in IOH
is  a fundamental  issue only because of its universality.
For mathematical
problems that are not universal, e.g. the Riemann hypothesis,  practical 
feasibility is all that matters. Because however hard they may be, they do not
say that discovery is hard. 



The flip considered so far  is {\em global} because it is 
based on a global  obstruction of $\poly(n)$ size 
that acts as a proof certificate of hardness for all small
circuits. We may also consider a  {\em local  (strong) flip}
based on a {\em local (strongly) explicit 
obstruction}, by which we mean .
a table specifying a counter example $X$ for each small circuit $C$ of size 
$m$ whose each row can be verified (constructed) in $\poly(n,m)$ time. 
It may be conjectured that the local strong flip is possible in 
the context of the $P$ vs. $NP$ problem: i.e. for
any $NP$-complete $f(X)$, there exists an algorithm that 
produces a counter example $X$ for 
any circuit  $C$ of $m=\poly(n)$ size in $\poly(n,m)=\poly(n)$ time. 
We shall refer to this as the {\em local strong flip conjecture} for
the $P$ vs. $NP$ problem--it is evidently much stronger than the nonuniform
$P\not = NP$ conjecture.
The local flip  crosses the  feasibility 
barrier {\em locally} in the sense that a 
locally  explicit  obstruction is fundamentally different and better 
than a trivial obstruction. Better locally but not  globally
because  verification 
of the whole locally   explicit obstruction still
takes exponential time. Similarly for a local strongly explicit obstruction.
The global   flip is intuitively stronger than the local  flip in
the sense that from a  global  obstruction one can get 
a local   explicit  obstruction once we have 
a polynomial time decoding algorithm (as we are intuitively imagining)
and  the $P\not = NP$ conjecture does 
not stand in the way of this decoding.
Hence intuively the global (strong) flip subsumes the local (strong) flip.












The feasibility barrier and the flip for other problems such as 
the $P$ vs. $NC$ and $\#P$ vs. $NC$ problems are analogous.
Though these problems  are not  universal, 
we  assume that the feasibility barrier is 
meaningful for them  because we look at them as  variants
of the $P$ vs. $NP$ problem.

The flip is the defining strategy of GCT. Indeed, GCT may be abstractly
defined as any (geometric) approach to the $P$ vs. $NP$ and related 
problems based on the flip, i.e., explicit construction of obstructions
(for a precise meaning of the phrase geometric see Section~\ref{scharsym}).
By based on the flip, we mean it uses the flip as a basic guiding principle
and goes for ``more or less'' explicit construction of obstructions, 
though it does not have to be completely explicit, i.e., 
some deviations and short cuts in steps I and II are fine as long as 
their spirit  is maintained.
The present (concrete) GCT is one such  approach.
It proposes  a scheme for implementing the flip for the $P$ 
vs. $NP$ and related problems via algebraic geometry, representation
theory and the theory of quantum groups.
This turns out to be a nontrivial affair, as to be expected, because of the
counterintuitive and paradoxical  nature of the flip as explained above.




But before we enter into it, let us 
ask ourselves if the flip, i.e.,  explicit construction, the root 
cause of all difficulties in GCT, is really necessary.
Because, to solve  the  lower bound problems under consideration
we only need to prove existence of obstructions, we do not have to
construct them,  and moreover,
the flip also has the following disturbing   feature.
Namely,  proving a superpolynomial 
lower bound for $f(X)$  via the flip 
is not very different from proving a superlinear 
lower bound, because the
heart of the flip, consisting of the steps I and II, is the same whether
$m$ is superpolynomial or superlinear, and only the final step III differs.
In other words, as per the flip,  modest as well as  strong lower bounds
lie on the other side of the feasibility barrier, and 
the main difficulty in getting to them--the feasibility barrier 
(steps I and II)--is the same.
One may wonder if there is any other gradual way towards the $P$ vs. $NP$
problem on which
we could meet  modest lower bounds much before strong lower bounds without
having to cross  the formidable feasibility barrier first.

After all the flip is only the most obvious and natural way to cross
the feasibility barrier. 
(Whenever we say natural in the context of GCT
we always mean explicit unlike in \cite{rudich} where it means probabilistic.) 
There may exist  nonobvious and 
unnatural (e.g. nonconstructive) ways to cross this barrier.
At present,  we only know 
that one class of nonconstructive techniques 
would not work, namely the ones with probabilistic flavour, which
are ruled out by the natural-(probabilistic)-proof-barrier \cite{rudich}. 
But the probabilistic  proofs constitute  only a 
small subarea of nonconstructive proofs, namely the ones 
which are of a  {\em nonspecific} kind, by which we mean nonconstructive
proofs which apply to most functions or structures under consideration.
Vast areas of
nonconstructive proofs in  mathematics, such as the ones  in algebraic 
geometry and representation theory, are of fundamentally different nature
than probabilistic proofs: they are nonconstructive yet 
{\em very specific};
i.e., they  apply to only very specific functions or structures
under consideration. The natural-(probabilistic)-proof-barrier 
does not apply to
such  nonconstructive but specific proof techniques. 
Indeed, one of the concrete lower bounds of GCT to be discussed below
(Section~\ref{}) has a nonconstructive   proof
which applies to only very specific (permanent-like) functions and which 
crosses  the natural-proof, relativization,
algebraic-degree (algebrization) and feasibility
barriers simultaneously  in a restricted   setting. 
This gives a concrete evidence that
explicit constructions are  not needed to cross these barriers, and that
they may be crossed by nonconstructive proof techniques as well.


But the mathematical evidence and arguments 
in [GCTflip] sugggest that such unnatural ways to cross the feasibility barrier
may not be any easier and perhaps even harder
than  the natural ways as one may intuitively expect. 
For example, the nonconstructive proof of the lower bound mentioned above
is not much different or easier than the explicit proof (and, in fact, 
a bit harder).
We do not go any further into such  arguments  here.
At a concrete level, 
all we can say is that we are going the natural  way because there 
is no  concrete  alternative.
After all, any approach to the $P$ vs. $NP$ problem has 
to provide  at least:
\begin{enumerate} 
\item[A] A concrete superpolynomial lower bound that  is a 
restricted form  of any of the fundamental separation problems 
in Figure~\ref{} 
(the center of complexity theory)
in a realistic and natural model of computation, where by natural and
realistic we mean a model that is actually used extensively in practice and is
not defined for the sake of proving  the lower bound, 
\item[B] A concrete  restricted  form  of
any of these separation problems   whose 
proof  demonstrates that the 
approach  bypasses the earlier 
relativization \cite{solovay}, natural-(probabilistic)-proof {rudich}, 
algebraic degree [GCTlocal], and 
algebrization \cite{aaronson} barriers simultaneously,
\item[C] A concrete programme to cross the feasibility barrier justified 
by  concrete mathematical results.
\end{enumerate}

We shall refer to these as criteria A, B, and C to evaluate any approach.

The $P \not = NC$ result without bit operations [GCTlocal] in GCT
(cf. Section~\ref{}) addresses (A).
The mathematical form of the $\#P\not = NC$ conjecture [GCT1,2,6] 
(cf. Section~\ref{})   addresses (B).
(These  lower bounds in restricted models  are easier than the modest 
lower bounds  in unrestricted models that  we mentioned above). 
The main result [GCT6] of GCT  (cf. Section~\ref{})  gives a conjectural
scheme supported by mathematical evidence to cross the feasibility barrier
via the flip for  the nonuniform
$P$ vs. $NP$ and $\#P$ vs.
$NC$ problems over fields of characteristic zero (as defined below);
[GCT11] does  the same for   any
field including the finite field (the usual case). This
addresses (C). 




At present,  we do not have any  concrete   alternative to GCT
which addresses A, B and C, or for that matter any one of them,
and hence  there is not much that we  can
do but follow  the most natural direction, as we are doing here.

Let us now explain what we mean by the (nonuniform) $\#P$ vs. $NC$ and 
$P$ vs. $NP$ problems in characteristic zero. 
The nonuniform (characteristic zero) version of the $\#P$ vs. $NC$ problem
is also known as the permanent vs. determinant problem \cite{valiant}. 
It  is to show that $\perm(X)$, the permanent of an $n\times n$ variable 
matrix $X$, cannot be represented 
linearly  as $\det(Y)$, the determinant of 
an $m\times m$ matrix $Y$,
if $m=\poly(n)$, or more generally, $m=2^{\log^a n}$, 
for a fixed constant $a>0$, 
and $n\rightarrow \infty$. %; the best known lower bound on $m$ at present is 
%quadratic \cite{ressayre}.
By linear representation, we mean
the  entries   of $Y$ are  (possibly nonhomogeneous) 
linear functions (over $\C$ or $Z$)
of the entries of $X$. 
There is an analogous characteristic zero version of
the $P$ vs. $NP$ problem defined in GCT1, where the role of
the permanent is played by an appropriate (co)-NP complete function and
the role of the determinant is played by an appropriate $P$-complete function.
We focus on characteristic zero  because
the nonuniform lower bounds over $Z$ are weaker implications of the
corresponding ones over a finite field (the usual case), and hence
easier. The additional problems that
need to be addressed when the underlying field of computation is finite
will be discussed in  GCT11. 
The main results of GCT for the $\#P$ vs. $NC$ problem in 
characteristic zero also extend to the $P$ vs. $NP$ problem in characteristic
zero. But for the sake of completeness,   we shall mainly
concentrate in this article 
on only the former problem, since it illustrates all the
basic ideas.

We now briefly  describe  the   concrete results of GCT 
which address A, B, and C.

\section{A: The $P\not = NC$ result without bit operations} \label{swithoutbit}
We  begin with 
a  special case of the $P \not = NC$ conjecture [GCTlocal],
which we are calling the $P\not = NC$ result without bit operations,
and which can be considered to be the
first concrete lower bound result of GCT. It was  proved using the weaker
local form of the flip much before the (global) flip was formalized
in [GCT6,GCTflip].
It  says that 
the $P$-complete max-flow problem
cannot be solved in $\polylog(N)$ parallel time using $\poly(N)$
processors in the PRAM model without bit operations,
where $N$ denotes
the total bit length of the input, not just the number of input parameters.
This model  is quite realistic and natural
since it includes virtually all known parallel algorithms for algebraic 
and weighted optimization problems. Hence, this lower bound meets 
the criterion B.
The proof technique of this result is {\em locally
explicit}, i.e.,  the weaker {\em local} form
of the flip,  in the sense that  for each branching program $C$  (i.e. 
a circuit with arithmetic, branching and comparison operations) 
of depth $\log^a N$ and size $\poly(N)$ (or even 
$2^{\log^a N}$, for some positive constant $a$),
it produces in $\log ^b N$ time using $2^{\log ^b N}$ 
processors, $b=O(a)$, 
an explicit   counter example  $X$ such that the output of $C$
on $X$ is different from what is expected in the maxflow (decision) problem.
This counter example $X$ is then a proof-certificate of hardness (obstruction)
against $C$.
We are calling this kind of explicitness local 
because the obstruction   here is
a short and easily-verifiable  proof 
certificate of hardness against a specific circuit   rather than 
a short and easily-verifiable {\em global obstruction} 
against  the
whole class of circuits of small depth and size, which is far harder to
achieve, and which was what the  (global) flip (described earlier in this
introduction) eventually goes for in the context of the harder 
lower bound problems.

Local explicitness here  may seem counterintuitve at the surface,
since the max-flow problem
is $P$-complete, and hence, it may seem that we may not
even be able to verify if a given $X$ is a counter-example in 
polylogarithmic parallel time. In other words, it may seem that the
$P\not = NC$ conjecture may stand in the way of local explicitness,
just as the $P\not = NP$ conjecture seems to stand in the way
of the step I of the flip.
But local explicitness  is  possible,
because  the proof technique in
GCTlocal produces for a given $C$ an explicit 
counter example $X$ for which 
max-flow can be computed in polylogarithmic time
nevertheless. This  provides a concrete evidence as to why
locally explicit trivial obstructions (Figure~\ref{fig:trivialtonew}) 
should also exist in the context of the $P$ vs. $NP$ problem.
Intuitively, it would specify for a given $C$ of size $m$ 
a counter example $X$ such that $f(X)$ can be evaluated on this specific 
$X$ in $\poly(n,m)$  time in spite of 
$NP$-completeness of $f(X)$ in general ($\poly(n,m)$
is $\poly(n)$ if $m=\poly(n)$).
Thus GCTlocal crosses the  feasibility barrier locally
in the context of the $P\not = NC$ problem without bit operations and 
provides a concrete evidence for the feasibility of 
the  local flip in the context of the fundamental problems of complexity
theory.

\noindent {\em Remark}:
Local explicitness was not  specifically mentioned 
in GCTlocal. But it is easy to see \cite{GCTpramappend}  that 
the proof technique there actually
produces a locally
explicit proof certificate of hardness, after a little postprocessing,
though the goal was only
to prove its existence (which is why explicitness was not mentioned).
In other words, the proof technique essentially produces a locally
explicit proof-certificate of hardness  whether one cares for it or not.


Local explicitness of the proof technique is the fundamental difference between
this lower bound result and the earlier ones, such as 
the lower bounds for constant depth circuits \cite{sipser}, monotone circuits 
\cite{monotone}, or 
algebraic decision trees \cite{benor}, whose proof techniques are inherently 
nonconstructive. For example, the random restriction method \cite{sipser}
for proving lower bounds for  constant depth circuits gives a randomized 
fast parallel algorithm to produce  for each such
circuit $C$ a local counter example $X$ on which it differs from
the parity function. But the best determistic algorithm to produce 
such a counter example, based on  derandomization of the switching
lemma \cite{agarwal},
takes sequential polynomial time. Locally explicit in this
setting would mean computable by a constant depth circuit. Again, at the
surface this may seem counterintuitive, since it may appear that 
even to verify if a given $X$ is a counter example against a given
$C$ may necessarily
require $NC$-computation, given that parity is not in $AC^0$. 
But this should still be possible in view 
of the weak form of the $P\not = NC$ conjecture above. 
Similarly, the proof of the lower bound for sorting in
the  algebraic-decision-tree 
model \cite{benor}  inherently requires
exponential time  to produce a counter example, 
so also the proof of the lower bound for monotone circuits \cite{monotone}.
It may be conjectured that there are
(locally) explicit proofs 
for the constant-depth or  monotone circuit lower bounds. 
At present this is  open. But the main point is that such  explicit 
proofs are not  required to prove these lower bounds,
whereas,
the only way we can prove the weak form of the $P \not = NC$ conjecture
at present is essentially via locally explicit construction. 
In view of the natural proof barrier, it should not be surprising 
that the proof of  $P \not = NC$ result without bit operations  should
require something fundamentally different from the nonconstructive
techniques of the kind used to prove lower bounds for constant depth
circuits, to which this barrier applies,
though, admitedly,  this barrier itself does not suggest that 
we should go for anything explicit (cf. Section~\ref{sexp}).
One may say that 
the proof technique of this result bypasses this barrier
in the sense that such locally explicit construction can be
carried out only for very special problems in $P$ 
such as the max flow problem, though this barrier cannot be
formally defined in the PRAM model without bit operations.
One may also say that the proof technique
bypasses the relativization barrier \cite{rudich}
since it is known that this barrier is not effective against the
proof techniques which algebrize computations.
Thus GCTlocal crosses/bypasses
the local feasibility, natural proof and  relativization
barriers simultaneously in a restricted setting. 






Another  feature of the proof of this lower bound result  is that  it
is based on classical algebraic geometry, though 
the result itself can be stated in purely 
elementary and combinatorial terms.  No elementary or combinatorial 
proof of this result is known so far.
At present,  the $P\not = NC$ result without bit operations seems to be the
only known  special case of any
of the fundamental separation  problems in 
Figure~\ref{fig:complexityclasses} that  holds unconditionally (and 
superpolynomially) in a realistic and 
natural model of computation. That its  proof needs 
geometry and explicit construction   provides  the first
concrete  support for the
geometric approach based on the flip  (explicit construction), i.e. GCT, 
albeit only in the local setting, and
hence, in retrospect, we shall refer to its proof technique as {\em local GCT}.

But the local  GCT turns out to be too weak for going ahead 
for two reasons.
First, GCTlocal (towards the end of its Chapter 7) 
pointed out a barrier (other than the earlier natural-proof
and relativization barriers), which we shall 
refer to  as the {\em algebraic degree barrier}, though it was not
given any name there. This  says that 
any low-degree proof technique, such as the one there,
which associates with a computation algebraic 
objects (polynomials, varieties, etc.) 
and then reasons solely on the basis of the degrees of those 
objects would not work in the context of the fundamental problems 
such as the $P$ vs. $NC$ problem.
The recent  algebrization barrier \cite{aaronson}
also says  something similar, but with different  motivation and framework.
Second, as we already pointed out before, 
the local flip does not seems good enough for the harder separation problems
for the reasons that we do not understand. 


GCTlocal also suggested an idea  for overcoming the
algebraic degree barrier and the locality limitation of local GCT:
namely, associate with complexity classes 
algebraic varieties with group action, as studied in geometric invariant theory
\cite{mumford}, which   intuitively 
capture the symmetries among the  computations in  that class,
and then reason globally on the basis of
the deeper representation theoretic structure of these
varieties, instead of just  their degrees.

\section{Geometric obstructions}
This then was the motivation behind the 
approach to the fundamental lower bound problems via geometric 
invariant theory that was initiated in GCT1 and 2. 


In GCT1, and 2  certain algebraic varieties with group action, 
called the {\em class varieties}, are associated with the fundamental 
complexity classes, and the $\#P$ vs. $NC$ and $P$ vs. $NP$ problems in
characteristic zero are reduced to showing existence of 
certain representation-theoretic {\em obstructions} to embeddings
amongs such varieties. Furthermore, some results in geometric invariant
theory are also proved to justify why such obstructions should exist 
in  the lower bound problems under consideration and
why they should be mathematically well behaved.

GCT 6 conjectures that these  new obstructions are (globally) explict; i.e., 
their specifications are easy to verify and a short obstruction
exists whenever an obstruction exists


\section{A mathematical form of the $\#P\not = NC$ conjecture}
Using  this notion of an obstruction and the geometric-invariant-theoretic
results in GCT1 and 2,  GCT6 (revised version) then proves a second concrete 
lower bound result of GCT, called a  {\em mathematical
weak form of the $\#P$ vs. $NC$ problem} in characteristic zero for the
reasons given below,
and verifies this conjecture in this special case.
This says  that for any generalized permanent of $k$
$n\times n$ variable matrices $X_1,\ldots,X_k$ 
cannot be represented as a polynomial in the traces of monomials in 
$\bar X^j$, $j\ge 0$, where 
$\bar X_i= B X_i C$, for all $i$,  for any (possibly singular) $n\times n$
complex 
matrices $B$ and $C$.
Here by a generalized permanent, we mean a function $p(X_1,\ldots,X_k)$ 
(of any degree not necessarily $n$)
which has exactly the same symmetries as that of the permanent: i.e., such
that for all nonsingular $n\times n$ complex matrices
$U$ and $V$, $p(U X_1 V,\ldots, U X_k V)=p(X_1,\ldots, X_k)$
iff $\perm(U X V)=\perm(X)$. 
It is called a {\em mathematical form} because there is no restriction here
on the complexity of the generalized permanent or the polynomial in traces.
In that sense, unlike the $P\not = NC$ result without bit operations,
this is a mathematical lower bound, rather than a 
complexity theoretic lower bound,  like the one in Galois 
theory which says that any general polynomial of degree greater than five
cannot be solved by any number of radical operations without any restriction
on the number of such operations.
The proof technique of this result 
produces a strongly explicit family $\{O_n\}$ of  (global) obstructions, 
where each $O_n$ has a specification of $O(n)$ size that can verified
and constructed in $O(n)$ time. The obstruction is global in the sense
that it is against all $B$, $C$ and polynomials in traces. 
Thus this result
provides a concrete support for the (global) flip. Its
proof technique  also  bypasses 
the natural-proof, relativization
and algebraic degree (algebrization) barriers 
simultaneously in this setting.


There is also a  nonconstructive 
proof of this result, which also bypasses these 
barriers.
It  is essentially the same as the
explicit proof, except for the last and the easiest step,
which can be carried out nonconstructively. 
Thus the situation here is again similar to the one for the
$P \not =NC$ result without bit operations. That is, the proof is such that 
it essentially (modulo a little postprocessing at the end) 
yields explicit proof certificates whether one cares for them or not.


To summarize the dicussion so far, the 
$P\not =NC$ result without bit operations in GCT is
a complexity theoretic lower bound proved using  a locally explicit  
technique, the mathematical form of the $\#P\not =NC$ conjecture is a 
mathematical lower bound  proved using a globally
explicit technique.
What is needed now to address 
the fundamental separation problems in Figure~\ref{fig:complexityclasses} 
following this line of investigation 
is  a global flip in this  complexity theoretic setting.
This is addressed next in characteristic zero.



\section{On the flip in general in characteristic zero}
The main result of GCT in this context is a conjectural scheme [GCT6,7,8] 
for explicit construction 
of obstructions (i.e. for the implementation of the global flip) 
for the general $\#P$ vs. $NC$ and $P$ vs. $NP$ 
problems in characteristic zero. 
Specifically, GCT6 shows that the feasibility barrier for verification
(and discovery) can be crossed for these problems assumming
a certain positivity hypothesis called PH1 (and its stronger form PH4).
PH1    says that 
certain  representation-theoretic counting  functions
associated with the class  varieties in GCT1 and 2 
have positive $(\#P)$  convex formulae.
By this we mean  positive convex
representations as the number of integer points in  explicitly 
specified polytopes, like the one for the permanent of a $0-1$-matrix 
as the number of integer points in the perfect matching polytope, which
is both positive (since each integer point is counted 
with a positive sign) and convex. 
Furthermore, GCT6,7,and 8   provide an evidence in support of validity
of PH1, and suggest  an approach for proving it via the theory of
nonstandard quantum groups, which are generalizations of
standard quantum groups \cite{drinfeld}. At the heart of this approach,
  lie certain conjectural positivity hypotheses [GCT8] in the theory
of these nonstandard quantum groups, which are  generalizations of the
known positivity results \cite{kazhdan,lusztig} for the standard quantum group.
The only known proofs of these positivity results are based  on the 
Riemann hypothesis over finite fields \cite{weil2}, which is
itself a profound  positivity result in mathematics. 
Thus the proposed scheme for explicit construction of obstructions 
in GCT6,7,8  seems to need  as yet unknown nonstandard
extension of the work surrounding this central positivity theorem,
which encompasses several areas of mathematics, such as algebraic geometry,
representation theory, quantum groups and so forth.

This should not be too surprising, given that 
the difficulty of explicit construction is by now well recognized 
in complexiy theory.
For example, the explicit construction of Ramanujan graphs \cite{sarnak},
which are the best (optimal) expanders,  also 
needs the Riemann hypothesis over finite fields (for curves).
But explicit expanders  cannot be used to prove a lower bound result.
Explicit constructions that yield hard lower bound results are bound
to be  more difficult. Hence, if a nontrivial  extension 
of the work surrounding the Riemann Hypothesis over finite fields 
is needed for explicit constructions in GCT, that is only to be expected.


\ignore{
If explicit construction is thus the root cause of all difficulties in
GCT, one may finally ask: can it not be avoided somehow?
The weak form of the $P\not = NC$ conjecture in GCT meets criterion (A),
and the generalized weak form of
the $\#P \not = NC$ conjecture meets criterion (B). 
These are the weak forms specific only to  this concrete form
of GCT. Other  approaches (GCT or nonGCT) may lead to other
comparable weak forms which are more suitable to them.
But, at present, these are the only such lower bounds that 
we can prove unconditionally in the context of the $P$ vs. $NP$, $P$ vs. $NC$
or $\#P$ vs. $NC$ problems, i.e., in the main testing ground 
shown in Figure~\ref{fig:complexityclasses} 
for  any approach.
And the only  way we can prove them at present 
is esentially (modulo some postprocessing at the end) 
via explicit constructions based on
geometry.  The situation is summarized in Figure~\ref{fig:summary}.
Here it can be
seen that as the circuit lower bounds start moving in the 
direction of the $P$ vs. $NP$ problem, the proof techniques, for some
mysterious reasons, become more and more geometric and explicit.
This sugests that there may be after all something inevitable 
about  geometry and   explicit constructions, 
which is what GCT means.}






\begin{figure} 
\begin{center}
\psfragscanon
\psfrag{pvsnc}{$P\not = NC$}
\psfrag{#pvsnc}{$\#P\not = NC$}
\psfrag{pvsnp}{$P\not = NP$}
\epsfig{file=summary.eps, scale=1}
\end{center}
      \caption{Circuit lower bounds vs. proof techniques}
      \label{fig:summary}
\end{figure} 



The rest of this article is organized in the form of three chapters,
one per  lecture. The first gives a short overview of the basic plan
of GCT for implementing the flip (explicit constructions) in characteristic
zero, which is elaborated in the next two lectures. 






\noindent {\em Acknowledgement:} The author is grateful to 
Avi Wigderson for arranging the lectures and the hospitality in IAS,
and to Janos Simon, Josh Grochow, and Hari Narayanan for 
the help in presentation. 









==> weak.tex <==
\section{Weak form of the (generalized) $\#P$ vs. $NC$ problem} 
We will also illustrate the GCT approach by applying it to prove a concrete 
lower bound result --namely a weak of form of the (generalized) 
$\#P$ vs. $NC$ problem. 
To begin with:

\begin{prop}  \label{pweak}
Then there do not exist (possibly singular) $n\times n$ complex
matrices $B$ and $C$  and a polynomial 
$e(w_0,\ldots, w_n)$ such that $\perm(X) = g(BXC)$, 
where $g(X)=e(\trace(X^0), \trace(X), \ldots, \trace(X^n))$. 
\end{prop}
This was referred to as 
the weak form of the $\#P$ vs. $NC$ problem in the original lecture. 
It has a surprisingly simple elementary proof \cite{}. But the 
proof is naturalizable in the terminology of \cite{}--i.e. does not
cross the natural-proof barrier therein--because it works for 
most functions in place of the permanent. The proof technique of
the quadratic lower bound \cite{} for the permanent is also naturalizable.
Hence, the  first goal in this context 
is to prove some weaker form of the $\#P \not = NC$ conjecture (nonuniform)
which cannot be proved by naturalizable proof techniques. 

We shall now describe such a weaker form. 
For that we need a definition.
A function $p(X)$ is called a {\em generalized permanent} if it has exactly 
the same symmetries as that of the permanent; i.e.,
for all nonsingular $n\times n$ matrices $U$ and $V$, 
\[ p(U X V)=p(X) \mbox{\ iff\ } \perm(U X V)=\perm (X).\] 
For a precise description of the symmetries of the permanent,
see Section~\ref{} (basically $U$ and $V$ above have to be permutation
or diagonal matrices (with product of the diagonal entries one), or 
product of such matrices.) 
It may be conjectured that any generalized permanent of $\poly(n)$ 
degree cannot be linearly represented in terms of the determinant 
of a matrix of $\poly(n)$ dimension--we shall refer to this as 
the generalized $\#P$ vs. $NC$ problem. It may be conjectured 
that the space of of generalized permanents has a $\#P$-basis, by which
we mean a basis  whose 
elements represent $P^{\#P$-computable functions.
Hence, this is essentially (and conjecturally) 
equivalent to the original conjecture (though a bit stronger).
The following is its weaker form:

\begin{theorem}[The weak form of the generalized $\#P$ vs. $NC$ problem]
Let $p(X)$ be any nonzero generalized permanent function.
Then there do not exist (possibly singular) $n\times n$ complex
matrices $B$ and $C$  and a polynomial 
$e(w_0,\ldots, w_n)$ such that $p(X) = g(BXC)$, 
where $g(X)=e(\trace(X^0), \trace(X), \ldots, \trace(X^n))$. 
\end{theorem}

The only thing that is common to all generalized permanents is that
they have the same symmetries. Hence any proof of this result can
rely only on these symmetries, and thus is essentially forced to
cross the natural-proof barrier, since most functions have no symmetries.
The classical relativization barrier is also automatically bypassed 
in this problem (and also in the original permanent vs. determinant problem)
because of its algbraic nature. So also 
the algebraic-degree [GCTweak] (algebrization
\cite{}) barrier, since 
$p(X)$ and $g(X)$ (like the 
permanent and the determinant)  have the same degree, 
and hence, (low) degree-based 
techniques would not work either.  Thus, the main significance 
of this result from the complexity-theoretic view point is that 
it cannot be proved by relativizable, low-degree, or naturalizable 
proof techniques, i.e. any proof of this result
is essentially forced to bypass all the 
earlier known barriers--namely, relativization, natural-proof, and
algebraic-degree/algebrization. In particular, it illustrates that
GCT bypasses all these barriers simultaneously.


But we are still referring to it as weak because it is a mathematical
lower bound rather than a complexity theoretic lower bound in the sense
that there is no restriction on the computational complexity of the 
polynomial $e(w_0, \ldots, w_n)$ in this result. If $e(w_0,\ldots,w_n)$
were $NC$-computable, then so would be $g(X)$ and $g(BXC)$, since traces are 
$NC$-computable. But the result does not require this. In that sense,
it is rather in the spirit of the classical result of Galois theory 
which says that a general prolynomial cannot be solved by any number of
radical operations, without any restriction on the number of radical
operations.

Though the statement of this result is elementary, its proof is nonelementary.
This is to be expected, since the generalized permanents are highly nontrivial
and mathematically formidable objects. Specifically, the problem
of finding a $\#P$-basis for the space of generalized permanents 
is intimately related to some formidable problems of representation
theory and algebraic geometry,
and the far simpler anlogues of this problem 
which can be solved at present (e.g. \cite{}) 
all require the deep Riemann Hypothesis over finite fields \cite{} for their 
proofs; cf. Section~\ref{}.
The proof of Theorem~\ref{} proceeds at an abstract level 
through algebraic geometry and representation theory without
having to know anything about such a basis.
At present, it is open if there is any alternative 
weaker form of the $\#P \not = NC$  conjecture,
which cannot be proved by relativizable, low-degree or 
naturalizable  techniques, but which can still be proved by elementary 
or not so  nonelementary techniques; that is, whether the earlier known
barriers mentioned above can 
be simultaneously bypassed in an elementary way in the context of 
the $\#P$ vs. $NC$ (or $P$ vs. $NC$  or $P$ vs. $NP$) problem.













